Extremely Low Bit Transformer Quantization for On-Device Neural Machine Translation

The deployment of widely used Transformer architecture is challenging because of heavy computation load and memory overhead during inference, especially when the target device is limited in computational resources such as mobile or edge devices. Quantization is an effective technique to address such challenges. Our analysis shows that for a given number of quantization bits, each block of Transformer contributes to translation quality and inference computations in different manners. Moreover, even inside an embedding block, each word presents vastly different contributions. Correspondingly, we propose a mixed precision quantization strategy to represent Transformer weights by an extremely low number of bits (e.g., under 3 bits). For example, for each word in an embedding block, we assign different quantization bits based on statistical property. Our quantized Transformer model achieves 11.8$\times$ smaller model size than the baseline model, with less than -0.5 BLEU. We achieve 8.3$\times$ reduction in run-time memory footprints and 3.5$\times$ speed up (Galaxy N10+) such that our proposed compression strategy enables efficient implementation for on-device NMT.

==> emnlp2020_rebuttal_guideline.tex <==
<emnlp2020 Response to the reviews Guideline>
If you choose to respond to the reviews:
  * Remember that reviewing is double-blind.
  * Do not include any information in the response that can identify you or your co-authors.
  * Do not include any URLs in your response.
  * Use the response judiciously. If a reviewer has expressed uncertainty about an issue, or is making an incorrect assumption, or has misunderstood a point in the paper, please address these concerns in your author response.
  * There is no need to respond to every minor question or suggestion for improvement.
  * In interpreting your review, and the numerical scores, please refer to the review instructions at https://2020.emnlp.org/blog/2020-05-26-instructions-for-reviewers/.
  * You are requested not to use the response form to debate the reviewers’ subjective opinions regarding the merit of your work. Nor should you try to “correct” your paper in any way - either in terms of its basic technical arguments, or in the presentation of those arguments. Above all, the response facility should not be used to report on new results, obtained after the submission deadline.
  * This process is intended to help produce more accurate reviews for your paper. It is not intended to strengthen the arguments in your paper.

If the paper is accepted, you will still have ample opportunity to make
revisions, i.e., before submitting your camera-ready copy.

Responses must be no more than 900 words in total, counting the text boxes for responding to each reviewer, and the general response box. Comments to the chair do not count towards this word count.

Each submission should have at least three reviews. If your paper has fewer than three reviews, please be assured that our senior program committee is working hard to chase the missing reviews. So please check back at a later point.




==> figures/emb_quant.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/emb_quant.eps}
    \caption{Illustration for Algorithm \ref{alg:embedding} where $b{=}4,r{=}2$.}
    \label{fig:emb-quant}
\end{figure}

==> figures/embed_retrain_quant.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/embed_retrain.png}
    \caption{\label{fig:embed-retrain}Detokenized-BLEU (beam=1, newstest2013, \texttt{sacrebleu}) after applying quantization to embedding layer with proposed mixed precision quantization strategy without retraining. Refer to Section \ref{sec:results} for results with retraining.}
\end{figure}

==> tables/qualitiative_analysis/deen_inputs.tex <==
Die Korruption wucherte hemmungslos, und das Volk ging mit bereits gekauften Stimmen zur Wahl" ... "Menschen mit Charakter bewarben sich nicht f\xfcr \xc4mter, so dass der Staat infolge dieses Niedergangs acht Monate lang keinen Konsul hatte" ... "Man begann schon wirklich dar\xfcber zu sprechen, dass die einzige Medizin in dieser schweren Situation eine Alleinherrschaft sei, und dass ein starker Mann gew\xe4hlt werden m\xfcsse"... Appian dachte dabei zwar an Pompeius, aber der starke Mann war dann schlie\xdflich C\xe4sar, der die Demokratie dauerhaft durch die Alleinherrschaft ersetzte.
Der derzeitige Premierminister Israels, der Falke Netanjahu, ist ein typisches Beispiel eines faschismusanf\xe4lligen, den internationalen Bankern loyal ergebenen Politikers, der alles daf\xfcr tut, um einen Krieg mit dem Iran zu entfachen, welcher sich angesichts der Mitgliedschaft Irans in der Schanghaier Organisation f\xfcr Zusammenarbeit (China, Indien, Russland, Pakistan...), rasch zu einem globalen Konflikt ausweiten k\xf6nnte, und bei dem es wegen der Kontrolle Irans \xfcber die nur 2 Meilen breite Stra\xdfe von Hormus, \xfcber die 20% der weltweiten Erd\xf6llieferungen laufen, zu einer Zerst\xf6rung der Weltwirtschaft kommen k\xf6nnte.
Um den Zweiten Weltkrieg einfacher entfachen zu k\xf6nnen, lie\xdfen die Banker durch die Politik eine latente Konfliktsituation schaffen, indem sie Deutschland mit gigantischen Kriegsreparationen belegten; dadurch schufen sie die Voraussetzung verarmter Massen, so dass sie den Deutschen nur noch einen ausreichend starken F\xfchrer unterjubeln mussten, der die Schuldigen benannte und einfache L\xf6sungen anbot; ein weiterer Faktor war die Schaffung des Vielv\xf6lkerstaates Tschechoslowakei mit einer starken deutschen Minderheit, die die Funktion einer f\xfcnften Kolonne einnehmen sollte und auch einnahm, um den Kriegsbrand zu entfachen.
Eine der Galerien in Somerset House wurde in einen glorreichen und 60 Meter langen Laufsteg verwandelt, der einen Rollentausch vorschl\xe4gt: der Benutzer nimmt den Platz des Modells ein und geht den Laufsteg entlang, um eine traumhafte "Audienz" zu bewundern, die Meisterwerke von Valentino tr\xe4gt, wie beispielsweise das Kleid, das Jackie Kennedy f\xfcr ihre Hochzeit mit Arist\xf3teles Onassis w\xe4hlte, die Kost\xfcme, die Monica Vitti in "La Notte" trug, oder ein Mantel aus Wolle und Leder, der der Kaiserin Farah Diba geh\xf6rte.
Der erste Krieg hatte zum Ziel, die gro\xdfen monarchistischen Staatenwesen Europas zu beseitigen, durch den zweiten Krieg sollte insbesondere die Kolonialherrschaft Gro\xdfbritanniens gebrochen werden, und der dritte Krieg soll die Weltbev\xf6lkerung auf ungef\xe4hr 0,5 - 1 Milliarden Menschen reduzieren (eine solche Anzahl w\xfcrde f\xfcr ihre Annehmlichkeiten und ihren Luxus sorgen und w\xfcrde auch nicht so viele Ressourcen verbrauchen), eine Universalreligion schaffen (der \xd6kumenismus ist hier nichts weiter als das Vorfeld) und schlie\xdflich zur \xdcbernahme der absoluten Macht f\xfchren.
Diesem Vorschlag stimmen die Fachleute und Beamte des Consejo Estatal de Prevenci\xf3n del Sida en Jalisco (Coesida) (staatlicher Ausschuss zur AIDS-Vermeidung in Jalisco) und auch die Patienten wie Fabrizio zu, der seinen Test bei einem privaten Labor durchf\xfchren lie\xdf, und dies aus dem einzigen Grund, weil es ein Freund von ihm gemacht hatte, der trotz seines jungen Alters bereits in der AIDS-Phase war und sogar das Kaposi-Sarkom (einen krebsartigen Tumor) hatte, was eine der \xfcblichen Komplikationen ist.
Der Fachmann f\xfcr Infektionskrankheiten und HIV/AIDS, Andrade Villanueva, kommentierte, dass die Wissenschaftler seit dem Jahr 2008 schlussfolgerten, dass AIDS zwar kein Todesurteil sei, dass aber die Jahre des \xdcberlebens und die Lebensqualit\xe4t vom Grad der Beeintr\xe4chtigung des Immunsystems der Personen bei Beginn der Behandlung abhinge, und dass jene gr\xf6\xdfere Chancen h\xe4tten, die nicht drogenabh\xe4ngig sind: bis zu 30 Jahren bei einer Z\xe4hlung von 200 CD4 und 50 Jahre bei einer Z\xe4hlung von 500 CD4.
Das Schwerwiegende an diesem Fall ist, dass das Gericht ein Dokument beiseite lie\xdf, das von der Regierung Mexikos unter der Figura amicus curiae (Freund des Gerichts) gesendet wurde, worin das von Vitro durchgef\xfchrte Verfahren im Rahmen des Gesetzes \xfcber Handelskonkurse beschrieben wird, und worin darauf hingewiesen wird, dass es sich strikt an die von beiden L\xe4ndern unterzeichneten Abkommen gehalten hatte, um dem Kapitel 15 des Konkursgesetzes der Vereinigten Staaten zu entsprechen.
Die Rothschilds sind an fast allen Zentralbanken der Welt beteiligt, und gegen die L\xe4nder, in denen sie nicht an den Zentralbanken beteiligt sind, f\xfchren sie Kriege oder r\xfcsten sich auf diese (vor dem \xdcberfall auf Afghanistan waren es 7 L\xe4nder, nach dem \xdcberfall auf den Irak waren es 5 L\xe4nder, nach dem Sturz Ghaddafis blieben nur noch vier, wobei Russland in der Zwischenzeit seine Zentralbank der russischen Regierung unterstellt hat).
31 Jahre nach dem Erscheinen des AIDS in der Welt, d. h. nach Auftreten der ersten berichteten F\xe4lle, "bedeutet der gro\xdfe Erfolg heute, dass das \xdcberleben eines Patienten, der die Behandlung rechtzeitig aufnimmt, und das \xdcberleben der allgemeinen Bev\xf6lkerung exakt gleich sind", erkl\xe4rte der Leiter der HIV-Einheit des HCG, Jaime Andrade Villanueva, wobei er sagte, dass diese Information im April dieses Jahres von einer angesehenen wissenschaftlichen Ver\xf6ffentlichung gest\xfctzt worden sei.
Correa gab an, dass die L\xf6sung f\xfcr das Asyl, das Assange seit dem Monat Juni in der Botschaft Ecuadors in London gew\xe4hrt wurde, die Gew\xe4hrung eines Freibriefs sei, womit er nach Ecuador reisen k\xf6nne, und dass dies in den H\xe4nden von Gro\xdfbritannien, Schweden und den juristischen Beh\xf6rden Europa's l\xe4ge. Er unterstrich, dass es mit London Gespr\xe4che gegeben habe, um eine L\xf6sung f\xfcr den eingesperrten Gr\xfcnder von WikiLeaks zu finden.
Dort verdiente er 75.000 Rupien (6,2 Euro) am Tag, und die Arbeit war nicht so hart, aber Anto ist mit seiner Familie nach Banyuwangi, einem Dorf in der N\xe4he, zur\xfcckgekehrt, und das aus einem Grund, der in Indonesien so wichtig wie der Schwefel ist: "Ich habe ein M\xe4dchen aus Bali geheiratet, wo sie Hinduisten sind, und ich habe sie nach Java gebracht, um sie zum Islam zu konvertieren".
Selbst wenn der Schwefel die Kehle verbrennt und die Augen jucken, wenn der Wind pl\xf6tzlich dreht und die Minenarbeiter in den dicken S\xe4ulen einklemmt, die aus dem Krater aufsteigen, sind die M\xe4nner so hart, dass niemand \xfcber schwere Krankheiten klagt ... nat\xfcrlich au\xdfer den \xfcblichen Atemproblemen, Arthrose, Schmerzen in den Knien und Blasen auf den Schultern, die sich vom Gewicht der K\xf6rbe verformt haben.
In ihrer Studie "The Unengaged Mind: Defining Boredom in Terms of Attention" - zu Deutsch etwa: "Der unt\xe4tige Verstand: Die Definition von Langeweile unter dem Aspekt der Aufmerksamkeit", die im September in der Fachzeitschrift "Perspectives on Psychological Science" erschien, weisen Professor Eastwood und seine Kollegen auf ein fr\xfcheres Experiment hin, bei dem Teilnehmer einem Band zuh\xf6rten, auf dem eine Person einen Magazinartikel vorlas.
Seit 2009 hat ein Service "zivil-milit\xe4rischer Aktionen" des Ministeriums f\xfcr Verteidigung (Cimic), der 2012 eingestellt wurde, in Dutzenden von Bergd\xf6rfern zahlreiche gemeinn\xfctzige Arbeiten und Ma\xdfnahmen f\xfcr die Sanierung der Landwirtschaft durchgef\xfchrt und von einer kleinen franz\xf6sischen Nichtregierungsorganisation durchf\xfchren lassen, um zu versuchen, die "Herzen und Geister zu gewinnen" und die unm\xf6gliche Aufgabe der Vereinbarkeit von Hilfen und offensiven Aktionen zu erreichen.
Die Sparma\xdfnahmen praktisch aller EU-S\xfcdstaaten werden zweifellos auf den gleichen Zustand hinauslaufen, bei dem die Menschen unter dem Druck eines katastrophalen Absturzes ihres sozialen Niveaus gezwungen sind, zu emigrieren (wie es im 19. Jahrhundert der Fall war), oder f\xfcr einen Hungerlohn am Rande der Gesellschaft zu darben und dabei darauf zu hoffen, dass irgendwann privates Investitionskapital ins Land flie\xdfen wird.
Selbst wenn sich die Sterblichkeit in den vergangenen Jahren bedeutend verringert hat (in Mexiko hat sich die Zahl der Personen, die an AIDS sterben, von 6.678 F\xe4llen im Jahr 2007 auf 4.862 im Jahr 2011 (Jahresbericht der ONUSIDA) verringert), ist es dennoch richtig, dass seit dem Erscheinen des AIDS 60 Prozent der in der nationalen Datenbank erfassten Patienten gestorben sind.
In Prag habe ich ein Grundst\xfcck mit einem Wert von 25 Millionen, eine Wohnung f\xfcr etwa 10 Millionen, eine weitere f\xfcr 8 Millionen, eine Kunstsammlung, die etwa 10 Millionen wert ist, sowie einen Aston Martin f\xfcr 3,5 Millionen und einen  \u2047 kodu Superb, der etwa eine Million wert ist. Und dann habe ich noch ein paar Millionen auf dem Konto.
"Mein Leben lang habe ich mir im Basketball viele H\xfcte aufgesetzt, sogar mehrere gleichzeitig, als ich Pr\xe4sident des BSN, Hauptgesch\xe4ftsf\xfchrer der Nationalmannschaft und Pr\xe4sident des Verbands in den 90er Jahren war", erinnerte sich Reyes bei einem Besuch von Primera Hora bei ihm zu Hause in Bayam\xf3n, wo er mit Isabel, seiner getreuen Ehefrau seit mehr als 50 Jahren, wohnt.
Neben einem alten Mann von 93 Jahren, der die letzte Familienzusammenkunft im Hof genie\xdft und gut von seinen Kopfkissen gest\xfctzt wird, w\xe4hrend man zu seinen Ehren anst\xf6\xdft, stirbt ein junger Mann von 36 Jahren, der von seinen Eltern, seiner Frau und seinen beiden kleinen Kindern umgeben ist, auf tragische Weise, nachdem er alles versucht hat, um zu \xfcberleben.
Denn selbst wenn die Teilchenphysik eine wirklich seltsame Welt ist, stellt sich heraus, dass f\xfcr sie ebenfalls ein derartiges Gesetz gilt: das Pauli'sche Ausschlussprinzip, das besagt, dass zwei Teilchen nicht den selben Raum zur selben Zeit besetzen k\xf6nnen, wenn sie sich im selben "Quantenzustand" befinden, wobei dieser "Zustand" im Gro\xdfen und Ganzen aus einigen ihrer Eigenschaften besteht.
Auswirkungen versp\xfcren wir bislang eher in der Vorbereitungsphase zuk\xfcnftiger Kontrollen - so haben wir das neue Kontrollinstrument "Erkennung von Risiken der Unwirtschaftlichkeit" eingef\xfchrt und mit diesem fast 14.000 \xf6ffentliche Auftr\xe4ge gepr\xfcft und analysiert - hier werden sich die \xc4nderungen selbstverst\xe4ndlich auswirken, da sich die Schwellenwerte \xe4ndern, die Bedingungen f\xfcr bestimmte Arten von Ausschreibungen modifiziert wurden u.a.
Der Zweite Weltkrieg brach aus, und ob sich nun Hitler von der Kette losriss, an der ihn die internationalen Banker anf\xe4nglich gehalten hatten, oder ob alles nach Plan lief, ist nur schwer abzusch\xe4tzen, auf jeden Fall schuf das Leid der europ\xe4ischen Juden in den Konzentrationslagern die Voraussetzung f\xfcr die Anerkennung des j\xfcdischen Staates durch die Weltgemeinschaft.
Obwohl Raketen aus dem Gaza-Streifen seit 2004 etwa 30 Israelis get\xf6tet haben, ist das Land relativ frei von Selbstmordattent\xe4tern geblieben - nicht zuletzt dank der Sperranlagen, die in das Westjordanland und damit in den Hauptteil eines etwaigen pal\xe4stinensischen Staates hineinverlaufen. Diese sch\xfctzen die j\xfcdischen Siedlungen, die zwar f\xfcr v\xf6lkerrechtswidrig erkl\xe4rt wurden, jedoch immer weiter ausgebaut werden.
Er teilte mit, dass Ma\xdfnahmen vorangetrieben w\xfcrden, um "die Zusammenarbeit im Kampf gegen die Unsicherheit in den St\xe4dten und gegen das organisierte, l\xe4nder\xfcbergreifende Verbrechen zu verbessern, sowie Ma\xdfnahmen, um den Zugang zu Medikamenten und zum Internet zu niedrigen Preisen in allen Gebieten S\xfcdamerikas zu verbessern und um im Fall von Naturkatastrophen gemeinsam und effizient zu handeln".
In der Tat hat uns der verstorbene Physiker Willard Boyle - der in den Bell Labs gearbeitet hat, in denen der Laser in den 1960er Jahren erfunden wurde, und der 1962 selbst den ersten Dauerstrichlaser (die ersten waren gepulst) entwickelt hat - bereits gesagt, dass der Laser am Anfang eher als eine "Laborspielerei" angesehen wurde.
Hier verbirgt sich eine weitere Aufgabe, mit der wir noch lange zu k\xe4mpfen haben werden, n\xe4mlich einen Menschen, der sich physisch in einem geschlossenen Raum befindet, glauben zu lassen, er befinde sich stattdessen in einem offenen, praktisch unendlichen Raum; hier arbeiten wir an Konzepten mit Laufb\xe4ndern (anderen als in Fitnessstudios), beweglichen Plattformen sowie gro\xdfen Kugeln.
Sandra Ha von Zico Import Pty Ltd, einem kleinen Familienunternehmen, merkt an, dass die Nachfrage nach Zigarettenetuis und Silikondeckeln zur Abdeckung der unertr\xe4glichen Verpackungen enorm angestiegen sind, seit die Konzerne British American Tobacco, Britain's Imperial Tobacco, Philip Morris und Japan Tobacco vor zwei Monaten am obersten australischen Gerichtshof mit ihrer Anfechtung der Gesetze scheiterten.
Efe versuchte wiederholt, Zugang zu dem unterzeichneten Dokument bei der VI. Ordentlichen Sitzung der Staats- und Regierungsoberh\xe4upter der Unasur zu erlangen. Quellen in der Staats- und Pr\xe4sidentenkanzlei teilten anfangs mit, dass sie es nach der Klausur \xfcbergeben w\xfcrden, erkl\xe4rten danach jedoch, dass es zu gewisser Zeit auf der Webseite der peruanischen Regierung ver\xf6ffentlicht w\xfcrde.
"Und es macht, dass die Kleinen und die Gro\xdfen, die Reichen und die Armen, die Freien und die Knechte allesamt sich ein Malzeichen geben an ihre rechte Hand oder an ihre Stirn, dass niemand kaufen oder verkaufen kann, er habe denn das Malzeichen, n\xe4mlich den Namen des Tiers oder die Zahl seines Namens.
Zu den kontroversen EU-Verordnungen geh\xf6rt u.a. die verbindliche Beimischung von Bioethanol zu Kraftstoffen, die in ihrer Folge natursch\xe4digend ist, des weiteren das Verbot der zuverl\xe4ssigen Quecksilberthermometer, nur weil diese eine relativ geringe Menge dieses Gefahrenstoffes enthalten, oder auch die Richtlinie zur Gr\xf6\xdfe von H\xfchnerk\xe4figen, wegen der in diesem Jahr Eier wesentlich teurer wurden.
Es gibt aber auch Technologien, die tats\xe4chlich darauf ausgerichtet sind, den "Bildern in der Luft" etwas Handfestes zu verleihen, zum Beispiel erzeugt die Interferenz von einigen gerichteten Ultraschallstrahlen in einem bestimmten Punkt, wo sich der Finger befindet, ein Gef\xfchl, das momentan aber noch so schwach ist, als pustete jemand \xfcber die Handballen.
Die besten Szenen des Films spielen in den Stra\xdfen und zeigen die Rekonstruktion von Ereignissen, die wirklich stattgefunden haben - die Eingangssequenz der Erst\xfcrmung der Botschaft ist in ihrer \xdcbersichtlichkeit sehr beeindruckend, und vermittelt dabei dennoch das Gef\xfchl der Verwirrtheit und der Unvorhersehbarkeit, das eintritt, wenn sich irgendwo einmal die Geschichte bewegt.
Mit dem Wenigen arbeitet er aber recht erfolgreich, wobei er der Realit\xe4t manchmal etwas nachhilft - was dann nicht immer so elegant wirkt (die Szenen, in der die drohende Krise auf dem Flughafen in Teheran von einem Telefonat in Amerika abgewendet wird, oder auch die Verfolgungsjagd auf der Startbahn, wirken etwas gek\xfcnstelt).
Im ersten Saal dieser Ausstellung, die noch bis zum 3. M\xe4rz zu sehen sein wird, gibt es eine Vielzahl an privaten Briefen und Fotos mit der Unterschrift der erlesensten Aristokratie, angefangen von der Prinzessin Salimah Aga Khan, \xfcber die Prinzessin Marie-Chantal von Griechenland und Margarita von England bis hin zu Lord Snowdon.
Es sind zwar nur 250 Meter bis zur Spitze des Vulkans, der sich bis in eine H\xf6he von 2386 Metern erhebt, aber die ersch\xf6pften Tr\xe4ger brauchen mehr als 40 Minuten f\xfcr den Aufstieg im Schildkr\xf6tentempo, wobei sie das Gleichgewicht behalten und ihre Schritte vorsichtig setzen m\xfcssen, damit sie nicht ausrutschen und abst\xfcrzen.
In diesem Sinne sagte der Pr\xe4sident von Kolumbien, Juan Manuel Santos, vor Beginn seiner Teilnahme an dem regionalen Treffen, dass er am Samstag in Mexiko ein Treffen mit seinem Gegen\xfcber von Nicaragua, Daniel Ortega, erwartete, um den maritimen Konflikt nach einem von Bogot\xe1 in Frage gestellten Urteil des IGH respektvoll zu behandeln.
Diese Bosonen gliedern sich gem\xe4\xdf der Webseite The Particle Adventure von den Berkeley Laboren (die \xfcbrigens absolut erstaunlich ist) in zwei Gruppen auf: die Mesonen, die wir hier nicht behandeln werden und die "Kraftteilchen", durch die sich die gro\xdfen Kr\xe4fte der Natur verbreiten und mit denen das Higgs-Boson irgendwie verwandt w\xe4re.
Der offiziellen Statistik des Innenministeriums zufolge ging die Zahl der Delikte mit illegalen Waffen in ganz Russland im Zeitraum von Januar bis Oktober 2011 um 7% auf 22,9 Tausend zur\xfcck, w\xe4hrend die Zahl der aufgedeckten F\xe4lle von Diebstahl und Erpressung im Zusammenhang mit Waffen, Munition, Sprengstoffen und Sprengvorrichtungen um 7,8% schrumpfte.
Der einzige Grund, warum so viele Menschen mexikanischer Herkunft in St\xe4dten wie Los Angeles, Las Vegas, Phoenix, Denver oder San Antonio leben, besteht darin, dass an einem Punkt in unserem Stammbaum eine Person - vielleicht ein Eltern- oder Gro\xdfelternteil - keine Chance in Mexiko geboten bekam und in Richtung Norden auswanderte.
Restall wies darauf hin, dass \xfcber die Jahre viele Tage vom letzten Gericht gesprochen wurde, und sagte, dass wenn am 21. Dezember nichts passiert, "die Leute sofort an ein neues Datum denken" oder dar\xfcber philosophierten, dass der 21. Dezember der Beginn einer siebenj\xe4hrigen Periode sei, wonach das Ende der Welt k\xe4me.
Sebelew ist davon \xfcberzeugt, dass ein k\xfcnftiger Migrant ohne Sprachkenntnisse zwangsl\xe4ufig Menschen mit b\xf6sen Absichten begegnen wird, die ihn unter dem Vorwand von Hilfe in eine dunkle, enge Baracke stecken, wo er mit Dutzenden seinesgleichen Monate ohne Essen und Dokumente ausharren und 12 bis 14 Stunden am Tag schuften wird.
Besonders katastrophal ist die Tatsache, dass die heutigen Eliten den in Zukunft m\xf6glichen Verlusten von Hunderttausenden von Menschenleben, den humanit\xe4ren und sozialen Katastrophen, deren Zeugen wir bereits heute sind, sowie den Verbrechen gegen die Menschlichkeit, wie wir sie aus der \xe4lteren und neueren Geschichte kennen, in vollkommener Ignoranz gegen\xfcber stehen.
Dem Patienten muss das Ausma\xdf des Risikos seiner Krebserkrankung wirklich verst\xe4ndlich gemacht werden, indem ihm die m\xf6glichen Optionen aufgezeigt werden, bei denen Prostatakrebse unbehandelt bleiben kann, wenn er die Lebensqualit\xe4t auf lange Sicht nicht beeintr\xe4chtigt, und man sich in diesen F\xe4llen eher f\xfcr eine aktive \xdcberwachung der Krankheit entscheidet.
Die Teilnehmer der Proteste, die am Donnerstag um 6.30 Uhr morgens vor dem McDonald's in der 40th Street und in der Madison Avenue begannen, forderten, dass die Kassierer und K\xf6che von Fast-Food-Restaurants einen Mindestlohn von 15 US-Dollar die Stunde erhalten, was mehr als einer Verdoppelung des jetzigen Mindestlohns entspricht.
Der H\xf6hepunkt der Proteste war eine Versammlung am Mittag vor dem McDonald's am Times Square, bei dem einige lokale Demokraten sprachen, darunter Stadtratsmitglied Jumaane Williams, der sagte: "McDonald's sagt, es verkaufe Milliarden Portionen, und trotzdem gew\xe4hrt man euch keine Krankentage, und ihr werdet f\xfcr eure ehrliche Arbeit nicht bezahlt!"
Samuel Roberts, 21 und Geschichtsstudent in Corpus Christi, der das Gesuch f\xfcr gr\xf6\xdferen Schutz initiierte, ist der Ansicht, ein solches Klima ist "unangenehm". Die 19-j\xe4hrige Stephanie Cherill, designierte Pr\xe4sidentin der konservativen studentischen Vereinigung von Oxford sagt, sie habe bei JCR-Mitgliedern eine wachsende Ablehnung gegen\xfcber Studenten der gem\xe4\xdfigten Rechten beobachtet.
Die Best\xe4tigung beider Pr\xe4sidenten, dass sie sich dem IGH unterwerfen w\xfcrden, erfolgte, nachdem Kolumbien nach einer Entscheidung \xfcber die maritimen Grenzen mit Nicaragua, die es f\xfcr einen schweren Fehler hielt, Klage gegen das Abkommen von Bogot\xe1 erhoben hatte, worin es zustimmte, sich den Urteilen dieses internationalen Gerichtshofs zu unterwerfen.
Correa unterst\xfctzte auch die Entscheidung, das Veto gegen Paraguay in der Unasur mindestens bis zu seinen n\xe4chsten Wahlen aufrechtzuerhalten, wobei er argumentierte, dass der Organismus "hart bleiben muss und keinem Opportunismus und keinem als legal verkleideten Staatsstreich stattgeben darf", weil dadurch "die Legitimit\xe4t der Demokratie in Paraguay zerst\xf6rt wurde."
"Ich arbeite, unternehme viel, habe ein aktives, aber verantwortliches Sexleben, ich achte auf meine Gesundheit und die der anderen Person", z\xe4hlt Fabrizio auf, der zustimmte, seine intimen Details mit MILENIO JALISCO zu teilen, um mit seinem Zeugnis jene zu animieren, die heute im Rahmen des weltweiten AIDS-Tages Angst haben.
Afghanistan, das Land der Berge mit starken lokalen Identit\xe4ten h\xe4tte von einer gewissen Dezentralisierung am Beispiel der westlichen Nationen profitieren sollen, aber durch Abschaffung des Amtes des Ministerpr\xe4sidenten, das seit der Konstitution von 1964 bestand, wollten die USA aus ihm einen zentralisierten Staat mit einer starken Pr\xe4sidialgewalt machen.
Wenn es aus einem anderen EU-Land kommt, wandert lediglich die Armut von einem Land ins andere; oder das Kapital bleibt gleich ganz aus, denn in China, Indien, Brasilien, in der T\xfcrkei, in Marokko oder \xc4gypten bzw. in Afrika \xfcberhaupt arbeiten die Besch\xe4ftigten f\xfcr einen Bruchteil der europ\xe4ischen L\xf6hne.
Dem CIA gelang es in Zusammenarbeit mit den kanadischen Beh\xf6rden, die Fl\xfcchtlinge aus dem Iran zu bringen; dabei half ihnen eine extravagante Story zur Verdeckung ihrer wahren Identit\xe4t - sie reisten mit kanadischen P\xe4ssen getarnt als Mitglieder eines Filmstabes, der angeblich im Land Drehorte f\xfcr einen Science-Fiction-Film besuchte.
Weil die Regierung einer Anfrage des Senats, zu erkl\xe4ren, unter welchen Bedingungen und Umst\xe4nden der mexikanische Botschafter in Japan das Anti-Counterfeiting Trade Agreement unterzeichnete, das unter der englischen Abk\xfcrzung ACTA bekannt ist, nicht nachgekommen ist, ist die Angelegenheit gem\xe4\xdf dem mexikanischen Institut f\xfcr intellektuelles Eigentum bereits archiviert worden.
Er empfiehlt eine komplette \xdcberarbeitung des Systems f\xfcr die Vergabe \xf6ffentlicher Auftr\xe4ge und die Finanzierung der Parteien: "Wir k\xf6nnen nicht tiefer fallen; indem wir den Dingen mit Mut auf den Grund gehen, k\xf6nnen wir das Haus auf einer solideren Basis mit mehr Kontrollen und Gesetzen wieder aufbauen."
Die einen stehen hinter Israel und argumentieren mit dessen Recht auf Selbstverteidigung, w\xe4hrend sie die Pal\xe4stinenser als Terroristen bezeichnen; die anderen wiederum unterst\xfctzen die Pal\xe4stinenser, argumentieren mit dem Rassismus des israelischen Staates, mit dem an den pal\xe4stinensischen Arabern ver\xfcbten V\xf6lkermord und bezeichnen den Staat Israel als terroristisch.
Inmitten der \xfcblichen Schuldzuweisungen wurden zahllose Geb\xe4ude in Schutt und Asche gelegt, mehr als 140 Pal\xe4stinenser, die meisten davon Zivilisten, und sechs Israelis get\xf6tet - und zum ersten Mal sind Raketen aus Gaza in der N\xe4he der israelischen Metropole Tel Aviv und der heiligen Stadt Jerusalem eingeschlagen.
Jubelnde Hamas-Anh\xe4nger glauben, dass sich um Israel ein islamistischer Halbmond bildet - vom Libanon im Norden, wo die militante Hisbollah die Macht hat, \xfcber Syrien, wo Rebellen einer zunehmend islamistischeren Pr\xe4gung vor der St\xfcrzung Bashar Assads stehen k\xf6nnten, bis hin zu Jordanien, wo Hamas-Verb\xfcndete dem K\xf6nig drohen.
Bei jener Mannschaft waren nicht nur Mincy, Gausse, Ramon Rivas, Fico L\xf3pez und "Picul\xedn" (Ortiz) wieder dabei, sondern auch die jungen Spieler (Javier) "To \u2047 ito" Col\xf3n und James Carter, die Br\xfcder Le\xf3n (Francisco und Edgar) und Mario "Quijote" Morales, der 1990 wegen einer Knieverletzung nicht dabei sein konnte.
\xc4gypten muss nun gemeinsam mit der T\xfcrkei und Katar die Waffenlieferungen in den Gaza-Streifen stoppen und ist besser positioniert als je zuvor, um die Hamas von der Idee eines j\xfcdischen Staates auf Grundlage der Grenzen von 1967, erg\xe4nzt durch Gebietstausch und ein gemeinsames Jerusalem, zu \xfcberzeugen.
In diesem Sinne begl\xfcckw\xfcnschte er sich, dass Ecuador nicht mehr von solchen Journalisten "und auch nicht von den Bankern oder hegemonischen und spie\xdfb\xfcrgerlichen L\xe4ndern beherrscht wird", und nahm vorweg, dass er bei einer Wiederwahl "die Revolution vertiefen wird, um den Weg in diese richtige Richtung fortzusetzen."
Richtig ist au\xdferdem, dass nach Abzug der Stimmen der Filialen die Gl\xe4ubiger von Vitro, die Gl\xe4ubiger, die bei den Gerichten der Vereinigten Staaten gegen Vitro klagten, d. h. die Geier-Fonds wie z. B. Aurelios Capital, Aurelios Convergencia, Elliot Internacional und Liverpool Limited, keine Mehrheit erreicht h\xe4tten.
Bevor er durch einen Schlaganfall im Jahr 2008 an den Rollstuhl gebunden wurde, war Rexes 6 Jahre lang Teil dieses Sports, sei es als Spieler niedrigerer Klassen, Spieler der ersten nationalen Liga, Bevollm\xe4chtigter und Leiter im BSN mit den Vaqueros de Bayam\xf3n oder Pr\xe4sident des Basketballverbands.
Dies alles haben wir miteinander verglichen, und obgleich die Pr\xfcfung noch nicht abgeschlossen ist, konnten wir \xe4u\xdferst interessante Unterschiede feststellen. Allgemein gesagt, sind die Gesetze bei uns vielleicht sogar noch etwas "strenger und perfekter", die eigentliche Anwendung jedoch ist in Deutschland in einigen Parametern besser.
Ich m\xf6chte an dieser Stelle nicht dar\xfcber schreiben, wer in diesen immer wiederkehrenden Wellen des T\xf6tens Schuldiger und wer Opfer ist; letztendlich wurden die heutigen Bewohner Israels einschlie\xdflich der Selbstverwaltungsgebiete in die derzeitige politische Situation hineingeboren und haben den Beginn der Gewalt selbst nicht erlebt.
Relativ absurd ist auch eine Richtlinie, die die europ\xe4ischen Beamten selbst betrifft - jeder, der in der EU eine offizielle Funktion einnimmt, darf wegen der Sensibilit\xe4t des Themas f\xfcr Griechenland nicht die Bezeichnung Mazedonien verwenden und muss stattdessen FYROM (Former Yugoslav Republic of Macedonia) sagen.
Am Freitag befragte die Richterin Manning ebenfalls zu einer Anschuldigung, die er in seiner Aussage am Donnerstag erhoben hatte - so habe er eine Nacht nackt in seiner Zelle in Quantico schlafen und bei einer morgendlichen Z\xe4hlung nackt vor Wachen und anderen Gefangenen stehen m\xfcssen.
Meine Frau, die in Guadalajara geboren wurde und als Kind legal in die Vereinigten Staaten einwanderte, erinnert mich daran, dass zwischen Mexikanern und mexikanischen Amerikanern Spannungen bestehen, weil Mexikaner eine klarere Vorstellung dar\xfcber besitzen, wer sie sind - und mexikanische Amerikaner nehmen ihnen dies \xfcbel.
Wenn zumindest einige Mexikaner noch nicht bereit sind, den Vereinigten Staaten f\xfcr den Umgang mit Mexiko vor anderthalb Jahrhunderten zu vergeben, m\xfcssen sie auch akzeptieren, dass einige mexikanische Amerikaner einen Groll daf\xfcr hegen, wie ihre Familienmitglieder erst vor gar nicht so langer Zeit behandelt wurden.
Nach langer Lekt\xfcre von Forschungsliteratur und der Pr\xe4sentation der Idee vor einer Fokusgruppe von etwa 100 Personen kamen Professor Eastwood und seine Kollegen zu dem Schluss, dass sich Langeweile als die Erfahrung, "eine befriedigende T\xe4tigkeit aus\xfcben zu wollen, dies aber nicht zu k\xf6nnen" definieren l\xe4sst.
Die Pr\xe4sidenten von Peru, Ollanta Humala, und Chile, Sebasti\xe1n Pi \u2047 era, trafen sich w\xe4hrend des regionalen Treffens und best\xe4tigten, dass sie die Entscheidung des IGH annehmen w\xfcrden, der am Montag in Den Haag beginnt, im Prozess, den Lima gegen Santiago einleitete, die Pl\xe4doyers beider Seiten anzuh\xf6ren.
In Bezug auf die M\xf6glichkeit, dass er sich als Kandidat f\xfcr die n\xe4chsten Pr\xe4sidentschaftswahlen in Ecuador stellt, um sein drittes Mandat in Folge zu erreichen, gab er an, dass er diese M\xf6glichkeit "mit viel Optimismus und Freude sieht, obwohl es manchmal auch sehr schwer f\xe4llt."
An den dazu bestimmten Orten "wurde die Verteilung von Kondomen tats\xe4chlich erh\xf6ht; fr\xfcher wurden sie einzeln abgegeben, jetzt geben sie uns Pakete zu mit hundert St\xfcck, was schon gut ist, es gibt aber noch immer Menschen, die keinen Zugang zu einem Kondom haben", sagte er.
Bei einem Treffen am Wochenende auf einem Forum der Universit\xe4t der Karibik haben eine Gruppe nationaler und ausl\xe4ndischer Umweltsch\xfctzer, Akademiker, Unternehmer und allgemeinen Mitglieder der b\xfcrgerlichen Gesellschaft die Schaffung einer Breiten Front beschlossen, um sich der Er\xf6ffnung des chinesischen Dragon Mart in Canc \u2047 n zu widersetzen.
Jedes Semester, wenn der Religionsprofessor beschloss, einen Kurs \xfcber das Ende der Welt abzuhalten, wusste er, dass er \xfcber einen unwiderstehlichen Angelhaken verf\xfcgte: das Ende der "langen R\xfcckw\xe4rtsz\xe4hlung" des Maya-Kalenders am 21. Dezember, von dem viele Menschen glaubten, dass es das Ende der Welt bedeute.
"Dieses Experiment, das wir gemeinsam vornehmen, n\xe4mlich die Geburt eines Kindes in einer fremden Umgebung, wird dazu f\xfchren, dass wir einen Behinderten, einen vollkommen unangepassten Menschen zur Welt bringen werden", sagt der Leiter der Bioethikkommission des Instituts f\xfcr medizinisch-biologische Probleme RAN, Igor Pestow, voraus.
Die weltweit ersten Gesetze f\xfcr einheitliche Zigaretten- und Tabakverpackungen sind in Australien in Kraft getreten. Damit werden Markenlogos und Farben durch neutrale, olivgr\xfcne Deckel ersetzt, die dar\xfcber hinaus mit drastischen Bildern bedruckt sind, welche kranke K\xf6rperteile und durch Zigarettenrauch erkrankte S\xe4uglinge und Kinder zeigen.
"Man kann schon bei Kindern jungen Alters sehen, dass sie die Botschaft verstehen, die Tabakkonzerne mit ihrem Markenbild zu bewerben versuchen", so Bundesgesundheitsministerin Tanya Plibersek. Sie zitiert Studien, die beispielsweise gezeigt haben, dass Kinder die Krone eines Logos mit der Idee einer Prinzessin assoziieren.
Sie erhalten auch keinen Anteil an den 30.000 Rupien (2,5 Euro) Zuschlag pro Fotoapparat, den die W\xe4chter dieses Naturparks zusammen mit dem Eintrittsgeld in H\xf6he von 15.000 Rupien (1,2 Euro) von den Touristen verlangen, die zum Fotografieren des Vulkans und der menschlichen Tragesel kommen.
Der Pr\xe4sident Ecuadors h\xe4lt au\xdferdem den Wunsch seines kolumbianischen Gegen\xfcbers, Juan Manuel Santos, jetzt und nach dem Urteil des Internationalen Gerichtshofs von Den Haag, das die maritime Staatshoheit von Nicaragua bevorteilte, mit Nicaragua die seerechtlichen Grenzen zwischen beiden L\xe4ndern zu verhandeln, f\xfcr "absolut berechtigt."
Ebenso vertraute er auf einen guten Abschluss der Streitigkeiten \xfcber die Seegrenzen zwischen Peru und Chile vor demselben Gerichtshof und meinte, dass "es f\xfcr Lateinamerika richtig ist, internationale Instanzen anzurufen, wenn sich beide L\xe4nder verpflichten, das Urteil anzunehmen, selbst wenn es sehr hart ausf\xe4llt."
Nachdem das Berufungsgericht der Vereinigten Staaten ein Urteil best\xe4tigt hat, das die Neustrukturierung der Verbindlichkeiten der Gruppe Vitro nicht anerkennt, die \xfcber einen Handelskonkurs in Mexiko erreicht wurde, wird ein unheilvoller Pr\xe4zedenzfall f\xfcr jedes nationale Unternehmen mit Niederlassungen im Nachbarland geschaffen, das Zahlungsprobleme hat.
Der ehemalige Bauingenieur Gilles Surprenant hat dies vor der Kommission ausf\xfchrlich beschrieben: in zehn Jahren erhielt er vom Bauunternehmen Geschenke, Einladungen zu Reisen, Golf-Turnieren, Restaurants und Eishockey-Spielen, sowie Bestechungsgelder in H\xf6he von 736.000 Dollar als Gegenleistung f\xfcr Kanalisationsvertr\xe4ge, deren Kosten er k\xfcnstlich aufbl\xe4hte.
Nachdem der Kurs von Bitcoin im Juni 2011 einen H\xf6chststand von 30 Dollar (23 Euro) erreicht hatte, fiel er f\xfcnf Monate sp\xe4ter auf 2 Dollar, bevor er sich heute auf rund zehn Dollar erholt hat (die Kurse sind auf der Webseite bitcoincharts.com aufgef\xfchrt).
Die Demonstranten wurden auch von anderen prominenten New Yorker Demokraten unterst\xfctzt, zum Beispiel, B\xfcrgermeisterkandidat Bill De Blasio, der sagte, dass "wir sollten gemeinsam die Fast-Food-Mitarbeiter unterst\xfctzen, damit sie einen gerechten Lohn erhalten und den wirtschaftlichen Wohlstand erreichen k\xf6nnen, den jeder New Yorker verdient!".
Offensichtlich geraten die liberalen Demokratien derzeit schnell in eine Situation, wie sie Appian in seinem Werk zur Krise der r\xf6mischen Republik zu Zeiten C\xe4sars und Pompeius' beschreibt: "Der Staat war schon seit langem im Zerfall begriffen, und die \xc4mter wurden mit Gewalt besetzt.
Um den kulturellen Austausch etwas zu f\xf6rdern, reist der Imbongi-Chor alle zwei, drei Jahre gemeinsam durch den S\xfcden Afrikas und singt Lieder voller Wehmut, Kampfgeist, Zuversicht und schwarzem Selbstbewusstsein, die viele am s\xfcdlichen Zipfel des schwarzen Kontinents noch aus Zeiten der Apartheid kennen.
Man hatte mich nur aus einem Grund schikaniert - ein Grund, der in dieser angeblichen Wiege der Erleuchtung um so engstirniger und grausamer schien: Mein mittlerweile verstorbener Vater Woodrow Wyatt war ein wichtiger Berater Margaret Thatchers gewesen und ich Bef\xfcrworterin der Konservativen Partei.
"Der Tagelohn der Minenarbeiter hier, wo bei der Kaffeeernte 15.000 Rupien (1,2 Euro) am Tag gezahlt werden und das durchschnittliche Monatseinkommen zwei Millionen Rupien (167 Euro) betr\xe4gt, ist sehr hoch", erl\xe4utert der Tr\xe4ger, der vorher als Maurer auf der touristischen Insel Bali arbeitete.
"Meine tiefsten Geheimnisse w\xfcrde ich nicht in einem Post bekannt geben" sagt der 10 Jahre alte Jorge beim Versuch, die Bedeutung von "privat" in Webseiten wie Facebook, Twitter, Hotmail und Windows Live Messenger zu erkl\xe4ren, wo er seit zwei Jahren \xfcber Konten verf\xfcgt.
"Chile war, ist und bleibt auch weiterhin ein Land, das sich an die internationalen Gesetze h\xe4lt, friedliche L\xf6sungen f\xfcr Streitigkeiten sucht, Abkommen schlie\xdft und sich den internationalen Gerichtsh\xf6fen unterwirft", f\xfcgt Pi \u2047 era hinzu und gr\xfc\xdfte Humala mit einem H\xe4ndedruck vor den Fahnen beider L\xe4nder.
"Wir haben beschlossen, einer Reihe von 31 emblematischen Projekten den Vorrang zu geben, die die r\xe4umlichen Verbindungen in S\xfcdamerika und besonders in l\xe4ndlichen und Grenzgebieten verbessern sollen...und somit unsere L\xe4nder vereinen und neue Wirtschaftsformen erschlie\xdfen", sagte der peruanische Pr\xe4sident in einer verlesenen Erkl\xe4rung.
Er kritisierte au\xdferdem die schwedische Justiz, die von ihm verlangt habe, ihn auf seinem Staatsgebiet einem Verh\xf6r wegen eines angeblichen Sexualdelikts zu unterziehen, w\xe4hrend "die schwedische Rechtsprechung dies mittels einer Videokonferenz erlaubt, die \xfcber die Botschaft Ecuadors in London h\xe4tte ausgef\xfchrt werden k\xf6nnen."
Er macht eine schlagende Aussage: "Neun von zehn Patienten kommen zu uns, wenn sie bereits eine begleitende Infektion haben. Um die globale Sterblichkeit beeinflussen zu k\xf6nnen, sind fr\xfchzeitigere Diagnosen erforderlich, weshalb allen Personen, bei denen dies erforderlich ist, massiv Erkennungstests angeboten werden m\xfcssen."
In der Praxis f\xfchrt die am 15. Juni ergangene Anerkennung des Urteils durch den Richter Harlin Hale am Gericht in Bancarrotas f\xfcr den n\xf6rdlichen Distrikt in Texas dazu, dass die mexikanischen Unternehmen der Beschlagnahme ihres Eigentums jenseits des Flusses Bravo hilflos ausgesetzt sind.
Aber Charm\xe9 hatte keine Ahnung, was ihn in den folgenden beiden Monate erwarten sollte: der zerst\xf6rerische Hurrikan Sandy, den einige als "Deudarmaggedon" bezeichnet haben, sowie ein wachsender Konflikt unter Beteiligung Israels, dem Ort, von dem die christlichen Theoretiker glauben, dass die Apokalypse beginnt.
Ich hatte mir Webseiten und Blogs angesehen, als jemand auf mich aufmerksam wurde und mir vorschlug zur Station "Begowaja" zu kommen, wo eine Person auf mich warten w\xfcrde, die mich an einen gewissen Ort br\xe4chte, wo wir dann den Preis verhandeln k\xf6nnten.
- Nat\xfcrlich ist es nicht angenehm, unterwegs immer ein Smartphone in der erhobenen Hand zu halten, aber ich denke Folgendes: Die tollste Variante w\xe4re eine "wechselnde" erweiterte Realit\xe4t, bei der wir \xfcber eine Cloud von der Brille auf das Smartphone umschalten k\xf6nnten,
"Ein Gesetz muss doch seine G\xfcltigkeit haben, und wenn etwas gesetzlich verboten ist, dann kann doch nicht einfach der Regierungsvorsitzende kommen, und das Kontrollamt, dessen Pflicht nun einmal die Kontrolle der Einhaltung des Gesetzes ist, in seiner T\xe4tigkeit behindern", stellt Kala fest.
Die Temperaturen bleiben auch in tieferen Lagen unter Null, so dass sich Schnee und Eis auf den Stra\xdfen halten werden. Aus den Tiefebenen, insbesondere s\xfcd\xf6stlich vom B\xf6hmischen Mittelgebirge, sind dagegen keine Probleme gemeldet, und die Stra\xdfen sind dort in der Regel trocken.
Die r\xfccksichtslose Praxis des Privatkapitals schafft in den einzelnen Volkswirtschaften eine Situation, in der die Regierungen sich gezwungen sehen, in Konkurrenz miteinander zu treten, um das soziale Niveau der eigenen Bev\xf6lkerung k\xfcnstlich zu senken und damit ausl\xe4ndisches Kapital ins Land zu locken.
Wir m\xfcssen uns eingestehen, dass wir in einer Zeit leben, in der sich der Reichtum der Welt in der Hand weniger Einzelner konzentriert, und dass diese Konzentration des Geldes und der daraus hervorgehenden Macht nicht innerhalb der Lebensspanne einer Generation entstanden ist.
Die erste Presseagentur (Reuters) wurde von den Rothschilds bereits in den 90er Jahren des 19. Jahrhunderts gekauft, um die Verbindung ihres Namens mit hochkriminellen Taten zu unterbinden, in deren Hintergrund immer die Festigung ihrer Macht, die Vermehrung ihres Verm\xf6gens oder beides stand.
Der EU-Apparat entscheidet oft unter dem Druck dieser oder jener Lobby aus Handel und Industrie, deren Forderungen in Br\xfcssel in der Regel von einem oder mehreren Mitgliedsl\xe4ndern vertreten werden (so versucht Tschechien derzeit beispielsweise, auch mit Veto-Drohung die Forderungen tschechischer Banken durchzusetzen).
In der offiziellen Liste der in der EU registrierten Produkte tauchen in der Gesellschaft der weltber\xfchmten K\xe4sesorten Feta und Gorgonzola, des L\xfcbecker Marzipans oder des Parmaschinkens nun auch der Karlsbader Zwieback, Karpfen aus Poho \u2047 elice und T \u2047 ebo \u2047 , oder auch der Saazer Hopfen auf.
Am 21. November sandte Chief Oates seinen Mitarbeitern in Aurora eine E-Mail, in der er erkl\xe4rte, der Staatsanwalt w\xfcrde kleinere Marihuanadelikte bei Personen \xfcber 21 Jahren nicht l\xe4nger verfolgen, und dass die Polizei "ab sofort" keine Strafanzeigen f\xfcr diese Vergehen anstreben werde.
Oben angekommen, bahnen sie sich den Weg zwischen den Touristen, die sie wie Zirkusaffen fotografieren und laufen mit den erm\xfcdend schweren K\xf6rben drei Kilometer bis zur Waage, die eine Minengesellschaft ein wenig weiter unten auf einer H\xf6he von 1850 Metern aufgestellt hat
W\xe4hrend der Richter der Sache darauf hinweist, dass die Gl\xe4ubiger dem Konkursrecht der Vereinigten Staaten unterliegen m\xfcssen, sagt das Berufungsgericht des Fifth Circuit mit Sitz in New Orleans zun\xe4chst, dass es sich bei dem Hauptverfahren um den in Mexiko behandelten Handelskonkurs handelt.
Der Sprecher des Unternehmens, Dan Fogelman, behauptete in einem Interview auf der Webseite der linksgerichteten Huffington Post, dass insgesamt "weniger als f\xfcnf" Walmart-Mitarbeiter die Arbeit niederlegten und die Protestaktion lediglich "ein weiterer PR-Trick" der Gewerkschaft, die die Proteste organisierte, gewesen sei.
Unter diesem Begriff ist ein Zustand zu verstehen, bei dem der Hersteller versucht, durch Einfuhr g\xfcnstiger Waren im wirtschaftlichen Wettbewerb zu bestehen, indem er die Konkurrenz "unterbietet", um dadurch einen gr\xf6\xdferen Marktanteil an sich zu rei\xdfen und seinen Gewinn zu erh\xf6hen.
W\xe4hrend die restliche arabische Welt zaghafte Schritte in Richtung Demokratisierung unternimmt, werden Pal\xe4stinenser weiterhin ihres Selbstbestimmungsrechtes beraubt - ein Pulverfass, das zweifellos eines Tages in den israelisch besetzten Gebieten explodieren wird, genau wie diese Woche ein Bus in Tel Aviv explodierte.
Kevin A. Sabet, fr\xfcherer Drogenpolitik-Berater der Obama-Regierung ist der Ansicht, dass Kriminalbeamte zwar wahrscheinlich keine T\xfcren eintreten werden, um kleinere Mengen der Drogen zu beschlagnahmen, sich aber vermutlich str\xe4uben werden, die unter der neuen Gesetzgebung legalen, staatlich regulierten Marihuana-Gesch\xe4fte zu dulden.
Er erkl\xe4rt, dass es sich um ein komplexes Thema handelt, "weil wir von ihnen verlangen, dass sie ein definiertes Kriterium dar\xfcber haben, was verbreitet, ver\xf6ffentlicht oder gesagt werden darf, und dies in einem Alter, wo die Reife daf\xfcr nicht ausreichend ist."
Correa, der am 6. Gipfeltreffen der Pr\xe4sidenten der Union S\xfcdamerikanischer Nationen (Unasur) teilnahm, das in Lima stattfand, erkl\xe4rte dem staatlichen Fernsehen in Peru, dass sich die Europ\xe4er "im zweiten Weltkrieg und in anderen Auseinandersetzungen umbrachten" und "heute praktisch ein Vaterland sind."
Der ecuadorianische Staatschef nahm heute in Lima am 6. Gipfeltreffen der Staats- und Regierungschefs der Union s\xfcdamerikanischer Nationen (Unasur) teil, die mit dem Aufruf zu einer h\xf6heren regionalen Integration beendet wurde, um f\xfcr einen nachhaltigen Fortschritt, Gleichheit und Sicherheit zu sorgen.
Auf dem Hauptcampus der Universit\xe4t Pennsylvania haben der Professor f\xfcr lateinamerikanische Geschichte Matthew Restall und seine Kollegin Amara Solari, eine beisitzende Professorin f\xfcr Kunstgeschichte und Anthropologie ein Team gebildet, um einen Kurs mit der schlichten Bezeichnung "Das Ende der Welt" anzubieten.
Und in der anderen bewegen sich die Bosonen, eine \xfcble Bande von Anarchisten, denen nichts heilig ist - auf jeden Fall nicht dieses Prinzip, was bedeutet, dass sie sich in der Tat zur selben Zeit am selben Ort befinden k\xf6nnen.
Man sagt, dass 77% der Kanadier keinen Zugang zur Palliativpflege haben, d. h. zu einer Pflege, die das Leiden von Patienten lindern soll, wenn letztere das Endstadium ihres Lebens erreicht haben, sowohl zu Hause, im Krankenhaus oder in einem Pflegeheim.
Es geht mir darum, den Lesern den Blick hinter die Kulissen zu er\xf6ffnen, den Blick darauf, wem die 95 Jahre Spannung (gerechnet ab der Balfour-Deklaration im November 1917) in dem kleinen Flecken Land im Nahen Osten vor allem dienlich sind.
Ein Kandidat f\xfcr den Sieg in dieser Umfrage ist m\xf6glicherweise die EU-Verordnung vom vergangenen Jahr, der gem\xe4\xdf Luftballons beim Verkauf mit dem Hinweis versehen werden m\xfcssen, dass Kinder unter acht Jahren den Luftballon nicht ohne Aufsicht eines Erwachsenen aufblasen d\xfcrfen.
Winy Maas vom Rotterdamer Architekturb\xfcro MVRDV, Meister der tollk\xfchnen Balkendiagramme und Produzent von witzigen, ja oft zynischen Bauten, nahm die Sache mit gewohnter Gelassenheit und erschien zum Wettbewerbs-Hearing anno 2003 mit f\xfcnf B\xfcchern unterm Arm und einem Grinsen im Gesicht.
"Om'Obani" ist kein einfaches St\xfcck, jede Chorstimme hat einen anderen Text und diesen auch noch in einer sehr fremden Sprache: Zulu, das von elf Millionen Menschen in S\xfcdafrika, Botswana, Lesotho, Malawi, Mosambik und und in Teilen von Swasiland gesprochen wird.
Die Richterin, Oberst Denise Lind, fragte Manning auch, warum er sich nicht \xfcber seine Behandlung beschwerte, als er sich im Januar 2011 mit einem Ausschuss traf, der die von ihm einige Monate vorher auf einem Formular erw\xe4hnten Suizidgedanken untersuchen sollte.
Bei der Befragung am Freitag gab Manning an, er habe aus einem Befehl seiner Wache geschlossen, dass er die Decke, mit der er sich h\xe4tte bedecken k\xf6nnen, fallen lassen sollte. Er gab jedoch zu, dass ihn niemand dazu aufgefordert hatte.
Sie ist sogar so weit gegangen, die Ukraine, Honduras und die Dominikanische Republik zu bezahlen, um die neuen Regelungen anzufechten - jene L\xe4nder beschweren sich bei der Welthandelsorganisation \xfcber ungerechte Handelseinschr\xe4nkungen, obwohl keines der L\xe4nder gr\xf6\xdferen Handel mit Australien betreibt.
Wenn man versucht, sich auf eine schwierige oder anstrengende Aufgabe zu konzentrieren, kann die St\xf6rung der Aufmerksamkeit zu Langeweile f\xfchren, sagt Mark J. Fenske, assoziierter Professor f\xfcr Neurowissenschaften an der Universit\xe4t Guelph in Ontario und einer der Autoren der Studie.
Und unangenehme Praxisfragen m\xfcssen in dieser Zeit gekl\xe4rt werden - etwa, wie die staatliche Vorgabe eines "angemessenen Zugangs" zu lizenziertem Marihuana mit dem Verbot von Cannabisgesch\xe4ften im Umkreis von 300 Metern um Schulen, Parks, Spielpl\xe4tzen und Kinderbetreuungseinrichtungen vereinbart werden soll.
Sowohl mein Vater als auch mein \xe4lterer Bruder hatten jene Universit\xe4t besucht, die ich einst f\xfcr den gr\xf6\xdften Wissenstempel der Welt hielt, f\xfcr ein modernes griechisches Symposion, das die gro\xdfen S\xe4ulen der Zivilisation - freies Denken und Toleranz - f\xf6rderte.
Im vergangenen Oktober war Peru Gastgeber des III. Gipfels S\xfcdamerika - Arabische Staaten (ASPA), und auch bei dieser Gelegenheit wurde trotz nachdr\xfccklicher Aufforderung durch die Presse die so genannte Erkl\xe4rung von Lima, die man vorher angek\xfcndigt hatte, ebenso wenig ver\xf6ffentlicht.
Nachdem die Anzeigen durch die mexikanischen Gewerkschaften f\xfcr Luftverkehr gegen den ehemaligen Eigent\xfcmer Gast\xf3n Azc\xe1rraga Andrade, der einer betr\xfcgerischen Verwaltung beschuldigt wird, mehrere Monate nicht vorw\xe4rts kamen, hat die Asociaci\xf3n Sindical de Pilotos Aviadores (Gewerkschaftsverband der Piloten) endlich Fortschritte gemacht.
Larry Hagman wurde am 21. September 1931 in Forth Worth (Texas) geboren und wurde weltweit ber\xfchmt mit seiner Rolle als John Ross Ewing, besser bekannt als "J.R". in der Fernsehserie "Dallas", wo er einen skrupellosen, heimt\xfcckischen und manipulierenden Gesch\xe4ftsmann spielte.
Als die Antwort in einem Kapitel im November 1990 bekannt wurde, wurde sie von durchschnittlich 41 Millionen Zuschauern gesehen, die "Dallas" in das zweite am meisten gesehene Unterhaltungsprogramm seit dem Ende von "MASH" 1983, das 50 Millionen Zuschauer hatte, verwandelten.
Jacques Duchesneau merkt seinerseits an, dass "Beamte mehrere Hundert Millionen Dollar gestohlen haben", macht sich aber vor allem Gedanken \xfcber die Rolle der "Mandatstr\xe4ger, die \xfcber die Taktik im Bilde sind", wenn sie nicht in den Betrug verwickelt waren!
In der Tat ist das von Satoshi Nakamoto (ein Pseudonym) erfundene Bitcoin sowohl eine virtuelle W\xe4hrung (aber in Dollar, Euro usw. konvertierbar) als auch ein Protokoll f\xfcr den sicheren Austausch wie BitTorrent, das den direkten Austausch von Dateien erm\xf6glicht.
Wenn ein Benutzer zum Betr\xfcgen zwei Mal sehr schnell (weniger als 10 Minuten) mit demselben Geld bezahlen will, w\xfcrde nur eine der beiden Transaktionen vom Netzwerk validiert werden und die andere bleibt ohne Verkn\xfcpfung, da beide unterschiedliche Fingerabdr\xfccke besitzen.
Die Kommentatoren fanden es \xfcbrigens unterhaltsam, dass die einzige Meinungsverschiedenheit des Tages... in der Uhrzeit f\xfcr das Gebet zum Ausdruck gekommen ist, da einige Mitglieder des Gremiums der Meinung waren, dass die Pendeluhr der verfassungsgebenden Versammlung nicht genau ging.
Ein Gesetz muss doch seine G\xfcltigkeit haben, und wenn etwas gesetzlich verboten ist, dann kann doch nicht einfach der Regierungsvorsitzende kommen, und das Kontrollamt, dessen Pflicht nun einmal die Kontrolle der Einhaltung des Gesetzes ist, in seiner T\xe4tigkeit behindern.
Damit ist die gesichtslose Kleinstadtretorte, die bis dato nicht mehr zu bieten hatte als eine postmoderne Fu\xdfg\xe4ngerzone und ein fassungslos h\xe4ssliches Rathaus, hinter dessen wei\xdfen Fassaden man geneigt w\xe4re, eine Molkereifabrik zu vermuten, um ein St\xfcck zeitgen\xf6ssischer Architektur reicher.
"Aber \xd6l ist nicht der einzige Grund, warum es uns so gut geht", sagt Anna, unsere Kellnerin, die runde Tabletts mit reifem Rakfisk verteilt und mit ihrem langen blonden Haar und den stechend blauen Augen das nordische Ideal verk\xf6rpert.
Die Staatsanwaltschaft hat am Freitag versucht, festzustellen, dass der Armeegefreite Bradley Manning - angeklagt f\xfcr die gr\xf6\xdfte Enth\xfcllung vertraulicher Informationen der US-amerikanischen Geschichte - mehrere Gelegenheiten vers\xe4umte, sich \xfcber die von ihm angeblich erlittene Misshandlung in Milit\xe4rhaft zu beschweren.
Einen Tag vor dem Kreuzverh\xf6r, das infolge eines Antrags der Verteidigung zur Abweisung der Anklage abgehalten wurde - Manning sei durch die harte Haftzeit bereits ausreichend bestraft worden - hatte Manning ausgesagt, er h\xe4tte im Gef\xe4ngnis den Suizid erwogen.
In der Anh\xf6rung am Freitag ging Fein mit Manning die Formulare durch, die Beamte nach ihren Treffen mit Manning w\xe4hrend seiner Haft im Quantico-Milit\xe4rgef\xe4ngnis ausgef\xfcllt hatten, wo er von Juli 2010 bis April 2011 unter verst\xe4rkten Haftbedingungen eingesessen hatte.
Die meisten Amerikaner verschwenden vermutlich nie einen einzigen Gedanken daran, dass die Vereinigten Staaten im Jahre 1848 in Mexiko einfielen und die F\xfchrung des Landes unter vorgehaltenem Gewehr dazu zwangen, ihnen mehr als die H\xe4lfte ihres Territoriums zu \xfcberlassen.
Die Personen, die das kaum h\xf6rbare Fernsehen vernahmen, gaben an, mehr Langeweile als die beiden anderen Gruppen zu versp\xfcren - sie hatten Probleme, sich zu konzentrieren, konnten f\xfcr diese keinen Grund finden und schrieben ihre Schwierigkeiten der Langeweile zu.
Der 19-j\xe4hrige Community College-Student und Fu\xdfballspieler Anthony Orozco steht im S\xfcdosten Colorados f\xfcr ein Vergehen vor Gericht, das in diesem Staat schon bald legal sein wird: Der Besitz einiger weniger Marihuanabrocken und einer Pfeife, mit der er diese rauchte.
Dies hat der Designer bei der Er\xf6ffnung von "Valentino - Meister der Couture" anerkannt, einer grandiosen Retrospektive, f\xfcr die mehr als 130 Kleider der Haute Couture zusammengestellt wurden, die von seinem "Maison" in den letzten 50 Jahren geschaffen wurden.
"Es ist unverst\xe4ndlich, dass die interamerikanische Kommission f\xfcr Menschenrechte ihren Sitz in Washington hat und von den Vereinigten Staaten finanziert wird", erkl\xe4rte er als Anspielung auf das politische Asyl, das Ecuador dem Gr\xfcnder von WikiLeaks, Julian Assange, gew\xe4hrt hat.
Ich habe gerade mit dem Vizepr\xe4sidenten von Venezuela, Nicol\xe1s Maduro, gesprochen. Er hat mir gesagt, dass er f\xfcr eine geplante, routinem\xe4\xdfige Behandlung dorthin gereist habe, und dass erwartet w\xfcrde, dass er nach der Wahlkampagne wieder nach Kuba reisen k\xf6nne.
Au\xdferdem wird darauf hingewiesen, dass sich das Land den Prinzipien der Kommission der Vereinten Nationen f\xfcr den internationalen Handel unterworfen hat, d. h. den festgelegten Regeln f\xfcr die F\xe4lle grenz\xfcberschreitender Zahlungsunf\xe4higkeit, die die Gleichstellung von Schuldner und Gl\xe4ubigern garantieren.
Im Vorfeld hat die Canacintra (die nationale Kammer der verarbeitenden Industrie) erreicht, die Gouverneure im S\xfcdosten zu vereinen, um sich der monumentalen Einrichtung zu widersetzen, die zum Teil gesch\xfctzte Gebiete vernichtete und die Mutter aller Bedrohungen der Industrie darstellt.
Er selbst hat mehrere Jahre lang 3% des Wertes der in Montreal erhaltenen Vertr\xe4ge an einen mit der Mafia in Verbindung stehenden Vermittler gezahlt, der das Geld an die Union Montreal \xfcbertrug, die Partei von B\xfcrgermeister G\xe9rald Tremblay.
Die Regierung Quebecs schl\xe4gt vor, die Spenden an Parteien auf 100 Dollar zu beschr\xe4nken, was ihm zufolge nichts an der Situation \xe4ndern w\xfcrde: "Solange die Wahlkampfausgaben nicht streng begrenzt werden, wird Schwarzgeld in der Politik im Umlauf sein."
Die Brille ist ein pers\xf6nliches Gadget und darin liegt ihre St\xe4rke (Privates k\xf6nnen nur Sie sehen), aber gleichzeitig auch ihre Schw\xe4che, denn eine erweiterte Realit\xe4t mittels Brille verhindert, dass Sie gemeinsam mit Anderen an virtuellen Objekten arbeiten k\xf6nnen.
Was die Beh\xf6rden betrifft, so ist das deutsche Pendant zum NK \u2047  der Bundesrechnungshof, der \xe4hnlich aufgebaut ist wie bei uns und ebenfalls \xfcber ein Kollegium verf\xfcgt, das lediglich etwas anders gebildet wird. Grunds\xe4tzlich arbeiten beide Beh\xf6rden jedoch \xe4hnlich.
N\xe4chstes Jahr m\xf6chten wir auch gern im Tschechischen Haus in New York auftreten, und ich pers\xf6nlich - wenn wir dann schon mal in den USA sind - w\xfcrde dies auch gern mit Auftritten in Washington und Chicago verbinden.
Vergangene Woche wurde Polen auf einer Ministerratssitzung der Mitgliedsl\xe4nder der Europ\xe4ischen Weltraumorganisation ESA als zwanzigstes Mitglied dieser Weltraumbeh\xf6rde aufgenommen. Polen ist damit das zweite Mitgliedsland aus dem ehemaligen Ostblock (nach Tschechien, das am 12. November 2008 ESA-Mitglied wurde).
Wer ist der Schuldige und wer das Opfer im Konflikt zwischen Pal\xe4stinensern und Israeliten, wo Unrecht nur Unrecht in einer endlosen Spirale der Gewalt ausl\xf6st, wobei am Anfang die Gier Einzelner und ihr Streben nach globaler Macht stand?
Dadurch wechseln sich im Film die Stimmungsebenen ab - auf der einen Seite die Dokumentarszenen aus Teheran (in der Titelsequenz werden ikonische zeitgen\xf6ssische Fotografien gezeigt, und auch in der Filmfassung der gleichen Situationen gibt es keine gro\xdfen Unterschiede).
Und w\xe4hrend die Jury noch verdutzt um sich blickte und mit den Achseln zuckte, stapelte der freche Maas seine erlesenen Mitbringsel der Gr\xf6\xdfe nach zu einer Pyramide und beendete seine aktionistisch untermauerte Rede mit den Worten: "Liebe Stadtgemeinde!"
Bei einer gemeinsamen Afrika-Reise im Fr\xfchjahr 2005 entdeckte der Chor das Dorf, vor allem aber sahen die Imbongis viele Kinder auf den Stra\xdfen, denen es nicht nur an elterlicher F\xfcrsorge mangelte, sondern schlicht an allem: Essen, Kleidung, Bildung.
Doch dass ausgerechnet die kalorienreiche Kost der Talyschen so gesund sein soll, die Fleisch, Brot und vor allem Milchprodukte lieben und von denen viele t\xe4glich ein Glas geschmolzene Butter trinken, erscheint aus ern\xe4hrungswissenschaftlicher Sicht auch nicht gerade plausibel.
W\xe4hrend der Amtszeit von Gouverneur Pena Nieto wurden im Staat Mexiko \xfcber 1.000 Frauen ermordet - eine Statistik, die selbst die der Stadt Ciudad Juarez \xfcbertrifft, welche f\xfcr ihre Gewalt und die Morde an unschuldigen Frauen ber\xfcchtigt ist.
Bei einem Kreuzverh\xf6r Mannings w\xe4hrend einer vorgerichtlichen Anh\xf6rung in Ft. Meade, Maryland erkl\xe4rte Maj. Ashden Fein, dass Unterlagen zu w\xf6chentlichen Besuchen, die Gef\xe4ngnisbeamte w\xe4hrend Mannings neunmonatiger Haftzeit in Quantico, Virginia vorgenommen hatten, keinerlei Beschwerden \xfcber seine Behandlung aufwiesen.
Einige Gruppen h\xf6rten ein lautes Fernsehprogramm aus dem benachbarten Raum, das nichts mit dem Inhalt zu tun hatte. Andere h\xf6rten es auf niedriger Lautst\xe4rke, sodass es kaum wahrnehmbar war, w\xe4hrend die dritte Gruppe diese Ger\xe4usche \xfcberhaupt nicht vernahm.
Im Jahre 1991 f\xfchrte Reed Larson, Professor f\xfcr menschliche und Gemeinwesensentwicklung an der Universit\xe4t von Illinois, ein Experiment durch, bei dem er fast 400 Teenager und ihre Eltern sieben bis acht Mal am Tag mit einem Pager kontaktierte.
Bei Bezirksstaatsanw\xe4lten handele es sich um eine "kulturelle Barriere", sagt Sean McAllister, ein Rechtsanwalt aus Denver, der f\xfcr Marihuanadelikte vor Gericht stehende Angeklagte vertritt und vor Ort als Sprecher f\xfcr die nationale Organisation zur Reform von Marihuanagesetzen agiert.
Doch innerhalb von zwei Wochen nach meinem Einzug im Worscester College Ende der achtziger Jahre - dort hatte ich vorgehabt, Geschichte zu studieren - hatte ich wieder meine Koffer gepackt und so den ersten Skandal meines Lebens herbeigef\xfchrt.
Wenigstens in den vergangenen 12 Jahren hatten wir keine Versorgungsprobleme bei den Medikamenten. Das Problem ist, dass die Personen in weit fortgeschrittenem Zustand kommen, weil sie ihren Infektionszustand nicht kennen, d. h. in sehr sp\xe4ten Phasen der Krankheit.
Sie sollten den Test machen, wenn sie zur Risikogruppe geh\xf6ren. Je fr\xfcher sie wissen, ob sie HIV-positiv sind, desto besser, und wenn sie die Diagnose bereits kennen, sollen sie lernen, wie man wie alle Menschen verantwortungsvoll leben kann.
Zweitens bestimmt das Urteil, dass ohne die Stimmen der Gesellschaften nach Anerkennung der Verbindlichkeiten in der Konkursmasse, die die Filialen von Vitro mit ihrer Muttergesellschaft hatten, nicht die erforderliche Mehrheit f\xfcr die Umstrukturierung der Verbindlichkeiten erreicht worden w\xe4re.
In der Tat verf\xfcgen 25% der Afro-Amerikaner, 15% der Personen mit einem Einkommen von weniger als $35.000, 18% der B\xfcrger \xfcber 65 Jahre und 20% der W\xe4hler zwischen 18 und 29 Jahren nicht \xfcber den erforderlichen Lichtbildausweis.
Als B\xfcrgermeisterin des Stadtbezirks Rivi\xe8re-des-Prairies, im Osten der Insel, lehnte sie sich ab 2010 gegen den Verkauf eines Gemeindegrundst\xfccks auf, dass f\xfcr 5 Millionen Dollar erworben und f\xfcr 1,6 Millionen an Bautr\xe4ger im boomenden Immobilienmarkt weiterverkauft wurde.
Sie haben sich in Gesch\xe4ftemacher verwandelt, indem sie Grundst\xfccke der Regierung beschlagnahmt haben, um sie als Bauland an Fl\xfcchtlinge aus dem Iran und Pakistan zu verkaufen und so Nutzen aus der massiven amerikanischen Vergabe von Unterauftr\xe4gen zogen.
Zumal dem \xe4gyptischen Volk mit diesem Zur\xfcckgreifen auf eine \xfcbereilte Abstimmung ein Ultimatum gestellt wird: "Entweder stimmt ihr f\xfcr meinen Entwurf oder ich behalte die unbeschr\xe4nkte Vollmacht", letztere sollte nach Annahme der Verfassung vermeintlich ein Ende nehmen.
Der Weg beginnt bei der r\xf6mischen Festung Antonia, Pretorium, wo das Gericht war, und f\xfchrt durch die Stra\xdfen der Altstadt zur Grabeskirche auf dem Berg Golgotha, wo sich die Kreuzigungsstelle, der Salbungsstein und das Grab Jesu befinden.
"In der Heimat wird Ihnen das Eine versprochen, und bei der Ankunft werden Sie betrogen, bekommen ihre P\xe4sse abgenommen und erhalten nicht den versprochenen Lohn", best\xe4tigt der Leiter der Hauptverwaltung f\xfcr Arbeitsmigration der tadschikischen Migrationsbeh\xf6rde, Tolib Schwaripow.
Vielleicht ist es sogar so, dass wir das System auf diese Weise nur mit \xfcberm\xe4\xdfigem "Papierkram" belasten, und diejenigen, die L\xfccken im System suchen, es wesentlich einfacher haben, das System auszunutzen, als wenn die Schwellenwerte h\xf6her blieben.
J.F. Kennedy begann, eigene Banknoten herauszugeben und wollte die FED abschaffen - er wurde 1963 ermordet; der Abgeordnete Louis Mc Fadden wurde 1936 vergiftet, nachdem er die FED wegen Ausl\xf6sung der Weltwirtschaftskrise im Jahr 1929 verklagen wollte.
Israel wurde im Jahr 1948 gegr\xfcndet, und ebenso wie durch die Kriegsreparationen gegen Deutschland der Boden f\xfcr den Zweiten Weltkrieg bereitet wurde, stellt die Ausrufung des Staates Israel die Schaffung des Brennpunktes f\xfcr den Dritten Weltkrieg dar.
Wenn es den internationalen Bankern gelingen wird, diesen Krieg zu entfesseln, wird das j\xfcdische Volk \xe4hnlich wie im Zweiten Weltkrieg zum Opfer in der vordersten Kampflinie, diesmal zusammen mit der arabischen bzw. muslimischen Bev\xf6lkerung des Nahen Ostens.
F\xfcr die amerikanische Regierung gab es aus dieser Situation keinen positiven Ausweg - sie konnte es sich nicht leisten, den Schah \xfcber Bord zu werfen, da dies das Vertrauen ihrer Verb\xfcndeten in anderen L\xe4ndern massiv besch\xe4digt h\xe4tte.
"Auf diese Idee brachte uns der unl\xe4ngst von der EU vorgebrachte Plan, eine Frauenquote von 40% im Management gro\xdfer europ\xe4ischer Firmen einzuf\xfchren", sagte Patrik Nacher, der sich um die Organisation dieser Umfrage k\xfcmmert, gegen\xfcber der Zeitung Pr\xe1vo.
Und obwohl wir vielleicht nun den amerikanischen Traum leben, gute Schulen besucht und gute Jobs erhalten haben, d\xfcrfen wir niemals aus den Augen verlieren, dass es der amerikanische Traum ist, den wir leben - nicht der mexikanische.
Mithilfe solcher Skalen haben Forscher herausgefunden, dass Jungen \xf6fter langweilig wird als M\xe4dchen, so Stephen Vodanovich, Professor f\xfcr Psychologie an der Universit\xe4t Westflorida - insbesondere, was den Bedarf nach mehr und einer gr\xf6\xdferen Vielfalt externer Reize betrifft.
Das verkauft sie dann f\xfcr je 10.000 Rupien (83 Eurocent) an die petrochemische Industrie, weil dieses Mineral im Alltag weitverbreitet ist und zur Herstellung von Streichh\xf6lzern, Feuerwerksartikeln, Kosmetik, Dynamit und sogar zum Bleichen von Zucker verwendet wird.
Er ist in der Lage, bis zu 110 kg zu tragen und versichert, dass er weitermacht, "solange es geht", weil er das Geld f\xfcr die Erziehung seiner drei Kinder im Alter zwischen 10 und 18 Jahren braucht.
"Erreicht werden muss der freie Verkehr der B\xfcrger und Arbeiter in allen s\xfcdamerikanischen L\xe4ndern, wie dies bereits in der Andengemeinschaft der Fall ist;es gibt allerdings noch reaktion\xe4re Sektoren, die eine R\xfcckkehr in die Vergangenheit anstreben", warnte er.
Danach kam die Weltmeisterschaft 1990, bei der wir den vierten Platz belegten, was eigentlich Bronze h\xe4tte sein sollen, wenn nicht dieser kanadische Schiedsrichter gewesen w\xe4re, der uns den letzten Spielzug zum zweiten Mal wiederholen lie\xdf, sagte Reyes.
Dar\xfcber hinaus werden durch diese Gesetze ebenfalls die Zeitr\xe4ume f\xfcr die vorzeitige Stimmabgabe verk\xfcrzt, das Recht f\xfcr ung\xfcltig erkl\xe4rt, sich am Wahltag als W\xe4hler zu registrieren, und Staatsb\xfcrgern das Wahlrecht abgesprochen, f\xfcr die eine Gerichtsakte vorliegt.
Und schlie\xdflich handelt es sich um das letzte Teilchen, dessen Existenz vom Standardmodell - unserer besten oder "am wenigsten falschen" Erkl\xe4rung der Natur und dem Verhalten der Materie - vorausgesagt, aber empirisch noch nicht beobachtet wurde.
Allerdings ist das Higgs-Feld sehr viel stabiler als das elektromagnetische Feld; der Erreger muss sehr hohe Energien erreichen, ein wenig vergleichbar mit einem gefrorenen Teich, dessen Oberfl\xe4che nur von einem sehr gro\xdfen Felsen zerfurcht werden k\xf6nnte.
Herr Zambito hat in den 2000er Jahren \xfcberall seine Hand im Spiel gehabt, indem er mehr als 88.000 Kanadische Dollar (ca. 68.000 Euro) an Provinzparteien gab, vor allem an die damals an der Macht gewesenen Liberalen.
Von der Untersuchung, die letztendlich durchgef\xfchrt wird, sagt sie, dass sie "an einem Faden zieht, der es erm\xf6glicht, die Funktionsweise des von Ameisen unterwanderten Systems zu verstehen, um das \xdcbel zu stoppen und die Schuldigen anzuprangern".
Damit sich die Landwirte von dem von ausl\xe4ndischen Gruppen gef\xfchrten Aufstand befreien, was nach ihren eigenen Aussagen ihr Wunsch ist, w\xe4re die Weiterf\xfchrung geringer, gut kontrollierter und sie direkt betreffender ziviler Hilfen zu ihren Gunsten erforderlich.
In der Stadt kommen Sie zumeist mit dem Bus voran, doch in Jerusalem gibt es auch eine Schnellstra\xdfenbahn und in Haifa die einzige U-Bahn-Linie des Landes mit sechs Stationen, die die Unterstadt mit der Oberstadt verbindet.
Dennoch geben viele B\xfcrger der zentralasiatischen Republiken, die in Russland ihr Geld verdienen wollen, zu, dass sie nicht nur die Sprache des Ziellandes nicht beherrschen, sondern sich auch in ihrer eigenen Sprache kaum schriftlich ausdr\xfccken k\xf6nnen.
In den vergangenen Tagen kam es \xfcberall in den USA zu massiven Protesten gegen niedrige L\xf6hne in Filialen von Walmart und Restaurants beliebter Fast-Food-Ketten wie Mc Donald's, Burger King, Taco Bell, Wendy's und Kentucky Fried Chicken.
Bereits unter den vorherigen Regeln sind die einer Pr\xfcfung unterzogenen Personen gegen\xfcber dem Tr\xe4ger (beispielsweise, im Falle eines operationellen Programmes der Regionalpolitik, dem Regionalrat) dahingehend rechenschaftspflichtig, dass jede Nichteinhaltung des Vergabegesetzes einer Verletzung der Haushaltsdisziplin gleichkommt.
Eine weitere Entwicklungsstufe sollte bereits in der Lage sein, echte wissenschaftliche Arbeit zu leisten - die Rakete RM-34 sollte eine Flugh\xf6he von bis zu 14,5 km erreichen und f\xfcr die Beobachtung von H\xf6henwinden zum Einsatz kommen.
Im gro\xdfen Ma\xdfstab bedeutet dies f\xfcr die meisten Unternehmen, ihre Fertigung ins Ausland zu verlegen oder dort g\xfcnstig einzukaufen, oder aber ihr Gesch\xe4ft aufzugeben. Das Ergebnis ist eine hohe Arbeitslosigkeit in L\xe4ndern mit vergleichbar hohen Arbeitskosten.
Die einzige L\xf6sung sind gezielte politisch-soziale Reformen, die die Kapitalbeteiligung des Staates an der Wirtschaft steigern, den Einfluss der B\xfcrger auf die Regierung erh\xf6hen und die Monopolstellung des Privatkapitals in der Gesellschaft zugunsten des Staates schw\xe4chen.
Das, was weniger augenscheinlich ist, ist die Frage, ob es wirklich immer diese Pers\xf6nlichkeiten selbst waren, die ihre Schritte autonom bestimmten, oder ob hinter ihrem Thron jemand stand, der ihre Taten auf ein vorbestimmtes Ziel lenkte.
Israel ist wie ein riesiges Labor, eine Quelle des Streits und des Chaos, nicht nur im Land selbst, sondern auch international (man denke nur daran, wie scharf sich die Menschen in Anh\xe4nger und Gegner Israels unterteilen).
Verordnungen werden in den Mitgliedsl\xe4ndern zwar leicht zur Zielscheibe der Kritik, die Bem\xfchungen der EU um Regulierung und damit auch um Effektivit\xe4t und Entwicklung der gesamten Europ\xe4ischen Union verdient nach Meinung einiger Experten jedoch eher Anerkennung.
Tschechien konnte zwar nach einem sechsj\xe4hrigen Kampf mit Deutschland und \xd6sterreich die Bezeichnung "Olomouck\xe9 tvar \u2047 ky" verteidigen, den Inl\xe4nderrum (Tuzemsk \u2047  rum), dessen Tradition bei uns bis ins 19. Jahrhundert zur\xfcckreicht, mussten unsere Hersteller jedoch in "Tuzem\xe1k" umbenennen.
Pena Nieto war auch sehr daran interessiert, \xfcber das Wachstum der mexikanischen Wirtschaft zu sprechen. Sie ist ein Grund daf\xfcr, dass Mexikaner heutzutage mit ebenso hoher Wahrscheinlichkeit in Mexiko bleiben, statt in die Vereinigten Staaten auszuwandern.
Unter diesen Projekten w\xe4ren auch f\xfcnf peruanische, die auf den Querachsen seines Gebiets von der K\xfcste nach Brasilien l\xe4gen, und wovon zwei f\xfcr eine bessere Verbindung mit Ecuador sorgen sollen, obwohl er keine weiteren Details gab.
Als Teil des Gipfeltreffens trafen sich auch im Vorfeld die Verteidigungsminister des Blocks zur Verabschiedung des Ma\xdfnahmenplans f\xfcr das Jahr 2013, worin der Dialog und Konsens in Bezug auf die Verteidigung der Region gest\xe4rkt werden soll.
Der Pr\xe4sident Ecuadors bef\xfcrwortete au\xdferdem die Neugestaltung der Organisation amerikanischer Staaten (OEA) unter der Vorgabe, den Einfluss der angels\xe4chsischen Staaten zu verringern und jene zu ber\xfccksichtigen, die das Abkommen von San Jos\xe9 \xfcber Menschenrechte unterzeichnet haben.
Allerdings kommen noch immer viele Personen in die Klinik, die nichts von ihrer Krankheit wissen und bei denen das Virus bereits Schaden angerichtet hat und ihr Immunsystem ersch\xf6pft hat, und die Opfer von opportunistischen Infektionen sind.
Danach hat sich die Aufsichtsbeh\xf6rde systematisch geweigert, die Hauptverwaltung der Republik \xfcber eine vom Unternehmer durchgef\xfchrte Transaktion zu informieren, um vom Treuh\xe4nderkonto F/589 der Bank IXE auf den Namen Mexicana de Aviaci\xf3n 198 Millionen Pesos abzuheben.
Mit Spielern wie "Canito" Nieves, Pablo Alicea und dem jungen Rolando Hourruitiner als Ersatz f\xfcr die gesperrten Spieler wegen der Vorkommnisse auf den Panamerikanischen Spielen in Mar del Plata, gewannen wir entgegen jeder Prognose die Goldmedaille.
Stattdessen haben Sie die Wahl zwischen verschiedenen Gerichten mit Hammel- und Rindfleisch, Suppen und Desserts (zubereitet mit Kokosmilch), traditioneller j\xfcdischer Humus-Paste, verschiedenen So\xdfen, frittierten B\xe4llchen aus p\xfcrierten Bohnen und Erbsen (Falafel) sowie Fr\xfcchten und Gem\xfcse.
An diesem Tag legten einige Walmart-Mitarbeiter, von denen es weltweit 2,2 Millionen gibt, ihre Arbeit nieder und bestreikten zusammen mit Gewerkschaften und linken Aktivisten Filialen der Kette, deren Zielgruppe Personen niedrigen und mittleren Einkommens sind.
Auf der erlesenen Liste landeten bereits hochrangige Vertreter der Petersburger Kunstszene, deren Erfolge \xfcber die Grenzen der Stadt hinaus gehen und die oft Anerkennung in Europa finden, ohne im Rest von Russland bekannt zu sein.
Gerade eine solche gemeinsame Kontrolle k\xf6nnte dazu beitragen, dass wir aufh\xf6ren, uns st\xe4ndig um eine Perfektionierung der Gesetze und die Senkung und Austarierung von Schwellenwerten zu bem\xfchen, wenn sich dies augenscheinlich nicht besonders positiv auswirkt.
Auch die Kompetenzen sind zu einem gewissen Ma\xdfe vergleichbar, wobei Deutschland jedoch ein Bundesstaat ist, d.h. dass es diese Rechnungsh\xf6fe auch in den einzelnen Bundesl\xe4ndern gibt - darin unterscheidet sich das deutsche System von unserem.
Mit unserer Band The Tap Tap machen wir uns eher dar\xfcber lustig und sagen, dass wir die einzige Band der Welt sind, die gen\xfcgend positive Energie sammeln kann, um den Weltuntergang aufzuhalten oder zu verhindern.
Manche kommen zu uns mit romantischen Vorstellungen, und wenn sie dann feststellen, dass sie zweimal die Woche Probe haben, Vorbereitungsphasen absolvieren m\xfcssen und viel Zeit auf Konzertreisen verbringen, dann erlischt die Begeisterung bei vielen schnell.
Im Jahr 1937 tauchte in der Fachpresse der von Ing. Rohozi \u2047 ski stammende Entwurf einer fotoelektrischen Jagdrakete auf, und im darauf folgenden Jahr erschien das Werk "Rakieta - torpeda powietrzna i rakietobomba lotnicza" des Autors Leliwa-Krzywoblocky.
Bereits in ihren Anf\xe4ngen im Jahr 1956 bem\xfchte sich die Polnische Raumfahrtgesellschaft PTA um einen Beitritt zu der 1951 gegr\xfcndeten Internationalen F\xf6deration f\xfcr Raumfahrt, und tats\xe4chlich wurde die PTA bereits im Herbst 1956 ordentliches Mitglied.
Meine Gedanken st\xfctzen sich teilweise auf zug\xe4ngliche historische Fakten, andere sind von diesen abgeleitet und gehen aus meinem eigenen Verst\xe4ndnis davon hervor, wer bzw. welche Gruppe von Menschen die Ereignisse der modernen Geschichte ma\xdfgeblich beeinflusst.
Unter diesen astronomisch reichen Familien sticht eine besonders hervor, die man als Kopf des Kraken bezeichnen k\xf6nnte (ich wei\xdf nicht, ob \xfcber ihnen noch jemand steht, ich schlie\xdfe dies aber nicht aus) - die Rothschilds.
Die Methode, mit denen die Gruppe der reichsten Familien mit den Rothschilds an der Spitze arbeitet, ist die Ausl\xf6sung einer Krise und das anschlie\xdfende Angebot einer L\xf6sung (order ab chao - Ordnung aus dem Chaos).
F\xf6rdergelder f\xfcr Antr\xe4ge auf F\xf6rdergelder bot den Gemeinden das Ministerium f\xfcr Regionalentwicklung unter Leitung von Minister Pavel N \u2047 mec (US-DEU) an, konkret sollte es sich dabei um Mittel f\xfcr die Aufsetzung von F\xf6rdergeldantr\xe4gen an Br\xfcssel handeln.
Ein ernsteres Problem sind nach Meinung dieser Experten eher die EU-F\xf6rdergelder f\xfcr Projekte, die rein gar nichts mit der Vertiefung der europ\xe4ischen Integration gemeinsam haben, die jedoch bei den Haushaltsverhandlungen von einzelnen Mitgliedsl\xe4ndern erzwungen wurden.
Sobald also ein US-Regierungsbeamter auch nur mildeste Kritik an Mexiko \xfcbt, h\xf6rt man - in der mexikanischen Presse und unter den Eliten des Landes - Beschwerden dar\xfcber, wie die Amerikaner die Souver\xe4nit\xe4t ihres Nachbarlandes bedr\xe4ngen.
Eine Reihe australischer Gesetze hat Tabakkonzerne aus der TV-Werbung verbannt, es ihnen untersagt, als Sportsponsoren aufzutreten und die meisten H\xe4ndler dazu gezwungen, Zigaretten in Gesch\xe4ften nicht l\xe4nger auszulegen. Jetzt ist die Tabakwerbung ins Internet gewechselt.
Nachdem der Polizeibeamte Marihuana im Auto gefunden hatte, wurde Orozco f\xfcr den Besitz von Drogen und Drogenutensilien vorgeladen - Kavaliersdelikte, die jeweils mit einer Strafe von 100 US-Dollar versehen sind - und erhielt einen Gerichtstermin.
In Washington ist man der Ansicht, dass Colorado in jedem Falle den meisten Staaten voraus ist, was die Regulierung von Marihuana betrifft. Dort wurde die Droge erst zu medizinischen Zwecken und dann zum Eigenkonsum legalisiert.
"Nirgendwo wird es schwerer sein, einen Standort f\xfcr ein lizenziertes Cannabisgesch\xe4ft zu finden als in Stadtgebieten, insbesondere im Ballungsgebiet von Seattle", meint Ben Livingston, Sprecher f\xfcr das "Center for Legal Cannabis", einer k\xfcrzlich gebildeten Forschungsgruppe.
Obwohl 55% der W\xe4hler in Colorado die Ma\xdfnahme unterst\xfctzten, war schon von Anfang an deutlich, dass es nicht einfach sein w\xfcrde, den pers\xf6nlichen Konsum von Marihuana mit den Komplexit\xe4ten von Regierung und Rechtssystem zu vereinbaren.
W\xe4hrend F\xfcrsprecher und Staatsbeamte sich auf ein Zeitalter legalen Verkaufs vorbereiten, warten sie gleichzeitig auch nerv\xf6s auf Anweisungen der Bundesregierung, welche den Verkauf und den Anbau von Marihuana auf Bundesebene weiterhin als Straftat behandeln will.
Der 27 j\xe4hrige Anto setzt seit drei Jahren sein Leben am Kawah Ijen aufs Spiel, dessen Schwefel beim ihm bereits die ersten Spuren hinterlassen hat, obwohl er sein Gesicht mit einer Maske und Spezialbrille abdeckt.
Danach sendete das Pr\xe4sidentenamt von Peru den Medien eine E-Mail mit der "Abschlusserkl\xe4rung" des Gipfeltreffens, wobei es sich aber um die Erkl\xe4rung von Humala handelte und nicht um das offizielle Dokument zum Abschluss des Gipfeltreffens.
"Seitdem er sich in unserer Botschaft befindet, habe ich nicht mit ihm gesprochen, die Botschafterin hat mich allerdings informiert, dass er ein leichtes Problem mit den Lungen hat, aber kein schwerwiegendes", sagte das Staatsoberhaupt Ecuadors.
"Die L\xf6sung f\xfcr dieses Problem liegt in H\xe4nden von Gro\xdfbritannien, Schweden und den juristischen Beh\xf6rden Europas , weil der Anwalt von Assange, Baltazar Garz\xf3n, eine Reihe von Verfahren auf verschiedenen europ\xe4ischen Instanzen f\xfchrt", erkl\xe4rte er.
Correa nutzte die Gelegenheit, um sich als Verteidiger der Pressefreiheit zu best\xe4tigen und sagte, dass das, was er nicht toleriere, " die Mittelm\xe4\xdfigkeit, die b\xf6se Absicht und die L\xfcge sind, die die freie Meinungs\xe4u\xdferung entkr\xe4ften."
Allein in Jalisco starben im Jahr 2011 255 Personen, und bis zum Monat Mai dieses Jahres sind es bereits 187 Todesf\xe4lle; allerdings wird versichert, dass es seit 2005 universellen Zugang zu den antiretroviralen Arzneimitteln gibt.
Wie Sie wissen, sprechen wir von einem riesigen Verkaufs- und Vertriebszentrum in Mexiko, Zentralamerika und der Karibik mit Produkten aus dem Land jenseits der Mauer, erg\xe4nzt um einen Wohnbereich f\xfcr die Mitarbeiter von 150 Unternehmen.
Die emotionalsten Erinnerungen sind jene, die an seine Zeit bei den Vaqueros von der Mitte der 50er Jahre als Spieler bis 1982 erinnern, wo er sein 15-j\xe4hriges Jubil\xe4um als Mitgesch\xe4ftsf\xfchrer oder Gesch\xe4ftsf\xfchrer des Clubs feierte.
Mein Favorit ist aber die Mannschaft der panamerikanischen Spiele 1991 in Kuba, wo wir Gold gewannen und dem Team der USA einen Kampf boten, wie damals, als sie gegen uns bei der Weltmeisterschaft Bronze gewannen.
Der Werbespruch "Wer schoss auf J.R.?", die Erwartung f\xfcr eine Episode voller Emotionen schaffen sollte, wo die Figur von Hagmann fast get\xf6tet wurde, f\xfchrte zu einer internationalen Spekulation, und Millionen Dollar wurden in Wetth\xe4usern gewettet.
Seit dem Monat Oktober ist ein Manifest im Umlauf, das von prominenten Pers\xf6nlichkeiten der Palliativpflege wie Dr. Balfour Mount und Dr. Bernard Lapointe unterzeichnet wurde, um ihren Widerspruch zu einer derartigen Initiative zu bekunden.
Beamte des Stra\xdfenbauamtes, Unternehmen des Bauhauptgewerbes, Geldbeschaffer politischer Parteien und Spezialisten der italienischen Mafia erz\xe4hlen jeden Tag, was sie \xfcber ein gro\xdfartiges "System" wissen, in dem Bauwirtschaft, Beamte, Politiker, Gewerkschafter und Mafioso verstrickt sind.
Die Chinesen haben die Kupfermine von Mes Aynak bereits fast verlassen, lassen die internationalen Arch\xe4ologen (finanziert von der Weltbank) auf der riesigen buddhistischen St\xe4tte ihre Ausgrabungen machen und bleiben die wichtigsten Arbeitgeber der Provinz.
Die meisten Juristen, die an diesem Text gearbeitet haben, sind keine Ulema, sondern Akademiker, die zum Teil im franz\xf6sischen System ausgebildet worden sind", beschwichtigt Alexis Blouet, der eine Doktorarbeit \xfcber die \xe4gyptische Verfassungstransition schreibt.
Von Januar bis Oktober 2012 kamen 118,8 Tausend ukrainische Touristen ins Gelobte Land, was gegen\xfcber dem Vergleichszeitraum im Jahr 2010 einem Anstieg von 51% entspricht, vor der Aufhebung der Visumspflicht am 9. Februar 2011.
"Die Polizei wei\xdf nat\xfcrlich \xfcber alles Bescheid und f\xfchrt deshalb, wenn sie den Plan zur Aufdeckung von Verbrechen nicht einhalten kann, periodisch Kontrollk\xe4ufe bei H\xe4ndlern durch, die illegale Waffen anbieten", f\xfcgt der Verkaufsberater hinzu.
Die Proteste gingen diese Woche in New York weiter, wo ihr Ziel jedoch nicht Walmart-Filialen (die in dieser fortschrittlichen Stadt nicht erw\xfcnscht und deshalb bisher inexistent sind), sondern McDonald's und andere preisg\xfcnstige Restaurants waren.
Dabei m\xf6chten wir nicht nur ausreichend positive Energie sammeln, um den Weltuntergang zu verhindern, sondern wir m\xf6chten auch zusammen mit der \xd6ffentlichkeit dar\xfcber nachdenken, in welchem Zustand wir diese Welt einmal unseren Kindern \xfcbergeben.
Die globalen Machtgel\xfcste der Rothschilds f\xfchrten in den Jahren 1859 - 1871 zur Formulierung eines Plans zur Entfesselung von drei Weltkriegen durch Albert Pik, einen Freimaurer des 33. und damit h\xf6chsten Grades der Erkenntnis.
Ende des 19. Jahrhunderts initiierten die Rothschilds die Gr\xfcndung der zionistischen Bewegung, bei der ein Zweig die Gr\xfcndung eines Judenstaates anstrebte, m\xf6glichst auf dem historischen Gebiet Jud\xe4as mit Jerusalem als Hauptstadt (R\xfcckkehr nach Zion).
Afflecks Film verliert dadurch etwas an Zugkraft. Es ist ein Film, den man mit gewissem Interesse verfolgen und dabei die Gestaltung und den an einen Thriller aus den 70. Jahren erinnernden Retro-Stil goutieren kann.
Die Organisatoren der Umfrage waren auch von der Idee beeindruckt, dass bestimmte L\xe4nder Geld daf\xfcr erhalten sollten, dass sie kein Meer haben, oder aber von der Idee, F\xf6rdergelder f\xfcr Antr\xe4ge auf F\xf6rdergelder zu geben.
Das legt zumindest ein neu hinzugef\xfchrter Artikel nahe: In allen die Scharia betreffenden Angelegenheiten m\xfcsse die Al-Ashar-Universit\xe4t zurate gezogen werden, die wichtigste islamische Institution des Landes mit gro\xdfer Strahlkraft in den gesamten sunnitischen Islam.
Selbst an besseren Tagen ist dies eine stets verstopfte Stadt, doch am Montag wurde ein Ring aus Stahl errichtet, der mehrere wichtige Verkehrsrouten in die Hauptstadt absperrt und auf den Stra\xdfen f\xfcr Chaos sorgt.
Manning sagte am Donnerstag zu seiner Verhaftung und Verlegung nach Kuwait aus, wo er ann\xe4hernd zwei Monate festgehalten wurde, bevor er im Juli 2010 in das Gef\xe4ngnis der Marinebasis Quantico in Virginia verlegt wurde.
Obwohl mehrere Hamas-F\xfchrer get\xf6tet und die 1,7 Millionen Einwohner des Gazastreifens in einem der desolatesten und dicht bev\xf6lkertesten Ecken des Planeten eingepfercht werden, ist es Israel bis jetzt nicht gelungen, die Hamas zu vernichten.
Und insbesondere der Aufstieg der Muslimbruderschaft unter Pr\xe4sident Muhammad Mursi in \xc4gypten - dem mit Abstand einwohnerst\xe4rksten und wichtigsten arabischen Land - an der s\xfcdlichen Flanke Israels hat das Gleichgewicht der Region nachhaltig ver\xe4ndert.
Cavaliere di Gran Croce (die h\xf6chste Auszeichnung Italiens), Cavaliere del Lavoro, Commandeur de L'Ordre des Arts et des Lettres, ausgezeichnet mit der Ehrenlegion, kumuliert Garavani so viele Ehren, wie jeder der Ehem\xe4nner seiner Kundinnen.
Selbst wenn diese neuen Regeln den Weg zu einem Anstieg der nationalen Geburtenrate bereiten k\xf6nnten, ist den Gespr\xe4chen mit den Singapurern, die im Finanzviertel arbeiten, zu entnehmen, dass sie keine gro\xdfe Wirkung haben werden.
Das 6. Gipfeltreffen der Pr\xe4sidenten der Union S\xfcdamerikanischer Nationen (Unasur) endete heute in Peru ohne Ver\xf6ffentlichung der Erkl\xe4rung von Lima, die vorher angek\xfcndigt wurde und theoretisch von den sieben anwesenden Regierenden unterzeichnet werden sollte.
Einfach gesagt, bedeuten die obigen Ausf\xfchrungen, dass, wer im Alter von 25 Jahren die Diagnose HIV-positiv erh\xe4lt, in diesem Sinne "problemlos 75 Jahre alt werden kann, solange er unter Kontrolle steht", erkl\xe4rte dieser Fachmann.
Eine Mannschaft, die vielleicht in Bezug auf Pers\xf6nlichkeiten nicht die Beste war, mit der wir aber eine Goldmedaille gewannen und die uns gro\xdfe Freude bereitete, war jene des vorolympischen Turniers 1995 in Neuqu\xe9n, Argentinien.
Hagman, der dieses Jahr als J.R. in einer neuen Staffel von "Dallas" zur\xfcckkam, starb Freitag Nachmittag aufgrund von Krebskomplikationen gem\xe4\xdf einer Pressemitteilung der Familie an The Associated Press durch Warner Bros., Produzent von "Dallas".
Hagman interpretierte die Rolle des Ewing als einen korrupten, uners\xe4ttlichen Mann mit einem charismatischen L\xe4cheln: ein hinterh\xe4ltiger Gesch\xe4ftsmann und untreuer Ehemann, der danach strebte, seine alkoholkranke Ehefrau Sue Ellen (Linda Gray) einweisen zu lassen.
Dar\xfcber hinaus scheint dies durch neue Daten best\xe4tigt zu werden, die in dieser Woche auf einem gro\xdfen Physik-Kongress in Kyoto vorgestellt wurden, aber es fehlen noch Daten, um dar\xfcber vollkommen sicher zu sein.
Wenn n\xe4mlich ein Teilchen mit einer elektrischen Ladung beschleunigt oder die Richtung \xe4ndert, wird das elektromagnetische Feld genau an diesem Ort "gest\xf6rt", in etwa wie ein Kieselstein, der in einen Teich geworfen wurde.
"Sie gaben mir f\xfcnf Jahre zu leben, ich habe sieben Jahre geschafft", sagte er halbherzig, in seinem Bett im Heim f\xfcr Palliativpflege Victor-Gadbois in Beloeil liegend, in dem er am Vortag angekommen war.
Dr. Martel glaubt, dass 90% der Patienten, die gebeten haben zu sterben, dem Pflegepersonal danken, dass es diesem Wunsch nicht stattgegeben hat, nachdem ihre Schmerzen von einem Team der Palliativpflege gelindert worden sind.
Die Gesamtheit der Pr\xfcfungsstellen wird unter der \xc4gide des Puschkin-Instituts f\xfcr die Russische Sprache, der Russischen Universit\xe4t der V\xf6lkerfreundschaft, der Moskauer Staatlichen Universit\xe4t, der Sankt Petersburger Staatlichen Universit\xe4t und anderer russischer Hochschulen stehen.
"Das Problem besteht darin, dass das K\xfcken Halt finden muss; es muss auf seinen Beinen stehen k\xf6nnen und anfangen, sich zu bewegen", erl\xe4utert der Laborleiter des Instituts f\xfcr medizinisch-biologische Probleme RAN, Wladimir Sychew.
"Zweimal lie\xdfen wir K\xfcken schl\xfcpfen und stellten das Ganze dann ein, weil es einfach unm\xf6glich ist, dort mit ihnen zu arbeiten", h\xe4lt Wladimir Sychew zum gescheiterten Experiment mit den K\xfcken im All fest.
Allgemein w\xfcrde ich dies ohne konkrete Angaben nur ungern vergleichen. Nichtsdestoweniger wird Deutschland in gewisser Hinsicht oft als Vorbild bezeichnet, wobei man aber bestimmt nicht sagen kann, dass Deutschland in allem besser ist.
Auf einigen Stra\xdfen Ostb\xf6hmens besteht Gefahr wegen Eisgl\xe4tte, in h\xf6heren Lagen und in den Bergen liegt auf den Stra\xdfen mitunter noch eine ausgefahrene Schneeschicht, teilt die Stra\xdfen- und Autobahndirektion auf ihren Internetseiten mit.
Es ist aber nicht gerade \xfcblich, dass sich dort eine gr\xf6\xdfere Gruppe behinderter Menschen aktiv am gesellschaftlichen Geschehen beteiligt, darin sind wir mit der Band The Tap Tap dem Westen ein wenig voraus!
Der Erste Weltkrieg endete mit der pl\xf6tzlichen, milit\xe4risch und \xf6konomisch unbegr\xfcndeten Kapitulation Deutschlands (f\xfcr die Vernichtung des russischen Zarenreiches war der Krieg nicht mehr erforderlich), anschlie\xdfend erfolgte die Aufl\xf6sung der mitteleurop\xe4ischen Gro\xdfmacht \xd6sterreich-Ungarns.
Emotionen ruft hierzulande auch die Tatsache hervor, dass Tschechien \xe4hnlich wie andere Mitgliedsl\xe4nder in Br\xfcssel um das Recht auf Verwendung spezifischer Bezeichnungen traditioneller Produkte k\xe4mpfen muss und diesen Kampf dabei nicht immer gewinnt.
Manche von ihnen haben bis zu 14 Waisen bei sich aufgenommen, geben ihnen ein Dach \xfcber dem Kopf und sorgen daf\xfcr, dass die Kinder in ihren Uniformen jeden Tag p\xfcnktlich zum Schulunterricht erscheinen.
Das Hotel, in dem ich logiere, ist einer von mehreren Veranstaltungsorten, die ein Rakfisk-Dinner organisieren, bei dem G\xe4ste f\xfcr den besten - oder vielleicht die Geruchssinne am st\xe4rksten herausfordernden - Fisch stimmen k\xf6nnen.
Um die Stadt zu erreichen, kann man auf einer der Autobahnen fahren, die Pena Nieto bauen lie\xdf und die eine gro\xdfe Verbesserung gegen\xfcber den br\xfcchigen, holprigen Stra\xdfen darstellen, die es hier einmal gab.
Als Fein ihn am Freitag zu den Formularen befragte, gab Manning zu, dass er die Behandlung durch seine Wachen als "exzellent" und die Behandlung durch die Einrichtung insgesamt als "sehr professionell" beurteilt hatte.
Am Donnerstag hatte Manning ausgesagt, dass er in der vorherigen Nacht dazu gezwungen wurde, nackt zu schlafen. Er h\xe4tte zuvor versucht, einem Beamten zu zeigen, dass er keine Gefahr f\xfcr sich selbst darstelle.
Seine Anw\xe4lte hoffen, dass die Richterin seine Hafterlebnisse zumindest ber\xfccksichtigen und sein Haftma\xdf drastisch verringern werde, sollte er bei seiner Verhandlung vor dem Milit\xe4rgericht verurteilt werden. Diese ist f\xfcr Anfang n\xe4chsten Jahres angesetzt.
Man muss sich die Frage stellen: Ist das blo\xdf eine Privatperson, die so gro\xdfen Gefallen an Marlboro-Zigaretten findet, dass sie daf\xfcr sogar ein Video aufnimmt - oder hat eine Marketing-Agentur damit zu tun?
Sie warten auf eine Orientierungshilfe zur Einrichtung eines Lizenzsystems f\xfcr die Produktion, Herstellung, den Vertrieb und den Verkauf der Droge - und haben dabei eine Frist bis zum 1. Dezember 2013 vor Augen.
Das Washingtoner Gesetz, genannt I-502, tritt am 6. Dezember in Kraft und bildet damit auch den Endpunkt einer Grauzone, in der das staatliche Lizenzsystem zwar noch nicht existiert, aber der Besitz legalisiert ist.
Der organisierte und steigende Hass auf Tory-Studenten in Oxford hat mittlerweile derartige Dimensionen entwickelt, dass eine Gruppe von ihnen letzte Woche den gleichen Gleichberechtigungsschutz forderte, der Schwulen, Behinderten und ethnischen Minderheiten zugute kommt.
Er teilt sich eine schmutzige Holzh\xfctte mit anderen Tr\xe4gern und steht jeden Morgen um zwei Uhr auf, weil der Schwefel auch nachts ausstr\xf6mt, wo seine charakteristische gelbe Farbe in der Dunkelheit bl\xe4ulich gl\xe4nzt.
Jeden Tag brechen er und seine Gef\xe4hrten 15 Tonnen Schwefel aus dem Vulkan, die von drei LKWs \xfcber einen Ziegenpfad zwischen dem Geb\xfcsch zum Lager in Tamansari in 18 Kilometern Entfernung transportiert werden.
In Singapur gibt es Webseiten, wo die kaum kaschierte Xenophobie gegen viele neue Zuwanderer bl\xfcht, besonders gegen die Chinesen, die daf\xfcr kritisiert werden, dass sie die L\xf6hne niedrig halten und sich nicht integrieren.
Er schlug vor, diese ineffiziente Verteilung neu zu orientieren; die Kondome sollen sich nicht nur hinter dem Ladentisch befinden, sondern in Ausgabeger\xe4ten in \xf6ffentlichen Toiletten von Einrichtungen, die h\xe4ufig von Jugendlichen besucht werden.
"Unser erstes Projekt behandelte die Prophezeiung der Mayas, und auf bestimmte Art und Weise diskreditieren wir sie", sagte Julie Zeglen, Student im letzten Jahr in Temple, 21 Jahre alt und aus West Chester.
Er merkt allerdings an, dass in der westlichen Gesellschaft eine apokalyptische Angst besteht, die mehrere Jahrhunderte zur\xfcckf\xfchrt, als die Leute auf \xc4nderungen in ihrer Umgebung mit der Vorhersage des Endes der Welt reagierten.
Gehen wir trotzdem davon aus, dass es sich tats\xe4chlich um das Higgs handelt, da scheinbar nur ein geringes Risiko besteht, sich zu t\xe4uschen, und schauen wir uns an, um was es geht.
Man muss sagen, dass letzteres noch gro\xdfe M\xe4ngel aufweist, da es keine Erkl\xe4rung f\xfcr die Schwerkraft (ups!) und die dunkle Materie bietet, die ca. 80% der Materie des Universums bildet (erneut ups!).
"Seit dem Beginn der Untersuchung im Jahr 2010", betont er, "h\xe4tte allein das Verkehrsministerium eine Milliarde Dollar an den Vertr\xe4gen gespart", denn einige z\xfcgelten dabei ihren Instinkt, um ihren Anteil zu erhalten!
Der neue Kooperationsvertrag sieht die Fortsetzung traditioneller Hilfen vor: M\xe4dchen- und Jungengymnasien, Institut f\xfcr Franz\xf6sisch an den Universit\xe4ten, Franz\xf6sisches Institut, Zusammenarbeit im milit\xe4rischen, rechtlichen, medizinischen und landwirtschaftlichen Bereich, Unterst\xfctzung der arch\xe4ologischen Delegation.
Stephen Betishes entwickelte in unserem Labor in Redmond einen Ber\xfchrungssensor mit einer regulierbaren Verarbeitungsverz\xf6gerung zwischen 1 bis 100 Millisekunden, wobei die heutigen kommerziellen Sensoren n\xe4her am zweiten Wert liegen (60 bis 100).
Vor Kurzem schnappte er sich eine Drehorgel und wurde zum Petersburger Drehorgelspieler, da er sich f\xfcr diese schwierige Rolle im Hinblick auf sein K\xfcnstlerdasein, seine Philosophie und sein Image endlich bereit f\xfchlte.
Es gibt einen Zusammenhang zwischen der Tatsache, dass ein Kind sich etwa 9 Monate im Bauch der Mutter im Fruchtwasser befindet, und dem, dass es sich dann leichter an Wasser gew\xf6hnen kann.
Anl\xe4sslich des Endes des Maya-Kalenders haben wir auch eine einzigartige Kollektion von Schuhen, T-Shirts, Taschen und Schl\xfcsselanh\xe4ngern gegen den Weltuntergang entwickelt, mit deren Kauf \xfcber www.e-tap.cz uns die Leute ebenfalls unterst\xfctzen k\xf6nnen.
Im Zuge der Steigerung der Konkurrenzf\xe4higkeit der deutschen Wirtschaft kommt es regelm\xe4\xdfig zu F\xe4llen, in denen Arbeitnehmer einen derart geringen Lohn erhalten, dass der Staat ihr Einkommen bis zum Existenzminimum aufstocken muss.
Abraham Lincoln lehnte es ab, den Status von Rothschilds Bank of America als Zentralbank zu erneuern, begann w\xe4hrend des B\xfcrgerkrieges, eigene (sprich: staatliche) Banknoten herauszugeben und wurde 1865 in einem Theater ermordet.
F\xfcr deren Freilassung forderten sie die Auslieferung des gest\xfcrzten Schahs Mohammad Reza Pahlavi, der nach der Revolution in die USA geflohen war, die \xfcber Jahrzehnte das Patronat \xfcber sein Regime gewahrt hatten.
Alan Arkin und John Goodman sind in ihren Rollen als Hollywood-Mitarbeiter zwar sehr charmant, ihre Figuren h\xe4tten aber mehr Raum verdient, und damit stehen sie in dem Film bei weitem nicht allein.
Als Erinnerung an ein bis heute auf gewisse Weise lebendiges St\xfcck Geschichte und als Beweis dessen, wie \xfcberzogen doch die Vorstellungen von den allm\xe4chtigen und allwissenden Geheimdiensten sind, ist er jedoch ausreichend.
Und da ich schon \xfcber 40 bin, und dazu unabh\xe4ngig und parteilos, habe ich keine andere M\xf6glichkeit, die Dinge zu beeinflussen, als f\xfcr das Amt eines Senators oder des Pr\xe4sidenten zu kandidieren.
Pattlochs F\xe4lle aber sind anders: Im Auftrag seiner Mandanten geht er dagegen vor, dass chinesische Unternehmen vom Markenamt ganz offiziell das Recht erhalten, eine Bezeichnung zu nutzen, die bereits anderswo gesch\xfctzt ist.
Wer niemanden mehr hat, kommt ins Schutzhaus zu Khanyisile, einer alleinstehenden Frau, die genauso vom Verein bezahlt wird wie die beiden K\xf6chinnen, die jeden Tag f\xfcr mehr als 200 hungrige Kinder kochen.
Ein Bus voller Wei\xdfer, die Lieder in einer schwarzen Sprache singen - so viel Anerkennung bringt nicht nur Stimmung und Freude, sondern hat auch schon manchen grimmigen Grenzsoldaten ein paar Tr\xe4nen abgetrotzt.
Unter der scheidenden Regierung Felipe Calderons hat sich Mexiko wirtschaftlich gut bew\xe4hren k\xf6nnen, doch das Land ist im Griff eines Drogenkriegs, der in den letzten sechs Jahren bereits 60.000 Menschenleben gekostet hat.
Selbst wenn die Islamisten, die nun in \xc4gypten und in anderen L\xe4ndern an der Macht sitzen, wenig f\xfcr Israel \xfcbrig haben, werden sie sich zun\xe4chst auf die Schwierigkeiten im eigenen Land konzentrieren.
Die richtige Antwort ist jene, die von den vern\xfcnftigeren Vertretern beider Seiten, dem Gro\xdfteil der restlichen Welt und von dieser Zeitung vertreten wird: Zwei Staaten, bei denen Israel zu Sicherheitszwecken Gebiete abtritt.
Aber Professor Eastwood glaubt, obwohl diese beiden Zust\xe4nde in Zusammenhang stehen k\xf6nnten, sehen gelangweilte Personen das Problem in ihrer Umgebung oder der Welt, w\xe4hrend depressive Personen das Problem in sich selbst sehen.
Auf der Skala finden sich Aussagen wie "Viele Dinge, die ich tun muss, wiederholen sich und sind monoton" und "Ich habe so viele Interessen, dass ich nicht genug Zeit f\xfcr alles habe".
Wer seinem gelangweilten Kind also ein iPad reicht, kann es damit zwar von der Langeweile abbringen. Es hat damit jedoch nicht gelernt, sich selbst zu unterhalten oder zu kontrollieren, sagt Professor Fenske.
"Wir alle freuten uns, wenn wir in sein Haus in Gstaad eingeladen wurden", erkl\xe4rt die Exfrau von "Heini" Thyssen, eng befreundet mit vergessenen Sch\xf6nheiten wie z. B. Marella Agnelli oder Eugenie Niarchos.
Die Gesellschaft ist PT Candi Ngrimbi, die seit 1960 die Vorkommen im Vulkan und (nie besser gesagt) seine Arbeiter ausnutzt, denen sie 662 indonesische Rupien (5 Eurocent) f\xfcr jedes Kilo Schwefel zahlt.
Es erscheint unglaubhaft, dass die Verse Teil einer Werbung f\xfcr Minzbonbons sind, aber dennoch - oder gerade deswegen - wurden sie anfangs dieses Jahres in Singapur zu einem viralen Video auf YouTube.
Er gibt allerdings zu, dass die neuen Normen den Entwicklern klarere Orientierungen geben, denen vorher Hindernisse in den Weg gelegt wurden, wenn sie zu viele kleine Wohneinheiten innerhalb eines Projekts bauen wollten.
Marielos Porras, Lehrerin f\xfcr Englisch mit Hochschulabschluss in Erziehung und Lernen, meint, dass um die Kinder und Jugendlichen zu orientieren, verstanden werden muss, dass es Zweck der sozialen Netzwerke ist, zu informieren.
Das Staatsoberhaupt verlas das Abschlussdokument, worin es mitteilte, dass 16 Beschl\xfcsse getroffen und die Handlungslinien f\xfcr 31 Projekte zwischen den s\xfcdamerikanischen L\xe4ndern \xfcber einen Investitionsbetrag von insgesamt 17 Milliarden Dollar festgelegt wurden.
Mit der Krise in Europa darf "die wirtschaftliche Konsolidierung (in Lateinamerika) keine triumphierenden Z\xfcge annehmen, sondern soll dazu dienen, unsere Produktionsleistung auszuweiten und unseren V\xf6lkern eine bessere Zukunft aufzuzeigen", f\xfcgte Humala hinzu.
Ich wei\xdf noch, dass mir Gene Bartow, der hier als Trainer arbeitete und an der Universit\xe4t von Alabama (Birmingham) angestellt war, sagte: "Ich habe einen sehr kr\xe4ftigen und 2 m gro\xdfen Spieler.
In Penn State wird die Abschlusspr\xfcfung am Vorabend der Apokalypse durchgef\xfchrt, weshalb die Studenten keine andere Chance haben, als "bis zur Nacht weiterzuarbeiten, wo die Welt angeblich zu Ende geht", sagte Restall.
Joseph Dougherty, ein Religionsprofessor der Universit\xe4t La Salle, der dieses Jahr auf den Philippinen unterrichtet, antwortet schnell auf die Frage, ob er dort einen Kurs \xfcber das "Ende der Welt" kennen w\xfcrde.
Ein Bericht des Brennan Centers von 2011 zeigt, dass diejenigen Staaten, die diese Gesetze verabschiedet haben, 171 der 270 Stimmen ausmachen, die im Wahlm\xe4nnergremium erforderlich sind, um die Pr\xe4sidentschaft zu gewinnen.
Es gibt \xfcbrigens zahlreiche Physiker, die sehnlichst hoffen, dass solche Abweichungen gefunden werden, da der geringste Unterschied eine T\xfcr zu einer "neuen Physik" \xf6ffnen und einige L\xf6cher des Modells stopfen k\xf6nnte.
Genau diese gro\xdfe Unzul\xe4nglichkeit in der Gesundheitsversorgung Quebecs sorgt daf\xfcr, dass mehrere in der Palliativpflege spezialisierte \xc4rzte der Verabschiedung eines Gesetzes zur Regelung von Sterbehilfe und assistiertem Suizid mit Bedenken entgegensehen.
Bitcoin unterscheidet sich von anderen Arten virtueller W\xe4hrungen wie den "Credits", die verwendet werden, um in einem Videospiel voranzukommen, die man durch Spielen gewinnen oder kaufen (und manchmal auch zur\xfccktauschen) kann.
"Die genutzte Schwachstelle betrifft nicht das eigentliche Protokoll", versichert Pierre Noizat, der gerade Paymium eingef\xfchrt hat, das ein Unternehmen f\xfcr die Bezahlung mit echtem Geld ist und das Netzwerk Bitcoin nutzt.
Die salafistischen Parteien, f\xfcr die die Errichtung des islamischen Rechts eine wichtige Forderung ist, hatten die Hoffnung, "die Grunds\xe4tze" durch "die Regeln" zu ersetzen, was eine striktere Anwendung m\xf6glich gemacht h\xe4tte.
Galil\xe4a ist der Ort, an dem Jesus seine Wunder vollbrachte: die Wandlung von Wasser in Wein auf einer Hochzeitsfeier, das Gehen auf dem Wasser, die Stillung des Seesturms und der Fischfang.
Laut der Statistik des Innenministeriums wurden 142 Verbrechen mit Anwendung der registrierten Waffen im Verlauf von sechs Monaten in 2012 ver\xfcbt, w\xe4hrend f\xfcr denselben Zeitraum insgesamt 1,168 Tausend Delikte verzeichnet wurden.
Es gibt H\xe4ndler auf den M\xe4rkten, doch dort muss man hingehen und sich mit einem Code verabreden wie "von Iwan Iwanowitsch, der ausrichten l\xe4sst, dass die Tochter einen Zahn verloren hat".
Im Gespr\xe4ch mit dem Leiter der Gruppe f\xfcr interaktive 3D-Technologien im Microsoft-Labor in Cambridge Shahram Izadi, wird allerdings deutlich, dass die Brille f\xfcr die Wissenschaftler des Unternehmens nur eine Durchgangsstation war.
Vereinfacht gesagt, geht es darum, dass die europ\xe4ische Legislative festlegt, wie \xf6ffentliche Auftr\xe4ge zu handhaben sind. Darauf bauen die einzelstaatlichen Gesetzgebungen auf. Und schlie\xdflich gibt es noch die eigentliche praktische Anwendung.
Nach Madrid, Luxemburg, London und weiteren St\xe4dten, in denen alles besser funktioniert als bei uns, waren wir gerade in Russland Zeugen dessen, dass im Osten noch alles in seinen Anf\xe4ngen ist.
Respekt in der \xd6ffentlichkeit und Barrierefreiheit ist eine Sache, aber erst wenn aus unseren Reihen bedeutende Sportler, K\xfcnstler, Schauspieler, Politiker oder Rechtsanw\xe4lte kommen, werden die Dinge wirklich anfangen, sich zu \xe4ndern.
Polen beteiligte sich im Rahmen des Interkosmos-Programms auch an der Weltraumforschung mit sowjetischen Satelliten, und im Jahr 1978 wurde der polnische Pilot Miroslaw Hermaszewski nach dem Tschechen Vladim\xedr Remek zweiter Interkosmonaut.
In welchem Licht erscheinen da die Worte David Rockefellers aus dem Jahr 1994: "Das einzige, was wir brauchen, ist eine alles umspannende Krise, und die Menschen werden die neue Weltordnung begr\xfc\xdfen."
Die Normen bez\xfcglich Obst und Gem\xfcse wurden von der EU gegen den Widerstand einiger L\xe4nder bereits mit dem Hinweis aufgeweicht, dass die bisherigen Richtlinien zu einer Vergeudung von Lebensmitteln f\xfchren w\xfcrden.
Als Pr\xe4sident w\xe4re es f\xfcr mich kein Problem, die Vorsitzenden der Parlamentsparteien live im Fernsehen dazu aufzufordern, die materielle und strafrechtliche Haftung f\xfcr Politiker, Beamte, Richter und Staatsanw\xe4lte gesetzlich zu verankern.
Seit fast zehn Jahren \xfcbt der Chor Lieder in dieser fremden weichen Sprache ein und bringt sie ab und an auch dahin zur\xfcck, wo sie urspr\xfcnglich herkommen: in den S\xfcden Afrikas.
Im Sternbild Schlangentr\xe4ger haben Astronomen die Vorboten einer kosmischen Karambolage fotografiert: 400 Millionen Lichtjahre von der Erde entfernt rasen die Kerne zweier verschmelzender Galaxien aufeinander zu und werden unausweichlich miteinander kollidieren.
Wenn in Norwegen die Dunkelheit \xfcber das Land kommt und das Wetter k\xe4lter wird, str\xf6men Norweger zu einem Fest hier in Fagernes, das dieser, nun, wirklich sehr bestechenden Spezialit\xe4t gewidmet ist.
"Man isst es roh und sp\xfclt es dann mit einem Glas Aquavit herunter", sagt Havard Halvarsen, der eigentlich in der \xf6rtlichen Feuerwache arbeitet, aber als sogenannter "Rakfisk-General" auch das Festival veranstaltet.
Manning antwortete, er habe seine Bedenken m\xfcndlich zum Ausdruck gebracht und die Beamten h\xe4tten diese mit ihm besprochen und angegeben, sich mit diesen zu befassen. Sie seien jedoch nicht protokolliert worden.
"Ich wollte Mitarbeiter davon \xfcberzeugen, dass es mir gut ging, und den Beobachtungsstatus zur Pr\xe4vention von Verletzungen loswerden (...) um eine aus meiner Sicht h\xf6here Lebensqualit\xe4t erreichen zu k\xf6nnen", sagte Manning.
Als er nach Quantico verlegt wurde, habe Manning den Gro\xdfteil seiner Tage in einer kleinen Zelle verbracht - mindestens 21 Stunden und oft mehr als 23 Stunden - und ohne Gesellschaft.
"Wer Tabak vermarktet und nur einen kleinen Bereich \xfcbrig hat, um seine Produkte zu bewerben, kommt um das Internet nicht herum", sagt Becky Freeman, Forscherin im Gesundheitswesen an der Universit\xe4t Sydney.
Doch Peter Toohey, Professor f\xfcr griechische und r\xf6mische Geschichte an der Universit\xe4t von Calgary in Kanada und Autor von "Boredom: A Lively History" (Yale University Press, 2011) sieht das nicht so.
Manchmal nicht, denn im Extremfall f\xfchrt sie dazu, dass Menschen extreme k\xf6rperliche Risiken auf sich nehmen und dem Gl\xfccksspiel oder Drogen verfallen, um sie zu lindern - das haben Studien gezeigt.
Laut der Journalistin Suzy Menkes, der obersten Autorit\xe4t der Fachpresse, war dieses Kleid ein Meilenstein in der Haute Couture Ende des 20. Jahrhunderts, "die R\xfcckkehr zu den Kundinnen der obersten Gesellschaft".
Dies ist der Fall bei Anto Wijaya, einem der 400 Minenarbeiter, die sich ihr Leben verdienen, indem sie Schwefel aus dem Vulkan Kawah Ijen im Osten der indonesischen Insel Java holen.
Trotz ihrer gro\xdfen Gewinne hat die Minengesellschaft den Schwefelabbau nicht mechanisiert, um Kosten zu sparen, und liefert den Tr\xe4gern, die auf eigene Rechnung arbeiten und nach Gewicht bezahlt werden, keinerlei Ausr\xfcstung.
Die S\xe4tze sind Teil eines Rapper-Songs, der lokale Spr\xfcche wie z. B. "Schieben wird einen "bao" (Laib) in den Ofen, um sich \xfcber die niedrige Geburtenrate in Singapur lustig zu machen.
Porras erl\xe4utert, dass der Akademiker Marc Prensky, Inhaber eines Master-Titels in P\xe4dagogik an der Universit\xe4t Yale und Autor des Werks "Digital Natives and Immigrants" diese Begriffe zur Erkl\xe4rung des Ph\xe4nomens formte.
Das einzige Dokument, das w\xe4hrend des Tages verbreitet wurde, war die Liste der teilnehmenden Pr\xe4sidenten, was bei den hunderten Journalisten verschiedener nationaler und internationaler Medien Unbehagen hervorrief, die mehr Informationen forderten.
Und wenn Schweden Herrn Assange auf der Botschaft Ecuadors in London oder \xfcber Skype verh\xf6rte, wie es die schwedische Rechtsprechung zul\xe4sst und in anderen F\xe4llen gemacht wurde, sei das Problem erledigt.
Gebildet aus den Unternehmen NYCE, e-Qu\xe1lity und Kernet, f\xfchrenden Unternehmen der Informationstechnologie, wurde eine Unternehmensgruppe unter der Bezeichnung Competival gegr\xfcndet, deren Zielsetzung der Service-Markt der Software-Cluster in Zentral- und S\xfcdamerika ist.
Dort spielte er den Astronauten Tony Nelson, dessen Leben auf den Kopf gestellt wird, als er eine attraktive "Dschinn" trifft (gespielt von Barbara Eden), die bei ihm zu Hause leben wird.
Den Studenten, die als W\xe4hler angesehen werden, die ihre Stimme vermehrt f\xfcr demokratische Kandidaten abgeben, ist es in mehreren Staaten nicht erlaubt, ihren von ihrer Einrichtung ausgestellten Lichtbildausweis zu benutzen.
Wenn Sie in der Lage sind, diese Chronik zu lesen, dann nur dank eines Bosons von au\xdfergew\xf6hnlicher Banalit\xe4t: das Photon oder das "Lichtteilchen", das der "Bote" der elektromagnetischen Kraft ist.
Ganz am Ende des Lebens greifen die \xc4rzte somit h\xe4ufig auf die terminale Sedierung zur\xfcck, die darauf hinausl\xe4uft, den Patienten entweder sporadisch oder dauerhaft bis zum Zeitpunkt seines Todes einzuschl\xe4fern.
In den letzten Wochen hat sie reihenweise Hausdurchsuchungen vorgenommen und Beschuldigungen wegen Betrug und Korruption gegen kommunale Mandatstr\xe4ger wie Frank Tampino und Richard Marcotte erhoben, der B\xfcrgermeister einer Vorstadt ist.
Das Kloster des Heiligen Kreuzes in Jerusalem steht an dem Ort, an dem einer christlichen Legende zufolge der Baum wuchs, aus dem das Kreuz f\xfcr die Kreuzigung Jesu gemacht wurde.
Dar\xfcber, dass die wichtigste unmittelbare Aufgabe darin besteht, das System vor Korruption zu sch\xfctzen, damit die Bescheinigungen nicht einfach gekauft werden k\xf6nnen, sind sich sowohl Amtstr\xe4ger als auch B\xfcrgerrechtler einig.
Die Teilnehmer der Proteste am "Black Friday" forderten Lohnerh\xf6hungen und \xe4u\xdferten ihren \xc4rger dar\xfcber, dass der Beitrag f\xfcr die betriebseigene Krankenversicherung von 30 auf 100 Dollar im Monat gestiegen war.
Es gab einmal eine Zeit, in der fast ein Viertel aller US-amerikanischen Jugendlichen nach der Schule bei McDonald's hinter der Theke stand, allerdings lebten die Jugendlichen noch bei ihren Eltern.
Andererseits gibt es im Forum der Zeitung Wall Street Journal einen Kommentar, dessen Verfasser anmerkt, es sei verantwortungslos, Kinder zu bekommen, wenn man nicht wisse, wie man sie ern\xe4hren soll.
Im Jahr 1995 besetzte ich einen Raum in der Puschkinskaja 10, und dort gab es bis zu den Renovierungsarbeiten einen musikalisch-k\xfcnstlerischen Klub f\xfcr die Boheme, das Haus der Petersburger Boheme.
In Petersburg haben wir welche, die Experten sein k\xf6nnten, aber ihnen wird der Weg versperrt, da es hochrangigerer Experten bedarf, die die Ersteren richtig bewerten und ihnen den Weg freimachen.
Das Ende der Konzerte soll in etwa zu der Zeit sein, zu der auf der Pazifikinsel Kiribati, die in einer Zeitzone um 12 Stunden vor uns liegt, der Maya-Kalender endet.
Ziel des Konzertes ist es, die Mittel f\xfcr die Ausstattung eines multifunktionellen behindertengerechten Bildungszentrums aufzubringen, dass unter dem Namen STUDEO im Jedli \u2047 ka-Institut in Prag entstehen soll. Kostenpunkt: 25 Mio. CZK
Die Ideen des jungen Ingenieurs (geb. 1905) lie\xdfen die Zuh\xf6rer jedoch kalt, und nach Jahren erinnerte sich  \u2047 ternfeld noch, dass lediglich Dr. Jan Gadomski Interesse an seiner Arbeit gezeigt hatte.
Diese Situation wird noch dadurch verst\xe4rkt, dass die Herren Unternehmer absolut unwillig sind, ihre Steuern zu zahlen und dadurch die von ihnen verursachten gesamtgesellschaftlichen wirtschaftlichen und sozialen Sch\xe4den zu ersetzen.
"... dass nichts aus Gewalt entsteht, oder jemals entstehen k\xf6nnte" singt Sting im Lied Fragile, dessen wichtigster Vers im Refrain lautet: "...damit wir nicht vergessen, wie zerbrechlich wir sind" .
Man muss hier zwischen den Bewohnern Israels und ihrer F\xfchrung unterscheiden, setzen doch die internationalen Banker in Israel ebenso wie bei uns, dem Volk, ausschlie\xdflich ihre eigenen Kandidaten zur Wahl.
Der Server Bankovn\xedpoplatky.com nominierte in Zusammenarbeit mit dem Verband liberaler \xd6konomen Laissez Faire neben den o.g. Absurdit\xe4ten auch die EU-Verordnung \xfcber den Umfang von Lebensmittelvorr\xe4ten auf dem Gebiet eines Mitgliedslandes.
Das Problem ist die kleingeistige Politik - wenn jemand von rechts oder von links mit einem guten Vorschlag kommt, wird dieser absichtlich abgelehnt, und das h\xe4lt die Bev\xf6lkerung nur auf.
Der Aston Martin war \xfcbrigens ein Kindertraum - James Bond gefiel mir schon immer, wie er in dem Auto fuhr, galant zu Frauen war und gleichzeitig gegen das B\xf6se k\xe4mpfte.
Am Ende der fast 500 Meter langen Wanderschaft wird man im Literaturcaf\xe9 nicht nur mit einer fantastischen Aussicht auf die Stadt, sondern auch mit holl\xe4ndischen Kroketten und eingetopften Ficusb\xe4umen belohnt.
F\xe4llt es Deutschland schwer, seine engen Beziehungen mit Israel und den USA auf der einen, und der Position der wichtigsten Partner in der EU auf der anderen Seite zu vereinbaren?
Zudem hat "Voices for Africa" eine N\xe4hschule ins Leben gerufen, zwei H\xfchnerh\xe4user gebaut und gemeinsam mit der amerikanischen Gesundheitsorganisation PSI organisiert, dass viele im Dorf einen HIV-Test haben machen lassen.
"Auffallend viele hochaltrige Menschen gibt es auch in einigen Gegenden von China, in Japan oder im Hunza-Tal in Pakistan", sagt Scholz, "auch in Sardinien leben extrem viele sehr alte M\xe4nner".
Doch was der 61-j\xe4hrige Ingenieur, der einen Doktortitel der amerikanischen Universit\xe4t von S\xfcdkalifornien tr\xe4gt, wirklich retten will, dar\xfcber sind sich die \xc4gypter, ist sich die Welt nicht ganz im Klaren.
Das war und ist Auslegungssache und es steht zu bef\xfcrchten, dass die Islamisten die schwammige Formulierung und den damit einhergehenden juristischen Spielraum f\xfcr eine strengere Auslegung der Scharia nutzen werden.
Zehntausende mexikanische Familien wurden in den letzten sechs Jahren von Gewaltverbrechen in Mitleidenschaft gezogen, und der neue Pr\xe4sident hat versprochen, sich w\xe4hrend seiner Amtszeit besonders um dieses Problem zu k\xfcmmern.
Wie ich w\xe4hrend meiner Reise lernen sollte, gibt es etwas, das diese Beziehung noch komplizierter macht: Einige mexikanische F\xfchrungspersonen und Teile des Bildungsb\xfcrgertums m\xf6chten ihre Verbindungen zur Diaspora wieder aufnehmen.
Die Anf\xfchrer der Hamas, der islamistischen Bewegung, die seit 2007 den Gazastreifen kontrolliert, wird von sich behaupten, die Israelis zur\xfcckgedr\xe4ngt zu haben, obwohl seine Gruppierung selbst gro\xdfe Verluste verzeichnen musste.
Die T\xfcrkei, eine wiedererstarkende, regionale Macht, die einst als Israels engster muslimischer Verb\xfcndeter galt, hat f\xfcr die Hamas Partei ergriffen - genau wie Katar, einer der reichsten und dynamischsten Golfstaaten.
Dabei geht die Regierung von Studien aus, die gezeigt haben, dass Menschen, die mit 26 noch nicht angefangen haben, zu rauchen, mit 99%-iger Wahrscheinlichkeit auch danach nicht mehr anfangen werden.
John D. Eastwood, einem assoziierten Professor der Psychologie an der Universit\xe4t York in Ontario, Kanada zufolge besteht das Problem darin, dass Langeweile auf vielerlei Arten definiert und diskutiert worden ist.
Er fand heraus, dass 32% der Heranwachsenden in der Schule und beim Erledigen der Hausaufgaben gelangweilt waren, wohingegen 23% angaben, gelangweilt zu sein, wenn sie nicht in der Schule waren.
In den ungewissen Wochen nach dem Beschluss des Staates, kleine Mengen Marihuana zum Eigengebrauch zu legalisieren, h\xe4ngt die Antwort bei hunderten kleinerer Drogendelikte weniger vom Gesetz, als vom Standort ab.
Darin gezeigt wurde unter anderem Absolvent Joe Cooke, fr\xfcherer Pr\xe4sident der konservativen studentischen Vereinigung der Universit\xe4t Oxford, der in einem Rolls-Royce fuhr und mit silberfarbenem Anzug und silberbesetztem Gehstock protzte.
Und noch tragischer ist, dass es Oxford war - eine Universit\xe4t, die nicht nur 14 Tory-Premierminister hervorbrachte, sondern sich bis heute hinter einem unverdienten Ruf von Gleichberechtigung und Gedankenfreiheit versteckt.
Vier Monate Arbeit und 25 "Ragazze" (wie der Modemacher seine N\xe4herinnen nannte) waren notwendig, um dieses elfenbeinfarbene Seidenkleid mit Perlen, zw\xf6lf verschiedenen Stickereien und einem viereinhalb Meter langen Schweif anzufertigen.
"Diese Arbeit ist f\xfcr die Tiere und nicht f\xfcr den Menschen" protestiert Madrusin, ein st\xe4mmiger, 42 Jahre alter Tr\xe4ger, der drei Jahrzehnte seit Verlassen der Schule am Kawah Ijen arbeitet.
"Ich werde nicht in Rente gehen, ich werde hier sterben, weil der Vulkan mein ganzes Leben war" erkl\xe4rt Unainik, wobei er seinen Mund weit \xf6ffnet, in dem einige Z\xe4hne fehlen.
In vier der F\xe4lle verkn\xfcpften sie den Begriff mit "etwas sehr eigenem" auf pers\xf6nlicher Ebene und "auf das Passwort und den Benutzer", wenn sie ihn auf die sozialen Netzwerke anwendeten.
Man k\xf6nnte also sagen, dass die Verfahren zum \xdcberleben der Unternehmen, die die mexikanischen Gesetze zulassen, im Land der Stars und Stripes im Widerspruch zu internationalen Abkommen keine G\xfcltigkeit haben.
Aus diesem Grund legt die Familie Gonz\xe1lez Sada vor dem selben Berufungsgericht Widerspruch ein, damit die Abstimmung im Plenum erfolgt, d. h. von allen Richtern, weil nur drei davon abstimmten.
"Das waren meine besten Jahre, die ich am meisten genossen habe, weil ich Teil von acht Meisterschaften der Vaqueros seit 1967 sei es als Gesch\xe4ftsf\xfchrer, Mitgesch\xe4ftsf\xfchrer oder Trainer sein durfte.
"Es ist faszinierend zu sehen, was die Leute tun, um sich selbst zu tr\xf6sten", sagte Bridgid Robinson, eine 23-j\xe4hrige Studentin in Rutgers-Camden f\xfcr Religion und Soziologie aus Haddonfield, New Jersey.
Diese Studie hat ebenfalls gezeigt, dass bei einer Nachbeobachtung nach 12 Jahren die Wahrscheinlichkeit der Bildung von Metastasen um 30 bis 40% h\xf6her ist, wenn keine Fr\xfcherkennung durchgef\xfchrt wurde.
Durch diese "St\xf6rung" entsteht eine elektromagnetische Welle (Licht, Infrarot- oder Ultraviolettstrahlung usw.), und diese Welle ist nichts anderes als ein Photon und somit eines der Bosonen "Tr\xe4ger der Kraft".
Deshalb ist ein riesiger Teilchenbeschleuniger wie das CERN erforderlich - der Large Hadron Collider ist ein Ring mit einem Umfang von 27 km! - um derartige Energien zu erreichen.
F\xfcr die Wissenschaft dienen sie der \xdcberpr\xfcfung des Standardmodells (SM), und sie erm\xf6glichen den Physikern ebenfalls, alle Abweichungen zwischen den Beobachtungen und den Vorhersagen des SM genau zu untersuchen.
Der Skandal wurde durch ihn aufgrund einer eingehenden Untersuchung der Veruntreuungen im Zusammenhang mit den Vertr\xe4gen zu Stra\xdfenbauarbeiten in Quebec aufgedeckt, der der damalige Premierminister nur widerwillig zugestimmt hatte.
Es ist an der Zeit, dass die afghanische Armee den Besitz ihres Territoriums wieder ergreift, und dass die afghanische Bev\xf6lkerung ihre Zukunft entscheidet, ohne alles von uns zu erwarten.
Die Taliban bestehen aus ausl\xe4ndischen Extremisten, ehemaligen F\xfchrern, die nach Pakistan gefl\xfcchtet sind, aber h\xe4ufig auch aus Bauern, die eine bewaffnete ausl\xe4ndische Pr\xe4senz verweigern, wie zur Zeit der Sowjets.
Kurz vor der Verfassungserkl\xe4rung Mitte November haben sie sich abgewendet, da sie der Meinung sind, dass sie nicht in der Lage gewesen sind, ihre Sichtweisen zur Geltung zu bringen.
Artikel 2, der alle Aufmerksamkeit auf sich zog, bleibt schlie\xdflich identisch mit jenem der Verfassung von 1971 und besagt, dass "die Grunds\xe4tze der Scharia die Hauptquelle des Rechts sind".
F\xfcr die Islamisten ist die Tatsache, dass dieser Artikel nicht ge\xe4ndert wurde, ein Beweis f\xfcr ihren guten Willen und f\xfcr ihren Respekt gegen\xfcber den anderen Mitgliedern der \xe4gyptischen Gesellschaft.
Dabei haben sie besonders Artikel 220 im Auge, der der Universit\xe4t Al-Azhar eine beratende Funktion zuerkennt, insbesondere in Bezug auf die \xdcberpr\xfcfung der Konformit\xe4t mit den Gesetzen der Scharia.
Besucher kommen hierher f\xfcr Behandlungen unter Anwendung von Salzwasser (nat\xfcrliche Salzsole) und Heilschlamm sowie zur Behandlung von Hautentz\xfcndungen, Allergien, Asthma, Ekzemen, Arthritis, Bronchitis, Zuckerkrankheit und zur Beruhigung strapazierter Nerven.
Das Geld in der Reise nimmt man lieber in keinen Euros, sondern in Dollars mit, die einfach in Schekel gewechselt werden k\xf6nnen (aktueller Wechselkurs: 1 Dollar zu 3,8 Schekel).
"Heutzutage gibt es unz\xe4hlige private R\xfcstungsfabriken, die der internationalen Konkurrenz nicht standhalten und deshalb die Waffen unter der Hand auf dem Schwarzmarkt, etwa in Moskau, verschleudern", berichtet der Experte.
Der Black Friday dauerte in seinen Laden von 8 Uhr abends am Donnerstag bis Mitternacht den n\xe4chsten Tag, und in diesem Zeitraum verkaufte Walmart ungef\xe4hr 5000 Artikel pro Sekunde.
- Und all das vereinte sich in deiner Art-Klinik... - Es war mir wichtig, im Mittelpunkt der Petersburger Kultur zu stehen, wo sich die besten schaffenden K\xfcnstler versammeln sollten.
In der heutigen Zeit ist es einfach, ber\xfchmt zu werden, aber Kultur und Popularit\xe4t sind nicht das gleiche: Man kann ber\xfchmt sein, ohne damit einen kulturellen Beitrag zu leisten.
Dasselbe gilt f\xfcr das Erarta, jedoch mit dem Unterschied, dass sie ehrlich sagen, dass sie nicht alle zeitgen\xf6ssische Kunst annehmen und einige Maler sich deshalb andere Museen suchen m\xfcssen.
Das System muss diejenigen ausschlie\xdfen, die das System angreifen und missbrauchen wollen, und nicht diejenigen bestrafen, die einen Formfehler begangen haben, der sich auf die eigentliche Entscheidungsfindung nicht auswirkt.
Ich erinnere hier beispielsweise an den Vortrag von A.  \u2047 ternfeld vom 6. Dezember 1933 im Warschauer Observatorium, bei dem der Autor Gedanken aus seiner Pionierarbeit "Eingang zur Kosmonautik" vorstellte.
Diese L\xf6sungen sind aber falsch und f\xfchren immer zur Verschlimmerung der Situation (siehe Gr\xfcndung der FED, damit sich Krisen wie die von ihnen im Jahr 1907 ausgel\xf6ste nicht wiederholen).
Aber ich kann nicht mehr mit ansehen, wie die Republik seit 20 Jahren gepl\xfcndert wird, wie Diebe frei herumlaufen, w\xe4hrend den Menschen die Steuern und das Rentenalter erh\xf6ht werden.
Um diesem dummen Umstand entgegenzuwirken, beschloss man vor einigen Jahren, zur Allgemeinbildung beizutragen und die sieben fiktiven Br\xfccken, die auf den Euroscheinen dargestellt sind, als h\xfcbsch bepinselte Stahlbetonminiaturen nachzubauen.
Stephen Szabo ist stellvertretender Direktor der Transatlantic Academy in Washington, ein Institut, in dem Akademiker und Politikexperten aus Europa und Nordamerika gemeinsam zu den Herausforderungen der transatlantischen Gemeinschaft forschen.
Anfangs war es noch das private Engagement Einzelner, f\xfcr ein paar Euro im Jahr ein Kind zur Schule zu schicken und ihm eine warme Mahlzeit am Tag zu erm\xf6glichen.
Dieser Bildausschnitt einer Infrarot-Aufnahme des Spitzer-Teleskops zeigt ein "Familienportr\xe4t" ungez\xe4hlter Sternengenerationen: Die \xe4ltesten Sterne sind als blaue Punkte zu erkennen, schwerer zu identifizieren sind die pinkfarbenen "Neugeborenen" im Sternenkreissaal.
W\xe4hrend ihre Mutter ihre Geschichte erz\xe4hlt, blickt von der Wand ein Bild von Mariana auf uns herunter. Es ist neben einem Kreuz angebracht, das ein einziges Wort tr\xe4gt: Gerechtigkeit.
Dass sich der pragmatische Pr\xe4sident Mursi mit Barack Obama zusammentat, um einen Waffenstillstand zu erreichen, k\xf6nnte ein verhei\xdfungsvolles Zeichen sein - und vielleicht den Beginn einer neuen \xc4ra symbolisieren.
Obwohl Australien eine der geringsten Raucherquoten der Welt aufweist und die \xc4nderungen sich nur geringf\xfcgig auf die Gewinne der multinationalen Konzerne auswirken werden, erw\xe4gen andere L\xe4nder bereits \xe4hnliche Schritte.
Wenn man hingegen eine eint\xf6nige T\xe4tigkeit ausge\xfcbt - "so wie die Suche nach fehlerhaften Produkten auf einem Fabrikf\xf6rderband, kann Musik ablenken und dabei helfen, sich nicht gelangweilt zu f\xfchlen".
Die Polizeibeh\xf6rden verfolgen Erwachsene \xfcber 21 Jahren nicht l\xe4nger f\xfcr Besitz in kleinem Ma\xdfe. Dieser wird gesetzlich gestattet, sobald die neuen Gesetze in den n\xe4chsten Wochen in Kraft treten.
Zur gleichen Zeit stimmen mehrere St\xe4dte, von den Vorst\xe4dten Denvers bis zu den Western Mountains dar\xfcber ab, neue, staatliche lizenzierte Marihuanagesch\xe4fte an der Er\xf6ffnung in ihren Gemeinden zu hindern.
"Diese Situation entwickelt sich so schnell weiter, dass ich gar nicht wei\xdf, was als N\xe4chstes geschehen wird", sagt Daniel J. Oates, Polizeichef in Aurora, das \xf6stlich von Denver liegt.
Verschlimmert wurde ihre Situation durch eine k\xfcrzlich ausgestrahlte Dokumentation \xfcber politische Studenten auf BBC Two, "Wonderland: Young, Bright and on the Right", die Tories als Exzentriker und Neonazis darstellte.
"Ich schlage vor, dass sie in Ihrer Freizeit ein paar Franz\xf6sischstunden nehmen - also, wenn Sie nicht zu sehr mit Ihren gesellschaftlichen T\xe4tigkeiten besch\xe4ftigt sind", knurrte mich Pitt an.
Anl\xe4sslich der Ausstellung "Valentino - Meister der Couture", die diese Woche in London er\xf6ffnet wurde, spricht ABC mit Naty Abascal, Fiona Thyssen-Bornemisza und anderen ber\xfchmten Kunden des italienischen Modemachers.
Nachdem er gro\xdfe Schwefelsteine herausgebrochen hat, die insgesamt bis zu 70 Kilo wiegen k\xf6nnen, transportiert er sie in zwei Bambusk\xf6rben auf seinen Schultern \xfcber die absch\xfcssigen Pfade aus Stein.
Diese \xc4nderungen in den sozialen Gegebenheiten haben zur h\xf6heren Zahl an Alleinstehenden und am Hinausz\xf6gern der Heirat und Geburten beigetragen, deren Ergebnis die Verringerung der Geburtenrate in Singapur ist.
Die Beh\xf6rde f\xfcr st\xe4dtische Entwicklung hat damit begonnen, die Zahl an kleinen Appartements zu kontrollieren, die als "Schuhschachteln" bekannt sind und in bestimmten Gebieten der Stadt gebaut werden d\xfcrfen.
Zu den getroffenen Beschl\xfcssen sagte er, dass die L\xe4nder der Unasur "bedeutende Schritte in Richtung des Ziels einer s\xfcdamerikanischen Staatsb\xfcrgerschaft unternehmen werden, wozu wir die Beschl\xfcsse \xfcber Aufenthaltsrechte ausweiten."
Die Notwendigkeit, dass Lateinamerika auch weiterhin eine integrierte Region f\xfcr Wohlstand und Frieden und mit guten nachbarschaftlichen Beziehungen bleibt, war ein weiterer Aspekt, der auf dem Gipfeltreffen betont wurde.
Santos und Ortega w\xfcrden sich am Samstag in Mexiko treffen, wo sie die Absicht haben, bei der Amts\xfcbernahme des neuen Pr\xe4sidenten dieses Landes, Enrique Pe \u2047 a Nieto, anwesend zu sein.
Wie Sie wissen, erfolgten diese Ma\xdfnahmen, obwohl der Senat die M\xf6glichkeit au\xdfer Betracht gezogen hatte, weil er sie als Versto\xdf gegen die freie Meinungs\xe4u\xdferung in den sozialen Netzwerken betrachtete.
"Wir analysieren, weshalb sich diese Ideen mit der Zeit ausbreiten", sagte er, sowie die Art und Weise, wie hypothetische Szenarien angeboten werden, die zu einem bestimmten menschlichen Verhalten f\xfchren.
Allerdings h\xe4lt das Brennan Center letzteres f\xfcr einen Mythos, indem es bekr\xe4ftigt, dass der Wahlbetrug in den USA seltener ist als die Anzahl der vom Blitzschlag get\xf6teten Menschen.
Die demokratischen Kritiker prangern die parteipolitische Natur der verabschiedeten Gesetze an und sehen in ihnen als klares Ziel die Beeinflussung der Ergebnisse in den f\xfcr 2012 ausschlaggebenden Staaten.
Es ist zu fr\xfch, um mit Gewissheit zu best\xe4tigen, dass diese \xc4nderungen der Rechtsvorschriften am Wahlsystem erhebliche Auswirkungen auf das Ergebnis der Pr\xe4sidentschaftswahlen im Jahr 2012 haben werden.
Mutig gelingt es ihm sogar zu l\xe4cheln und mit den Fremden zu sprechen, die um ihn herum besch\xe4ftigt sind, ihm seine Medikamente bringen, und ihm ein Bad bieten.
Dr. Christiane Martel zufolge ist das Gesundheitssystem Quebecs nicht leistungsf\xe4hig genug, um sicherzustellen, dass alle Recht auf eine qualitativ hochwertige Palliativpflege haben, bevor man akzeptiert, zur Sterbehilfe \xfcberzugehen.
Vor Kurzem, sagt sie, habe ich eine Patientin gesehen, die 14 Tage mit gro\xdfen Schmerzen in der Notaufnahme war, ohne dass man Ma\xdfnahmen zu ihrer Linderung ergriffen hat.
Ausgehend von einem Anteil von 70% Schwarzgeld bei der Finanzierung der Wahlkampagnen in Quebec witzelt er: "Mir wurde gesagt, dass dies nur ein schwacher Abklatsch der Wirklichkeit sei."
Falls diese Geschichte das internationale Ansehen Quebecs und jenes von Montreal sch\xe4digt, fordert Herr Duchesneau diejenigen auf, die dar\xfcber lachen, einen Blick in ihren eigenen Hinterhof zu werfen...
Dies geschieht \xfcber eine mathematische Aufgabe, die auf den Computern gestartet wird, wobei der Gewinner, der eine Art vorl\xe4ufiger Zentralbankier ist, das Privileg besitzt, diese zus\xe4tzliche Zeile hinzuzuf\xfcgen.
Diese Arbeiten, f\xfcr die zahlreiche lokale Arbeitskr\xe4fte erforderlich waren, haben dazu beitragen k\xf6nnen, den Aufstand zu unterdr\xfccken: Bew\xe4sserung, Brunnen, Trinkwasser, Wiederaufforstung, Obstb\xe4ume, Bodenschutz und Erh\xf6hung der landwirtschaftlichen Nutzfl\xe4chen.
Ein viel bescheideneres Budget wird zur Verbesserung der lokalen Lebensbedingungen beitragen, die in diesen oft in einer H\xf6he von mehr als 2000 Metern liegenden T\xe4lern sehr hart sind.
W\xe4hrend \xc4gypten in Bezug auf die Verfassungserkl\xe4rung, die ihm vor\xfcbergehend die unbeschr\xe4nkte Vollmacht gew\xe4hrt, mehr denn je gespalten bleibt, hat er beschlossen, alles auf eine Karte zu setzen.
In Jerusalem befindet sich auch der heiligste Ort der Juden - die Klagemauer, die \xdcberreste eines Tempels, der von den R\xf6mern im Jahr 70 n. Chr. zerst\xf6rt wurde.
Die H\xe4lfte aller Waffen auf dem Schwarzmarkt seien dorthin durch die "Schuld von Verantwortlichen, die in ihrer Arbeit mit Waffen zu tun haben gelangt", hei\xdft es im Bericht.
Ein Verkaufsberater eines Waffenladens, der nicht namentlich genannt werden will, versichert, dass Waffen, die bei illegalen Ausgrabungen gefunden werden, schon lange niemand mehr kauft, da sie veraltet sind.
Die Proteste begannen vergangene Woche nach Thanksgiving, am sogenannten Black Friday, an dem in den USA Ausverk\xe4ufe stattfanden, die Millionen von Kunden anlockten, was zuweilen zu Handgemengen f\xfchrte.
Zum Beispiel arbeiteten wir im Bereich der Steuerung von Objekten auf \xf6ffentlichen Pl\xe4tzen an einem Projekt, bei dem wir mit kurzen und knappen, statt mit ausladenden Gesten experimentierten.
- Stellen wir uns einen Moment lang vor, dass die Manipulation virtueller Hologramme in der Luft nicht nur Tony Stark aus Iron Man, sondern auch Normalsterblichen zug\xe4nglich ist.
Er ist auch ein Mann der Stadt und zaubert durch seine Anwesenheit auf der Stra\xdfe seinen Mitb\xfcrgern ein L\xe4cheln ins Gesicht und sorgt bei ihnen f\xfcr gute Laune.
Unter dem Druck des globalen und europ\xe4ischen wirtschaftlichen Wettbewerbs wird Tschechien gezwungen sein, auch weiterhin Wege zu suchen, um das soziale Niveau der Bev\xf6lkerung nach unten zu dr\xfccken.
Nachdem es ihnen durch den Mord am Habsburger Thronfolger Ferdinand in Sarajevo gelungen war, den Ersten Weltkrieg auszul\xf6sen, zerst\xf6rten sie das russische Zarenreich durch die Revolution der Bolschewiken.
Auf der einen Seite ist er ein realistischer Politthriller, gleichzeitig aber auch ein sog. "Caper Movie", d.h. die Geschichte eines gelungenen Husarenst\xfccks wie beispielsweise der Film Ocean's Eleven.
Ich glaube, dass die deutsche Au\xdfenpolitik von der Wirtschaftspolitik motiviert ist, also von den Exporten und seinen Beziehungen zu bestimmten Regionen, etwa Russland, China oder dem Nahen Osten.
"Es wird f\xfcr Ausl\xe4nder immer schwieriger, ihre Marken in China zu sch\xfctzen", sagt Thomas Pattloch, Anwalt in der Kanzlei Taylor Wessing, der auf Schutzrechtsverletzungen in Fernost spezialisiert ist.
Und wenn man die 8733 Kilometer Luftlinie nach Heidelberg zur\xfcckkehrt, zu den stampfenden S\xe4ngern in den Proberaum an der Bergheimer Stra\xdfe, dann sieht man es auch da leuchten.
Zehntausende versammelten sich in ungewohnter Eintracht am Freitagabend auf dem Tahrir-Platz in Kairo und gelobten, die Charta zu Fall zu bringen, noch bevor sie in Kraft treten kann.
W\xe4hrend sich Mexikos zuk\xfcnftiger Pr\xe4sident Enrique Pena Nieto auf seinen Amtsantritt vorbereitet, analysiert Will Grant von der BBC die ihm bevorstehenden Herausforderungen und die gemischten Gef\xfchle seines Volkes.
"Wir erwarten von ihm echte und anhaltende Ver\xe4nderungen", so sein Freund und politischer Verb\xfcndeter Gabriel Olvera Hernandez, der als Kongressabgeordneter f\xfcr die Partei Pena Nietos, die PRI arbeitet.
Zu den Anklagepunkten gegen Manning z\xe4hlen die Beg\xfcnstigung des Feindes, unrechtm\xe4\xdfige Ver\xf6ffentlichung von geheimdienstlichen Informationen im Internet, die \xdcbertragung nationaler Verteidigungsinformationen und der Diebstahl \xf6ffentlichen Eigentums oder Dokumente.
Und angesichts der ungerechten Einkommensverteilung, der ungez\xfcgelten Korruption und der Drogengewalt sind viele von uns gar nicht so sicher, ob es sich wirklich um ein tolles Land handelt.
Von den unterschiedlichen Gesundheitswarnungen und Bildern einmal abgesehen besteht ab kommendem Samstag der einzige Unterschied zwischen den Packungen in den Markennamen, die in identischer, kleiner Schrift abgedruckt sind.
"Man nimmt sich einfach eine Kippe und steckt die Schachtel weg", sagt Victor El Hage beim Kauf einer Zigarettenschachtel, auf der ein Foto mit einem Mundtumor abgedruckt ist.
Trotz mehrerer aufsehenerregender Verhaftungen von Konsumenten und Verk\xe4ufern medizinischen Marihuanas hat die Bundesregierung den Verkauf von medizinischem Marihuana in Colorado, Washington und 16 anderen Staaten zum Gro\xdfteil gestattet.
Konservative Mitglieder des Junior Common Room (JCR) des Corpus Christi College geben an, sie werden aufgrund ihrer politischen Ansichten "oft aktiv isoliert, pers\xf6nlich angegriffen und f\xfcr unerw\xfcnscht erkl\xe4rt".
Somerset House, die ehemalige Residenz von Isabel I von England, ist der einzige Ort in der britischen Hauptstadt, die der Beherbergung einer Ausstellung \xfcber Valentino Garavani w\xfcrdig ist.
In diesem Publikum aus Modepuppen strahlen Namen wie der von Sibilla de Luxemburgo, Gloria von Thurn und Taxis, Mette-Marit von Norwegen, Rosario von Bulgarien oder Sof\xeda von Habsburg.
"Da wir normalerweise 70 kg tragen, erhalten wir f\xfcr jeden Weg ungef\xe4hr 46.000 Rupien (3,8 Euro) ", erkl\xe4rt uns Anto, der im Normalfall drei Strecken am Tag macht.
Dieser sympathische und intelligente, aber vom Leben gestrafte junge Mann k\xf6nnte als Touristenf\xfchrer, Kellner oder am Empfang eines Hotels arbeiten, aber stattdessen verrichtet er die Arbeit eines Tragesels.
Die Zeit vergeht, aber die Armseligkeit h\xe4lt Generation auf Generation in einem der h\xe4rtesten Berufe der Welt an: den derjenigen, die als menschliche Lastesel am Kawah Ijen arbeiten.
"Dies hat den Menschen erm\xf6glicht, au\xdfer zu heiraten und eine Familie zu bilden wesentlich mehr Optionen in Bezug auf Lebensziele zu haben und Priorit\xe4ten zu setzen", erkl\xe4rt sie.
Der Teenager hat Benutzerkonten in Hotmail, Facebook, My Space und Ask. In Ask gibt er zu, 20 der Personen nicht zu kennen, die er seiner Freundesliste angef\xfcgt hat.
Es bestehe allerdings die Gefahr, dass er k\xf6rperlichen und psychischen Schaden n\xe4hme, weil er in einem engen Raum gefangen sei und keine k\xf6rperlichen \xdcbungen im Freien durchf\xfchren k\xf6nne.
Er beschloss, sich allein um seine Krankheit zu k\xfcmmern und begann damit, sich dar\xfcber zu informieren; und dies mit solchem Einsatz, dass er gerade seinen 43. Geburtstag feierte.
Fabrizio lebt mit dem humanen Immundefizienz-Virus (HIV) seit 22 Jahren, was anfangs der 90er Jahre schwer vorstellbar war, als es viele Zweifel, wenige Behandlungsm\xf6glichkeiten und mehr Stigmata gab.
"Wozu brauchst du die?" ist eine verbreitete Spottfrage von Sozialarbeitern, Orientierungspersonal in Schulen, Angestellten in Apotheken und im Gesundheitssystem, der sich Jugendliche nicht aussetzen m\xf6chten, versicherte der Korrespondent.
Es gibt ein halbes Dutzend Beispiele, darunter Agremex und Comercial Mexicana, deren Verbindlichkeiten unter Unternehmen der Gruppe vom Instituto Federal de Concursos Mercantiles (Bundesinstitut f\xfcr Handelskonkurse) best\xe4tigt wurden.
Wird dem nicht stattgegeben, wird der Cerciorare-Einspruch eingelegt, der die \xdcberpr\xfcfung des Verfahrens durch eine h\xf6here Instanz fordert, in diesem Fall durch den Obersten Gerichtshof der Vereinigten Staaten.
Linda Gray, die die Rolle seiner Ehefrau in der Original- und Folgeserie spielte, war bei Hagman, als er im Krankenhaus von Dallas starb, sagte ihr Publizist Jeffrey Lane.
J.R. hatte sie geschw\xe4ngert und drohte damit, sie als Prostituierte darzustellen, wenn sie nicht die Stadt verlie\xdfe. Aber auch andere hatten Gr\xfcnde daf\xfcr, ihn tot sehen zu wollen.
Er ist f\xfcr Millionen Verehrer in der Welt unvergesslich und unersetzbar und bleibt uns, die das Gl\xfcck hatten, ihn zu kennen und zu lieben, in unseren Herzen erhalten.
Andererseits erlauben dieselben Staaten es Mitgliedern von Angel- oder Jagdvereinen, die st\xe4rker f\xfcr die republikanische Seite w\xe4hlen, die von diesen Vereinen ausgestellten Karten f\xfcr Wahlen zu benutzen.
Beispielsweise waren bei den allgemeinen Wahlen 2008 in Florida 33% der W\xe4hler, die im Voraus gew\xe4hlt haben, Afro-Amerikaner, obwohl sie nur 13% der W\xe4hler des Bundesstaates ausmachen.
Heute findet bei vielen M\xe4nnern, bei denen man Krebs erkannt hat, keine Behandlung statt, da ihr Krebs nicht aggressiv ist und keine Bedrohung f\xfcr ihr Leben darstellt.
Und mehrere Organisationen, wie das Heim Victor-Gadbois und die Gesellschaft f\xfcr h\xe4usliche Palliativpflege im Gro\xdfraum Montreal spezialisieren sich mehr oder weniger ausschlie\xdflich auf die Pflege von Krebspatienten.
Au\xdferdem hat ein Veranstalter der Partei des B\xfcrgermeisters, Martin Dumont, Herrn Tremblay beschuldigt, dass er absichtlich \xfcber einen Schattenhaushalt hinweggesehen hat, der seine Kassen mit Schwarzgeld f\xfcllte.
Wenn wir allerdings bei einem Heimspiel gegen Troyes 4-0 gewinnen, und man immer noch etwas findet, was man uns vorwerfen kann, ist das mit Sicherheit etwas frustrierend.
Sein System Paytunia entspricht einer Kreditkarte (mit echtem Geld) oder einer kontaktlosen Zahlung mit einem Mobiltelefon, nutzt aber Bitcoin zur Validierung der Transaktionen, die dadurch billiger sind.
Sie m\xfcssen einfach nur eine Adresse angeben, die von einem Telefon "fotografiert und erkannt" werden kann, gibt Pierre Noizat an, der versichert, dass er tausende Benutzer hat.
Der Abzug der franz\xf6sischen Truppen vom St\xfctzpunkt in Nijrab, den ich von einem mit Mandelb\xe4umen bepflanzten H\xfcgel beobachtet habe, der mithilfe franz\xf6sischer Kredite finanziert wurde, erfolgte ordnungsgem\xe4\xdf.
Auf Seiten seiner Bef\xfcrworter versichert man, dass es ein Weg ist, die institutionelle und politische Krise so schnell wie m\xf6glich zu beenden und den \xdcbergangsprozess zu beschleunigen.
Die Ruinen der Festung Massada bilden die \xdcberreste des geheimen Verstecks vor Feinden, das Herodes der Gro\xdfe im Jahr 25 n. Chr. f\xfcr seine Familie erbauen lie\xdf.
Dort werden alte Qumranhandschriften oder Schriftrollen vom Toten Meer, die in Felsh\xf6hlen in der Jud\xe4ischen W\xfcste gefunden wurden, aufbewahrt sowie ungef\xe4hr 500 Tausend arch\xe4ologische und anthropologische Exponate.
Die ergreifendste Abteilung ist das Denkmal f\xfcr die Kinder, das zum Gedenken an die 1,5 Millionen Kinder, die in den Konzentrationslagern und Gaskammern vernichtet wurden, erbaut wurde.
Erstaunlicherweise wird im Roten Meer auch in den Wintermonaten gebadet, da die Wassertemperatur dort nicht unter 21  \u2047 C f\xe4llt und die Luft sich bis 23  \u2047 C erw\xe4rmt.
\xdcberlieferungen zufolge baute Noah gerade hier seine Arche, und Perseus rettete hier die sch\xf6ne Andromeda, mit der er an diesem Ort ein langes und gl\xfcckliches Leben f\xfchrte.
In vielen Caf\xe9s, Restaurants und Gastst\xe4tten wird nur koscheres Essen serviert, was Schweinefleisch, Meeresprodukte, Fisch ohne Schuppen und Speisen, die sowohl Milch- als auch Fleischprodukte enthalten, ausschlie\xdft.
Den Vorschlag hat die Vorsitzende des Duma-Ausschusses f\xfcr Sicherheit und Korruptionsbek\xe4mpfung, Irina Jarowaja, unterst\xfctzt und versprochen, dass die \xc4nderungen am Waffengesetz in K\xfcrze der Duma vorgelegt werden.
Forscher aus der kalifornischen Universit\xe4t in Berkeley belegen, dass, wenn das Unternehmen den Durchschnittslohn auf 12 Dollars die Stunde erh\xf6ht, es Walmart 3,2 Milliarden Dollars kosten w\xfcrde.
In Fast-Food-Restaurants wird der Mindestlohn nach und nach angehoben, allerdings nicht zu stark, und im Durchschnitt bekommen ihre einfache Mitarbeiter in New York 8,90 US-Dollar die Stunde.
Nun begegnen mir bei Interviews mit Mitarbeitern von McDonald's st\xe4ndig Menschen, die sich beklagen, dass sie mit diesem Lohn auskommen und manchmal sogar ihre Kinder ern\xe4hren m\xfcssen.
Ich denke, dass wir in der n\xe4chsten Zeit vor allem an der Entwicklung neuer Sensortypen arbeiten werden m\xfcssen, die es erm\xf6glichen, Reaktionen von Personen genauer zu erfassen.
Die ganze Stadt kennt Kirill Miller, den in Rot gekleideten B\xe4rtigen, den man mal beim Russischen Museum, mal beim Sommergarten, mal bei Szene-Treffen oder auf Vernissagen antrifft.
Ich bin ein Mensch der vergangenen Kultur und wuchs mit K\xfcnstlern auf, die in Armut lebten und in Armut starben und Geld ablehnten, um malen zu k\xf6nnen.
"Ein Gesetz ist niemals vollkommen, aber es muss richtig angewendet werden - und dies ist meines Erachtens bei uns nicht der Fall", kommentiert Kala die aktuelle Situation.
Auf der Sitzung des Kontrollausschusses der Abgeordnetenkammer sprachen Sie \xfcber ein gemeinsames tschechisch-deutsches Projekt, in dessen Rahmen die Gesetze beider L\xe4nder bez\xfcglich \xf6ffentlicher Auftr\xe4ge miteinander verglichen wurden.
Auch ihre Kollegen im Kreis Jesen\xedk mussten in der Nacht heraus, laut ihren Angaben sind die Stra\xdfen bis in die H\xf6henlagen nach chemischer Behandlung frei und nass.
Nichtsdestotrotz hat es bisher immer ohne Probleme geklappt,  \u2047 SA und British Airways waren immer sehr gut auf uns vorbereitet, dass ich mich manchmal teilweise schon gewundert habe.
In London und Madrid ist es absolut \xfcblich, dass sich auch Menschen mit schweren Behinderungen selbstst\xe4ndig im \xf6ffentlichen Raum bewegen, ins Museum gehen, Toiletten nutzen k\xf6nnen usw.
Liberale Theorien und Medien behaupten bis zum \xdcberdruss, dass sich der Staat nicht mit Kapital an seiner eigenen Volkswirtschaft beteiligten darf, und dass Planwirtschaft zur Wirtschaftskatastrophe f\xfchrt.
Der Server www.bankovnipoplatky.com, der allj\xe4hrlich eine Umfrage \xfcber die absurdesten Bankgeb\xfchren ausruft, hat dieses Jahr beschlossen, den Wettbewerb "Absurdeste Verordnung bzw. Idee aus der EU-Werkstatt" zu veranstalten.
Die Europ\xe4ische Kommission kam Tschechien schlie\xdflich so weit entgegen, dass sie eine Ausschreibung \xfcber den Einkauf von Getreide aus L\xe4ndern organisierte, die keinen Zugang zum Meer haben.
Stets unterst\xfctze ich \xf6ffentlich jeden guten L\xf6sungsansatz, auch wenn dieser von der KS \u2047 M oder von der ODS kommt, und ebenso werde ich mich gegen schlechte Ideen wenden.
Man kann dies meinetwegen als Populismus bezeichnen, aber alle Vorschl\xe4ge, von denen ich gesprochen habe, funktionieren in der Welt bereits, oder sie wurden von wichtigen Experten er\xf6rtert.
Unter Hitzeeinwirkung und Druck verf\xe4rbt sich das sogenannte Landbouwplastic (KLP) zu einem dunklen, homogenen, belastungsf\xe4higen Material, das ein bissl nach Neuwagen und ein bissl nach Sportschuh riecht.
Das liegt daran, dass es gerade seine Au\xdfenpolitik umstellt und zwar weg von einer Politik, die sozusagen von den USA gemanaged wurde, hin zu einer deutschen Au\xdfenpolitik.
Deutschland ist noch nicht daran gew\xf6hnt, das ist noch immer unangenehm und, aus offensichtlichen Gr\xfcnden, f\xe4llt es dem Land noch immer schwer, eine gr\xf6\xdfere Rolle zu spielen.
Ich dachte \xfcber jenen Moment dieser Woche nach, als der zuk\xfcnftige mexikanische Pr\xe4sident Enrique Pena Nieto das Wei\xdfe Haus besuchte, um sich mit Pr\xe4sident Obama zu treffen.
Wir sollen unseren amerikanischen Kollegen davon erz\xe4hlen, wie toll ein Besuch dieses Landes ist und Druck auf die politische F\xfchrung aus\xfcben, ihre Bindungen zu Mexiko zu intensivieren.
Einen halben Tag am Flughafen auf einen Flug zu warten, ist ziemlich nervt\xf6tend - selbst, wenn B\xfccher, Magazine und iPhones (und nat\xfcrlich steuerfreies Shopping) zur Verf\xfcgung stehen.
"Wir m\xf6chten nicht in eine Position geraten, bei der wir jemanden lizenzieren und dann auf Bundesebene vor einem gro\xdfen Problem stehen", so Bob Nicholson, Mitglied des Stadtrats.
Politische Themen wie der Bergarbeiterstreik, die Privatisierung und die Ablehnung der Regierung von Sanktionen gegen das Apartheid-Regime S\xfcdafrikas fanden ihren Weg in die holzget\xe4felten R\xe4ume des Tutoriums.
Bei meiner ersten dieser Veranstaltungen sollte ich franz\xf6sische Texte aus dem 18. Jahrhundert ins Englische \xfcbersetzen. Auf das, was dann kommen sollte, war ich nicht gefasst gewesen.
Ein Studienanf\xe4nger im Fach Philosophie, Politik und Wirtschaft, der ironischerweise das als konservativ geltende Eton College besucht hatte, sagte zu mir: "Du bist die Tochter eines Faschistenschweins".
W\xe4hrend eines Tutoriums in der folgenden Woche, bei dem ein weiterer Geschichtstutor ernsthaft behauptet hatte, ich sei "ein Feind des Volkes", entschloss ich mich, dasselbe zu tun.
F\xfcr vier Euro setzen die Tr\xe4ger des indonesischen Vulkans ihr Leben und ihre Gesundheit aufs Spiel, wenn sie 70 Kilo Schwefel \xfcber die steilen, steinigen Wege tragen.
Dazu muss er jeden Tag hinunter auf den Boden seines Kraters steigen, wo sich das aus der Erde ausstr\xf6mende schwefelhaltige Gas im Kontakt mit der Luft verfestigt.
"Ich werde hier noch zwei Jahre arbeiten, weil ich einen Laden aufmachen oder Spanisch oder Franz\xf6sisch lernen m\xf6chte", verspricht er in einem mehr als nur annehmbaren Englisch.
W\xe4hrend die fallende Geburtenrate die bekannten Auswirkungen auf das Wirtschaftswachstum einer Nation, die Steuereinnahmen, die Gesundheitskosten und die Einwanderungspolitik hat, zeigt das Beispiel Singapur auch unerwartete Folgen.
M\xe4nner und Frauen f\xfchren ihre Karriere, den Stress und die Kosten f\xfcr das Eigentum und die Erziehung als Gr\xfcnde daf\xfcr an, dass sie keine Kinder haben k\xf6nnen.
Gem\xe4\xdf dem W\xf6rterbuch handelt es sich dabei um die Eigenschaft privat oder "jenen Bereich des Privatlebens, wo man Anspruch auf Schutz vor jeder Art von Einmischung hat".
Laut dem Fachmann ist die wirksamste Art und Weise, den Kindern und Jugendlichen zu lehren, was Privatsph\xe4re ist, ihnen Fragen zu stellen, die sie zum Nachdenken bringt.
Auf beiden internationalen Treffen betonten die peruanischen Beh\xf6rden, dass die Informationssysteme f\xfcr die Journalisten vorhanden w\xe4ren, sie beschr\xe4nkten aber in einem hohen Ma\xdfe den Zugang zur Information.
Das Gipfeltreffen endete auch mit der gemeinsamen Verpflichtung von Chile und Peru, ein Urteil des Gerichtshofs von Den Haag anzunehmen, das einen Grenzkonflikt zwischen beiden L\xe4ndern beilegt.
Correa versicherte, dass er diese Entscheidung nicht bedauere, weil er damit nicht seine Prinzipien verraten habe, sondern seinen "tiefen demokratischen Werten und Ansichten \xfcber Menschenrechte" nachgekommen sei.
Es soll ihnen nicht das Bier und Motel bezahlt werden, wie der Gouverneur Emilio Gonz\xe1lez auf die Frage antwortete, ob unter seiner Verwaltung Pr\xe4servative verteilt werden w\xfcrden.
"Sexualit\xe4t sieht so nicht aus; am Besten ist es, die Kondome jenen n\xe4her zu bringen, die bereits eine sexuelle T\xe4tigkeit aus\xfcben", brachte er es auf den Punkt.
Ich war Teil der erfolgreichsten \xc4ra der Nationalmannschaft von 1988 bis 1995, die die BSN anfangs der 90er Jahre bis zu 17 Mannschaften in einer Saison umfasste.
In den Jahren vor "Dallas" wurde Hagman im Fernsehen als netter Typ in den Jahren 1965 bis 1970 mit der Sitcom "Bezaubernde Jeannie" der Fernsehanstalt NBC bekannt.
Er war auch Darsteller von zwei Kom\xf6dien, die nur kurze Zeit ausgestrahlt wurden, wie z. B.The Good Life" (NBC, 1971-72) und "Here We Go Again" (ABC, 1973).
"Ich habe nicht gemerkt, dass dies das apokalyptischste Semester sein wird, das es jemals gab" sagte Charm\xe9 diese Woche den Studenten an der Universit\xe4t Rutgers-Camden (New Jersey).
"Wir nehmen 2012 nicht auf, damit wir immer die Option behalten, den Kurs neu abhalten zu k\xf6nnen, f\xfcr den Fall, dass die Welt nicht untergeht", sagte Restall.
Bei den in den USA durchgef\xfchrten Studien bestanden zahlreiche St\xf6rfaktoren zwischen den Kontrollgruppen, sodass es schwierig ist, diese Daten zu interpretieren und eindeutige Empfehlungen zu geben.
Deshalb empfehle ich den Test ab einem Alter von 50 Jahren bzw. 40 Jahren, wenn man einen direkten Verwandten hat, der bereits an Prostatakrebs erkrankt war.
In Zusammenarbeit mit der internationalen Gesellschaft f\xfcr Urologie hat Movember ein Instrument entwickelt, mit dem es m\xf6glich ist, die Vor- und Nachteile des PSA-Tests zu bewerten.
Man glaubt in der Tat, dass dieses Boson an nichts weniger als am Mechanismus beteiligt ist, der f\xfcr die Masse aller Objekte im Universum verantwortlich ist.
Und gleicherma\xdfen interagieren nicht alle Teilchen mit dem Higgs-Feld: diejenigen, die es tun, besitzen eine Masse, w\xe4hrend die anderen (wie \xfcbrigens das Photon) keine Masse besitzen.
Als ich meiner Onkologin mitgeteilt habe, dass ich die Behandlung abbrechen werde, hat sie mir geantwortet, dass sie bedauere, dass ich den Kampf aufgebe, erz\xe4hlte sie.
"Es ist merkw\xfcrdig, wie das System zerf\xe4llt, seitdem man drastische Ma\xdfnahmen ergriffen hat", witzelt Jacques Duchesneau, Abgeordneter in Quebec und ehemaliger Leiter der Polizei von Montreal.
Wir sind dabei, die Wunde zu s\xe4ubern, br\xe4uchten allerdings eine nur f\xfcr Montreal bestimmte Ermittlungseinheit, sowie eine Aufsicht, um eine R\xfcckkehr der fragw\xfcrdigen Praktiken zu verhindern.
Mithilfe des Inhalts der Datei ist es ebenfalls m\xf6glich sicherzustellen, dass die gehandelten Bitcoins in dem im gesamten Netzwerk verbreiteten Rechnungsbuch der \xf6ffentlichen Konten vorhanden sind.
Die afghanischen Frauen haben den Preis f\xfcr den Obskurantismus der von der Organisation Al-Qaida \xfcberw\xe4ltigten Bauern bezahlt, aber ihre Lage hat sich bis heute nicht verbessert.
Laut der \xc4gyptenspezialistin Sophie Pommier ist dies beunruhigend, da "die Personen, die zu einer Stellungnahme aufgefordert werden, nicht gew\xe4hlt worden sind und keinerlei demokratische Legitimit\xe4t besitzen.
Der Tatbestand der Blasphemie wird aufrechterhalten, und Beleidigungen sind jetzt verboten, was schwerwiegende Folgen f\xfcr das Recht auf freie Meinungs\xe4u\xdferung haben k\xf6nnte, insbesondere f\xfcr die Presse.
Nat\xfcrlich ist das nicht so sehr ihre Schuld, als vielmehr das \xdcbel: Nur wenige Turkmenen, Usbeken und Tadschiken k\xf6nnen sich auch nur eine vern\xfcnftige Grundschulbildung leisten.
Die Verfasser des offenen Briefs sind \xfcberzeugt, dass eine Versch\xe4rfung des Gesetzes f\xfcr private Waffenbesitzer Kriminelle nicht davon abhalten wird, sich auf dem Schwarzmarkt zu bedienen.
"Ich kann dann dort schie\xdfen, und wenn ich davon \xfcberzeugt bin, dass die Waffe einen guten Schuss hat, verhandeln wir miteinander", beschreibt der Experte das Vorgehen.
Jedoch waren nur einige Hundert Menschen vor Ort, von denen bei Weitem nicht alle in der Fast-Food-Branche besch\xe4ftigt sind, in der in New York Zehntausende arbeiten.
- Sie ist sicher nicht die Allzweckl\xf6sung, da sie Fragen zur Privatsph\xe4re aufwirft, weil man nicht immer alle Umstehenden \xfcber seine Handlungen und Absichten informieren m\xf6chte.
Sch\xf6n w\xe4re ein flexibles, Kinect-\xe4hnliches System, bei dem wir mit verschiedenen Kameraneigungen spielen k\xf6nnten, um festzustellen, wie uns das bei der dreidimensionalen Ermittlung einer Position hilft.
Irgendwann wird sie aber Realit\xe4t, wenn die Erdbewohner in ihren Raumschiffen zu einem fernen Planeten aufbrechen, der das Zuhause f\xfcr ihre im All geborenen Nachkommen wird.
Im Kreis Olomouc sind die Stra\xdfen uneingeschr\xe4nkt befahrbar, im Kreis  \u2047 ternberk m\xfcssen die Fahrer jedoch in Waldabschnitten vorsichtig fahren, da hier die Fahrbahnen noch feucht sind.
The Tap Tap ist derzeit sehr popul\xe4r. Wenn wir aber ein paar Jahre zur\xfcckgehen: Was hat Sie im Jahr 1998 dazu motiviert, eine Band zu gr\xfcnden?
Uns ist bewusst geworden, dass, wenn man etwas leistet und dies nach au\xdfen hin nicht zu sehen ist, die eigene Leistung in gewissem Sinne nicht existiert.
Alle drei Veranstaltungsorte werden zum Schluss per Live-Schaltung miteinander verbunden und es erklingt eine gemeinsame Interpretation der Hymne "Weltuntergang f\xe4llt aus" der Band The Tap Tap.
Gadomskis weltweit anerkannter Beitrag zur Entwicklung der Raumfahrt wurde u.a. dadurch gew\xfcrdigt, dass einer der Krater auf der erdabgewandten Seite des Mondes nach ihm benannt wurde.
Meteor-2 hatte ein Startgewicht von 380 kg und war in der Lage, eine Nutzlast von 10 kg in eine H\xf6he von ungef\xe4hr 60 km zu bef\xf6rdern.
Erw\xe4hnenswert ist auch der Beitritt Polens zum COSPAR (Committee for Space Research) im Jahr 1960, auf den zwei Jahre sp\xe4ter die Gr\xfcndung eines nationalen COSPAR-Ausschusses folgte.
Wie sich zeigt, gr\xfcndet sich die heutige Gesellschaft ebenso wie in der Antike auf der r\xfccksichtslosen Pr\xe4ferenz des eigenen Vorteils, ohne auf gesamtgesellschaftliche Interessen zu achten.
Vom heutigen Zustand aus gesehen, kann der Untergang dieser Regimes zugunsten liberaler Demokratien als gewisse Pause angesehen werden, bei der sich die n\xe4chste Runde schon abzeichnet.
Die Schw\xe4che von Argo ist seine allzu breite Streuung, die durch die Notwendigkeit bedingt ist, zu viel an Handlung an zu vielen Orten zeigen zu m\xfcssen.
Die Schwierigkeit besteht aber nicht nur darin, dass wir als Volk in der Kneipe und vor dem Fernseher schimpfen, aber jeden niedermachen, der etwas ver\xe4ndern will.
Den Kampf um die Burg haben Sie mit der These der materiellen und strafrechtlichen Haftung von Politikern sowie mit r\xfcckwirkenden Verm\xf6genserkl\xe4rungen \xfcber 20 Millionen Kronen aufgenommen.
Dar\xfcber habe ich noch nicht nachgedacht, weil ich keine Zeit habe, die Vergangenheit jedes potentiellen Parteimitglieds zu \xfcberpr\xfcfen, und auch gar nicht das Geld daf\xfcr habe.
Die MVRDV Architekten beweisen, dass die wahren Abenteuer nicht nur im Kopf sind - am Beispiel von Spijkenisse und dem j\xfcngst errichteten B\xfccherberg - 2 Fotos
Nach Angaben der Marktforschungsgesellschaft CLSA ist China mit einem Volumen von 15 Milliarden Euro im Jahr der drittgr\xf6\xdfte Markt f\xfcr Luxusartikel und der am schnellsten wachsende.
Man selbst habe das vers\xe4umt, da in Deutschland Familiennamen nicht gesch\xfctzt werden k\xf6nnten, sagt Hanno Wentzler, der Vorsitzende der Gesch\xe4ftsf\xfchrung von Freudenberg Chemical Specialities in M\xfcnchen.
Es reiche nicht aus, sich auf internationale Markenrechte zu verlassen, vielmehr sollten die Ausl\xe4nder "alles, was irgendwie sch\xfctzenswert ist, auch in China anmelden", wie Wentzler sagt.
Denn 8 733 Kilometer Luftlinie von Heidelberg entfernt, im Nordwesten des K\xf6nigreichs Swasiland, gibt es das Dorf Esitjeni, das von der Stimmgewalt des deutschen Chores abh\xe4ngt.
Die gut organisierte Muslimbruderschaft blies ihrerseits zur Gegendemonstration, vorsichtshalber aber nicht auf dem Tahrir-Platz, sondern nach einem Massengebet auf dem anderen Nilufer vor der Kairoer Universit\xe4t.
Rakfisk ist mit Salz bestreute Forelle, die - abh\xe4ngig davon, wie stinkend man seinen Fisch gerne h\xe4tte - bis zu ein Jahr in Wasser fermentiert wird.
Wenn man es vermeidet, den Rakfisk in Nasenn\xe4he zu bringen, ist er nicht schlecht - etwa wie Sushi, das eine recht lange Busfahrt hinter sich hat.
Rakfisk ist das Produkt einer ganz anderen, weitaus \xe4rmeren norwegischen Epoche, als es noch keine K\xfchlm\xf6glichkeiten gab und Fisch im Herbst in luftdichten Salzwasserf\xe4ssern getr\xe4nkt wurde.
Das Milit\xe4r sagte aus, es habe ihm diesen restriktiven Status - der eine Stufe unter der Selbstmordgef\xe4hrdung steht - zu seinem und dem Schutz anderer zugewiesen.
Auf einer k\xfcrzlichen Reise nach Mexiko-Stadt hatte ich gerade erst die Halle durchquert und war an der Passkontrolle angekommen, als sich Ratlosigkeit in mir breit machte.
Und doch liegt die gr\xf6\xdfte Herausforderung Mexikos in Wahrheit in der Beziehung mit den mehr als 35 Millionen mexikanischen Amerikanern, die in den Vereinigten Staaten leben.
Tats\xe4chlich, so sagt er, wissen wir nun, dass Herumzappeln und Kritzeln, oft als Zeichen f\xfcr Langeweile interpretiert, diese sogar bek\xe4mpfen k\xf6nnen, indem Personen k\xf6rperlich aufmerksamer bleiben.
Andererseits untersuchen viele Philosophen und Autoren die Beziehung zwischen Langeweile und Kreativit\xe4t. Dieser Meinung ist Professor Vodanovich, der das Thema seit mehr als zwei Jahrzehnten erforscht.
"Colorado hat einen st\xe4rker regulierten Markt. Der Staat eignet sich daher gut zur Orientierung", sagt Brian E. Smith, Sprecher der Aufsichtsbeh\xf6rde f\xfcr Spirituosen im Staat Washington.
Aktuell m\xfcssen sich 119 Personen f\xfcr den Besitz von etwa 50 Gramm oder weniger Marihuana vor Gericht verantworten, obwohl viele auch f\xfcr andere Delikte angeklagt wurden.
"Sie haben einen derart gro\xdfen Teil ihres Lebens damit verbracht, Personen daf\xfcr strafrechtlich zu verfolgen, dass sie die Legalisierung immer noch nicht akzeptieren k\xf6nnen", glaubt er.
Die Prinzessin D'Arenberg bewahrt ihre Abendkleider des Modemachers "mit absoluter Sorgfalt" auf, "weil ein Kleid nicht nur ein Kleid ist, sondern auch die damit verbundenen Erinnerungen".
Die Werbefirma BBH, die das Video gedreht hat, wahrt die Hoffnung, dass der Werbespot auf lustige Art und Weise erreicht, auf das Problem aufmerksam zu machen.
Der Anstieg der Immigration wird auch als einer der Gr\xfcnde daf\xfcr angesehen, dass die Regierungspartei in Singapur letztes Jahr ihr schlechtestes Wahlergebnis seit der Unabh\xe4ngigkeit erzielte.
Der Junge ist sich dar\xfcber im Klaren, dass es falsch ist, obsz\xf6ne Fotos, von Nackten, von Verbrechen zu ver\xf6ffentlichen, oder beleidigende oder gewaltsame Kommentare zu schreiben.
"Sie sollen auch w\xe4hlerisch sein, wenn es ihnen am Wichtigsten ist, beliebt zu sein, tausende Freunde zu haben, ohne \xfcber die Folgen nachzudenken", f\xfcgt er hinzu.
Die wenigen Informationen, die unter den Journalisten zirkulierten, wurden von den Pressesprechern einiger der beim Treffen anwesenden Regierungen der Unasur erhalten, aber nicht vom peruanischen Pressesprecher.
Argentinien, Bolivien, Kolumbien, Ecuador, Peru, Brasilien, Uruguay, Venezuela, Chile, Guyana, Surinam und Paraguay sind Mitglieder bei der UNASUR, auch wenn das letztere Land derzeit ausgeschlossen ist.
"Es war, als ob eine Bombe einschlug", sagt er \xfcber den Moment, in dem er die Diagnose erhielt, die der Arzt ohne erkennbaren Erfolg "abzuschw\xe4chen versuchte".
Tats\xe4chlich wurde zu diesem Zweck das Modellgesetz der Vereinten Nationen f\xfcr die Vereinheitlichung des internationalen Handelsrechts geschaffen, wobei das American Law Institute als Schlichter eingesetzt wurde.
Andererseits gibt es Vitro Schuld f\xfcr seine schwierige Situation ab 2008 im Rahmen der gro\xdfen wirtschaftlichen Krise in den Vereinigten Staaten, die dem Land Schl\xe4ge erteilte.
Dass die Jungs in Ponce z. B. nur in ihrem Gebiet spielen und erst in den nationalen Playoffs auf Mannschaften aus anderen Ecken der Insel treffen.
Er versuchte sein Gl\xfcck auf den Theaterb\xfchnen in New York Anfang der 50er Jahre, danach diente er von 1952 bis 1956 in den Luftstreitkr\xe4ften in England.
Und er ist nicht der einzige Professor, der dieses Semester, das eigentlich das letzte in der Geschichte sein sollte, Kurse \xfcber das "Ende der Welt" anbietet.
Der PSA-Test weise in der Tat manchmal fehlerhafte Ergebnisse auf, mit falschen negativen oder aber auch falschen positiven Ergebnissen, die zu unn\xf6tigen medizinischen Eingriffen f\xfchren.
Obwohl es nicht der urspr\xfcngliche Zweck war, dient dieser Sensor heute allen Digitalkameras weltweit als "Auge" und hat ihm 2009 den Nobelpreis f\xfcr Physik eingebracht.
"Seit sechs Monaten sind drei bis f\xfcnf Betten immer mit Krebspatienten im Alter von weniger als 45 Jahren belegt", teilt Dr. Christiane Martel beunruhigt mit.
Die Charbonneau-Kommission "hat bereits zwei B\xfcrgermeister zu Fall gebracht", f\xfcgt er hinzu, in der Hoffnung, dass es ihr gelingt, "die Taktiken hinter den Einzelpersonen aufzuzeigen".
Auch wenn die gro\xdfen Mannschaften wie Marseille, Lyon oder Bordeaux um den Titel ringen, glaube ich, dass wir das Zeug dazu haben, ihn zu gewinnen.
Betrachten Sie Manchester City, ein Verein der seit zwei Saisons nicht schafft, sich f\xfcr das Achtelfinale zu qualifizieren, und der ebenfalls riesige Ausgaben get\xe4tigt hat!
Aus dem, was sich in der Ukraine ereignet hat, haben wir unsere Lehre gezogen, und heute m\xfcssen wir ein vorbildliches Verhalten an den Tag legen.
Dar\xfcber hinaus ist wie so oft in diesen Technologien eine politische Vision greifbar: die \xdcberzeugung, dass das aktuelle, von Bankmonopolen gestaltete W\xe4hrungssystem, zu Finanzkrisen f\xfchrt.
K\xfcrzlich haben Adi Shamir und Dorit Ron vom Weizmann-Institut in Israel das Rechnungsbuch analysiert und gezeigt, dass fast 80% der Bitcoins nicht im Umlauf sind.
\xc4gypten st\xfctzt sich jetzt seit fast zwei Jahren auf einen vorl\xe4ufigen, mehrfach abge\xe4nderten Text, was die institutionelle Stabilit\xe4t schw\xe4cht und zu einem rechtlichen Durcheinander f\xfchrt.
Im Norden des Landes in 1600 bis 2040 Meter H\xf6he befindet sich das ber\xfchmte Skigebiet Hermon, in das es in den Wintermonaten unz\xe4hlige Touristen zieht.
In Akko k\xf6nnen Sie das Museum im Bad Al Basha besuchen, das mehrere S\xe4le alter t\xfcrkischer B\xe4der mit Skulpturen der damaligen Besucher und Badediener beherbergt.
Denn in ihren Familien gibt es noch nicht einmal Geld, um die Kinder zu ern\xe4hren, geschweige denn, ihnen anst\xe4ndige Kleidung, Schuhe und Schulsachen zu kaufen.
Nat\xfcrlich erhielten die neuen Besitzer diese nicht umsonst: Jeder Migrant, der hoffte, sich so die Tests ersparen zu k\xf6nnen, zahlte f\xfcr das Dokument siebentausend Rubel.
Die Polizei will das Tragen nicht-t\xf6dlicher Waffen in der \xd6ffentlichkeit verbieten und das Alter f\xfcr den Besitz von Schusswaffen von 18 auf 21 Jahre heraufsetzen.
Den Daten der Forscher zufolge stammen 17% der Waffen aus Konfliktgebieten, 14% gehen auf Diebst\xe4hle bei der Waffenproduktion zur\xfcck, und 5% stammen aus illegalen Ausgrabungen.
"Um eine Waffe zu besorgen, ben\xf6tige ich einen Bekannten, der Kontakte hat", erz\xe4hlt der Verkaufsberater. "Ich habe so einen Bekannten, aber ich vertraue ihm nicht".
Zuerst pr\xe4sentierte Google im Sommer bei seiner j\xe4hrlichen Konferenz ein funktionierendes Modell, im November wurde dann bekannt, dass auch Microsoft ein entsprechendes Patent angemeldet hatte.
Ich befreundete mich mit den Malern der neuen Generation, also mit den Vertretern der "Gazonewschina"; daraus entstand "Puschkinskaja 10", und dann war erst einmal Schluss.
Im Jahr 1988 gebar die zweite Frau im All, Swetlana Sawizkaja, die zweimal im Orbit war und sogar Arbeiten au\xdferhalb des Raumfahrzeugs verrichtete, einen Sohn.
Damit best\xe4tigt sich, dass es nicht reicht, immer wieder neue und genauere Regeln aufzustellen. Man muss sich auch mit der eigentlichen Anwendung des Rechts befassen.
Wirtschaftlichkeit bedeutet, eine Sache zu einem vern\xfcnftigen Preis (was nicht immer der niedrigste Preis ist) zu erwerben und unrechtm\xe4\xdfige Bereicherung oder gar kriminelle Handlungen auszuschlie\xdfen.
Zu Eisgl\xe4tte kann es insbesondere auf Verkehrswegen der zweiten und dritten Stra\xdfenklasse in den Kreisen Lan \u2047 kroun,  \u2047 st\xed nad Orlic\xed, Poli \u2047 ka, Svitavy und Vysok\xe9 M \u2047 to kommen.
Auf dem Pass  \u2047 ervenohorsk\xe9 sedlo m\xfcssen die Fahrer in Richtung Jesen\xedk mit Schneematsch rechnen", sagte ein Mitarbeiter der Stra\xdfenverwaltung  \u2047 umperk heute gegen\xfcber der Agentur  \u2047 TK.
Nach Angaben von Meteorologen gab es hierf\xfcr in der Nacht ideale Bedingungen - tags\xfcber Regen und schmelzender Schnee, in der Nacht wolkenloser Himmel und Frost.
Die Band The Tap Tap hat zusammen mit anderen Interpreten au\xdferdem auch die sog. Hymne gegen den Weltuntergang mit dem Titel "Weltuntergang f\xe4llt aus" aufgenommen.
Im Mai treten wir zum ersten Mal beim Prager Fr\xfchling auf, und auch f\xfcr dieses Konzert bereiten wir ein interessantes Programm mit interessanten G\xe4sten vor.
Seit 1956 beteiligte sich die PTA ma\xdfgeblich an der Entwicklung der \xe4u\xdferst erfolgreichen meteorologischen Rakete (Rakieta Meteorologiczna), der ersten polnischen Rakete f\xfcr die wissenschaftliche Forschung.
In Deutschland gibt es schon seit einigen Jahren \xf6ffentliche Lebensmittelabgabestellen f\xfcr Arme, die nicht mehr in der Lage sind, sich durch eigene Arbeit zu ern\xe4hren.
Dann muss man sich aber fragen, ob nicht das Privatkapital die Politik und damit den gesamten Staat im eigenen egoistischen Sinne beeinflusst oder gar lenkt.
Die Ursache f\xfcr das Aufkommen des Faschismus und des Kommunismus m\xfcssen wir daher in der r\xfccksichtslosen Liberalisierung der Wirtschaftssysteme im 19. und 20. Jahrhundert suchen.
Es war ein schwerer Schlag f\xfcr den Ruf der vereinigten Staaten, und das anschlie\xdfende Fiasko beim gewaltsamen Versuch der Geiselbefreiung machte alles nur noch schlimmer.
Ich wei\xdf, dass ich allein nichts erreiche; deshalb habe ich mit mehreren bekannten Pers\xf6nlichkeiten dar\xfcber gesprochen, ob sie nicht auch f\xfcr den Senat kandidieren m\xf6chten.
"Ich finde das Geb\xe4ude lustig, es sieht futuristisch aus, und endlich gibt es wieder etwas Interessantes zu sehen", sagt Lisette Verhaig, eine Passantin am Stra\xdfenrand.
"Normalerweise stehen die B\xfccherregale entlang der Fassade, und in der Mitte liegt ein gro\xdfer, dunkler Raum, der meist ungem\xfctlich und unpers\xf6nlich ist", sagt Winy Maas.
Deutsche Welle: Anfang der Woche hatte Deutschland zun\xe4chst signalisiert, dass es gegen den Antrag auf einen Beobachterstatus der Pal\xe4stinenser bei den Vereinten Nationen stimmen w\xfcrde.
Nun nimmt der Einfluss der USA in der europ\xe4ischen Politik kontinuierlich ab, die EU f\xfcllt im Moment dieses Vakuum aber nicht, wer bleibt da sonst?
Am 14. September 2010 lie\xdf dort ein chinesisches Unternehmen das Warenzeichen Zegna DF Puma sch\xfctzen, einen Kunstnamen, der sich auch beim Modehaus Ermenegildo Zegna bediente.
In der Tat: Falls Freudenberg im letzten Akt seines Markendramas unterliege, dann m\xfcsste man wohl der Gegenseite Lizenzgeb\xfchren f\xfcr den eigenen Namen zahlen, erkl\xe4rt Wentzler.
Hier lebt die kaukasische Volksgruppe der Talyschen, von der nicht viel bekannt ist, au\xdfer dass sie perfekt Persisch sowie Aserisch spricht und sehr langlebig ist.
"Baku wurde im Mai mit dem Eurovision-Song-Festival ber\xfchmt - und im n\xe4chsten Jahr haben wir hier ein Festival der \xe4ltesten Menschen der Welt", sagt Fatulayeva.
Auslegungssache, wie so vieles in dem Entwurf, der Mursi zur Unterschrift vorliegt und nach seinen Worten "sehr bald" den \xc4gyptern zur Volksabstimmung pr\xe4sentiert werden wird.
Der 48-j\xe4hrige Menschenrechtsanwalt und Vorsitzende der \xe4gyptischen Organisation f\xfcr Menschenrechte (EOHR) verteidigte die Muslimbr\xfcder, als sie unter Mubarak im Gef\xe4ngnis sa\xdfen oder vor Gericht standen.
Noch vor einer Generation sahen sich tausende Norweger auf der Suche nach Arbeit gezwungen, ihr Land zu verlassen und wanderten haupts\xe4chlich in die USA aus.
Hier hasst man es immer noch, Anders Breivik beim Namen zu nennen - jenen rassistischen Rechtsextremisten, der letztes Jahr 77 M\xe4nner, Frauen und Kinder erschoss.
Anfang dieses Jahres wurde das Milit\xe4r eingeschaltet, um die in den Vierteln operierenden Drogenbanden zu bek\xe4mpfen, und Gewalt gegen Frauen ist ein besonders akutes Problem.
Manning habe dem Beamten gesagt, er h\xe4tte den Bund seiner Unterhose oder seiner Flip-Flops benutzen k\xf6nnen, um sich selbst zu verletzen, dies jedoch nicht getan.
Die Verteidigung hat angegeben, dass Manning sich geringerer Vergehen f\xfcr schuldig bekennen wird, w\xe4hrend andere Anklagepunkte, die als zu extrem angesehen werden, angefochten werden sollen.
Das Pentagon bleibt bei seiner Position, dass Manning gem\xe4\xdf der Bestimmungen festgehalten wurde, die f\xfcr alle unter den h\xf6chsten Sicherheitsvorkehrungen in Quantico verwahrten H\xe4ftlinge gelten.
Und dann w\xfcrden wir uns jetzt nicht hinter dem Seidenvorhang gefangen sehen - mit einem angenehmen Leben in den Vereinigten Staaten, aber doch irgendwie verloren.
Der arabische Fr\xfchling hat eine neue, ungewisse Situation geschaffen, und ob sie es wollen oder nicht - Pal\xe4stinenser und Israelis sind Teil dieser Wirren geworden.
"Die Regierung h\xe4tte Zigaretten einfach komplett verbieten sollen - dann h\xe4tten wir uns gesagt okay, das war's, wir machen dicht", f\xfcgt er sichtlich erbost hinzu.
Und weil die meisten von uns heutzutage fast st\xe4ndig auf den ein oder anderen Bildschirm starren, kommen uns die Vorteile der Langeweile nicht mehr zugute.
Die Schl\xfcsselerfahrung der Langeweile, sagt er, bestehe in einer "St\xf6rung des Aufmerksamkeitsprozesses, gepaart mit schlechter Laune und dem Gef\xfchl, dass die Zeit nur langsam vergeht".
Er sei sich jedoch sicher, dass "die Jugend als besonders langweilig empfunden wird", haupts\xe4chlich, weil Kinder und Teenager keinen gro\xdfen Einfluss auf ihren Alltagsablauf haben.
"Mit der Langeweile will das Gehirn einem sagen, dass man etwas anderes tun sollte", so Gary Marcus, Professor f\xfcr Psychologie an der Universit\xe4t New York.
Orozco zufolge waren er und einige Freunde an einem Septembertag mit dem Auto in Lamar nahe der Grenze zu Kansas unterwegs, als sie angehalten wurden.
Der einzige Tutor, der sich offen als Tory zu erkennen gab, war Norman Stone, Professor f\xfcr zeitgen\xf6ssische Geschichte, der seinen Sitz in meinem College hatte.
Er wurde nicht nur daf\xfcr gehasst, ein Konservativer zu sein, sondern auch, weil er Thatcher in Sachen Au\xdfenpolitik beraten und f\xfcr sie Reden geschrieben hatte.
Diese Ausstellung ist der Abschluss einer Geschichte, deren einziger Protagonist "il signore" Garavani ist, die aber ohne seine distinguierte Klientel nicht h\xe4tte geschrieben werden k\xf6nnen.
"Ich ziehe ihn allen anderen wegen seiner gro\xdfen Liebe f\xfcr die Frauen und weil er unsere Sch\xf6nheit hervorhebt, vor", f\xfcgt die Ex-Herzogin von Feria hinzu.
Sie wissen, dass jeder Schritt ihr Leben kosten kann, wie dies einer franz\xf6sischen Touristin passierte, die vor Jahren an den Steilh\xe4ngen des Kawah Ijen abst\xfcrzte.
F\xfcr jede Strecke ben\xf6tigt er drei Stunden, wonach er v\xf6llig geschafft ist, am Ende des Tages hat er aber dann 138.000 Rupien (11,5 Euro) zusammen.
Was wie ein miserabler Lohn f\xfcr eine solch schier unmenschliche Anstrengung aussieht, ist aber das Dreifache von dem, was er mit der Feldarbeit verdienen w\xfcrde.
Die Schatten herausfordernd, steigt er im Licht einer kleinen Stirnlampe an seinem Helm, die er sich von seinem eigenen Geld gekauft hat, in den Krater.
Allerdings besteht die Sorge, dass sie den Lebensstil des Alleinstehenden f\xf6rdern k\xf6nnen, und dass sie die Baufirmen davon abschrecken, gro\xdfe Wohnung f\xfcr Familien zu bauen.
Wenn sie alle Abschnitte verstehen, verf\xfcgen sie \xfcber solide Grundlagen, um mit ihren Kindern \xfcber die Bedeutung des Er\xf6ffnens eins Benutzerkontos im Internet zu reden.
Der Pr\xe4sident von Ecuador, Rafael Correa, best\xe4tigte heute, dass die Schaffung einer gemeinsamen Staatsb\xfcrgerschaft ein Ziel ist, wobei "S\xfcdamerika tats\xe4chlich etwas von Europa lernen kann."
Macht hat mich pers\xf6nlich nie interessiert, aber unter so ungerechten Umst\xe4nden wie in Ecuador kann diese sozio\xf6konomische Armut nur von der politischen Macht korrigiert werden.
Das von Carlos D\xedaz Ch\xe1vez Morineau angef\xfchrte Gesuch hat nun ein Strafverfahren gegen die Nationale Bank- und Wertpapierkommission eingereicht, der Behinderung der Justiz vorgeworfen wird.
Die Meisterschaft der Vaqueros mit Gausse wurde ihm gew\xe4hrt, aber schon aus einem Abstand heraus, weil er 1988 bereits an oberster Stelle des Verbands stand.
Geboren in Fort Worth, Texas, war er der Sohn der Schauspielerin und S\xe4ngerin Mary Martin, die klassische Werke wie "South Pacific" und "Peter Pan" spielte.
"Ich habe nichts geschrieben, von dem ich glaubte, dass es jemandem schaden oder ihn auf irgendeine weise beeintr\xe4chtigen k\xf6nnte", sagte der der Associated Press seinerzeit.
Ich m\xf6chte ihnen etwas Trost spenden, wie z. B. "keine Angst, es ist ein bisschen unbequem die erste Zeit, aber es wird Ihnen gut gehen".
In diesem Sinne hat die Mehrheit der amerikanischen Regierungen seit 2009 neue Gesetze verk\xfcndet, die das Verfahren f\xfcr die Registrierung oder den Urnengang erschweren.
Dieses Ph\xe4nomen hat nach den Wahlen vom November 2010 an Bedeutung gewonnen, bei denen 675 neue republikanische Vertreter in 26 Staaten verzeichnet werden konnten.
Eine weitere Studie, dieses Mal aus Europa, kam zu der Schlussfolgerung, dass ein Unterschied bei der Sterblichkeit von Patienten mit und ohne Fr\xfcherkennung besteht.
Trotz der Fortschritte in der Forschung bleibt die Annahme einer gesunden Lebensweise der beste Weg, um das Risiko zu verringern, an ihm zu erkranken.
Wir wissen ohne den Schatten eines Zweifels, dass wir ein echtes neues Teilchen haben, und dass es dem vom Standardmodell vorausgesagten Higgs-Boson stark \xe4hnelt.
\xdcbrigens: in den fr\xfchen 60er Jahren haben die Pioniere des Lasers in den Bell-Laboren nicht vermutet, dass ihre Arbeiten eine derartige Revolution ausl\xf6sen w\xfcrden.
Nat\xfcrlich bedeutet dies nicht, dass die Aktivit\xe4ten des LHC zwangsl\xe4ufig unser Leben ver\xe4ndern werden, aber es bedeutet, dass man es wirklich nie wissen kann...
Ich hoffe, dass wir im Monat Mai der l\xe4chelnde Sieger sein werden und uns sagen, dass wir sie trotz aller Schwierigkeiten schlie\xdflich gewonnen haben.
Die EZB sieht in ihrem Bericht \xfcbrigens vor, die verschiedenen, heute als hoch angesehenen Risiken im Falle eines Erfolgs dieser W\xe4hrung neu zu bewerten.
Diesen jungen Menschen, die weder zum Obskurantismus der einstigen Parteien noch zur Korruption gewisser F\xfchrungskr\xe4fte zur\xfcckkehren wollen, wird man Arbeitspl\xe4tze zur Verf\xfcgung stellen m\xfcssen.
Ehemalige Kommandeure des antisowjetischen Kampfes bem\xfchen sich bereits um die Wiederherstellung der Milizen in der Provinz, die sich der Macht der Zentralregierung entziehen werden.
Ohne Energie, um das Eisen- oder Kupfererz vor Ort zu verarbeiten, bzw. ohne Transportmittel f\xfcr einen Export \xfcber die Berge ist kein Bergbau m\xf6glich.
Eines Tages wird es auch erforderlich sein, dass Afghanistan und Pakistan, von dem weitgehend die Ein- und Ausfuhren abh\xe4ngig sind, wieder normale Beziehungen herstellen.
Die Bef\xfcrchtungen der Liberalen werden au\xdferdem von der Tatsache gen\xe4hrt, dass der n\xe4chste Rektor dieser Universit\xe4t weitaus weniger gem\xe4\xdfigt als der jetzige sein d\xfcrfte.
Er r\xe4umt aber ein, "dass in Bezug auf den Artikel 220 eine Mehrdeutigkeit vorliegen kann, da die verwendeten Begriffe dem religi\xf6sen Wortschatz entlehnt sind.
Bereits an dem Tag, an dem das Gesetz in Kraft trat, stellte sich heraus, dass nicht nur die Registrierungsdokumente der Migranten gef\xe4lscht sein k\xf6nnen.
F\xfcr den Moment k\xf6nnen die Beh\xf6rden Gastarbeitern, die beim ersten Mal durch den Test fallen, nur versprechen, dass sie Zeit f\xfcr einen Sprachgrundkurs erhalten.
Im Internet wurde ein offener Brief ver\xf6ffentlicht, dessen Verfasser - Vertreter verschiedener Waffenverb\xe4nde - von den Beh\xf6rden fordern, von "sinnlosen Versch\xe4rfungen" Abstand zu nehmen.
Die Experten analysierten Berichte des Innenministeriums und des F\xf6deralen Dienstes f\xfcr Staatliche Statistik, kriminologische Literatur und \xf6ffentlich zug\xe4ngliche Daten auf Portalen zum Thema Waffen.
"Als Antwort erh\xe4lt er ein Foto und eine Beschreibung des Verstecks der Waffe", berichtet der Pressesprecher der gemeinn\xfctzigen Organisation "Pravo na oryzhie" Dmitrij Kislow.
Beispielsweise sind die Xbox-Konsole und die Kinect-Sensoren ein Fortschritt, und heutzutage wird keine Xbox mehr ohne Kinect verkauft, da sich alle f\xfcr Bewegungssteuerung interessieren.
Gerade das macht die Arbeit auf dem Gebiet der virtuellen Realit\xe4t f\xfcr einen Forscher so anziehend: Bei vielen Themen stehen wir erst am Anfang.
Dann ging die Zeit der alten freien, jedoch nicht offiziell anerkannten Maler damals zu Ende, und neue und freie Maler wie ich waren unverst\xe4ndlich.
Es ist nicht leicht, in neuen Zeiten nach alten Regeln zu arbeiten; ich bin ein Mensch der Wahrheit, Ehrlichkeit und Kultur des vergangenen Jahrhunderts.
In meiner Jugend habe ich solche Bilder gemalt, die bei einem Sammler sogar in einer Reihe mit den Werken von Falk und Larionow hingen.
Bei den echten Zaren war es anders, denn die Zaren verstanden vielleicht nicht viel von Kultur, aber sie verstanden, dass richtige Experten notwendig sind.
"Je mehr, desto gef\xe4hrlicher ist es selbst bei Fl\xfcgen in den Orbit", schlussfolgert Kosmonaut Waleri Poljakow, Held der Sowjetunion und Held der Russischen F\xf6deration.
Er kann sagen: "Wir \xe4ndern das Gesetz und erlauben die Sache", aber er kann nicht sagen, dass wir so tun, als wenn nichts w\xe4re.
Das Vergabegesetz enth\xe4lt relativ strenge Regeln \xfcber die formale Ausf\xfchrung bestimmter Vorg\xe4nge - und das ist f\xfcr den Schutz des \xf6ffentlichen Wettbewerbs auch richtig.
Durch Ihre Auslandsreisen haben Sie einen Vergleich, wie es in den einzelnen L\xe4ndern mit Barrierefreiheit aussieht, wie man dort mit behinderten Menschen umgeht usw.
Damals fing ich als Betreuer im Jedli \u2047 ka-Institut an, wo ich vielen jungen Leuten begegnete, die daran interessiert waren, sich mit etwas intensiv zu besch\xe4ftigen.
Ich sage immer, dass wenn Menschen mit Behinderungen etwas gelingt, dies nicht nur f\xfcr sie selbst ein Fortschritt ist, sondern f\xfcr die ganze Gesellschaft.
Das Ergebnis ist eine verzweifelte Situation im Bereich der Korruption, der gegenseitigen Bevorteilung, einer Gesetzgebung, in der praktisch alles str\xe4flich, aber nichts strafbar ist.
In Deutschland ist die Situation so, dass ein Staatsministerium mangels Finanzen private, dicht mit der Industrie verflochtene Rechtsunternehmen mit der Ausarbeitung von Gesetzentw\xfcrfen beauftragt.
Alle Gewalt geht dann nicht mehr vom Volke aus, wie es die westlichen Verfassungen verk\xfcnden, sondern von starken Finanzgruppen, die ihre eigenen Interessen vorziehen.
Die bereits erw\xe4hnte Balfour-Deklaration schuf die Voraussetzung f\xfcr die Masseneinwanderung von Juden nach Pal\xe4stina; es kam zu ersten Zusammenst\xf6\xdfen mit der ans\xe4ssigen arabischen Bev\xf6lkerung.
Gleichzeitig war sie nicht in der Lage, im Iran, wo die Revolution in die Einsetzung eines theokratischen Regimes m\xfcndete, die Freilassung der Geiseln durchzusetzen.
Damit die Tarnung glaubw\xfcrdig wurde, erschienen Artikel \xfcber dieses Filmprojekt in Fachzeitschriften, es wurden Pressekonferenzen abgehalten, und die fiktive Produktionsgesellschaft hatte ein reales B\xfcro.
Und dann gibt es noch die Szenen aus der CIA-Zentrale und anderen Institutionen - M\xe4nner in Anz\xfcgen am Besprechungstisch, auf den Amtsfluren, am Telefon...
Mein Vorteil besteht darin, dass ich mir ohne Schubladendenken und Parteidogmen von jeder Partei das nehmen kann, was f\xfcr unser Land das Beste ist.
Oder meinen Sie, dass es Ihnen, wenn Sie nur lange genug mit den Leuten reden, gelingen wird, beispielsweise die materielle und strafrechtliche Haftung durchzusetzen?
Ich versuche immer, die Dinge selbst zu beurteilen; und wenn es nicht klappt, dann gehe ich in sechs Jahren wieder in den Privatsektor zur\xfcck.
Aber vom Senatorengehalt allein k\xf6nnte ich nicht leben; so k\xf6nnte ich z.B. meinem Sohn nicht die englische Schule finanzieren, die 30.000 pro Monat kostet.
Hat Deutschland seine Beziehungen mit den USA besch\xe4digt, indem es sich bei wichtigen Entscheidungen der Stimme enthalten hat, etwa bei der Abstimmung \xfcber Pal\xe4stina?
Es w\xe4re nat\xfcrlich ein bisschen einfacher f\xfcr die Deutschen, wenn es eine koh\xe4rente und einheitliche europ\xe4ische Politik g\xe4be, was derzeit nicht der Fall ist.
Das sei ein Rekord und bedeute, dass China zum zehnten Mal hintereinander die Liste der Neuanmeldungen in aller Welt anf\xfchre, teilt die Beh\xf6rde mit.
Doch schon ein Jahr sp\xe4ter gr\xfcndete der Chor den Verein "Voices for Africa", der sich seither fast professionell um die Aids-Waisen in Esitjeni k\xfcmmert.
Die Zahl der Syphilis-Infektionen hat sich laut dem Robert-Koch-Institut von 1697 Erkrankungen im Jahr 2001 auf 3698 Erkrankungen im Jahr 2011 mehr als verdoppelt.
Obwohl er der Sonne am n\xe4chsten liegt, gibt es auch dort gefrorenes Wasser, wie aus drei am Donnerstag im Fachmagazin "Science" ver\xf6ffentlichten Studien hervorgeht.
Niemand bringe den Fund von Eis aber mit der Existenz von Leben auf dem Planeten in Zusammenhang, sagte der Chefwissenschaftler der Messenger-Sonde, Sean Solomon.
Diese sternenbildende Region - von Wissenschaftlern unromantisch W5 genannt - hat das Teleskop Spitzer im Sternenbild Cassiopeia entdeckt, in einer Entfernung von 6500 Lichtjahren.
Der Mann sei drei Mal verheiratet gewesen und habe 23 Kinder gehabt, im Alter von 136 Jahren soll er noch eine Tochter gezeugt haben.
Mirzayevas wei\xdfe Z\xe4hne stehen perfekt in Reih und Glied, unter ihrem Kopftuch verbirgt sie lange, dunkelblonde Z\xf6pfe, die ihr Sohn stolz vor uns enth\xfcllt.
230 Manat (etwa die gleiche Summe in Euro), erh\xe4lt Mirzayeva monatlich als Rente, f\xfcr hiesige Verh\xe4ltnisse ein Betrag, von dem man gut leben kann.
Tats\xe4chlich sind die 234 Artikel, die von der islamistisch dominierten 100-k\xf6pfigen Verfassungsgebenden Versammlung da in einem n\xe4chtlichen, 15-st\xfcndigen Parforceritt durchgepeitscht wurden, teilweise Besorgnis erregend.
Saeda f\xfchlt sich allein gelassen, auch von der internationalen Gemeinschaft, die den ideologischen Richtungskampf am Nil mit einer Mischung aus Neugier und Spannung betrachtet.
Norwegen ist mit seinem \xd6lreichtum sehr vorsichtig umgegangen - ein gro\xdfer Teil der Branchenertr\xe4ge wird zum Wohle zuk\xfcnftiger Generationen in einen besonderen Fonds investiert.
Als in den Jahren bis zur Weltwirtschaftskrise alle mit Geld um sich warfen, das sie gar nicht besa\xdfen, hielt Norwegen seine Geldb\xf6rse fest verschlossen.
"Meine Regierung engagiert sich stark daf\xfcr, die Gewalt zu reduzieren", erkl\xe4rte Pena Nieto Anfang dieser Woche im Oval Office dem US-amerikanischen Pr\xe4sidenten Barack Obama.
Der Kongressabgeordnete Olvera gibt zu, dass die Partei nach 12 Jahren au\xdferhalb des Pr\xe4sidentenpalasts von Los Pinos gro\xdfe Erwartungen an Enrique Pena Nieto stellt.
In einem Betonbau, typisch f\xfcr das heruntergekommene Viertel, k\xe4mpft Irinea Buendia mit den Tr\xe4nen, als sie mir Fotos ihrer verstorbenen Tochter Mariana Luna zeigt.
Hosni Mubarak, der laizistische Despot, der \xc4gypten bis zu seinem Sturz 2011 30 Jahre lang regierte, hatte nur wenig Zeit f\xfcr die Hamas \xfcbrig.
In diplomatischer Hinsicht halten die Vereinigten Staaten unersch\xfctterlich an ihrer Position fest. Viele europ\xe4ische L\xe4nder haben die Hamas f\xfcr die neuesten Gewalteskalationen verantwortlich gemacht.
Netanyahu steht gut da. Seine Likud-Partei hat sich im Vorfeld der Wahlen am 22. Januar unter Avigdor Lieberman mit einer noch k\xe4mpferischeren Gruppe verb\xfcndet.
Auf sozialen Medien wie YouTube, Twitter und Facebook hat Freeman einen Anstieg an Erfahrungsberichten zu Marken festgestellt, die von "ganz normalen Leuten" verfasst wurden.
James Yu, Betreiber des Tabakhandels "King of the Pack" in der Innenstadt von Sydney, sagt, die einheitliche Verpackung habe das Auff\xfcllen seiner Regale erschwert.
Dieses Thanksgiving verbrachte ich unerwartet f\xfcnf Stunden im Flughafen, als unser Flugzeug aufgrund mechanischer Probleme ausfiel und wir auf einen anderen Flieger warten mussten.
"Studien haben gezeigt, dass Kinder, die herumhampeln d\xfcrfen, mehr lernen und mehr Informationen behalten als diejenigen, die zum Stillsitzen gezwungen werden", so Professor Fenske.
Chief Oates f\xfcgte hinzu, dass die Polizei weiterhin st\xe4dtische Vorgaben zur Regulierung von Anbauern von medizinischem Marihuana durchsetzen werde und Drogenh\xe4ndler weiterhin verfolgt w\xfcrden.
Valentino zeigt diese pers\xf6nlichen Erinnerungen als Troph\xe4en seines sozialen Aufstiegs vom bescheidenen Modemacher in der Stadt Voghera in Norditalien zum Idol des internationalen Jetsets.
"Wenigstens treten sie ihre Kippen nicht auf deinem herrlichen Teppich aus, wie es einige sch\xf6ne Ber\xfchmtheiten aus der Popmusik tun", sagt Baronin Fiona Thyssen-Bornemisza.
"Alle Eingeladenen f\xfchlten sich wichtig und geliebt", erinnert sich das "Top-Modell", das ihre Laufbahn bei der Woche der Haute Couture 1995 in Paris begann.
"Valentino h\xe4ngt nicht von der Mode ab, seine Besessenheit ist zeitlos", erl\xe4utert diese italienische Aristokratin, die zwischen Par\xeds, New York und Buenos Aires lebt.
Das gro\xdfe Finale der Ausstellung in Somerset House ist das Hochzeitskleid von Marie-Chantal Miller f\xfcr ihre Hochzeit mit Pablo de Grecia im Jahre 1995.
Die Singapurer schieben die Schuld daf\xfcr, dass sie keine Kinder haben, auf die Karriere, den Stress und die Kosten der Immobilien und die Kindererziehung.
Ihr kreativer Leiter Douglas Hamilton sagt, dass er die Macht der Musik dazu verwenden wollte, die Leute dazu zu bringen, ihre "nationale Pflicht" erf\xfcllen.
Beim Fortpflanzen sind wir die Schlechtesten der Welt, deshalb merkten wir, dass es sich um ein Thema handelt, um das wir uns k\xfcmmern mussten.
Wir wussten, dass die Regierung vieles versucht hatte, wie z. B. die Vermarktung von Parf\xfcm mit Pheromonen oder die Organisation von Speed-Dating-Abenden (schnellen Flirts).
W\xe4hrenddessen f\xfchrte eine Einwanderungspolitik, die auf einen drastischen Anstieg der Zuwanderungen abzielt, um der Verringerung der Bev\xf6lkerung entgegenzuwirken, zu Ressentiments bei der \xf6rtlichen Bev\xf6lkerung.
Bei Fragen zum Text gaben sie an, dass der Inhalt vom Pr\xe4sidenten von Peru, Ollanta Humala, bei kurzen Erkl\xe4rungen an die Presse dargelegt wurde.
"Wir werden das Urteil \xfcber die Differenzen, die wir gegenw\xe4rtig diesem internationalen Gerichtshof vorbringen, befolgen und ausf\xfchren", sagte Humala zusammen mit seinem chilenischen Gegen\xfcber.
"Wir werden alle diese Wege \xfcberpr\xfcfen - sie sind nicht ausschlie\xdfend, und auch das Abkommen mit Nicaragua machen Gespr\xe4che mit Nicaragua notwendig", unterstrich er.
Zwischen den Gesundheitsprogrammen und dem einfachen B\xfcrger bestehen gro\xdfe L\xf6cher, erkl\xe4rt Ricardo Salazar, Journalist aus Guadalajara, der sich der Sache des HIV angenommen hat.
Es wird gesch\xe4tzt, dass 50.000 Personen mit HIV leben, weil es f\xfcr jeden registrierten Fall 4 oder 5 Personen gibt, die es nicht wissen.
Im Streben danach, langfristige Verbindlichkeiten ohne Beeintr\xe4chtigung der kurzfristigen Verbindlichkeiten zu zahlen, bringt das Bauunternehmen Homex B\xf6rsenzertifikate \xfcber 500 Millionen Pesos auf den Markt.
Ich h\xf6re gern Musik, sehe Videos von Musik meiner Zeit in YouTube, genie\xdfe meine Enkelkinder und ab und zu gehe ich zu einem Basketballspiel.
Larry Hagman, dessen Rolle als der \xd6lmagnat J.R. Ewing in der Fernsehserie "Dallas" zu einem Symbol der Habgier der 80er Jahre wurde, ist tot.
Das Paar hatte zwei Kinder, Preston und Heidi, und sie lebten lange Zeit in der kalifornischen Stadt Malibu, wo viele Ber\xfchmtheiten ihren Wohnsitz haben.
Wenn jemand analysiert, was heute in der Welt vorgefallen ist, als ob wir drei\xdfig Tage davon entfernt w\xe4ren, w\xe4re dies eine wirklich gute Periode.
"In zwei Stunden gab es keine Pl\xe4tze mehr" sagte Restall \xfcber seinen Kurs f\xfcr Studenten mit hohem Durchschnitt, der sich mit 35 Studenten f\xfcllte.
Denn durch die seit 2009 verabschiedeten Ma\xdfnahmen hat sich der Anteil der Registrierung von Neuw\xe4hlern 2010 im Vergleich zu 2006 um 17% verringert.
In diesem Stadium werden sie von den \xc4rzten und Krankenschwestern, die sich um sie k\xfcmmern, nicht mehr mit so genannter "heilenden" Pflege \xfcberh\xe4uft.
"Ich habe keine W\xfcnsche mehr im Leben", sagt sie, bevor sie akzeptiert, dass man ihr eine Maske aufsetzt, die ihr beim Atmen hilft.
Nach Elsie Monereau, Leiterin der Palliativpflege der Gesellschaft der h\xe4uslichen Palliativpflege des Gro\xdfraums Montreal sprechen 8% der Patienten nicht auf eine Schmerzbehandlung an.
Au\xdferdem die Polizisten der "Marteau-Truppe", die seit 2009 bewirkt hat, dass das "Kanalisationskartell" von Montreal bei der k\xfcnstlichen Aufbl\xe4hung der Vertr\xe4ge zur\xfcckhaltender vorgeht...
Der n\xe4chste auf der Liste w\xe4re Gilles Vaillancourt, der gerade von seinem Amt als B\xfcrgermeister von Laval, der drittgr\xf6\xdften Stadt Quebecs, zur\xfcckgetreten ist.
Seit meinen Anf\xe4ngen im Zentrum der vorbereitenden Ausbildung des INF Clairefontaine bis zu meiner Spielzeit bei Saint-Etienne habe ich immer schrittweise Fortschritte gemacht.
W\xe4re es ein gro\xdfer Misserfolg, nicht den Titel in der Ligue 1 zu gewinnen, wie dies in der letzten Saison der Fall war?
Sie beschreibt Bitcoin als "die virtuelle W\xe4hrung mit dem gr\xf6\xdften Erfolg", "im Wettbewerb mit dem Dollar oder Euro" und "\xe4hnlich den herk\xf6mmlichen W\xe4hrungen".
Viele junge Leute wollen das Land verlassen, so wie diejenigen, die sich die amerikanischen Zuwendungen zu Nutze machen konnten: die Kapitalflucht ist betr\xe4chtlich.
Alle, auch die bewaffneten Parteien, sind besessen von Mobiltelefonen; das Fernsehen mit seinen t\xfcrkischen Serien, die eine moderne Welt darstellen, wird \xfcberall angeschaut.
Ein sehr kurzer Zeitraum, der die Br\xfcder dazu zwingt, auf ihr Vorhaben zu verzichten, den \xc4gyptern den Text Abschnitt f\xfcr Abschnitt zu erkl\xe4ren.
F\xfcr den Pr\xe4sidenten ist es auch eine Art und Weise, seine \xf6ffentliche und demokratische Legitimit\xe4t wiederzufinden, w\xe4hrend der Protest im ganzen Land tobt.
Nach Bekr\xe4ftigungen in einem Interview mit der amerikanischen Wochenschau Time scheint Mohammed Mursi \xfcberzeugt davon zu sein, dass die \xc4gypter wohlwollend stimmen werden.
Eine Fahrt innerhalb der Stadt kostet unabh\xe4ngig vom Verkehrsmittel 6 Schekel, das reicht inklusive Umsteigen f\xfcr eine Fahrt von bis zu 1,5 Stunden.
Die Mitarbeiter der russischen Polizei wissen, dass unsere Dokumente gr\xf6\xdftenteils gef\xe4lscht und wir nicht registriert sind, und daraus entstehen dann F\xe4lle von Erpressung.
Damit reagieren die Beh\xf6rden auf die j\xfcngsten Ereignisse: Verletzte bei Schie\xdfereien auf Hochzeiten sowie sieben Tote beim Amoklauf des Moskauer Juristen Dmitri Winogradow.
"Es gibt Beweise, dass es sich bei einigen F\xe4llen um Brandstiftung handelte, um das Fehlen von Waffen zu vertuschen", sagt der ehemalige Milit\xe4rangeh\xf6rige.
Ich als potenzieller Kunde kaufe nicht einfach nur, sondern fahre mit dem Verk\xe4ufer in den Wald, und dort stellen wir eine Zielscheibe auf.
Viktor Baranez betont, dass man zum Schluss auch leer ausgehen und hinter Gittern kommen kann, wenn man eine Anfrage auf einer Webseite platziert.
McDonald's sagt, das Unternehmen verkaufe Milliarden Portionen, und trotzdem gew\xe4hrt man euch keine Krankentage, und ihr werdet f\xfcr eure ehrliche Arbeit nicht bezahlt!
Das bei Anh\xe4ngern moderner Technologien beliebte Thema der erweiterten Realit\xe4t wird in letzter Zeit f\xfcr gew\xf6hnlich durch die Linse einer speziellen Brille wahrgenommen.
Bisher ist die Menschheit gr\xf6\xdftenteils in der Phase stecken geblieben, in der mit Pixeln auf Flachbildschirmen gearbeitet wird, die manchmal auch ber\xfchrt werden.
- Hei\xdft das, Sie wollen, dass der Benutzer sich an das anpasst, was eine Maschine zum jeweiligen Zeitpunkt leisten kann und was nicht?
- Kinect arbeitet gegenw\xe4rtig mit drei "Kameras", wobei eine davon eigentlich ein Infrarotsender und die zweite ein Empf\xe4nger f\xfcr das reflektierte Signal ist.
- In meinen Vorlesungen spreche ich oft davon, dass die erweiterte Realit\xe4t den siebten Durchbruch bei der Interaktion zwischen Mensch und Maschine darstellt.
Schnur und seine Freunde sangen einfache Lieder zum Play-back, trugen enge Trikots und zu ihnen geh\xf6rte auch der heute angesagte Komponist Igor Wdowin.
"Das war gerade mit den Biosatelliten, aber erneut war es nur ein einzelnes Experiment, und die Forschungen m\xfcssen fortgesetzt werden", bemerkt Wladimir Sychew.
Im Zustand der Schwerelosigkeit bildet sich die Bauch- und Beckenmuskulatur enorm schnell zur\xfcck und damit nimmt auch die F\xe4higkeit ab, das Kind herauszupressen.
Unl\xe4ngst sagte der Premierminister, dass die ODS die Unternehmer nicht mit Kontrollen bel\xe4stigen w\xfcrde - ist das System also nun verboten oder erlaubt?
Das Gesetz wird niemals vollkommen sein, aber es muss richtig angewendet werden - und das ist das, was bei uns meines Erachtens fehlt.
Die Stra\xdfen im Bezirk Pilsen sind heute gut befahrbar, \xf6rtlich ist jedoch erh\xf6hte Aufmerksamkeit geboten, und die Fahrweise ist an das Wetter anzupassen.
Neben mehreren Stellen mit Schnee oder Eisgl\xe4tte ist die Bergstra\xdfe von Telnice nach Kn\xednice im Kreis  \u2047 st\xed n.K. laut Angaben der Verkehrspolizei gesperrt.
Die Sperrung der Stra\xdfe zwischen Telnice und Kn\xednice war aufgrund von \xc4sten erforderlich, die von der Schneelast bis auf die Fahrbahn gedr\xfcckt wurden.
F\xfcnf unserer Mitglieder sind Rollstuhlfahrer, d.h. die Rollst\xfchle m\xfcssen im Gep\xe4ckraum bef\xf6rdert werden. Au\xdferdem m\xfcssen wir nat\xfcrlich viele Instrumentenkoffer und anderes Gep\xe4ck mitschleppen...
Zu der Zeit gab es bereits die ersten Projekte zur Satellitentechnik, und es war abzusehen, dass die Erforschung des Weltraums Zukunft haben w\xfcrde.
Von dieser Rakete wurden drei Typen entwickelt (Meteor-1A, -1B und -1C), die sich voneinander in der Gr\xf6\xdfe des Transportraums f\xfcr wissenschaftliche Instrumente unterschieden.
Ursache daf\xfcr ist das Prinzip des freien Handels und der freien, uneingeschr\xe4nkten Bewegung des Privatkapitals, die mit z\xfcgellosen Finanzspekulationen Hand in Hand geht.
Lobby-Interessen standen auch dahinter, dass Bananen der h\xf6chsten Handelsklasse in der EU mindestens 14 cm lang sein m\xfcssen und keine "Kr\xfcmmungsanomalie" aufweisen d\xfcrfen.
Die EU legte damit das H\xf6chstvolumen an Lebensmittelvorr\xe4ten fest, das sich am Tag unseres EU-Beitritts auf dem Gebiet der Tschechischen Republik befinden durfte.
Er ist Teil eines Revitalisierungsprojekts, zu dem auch Tiefgarage, Supermarkt, Post und ein paar angrenzende Wohn- und Reihenh\xe4user mit insgesamt 50 Wohnungen geh\xf6ren.
Es gibt zwar einen Lift, der mitten durchs Bergmassiv f\xfchrt, doch die wahren Raum- und Lesefreuden erschlie\xdfen sich beim fu\xdfl\xe4ufigen Erklimmen der Topografie.
Wie Pluto, der hinter Neptun um die Sonne kreist, ist Ceres nach der neuen Begriffsdefinition der Internationalen Astronomischen Union von 2006 kein "Planet".
Das Innenleben des Gran Telescopio Canarias auf der Kanareninsel La Palma ist riesig - alleine der Spiegel kommt auf 10,4 Meter im Durchmesser.
Oder ist es die urspr\xfcngliche Lebensweise, die die Menschen jung h\xe4lt? In Cengemiran, einer winzigen Siedlung unweit der Stadt Lerik, wohnt Rubaba Mirzayeva.
Doch der Kult, der um die Vaterfigur der Nation getrieben wird, der sein Land wie ein Diktator regierte, kennt kaum Grenzen in Aserbaidschan.
Er habe, so sagte Mohammed Mursi fast entschuldigend, die Kompetenzen des Verfassungsgerichts vor\xfcbergehend beschnitten und seine Kompetenzen erweitert, "um die Revolution zu retten".
Das muss nicht, aber es kann bedeuten, dass die Geistlichkeit die Gesetzgebung beaufsichtigt, was de facto die Entm\xfcndigung der Judikative zur Folge h\xe4tte.
Der Staat solle auch, so steht es im Entwurf, "das wahre Wesen der \xe4gyptischen Familie" sch\xfctzen "und ihre Moral und ihre Werte f\xf6rdern".
Das Ziel war es jedoch nicht, Pendler auf dem Weg zur Arbeit zu st\xf6ren, sondern Demonstranten daran zu hindern, das Parlament zu erreichen.
Auf einem Flecken Brachland in der N\xe4he einer gro\xdfen M\xfclldeponie wurden allein in den letzten zwei Jahren die Leichen dutzender ermordeter Frauen zur\xfcckgelassen.
Dem Geheimdienstanalyst der US-Armee, der im Juni 2010 verhaftet wurde, wird vorgeworfen, w\xe4hrend seiner Dienstzeit im Irak tausende vertrauliche Dokumente gestohlen zu haben.
Manning sagte, er habe versucht, in Bewegung zu bleiben, denn am Tag sei es verboten gewesen, zu schlafen oder sich auch nur hinzulegen.
Wenn er sich nachts umgedreht habe und Wachen sein Gesicht nicht mehr sehen konnten, habe man ihn aufgeweckt, damit er sich wieder zur\xfcckdreht.
So, wie Islamisten in der arabischen Welt an Einfluss gewonnen haben, hat die Hamas m\xe4chtige und reiche Freunde auf ihre Seite ziehen k\xf6nnen.
Bei zuk\xfcnftigen diplomatischen Verhandlungen k\xf6nnte sich die Hamas als Akteur erweisen, der selbst von Israel und den Vereinigten Staaten nicht herausgedr\xe4ngt werden kann.
Nein, es ist besser, sie hinter der Mauer in Schach zu halten und zu bestrafen, sollten sie es wagen, die K\xf6pfe zu heben.
Die Unterdr\xfcckung untergr\xe4bt schon jetzt die Demokratie im j\xfcdischen Staat, und mit dem Wachstum der arabischen Bev\xf6lkerung wird sich diese Situation nur versch\xe4rfen.
Wie viele Menschen auch bin ich stets davon ausgegangen, dass Langeweile ein relativ aktuelles Ph\xe4nomen ist, das sich mit zunehmender Freizeit entwickelt hat.
"Unsere Beh\xf6rde hat die Pflicht, Verst\xf6\xdfe zu verfolgen, bei denen es sich zum Tatzeitpunkt um Straftaten handelte", lie\xdf Buck in einer Erkl\xe4rung verlauten.
Und die widerspr\xfcchlichen Reaktionen im ganzen Staat f\xf6rderten unter \xf6rtlichen Beamten einen tiefgreifenden Zwiespalt im Hinblick auf das gro\xdfe gr\xfcne Experiment zu Tage.
Als erste Staaten, die kleinere Mengen Marihuana wie Alkohol behandeln, werden Colorado und Washington als nationale Musterf\xe4lle f\xfcr die Legalisierung von Drogen gehandelt.
Der 20-j\xe4hrige Luke Black, Vizepr\xe4sident der konservativen Studentenvereinigung der Universit\xe4t Nottingham, lie\xdf in einer Sonntagszeitung verlauten: "Es gibt eine wachsende Linkstendenz an Universit\xe4ten.
Im Vorjahr hatte die Universit\xe4t daf\xfcr gestimmt, Margaret Thatcher - einer fr\xfcheren Studentin - aufgrund von K\xfcrzungen im Hochschulwesen keinen Ehrentitel zu verleihen.
In den ersten Tagen der Erstsemester-Woche, bei der neue Studenten sich und die Tutoren kennenlernen, erhielt ich einen Vorgeschmack auf die zuk\xfcnftigen Geschehnisse.
F\xfcr mich ist es schon schlimm genug, aber sie wissen, dass dein Vater Margaret Thatcher nahesteht, deshalb wird es f\xfcr dich schlimmer sein.
Auch die Prinzessin und Meinungsf\xfchrende bei der Mode Patricia della Giovampaola d'Arenberg kann das erste Mal nicht vergessen, als sie einen Valentino trug.
Als ich als Teenager in Italien lebte, tr\xe4umte ich davon, endlich das Alter und die Gelegenheit zu haben, eines seiner Abendkleider zu tragen...
Daher dachten wir: Warum machen wir nicht etwas so kreativ wie m\xf6glich, um dieses Problem anzugehen, wie z. B. einen Rap zu komponieren?
Singapur ist ein reicher, hochtechnologischer Stadtstaat im S\xfcdosten Asiens, der auch f\xfcr den Konservatismus seiner Regierenden und seine strikten sozialen Kontrollen bekannt ist.
Tan Wei Ming, Direktorin f\xfcr Ehe- und Familienpolitik der nationalen Bev\xf6lkerungsbeh\xf6rde, sagt, dass dies auf eine "bessere Ausbildung" und "gr\xf6\xdfere Karrierechancen" zur\xfcckzuf\xfchren sei.
"Die Leute sind stark gestresst, die Wohnungen und auch die Erziehung sind teuer, weshalb es von vielen hinausgeschoben wird" sagt ein junger Manager.
Deshalb haben die Singapurer das letzte Wort, wenn es darum geht, Kinder zu bekommen - da kann die Regierung noch so viel tun.
Versteht er die Gefahren, denen er sich aussetzt, wenn er im Internet Situationen bekannt macht, die er im realen Leben nicht teilen w\xfcrde?
"Das Internet entstand als Medium f\xfcr die Suche nach Informationen; mit dem Erscheinen dieser Seiten haben sich die Spielregeln aber ge\xe4ndert", sagt sie.
Beim Gipfeltreffen anwesend waren die Pr\xe4sidenten von Brasilien, Dilma Rouseff, von Venezuela, Hugo Ch\xe1vez, von Bolivien, Evo Morales, und von Argentinien, Cristina Kirchner.
"Wir hoffen, dass der Wahlvorgang in diesem Land f\xfcr seine Wiederaufnahme in der Union s\xfcdamerikanischer Nationen dient", von der es gegenw\xe4rtig ausgeschlossen ist.
"Ich hoffe dem Pr\xe4sidenten Ortega sagen zu k\xf6nnen, dass wir diese Angelegenheit so zivilisiert und respektvoll wie m\xf6glich behandeln werden", f\xfcgte Santos hinzu.
"Die gr\xf6\xdften Feinde der Pressefreiheit sind nicht die b\xf6sen und perversen Politiker, sondern schlechte Journalisten, die nach Gewinn streben und erpressen", sagte er.
"Meine politische Bewegung hatte den Glauben, dass ich es war, der diesen wahrscheinlichen Sieg garantierte, deshalb muss ich dieser Verantwortung nachkommen", sagte er.
Er ist zweifelsohne einer der \xe4ltesten Patienten der HIV-Einheit des Hospital Civil de Guadalajara (HCG), in das er nach mehreren K\xe4mpfen 1994 kam.
Allerdings \xf6ffnet der Beschluss dem gr\xf6\xdften Glashersteller in Mexiko T\xfcr und Tor, um wegen dreier Inkonsistenzen den obersten Gerichtshof der Vereinigten Staaten anzurufen.
"Larry war zur\xfcck in seiner geliebten Geburtsstadt Dallas, wo er nochmals die ikonische Rolle spielte, die ihm am meisten gefiel", sagte die Familie.
Die dramatische Serie der Fernsehkette CBS \xfcber den Ewing-Clan und sonstige Figuren in deren Umgebung wurde von April 1978 bis Mai 1991 ausgestrahlt.
Au\xdferdem haben die republikanischen Gesetzgeber in f\xfcnf weiteren Bundesstaaten Gesetze verabschiedet, die darauf abzielen, den Zeitraum f\xfcr die vorzeitige Stimmabgabe zu verk\xfcrzen.
Es gibt in dieser Welt ein zwangsl\xe4ufig unumg\xe4ngliches Gesetz, das bewirkt, dass zwei Objekte nicht gleichzeitig am selben Ort vorhanden sein k\xf6nnen.
Es ist nicht m\xf6glich, gegen diese Regel zu versto\xdfen - und versuchen Sie es nicht zu stark, da Sie sich wehtun werden.
Gleiches gilt f\xfcr das Higgs-Boson, mit dem Unterschied, dass ein anderes Feld, das Higgs-Feld, "gest\xf6rt" werden muss, damit sich dieses Boson zeigt.
Die Krankheit macht ihre Arbeit: eine unermessliche Schw\xe4che hindert ihn daran, allein auf die Toilette zu gehen und sogar selbst zu essen.
Andere Beamte des Stra\xdfenbauamtes haben zugegeben, dass sie sich schmieren lie\xdfen, indem sie die Rechnungen mit falschen Zusatzleistungen k\xfcnstlich um 30-40% aufbl\xe4hten.
In Anbetracht dessen, was investiert worden ist und die Spieler, die wir haben, ist es normal, dass viel von uns erwartet wird.
Die im Umlauf befindlichen Bitcoins sind somit auf 21 Millionen begrenzt, aber bis auf ein Hundertmillionstel teilbar, was einen gewissen Spielraum l\xe4sst...
F\xfcr seine Gegner verharrt der Pr\xe4sident in seinem "autokratischen Delirium", indem er weiterhin "sein Wort bricht" und "das Recht mit F\xfc\xdfen tritt".
Neben seinem religi\xf6sen Aspekt wird der gestern verabschiedete Text stark aufgrund der weitreichenden Befugnisse kritisiert, die er dem Pr\xe4sidenten der Republik gew\xe4hrt.
W\xe4hrend Abgeordnete und B\xfcrgerrechtler dar\xfcber diskutieren, welchen Nutzen das Gesetz \xfcber verbindliche Sprachtests f\xfcr Migranten bringt, handeln Kriminelle bereits mit gef\xe4lschten Zertifikaten
Am 1. Dezember trat ein Gesetz in Kraft, dem zufolge jeder Arbeitsmigrant einen Test, der Kenntnisse der russischen Sprache bescheinigt, ablegen muss.
Ebenfalls von diesem Gesetz ausgenommen sind Personen, die ihre Ausbildungszeugnisse und Diplome vor dem Zerfall der UdSSR im Jahr 1991 erhalten haben.
"Viele reden jetzt \xfcber den Schutz der Rechte von Arbeitsmigranten", sagt der Leiter der Vertretung der F\xf6deralen Migrationsbeh\xf6rde in Tadschikistan, Viktor Sebelew.
Baranez erl\xe4utert, dass hierzu Waffen z\xe4hlen, die sowohl aus den Waffenkammern der Polizei als auch direkt von Mitarbeitern der Strafverfolgungsbeh\xf6rden gestohlen wurden.
"Der H\xe4ndler bringt die Waffe in die Stadt und verkauft sie dort f\xfcr 900 Euro pro St\xfcck mit zwei Magazinen", erz\xe4hlt er
Der ehemalige Milit\xe4rangeh\xf6rige Viktor Baranez versuchte sich Mitte der 1990er als K\xe4ufer illegaler Waffen, als er einen Artikel zu diesem Thema schrieb.
Laut Dmitrij Kislow von der Organisation "Pravo na oryzhie" kann man eine Pistole vom Typ Makarow f\xfcr 100 bis 300 Dollar kaufen.
Bef\xfcrworter von Walmart stellen zufrieden fest, dass es nur in neun Bundesstaaten zu Protesten kam und diese dem Unternehmen keinerlei Verluste bescherten.
- Obwohl Kinect die Interaktion auf eine physische Ebene gebracht hat, spielt sich vieles noch auf dem Flachbildschirm ab, manchmal in 3D.
Denken Sie nicht, dass im Hinblick auf die Anwendung der Technologie der erweiterten Realit\xe4t im Alltag die Brille die besten Aussichten hat?
Um die Menschheit zu retten, stellt sich die wichtige Frage, wie wir uns in der Schwerelosigkeit oder auf dem Ersatzplaneten fortpflanzen k\xf6nnen?
In Anbetracht dessen, dass diese Novelle erst kurze Zeit in Kraft ist, wirkt sie sich bei unseren Pr\xfcfungen bislang noch nicht aus.
Der Premierminister sagte unl\xe4ngst, dass die ODS die Unternehmer nicht mit Kontrollen des sog. "Schwarz-Systems" behelligen w\xfcrde - was hei\xdft das genau?
Auf der anderen Seite ist es aber auch tragisch, wenn der Bieter mit dem besten Angebot allein aufgrund von Formfehlern ausgeschlossen wird.
Der Text der Hymne stammt von Tom\xe1 \u2047  Han\xe1k, der auch die Hauptfigur des Jesus im Videoclip spielt, auch Xindl X singt mit...
Gegen\xfcber Prag ist Moskau absolut nicht behindertengerecht. Dort ist es immer noch ungew\xf6hnlich, wenn jemand im Rollstuhl allein im Stadtzentrum unterwegs ist.
Die erste Erw\xe4hnung dieser Gesellschaft erfolgt 1954 in der Novemberausgabe der Zeitschrift Problemy, in der vier umfangreiche Artikel der Raumfahrt gewidmet sind.
Da das Privatkapital keine gesellschaftliche Verantwortung und damit auch keine Verantwortung f\xfcr die von ihm verursachte Arbeitslosigkeit tr\xe4gt, steigen notwendigerweise die Staatsausgaben.
Das Privatkapital ist schon von seiner Natur her nicht in der Lage, den Vorteil f\xfcr die gesamte Gesellschaft zu erkennen und durchzusetzen.
"Wenn meine S\xf6hne keinen Kriege wollten, g\xe4be es keine", sagt die sterbende Gutele Schnaper, Ehefrau von Mayer Amschel Rothschild, im Jahr 1849
Aus einem bel\xe4chelten Schauspieler ist eine respektabler Regisseur geworden, und auch als Schauspieler ist er nun nicht mehr das Ziel ironischer Anmerkungen.
Das Gesp\xfcr f\xfcr die Atmosph\xe4re des Ortes geh\xf6rte dabei zu den Merkmalen, die die vorherigen Filme dieses Regisseurs vom Standard Hollywoods abhoben.
Die Europ\xe4ische Kommission verteidigte sich dabei mit dem Argument, dass sie lediglich die uneinheitlichen einzelstaatlichen Normen harmonisiere, die den Handel behindern w\xfcrden.
Als Argument f\xfchrte er an, dass die Getreideernte sehr hoch gewesen sei und die staatlichen Lager infolge der sog. Interventionseink\xe4ufe \xfcberf\xfcllt waren.
Sp\xe4ter habe ich dies pr\xe4zisiert und gesagt, dass ich f\xfcr das Amt des Pr\xe4sidenten kandidieren werde, sofern ich zum Senator gew\xe4hlt werde.
Dazu kommen die Medien, die einem die Ehre rauben wollen, und die die Freiheit des Wortes mit der Freiheit zu l\xfcgen verwechseln.
Sechzig Prozent der Wahlberechtigten sind \xfcberhaupt nicht zu den Wahlen gegangen, und die, die gegangen sind, haben meist Vertreter des Establishments gew\xe4hlt.
Der rundum verglaste Innenraum ist hell und \xfcbersichtlich, der gebrannte Klinkerboden und die eleganten Stra\xdfenlaternen sprechen unmissverst\xe4ndlich die Sprache eines \xf6ffentlichen Stadtplatzes.
W\xe4hrend des Aufstandes in Libyen im M\xe4rz 2011 hat Deutschland sich ebenfalls der Stimme enthalten, als es darum ging, eine Flugverbotszone einzurichten.
Wenn Sie sich die Beziehungen zwischen Obama und Premierminister Netanjahu ansehen, dann ist Obama gar nicht so hellauf begeistert von Netanjahus Politik.
Wenn wir uns zum Beispiel die Eurokrise anschauen, da werden jedes Mal, wenn Deutschland eine gr\xf6\xdfere Rolle annimmt, verschiedenste anti-deutsche Gef\xfchle frei.
Pattloch berichtet von F\xe4llen, in denen das Gericht Klagen abwies, weil nach der langen Dauer der beanstandete Name zur "Marktrealit\xe4t" geworden sei.
Der Modehersteller Lacoste verlor in China gegen Nachahmer aus Hongkong und Singapur, die das ber\xfchmte Krokodil in die andere Richtung schauen lie\xdfen.
Das Robert-Koch-Institut geht davon aus, dass mindestens vier von f\xfcnf aller in Deutschland gemeldeten Syphilis-F\xe4lle durch sexuelle Kontakte zwischen M\xe4nnern \xfcbertragen werden.
Die Verbreitung von HIV ist unter heterosexuellen Erwachsenen hierzulande vergleichsweise gering - dennoch: Rund 20 Prozent der HIV-Neuinfektionen entfallen auf diese Gruppe.
Unter anderem ist es auch dieser staatlich sanktionierten Lebensform geschuldet, dass sich der HI-Virus in den vergangenen Jahrzehnten so schnell ausgebreitet hat.
Die Funde k\xf6nnten aber dabei helfen zu kl\xe4ren, wie Wasser und andere Bausteine des Lebens in andere Gegenden des Sonnensystems gelangt sind.
Das Teleskop soll 1608 von Hans Lipperhey erfunden worden sein - noch bevor Galileo Galilei es ein Jahr sp\xe4ter zur Sternenbeobachtung einsetzte.
Hier ist die Vita von etwa acht Dutzend Talyschen aus der Gegend dokumentiert, die \xe4lter als 100. Fatulayeva zeigt auf ein Schwarz-Wei\xdf-Foto.
Seine Rede war an das ganze Volk gerichtet, vor allem aber wohl an die christlichen Kopten, die Liberalen, aufgekl\xe4rten Muslime und S\xe4kularen.
Das ist juristisch so unscharf formuliert, dass staatliche Institutionen mit Hilfe dieses Artikels sogar die Inhalte von Filmkunst und Literatur kontrollieren k\xf6nnte.
Hafez Abu Saeda ist w\xfctend \xfcber diesen forcierten Verfassungsprozess, der eigentlich bis zum Februar h\xe4tte gehen und alle gesellschaftlichen Kr\xe4fte einbinden sollen.
Die f\xfcnf Millionen Einwohner Norwegens genie\xdfen einen der h\xf6chsten Lebensstandards - und das nicht nur in Europa, sondern auf der ganzen Welt.
Heute w\xe4chst die Bev\xf6lkerung rapide - mehr als 13% sind Einwanderer, angelockt von einem florierenden Arbeitsmarkt, hohen L\xf6hnen und einem umfassenden Gesundheitswesen.
Hauptverantwortlich f\xfcr den heutigen Reichtum Norwegens ist seit den fr\xfchen 1970er Jahren das Wachstum einer der gr\xf6\xdften \xd6l- und Gasindustrien der Welt.
Auf der Agenda standen all jene Themen, die man erwartet, wenn sich die K\xf6pfe dieser beiden L\xe4nder treffen: Einwanderung, Drogen und Handel.
Wenn sie tats\xe4chlich die Kontrolle \xfcber das Westjordanland h\xe4tten, w\xfcrden sie dann nicht genau wie ihre Mitstreiter im Gazastreifen auch Raketen abfeuern?
Die - f\xfcr die nahe Zukunft kleine - Hoffnung besteht darin, dass der Waffenstillstand Au\xdfenstehenden mehr Einfluss zur Durchsetzung dieser L\xf6sung gew\xe4hrt.
"Es klingt so, als m\xfcsste uns \xf6fter langweilig sein. Aber Langeweile ist der qu\xe4lende, unabl\xe4ssige Wunsch, etwas Sinnvolles zu tun", sagt er.
Im Evening Standard hie\xdf es, ich w\xe4re gegangen, weil ich ein Problem damit gehabt h\xe4tte, dass Kommilitonen im benachbarten Zimmer Sex hatten.
Der Autor A N Wilson erkl\xe4rte schelmisch, ich h\xe4tte die Universit\xe4t verlassen, weil ich dazu gezwungen war, aus besch\xe4digten Tassen zu trinken.
Ich begann, zwischen Oxford und dem Haus meiner Eltern zu pendeln und fand Zuflucht bei aufgeschlosseneren Freunden und Familienmitgliedern in der Stadt.
Obwohl ich insgeheim vor Scham zerging, gab ich zu, dass mich meine Eltern einer "Gehirnw\xe4sche" unterzogen hatten, und nannte sie "alte Trottel".
Ein Paket der Regierung f\xfcr Ehepaare und Eltern gew\xe4hrt bis zu 15.000 Dollar pro Kind, verl\xe4ngert den Mutterschaftsurlaub und verteilt steuerliche Vorteile.
Aber Lim Yew Soon, Generaldirektor der Immobilienfirma EL Developers, sagt, dass sich seine "Schuhschachteln" sehr viel schneller als gr\xf6\xdfere Wohneinheiten verkaufen lassen.
Porras nennt anschlie\xdfend einige M\xf6glichkeiten: Es gibt Dinge, die du einem Fremden nicht erz\xe4hlen w\xfcrdest. Warum machst du es dann im Internet?
Paraguay, das seit 2011 nach der Absetzung seines Pr\xe4sidenten Fernando Lugo von der Unasur ausgeschlossen ist, nahm an dem Treffen nicht teil.
Er f\xfcgte hinzu, dass es seinerzeit "begr\xfcndete Vermutungen gegeben habe, dass Assange an einen Drittstaat ausgeliefert und sein Verfahren nicht eingehalten w\xfcrde."
Diesen Monat analysierten die Studenten Filme mit apokalyptischem Inhalt und untersuchten, wie sie sich im Vergleich mit dem wirklichen Leben vergleichen lie\xdfen.
Aber keiner der befragten Studenten - und weniger noch ein Professor - erkl\xe4rte, an das letzte Datum des 21. Dezembers zu glauben.
Im Laufe der letzten beiden Jahre f\xf6rderten sie in 34 Bundesstaaten Gesetzesentw\xfcrfe, mit denen die W\xe4hler gezwungen werden, einen Lichtbildausweis vorzuzeigen.
In der Tat besitzen 11% der US-B\xfcrger, d. h. 21 Millionen wahlberechtigte Personen keinen von einer Regierungsbeh\xf6rde ihres Staates ausgestellten Lichtbildausweis.
Dar\xfcber hinaus haben republikanische Gesetzgeber 2011 in acht Bundesstaaten Gesetze gef\xf6rdert, mit denen die Registrierung von W\xe4hlern am Wahltag abgeschafft wurde.
Nat\xfcrlich haben sich die demokratischen Gesetzgeber und ihre Anh\xe4nger energisch der Verabschiedung von Gesetzen entgegengestellt, die die Registrierung der W\xe4hler einschr\xe4nken.
Dieses Dokument (derzeit nur auf Englisch, aber eine \xdcbersetzung wird in K\xfcrze verf\xfcgbar sein) kann unter folgender Adresse heruntergeladen werden: http://ca.movember.com/fr/mens-health/prostate-cancer-screening
Ermutigende Daten: 10 Jahre nach dem Verzicht auf die Zigarette, verringert sich das Risiko an Krebs zu sterben um die H\xe4lfte.
Dar\xfcber hinaus betont Herr Beaulieu, wie wichtig es ist, mit seinem Arzt \xfcber seine Bedenken und seine famili\xe4re Vorbelastung zu sprechen.
Die 2011 ins Leben gerufene, permanente Antikorruptionseinheit unternimmt mit ihren Truppen an Wirtschaftspr\xfcfern, Ermitteln und Analysten der Regierung ebenfalls gro\xdfe Anstrengungen.
Es handelt sich um ein Zerst\xfcckeln der Datei, d.h. die Umwandlung einer gro\xdfen Datei in einen k\xfcrzeren und eindeutigen elektronischen Fingerabdruck.
Dort wird die Sammlung von Werken der Impressionisten und Expressionisten Monet, Pissaro, Renoir, C\xe9zanne, Sisley, Matisse, Modigliani, Chagall und Picasso ausgestellt.
\xdcbrigens ist dieses ungew\xf6hnliche Meer mit einer Lage von 417 Metern unter dem Meeresspiegel das am tiefsten gelegene Meer der Welt.
Die Migranten k\xf6nnen die Tests in allen St\xe4dten ablegen; schon jetzt wurden in Russland bereits mehr als 160 entsprechende Zentren er\xf6ffnet.
Das Prozent der Verbrechen mit registrierten Waffen ist sehr gering, \xe4u\xdferte der Strafrechtler , Wasilij Lesnikow, dem russischen Dienst der BBC.
Es gibt f\xfcnf solche Hauptkan\xe4le, erz\xe4hlt ein ehemalige Oberst Viktor Baranez, der zehn Jahre im Bildungsministerium und im Generalstab t\xe4tig war.
"Die Leute kommen wie hungrige Fische bei der F\xfctterung und landen dann im sibirischen Arbeitslager und d\xfcrfen Kohle schaufeln", sagt er.
Neben der Erh\xf6hung der bescheidenen L\xf6hne von einfachen Walmart- und Fast-Food-Besch\xe4ftigten verfolgen die Organisatoren der Proteste das Ziel, Gewerkschaften zu gr\xfcnden.
Dabei wurden die Gesten nicht von der Objektkamera, sondern von einem Armband aufgezeichnet, das die Bewegungen der Knochen und Muskeln registrierte.
Es gibt auch B\xe4nder f\xfcr das Handgelenk, die auf die Nervenendungen in den Fingern einwirken, auch das ist eine potenzielle Richtung.
- Kirill, warum bist du eigentlich immer in Rot und nicht zum Beispiel in Gelb oder T\xfcrkis in der Stadt unterwegs?
Viele wurden dort geboren: N.O.M., Tequilajazzz, und ich erinnere mich auch, wie Schnur mit seinem Projekt "Ucho Van Goga" dorthin kam.
Wir ben\xf6tigen einen kulturellen N\xe4hrboden, denn zum Beispiel haben wir mittlerweile mehr Schriftsteller als Leser, und das ist doch nicht richtig.
W\xe4hrend jedoch die Bedingungen auf dem Mars vergleichsweise lebensfreundlich sind, herrscht auf der Oberfl\xe4che der Venus eine Temperatur von 500 Grad.
Im Jahr 1979 wurden Wachteleier ins Weltall geschickt, um zu erforschen, wie sich die Schwerelosigkeit auf die Entwicklung von Embryos auswirkt.
Von den Hauptstrecken sowie von der Stra\xdfe I/13 an der Grenze der Bezirke  \u2047 st\xed n.L. und Liberec werden schlechte Verkehrsbedingungen gemeldet.
F\xfcr die Einrichtung des barrierefreien Bildungszentrums Studeo, an dem wir bereits sechs Jahre zusammen mit dem Verein Tap im Jedli \u2047 ka-Institut arbeiten.
Es stimmt, dass uns die Zusammenarbeit mit bekannten S\xe4ngern geholfen hat; au\xdferdem haben wir auch angefangen, aktiv f\xfcr uns zu werben.
Wenn man etwas gut machen m\xf6chte, darf man in vielen Dingen keine Kompromisse eingehen und muss auch eine gewisse Disziplin einfordern.
Polen begann im Jahr 1994 eine enge Zusammenarbeit mit der ESA und beteiligte sich in den folgenden Jahren an mehreren ESA-Projekten.
Weitere Artikel zur Raumfahrt erschienen nach dem Krieg dank der Arbeit der Polnischen Raumfahrtgesellschaft (Polskie Towarzystwo Astronautyczne) in der polnischen Presse.
Die liberal orientierten Wirtschaftssysteme in der EU und in der globalisierten Welt gr\xfcnden sich auf dem Prinzip des unregulierten wirtschaftlichen Wettbewerbs.
Eine Welt, in der jedem Neugeborenen bei der Geburt ein Chip implantiert wird, um dieses Wesen der totalen Kontrolle zu unterwerfen.
Der Film Argo des Regisseurs und Schauspielers Ben Affleck beschreibt eine Episode dieser Geschichte, die den USA einen kleinen Teilsieg bescherte.
Argo ist sein dritter Spielfilm nach dem Krimi Kein Kinderspiel (Gone Baby Gone, 2007) und dem Thriller Stadt ohne Gnade (2010).
Unter den nominierten Absurdit\xe4ten befindet sich beispielsweise das Urteil des Europ\xe4ischen Gerichtshofes \xfcber die Vereinheitlichung der Versicherungstarife f\xfcr M\xe4nner und Frauen.
Kritik erntete in der Vergangenheit auch das faktische Verbot der Verwendung des Begriffs "Butteraufstrich" oder auch das Verkaufsverbot f\xfcr herk\xf6mmliche Gl\xfchbirnen.
Ich habe mir die ganze Zeit gesagt, dass ich den Kampf um die Burg nach dem Ergebnis der Senatswahlen aufnehmen werde.
Meine Kandidatur begann ich mit der Voraussetzung, dass die Menschen tief unzufrieden sind, aber jetzt bin ich mir nicht mehr sicher.
Und so erkannten die Stadtv\xe4ter, dass es nur eine einzige M\xf6glichkeit g\xe4be, der Statistik Herr zu werden: Eine Bibliothek m\xfcsse her!
"Man w\xfcrde es ja nicht glauben, aber dieses Haus ist trotz der vielen Glasfl\xe4chen ein Vorzeigeprojekt in puncto \xd6kologie", sagt Trouborst.
Damit sollen vorerst einmal die optischen L\xfccken in der noch nicht vollst\xe4ndig best\xfcckten Bibliothek - derzeit 70.000 St\xfcck - gef\xfcllt werden.
Sie zeigt die Bereitschaft, bei nationalen Interessen auch Positionen zu beziehen, die unabh\xe4ngig sind von denen der USA oder europ\xe4ischen Partnern.
Deutschlands Wirtschaftsinteressen sind zu einem bestimmten Grad anders als die der anderen gro\xdfen M\xe4chte und deshalb muss Deutschland seine Interessen sch\xfctzen.
Deshalb muss es vorsichtig sein, die \xd6ffentlichkeit, aber auch die Eliten, in den arabischen L\xe4ndern nicht vor den Kopf zu sto\xdfen.
Szabo ist au\xdferdem ein Mitglied des German Marshall Fund, wo er sich auf deutsche Politik, US-Au\xdfenpolitik und transatlantische Beziehungen spezialisiert hat.
Wenn der Kl\xe4ger Pech habe, m\xfcsse er dem Plagiator sogar Geld zahlen, weil er dessen Marke in China verletzte, sagt Pattloch.
Das Markenamt CTMO in Peking gibt zwar zu, dass es dort 2010 wegen zu geringer Personal- und Raumausstattung Engp\xe4sse gegeben habe.
Die internen Kosten lie\xdfen sich kaum beziffern, das Firmenarchiv habe sogar einhundert Jahre alte Akten durchsehen m\xfcssen, um Beweise zu erbringen.
Dann erst schwellen die Stimmen der S\xe4nger langsam an - Alt, Bass, Tenor und Sopran - bedr\xe4ngen, bet\xf6ren und verfolgen sich.
Und Fiete Hopf, den 29-j\xe4hrigen Dirigenten, hebt es fast aus seinen Stoffschuhen, wenn er sie mit seinen geschmeidig wilden Gesten zusammenf\xfchrt.
Mehr als vierzig Prozent der Menschen in Swasiland tragen den Immunschw\xe4che-Virus in sich, mit Mitte drei\xdfig zu sterben ist keine Seltenheit.
Die Sonde Messenger habe Beweise daf\xfcr gefunden, dass es in der permanent im Schatten liegenden Region des Planeten eine Eisdecke gibt.
30 Jahre lang, n\xe4mlich von 1947 bis 1975, war das Hale-Teleskop im Palomar-Observatorium nahe San Diego das gr\xf6\xdfte Fernrohr der Welt.
Das kleine St\xe4dtchen protzt mit zu wuchtig geratener Architektur aus Sowjetzeiten, die so gar nicht in die malerische Berglandschaft passen will.
"Wir sind noch nicht m\xfcde, das Blut unserer Br\xfcder ist noch nicht ges\xfchnt", zitierten die \xe4gyptischen Medien den Oppositionspolitiker Chaled Ali.
"Und jetzt steht das Wort Menschenrechte nicht einmal in der neuen Verfassung", beklagt er im Gespr\xe4ch mit der "Welt am Sonntag".
Im tiefsten Winter wurde er dann nach langer Fermentierung herausgenommen und - zweifellos unter mithilfe von Alkohol ged\xe4mpften Sinnen - verzehrt.
Insbesondere, was die Sicherheit und Wirtschaft anbetrifft, hoffen wir auf eine interessante und wirkliche Ver\xe4nderung, die unser Land so dringend braucht.
In Nezahualcoyotl, auch bekannt als Ciudad Neza, k\xf6nnte der Kontrast zu den gepflasterten Stra\xdfen von Valle del Bravo nicht gr\xf6\xdfer sein.
Die Kritiker Pena Nietos sind der Auffassung, dass er das Problem der Frauenmorde w\xe4hrend seiner Amtszeit zumindest nicht angemessen angegangen ist.
"Sie schrieben (nach Besprechung der Bedenken) "Keine Probleme" auf, und das bedeutete nicht notwendigerweise, dass ich \xfcberhaupt nichts sagte", so Manning.
Ein ethnisches K\xfcrzel - genau so, wie sich meine Freunde in Boston "Iren" oder meine Freunde in New York "Italiener" nennen.
Israel ist es in letzten Jahren gut ergangen, insbesondere unter Premierminister Binyamin Netanyahu, der den Friedensprozess zu gro\xdfen Teilen ignoriert hat.
"In einer Umgebung, in der wir st\xe4ndig \xfcberstimuliert werden, f\xe4llt es schwer, sich zu besch\xe4ftigen, wenn der L\xe4rm einmal verstummt ist."
Aber Smith gibt auch zu, dass kein Ort oder System mehr tun kann, als im Sinne eines groben Leitfadens zu dienen.
Nach der Abstimmung gab er an, seine Beh\xf6rde w\xfcrde F\xe4lle von Marihuanabesitz weiterhin verfolgen, haupts\xe4chlich, um Konsumenten zum Entzug zu bewegen.
Noch vor dem Wahltag genehmigten einige \xf6rtliche Gemeindeverwaltungen Moratorien f\xfcr neue Marihuana-Gesch\xe4fte, obwohl diese erst in etwa einem Jahr \xf6ffnen k\xf6nnten.
Wir richten uns danach, f\xfcr was sich die Gemeinde entschieden hat und nicht danach, f\xfcr was sich der Staat entschieden hat.
Das letzte Mal, als diese Rate \xfcber 2 betrug - was auch als Ersetzungsrate bekannt ist - war im Jahr 1976.
"F\xfcr mich ist es wichtig, \xfcber mein eigenes Geld und Zeit zu verf\xfcgen" sagt ein anderer, ungef\xe4hr zwanzig Jahre alter Mann.
Oder: W\xfcrde es Dir gefallen, wenn man ein Foto von dir ver\xf6ffentlicht, wie das, das du von einem Freund ver\xf6ffentlicht hast?
"Jemand au\xdferhalb des Internets handelt mit Respekt, Sittlichkeit und anderen Prinzipien, und dasselbe muss f\xfcr die sozialen Netzwerke gelten", erkl\xe4rt er.
Estuardo Guardia, Universit\xe4tsprofessor, Grundschullehrer und erzieherischer Berater, kommentiert, dass es unverzichtbar, dass die Eltern die Richtlinien der sozialen Netzwerke sorgf\xe4ltig durchlesen.
W\xe4hrend des Tages wurde im Presseraum nur das Bild des Pr\xe4sidententreffens ohne Ton mit der Meldung "private Sitzung, beschr\xe4nktes Audio" \xfcbertragen.
Wir handeln nicht mit den Menschenrechten, dieses Wort wenden wir f\xfcr diesen Fall nicht an, es habe allerdings st\xe4ndige Gespr\xe4che gegeben.
Um diesen Fortschritt richtig einordnen zu k\xf6nnen, muss daran erinnert werden, dass die Lebenserwartung der Mexikaner heute durchschnittlich 76 Jahre betr\xe4gt.
Der erste Punkt w\xfcrde bedeuten, dass die internationale Zusammenarbeit in Verfahren bei Zahlungsunf\xe4higkeit von Unternehmen mit l\xe4nder\xfcbergreifendem Profil nicht bekannt ist.
Der Weltenbummler des Basketballs, H\xe9ctor "Hetin" Reyes, war dem Korbsport l\xe4nger als 60 Jahre verbunden und hat die ganze Welt bereist.
Wenige in Puerto Rico verf\xfcgen \xfcber eine so gro\xdfe geistige Sammlung der Geschichte des Basketballs des Landes wie H\xe9ctor "Hetin" Reyes.
Ich wei\xdf noch, wie er sagte, dass, wenn Mincy eine Meisterschaft f\xfcr Bayamon erm\xf6glicht hatte, Gausse f\xfcr eine weitere sorgen w\xfcrde.
Die Aufnahme von f\xfcnf Kapiteln f\xfcr die zweite Staffel war abgeschlossen, und ein sechstes Kapitel wurde gerade gedreht, informierte der Sender.
Von Warner oder von TNT gab es keine sofortige Erkl\xe4rung dazu, wie der Verlust von Hagmann in der Serie behandelt w\xfcrde.
Es ist wichtig anzumerken, dass die US-B\xfcrger im Gegensatz zu Quebec nicht \xfcber eine universelle Ausweiskarte wie die Krankenversicherungskarte verf\xfcgen.
Dar\xfcber hinaus haben Sie das Recht von Einzelpersonen und Gruppen beschr\xe4nkt, jenen W\xe4hlern Hilfestellung zu leisten, die sich registrieren m\xf6chten.
Im Gegensatz dazu machten die Wei\xdfen, die 76% der W\xe4hler darstellten, nur 46% der W\xe4hler aus, die im Voraus w\xe4hlten.
Am wichtigsten ist es aber, mit seinem Arzt zu sprechen, um zu bestimmen, ob er durchgef\xfchrt werden sollte oder nicht.
"Wenn es keine Raucher mehr g\xe4be, w\xfcrde dieser Wert mindestens auf 50% ansteigen", betont Andr\xe9 Beaulieu, Sprecher der kanadischen Krebsgesellschaft.
Die Ank\xfcndigung der wahrscheinlichen Entdeckung des Higgs-Bosons hat im letzten Sommer ein gewisses Aufsehen erregt, und dies aus gutem Grund.
Die Analogie mit dem elektromagnetischen Feld ist erneut hilfreich, um die Beziehung zwischen dem Higgs und der Masse zu erkl\xe4ren.
Einige, wie Magnete, tun dies, aber andere nicht - beispielsweise w\xfcrde ein Blatt Papier niemals von selbst am K\xfchlschrank halten.
\xdcberall dort, wo er gespielt hat, hat er vor Augen gef\xfchrt, dass er ein gro\xdfartiger Spieler und ein Weltstar ist.
Pierre Noizat, der ebenfalls Autor eines Buchs \xfcber diese W\xe4hrung ist, glaubt fest an das Potenzial dieser Technologie als Transaktionsnetzwerk.
Sie wollen ihre jahrhundertealten und archaischen Traditionen verteidigen, auch wenn sich ihnen Dschihadisten, Pakistani, Araber, Usbeken und Tadschiken angeschlossen haben.
Ehemalige Mudschaheddin, die afghanische Regierung und aktuelle Taliban haben den gemeinsamen Wunsch, die Frauen in einer untergeordneten Position zu halten.
Wie ich es in den Kampagnen geh\xf6rt habe, w\xfcnschen sich die Leute eine Regierung, die sich nicht aus Dieben zusammensetzt.
Etwa 65% der Bev\xf6lkerung ist unter 25 Jahren; Kabul hat jetzt 5 Millionen Einwohner, was ein F\xfcnftel der Gesamtbev\xf6lkerung ist.
Zur \xdcberraschung aller hat er am Mittwoch verk\xfcndet, dass die verfassungsgebende Versammlung am n\xe4chsten Tag seine endg\xfcltige Fassung verabschieden werde.
Im Einklang mit dem Wunsch des Milit\xe4rs wird die Pr\xfcfung des Verteidigungshaushalts nicht dem Parlament vorgelegt, sondern einem nationalen Verteidigungsrat.
Ebenso wird es kein Verbot von Zivilverfahren in Milit\xe4rgerichten geben, wie es die Vereinigungen zur Verteidigung der Menschenrechte gefordert haben.
Das f\xfcnfte Museum, n\xe4mlich das Holocaust-Museum bzw. Yad Vashem in Tel Aviv, erz\xe4hlt von einem der ersch\xfctterndsten Kapitel der Geschichte.
In Caesarea, der Stadt von K\xf6nig Herodes, k\xf6nnen Sie durch das r\xf6mische Theater streifen und die Festung der Kreuzritter erobern.
Wenn Sie nach Israel fahren, machen Sie sich keine Sorgen wegen Ihrer schlechten Englischkenntnisse: Ungef\xe4hr 30% der Israelis sprechen Russisch.
Ein Mietwagen kostet je nach Marke zwischen 37 Dollar pro Tag (Hyundai Getz) bis 188 Dollar (Audi A6, Volvo S80).
Das ist mehr als doppelt so viel wie die Kosten f\xfcr den offiziellen Test: Dieser kostet einen Arbeitsmigranten dreitausend Rubel.
Der erste Kanal ist die Armee bzw. das Milit\xe4r, d. h. Waffen, die w\xe4hrend der K\xe4mpfe im Kaukasus gestohlen wurden.
Der F\xf6derale Sicherheitsdienst schaltete vor Kurzem unz\xe4hlige Scheinwebseiten, und K\xe4ufer, die Waffen erwerben wollen, gehen dem Dienst zuhauf ins Netz.
Der F\xf6derale Sicherheitsdienst schaltete vor Kurzem unz\xe4hlige Scheinwebseiten, und K\xe4ufer, die Waffen erwerben wollen, gehen dem Dienst zuhauf ins Netz.
Noch kann niemand vorhersagen, ob die Proteste noch weiter anschwellen werden oder ob ihnen schon bald wieder die Luft ausgeht.
Die Bewegungen des Menschen sind \xe4u\xdferst dynamisch und offen gesagt, sind die jetzigen 30 fps insbesondere f\xfcr Gesten zu wenig.
Im Jahr 2000 gab es in der Presse eine Umfrage, bei der es um die Auszeichnung "Pers\xf6nlichkeiten unserer Stadt" ging.
- Vor Kurzem sahen wir dich in der Rolle des st\xe4dtischen Drehorgelspielers. - Eine Kulturstadt sollte so einen Helden haben.
Aus kulturellen Gr\xfcnden kommen 300 Personen und nicht 10 Tausend, folglich gibt es weniger Management, Geld, und alles geht zugrunde.
W\xe4hrend f\xfcr ein neugeborenes Kind die Schwerelosigkeit also ein viel nat\xfcrlicherer Zustand ist, kommt die Frau nicht ohne Schwerkraft aus.
Hierzu ist noch anzumerken, dass auch diejenigen L\xe4nder, die f\xfcr uns ein Vorbild sind, ebenfalls mit Problemen zu k\xe4mpfen haben.
Was die tschechische Gesetzgebung betrifft, welche Bedeutung hatte f\xfcr Ihre Beh\xf6rde die Novellierung des Vergabegesetzes, sp\xfcren Sie schon irgendwelche Auswirkungen?
Ich denke, dass dieses Gesetz bestimmt ein Schritt in die richtige Richtung ist und hoffe, dass sich diese Annahme best\xe4tigt.
Die Autobahn D5 ist praktisch uneingeschr\xe4nkt befahrbar, erh\xf6hte Aufmerksamkeit empfehlen die Stra\xdfenmeistereien jedoch zwischen dem 80. und dem 131. Kilometer.
Die Fahrbahnen der zweiten und dritten Stra\xdfenklasse sind feucht, und daher gilt auch hier der Hinweis auf m\xf6gliche vereiste Abschnitte.
Nach dem Einsatz von Streufahrzeugen bleibt Schneematsch auf dem Pass  \u2047 ervenohorsk\xe9 sedlo sowie auf der Stra\xdfe in Richtung Videlsk \u2047  k \u2047 \xed \u2047 .
Hierf\xfcr wollen wir das Marketingpotenzial des Maya-Kalenders nutzen, dessen Ende f\xfcr den 21. Dezember um 11:10 Uhr morgens prognostiziert ist.
Am Tag davor, d.h. am 20. Dezember, finden ab 21:00 Uhr gleichzeitig drei Konzerte in Prag, Brno und Ostrava statt.
Da die Sch\xfcler selbst nicht \xfcber die Mittel verf\xfcgen, um die Lektoren aufzusuchen, m\xf6chten wir ihnen auf diese Weise helfen.
In Prag treten beispielsweise Chinaski, Support Lesbiens, Illustratosphere mit Dan B\xe1rta, The Tap Tap, Mari\xe1n Bango und Ji \u2047 \xed Such \u2047  auf.
Na, und mit der Zeit ist das, wie unser Moderator, L\xe1 \u2047 a Angelovi \u2047 , zu sagen pflegt, etwas au\xdfer Kontrolle geraten (lacht).
Aber dieses Mitleid ist absolut \xfcberfl\xfcssig, weil Menschen mit Behinderungen keine einsamen und verlassenen Wesen sind, die wir bedauern m\xfcssten.
Schon vor dem Zweiten Weltkrieg besch\xe4ftigten sich polnische Kosmosbegeisterte mit der Raumfahrt, wobei sie damit nicht immer auf Verst\xe4ndnis stie\xdfen.
 \u2047 ternfeld gewann im Jahr 1934 f\xfcr "Eingang zur Kosmonautik" den von Robert Esnault-Pelterie und Andr\xe9 Louis Hirsch gestifteten Prix REP-Hirsch.
Kurz vor dem Krieg wurden alle Projekte zur milit\xe4rischen Nutzung der Raketentechnik vom Vor\xfcbergehenden wissenschaftlichen Beratungsausschuss (Tymczasowy Komitet Doradczo-Naukowy) koordiniert.
Die Rakete mit einer maximalen Flugh\xf6he von 1800 m war etwa 80 cm lang und wog nicht ganz 5 kg.
Ziel dieser Ma\xdfnahmen ist es, die eigene Bev\xf6lkerung dazu zu zwingen, das Diktat des Privatkapitals insbesondere im Lohnbereich zu akzeptieren.
Das Ergebnis, heute wie damals, ist eine beispiellose Dekadenz der Eliten, die sich nicht im Geringsten um tiefergehende Reformen bem\xfchen.
Im November 1979 besetzte ein Mob demonstrierender islamistischer Studenten die US-amerikanische Botschaft in Teheran und nahm 52 Diplomaten als Geiseln.
Das Debakel im Iran trug erheblich zur Niederlage Jimmy Carters gegen Ronald Reagan bei den Pr\xe4sidentschaftswahlen im Jahr 1980 bei.
Eine \xe4hnliche Wirkung erzielt Affleck mit seinem Team auch bei fiktiven Szenen (der falsche Filmstab auf einem Basar in Teheran).
Die EU berief sich dabei auf eine amerikanische Studie, der gem\xe4\xdf Luftballons die f\xfchrende Ursache beim Erstickungstod von Kindern sind.
Als einfacher B\xfcrger habe ich mich daf\xfcr eingesetzt, dass der Reisef\xfchrer ein freies Gewerbe bleibt, und dies konnte durchgesetzt werden.
Politiker, Journalisten und die \xd6ffentlichkeit zu \xfcberzeugen und zu versuchen, sie auf unser Seite zu bringen, um diese Ziele durchzusetzen.
Ich glaube, sie tasten sich noch an ihre Rolle heran, aber sie sind auf dem Weg zu einer "normaleren" Au\xdfenpolitik.
Auch wenn es ihnen nicht gef\xe4llt, es ihnen unangenehm ist und sie noch viel unbeliebter macht - c'est la vie!
Der Volvo-K\xe4ufer Geely nutzte urspr\xfcnglich ein blau-wei\xdfes Logo, das an BMW erinnerte; der Streit wurde geschlichtet, Geely musste es \xe4ndern.
Im vergangenen Jahr gingen beim CTMO mehr als 1,4 Millionen Antr\xe4ge auf Markenschutz ein, fast ein Drittel mehr als 2010.
An die f\xfcnfzig S\xe4ngerinnen und S\xe4nger sind gekommen, zwischen 23 und 69 Jahre alt, von der Humangenetikerin bis zum Hausmann.
Das ist keine Selbstverst\xe4ndlichkeit, denn so offensichtlich die Krankheit im ganzen Land auch ist, man schweigt sie am liebsten tot.
Der Name Trifid stammt von dem lateinischen Wort trifidus (dreigeteilt, dreigespalten), da dunkle Staubstreifen das gl\xfchende Herz der Sternen-Geburtsst\xe4tte dreiteilen.
Die Keck-Teleskope sind Teil des Mauna-Kea-Observatoriums, das neben ihnen noch mit dem Subaru-Teleskop und dem IRTTF in den Himmel blickt.
Der sagenhafte Reichtum, den das Land seinem \xd6l im Kaspischen Meer verdankt, ist hier in der Provinz noch nicht angekommen.
Viele verschleierte Frauen und Anh\xe4nger der Salafisten nahmen daran teil und riefen: "Das Volk fordert die Anwendung von Gottes Gesetz."
Ein Kampf um die Hoheit \xfcber den symboltr\xe4chtigen Tahrir-Platz, auf dem alles seinen Anfang nahm, h\xe4tte wohl b\xfcrgerkriegs\xe4hnliche Zust\xe4nde heraufbeschworen.
Selbst aus Schweden, dem alten Rivalen, der vor noch nicht allzu langer Zeit weitaus reicher war als Norwegen, str\xf6men Einwanderer.
In diesem dicht besiedelten, weitl\xe4ufigen Teil des Landes, der die Hauptstadt umgibt, sind die Meinungen \xfcber das neue Staatsoberhaupt geteilt.
"Ich hoffe, als Pr\xe4sident ist er so, wie er als Gouverneur war", sagt der PRI-Kongressabgeordnete Olvera in Valle del Bravo.
Er m\xf6chte sich mit den Vereinigten Staaten und Kanada verb\xfcnden und einen nordamerikanischen Handelsblock nach Vorbild der Europ\xe4ischen Union schaffen.
Mexiko hat Gewinner und Verlierer. Menschen, f\xfcr die das Land Chancen bietet, und andere, f\xfcr die es dies nicht tut.
Experten zufolge liegt der Haken in der Beliebtheit sozialer Medien bei genau der Bev\xf6lkerungsgruppe, an die sich der Plan richtet.
British American Tobacco Australia sagt, dass sich die Industrie statt auf Marketing darauf konzentriere, sich mit den neuen Gesetzen auseinanderzusetzen.
Professor Larson sagt heute, 21 Jahre sp\xe4ter, er wisse nicht, ob die Prozentanteile hinsichtlich der Langeweile gestiegen oder gesunken sind.
Hunderte von Ordnungswidrigkeiten, die sich um Marihuana drehen, werden hier und im Staate Washington, der \xe4hnliche Ma\xdfnahmen genehmigte, bereits fallengelassen.
Die Polizei in Grand Junction, der gr\xf6\xdften Stadt des Landkreises, zeigt Erwachsene f\xfcr den Besitz kleinerer Mengen nicht l\xe4nger an.
Ich machte die Erfahrung, dass die Tutoren die Verspottung von Tory-Studenten nicht nur duldeten, sondern sogar mit Freuden daran teilnahmen.
Die drei Jahre, die vor mir lagen, dehnten sich vor meinem geistigen Auge zu einem Fegefeuer der \xc4chtung und Isolation.
Vor vielen Jahren gingen wir nach einer Modeschau am Piazza di Spagna in Rom zu ihm nach Hause zum Abendessen.
Es war ein rotes Kleid mit fliegendem Rock und einem drapierten Oberteil mit einem Dekollet\xe9, das seinem Namen Ehre macht.
Anto hat Asthma, atmet mit Schwierigkeit, hustet h\xe4ufig und seine Augen sind wegen der giftigen Gase aus dem Vulkan gereizt.
Mit dem Korb auf seinem R\xfccken ist Unainik mit seinen 53 Jahren nurmehr in der Lage, 50 kg zu tragen.
"Die sozialen Netzwerke sind unterhaltsam, ich kann schnell mit Verwandten in der Ferne oder mit Freunden sprechen" gibt er an.
Der gastgebende Pr\xe4sident Ollanta Humala er\xf6ffnete die Gespr\xe4che am Vormittag und beendete das Gipfeltreffen kurz nach der Mittagszeit in Lima.
Wenn ich gewinnen sollte, w\xe4re es meine letzte Periode als Pr\xe4sident, danach ziehe ich mich aus dem \xf6ffentlichen Leben zur\xfcck.
Der Staat liegt national gesehen an 4. Stelle neuer und kumulierter AIDS-F\xe4lle, und an 13. Stelle in Bezug auf HIV.
Victoria Principal, Mitdarstellerin der Originalserie, erinnerte sich am Freitag an Hagman als eine "enorme Pers\xf6nlichkeit auf und au\xdferhalb des Bildschirms".
Nach der Lebertransplantation setzte er sich f\xfcr Leberspenden ein und arbeitete als Freiwilliger in einem Krankenhaus, um \xe4ngstlichen Patienten beizustehen.
"Ich berate sie, gebe ihnen Mut, ich treffe mich mit ihnen, wenn ihre Operationen bevorstehen und danach", erkl\xe4rte er 1996.
Jede Woche untersuchen die Studenten apokalyptische Themen wie z. B. den Atomkrieg, Zombies, Virus und Keime und die globale Erw\xe4rmung.
Jede Woche untersuchen die Studenten apokalyptische Themen wie z. B. den Atomkrieg, Zombies, Virus und Keime und die globale Erw\xe4rmung.
Die Mayas sagten nie das Ende der Welt voraus; es handelt sich nur um einen Schl\xfcsselpunkt im Kalender, sagte Restall.
"Vielleicht rufe ich ein paar Freunde an, damit wir zusammen lachen k\xf6nnen", sagte Samira Ford, eine 20-j\xe4hrige Studentin f\xfcr Kommunikationen.
Beispielsweise haben die Kampagnen zur W\xe4hlerregistrierung bei den allgemeinen Wahlen 2004 dazu beigetragen, ca. 10 Mio. Staatsb\xfcrger zu registrieren.
Es wird gesch\xe4tzt, dass 30% der Krebserkrankungen verhindert werden k\xf6nnten, wenn alle gut essen und sich ausreichend bewegen w\xfcrden.
F\xfcr die kanadische Krebsgesellschaft bleibt der Kampf gegen die Tabakabh\xe4ngigkeit eine Priorit\xe4t, trotz des R\xfcckgangs der Zahl der Raucher.
Es muss hier aber betont werden, dass diese Bosonen nicht alle derart exotische Kreaturen sind, wie man meinen k\xf6nnte.
Die Auswirkungen dieser Forschungen f\xfcr die Allgemeinbev\xf6lkerung sind schwieriger vorherzusagen, aber es w\xe4re falsch anzunehmen, dass es keine g\xe4be.
"Im Laufe unseres Lebens erfahren wir, dass ein Mann im Stehen pinkelt", erz\xe4hlt Pierre Brodeur, Psychologe im Heim Victor-Gadbois.
Aber das bedeutet nicht zwangsl\xe4ufig, "ich will, dass Sie mich einschl\xe4fern", sondern "ich m\xf6chte, dass meine Schmerzen gelindert werden".
Ausdr\xfccklich angeklagt wurden \xfcbrigens Ingenieure des Stra\xdfenbauamts von Montreal, sowie Unternehmer italienischen Ursprungs, wie Tony Accurso und Lino Zambito.
Letzterer hat Aufsehen erregt, indem er der Kommission die Funktionsweise des "Systems" f\xfcr den Erhalt \xf6ffentlicher Auftr\xe4ge erkl\xe4rt hat.
Zun\xe4chst wollen wir Erster unserer Gruppe vor Porto werden, damit wir das R\xfcckspiel des Achtelfinales als Heimspiel austragen k\xf6nnen.
Die Transaktion ist somit dauerhaft mit der Kette aller anderen Transaktionen verkn\xfcpft, und jegliche Modifikation w\xfcrde den Fingerabdruck \xe4ndern.
"Drei\xdfigtausend Dollar wurden eingetauscht", freut sich Jon Holmquist, der f\xfcr das Unternehmen Coinabul arbeitet, das Bitcoins in Gold konvertiert.
Toleriert, manchmal von den lokalen Aufst\xe4ndischen unterst\xfctzt, werden Letztere nicht mehr da sein, wenn die westlichen L\xe4nder diskreter werden.
W\xe4hrend ihres Exils in Iran oder Pakistan haben sie Kontakt zur modernen Welt gehabt, und haben deren Vorteile genossen.
In einem Land, das von 30 Jahren Krieg zugrunde gerichtet wurde, w\xe4re eine staatliche Kontrolle der Infrastrukturen erforderlich gewesen.
Dar\xfcber hinaus bezieht sich kein Artikel mehr auf den Schutz der Frauen, unterstreicht Heba Morayef von Human Rights Watch.
In Caesarea sollten Sie das einzigartige private Ralli Museum besuchen, wo Sie Skulpturen von Dali und Rodin bewundern k\xf6nnen.
In der r\xf6mischen Zeit war Caesarea die wichtigste Stadt Jud\xe4as und Residenz der r\xf6mischen Statthalter, darunter auch Pontius Pilatus.
Bisher gilt diese Regelung nur f\xfcr Migranten, die im Dienstleistungssektor, in der kommunalen Wohnungswirtschaft und im Einzelhandel arbeiten wollen.
Dabei muss man nicht nur Sprachtests, sondern auch Tests in die russische Geschichte und die Grundlagen der Gesetzgebung ablegen.
B\xfcrgerrechtler hingegen stellten vor dem Inkrafttreten des Gesetzes in der Presse mehrmals folgende Frage: Was bringt das Ganze eigentlich?
Dar\xfcber hinaus werden Neuank\xf6mmlingen ohne Sprachkenntnisse Stellen in Bereichen angeboten, in denen keine aktive Verst\xe4ndigung mit Menschen notwendig ist.
"Dort gibt es eine eigene, manchmal handwerkliche Produktion sowie eine Mafia, die den Schmuggel organisiert", erl\xe4utert der ehemalige Milit\xe4rangeh\xf6rige.
"Sie ben\xf6tigen nur die passende Summe Geld", hei\xdft es in der Werbeanzeige auf der Webseite "Kampfpistole oder Gewehr kaufen".
Ich habe von folgendem Schema geh\xf6rt: Die Webseite ist normalerweise im Ausland registriert, und russische Gesetze finden keine Anwendung.
Das US-amerikanische Gesetz verbietet es der Unternehmensf\xfchrung, diesem Ziel im Weg zu stehen und Gewerkschaftsmitglieder abzumahnen oder zu entlassen.
Sie reizt die M\xf6glichkeit, virtuelle Objekte in der Luft mit blo\xdfen H\xe4nden zu manipulieren und virtuelle Freifl\xe4chen zu erschaffen.
- Wir besch\xe4ftigen uns mit der Interaktion von Mensch und Maschine, wollen dabei jedoch die Grenzen dieser Interaktion erweitern.
Das k\xf6nnen zum Beispiel Lasersensoren sein, da sie in der Tiefe eine gute Aufl\xf6sung bieten, was sehr wichtig ist.
So gesehen sind alle gegenw\xe4rtigen Technologien f\xfcr uns nicht gut genug, da die Entwickler der Algorithmen mehr Arbeit haben.
Es muss nicht nur die Aufl\xf6sung entlang der X- und der Y-, sondern auch entlang der Z-Achse ber\xfccksichtigt werden.
Rosbalt setzt das Projekt "Petersburger Avantgarde" fort, das Stadtbewohnern gewidmet ist, die die Avantgarde der Kunst und Kultur bilden.
Wir haben nur \xe4u\xdferst wenige Kosmonauten, bei denen nach langen Fl\xfcgen alles gut ging und sie gesunden Nachwuchs bekamen.
Und doch muss die Menschheit nach neuen Wegen in der Biotechnologie, dem Strahlenschutz und dem Erzeugen k\xfcnstlicher Gravitation suchen.
Auch wenn Erwachsene Wasser als angenehm empfinden, ist es eine fremde Umgebung; doch S\xe4uglinge empfinden Wasser als nat\xfcrliches Element.
Tschechien verf\xfcgt im Zusammenhang mit \xf6ffentlichen Auftr\xe4gen \xfcber gute Kontrollinstanzen und ad\xe4quate Gesetze, f\xe4llt jedoch in deren Anwendung zur\xfcck.
N\xe4chtliches Schneetreiben zwang die Stra\xdfenmeistereien zum Einsatz, im Kreis  \u2047 umperk fielen laut Angaben der Stra\xdfenverwaltung etwa 3 cm Neuschnee.
Wir kooperieren auch mit weiteren Pers\xf6nlichkeiten der tschechischen Kulturszene, was damit zusammenh\xe4ngt, dass wir viele Benefizveranstaltungen und Konzerte realisieren...
In Rahmen der Fertigstellung des Jedli \u2047 ka-Instituts soll ein eigenes Geb\xe4ude entstehen, in das wir dann mit diesem Projekt einziehen.
Und da ich selbst Musiker bin und u.a. Saxofon spiele, habe ich zusammen mit einem Kollegen eine Musik-AG gegr\xfcndet.
Das ist auf seine Weise logisch, da alles Neue mit Vorsicht betrachtet und erst nach l\xe4ngerer Zeit akzeptiert wird.
Es sind Menschen, die ein vollwertiges Leben leben und sich entwickeln k\xf6nnen, sofern sie die dazu notwendigen Mittel haben.
War es f\xfcr diesen Erfolg auch hilfreich, dass Sie ein strenger Chef sind, wie man von vielen Leuten h\xf6rt?
Es ist noch nicht einmal gekl\xe4rt, ob die Rakete zum Starten oder zum Bremsen der Draisine eingesetzt werden sollte.
Im folgenden Jahr wurde der erste PTA-Vorsitzende, Kazimierz Zarankiewicz (1902 - 1959), Stellvertretender Vorsitzender der Internationalen F\xf6deration f\xfcr Raumfahrt.
Sp\xe4ter wurde eine verbesserte Version, die RM-1A, gebaut, und 1959 begannen in der B \u2047 d\xf3w-W\xfcste Flugtests mit der Zweistufenrakete RM-2.
Die Meteor-1A-Rakete verf\xfcgte \xfcber einen Transportraum mit 0,4 Litern Fassungsverm\xf6gen, Meteor-1B \xfcber 0,34 Liter und Meteor-1C \xfcber 0,62 Liter.
In den Jahren 1965 bis 1968 wurde im Luftfahrtinstitut die Meteor-2-Rakete entwickelt, deren erste Flugtests im Oktober 1970 begannen.
Nach der letzten Welle der Gewalt zwischen Israel und dem Gazastreifen gab es, wie immer, eine Unzahl von Reaktionen.
Die gefangen genommenen Diplomaten wurden schlie\xdflich nach 444 Tagen freigelassen, nachdem Verhandlungen durch die algerische Regierung vermittelt worden waren.
Der Regisseur musste sich auch damit auseinandersetzen, dass die Geschichte eigentlich nicht viele im filmischen Sinne spannende Szenen bietet.
Da Tschechien einen weiteren Weg zu Seeh\xe4fen habe, sollte die EU laut Palas Hunderte Millionen Euro an uns zahlen.
Wenn ich aber etwas sehe, was mir nicht gef\xe4llt, dann versuche ich eine L\xf6sung vorzuschlagen, um dies zu \xe4ndern.
Mein Ziel ist aber nicht die Funktion. Die Funktion ist ein Instrument, mit dem ich meine Visionen realisieren kann.
Als unabh\xe4ngiger Parteiloser verf\xfcge ich \xfcber ein weitaus gr\xf6\xdferes Potenzial, Unterst\xfctzung bei allen im Parlament vertretenen Parteien zu gewinnen.
Es geht mir nicht darum, ob jemand zum linken oder zum rechten Lager geh\xf6rt; ich m\xf6chte die Menschen verbinden.
Mit der Politik habe ich gerade erst angefangen und versuche, f\xfcr mein Programm die Unterst\xfctzung der Mehrheit zu finden.
Der Grund: Zur Er\xf6ffnung vor wenigen Wochen wurde jeder Bewohner eingeladen, ein Buch aus seinem pers\xf6nlichen Bestand zu spenden.
Also k\xf6nnen sie nicht Teil einer breiteren Linie sein und m\xfcssen stattdessen Dinge aus ihrer eigenen Position heraus vorantreiben.
Dahinter verbirgt sich eine in China ganz offiziell eingetragene Bezeichnung, die allerdings nichts mit den Ursprungsunternehmen zu tun hat.
Sowohl er als auch der Anwalt Pattloch raten deutschen Unternehmen dazu, bei Gesch\xe4ften mit China sehr vorsichtig zu sein.
Zuerst ist da das Stampfen: Cowboystiefel, Basketballschuhe, Damenpumps und Herrenslipper suchen auf dem Parkettboden den Takt, finden ihn schnell.
Es ist Montagabend, im Musikraum des Institutes f\xfcr Medizinische Psychologie in Heidelberg probt der Chor Imbongi ein neues Lied.
Weltweit gibt es rund 34 Millionen HIV-Infizierte, das sch\xe4tzt Unaids, das Programm der Vereinten Nationen zur Bek\xe4mfung von Aids.
Durch Patenschaften, Spenden und nicht zuletzt die Gagen, die sich der Chor in ganz Deutschland ersingt, kommt einiges zusammen.
Auch wenn man das kleine Dorf auf Landkarten kaum findet, im Tal des Ezulweni-Flusses ist es mehr als bekannt.
Unbemerkt von den Erdenb\xfcrgern sind Sonden, Teleskope und kleine Roboter wie Phoenix dabei, die Tiefen des Weltalls zu erforschen.
Auch diese Sternen-Wolke, verbunden mit dem Rosetten-Nebel, bringt laufend neue Babysterne hervor - 5000 Lichtjahre von der Erde entfernt.
Forscher vermuten, dass er erst kurz nach dem Urknall entstanden ist, als im Universum vorwiegend Wasserstoff zu finden war.
Eine der Aufgaben des Teleskops: Es soll nach Licht von den ersten Sternen und Galaxien nach dem Urknall suchen.
Durch die 2004 gestartete Messenger-Sonde - die erste, die um den Merkur kreist - haben die Wissenschaftler nun Gewissheit.
Mirzayeva, die behauptet, 143 Nachfahren zu haben, lebt in einem einfachen Holzhaus, das typisch ist f\xfcr die gesamte Kaukasusregion.
Acht Menschen leben hier unter einem Dach, darunter einer von Mirzayevas S\xf6hnen und eine Tochter, beide sind l\xe4ngst Gro\xdfeltern.
"Wenn er das Referendum ausruft, werden wir zu seinem Palast gehen und ihn st\xfcrzen", sagte der Oppositionelle Jasser Said.
Nun sei die Zeit, das Volk an der Wahlurne entscheiden zu lassen, in welche Richtung das Land gehen solle.
Es gibt hier Schnee, spektakul\xe4re Landschaften - und diesen hartn\xe4ckigen Geruch in der Luft, der einfach nicht verschwinden will.
Aber eigentlich ist hier ja alles teuer - ein kleines Glas Bier oder ein Sandwich kostet stolze 10 Euro.
Norweger tun sich schwer damit, zu akzeptieren, dass jemand in ihrem friedliebenden Land zu solch brutalen Morden f\xe4hig ist.
Die Formulare, so Fein, enthielten keine Beschwerden \xfcber Misshandlung, obwohl die Beamten Manning direkt zu seiner Behandlung befragt hatten.
Manning antwortete, seine Absicht w\xe4hrend dieses Treffens habe darin bestanden, seinen Beobachtungsstatus zur "Pr\xe4vention von Verletzungen" herabstufen zu lassen.
Aber f\xfcr Mexikaner, die in Jahrhunderten und nicht in Minuten denken, sind Erinnerungen an dieses Ereignis nicht zu \xfcbersehen.
Sie sehen uns als Mahnmal einer dem\xfctigenden Niederlage und schauen auf uns herab, weil wir nicht mexikanisch genug sind.
Doch viele mexikanische Amerikaner, die ich kenne, haben das Gef\xfchl, weder zum einen noch zum anderen Land zu geh\xf6ren.
Doch obwohl Israelis und Pal\xe4stinenser in ihrem historischen Konflikt gefangen scheinen, ver\xe4ndert sich der Nahe Osten um sie herum.
Selbst wenn der am 21. November vereinbarte Waffenstillstand anh\xe4lt, haben die diesw\xf6chigen K\xe4mpfe die Hartgesottenen auf beiden Seiten gest\xe4rkt.
Vielleicht werden sich die Hardliner durchsetzen k\xf6nnen. Doch der arabische Fr\xfchling k\xf6nnte ihnen einen Strich durch die Rechnung machen.
Wenn es nach ihnen geht, ist es f\xfcr uns - und unsere Kinder - okay, gelegentlich gelangweilt zu sein.
Wenn einem langweilig ist und man diese Energie verwendet, um Gitarre zu spielen und zu kochen, wird man gl\xfccklich.
Aber Staatsanw\xe4lte in den konservativeren Bezirken Colorados haben angek\xfcndigt, bestehende Marihuanadelikte weiterzuverfolgen und zitieren immer noch Menschen vor Gericht.
Es war ein Englischstudent aus dem zweiten Jahr namens James, der sich als Mitglied der konservativen studentischen Vereinigung vorstellte.
An jedem Detail seiner Wohnung, der Dekoration, am Essen und an der Musik erkannte und sp\xfcrte man seinen Einfluss.
Seit den Wahlen wurde ein Versuch unternommen, das Problem mit h\xf6heren Beitr\xe4gen und Abgaben f\xfcr ausl\xe4ndische Arbeiter zu korrigieren.
Sie sind so popul\xe4r, und die Einheiten sind um Tage und sogar Wochen schneller ausverkauft als die gr\xf6\xdferen Wohneinheiten.
"Ich w\xfcrde kein Foto teilen, das nicht von mir ist, oder von jemandem, der den Dummkopf macht" sagt er.
"Wenn jemand mich bedr\xe4ngt oder sie von mir verlangt, entferne ich ihn einfach von meinem Benutzerkonto" gibt er zu.
Ein weiterer Punkt ist, ihnen zu verstehen zu geben, dass sie online handeln m\xfcssen, wie sie es offline tun.
Auf der offiziellen Webseite des ASPA kann man sich davon \xfcberzeugen, dass das Dokument am vergangenen Dienstag ver\xf6ffentlicht wurde.
Correa versicherte, dass, wenn er die Wahlen im Februar 2013 verl\xf6re, er sich aus dem politischen Leben zur\xfcckziehen w\xfcrde.
Damals vermied es selbst der Direktor einer Klinik des IMSS, sich zu verabschieden, "weil es in eine Sackgasse f\xfchrte."
Zu seinen Kinoarbeiten geh\xf6rten von der Kritik gut bewertete Rollen in "The Group", "Harry and Tonto" und "Primary Colors".
Zehn Episoden der neuen Ausgabe von "Dallas" wurden vor ein paar Monaten mit gro\xdfem Erfolg im Fernsehkanal TNT ausgestrahlt.
"Die Philippinen beteiligen sich nicht am Ende der Welt", schrieb er als Andeutung auf eine Ausnahme einer h\xf6heren Instanz.
Die Rechtsanw\xe4lte der Republikaner haben in 10 Jahren in den USA \xfcbrigens nur 300 F\xe4lle von Wahlbetrug verzeichnet.
Infolgedessen wurden 180 Gesetzesentw\xfcrfe allein im Jahr 2011 eingef\xfchrt, die die Aus\xfcbung des Wahlrechts in 41 Staaten einschr\xe4nken.
Seit 2011 haben ein Dutzend Staaten Gesetze verabschiedet, die von den W\xe4hlern fordern, dass sie ihre US-Staatsb\xfcrgerschaft nachweisen.
"Die Forschung zeigt, dass eine regelm\xe4\xdfige k\xf6rperliche Aktivit\xe4t w\xe4hrend des gesamten Lebens gegen Grimmdarmkrebs sch\xfctzt", f\xfcgt er hinzu.
Aber f\xfcr die Physiker ist es noch nicht vollst\xe4ndig sicher, dass es sich wirklich um das Higgs handelt.
In einer Ecke befinden sich die guten B\xfcrger, die als Fermione bezeichnet werden und artig dem Pauli-Prinzip gehorchen.
Es sind in der Tat nicht alle Teilchen und nicht alle Materialien, die mit dem elektromagnetischen Feld interagieren.
In der Ligue 1 gibt es derzeit keine vergleichbare Person, und er z\xe4hlt zu den besten Trainern Europas.
Eines unserer wichtigsten Ziele ist die Champions League: wir haben uns in dieser Weise f\xfcr das Achtelfinale qualifiziert.
Das Gegenteil des aktuellen monet\xe4ren Austauschs auf der Grundlage von Zentralbanken, identifizierten Transaktionen und Bearbeitungsgeb\xfchren zwischen den Beteiligten.
Dennoch hat die Europ\xe4ische Zentralbank (EZB) in einem im Oktober ver\xf6ffentlichten Bericht \xfcber virtuelle W\xe4hrungen Interesse hierf\xfcr gezeigt.
Mit dem Unterschied, dass der Benutzer f\xfcr jede Bezahlung eine andere Adresse w\xe4hlen kann, was die Anonymit\xe4t sicherstellt.
Das System kann bei den H\xe4ndlern leicht implementiert werden, und Letztere m\xfcssen keine neuen Terminals oder Computerprogramme installieren.
Es ist ein allgemeiner Trend zu verzeichnen, bei dem hierarchische Systeme zugunsten st\xe4rker horizontal ausgerichteter Systeme \xfcberdacht werden.
Sie haben sich in Verruf gebracht, und die meisten von ihnen waren nicht selbst an den K\xe4mpfen beteiligt.
Dies verst\xe4rkt noch den Eindruck, dass die westlichen L\xe4nder nur vor Ort waren, um sich dessen zu bem\xe4chtigen.
Vor gerade einer Woche hatte das Staatsoberhaupt diesem Plenum zwei zus\xe4tzliche Monate f\xfcr den Abschluss seiner Arbeiten gew\xe4hrt.
Die drei wichtigsten Erholungsgebiete Israels liegen an den Ufern des Mittelmeeres, des Roten Meeres und des Toten Meeres.
Fortuna soll der Legende nach allen hold sein, die die W\xe4nde in der Gasse mit ihrem Sternzeichen ber\xfchren.
Welche Ver\xe4nderungen bringt die Vorschrift, Sprachkenntnisse vorweisen zu m\xfcssen, sowohl f\xfcr die Russen als auch f\xfcr die Gastarbeiter?
"Sie wollen ein- oder zweihundert Rubel f\xfcr Zigaretten und Tee", \xe4u\xdfert sich der Tadschike Umed Huschkadamow gegen\xfcber Journalisten.
Experten berechneten, welchen Anteil jeder der f\xfcnf Kan\xe4le an der Belieferung des Schwarzmarkts mit illegalen Waffen ungef\xe4hr hat.
Die Leute kommen wie hungrige Fische bei der F\xfctterung und landen dann in Sibirien und d\xfcrfen Kohle schaufeln
Kritikern zufolge kann Walmart die Ware oftmals nur deshalb so g\xfcnstig verkaufen, weil die Mitarbeiter schlecht bezahlt werden.
W\xfcrde Walmart die Lohnerh\xf6hungen vollst\xe4ndig auf die Kunden umlegen, kostete jeder Einkauf sie k\xfcnftig nur 46 Cent mehr.
Die Eingabe von Informationen (das System erh\xe4lt mehr Daten) konnte verbessert werden, die Ausgabe bisher noch nicht entscheidend.
- Die jetzige Generation ist im Grunde ein guter Ausgangspunkt f\xfcr unsere Arbeit im Bereich der dreidimensionalen Erkennung.
F\xfcr meine Arbeit brauchte ich genau so eine Vorrichtung, nur ohne Ber\xfchrungssteuerung und mit mehr Bildern pro Sekunde.
- Viele meiner Bilder sind echte Perlen und bringen deutlich die Aktualit\xe4t und Sch\xe4rfe der Gedanken zum Ausdruck.
Unsere M\xf6we flog davon, und niemand auf der Erde h\xe4tte folgende Frage beantworten k\xf6nnen: \xdcbersteht sie den Weltraumflug?
Im Juni 1964, nur ein Jahr nach ihrem Weltraumflug, gebar die erste weibliche Kosmonautin, Valentina Tereschkowa, eine Tochter.
Es ist, als w\xfcrden die kleinen Ichtyander Zeugnis davon ablegen, dass das Leben am Land dem Ozean entstieg.
Im Prinzip ist das logisch, da ab der Geburt bis zum ersten Schwimmen gerade einmal 2 Wochen vergehen.
\xd6ffentliche Mittel, die bei uns von den Bezirken und Gemeinden verwaltet werden, unterliegen dort der Kontrolle der Landesrechnungsh\xf6fe.
In der Region schneit es jetzt nicht mehr, und in den tieferen H\xf6henlagen bleibt lediglich eine d\xfcnne Schneedecke.
Da es vorher geschneit hat und die Temperaturen anschlie\xdfend fielen, kann es auf den Stra\xdfen zu Eisgl\xe4tte kommen.
Dabei hat sich gezeigt, dass die meisten an einer Zusammenarbeit mit uns interessiert sind, und Spa\xdf daran haben.
Ihre Auslandspl\xe4ne sind nicht gerade klein, bislang sind Sie schon in Madrid, Br\xfcssel, London oder in Moskau aufgetreten.
Die Forschungsarbeiten f\xfchrte das Institut Kom\xf3rka Techniki Uzbrojenia in Zusammenarbeit mit Prof. Mieczyslaw Wolfke und Prof. Gustaw Mokrzyckiegi.
Der erste Typ, die RM-1, wurde im Jahr 1957 fertiggestellt, der erste Start erfolgte am 10. Oktober 1958.
Mit anderen Worten: Die Regierungen liefern die eigene Bev\xf6lkerung ohne R\xfccksicht auf die sozialen Folgen dem Privatkapital aus.
Die Einzelheiten dieser Operation wurden lange geheim gehalten. Der Film st\xfctzt sich auf die Erinnerungen von Tony Mendez.
Bis dahin genossen Frauen bei Lebensversicherungen einen Vorteil, weil sie f\xfcr die Versicherungsgesellschaften objektiv ein geringeres Risiko darstellen.
In den Senat haben Sie es geschafft und sich dann gleich auf den Weg in die Burg gemacht.
\xdcber mich wurde beispielsweise behauptet, dass ich Journalisten bestechen w\xfcrde oder dass ich Berater von Ji \u2047 \xed Paroubek war.
Als Pr\xe4sident haben Sie in dieser Hinsicht keine Kompetenzen, und nur der Senat als Ganzes kann Gesetzesvorschl\xe4ge einbringen.
Au\xdferdem habe ich die investigative Journalistin Jana Lorencov\xe1 unterst\xfctzt, die den Betrug beim Handel mit leichtem Heiz\xf6l aufdeckte.
Sie fahren einen Aston Martin, haben ein Verm\xf6gen von 60 Millionen und haben kein Geld f\xfcr Ihre Kampagne?
"Wir wollten hier mit Recycling-Materialien arbeiten", erkl\xe4rt Joop Trouborst, Projektleiter bei der Stadtgemeinde Spijkenisse, auf Anfrage des Standard.
Und so sind wir in einem friesl\xe4ndischen Agrarbetrieb eines Tages auf ein passendes Abfallprodukt aus der Landwirtschaft gesto\xdfen.
Seit vielen Jahren verwendet man in den Niederlanden in Gew\xe4chsh\xe4usern und auf Feldern ein millimeterd\xfcnnes Kunststoffvlies als Wurzelunterlage.
F\xfcr die Bibliothek wurde das Vlies - erstmals in diesen Mengen - zu vier Zentimeter dicken Platten gepresst.
Obwohl der B\xfccherberg unter einem Glassturz steht, scheint die Sonne selbst an sonnigen Tagen nur kurz ins Innere.
Die breiten Holzleimbinder, die quer zur Glasfassade stehen, dienen als Beschattung und fangen einen Gro\xdfteil der Sonneneinstrahlung ab.
Denn es signalisiert doch, dass es als internationaler Spieler ernst genommen werden und seine Interessen bedacht werden m\xfcssen.
Sieht sich Deutschland selbst in der Rolle als wichtiger internationaler Spieler - will Deutschland \xfcberhaupt eine Hauptrolle \xfcbernehmen?
Die finanziellen Ausf\xe4lle und die Prozesskosten der betroffenen Branchen gehen in die Millionen, vor allem bei teuren Vorzeigeprodukten.
2009 verlor Daimler einen Rechtsstreit mit dem Baumaschinenhersteller Sany, jenem Unternehmen, das k\xfcrzlich den deutschen Betonpumpenbauer Putzmeister \xfcbernahm.
Beschneidungen der m\xe4nnlichen Vorhaut, die das Ansteckungsrisiko nachweislich um die H\xe4lfte verringern, werden von der Bev\xf6lkerung kaum angenommen.
Bei den heterosexuellen Erwachsenen sind Chlamydien-Infektionen, Trichomonaden, Candidose (Pilz), Tripper und Humane Pappilomaviren h\xe4ufig vorkommende sexuell \xfcbertragbare Krankheiten.
"Insgesamt haben wir schon rund 200 000 Euro nach Esitjeni geschickt", sagt Annette Lennartz, die Vorsitzende des Vereins.
Der 1400 Lichtjahre entfernte Nebel besteht aus Staubk\xf6rnchen, die zehn bis hundert Mal kleiner sind als gew\xf6hnlicher Hausstaub.
Seitdem wurden die Spiegel der optischen Teleskope immer gr\xf6\xdfer - und die Einblicke, die sie liefern, immer tiefer.
Nachteil der g\xfcnstigen Bauweise: Das Teleskop ist in seinem H\xf6henwinkel festgezurrt - und damit in seiner Beweglichkeit beschr\xe4nkt.
Auch auf dem Mauna Kea soll ein neues, riesiges Teleskop entstehen - mit einem Spiegel-Durchschnitt von drei\xdfig Metern.
Allerdings gibt es daf\xfcr keine verl\xe4sslichen Daten, da die Messenger weit n\xe4her am Nordpol um den Planeten kreist.
Doch das hier ist der tiefste S\xfcden von Aserbaidschan, die Grenze zum Iran ist nur wenige Kilometer entfernt.
Ich habe meine Haare immer mit Milch gewaschen, so gingen sie mir nie aus und behielten ihre Farbe.
"Und dass er gelingt, liegt in meiner Verantwortung, vor dem Volk und vor Gott", sagte er im Staatsfernsehen.
Wie in fr\xfcheren Verfassungen auch hei\xdft es in dem Entwurf, die Rechtsprechung gr\xfcnde auf den "Prinzipien islamischen Rechts".
Die Muslimbr\xfcder erkl\xe4rten, sowohl die Gegner des Verfassungsentwurfes als auch die Bef\xfcrworter h\xe4tten sich laut und deutlich ge\xe4u\xdfert.
Rakfisk wird als etwas Wichtiges angesehen - als ein essentieller, wenn auch streng riechender Teil der norwegischen Geschichte.
Ich stehe im Schnee und stelle mich f\xfcr ein anderes Gericht an - von Rakfisk habe ich genug.
Am Samstag wird Mexikos neuer Pr\xe4sident Enrique Pena Nieto die Pr\xe4sidentenbinde erhalten und die F\xfchrung der Nation \xfcbernehmen.
"Als ich bei ihr zuhause ankam, schien es, als sei ihr K\xf6rper gewaschen worden", erinnert sich Senora Buendia.
Manning hatte ausgesagt, er habe w\xe4hrend dieser Z\xe4hlung nie die Gelegenheit gehabt, sich mit seiner Decke zu umh\xfcllen.
In dieser Nacht, so sagte Manning aus, seien seine Unterhose, Flip-Flops und Brille aus seiner Zelle entfernt worden.
Die Fortsetzung der Anh\xf6rung ist f\xfcr dieses Wochenende angesetzt. Von der Staatsanwaltschaft wird eine Rechtfertigung der Haftbedingungen erwartet.
Ich spreche Spanisch, zumindest gut genug, um mich in dieser Sprache an beiden Enden eines Interviews zu behaupten.
Aber ich verf\xfcge nicht \xfcber das Vokabular eines Muttersprachlers, und meinen amerikanischen Akzent werde ich ebenfalls nicht los.
Und Pena Nieto schwor, den Krieg Mexikos gegen die Drogenkartelle fortzuf\xfchren, auch wenn er diesbez\xfcglich keine Einzelheiten nannte.
Und in den meisten F\xe4llen entsprach diese Person einem Profil - dunkelh\xe4utig, ungebildet, aus einem armen Dorf, usw.
Sie wollen mexikanische Amerikaner als provisorische "Botschafter" f\xfcr Mexiko einsetzen, die ihre Interessen in den Vereinigten Staaten vertreten.
Ein Krieg mit der \xf6rtlichen Supermacht wird den neuen arabischen Regierungen kaum bei der Instandsetzung ihrer Wirtschaft helfen.
So hie\xdf es, mit den Gesetzen w\xfcrde der Schwarzmarkthandel beg\xfcnstigt, was zu billigeren und leichter zug\xe4nglichen Zigaretten f\xfchre.
Die australische Regierung hat Internetwerbung durch \xf6rtliche Unternehmen und Seiten verboten, besitzt jedoch keinen Einfluss auf internationale Seiten.
Bezirksstaatsanwalt Pete Hautzinger unterst\xfctzte diese Entscheidung, entschloss sich aber auch dazu, nicht alle ausstehenden Besitzverfahren fallen zu lassen.
"Ich glaube nicht, dass ich meine Zeit damit verschwende, das Recht durchzusetzen, bis es sich \xe4ndert", sagt er.
An diesem Abend sa\xdf ich im College allein beim Abendessen, als mich jemand leicht auf die Schulter tippte.
Ich kaufte mir mein erstes Valentino-Kleid f\xfcr ein Fest im Schloss meines Vetters, dem Prinz Edouard de Ligne.
Ich bin ein patriotischer Ehemann, Du bist meine patriotische Ehefrau: Erf\xfcllen wir unsere B\xfcrgerpflicht und schaffen wir Leben!
Jedes Jahr gibt sie 1.300 US-Dollar f\xfcr politische Ma\xdfnahmen aus, um die B\xfcrger anzuregen, mehr Kinder zu bekommen.
El Peri\xf3dico interviewte f\xfcnf Jugendliche im Alter zwischen 10 und 15 Jahren, die h\xe4ufig im Netz unterwegs sind.
In diesem Sinne verteidigte er das Projekt, eine s\xfcdamerikanische Staatsb\xfcrgerschaft zu schaffen, die die Mitgliederstaaten der Unasur vorantreiben.
Die, die lehren, verpflichten sich nie zu etwas, und im Gegenzug dazu unterzeichnen wir die S\xfcdamerikaner immer alles.
Correa nahm auch auf die Behandlung der gesundheitlichen Probleme des Pr\xe4sidenten von Venezuela, Hugo Ch\xe1vez, in Kuba Bezug.
Die W\xe4nde seines Hauses sind fast alle mit Fotos und Erinnerungen seiner langen Karriere dekoriert und bezeugen sie.
Und dann verabschiedete ich mich mit einer Meisterschaft 1981, dem Jahr des Deb\xfcts von Jerome Mincy bei BSN.
Zu dieser Zeit zog er es vor, seine Vollstreckungen und die von Mincy in der Nationalmannschaft zu genie\xdfen.
Sie geh\xf6rt zu den Besten, wie auch jene, die bei der Olympiade 2004 gegen das Dream Team gewann.
Die Familie von Larry und seine engsten Freunde waren mit ihm in Dallas f\xfcr die Feiern des Erntedankfestes.
Im Gegensatz zu Kanada sind die US-Bundesstaaten f\xfcr die Durchf\xfchrung der Wahlen in den einzelnen Staaten verantwortlich.
Man schl\xe4gt ihnen eine aktive \xdcberwachung vor und bietet ihnen bei Fortschreiten der Krankheit eine Behandlung an.
Man bestimmt mit zunehmender Genauigkeit die Kriterien f\xfcr eine Entscheidung, wer behandelt werden sollte und wer nicht.
W\xe4hrend eine Studie die Verringerung des Risikos von Prostatakrebs herausgefunden hat, zeigte eine andere eher eine Erh\xf6hung.
Mit ihrem Ausschuss f\xfcr "Sterben in W\xfcrde" hat Quebec vor kurzem die heikle Frage des Lebensendes diskutiert.
Am Tisch vor einem leckeren Mittagessen sitzend, willigt er resigniert ein, sich beim Essen helfen zu lassen.
"Mein gr\xf6\xdfter Wunsch ist es, dass man meinen Durchfall heilt, da dies dem\xfctigend ist", teilt er mit.
Denn nach Ansicht mehrerer Personen, die in der Palliativpflege arbeiten, finden gro\xdfe Ereignisse inmitten dieser R\xfcckschritte statt.
Sie erwartet in den n\xe4chsten Tagen trotzdem noch einen letzten Besuch ihres Sohns, der aus Italien kommt.
Im Heim Victor-Gadbois bietet man mit einer Gruppe von Freiwilligen K\xf6rperpflege und Hilfestellung bei der Nahrungsaufnahme an.
Hier wird das Leben unter bestm\xf6glichen Bedingungen fortgesetzt, erkl\xe4rt Dr. Christiane Martel, eine der \xc4rztinnen des Heims.
Eine "Industrie", die f\xfcr den Steuerzahler Quebecs sehr teuer war, insbesondere in den 1990er und 2000er Jahren.
Dies f\xfchrt dazu, dass ein Spieler wie ich, die Stirn bieten muss und sein Bestes geben will.
Um ein gro\xdfer europ\xe4ischer Verein zu werden, muss Paris Titel gewinnen und sich langfristig einen Namen machen.
Lyon und Marseille, die in der letzten Saison nicht gut waren, wurden von diesem neuen PSG "geboostet".
Thiago Silva, der weltweit einer der besten Verteidiger ist, erm\xf6glicht es allen Anderen ebenfalls, Fortschritte zu machen.
Eine Reihe der mit dieser Transaktion in Zusammenhang stehenden Daten wird elektronisch durch ein doppeltes Verschl\xfcsselungssystem signiert.
Die Computer "nehmen" die neue Transaktion und f\xfcgen ihr eine Zahl hinzu, bevor das Ganze "zerhackt" wird.
Das Ziel ist es, diejenige Zahl zu finden, die einen besonderen Fingerabdruck (viele Nullen am Anfang) ergibt.
"Es wird einige Zeit dauern, bis sich Bitcoin durchsetzt, aber 2013 k\xf6nnte ein Wendepunkt sein", prognostiziert er.
Damals war Kabul leer und das Land aufgrund der K\xe4mpfe der verschiedenen aufr\xfchrerischen Gruppen vom Krieg \xfcberzogen.
W\xe4hrend sich der \xe4gyptische Pr\xe4sident gestern Abend im Fernsehen \xe4u\xdfern musste, sind Demonstrationen f\xfcr heute Nachmittag geplant.
Von Freitagabend bis zum Sonnenuntergang am Samstag sind M\xe4rkte und Gesch\xe4fte geschlossen, und der \xf6ffentliche Verkehr ruht.
Die meisten Abenteurer und Erholungssuchenden kamen aus Russland, Frankreich, Deutschland, Italien, England, den USA und der Ukraine.
Ihr einziges Ziel ist es, Geld f\xfcr den Unterhalt der in der Heimat verbliebenen Familien zu verdienen.
Jedoch sollen die Tests mit der Zeit laut F\xf6deraler Migrationsbeh\xf6rde k\xfcnftig f\xfcr alle Gastarbeiter zur Pflicht werden.
Die Initiative zur Einf\xfchrung der Tests wurde von den Abgeordneten der Staatsduma und der F\xf6deralen Migrationsbeh\xf6rde unterst\xfctzt.
Einige gef\xe4lschte Zertifikate, die die Absolvierung des Sprachtests bescheinigen, wurden schon von Mitarbeitern der F\xf6deralen Migrationsbeh\xf6rde beschlaggenommen.
Nicht alle sind damit zufrieden, dass die russischen Beh\xf6rden die Probleme durch "Anziehung der Schrauben" bek\xe4mpfen wollen.
Walmart verkauft alle Produkte, von Windeln \xfcber Jagdgewehre und Autobatterien bis hin zu Staubsaugern, Eiern und Milch.
Die Ware in den Walmart-Filialen ist im Schnitt zwischen 8 und 27% g\xfcnstiger als in gro\xdfen Superm\xe4rkten.
Ein typischer Walmart-Mitarbeiter, der 9,5 US-Dollar die Stunde verdient, k\xf6nne sich diese Erh\xf6hung nicht leisten, sagten sie.
Laut New York Times war dies die gr\xf6\xdfte Aktion ihrer Art in der Geschichte der US-amerikanischen Fast-Food-Industrie.
Wir versuchen das zu ver\xe4ndern, arbeiten an echten dreidimensionalen Darstellungssystemen auf der Grundlage verschiedener Technologien, darunter Projektionen.
- Wenn ich mich recht erinnere, pr\xe4sentierte Microsoft im Gegensatz zu Google seine Brille nicht der \xd6ffentlichkeit.
Ich habe die Farbe Rot als Modedesigner gew\xe4hlt, der sich mit der Optik und dem Image auseinandersetzt.
Wir gaben ihnen Trachtenberg, und es begann seine gro\xdfe Karriere, aber die Grundlagen lernte er bei uns.
Jetzt achtet jeder auf die Kleidung und orientiert sich am \xc4u\xdferen und nicht am Inneren des Menschen.
Fr\xfcher bildeten die Menschen gro\xdfe Gruppen: Die Bohemiens liebten das Eine und das einfache Volk das Andere.
Ich habe Anh\xe4nger, und das Wichtigste ist, sie nicht zu betr\xfcgen und das Erreichte nicht zu zerst\xf6ren.
- Petersburg ist nicht die Kulturhauptstadt; in Moskau gibt es viel mehr Kultur und einen entsprechenden N\xe4hrboden.
Die vierte Generation der im Orbit gez\xfcchteten Erbsen unterschied sich nicht im geringsten von den irdischen Arten.
Ein neugeborenes Kind kann im Orbit nicht wie ein Erwachsener zum Training in einen Belastungsanzug gesteckt werden.
Im Gespr\xe4ch f\xfcr Aktu\xe1ln \u2047 .cz sagt dies der Vizepr\xe4sident des H\xf6chsten Kontrollamtes (Nejvy \u2047 \xed kontroln\xed  \u2047 ad, NK \u2047 ), Miloslav Kala.
Es handelt sich dabei um eine parallele Pr\xfcfung, mit der wir vor etwa zwei Jahren begonnen haben.
Es kann jedoch das Problem auftreten, dass die Regeln "strenger" werden und nicht mehr eingehalten werden k\xf6nnen.
Dazu ist aber noch anzumerken, dass eine Verbesserung der Situation auch immer abh\xe4ngt vom Bem\xfchen der Betroffenen.
Es gibt nur wenige wirklich einzigartige Dinge, und ich wage zu behaupten, dass Tap Tap dazu geh\xf6rt.
Der Eintritt kostet 400 CZK, Kinder bis 12 Jahren kostenlos, Karten sind im Vorverkauf bei Bohemiaticket erh\xe4ltlich.
Nachfolgerin der ersten Raketen des Typs RM wurde die in den Jahren 1962 bis 1965 entwickelte Meteor-1-Rakete.
Die Rakete war als Zweistufenrakete konzipiert, ihre Gesamtl\xe4nge betrug 510 cm und das Startgewicht war 32,5 kg.
Dies geschieht zum einen durch \xf6konomischen Zwang bei langfristiger Arbeitslosigkeit, zum anderen durch die Beschneidung der Arbeitnehmerrechte.
Das Privatkapital beharrt engstirnig auf seinem Standpunkt, dass der Staat nicht lenkend in die Wirtschaft eingreifen darf.
Wir werden bei der EU R\xfcckerstattung beantragen", erkl\xe4rte im Herbst 2004 der damalige Landwirtschaftsminister Jaroslav Palas ( \u2047 SSD).
Wenn Sie in einer Firma einen Businessplan aufstellen, dann haben Sie auch ein Idealziel und eine Vision.
Ich sage ganz klar, dass ich ein Amateur bin; ich bin weder ein Genie noch ein Intellektueller.
Ich habe noch nicht mal Geld f\xfcr die Pr\xe4sidentenkampagne; auf meinem transparenten Konto sind lediglich 20.000 CZK.
Sie sagen, dass Sie die Republik ver\xe4ndern wollen, aber Ihr eigenes Geld m\xf6chten Sie nicht darin investieren.
Die Tatsache, dass ich keine Sponsoren habe, zeigt, dass mein Programm wohl nicht allzu viel Interesse weckt.
Wir haben die klassische Raumkonfiguration auf den Kopf gestellt und den Lesebereich von innen nach au\xdfen gest\xfclpt.
Das Innere des B\xfccherbergs ist geschickt genutzt: In der Mitte liegen B\xfcros, Internet-Bibliothek, Schachclub, Umweltzentrum und Haustechnikzentrale.
Aber ich w\xfcrde dem auch nicht zu viel Gewicht beimessen wollen, das ist keine v\xf6llig einseitige Beziehung.
Ich glaube, dass die Regierung unter Obama insgeheim wohl ziemlich viel Verst\xe4ndnis f\xfcr die europ\xe4ische Position hat.
Ich glaube, in Zukunft wird Deutschland eine f\xfchrende Rolle \xfcbernehmen, Europa zu einer europ\xe4ischen Position zu dr\xe4ngen.
Wentzler ist zuversichtlich, die Sache zu einem guten Abschluss zu bringen, und lobt die Professionalit\xe4t der Gerichte.
Aber er sagt auch: "Das Verfahren ist extrem aufwendig und kostet uns viel Zeit, Geld und Nerven."
Etwa 2000 Menschen leben dort, manche noch in einfachen Lehm- und Strohh\xfctten, ein Gro\xdfteil davon sind Kinder.
In Esitjeni zeigt sich im Kleinen, woran ganz Swasiland krankt: h\xf6chste HIV-Infektionsrate, niedrigste Lebenserwartung weltweit laut Unicef.
Denn zum Teil k\xf6nnen Erreger von sexuell \xfcbertragbaren Krankheiten auch durch Schmierinfektionen und engen K\xf6rperkontakt weitergegeben werden.
Die von der Europ\xe4ischen S\xfcdsternwarte ver\xf6ffentlichte Aufnahme zeigt den mehrere tausend Lichtjahre entfernten Trifid-Nebel im Sternbild Sch\xfctze.
In dieser hell strahlenden Galaxie mit einem kleinen Schwarzen Loch existiert noch kein Staub, sondern nur Gas.
Es l\xe4sst Blicke ins All gleich \xfcber zwei Spiegel zu, jeder mit einem Durchmesser von 8,4 Metern.
Bei der "Search for Extraterrestrial Intelligence" (SETI) kann jeder Computerbesitzer mithelfen, indem er Rechenleistung zur Verf\xfcgung stellt.
Bis 2007 galten die beiden Keck-Teleskope auf dem hawaiianischen Vulkan Mauna Kea als die gr\xf6\xdften der Welt.
Seit M\xe4rz 2009 sucht das Weltraumteleskop Kepler nach extrasolaren Planeten - vornehmlich nach solchen, die bewohnbar sind.
Der Kleinbus rumpelt \xfcber die kurvenreiche Stra\xdfe, vorbei an dicht bewaldeten H\xfcgeln, rei\xdfenden Fl\xfcssen und einfachen Bauernh\xe4usern.
Doch umstrittener Star des Museums ist der Schafhirte  \u2047 irali M\xfcsl\xfcmov, der 168 Jahre alt geworden sein soll.
Und angesichts des \xe4ltesten dokumentierten Menschen, der 122 Jahre alt wurde, erscheint M\xfcsl\xfcmovs Alter doch \xe4u\xdferst zweifelhaft.
Fakt ist aber, dass die Menschen der Region rund um Lerik auffallend h\xe4ufig ein biblisches Alter erreichen.
Und vielleicht hat ja auch Mirzayevas l\xe4ngst ergrauter Sohn recht: "Die Alten genie\xdfen in unserer Kultur Hochachtung."
Friedensnobelpreistr\xe4ger und Ex-Chef der Internationalen Atomenergiebeh\xf6rde Mohamed El-Baradei erkl\xe4rte, der Verfassungsentwurf geh\xf6re "auf den M\xfcllberg der Geschichte".
K\xf6nnte das Erfolgsgeheimnis des Landes etwas mit dem \xf6rtlichen Appetit auf ziemlich \xfcbelriechenden Fisch zu tun haben?
Norwegen schafft es nicht oft in die Weltpresse, und die meisten Leute scheint das nicht zu st\xf6ren.
"Solange wir im Winter Ski fahren und im Sommer wandern gehen k\xf6nnen, sind wir gl\xfccklich", sagt Anna.
Es gibt eine Live-TV-Schaltung zu einem mit Fliege bekleideten Showmaster, der von Tellern mit Rakfisk umgeben ist.
Bevor er mit dem US-Pr\xe4sidenten auf Augenh\xf6he ging, war Pena Nieto als Gouverneur seines Heimatstaats Mexiko t\xe4tig.
Plaketten mit seinem Namen h\xe4ngen auch au\xdferhalb eines modernen Sportzentrums und eines eindrucksvollen interaktiven Museums zum Klimawandel.
Aber auf der anderen Seite des Staats teilen nicht viele Menschen diese Ansicht \xfcber ihren fr\xfcheren Gouverneur.
Der Ort liegt versteckt unter Autobahn\xfcberf\xfchrungen und stellt in vielerlei Hinsicht eine Vorstadt von Mexiko-Stadt selbst dar.
Er sagte, in Kuwait habe er den Selbstmord erwogen und sei aufgrund der Hitze einmal bewusstlos geworden.
Mexikaner tendieren dazu, die Auswanderer zu beschuldigen - sie rufen ihnen schwere Zeiten ins Ged\xe4chtnis, sagt er
Im Gegensatz dazu ist die Bruderschaft mit der Hamas verschw\xe4gert und ihre Anf\xfchrer st\xe4rker von Volksansichten abh\xe4ngig.
Blutige Missionen zur Zur\xfcckdr\xe4ngung der Hamas im Gaza-Streifen werden \xfcber die Jahre zunehmend ihren diplomatischen Tribut fordern.
Damit w\xe4re mehr f\xfcr die Schaffung eines pal\xe4stinensischen Staates getan als mit dem bevorstehenden Antrag auf UN-Beobachterstatus.
Die australische Bundesregierung will junge Menschen vom Rauchen abbringen, indem das glamour\xf6se Bild des Tabakkonsums beseitigt wird.
Ehrlich gesagt gibt es nur einen Grund, warum ich aufh\xf6ren w\xfcrde, und das ist mein kleines M\xe4dchen.
Langeweile unterscheidet sich von Apathie demzufolge dahingehend, dass die Person nicht besch\xe4ftigt ist, dies aber sein m\xf6chte.
Uns allen wird irgendwann einmal langweilig - mein versp\xe4teter Flug, ein dr\xf6hnender Lautsprecher, ein besonders erm\xfcdender Film.
Er glaubt, dass die Menschen in Wahrheit nur nach einem Weg suchen, abzuschalten und sich zu entspannen.
Die Reaktionen sind selbst an Orten wie dem l\xe4ndlichen Mesa County, wo W\xe4hler die Marihuana-Initiative ablehnten, zwiesp\xe4ltig.
Letzte Woche beschloss Montrose, eine Stadt im Westen, ein sechsmonatiges Verbot, das vermutlich n\xe4chste Woche verabschiedet wird.
Sie fordern einen Platz im Gleichberechtigungskomitee ihres College, um sicherzustellen, dass ihre Meinungen frei ge\xe4u\xdfert werden k\xf6nnen.
"Dies stellt eine Gefahr f\xfcr den intellektuellen Diskurs und f\xfcr das Wohlbefinden der Mitglieder dar", sagt sie.
Ich f\xfchlte mich so, wie sich Homosexuelle vor der liberaleren Gesetzgebung der Vereinigten Staaten gef\xfchlt haben mussten.
Er hasste den Ort, fand ihn provinziell und kleinkariert und lehnte ihn f\xfcr seine marxistisch-deterministische Geschichtsperspektive ab.
Es war eine Hose, ein Hemd, eine Weste Typ "Gillette" und eine Jacke aus der Herbst/Winter-Kollektion 1971-1972.
Ich habe ihn das letzte Mal vor einem Monat bei einem Gala-Abendessen im Museum de Orsay gesehen.
Es gibt Menschen, f\xfcr die ihre Arbeit die H\xf6lle ist, und andere arbeiten wortw\xf6rtlich in der H\xf6lle.
Anto hat Asthma, atmet mit Schwierigkeit, hustet h\xe4ufig und seine Augen sind wegen der giftigen Gase gereizt.
Ich werde nicht in Rente gehen, ich werde hier sterben, weil der Vulkan mein ganzes Leben war.
"Das sind sehr vertrauliche Geheimnisse, meine Mutter darf sie kennen, aber nicht die ganze Welt", best\xe4tigt er.
Nach Angabe des Jungen hat ihm niemand Andeutungen gemacht oder ihn nach seiner Adresse oder Telefonnummer gefragt.
"Wir sind die digitalen Einwanderer, die sie lehren sollen, wo wir doch selbst noch lernen" sagt er.
Correa erkl\xe4rte, dass die Gefahr best\xfcnde, dass die Gesundheit und der psychische Zustand von Assange beeintr\xe4chtigt w\xfcrde.
Diese Mittel wurden f\xfcr den Erwerb von Aktien der Administradora Profesional de Hoteles (der professionellen Hotelverwaltung) eingesetzt.
Bartow empfahl danach den Freiwurfspezialisten Raymond Gausse, der sich einb\xfcrgern lie\xdf und einer unserer besten Werfer war.
Ich wei\xdf noch, als wir zum ersten Mal beim vorolympischen Turnier in Mexiko gegen die USA gewannen.
Wir hatten eine Reihe guter Trainer wie Julio Toro, Flor Mel\xe9ndez, Carlos Morales, Raymond Dalmau, Armandito Torres.
"Er war eine originelle Person und lebte das Leben in vollen Z\xfcgen", erkl\xe4rte Gray in einer Mitteilung.
Hagman wurde 1992 Leberzirrhose diagnostiziert, und er gab zu, dass er \xfcber Jahre hinweg viel getrunken habe.
In Temple gibt der beisitzende Professor Barry Vacker den Kurs "Medien, Kultur und das Ende der Welt."
"Ich habe versucht, die Studenten dar\xfcber zu informieren, was m\xf6glich, wahrscheinlich, glaubhaft und unm\xf6glich ist", sagte Vacker.
Der Oberste Gerichtshof der Vereinigten Staaten best\xe4tigte im Jahr 2008 die Verfassungsm\xe4\xdfigkeit des Gesetzes von Indiana.
Von den neuen Einschr\xe4nkungen sind junge Menschen, Minderheiten und Menschen mit niedrigem Einkommen unverh\xe4ltnism\xe4\xdfig stark betroffen.
Denn es liegt auf der Hand, dass zwei von drei hispanischen W\xe4hlern, die demokratische Partei bevorzugen.
Letztere machte nur 11% der W\xe4hler aus, aber 24% der B\xfcrger, die im Voraus gew\xe4hlt haben.
Beispielsweise hat wiederum Willard Boyle 1969 w\xe4hrend seiner Arbeiten in der Optik einen kleinen Lichtsensor entwickelt.
Gestern Abend haben wir Herrn X ein Bier serviert, der im Laufe der Nacht gestorben ist.
53% der ins Heim Victor-Gadbois eingewiesenen Patienten kommen von ihrer Wohnst\xe4tte, 47% kommen aus dem Krankenhaus.
Der "Duchesneau-Bericht" etablierte eine direkte Verbindung zwischen Industrie, geheimer Finanzierung von Parteien und Bestechung von Beamten.
Er gestand ebenfalls, eine illegale Mittelbeschaffung f\xfcr die ehemalige liberale Vizepr\xe4sidentin Nathalie Normandeau organisiert zu haben.
Infolge dieser Enth\xfcllungen ist Herr Tremblay Anfang November zur\xfcckgetreten, was Montreal in eine schwere Krise st\xfcrzte.
Man kann ihn durch eine pers\xf6nliche Einsicht, aber auch durch die neue Dimension des PSG erkl\xe4ren.
Welche Meinung haben Sie zu den ersten Monaten von Didier Deschamps an der Spitze der "Bleus"?
Vor diesem Zusammentreffen in Spanien habe ich noch nie ein vergleichbares Spiel in meiner Karriere erlebt.
Jede Transaktion zwischen zwei Benutzern findet in Wirklichkeit zwischen zwei E-Mail-Adressen in Form einer E-Mail statt.
Wenn diese Zahl gefunden wurde, k\xf6nnen die anderen Knoten m\xfchelos pr\xfcfen, ob es die richtige ist.
Allerdings ist sein Land seit den 50er Jahren und bereits lange zuvor von ausl\xe4ndischer Hilfe abh\xe4ngig.
Industrien wurden nicht wieder aufgebaut, funktionsf\xe4hige Stauwerke sind nicht vorhanden und wichtige Bew\xe4sserungssystems wurden nicht repariert.
In der Botschaft sind Dutzende schriftliche Anfragen kleiner landwirtschaftlicher Vorhaben von Gemeinden der Provinz Kapisa eingegangen.
85 gr\xf6\xdftenteils islamistische Mitglieder dieser verfassungsgebenden Versammlung haben den Text gestern in einer seltsamen Atmosph\xe4re verabschiedet.
Letztere teilen ebenfalls ihre Bef\xfcrchtungen in Bezug auf den Text mit, den sie als freiheitsbedrohend ansehen.
In Israel erwarten ukrainische Touristen heilige St\xe4tten, den Nabel der Welt und ein Meer aus Sole
Das Gelobte Land vereint in sich die Herrlichkeit biblischer Wahrheiten, modernen Komfort und eine unber\xfchrte Natur.
Hier befindet sich nach christlicher Auffassung der Nabel der Welt, der die Errettung der Menschheit symbolisiert.
Sein t\xfcrkisblaues Wasser hat einen hohen Salzgehalt und tr\xe4gt dadurch sogar Nichtschwimmer problemlos auf der Oberfl\xe4che.
In Jaffa k\xf6nnen Sie neuverm\xe4hlte Paare aus ganz Israel und sogar anderen L\xe4ndern bei Fototerminen antreffen.
"Die Waffen wurden sowohl von den russischen Offizieren als auch den Kaukasiern selbst gestohlen", sagt Baranez.
Der \xfcberwiegende Teil der illegalen Waffen stammt den Ermittlern zufolge von der Armee und den Rechtsschutzbeh\xf6rden.
Er liefert mir die Schlagringe ebenfalls nur deshalb, weil er wei\xdf, dass ich ihn nicht verpfeife.
Internetsuchmaschinen zeigen Suchergebnisse zu Webseiten und Gruppen in "Vkontakte", wo Waffen "f\xfcr verschiedene Zwecke" angeboten werden.
Beim Kauf illegaler Schusswaffen ist Experten zufolge mit Preisen von 100 bis 900 US-Dollar zu rechnen.
Dazu ist es aber erforderlich, dass nicht nur der Benutzer, sondern auch seine Umgebung erkannt wird.
- Welche Anspr\xfcche stellen Sie ausgehend von Ihrer Arbeit mit den Xbox Kinect-Sensoren an moderne Kameras?
Doch die Hauptsache sind nicht die Megapixel selbst, sondern die Qualit\xe4t der Matrix und der Tiefe.
Es gibt ein Problem, auf das Kritiker dieser Idee h\xe4ufig hinweisen: Es gibt keine f\xfchlbare Reaktion!
Es denken lassen, dass es das sp\xfcrt, was es sp\xfcren sollte, wenn es gerade etwas sieht?
Bisher l\xe4sst sich das Gehirn nur m\xe4\xdfig \xfcberlisten, und vor uns liegen noch viele arbeitsreiche Jahre.
Kirill Miller ist eine leuchtende Pers\xf6nlichkeit der Petersburger Avantgarde Ende der 80er bzw. Anfang der 90er.
In der Gesellschaft ruft alles, was etwas von der Graunorm abweicht, Aggressionen und schlechtes Verhalten hervor.
Retten wir zum Beispiel die Welt, indem wir vorschreiben, dass sich jeder vollst\xe4ndig zu verkleiden hat.
Aber vielleicht darf man einem Menschen nicht die Hand geben, sondern sollte ihm ins Gesicht spucken.
Leben w\xe4re nur in gro\xdfer H\xf6he oder in der Umlaufbahn der Venus, also im All, m\xf6glich.
Inwiefern kann Ihnen das Projekt eine Hilfe sein? Was ergibt sich f\xfcr Sie aus diesem Projekt?
Sehen Sie die Verabschiedung dieses Gesetzes eher positiv, oder wird das System mit weiterer B\xfcrokratie belastet?
Die Schnellstra\xdfe R6 und die Verkehrswege der ersten Stra\xdfenklasse in der Region sind derzeit uneingeschr\xe4nkt befahrbar.
Aufmerksamkeit ist jedoch beispielsweise auf Br\xfccken geboten, auf denen die Fahrbahnen mitunter vereist und glatt sind.
Die Stra\xdfenmeistereien warnen Fahrer vor Eisgl\xe4tte, die insbesondere in h\xf6heren Lagen im Bezirk Pardubice auftreten kann.
Eine ausgefahrene Schneeschicht liegt in H\xf6henlagen auf den Stra\xdfen der Kreise Rychnov nad Kn \u2047 nou und Trutnov.
\xd6rtlich ist au\xdferdem mit Nebel zu rechnen, wobei sich die Sicht jedoch im Tagesverlauf verbessern wird.
Mit Schneematsch m\xfcssen heute Fahrer rechnen, die in Richtung der H\xf6henlagen im Bezirk Olomouc unterwegs sind.
Urspr\xfcnglich wohl von mir, anschlie\xdfend haben wir die Idee gemeinsam mit unserem Grafiker Honza Augusta ausgestaltet.
Schon heute ist die Hymne auf YouTube sehr beliebt. Wird sie auch auf den Benefizkonzerten erklingen?
Dr. Jan Gadomski (1899 - 1966) wurde sp\xe4ter ein wichtiger Verfechter der Astronomie und der Raumfahrt.
In polnischen Zeitschriften ver\xf6ffentlichte er Hunderte von Artikeln und schrieb mehrere B\xfccher zu diesen wissenschaftlichen Disziplinen.
Bereits im Jahr 1925 wurde in Polen eine Eisenbahn-Draisine gebaut, f\xfcr die ein Raketenantrieb geplant war.
Aus den \xfcberlieferten Dokumenten ist ersichtlich, dass die Forschung bis ins Stadium praktischer Tests vorgedrungen war.
Auf der anderen Seite die lockeren Passagen aus Hollywood, die ironisch und leicht \xfcberspitzt daher kommen.
Die Bezeichnung Rum darf nur f\xfcr Produkte aus Zuckerrohrdestillat verwendet werden, nicht f\xfcr Produkte aus Zuckerr\xfcben.
"Die Leute wollen, dass ich die Republik rette, aber ich bin blo\xdf ein Amateur", behauptet Okamura.
Nehmen Sie nur einmal die direkte Wahl des Pr\xe4sidenten, die ein Verdienst des \xf6ffentlichen Drucks war.
Und Stefan Spermon, IT-Techniker in einem nahegelegenen Gro\xdfbetrieb, meint: "Doch, sch\xf6n ist es schon, das Haus."
Vor allem aber verf\xfcgt Spijkenisse nun \xfcber den ersten \xf6ffentlichen Kulturbau in der Geschichte seines Bestehens.
Stefan Spermon, der anf\xe4ngliche Skeptiker aus der IT-Branche, wagte bereits den Weg in die neue B\xfccherei.
Und auch die TCM-Lehrerin Cynthia Bogarde, die den Boekenberg gar als Spijkenisses "l\xe4ngst \xfcberf\xe4llige Seele" bezeichnet.
"Ich denke, dank unserer Einladung hat nun jeder Bewohner eine gewisse Beziehung zu diesem neuen Haus.
Man erwartet von ihnen, dass sie eine unabh\xe4ngigere Rolle spielen, daran sind sie aber nicht gew\xf6hnt.
Haben diese Wirtschaftsinteressen Einfluss auf die Haltung im Nahostkonflikt und der Abstimmung in der UN gehabt?
Ich glaube, in Europa und sogar in den USA herrscht gro\xdfes Verst\xe4ndnis f\xfcr die deutsche Position.
Deshalb glaube ich nicht, dass dies ein so dramatischer Bruch war, wie in der libyschen Frage.
In den n\xe4chsten beiden Instanzen bekam Freudenberg zwar recht, doch der Prozessgegner k\xe4mpft bis heute weiter.
F\xfcr 180 Aidswaisen im Dorf Esitjeni hat der Verein Voices for Africa Paten in Deutschland gefunden.
Die Infektionskrankheiten k\xf6nnen Geschw\xfcre im Genitalbereich, Beschwerden beim Urinieren, Ausfluss, Unterbauchschmerzen sowie Bl\xe4schen oder Warzen hervorrufen.
Kostenlose Kondome g\xe4be es zwar an jeder Ecke, sagt Annette Lennartz, "aber die werden kaum benutzt.
Das Wasser kam vermutlich von Kometen oder m\xf6glicherweise auch Asteroiden, die auf dem Merkur eingeschlagen sind.
Im riesigen Trifid-Nebel, 5400 Lichtjahre von der Erde entfernt, entstehen aus Gas und Staub neue Sterne.
Der Spiegel des Southern African Large Telescope in S\xfcdafrika ist segmentiert - um Kosten zu sparen.
Diese reicht n\xe4mlich - trotz vergleichsweise geringem Spiegeldurchmesser - an die der weltweit gr\xf6\xdften Spiegelteleskope heran.
Mit Hilfe eines Radioteleskops in Arecibo (Puerto Rico) h\xf6ren Forscher das All nach au\xdferirdischen Signalen ab.
Sein Hauptspiegel soll satte 42 Meter umfassen - und aus knapp 1000 Spiegelelementen zusammen gesetzt werden.
Am 2. Februar 2011 wurde von der Nasa bekanntgegeben, dass 1235 Planetenkandidaten seit Missionsbeginn ermittelt wurden.
Das James Webb Space Telescope (JWST) wird fr\xfchestens 2018 an Bord einer Ariane5-Rakete ins All geschossen.
Aber auch Rembrandt Scholz, Altersforscher am Max-Planck-Institut in Rostock, hat von den Hochbetagten in Mittelasien geh\xf6rt.
Wegen fehlender Unterlagen sei jedoch kein wissenschaftlicher Nachweis \xfcber das Alter zu f\xfchren, zumal Personenstandsregister fehlten.
In der K\xfcche bereitet man den G\xe4sten Tee, der in den typischen, bauchf\xf6rmigen Armadu-Gl\xe4sern serviert wird.
Via Kurznachrichtendienst Twitter bezichtigte er die Anh\xe4nger Mursis, einen "Putsch gegen die Demokratie" f\xfchren zu wollen.
Und mehrere Richter k\xfcndigten an, das Referendum nicht \xfcberwachen zu wollen, wodurch es ung\xfcltig werden w\xfcrde.
Diese Ma\xdfnahmen sind eklatante Verst\xf6\xdfe gegen demokratische Spielregeln und werden \xc4gypten in eine neue Diktatur f\xfchren.
Ein Demonstrant auf dem Tahrir warnt: "Ihr geb\xe4hrt ein Monster, das ihr nicht mehr kontrollieren k\xf6nnt."
So ungef\xe4hr muss man sich den nasenbet\xe4ubenden Geruch von Rakfisk vorstellen, einer der gro\xdfen Delikatessen Norwegens.
Um uns herum verzehren Leute kleine Fischw\xfcrfel und nehmen dazu gro\xdfe Mengen an Alkohol zu sich.
Nach 81 Jahren an der Macht wurde die PRI im Jahre 2000 von Vicente Fox abgel\xf6st.
Wenn Pr\xe4sident Pena Nieto am Samstag die Pr\xe4sidentenbinde empf\xe4ngt, \xfcbernimmt er damit auch eine gro\xdfe Verantwortung.
Unsere Identit\xe4t ist manchmal wom\xf6glich verschwommen, aber was unsere Loyalit\xe4t anbetrifft, ist dies nicht der Fall.
Der Waffenstillstand zwischen Israel und der Hamas k\xf6nnte sich als unerwarteter Grundpfeiler f\xfcr den Frieden erweisen
Tats\xe4chlich gewinnt die Hamas im Westjordanland hinzu, das von der rivalisierenden, gem\xe4\xdfigten Pal\xe4stinensergruppe Fatah kontrolliert wird.
Das israelische Raketenabwehrsystem, "Iron Dome", hat sich bew\xe4hren k\xf6nnen und viele der Hamas-Raketen sind zerst\xf6rt worden.
"Die Gesetze werden zu ernsthaften, unbeabsichtigten Konsequenzen f\xfchren", sagt Scott McIntyre von British American Tobacco Australia.
Mittlerweile wurden diese auf mehr als 40 L\xe4nder ausgeweitet, darunter Brasilien, die T\xfcrkei und die Ukraine.
"Fr\xfcher habe ich eine Stunde gebraucht, um eine Lieferung einzusortieren, jetzt brauche ich vier", sagt Yu.
Damit wird das Gehirn gezwungen, sich in interessanten Gedankeng\xe4ngen zu verlieren, was wom\xf6glich die Kreativit\xe4t f\xf6rdert.
Manchmal glauben wir, dass uns langweilig ist, auch wenn wir blo\xdf Schwierigkeiten haben, uns zu konzentrieren.
Das Kind lernt nicht nur, sich zu unterhalten, sondern erh\xe4lt auch in anderen Bereichen mehr Selbstkontrolle.
Schon immer war es mein gr\xf6\xdfter Traum gewesen, einen Platz an der Universit\xe4t Oxford zu erhalten.
Nun, aktuellen Berichten zufolge leidet eine neue Generation von Studenten der gem\xe4\xdfigten Rechten unter \xe4hnlicher Verfolgung.
An anderen Universit\xe4ten sagen konservative Studenten, sie werden als "S\xfcndenb\xf6cke f\xfcr die Einf\xfchrung h\xf6herer Studiengeb\xfchren" betrachtet.
In den 60er und 70er Jahren wohnten die beiden in den Alpen und waren gute Freunde.
Ich mag die Farben, die er verwendet, sehr; sie haben viel Licht und unterstreichen das Gesicht.
"Mir ist immer sein Raffinement, seine Ruhe, sein gepflegtes und perfektes \xc4u\xdferes aufgefallen", gibt D'Arenberg zu.
Jorge versichert, 35 Freunde zu kennen, die er in FB hat und neun Folger in Twitter.
Im Unterschied zu Jorge w\xfcrde dieser Junge Fotos von Bekannten in unbequemen oder peinlichen Situationen hochladen.
Ja, das w\xfcrde ich tun, wenn er mir unsympathisch ist oder ich ihm eins auswischen will.
Hast du die anderen Personen vorher um Erlaubnis gefragt, wenn du Fotos von Feiern etikettiert hast?
Laut Guardia m\xfcssen die Kinder an die Lektion "Du sollst nicht mit Fremden sprechen" erinnert werden.
"M\xf6glicherweise werde ich mich am morgigen Tag (Samstag) mit dem Pr\xe4sidenten Daniel Ortega treffen", sagte Santos.
Die \xc4nderung war zur hin Verbesserung, ich ern\xe4hre mich gut, treibe Sport und nehme die Medikamente.
Die Emission ist die erste von vier gleichen Emissionen, die eine Zinszahlung alle 28 Tage versprechen.
Und das war der Anfang von Mincy, einem der besten Spieler, die Puerto Rico je hatte.
Und dies, ohne seine Laufbahn in den verschiedenen Ligen zu ber\xfccksichtigen, in denen er gespielt hat.
Aber es war seine meisterhafte Interpretierung des bezaubernd verabscheuungsw\xfcrdigen J.R., die Hagman zu einem Superstar machte.
Martin war noch eine Jugendliche, als sie Larry w\xe4hrend ihrer Ehe mit Rechtsanwalt Ben Hagman bekam.
Der 25-j\xe4hrige Student Will Wekesa f\xfcr Psychologie und Krankenpflege erkl\xe4rt, alle apokalyptischen Filme gesehen zu haben.
Die neuen Wahlgesetze verlangen, dass die W\xe4hler einen Lichtbildausweis und einen Nachweis der US-Staatsb\xfcrgerschaft vorlegen.
Vor den Wahlen von 2006 hat kein US-Staat von den W\xe4hlern verlangt, einen Lichtbildausweis vorzuzeigen.
Allerdings sind h\xe4ufig mehr als hundert Dollar zu zahlen, um den erforderlichen Ausweis zu erhalten.
Beispielsweise haben nur 16 der 34 Bundesstaaten Gesetze verabschiedet, die das Vorzeigen eines Lichtbildausweises verlangen.
Allerdings werden die neu eingef\xfchrten Regeln im Jahr 2012 zweifellos die Aus\xfcbung des Wahlrechts erschweren.
In zu gro\xdfer Menge erh\xf6ht es das Risiko, an einem Grimm- bzw. Mastdarmkrebs zu erkranken.
Die Konservierung von Fleisch durch R\xe4uchern, Trocknen oder Salzen kann zur Bildung von Karzinogenen f\xfchren.
Vor ein paar Wochen lebte Herr L. noch allein in seiner Wohnung in der Mont\xe9r\xe9gie.
Die Patienten, die in das Heim f\xfcr Palliativpflege Victor-Gadbois eingewiesen werden, leiden alle an Krebs.
F\xfcr Frau A., 89 Jahre, ist die schlimmste Bef\xfcrchtung, "bewusst und durch Erstickung" zu sterben.
Ich bef\xfcrchte, dass die Patienten nur deshalb sterben wollen, weil sie keine angemessene Gesundheitsversorgung erhalten.
Und gleichzeitig behandeln mehrere Onkologen ihre Patienten trotz schlimmster Prognosen verbissen bis zum letzten Tag.
Die \xdcberlebenschancen von H\xe9l\xe8ne Richard waren bereits minimal, als sie eine beschwerliche Chemotherapie abgebrochen hat.
Es muss aber deutlich gesagt werden, dass die Palliativpflege bei der Schmerzbehandlung nicht omnipotent ist.
Wir k\xf6nnen nicht l\xe4nger so tun, als ob wir diese Seite des Leidens nicht wahrnehmen.
Er wird von Co-Trainern wie Claude Makelele unterst\xfctzt, der auf derselben Position spielte wie ich.
Er blickt auf eine reiche Erfahrung zur\xfcck und hat viele Titel mit angesehenen Vereinen gewonnen.
Das Vertrauen, das er in mich gesetzt hat, ist ebenfalls eine Erkl\xe4rung f\xfcr meine Leistungen.
Im Hinblick auf die investierten Summen glaubte man euch zur Spielpause mit 15 Punkten Vorsprung!
Deshalb ist er gekommen und er beweist, dass er der Star der Ligue 1 ist.
Mit Bitcoin sind alle Netzknoten gleichzeitig Verwahrer des Rechnungsbuchs, Pr\xfcfer, Geld-Emittenten sowie K\xe4ufer und Verk\xe4ufer.
Zur Erreichung der Beschlussf\xe4higkeit wurden gestern Morgen in aller Eile 11 Personen, stellvertretende Mitglieder, hinzugef\xfcgt.
Und in Zukunft k\xf6nnte die Frage aufgeworfen werden, inwieweit Zivilrichter kompetent sind, dar\xfcber zu entscheiden."
Ihrer Meinung nach ist der einzige positive Punkt das Verbot der Folter durch Artikel 36.
Sie liegen an einer Felswand in den Bergen in 450 Meter H\xf6he \xfcber dem Meeresspiegel.
Und es erklingen die Namen der j\xfcdischen Kinder und der L\xe4nder, in denen sie starben.
Das Tote Meer ist sogar noch w\xe4rmer und dort wird das ganze Jahr \xfcber gebadet.
Diese Geheimnisse birgt die Altstadt von Tel Aviv, n\xe4mlich die Stadt Jaffa an der Mittelmeerk\xfcste.
Durch diese Stadt verlief der ber\xfchmte Seeweg, der \xc4gypten, Syrien, Anatolien und Mesopotamien miteinander verband.
Vor allem, entgegnen Sprecher der Migrationsbeh\xf6rde, gehe es darum, die Zahl der Zwangsarbeiter zu verringern.
Haben Sie diesen Status nicht, so gibt es keine Pr\xfcfung und folglich keine offizielle Arbeit.
Viele Migranten best\xe4tigen, dass es nicht einfach ist, in Russland einen offiziellen Status zu erhalten.
Zurzeit kann man den Verfassern zufolge in Moskau jede m\xf6gliche Waffe f\xfcr wenig Geld finden.
Die Preise und das Warensortiment machten Walmart zu einem der gr\xf6\xdften Unternehmen in den USA.
Pro Jahr w\xe4ren das f\xfcr sie im Vergleich zu heute Mehrausgaben von nur 12,39 Dollars.
Derzeit liegt der Mindestlohn gem\xe4\xdf f\xf6deraler und New Yorker Gesetzgebung bei 7,25 Dollar die Stunde.
Wie es m\xf6glich ist, in New York mit so wenig Geld auszukommen, ist mir unbegreiflich.
Eigentlich ist jede Art von Interaktion mit Computern gut, allerdings jede in ihrer bestimmten Nische.
Noch ist es relativ gro\xdf, k\xf6nnte theoretisch jedoch auf die Gr\xf6\xdfe einer Armbanduhr verkleinert werden.
Wo immer die Bilder von Kirill Miller auch ausgestellt werden, locken sie gro\xdfe Menschenmassen an.
Mich zieht es zum Theater, zur Mode, zur Musik, eigentlich zu allem, au\xdfer der Literatur.
Auch die Galerie "D 137" oder der Klub "Griboedov" haben ihren Ursprung in der Art-Klinik.
Ich gewann in der Kategorie "K\xfcnstler des Jahres", und damit war ich am H\xf6hepunkt angelangt.
Karawanen von Raumschiffen mit Erdbewohnern an Bord machen sich auf die Suche nach einem Ersatzplaneten.
Die Frage der Fortpflanzung im All behandelten die Forscher zun\xe4chst im Hinblick auf die Flora.
Der Homo sapiens ist zu abstraktem Denken f\xe4hig und kann einen \xe4hnlichen emotionalen Hintergrund erzeugen.
Ohne die Erdanziehung zu f\xfchlen, kann der Organismus das Skelett und die Muskeln nicht ausbilden.
Zu einem \xe4hnlichen Ergebnis kommt anscheinend auch eine gemeinsame Kontrolle durch tschechische und deutsche Pr\xfcfer.
Als negatives Praxisbeispiel f\xfchrt er die Einstellung von Premierminister Petr Ne \u2047 as zum sog. "Schwarz-System" an.
Aber die Senkung von Schwellenwerten f\xfcr Auftr\xe4ge garantiert nicht, dass wir dieses Ziel auch erreichen.
Im Bezirk Karlsbad waren die Stra\xdfen heute Morgen gut befahrbar, vereinzelt herrschte Schnee- und Eisgl\xe4tte.
Dieses ist am Morgen frostig, mit Temperaturen zwischen 3 und 9 Grad unter dem Gefrierpunkt.
Selbstverst\xe4ndlich, und zwar ganz zum Schluss, vorausgesetzt, dass alles klappt und der Weltuntergang nicht stattfindet...
Die Sch\xfcler des Jedli \u2047 ka-Instituts werden regelm\xe4\xdfig von Lektoren betreut, die ihnen bei unterschiedlichen Freizeitaktivit\xe4ten helfen.
Es ist dort noch nicht einmal selbstverst\xe4ndlich, dass man einen Rollstuhlfahrer beispielsweise im Aufzug vorl\xe4sst.
Gl\xfccklicherweise entstehen auch dort Vereine, die versuchen, auf die Probleme von Menschen mit Behinderungen hinzuweisen.
Von Anfang an habe ich das Potential gesp\xfcrt, dass man die Dinge anders angehen kann.
Der erste Eindruck, den der Zuschauer meist hat, ist selbstverst\xe4ndlich Mitleid; das ist nur nat\xfcrlich...
So funktioniert es aber \xfcberall, in jeder Band, die ernsthaft arbeiten und etwas erreichen will.
Wir sind eine offene Gruppe. Die Leute kommen und gehen. Das kann man nicht verhindern.
Der Ausschuss wurde 1937 eingerichtet, nach zweij\xe4hriger T\xe4tigkeit wurde seine Arbeit jedoch vom Kriegsbeginn beendet.
Der Beweis daf\xfcr ist die Existenz einer praktisch allm\xe4chtigen und in allen Staaten allgegenw\xe4rtigen Lobby.
Die Geschichte der Menschheit ist in erster Linie eine Geschichte des Kampfes um die Macht.
Wer auch immer versucht hat, sich dieser Familie entgegenzustellen, musste mit dem Leben daf\xfcr zahlen.
Eine Welt, in der der Rest der menschlichen Population einer kleinen Gruppe von Finanzaristokraten dient.
Das Schicksal der Geiseln rief zu Hause eine Welle der Solidarit\xe4t sowie antiiranischer Stimmungen hervor.
Der vom Experten f\xfcr "Exfiltration", Tony Mendez, entwickelte Plan machte auch die Zusammenarbeit Hollywoods erforderlich.
Eine \xe4hnliche Einschr\xe4nkung gilt bereits f\xfcr Kinder bis 14 Jahren bei der Benutzung von Jahrmarktstr\xf6ten.
Tschechien \xfcberschritt dann z.B. das festgelegte Volumen f\xfcr Pilzkonserven, wof\xfcr uns eine hohe Geldstrafe drohte.
Herr Senator, wie kommt man auf die Idee, f\xfcr das Amt des Pr\xe4sidenten zu kandidieren?
Die Leute haben eine solche Senatszusammensetzung gew\xe4hlt, dass \xc4nderungen nur sehr schwer durchsetzbar sein werden.
Trotzdem werde ich f\xfcr meine Visionen k\xe4mpfen, z.B. f\xfcr die Direktwahl der B\xfcrgermeister und Bezirkshauptm\xe4nner.
Die Kosten f\xfcr die Kampagne werden im Grunde genommen durch mein Gehalt als Senator gedeckt.
Das ist er also, mein Vorschlag f\xfcr den B\xfccherberg von Spijkenisse, f\xfcr den sogenannten Boekenberg!
Anfang November wurde der B\xfccherberg mit dem zweiten Preis "Best Library of NL 2012" ausgezeichnet.
Eine besondere Freude sind die schwarzen B\xfccherregale, die mal Wandverkleidung, mal Br\xfcstung, mal Stiegengel\xe4nder sind.
Laut Stephen Szabo, Experte f\xfcr US-Europ\xe4ische Beziehungen, balanciert Berlin damit auf einem schmalen diplomatischen Grad.
Aber aufgrund der politischen Situation hier, kann die Regierung diese Position \xf6ffentlich nat\xfcrlich nicht vertreten.
Ich glaube, dass die tats\xe4chlichen Meinungsverschiedenheiten gar nicht so gro\xdf sind, wie sie immer erscheinen.
Aber ich glaube, dass den Deutschen klar ist, dass sie eine unabh\xe4ngigere Rolle spielen m\xfcssen.
Vor f\xfcnf Jahren bot Freudenberg der Gegenseite vergeblich einen "hohen sechsstelligen Eurobetrag" zur Beilegung an.
So wollte ein chinesischer Hersteller in Deutschland die Bezeichnung Freudenberg f\xfcr Schuhe und Leder anmelden.
Mehr als 300 von ihnen haben keine Eltern mehr, weil diese dem HI-Virus erlegen sind.
Nach europ\xe4ischen Erhebungen betreffen drei Viertel aller Infektionen junge Menschen zwischen 15 und 25 Jahren.
Im Dorf selbst verwaltet Zodwa Dlamini, eine selbstbewusste und durchsetzungsstarke Frau, die Gelder aus Deutschland.
Sie k\xfcmmert sich auch darum, dass die Waisen gut unterkommen, bei einer der Gro\xdfm\xfctter etwa.
Die Gogos, wie man die alten Frauen auf Zulu nennt, sind die St\xfctzen des Dorfes.
"Aids ist ein absolutes Tabu", sagt Annette Lennartz, "weil es mit Sexualit\xe4t zu tun hat."
Die Sonde Messenger hat Beweise daf\xfcr gefunden, dass es auf dem Planeten Merkur Eis gibt.
Der Plejaden-Sternhaufen, auch "Die sieben Schwestern" genannt, kann nachts mit dem blo\xdfen Auge gesehen werden.
Dieser Babystern konnte in seiner vollen Sch\xf6nheit erst durch die Infrarotdetektoren des Spitzer-Teleskops aufgenommen werden.
Saturn und seine Ringe: Wie diese entstanden sind, ist eines der gro\xdfen R\xe4tsel der Astronomie.
Diese Gruppe von Galaxien, Arp 273 genannt, nahm das Weltraumteleskop Hubble f\xfcr die Nasa auf.
Touristen aus Europa kommen kaum hierher, zu beschwerlich ist die Anfahrt von Aserbaidschans Hauptstadt Baku.
Sie hat immer nur das gegessen, was von ihrem eigenen Hof stammte, Tomaten, Kartoffeln, Erbsen.
Daf\xfcr verbietet ein anderer, den Propheten Mohammed und seine Gesandten zu beleidigen oder zu verleumden.
"Anstatt die Zivilgesellschaft zu st\xe4rken, setze der Pr\xe4sident sie de facto au\xdfer Kraft", beklagt Saeda.
Einwohner des Urlaubsorts schreiben ihm die Entwicklung des Tourismus und den Aufbau der Infrastruktur zu.
Er sei ein sehr direkter Mann, sehr engagiert und habe gro\xdfe Pl\xe4ne f\xfcr das Land.
Er sei ein hervorragender Staatsmann, vor allem sei er aber auch jemand, der zuh\xf6ren kann.
"Aber das ist nicht m\xf6glich, wenn es so viele Formfehler und Vers\xe4umnisse gab", sagt sie.
Nicht wissen zu d\xfcrfen, was mit ihm oder in der Au\xdfenwelt geschehe, sei belastend gewesen.
Dar\xfcber hinaus sind wir uns bewusst, dass uns viele Mitglieder der mexikanischen F\xfchrungsschicht nicht m\xf6gen.
Doch es gibt Gr\xfcnde zur Annahme, dass die t\xf6dliche Pattsituation endlich ihr Ende finden k\xf6nnte.
Und die Hamas-F\xfchrer k\xf6nnten zum Schluss kommen, dass sie die Zeit auf ihrer Seite haben.
Chinesische und indonesische F\xe4lscher werden weitaus gr\xf6\xdfere Mengen dieser Produkte auf den Stra\xdfen Australiens anbieten.
Die Hausw\xe4nde Pompejis ziert ein lateinisches Graffiti \xfcber Langeweile, das auf das erste Jahrhundert zur\xfcckgeht.
Um diese Unterschiede zu messen, entwickelten Forscher in den 1980er Jahren eine "Skala zur Langeweileanf\xe4lligkeit".
Stattdessen sollte unser Ziel darin bestehen, uns auch abseits der st\xe4ndigen Aktivit\xe4ts- und Technologieberieselung wohlzuf\xfchlen.
Nicht etwa aufgrund meines recht ungew\xf6hnlichen Namens, oder weil ich von einer Privatschule gekommen war.
Die Leute glauben, wir sind wie der Bullingdon Club, ohne uns \xfcberhaupt kennengelernt zu haben".
"Miss Wyatt", sagte der Tutor Harry Pitt (mittlerweile verstorben), "\xfcbersetzen Sie bitte den ersten Absatz".
"Weigern sich Thatcher-Anh\xe4nger, Franz\xf6sisch zu lernen, oder sind sie einfach nur dumm?", fragte er mich.
Ich bestand darauf, dass ich nicht in allen Punkten mit Mrs. Thatcher einer Meinung war.
1997 nahm er eine Professur an der Universit\xe4t Bilkent in Ankara in der T\xfcrkei an.
Aber keine 18-J\xe4hrige sollte jemals in einer Bildungseinrichtung unter derartiger Einsch\xfcchterung und Boshaftigkeit leiden m\xfcssen.
Er sa\xdf am Tisch der Gr\xe4fin Jacqueline de Ribes, einer sehr guten Freundin von mir.
Die Minenarbeiter von Kawah Ijen verdienen 5 Eurocent f\xfcr jedes Kilo Schwefel, das sie abbauen.
"Ich wei\xdf nicht, ob mir jemand antwortet, ich lade sie nur hoch" f\xfcgt er hinzu.
"Das erschreckt mich nicht, weil wir etwas gemein haben, zum Beispiel Musik", gibt er an.
Die Digitalen Natives sind sie, die Kinder und Jugendlichen, die mit dieser Technologie aufgewachsen sind.
"Wenn ich schon sterben muss, dann lieber drei Mal platzen", sagt man in meinem Fall.
Es gibt Dinge, die ich eingef\xfchrt h\xe4tte, wie z. B. die Regionalisierung der unteren Kategorien.
Wenigstens sehe ich das Ergebnis der vorgeschriebenen Ausbildungen und Kurse f\xfcr Trainer, Tisch-Offizielle und Schiedsrichter.
Und nat\xfcrlich genie\xdfe ich die Gesellschaft meiner Frau Isabel, die immer an meiner Seite war.
Er war kreativ, gro\xdfz\xfcgig, lustig, witzig, liebevoll und talentiert, und ich werde ihn sehr vermissen.
1995 wurde ein b\xf6sartiger Tumor in seiner Leber festgestellt, und er unterzog sich einer Transplantation.
2001 betitelte er seine Memoiren "Hello Darlin: Tall (and Absolutely True) Tales about My Life".
Wochenlang vor Semesterbeginn erhielten wir E-Mails von Studenten, die fragten, ob noch Pl\xe4tze frei seien.
Die apokalyptische Sekten- oder Religionsmentalit\xe4t ist eigentlich nur eine Frage von Trost oder dessen Fehlen.
"Nie habe ich etwas von einem Unterricht geh\xf6rt, wo dies unterrichtet wird", gab er an.
Die F\xfchrungskr\xe4fte der Republikaner rechtfertigen ihre Politik mit der Notwendigkeit, den Wahlbetrug zu bek\xe4mpfen.
Dar\xfcber hinaus verf\xfcgen f\xfcnf Millionen Neuw\xe4hler im Jahr 2012 nicht \xfcber einen derartigen Ausweis.
Aber eins ist sicher: diese neuen Bestimmungen werden sich negativ auf die Wahlbeteiligung auswirken.
Dies f\xfchrt zu st\xe4rkerem Z\xf6gern der bereits unentschlossenen M\xe4nner f\xfcr die Durchf\xfchrung von Fr\xfcherkennungstests.
"Heute noch gibt es in Quebec 1,5 Mio. Raucher", bedauert der Sprecher Andr\xe9 Beaulieu.
Sie scheinen das Risiko f\xfcr Brust-, Grimmdarm-, Mastdarm-, Speiser\xf6hren-, Bauchspeicheldr\xfcsen- und Geb\xe4rmutterkrebs zu erh\xf6hen.
In den letzten Jahren haben mehrere Wissenschaftler den Zusammenhang zwischen Vitaminzus\xe4tzen und Krebs untersucht.
Die Wirkung von Vitamin D auf den Krebs wurde ebenfalls noch nicht deutlich aufgezeigt.
Au\xdferdem k\xf6nnen sich Anwendungen auch aus all den Instrumenten ergeben, die die Forschung umgeben.
"Allerdings ist es immer ein Schock, darauf kann man nicht vorbereitet sein", sagt er.
"Das h\xe4ngt von der F\xe4higkeit der Person ab", einen R\xfcckschritt hinzunehmen, stellt er fest.
Das ist sehr wenig, wenn man ber\xfccksichtigt, dass wir eines Tages alle sterben werden.
Patienten ohne Schmerzlinderung werden immer h\xe4ufiger die M\xf6glichkeit haben, auf diese terminale Sedierung zur\xfcckzugreifen.
Im Mai waren wir entt\xe4uscht, da wir stark genug waren, um den Sieg davonzutragen.
Wir haben insbesondere die afghanischen Bauern bestraft, indem wir sie als Terroristen angesehen haben.
Die von Hubschraubern \xfcberflogenen Lastwagen- und Panzer-Konvois haben Kabul erreicht, ohne angegriffen zu werden.
Pr\xe4sident Karza \u2047  will keine ausl\xe4ndischen Kontrollen, insbesondere anl\xe4sslich der f\xfcr April 2014 geplanten Wahlen.
Traditionsgem\xe4\xdf hinterlassen dort Menschen verschiedener Glaubensrichtungen Zettel mit W\xfcnschen, die dann in Erf\xfcllung gehen.
Daf\xfcr gibt es viele wohlgen\xe4hrte Katzen, die gem\xfctlich und unbehelligt durch die Stra\xdfen streunen.
Im Jahr 2012 haben mehr als drei Millionen Touristen aus aller Welt Israel besucht.
Sprachkenntnisse m\xfcssen sowohl f\xfcr den Erhalt als auch die Verl\xe4ngerung der Arbeitserlaubnis nachgewiesen werden.
Im Jahr 2011 wurde ein Bericht vom Zentrum f\xfcr Problemanalysen und staatliche Verwaltung verfasst.
Ihm zufolge ist es h\xe4ufiger, dass H\xe4ndler sich den Nachschub in einem Waffenlager besorgen.
\xdcber einen F\xe4hnrich wird eine Waffe, zum Beispiel eine Pistole vom Typ TT, gekauft.
Der K\xe4ufer bekommt laut Baranez nicht die Katze im Sack, sondern kann alles ausprobieren.
Die Gr\xfcndung von Gewerkschaften in der Fast-Food-Branche ist aber auch aus objektiven Gr\xfcnden schwierig.
Lautstarke Proteste gab es an diesem Tag auch vor vielen anderen Fast-Food-Restaurants in Manhattan.
Eine interessante Methode ist derzeit die Verwendung der zweiten Hand als etwas ungew\xf6hnliche Projektionsunterlage.
Fr\xfcher war ich sozial, aber jetzt schmerzt es und bereitet Angst, so zu sein.
De facto gibt es nur zwei echte Planeten, die wir zumindest hypothetisch bewohnen k\xf6nnten.
Tiere, die aus ihrem nat\xfcrlichen Lebensraum gerissen werden, k\xf6nnen einfach ihrem Fortpflanzungstrieb nicht folgen.
Hier in einem Schwebezustand gewinnen die Kosmonauten Routine f\xfcr die Arbeit im offenen Weltraum.
Die Geburt k\xf6nnte zum Beispiel auch in einer Spezialkammer stattfinden, um das Kind herauszupressen.
Gibt es hier eine \xe4hnliche Beh\xf6rde wie unser NK \u2047 , oder funktioniert das System anders?
Die Temperaturen sanken auf -5 bis -10  \u2047 C, tags\xfcber soll es etwas w\xe4rmer werden.
In Ostb\xf6hmen ist es heute \xfcberwiegend sonnig oder heiter, und es bleibt weitgehend niederschlagsfrei.
Die Temperaturen bewegen sich zwischen -3 und +1  \u2047 C, es weht ein schwacher Wind.
Im S\xfcden der Kreise Pilsen und Tachov kann es jedoch abschnittsweise zu Eisgl\xe4tte kommen.
Fahrer sollten haupts\xe4chlich auf den weniger frequentierten Stra\xdfen im Bereich B\xf6hmerwald besonders vorsichtig sein.
Was denken Sie dar\xfcber, dass in weniger als einem Monat der Weltuntergang stattfinden soll?
Im Dezember realisieren Sie au\xdferdem ein einzigartiges Projekt mit drei Konzerten gegen den Weltuntergang.
The Tap Tap ist jedoch eine Gruppe, die sich aus Menschen mit Behinderungen zusammensetzt.
Bekannt wurde die Band aber erst in den letzten Jahren, oder irre ich mich?
Dank der EU-F\xf6rdergelder k\xf6nnen wir uns \xfcberdies gute Lektoren, hochwertige Ger\xe4te und u.\xe4. leisten.
Wer den Willen hat und die Lust am Mitmachen, ist bei uns immer willkommen.
Findet statt am Tag vor dem prognostizierten Weltuntergang, Donnerstag den 20.12.2012 um 21 Uhr
Es ist bestimmt interessant, die Problematik mal von einer breiteren Perspektive aus zu betrachten.
Im Endeffekt bedeutet dies, dass die einzelnen Volkswirtschaften in einem permanenten Konflikt miteinander stehen.
Diese Situation ist allgemein bekannt, so dass konkrete Statistiken an dieser Stelle \xfcberfl\xfcssig sind.
Ein derartiger Skandal wurde auch im Falle von im Deutschen Bundestag besch\xe4ftigten Hilfskr\xe4ften aufgedeckt.
Die Aufhebung des Gesetzes \xfcber gemeinn\xfctzige Arbeiten ist hier keine L\xf6sung, zumindest keine dauerhafte.
Gleichzeitig ist es Afflecks erster Film, der nicht im heimatlichen Boston des Regisseurs spielt.
Affleck beweist dieses Gesp\xfcr jedoch auch in Argo, wo Teheran von Kanada "gespielt" wird.
Mit einer EU-Marke k\xf6nnen sich da der Pardubicer Lebkuchen oder die Ho \u2047 icer Rollen br\xfcsten.
Eine starke Pers\xf6nlichkeit, die auf Missst\xe4nde hinweist, kann Druck auf die politische Szene aus\xfcben.
Das d\xfcnne Textil h\xe4lt ein, zwei Saisonen, danach ist es reif f\xfcr den Sperrm\xfcll.
Deutschland hat sich in der Abstimmung \xfcber die Aufnahme von Pal\xe4stina der Stimme enthalten.
Deutschland wollte seine Unabh\xe4ngigkeit demonstrieren - ohne allerdings zu kritisch gegen\xfcber Israel zu sein.
Das ist eigentlich das alte Problem: du willst nicht von feindseligen L\xe4ndern umringt sein.
Es muss empf\xe4nglich f\xfcr verschiedenste Nachbarn und Meinungen sein und das ist nicht einfach.
Den Nachahmern reichen schon ein paar zus\xe4tzliche Buchstaben, damit sie ihre Marken anmelden d\xfcrfen.
Dass die Chinesen Weltmeister im Kopieren und im Verletzten geistigen Eigentums sind, ist bekannt.
Doch L\xf6schungen dubioser Eintr\xe4ge im Markenregister sind schwer zu erreichen und gehen ins Geld.
Im vergangenen Jahr sei man aber von der "Notsituation im Arbeitsablauf zur Normalit\xe4t zur\xfcckgekehrt".
Vereinfacht hei\xdft das, dass jede Anmeldung im Schnitt 1280 Yuan oder 160 Euro kostet.
In Heidelberg probt der Chor Imbongi - und in Swasiland freuen sich Aidswaisen dar\xfcber.
Syphilis und Tripper kommen vor allem bei M\xe4nnern vor, die Sex mit M\xe4nnern haben.
Eigentlich seltsam in einem Land, in dem sich der K\xf6nig offiziell 14 Ehefrauen h\xe4lt.
Der letzte absolute Monarch Schwarzafrikas, K\xf6nig Mswati III., ist f\xfcr seinen exzessiven Lebensstil bekannt.
Diese soll mindestens 30 Zentimeter und m\xf6glicherweise sogar bis zu 20 Meter dick sein.
Von Zeit zu Zeit senden sie Bilder zur Erde: Kleine Guckl\xf6cher in unendliche Weiten.
M\xf6glicherweise sind sie die \xdcberreste eines Saturn-Mondes, der vor 4,5 Milliarden Jahren spurlos verschwand.
Wem technische Abk\xfcrzungen nicht liegen, der mag sie bei ihrem Spitznamen S\xfcdliches Feuerrad nennen.
Das Foto des Weltraumteleskops Hubble zeigt einen Ausschnitt aus dem Irisnebel im Sternbild Kepheus.
Es zeigt einen Ring aus schwarzen L\xf6chern, 430 Millionen Lichtjahre von der Erde entfernt.
F\xfcr die 323 Kilometer braucht man acht Stunden, weil die Stra\xdfe nur einspurig ist.
Doch Pilata Fatulayeva (48) ist davon \xfcberzeugt, dass Lerik das Zeug zur Touristenattraktion hat.
Sie ist die Direktorin des Museums f\xfcr Langlebigkeit, wohl das einzige auf der Welt.
Sie sitzt auf dem Boden mit einem Butterfass, das sie unerm\xfcdlich hin- und herrollt.
Mein ganzes Leben lang habe ich nicht ein einziges Mal im Supermarkt Lebensmittel gekauft.
Bis 2003 war er an der Macht, sp\xe4ter \xfcbernahm sein Sohn Ilham das Ruder.
Reicht da schon eine Karikatur des Pr\xe4sidenten oder ein Witz auf Kosten eines Rechtsgelehrten?
"Die Revolution ist zur\xfcckgekehrt und wir werden siegen", sagte Hamdin Sabbahi, Drittplatzierter der Pr\xe4sidentschaftswahlen.
Sie forderten von Mursi: "S\xe4ubere das Land!" und beteuerten: "Der Koran ist unsere Verfassung."
Nicht weil er deren Weltanschauung teilen w\xfcrde, sondern weil f\xfcr ihn Menschenrechte unteilbar sind.
Ich befinde mich in der kleinen Stadt Fagernes, etwa drei Stunden von Oslo entfernt.
So ein Elch-Burger ist auf jeden Fall etwas anderes. Das saftige Fleisch mundet mir.
"Welche Punktzahl habt ihr dort oben in den Bergen f\xfcr den besten Fisch, Thor-J\xfcrgen?"
In der entlegenen Kleinstadt Valle del Bravo erinnert man sich beispielsweise gerne an ihn.
Die Vorw\xfcrfe der Opposition, dem neuen Pr\xe4sidenten fehle es an Substanz, lehnt er ab.
Doch genau davor f\xfcrchten sich die Familien der Opfer in Ciudad Neza am meisten.
"Meine Welt schrumpfte auf Camp Arafjon, auf diesen K\xe4fig zusammen", sagte Manning am Donnerstag.
Man habe ihm nur eine Matratze, eine Decke, Flip-Flops, Kleidung und seine Brille erlaubt.
Stets habe er mit Licht schlafen m\xfcssen, das von au\xdfen in seine Zelle eindrang.
Schilder verwiesen auf zwei Warteschlangen: Eine f\xfcr "Mexicanos" ("Mexikaner"), eine andere f\xfcr "Extranjeros" ("Ausl\xe4nder").
Und in der Heimat meines Gro\xdfvaters gab es keinen Bedarf nach K\xfcrzeln oder Bindestrichen.
Also nahm ich meinen amerikanischen Reisepass und stellte mich in die Schlange f\xfcr Extranjeros.
Unser Spanisch wird niemals gut genug, unsere Bande zu Mexiko nie stark genug sein.
Auf den ersten Blick scheint Optimismus angesichts der aktuellen Lage alles andere als angebracht.
Weit entfernt im wei\xdfen Haus scheint es, als w\xe4re er ebenso einer Beteiligung abgeneigt.
Gesundheitswarnungen und erkrankte K\xf6rperteile auf neutralen gr\xfcnen Packungen, die f\xfcr alle Tabakmarken gleich sind
Zico habe bis zu 6.000 Einheiten an Gro\xdfhandelsgesch\xe4fte verkauft und warte auf neue Best\xe4nde.
Plibersek zufolge hat die Regierung Gespr\xe4che mit anderen L\xe4ndern gef\xfchrt, die \xe4hnliche Verpackungsgesetze erw\xe4gen.
Ich hatte also genug Zeit, um mir ein paar Gedanken zu Langeweile zu machen.
Doch Fernsehen kann zwar kurzfristig f\xfcr Gl\xfccksgef\xfchle sorgen, diese verfl\xfcchtigen sich langfristig aber wieder.
Pitt war ein kleiner Mann mit einem Gesicht wie aus Kuchenteig, und ziemlich geh\xe4ssig.
W\xfcrde es mir je gelingen, an der Universit\xe4t Oxford ein normales Leben zu f\xfchren?
Einer meiner m\xe4nnlichen Freunde, ebenfalls Tory-Anh\xe4nger, hatte dem Druck nachgegeben und seinen \xdcberzeugungen entsagt.
Es war mein Vater, der den letzten Nagel in den Sarg meiner Oxford-Karriere schlug.
Ich versteckte mich in meinem Zimmer, und nach f\xfcnf Minuten gaben meine H\xe4scher auf.
Als sie gingen, packte ich einen Koffer und nahm den ersten Zug nach London.
"Er kommt nie aus der Mode, weil seine Designs Kunstwerke sind" sagt sie abschlie\xdfend..
Er mag Leute mit guter Erziehung und den h\xf6chsten Titeln, und sie lieben ihn.
"Es war ein Geschenk von ihm", sagt Naty Abascal, eine der Musen des Designers.
Ungef\xe4hr 400 Tr\xe4ger laden sich am Kraterboden die K\xf6rbe mit Schwefel auf ihre Schultern.
Von seinen f\xfcnf Kindern arbeitet der \xc4lteste mit seinen 30 Jahren auch als Schwefel-Tr\xe4ger.
Dies ist etwas nur f\xfcrs Internet, deshalb mussten wir es lustig und witzig gestalten.
M\xf6glich, dass viele dieser Ideen kreativ waren, sie f\xfchrten aber nicht zwingend zum Erfolg.
Ich meldete mich bei Twitter an, um mich auszudr\xfccken und interessante Tweets zu schreiben.
Der Zugang der Journalisten zur Information \xfcber das Gipfeltreffen war zu jedem Zeitpunkt beschr\xe4nkt.
Konflikte sind unvermeidbar, sie m\xfcssen aber im Streben nach einem gemeinsamen Weg \xfcberwunden werden.
Sie m\xfcssen umfassend behandelt werden, damit man sie \xfcberwinden und nach vorne schauen kann.
"Es bedeutet in keinem Fall einen R\xfcckfall im Gesundheitszustand des Pr\xe4sidenten Ch\xe1vez", kommentierte er.
Es waren viele erf\xfcllende Jahre, einschlie\xdflich der f\xfcnf Meisterschaften nacheinander von 1971 bis 1975.
War diese Gruppe der Weltmeisterschaft 1990 die beste Nationalmannschaft, die du je gesehen hast?
Es war Kristin, die Schw\xe4gerin von J.R. (interpretiert von Mary Crosby) die geschossen hatte.
Ebenso setzte er sich gegen das Rauchen ein und nahm an mehreren Kampagnen teil.
Und er erinnert daran, dass das Schlechte gut f\xfcr jene mit apokalyptischer Mentalit\xe4t ist.
Wenn nukleares Material in die H\xe4nde von Terroristen gelangt, k\xf6nnte beispielsweise ein Krieg ausbrechen.
Trotz des "bevorstehenden Untergangs" m\xfcssen die Studenten studieren, Projekte erstellen und an Abschlusspr\xfcfungen teilnehmen.
Eins ist sicher: diese neuen Bestimmungen werden sich negativ auf die Wahlbeteiligung auswirken.
Vor 2004 hat kein Bundesstaat f\xfcr das W\xe4hlen einen Nachweis der Staatsb\xfcrgerschaft gefordert.
Das Wichtigste ist, die richtige Entscheidung zu treffen, sobald eine Krebserkrankung erkannt wurde.
Allerdings wird davon ausgegangen, dass etwa 10% der Krebserkrankungen durch Vererbung verursacht werden.
Gem\xe4\xdf der kanadischen Krebsgesellschaft f\xf6rdern \xdcbergewicht und Adipositas ebenfalls den Ausbruch der Krankheit.
"Letztere k\xf6nnen die K\xf6rperzellen sch\xe4digen und zur Entwicklung von Krebs f\xfchren", erkl\xe4rt er.
Die Debatte muss in K\xfcrze wieder aufgenommen werden, obwohl ein Gesetzesentwurf vorbereitet wird.
Der Prostatakrebs, der ihn aufzehrte, hatte ihm eine Frist von zwei Jahren gelassen.
Man gew\xe4hrt dem Sterbenden je nach Wunsch eine Mundpflege mit Brandy oder Pepsi.
Patienten, deren Schmerzen nicht gelindert werden, sagen alle denselben Satz: "Ich will sterben."
Er wird verd\xe4chtigt, im Austausch f\xfcr \xf6ffentliche Auftr\xe4ge wiederholt Schmiergelder entgegengenommen zu haben.
Finanziell gibt sich der PSG die Mittel, damit dieses Vorhaben konkrete Formen annimmt.
Aber eine andere Mannschaft, jene von Montpellier, hat eine noch bessere Saison erzielt.
Das hie\xdfe, dass unsere Gegner und die franz\xf6sische Meisterschaft au\xdfer Acht gelassen w\xfcrde.
Der PSG scheint vollst\xe4ndig von den Leistungen von Zlatan Ibrahimovic abh\xe4ngig zu sein.
Der Nationaltrainer ist strikt, steht den Spielern nahe und regt zum Sieg an.
Blanc hatte sein Ziel erreicht, indem er uns f\xfcr die EM qualifiziert hatte.
Stellt das am 16. Oktober in Spanien erzwungene Unentschieden (1:1) ein Auftaktspiel dar?
Allerdings wird der Handel jedes Mal von einer zentralen Beh\xf6rde kontrolliert und bearbeitet.
Zur Verhinderung einer Inflation wird diese Belohnung regelm\xe4\xdfig halbiert, wahrscheinlich vor Ende 2012.
Dar\xfcber hinaus wird die Schwierigkeit der Aufgabe mit jeder Verbesserung der Rechenleistung erh\xf6ht.
Die Webseiten, die Dienste f\xfcr Bitcoin bereitstellen, wurden angegriffen und die Bitcoin-Einlagen gestohlen.
Die EZB berichtet auch \xfcber die M\xf6glichkeiten der Geldw\xe4sche mithilfe dieses anonymen Dienstes.
Und uns selbst mit unseren 88 get\xf6teten Soldaten, sowie den Verletzten und Versehrten.
Ab Ende 2014 wird es kein Einstr\xf6men mehr der Taliban in Kabul geben.
Seit ihrem unwiderstehlichen Vormarsch von 1994 bis 1996 haben sich die Bedingungen ge\xe4ndert.
Ihre Macht\xfcbernahme wurde damals als eine Art Befreiung und R\xfcckkehr zur Sicherheit angesehen.
Die wichtigsten Pers\xf6nlichkeiten des antisowjetischen Kriegs sind 2001 wieder an die Macht gekommen.
Diese neue Initiative hat nur f\xfcr eine noch st\xe4rkere Spaltung des Landes gesorgt.
Die Text, der gestern Abend noch verabschiedet worden ist, besteht aus 234 Artikeln.
Man bezieht sich hier insbesondere auf den "Fiqh" [islamische Rechtsprechung, Anm. d. Red.].
Die Moslembr\xfcder argumentieren, dass diese verglichen mit dem ehemaligen Regime deutlich reduziert sind.
Gl\xe4ubige begehen hier den Leidensweg bzw. Kreuzweg Jesu Christi (auf Latein: Via Dolorosa).
J\xe4hrlich kommen 13 Millionen Gastarbeiter nach Moskau, Sankt Petersburg und andere St\xe4dte Russlands.
Die meisten von ihnen sind die B\xfcrger des Zentralasiens: Usbekistan, Tadschikistan und Turkmenistan.
Auf dem zweiten Kanal kommen illegale Waffen, die Ordnungsh\xfctern von Kriminellen gestohlen werden.
Ich komme derzeit sogar an einige Schlagringe \xfcber einen Bekannten, dem ich vertraue.
Noch ist nicht abzusehen, ob der Funke dieser Proteste ganze Massen mobilisieren wird.
Wir jedoch wollen 5-10 Jahre vorausblicken und die radikalen Ver\xe4nderungen dieser Interaktion vorhersehen.
Wir m\xfcssen die Computerwelt in unsere physische Welt entlassen und sie fassbarer machen.
- Wir w\xfcrden Sie mich zum Beispiel bitten, Ihnen diese Sprudeldose zu reichen?
Nicht alle verstehen, wie sehr das die Interaktion von Mensch und Maschine beeinflusst.
Ich denke, der achte Durchbruch k\xf6nnte durchaus die Integration der taktilen Wahrnehmung werden.
- Das ist eine gute Idee, so haben wir es noch nicht versucht.
Kirill Miller ist einer der typischen Petersburger sozial-philosophischen K\xfcnstler, die neue Mythen erschaffen.
- Bei einer Ausstellung im Kulturpalast Newskij, bei der meine Arbeiten ausgestellt waren.
Ich werde eine Ausstellung mit dem Thema "Das russische Museum als Clowns" haben.
- Zu ihm kommen verlassene Frauen, dort spielt die sexuell-soziale Sph\xe4re eine Rolle.
"N\xe4mlich Mars und Venus", sagt der wissenschaftliche Mitarbeiter des Astronomischen Sternberg-Instituts Wladimir Surdin.
Es folgte die Z\xfcchtung von Insekten, genauer von winzigen Fruchtfliegen (Drosophila), im Orbit.
Es gab ein Experiment mit Ratten, die bereits befruchtet ins All geschickt wurden.
Das Hydrolabor im Vorbereitungszentrum der Kosmonauten ist eine obligatorische Station w\xe4hrend der Flugvorbereitung.
"Das ist zu wenig Zeit, um etwas zu vergessen", sagt Babyschwimmlehrerin Marina Aksenowa.
Ihm wird einfach das fehlen, was f\xfcr sein Leben von elementarer Bedeutung ist.
Das bestimmt nicht, aber wie gesagt: Derartige Vergleiche mag ich nicht besonders gern.
Andernfalls h\xe4tten sie ja nichts von einer Zusammenarbeit mit unserer Beh\xf6rde, nicht wahr?
Da unsere Kontrollen nachtr\xe4glich stattfinden, muss man hier mit einer gewissen Verz\xf6gerung rechnen.
Befahrbar sind gleichfalls alle Verkehrswege der zweiten und dritten Stra\xdfenklasse, einschlie\xdflich der Bergstra\xdfen.
Schnee liegt insbesondere auf den Stra\xdfen im Riesengebirge und im Gebirge Orlick\xe9 hory.
Das ist eine von jenen Katastrophenmeldungen, auf die wir Menschen so gerne anspringen.
Es handelt sich um eine landesweite Benefizveranstaltung, die wir schon zwei Jahre planen.
Die Hymne soll von allen Interpreten auf allen drei Konzerten gleichzeitig gesungen werden.
Au\xdferdem werden die Hymnen zusammen in einer Direktschaltung vom Tschechischen Fernsehen live \xfcbertragen.
War es Ihr Ziel, es mit The Tap Tap so weit zu bringen?
Im Jahr 1933 begann die polnische Infanterie, sich mit raketenbetriebenen Geschossen zu befassen.
Der Artikel von Prof. M. Subotowicz enth\xe4lt den Vorschlag zur Gr\xfcndung einer Raumfahrtgesellschaft.
In der vergangenen Woche hob das Verfassungsgericht das Gesetz \xfcber gemeinn\xfctzige Arbeiten auf.
Aufgrund der gro\xdfen Unterschiede des Werts von Arbeit (L\xf6hne) kommt es zu Preisspannungen.
Das Ergebnis sind wachsende Armut, sowie immer gr\xf6\xdfere Unterschiede zwischen Arm und Reich.
In jeder Epoche k\xf6nnen wir einen Alexander den Gro\xdfen oder einen Napoleon ausmachen.
In ihrer Vorstellung ist die neue Weltordnung eine Welt der Herren und Sklaven.
"Weitere unglaubliche Einf\xe4lle aus der EU-Werkstatt k\xf6nnen bis Ende dieses Jahres nominiert werden.
Wenn in unserem Land alles ohne Probleme funktionieren w\xfcrde, w\xfcrde ich nirgendwohin kandidieren.
Man h\xe4lt bereits Ausschau nach Parkbank, Hund und Fu\xdfball spielenden Jungs und M\xe4dels.
Sie sorgen f\xfcr Atmosph\xe4re, vor allem aber f\xfcr die richtige Luftfeuchtigkeit im Literaturgebirge.
Stephen Szabo: Deutschland unterst\xfctzt das, was die Israelis in Gaza getan haben, nicht.
F\xe4llt es Deutschland schwer, bei wichtigen internationalen Themen eine klare Position zu beziehen?
Zum einen hat Deutschland gro\xdfe Absatzm\xe4rkte im Nahen Osten, besonders in den Golfstaaten.
Das ist nat\xfcrlich nicht einfach f\xfcr Deutschland, schon wegen der Beziehung zu Israel.
Auch deutsche Unternehmen werden auf diese Weise legal kopiert, etwa der Sportartikelhersteller Puma.
In den gro\xdfen St\xe4dten gibt es mehrst\xf6ckige Kaufh\xe4user, die fast ausschlie\xdflich F\xe4lschungen verkaufen.
Die Chinesen d\xfcrfen deshalb bis heute ein Emblem verwenden, das dem Mercedes-Stern \xe4hnelt.
Fast 57.000 solcher F\xe4lle habe man abgeschlossen, 75 Prozent mehr als im Vorjahr.
Das gelte auch f\xfcr den Bestand aller g\xfcltigen Markenzeichen, insgesamt 5,5 Millionen St\xfcck.
Dagegen anzugehen kostet ein Vielfaches, wie der Fall des deutschen Familienunternehmens Freudenberg zeigt.
Zwar konnten die Deutschen erreichen, dass dessen illegale Fabrikation imitierter Kraftfahrzeugteile ausgehoben wurde.
Doch sicherte sich der Nachahmer weiterhin die chinesischen Rechte an der Marke Freudenberg.
Dieses Gesch\xe4ftsfeld hat der Konzern l\xe4ngst aufgegeben, trotzdem konnte er die Registrierung abwenden.
Sie garantiert dem Kind Schulgeld, Schuluniform und eine warme Mahlzeit t\xe4glich im Gogo-Center.
Oft verursachen sie jedoch keine Schmerzen oder andere Symptome und bleiben deshalb unbemerkt.
Die Reise f\xfchrt immer auch nach Esitjeni, wo die S\xe4nger ihre Patenkinder besuchen.
Die US-Raumfahrtbeh\xf6rde NASA hat die Existenz von Eis auf dem Planeten Merkur nachgewiesen.
Das Bild kommt von einer Kamera, die deutsche Forscher vom Max-Planck-Institut entwickelt haben.
Wie ein rotes Age blickt der Helix-Nebel auf diesem Infrarot-Foto dem Betrachter entgegen.
Seine \xc4hnlichkeit mit einem irdischen Kontinent brachte diesem Nebel den Titel Nordamerika ein.
Hier steht das Very Large Telescope - das seinem Namen alle Ehre macht.
Mit seinen insgesamt vier Spiegeln kann das Fernrohr auch das mittlere Infrarotspektrum ausleuchten.
Radarmessungen haben seit Jahrzehnten darauf hingedeutet, dass es auf dem Merkur Eis gibt.
Alles ist gr\xfcn und saftig, man k\xf6nnte meinen, man bef\xe4nde sich im Schwarzwald.
"1805 wurde er hier in der Region geboren, 1973 starb er", erl\xe4utert Fatulayeva.
Hat sich  \u2047 irali M\xfcsl\xfcmov also bei seinem Alter um ein paar Jahrzehnte verrechnet?
Der aserische Reisef\xfchrer Farid Mugimzadeh erkl\xe4rt das mit den besonderen Genen der Talyschen.
Doch alles wurde besser, als der "geliebte Vater" Heydar Aliyew das Ruder \xfcbernahm.
Wenn das kein Grund ist, so lange wie m\xf6glich am Leben zu bleiben
Was aber eine Beleidigung ist und wie sie geahndet werden soll, bleibt unklar.
Ich werde eine neue Sicherheitsstrategie vorschlagen, mit der wir dieses Ziel erreichen k\xf6nnen.
Doch im schlimmsten Falle habe seine Regierung ihre Augen vor dem Problem verschlossen.
Es gab Anzeichen, dass sie geschlagen wurde, und die Leichenstarre hatte bereits eingesetzt.
Im April 2011 wurde Manning in das Milit\xe4rgef\xe4ngnis von Fort Leavenworth, Kansas verlegt.
Wird er in allen Anklagepunkten f\xfcr schuldig befunden, droht ihm eine lebenslange Haftstrafe.
Ich stand dort einige Sekunden lang, unsicher, zu welcher ich mich begeben sollte.
Ich bin in Zentralkalifornien aufgewachsen und wurde mein ganzes Leben lang "Mexikaner" genannt.
Wir lieben die mexikanische Band Los Tigres del Norte, aber auch Bruce Springsteen.
Kann es jemals anhaltenden Frieden zwischen Arabern und Juden im Nahen Osten geben?
Au\xdfenstehende arabische Nationen sollten ebenfalls die Hamas und Fatah zu einer Einigung bewegen.
In einer st\xe4ndig elektrisierten Welt ist es sch\xf6n, auch mal gelangweilt zu sein
Aber das Gehirn wei\xdf nicht immer, was man gerade am besten tun sollte.
Und er f\xfcgt hinzu: "Selbstkontrolle \xfcbertr\xe4gt sich von einer Situation auf die andere".
In Weld County im Norden Colorados vertritt Bezirksstaatsanwalt Ken Buck eine strengere Ansicht.
Mehrere St\xe4dte in Colorado warten erst gar nicht darauf, dass die Bundesbeh\xf6rden handeln.
Meinem Vater erz\xe4hlte ich, dass ich Oxford hasste, und warum ich es tat.
So etwas w\xfcrden sie nie tun, nicht in meiner Stadt der tr\xe4umenden Turmspitzen.
Valentino versp\xfcrte immer schon Faszination f\xfcr die stickige und ferne Welt des Adels.
Wir waren ungef\xe4hr 20 Personen, darunter auch Sharon Stone und John Kennedy Jr.
Das Leben von Garavani ist keine Geschichte von Versessenheit, eher von gegenseitigen Liebschaften.
Viele dieser Kundinnen sagen, der erste Valentino ist wie die erste Liebe, "unvergesslich".
Jahrelang mit dem "savoir- \u2047 tre" der Elite getr\xfcbt, ist Valentino jetzt ihr bestes Exemplar.
Dies ist der Preis, den er f\xfcr das Erreichen seines Traumes bezahlen muss.
Gem\xe4\xdf seiner nationalen Bev\xf6lkerungsbeh\xf6rde liegt die Geburtenrate gegenw\xe4rtig bei 1,2 Kindern pro Frau.
Die Regierung versucht zu erreichen, dass nicht so viele kleine Wohnungen gebaut werden.
Diese Appartements haben eine Wohnfl\xe4che von 46 Quadratmetern und zeigen einen gro\xdfen Verkaufserfolg.
Dies f\xfchrt dazu, dass sie f\xfcr unseren Cash Flow sehr viel besser sind.
Gefragt antwortet er, dass er nie eine Einladung von einem Unbekannten annehmen w\xfcrde.
Jos\xe9 meldete sich bei Ask, nachdem er in Twitter eine Empfehlung gelesen hatte.
Danach erl\xe4utert er eine Reihe von Schritten, um ein Benutzerkonto sicher zu konfigurieren.
Und noch eine Frage: M\xfcssen alle wissen, was du in jedem Moment tust?
Und "wenn Gro\xdfbritannien Morgen diesen Freibrief gew\xe4hrt, ist dies meiner Meinung nach erledigt."
Es handelt sich um ein Problem zwischen einem s\xfcd- und einem mittelamerikanischen Staat.
92% der Ansteckungsf\xe4lle erfolgen \xfcber Geschlechtsverkehr, 6% \xfcber das Blut und 2% perinatal.
Tats\xe4chlich ist Vitro nicht der erste Fall, bei dem dieses Schema zugelassen wurde.
Ab dann \xfcbernahm "Cuco" Ortiz, der ein sehr guter Verwalter war", sagt Reyes.
"Ich wei\xdf, was auf dem Grabstein von J.R. stehen soll", sagte Hagman 1988.
Mehrere sagten, dass sie zu Feiern \xfcber "das Ende der Welt" gehen m\xf6chten.
In diesem Sinne untergraben diese Ma\xdfnahmen teilweise das demokratische System der USA.
In diesem Sinne untergraben diese Ma\xdfnahmen teilweise das demokratische System der USA.
F\xfcr was k\xf6nnen all diese Forschungen nun "gut sein", fragt Frau Plamondon?
Einige Stunden sp\xe4ter hat das Team ein Heilmittel f\xfcr dieses \xdcbel gefunden.
Die Palliativpflege wird dann eingesetzt, wenn es keine anderen M\xf6glichkeiten mehr gibt.
Heute Morgen wird sein Sohn das Bier zu F\xfc\xdfen des Verstorbenen austrinken.
Chantal Rouleau war eine der ersten Abgeordneten von Montreal, die Alarm schlug.
Die Neuzug\xe4nge dieses Sommers sind daran gew\xf6hnt, Spiele sehr hohen Niveaus auszutragen.
In der Ligue 1 hat Lyon uns den Platz des Spitzenreiters genommen.
Allerdings werden wir gegen sehr gute europ\xe4ische Mannschaften unser W\xf6rtchen mitzureden haben.
Innerhalb der Mannschaft respektieren wir sowohl den Spieler als auch die Person.
Nichts besonders Beeindruckendes im Vergleich zum Welthandel von realen W\xe4hrungen oder Finanzprodukten.
Der entscheidende Schritt besteht darin, diese neue Transaktion in dieses Buch einzutragen.
Dar\xfcber hinaus verwaltet der Inhaber seine Identit\xe4t und kann somit anonym bleiben.
In den St\xe4dten sind die staatlichen Schulen voll von M\xe4dchen wie Jungen.
Werden die Beh\xf6rden, unter deren Befehlsgewalt sie stehen wird, als legitim angesehen?
AIF nennt Ihnen die f\xfcnf wichtigsten Gr\xfcnde f\xfcr einen Besuch in Israel.
Es hei\xdft, dass alle, die in diesem Fluss baden, Gottes Segen empfangen.
Doch zumindest den f\xfcnf interessantesten von ihnen sollte ein Besuch abgestattet werden.
Auch das Museum of Art in Tel Aviv ist einen Besuch wert.
An jedem der drei Orte gibt es Schwimmb\xe4der, Wasserparks, Delfinarien und Ozeanarien.
Touristen schlendern gerne durch die engen Gassen, die nach Sternzeichen benannt sind.
"Das gro\xdfe und m\xe4chtige" f\xfchrt bis Moskau: Migranten sparen Geld f\xfcr Sprache
Ausnahmen gelten nur f\xfcr B\xfcrger von L\xe4ndern, in denen Russisch Amtssprache ist.
Nur eine organisierte Rekrutierung wird zu 90% die Probleme ausl\xe4ndischer Arbeiter l\xf6sen.
Als Teenager ergreifen diese Kinder dann sogleich die erste Gelegenheit zum Geldverdienen.
W\xe4hrenddessen h\xe4lt sich der Gro\xdfteil der Gastarbeiter weiterhin illegal in Russland auf.
Eine gef\xe4lschte Registrierung kann man schnell und lediglich f\xfcr eineinhalb Tausend machen.
W\xe4hrenddessen betont das Innenministerium, dass die Verbreitung illegaler Waffen unter Kontrolle ist.
Jeder vierte US-amerikanische Jugendliche sitzt irgendwann hinter der Kasse von Mc Donald's
Deshalb kaufen viele der geringf\xfcgig bezahlten Walmart-Besch\xe4ftigten nur am eigenen Arbeitsplatz ein.
Letztere klagen auch \xfcber schwere Arbeitsbedingungen, zum Beispiel fehlende Gabelstapler oder Handscanner.
Insgesamt f\xfchrten die Walmart-Kassen am "Black Friday" fast 100 Millionen Transaktionen aus.
Kaum einer sah darin die Haupteinkommensquelle oder plante, l\xe4nger dort zu bleiben.
Dann k\xf6nnten wir die reale Welt viel einfacher durch virtuelle Objekte erg\xe4nzen.
Aber insgesamt geh\xf6rt die Zukunft allerdings gemischten Steuerungstypen, beispielsweise Gestik und Sprache.
Nat\xfcrlich w\xe4ren 8 Megapixel mit einer Geschwindigkeit von 1000 fps nicht schlecht.
Auch die Geschwindigkeit und die Anzahl der Bilder pro Sekunde sind wichtig.
In dieser Welt ist Rot der Kompromiss zwischen K\xfcnstler, Imageberater und Gesellschaft.
Ich will aber durch meine Provokationen mit den Menschen ins Gespr\xe4ch kommen.
Ich bin ein Held des vergangenen Jahrhunderts, als Kultur noch etwas bedeutete.
Ich begann mit Bildern, die normalerweise erst am Ende der Karriere kommen.
In Europa gibt es viele neugierige Menschen, die Ausstellungen oder Konzerte besuchen.
Kunst muss wieder modern sein, so wie zu Beginn des vorigen Jahrhunderts.
Der letzte Brutk\xe4fig mit Tieren flog vor 16 Jahren in den Orbit.
Die Problematik der Fortpflanzung direkt im Weltraum konnte man bisher nicht l\xf6sen.
"Aber was passiert dann?", lautet die nicht unbedeutende Frage von Waleri Poljakow.
Sie sprechen \xfcber die Probleme bei der praktischen Umsetzung des tschechischen Vergabegesetzes.
\xdcberwiegend sind die Stra\xdfen jedoch gut befahrbar, mitunter ist erh\xf6hte Vorsicht geboten.
In den \xfcbrigen Gebieten des Bezirks sind die Fahrbahnen meist uneingeschr\xe4nkt befahrbar.
Es ist nicht so schlimm, wie es auf den ersten Blick erscheint.
Und in welcher Hinsicht m\xfcssen wir gegen\xfcber den weiter entwickelten L\xe4ndern aufholen?
Veranstaltungsorte sind: Incheba-Arena/Prag, Fl\xe9da/Brno und Plynojem/Ostrava; 12 tschechische Bands und weitere Musiker
Der Autor des Entwurfs und die Details dieses Vorhabens blieben leider unbekannt.
Die Forschung wurde dann freilich durch den Einmarsch der deutschen Wehrmacht unterbrochen.
Dieses Amt hatte er bis zu seinem Tod im Jahr 1959 inne.
Gegen Schmiergeld, durch ungesetzliche Erschleichung von Vorteilen oder mit Stein und Schwert.
Hier ist Weisheit! Wer Verstand hat, der \xfcberlege die Zahl des Tieres.
Ben Affleck ist mit diesem Film ein bemerkenswerter Neustart seiner Karriere gelungen.
Richtlinien f\xfcr das Aufblasen von Luftballons, f\xfcr Bananen und f\xfcr den Zirkus
Die eigentliche Abstimmung erfolgt dann bis Ende Februar 2013", teilte Nacher mit.
Sehen Sie sich als Mensch in der Politik eher rechts oder links?
Aus tschechischer Sicht scheint mir, dass mich die Leute eher links sehen.
Ich habe z.B. mit Radim Jan \u2047 ura gesprochen, der jedoch wegen Arbeits\xfcberlastung ablehnte.
Und ich bin nicht verpflichtet, die Kampagne aus eigenen Mitteln zu bestreiten.
Wenn ich nur Geld verdienen wollte, w\xfcrde ich f\xfcr gar nichts kandidieren.
Bleiben Sie also weiter als Unternehmer t\xe4tig, um Ihr Auskommen zu haben?
Spijkenisse, eine kaum besichtigungsbed\xfcrftige Schlafstadt vor den Toren Rotterdams, ist sonderbarer Rekordhalter.
Au\xdferdem ist das Projekt f\xfcr den Dutch National Wood Award 2012 nominiert.
Selbst eingefleischte Architekten und Bauingenieure sch\xfctteln ob des unbekannten Baustoffs den Kopf.
Damit ist MVRDV jene K\xf6nigsdisziplin gelungen, die man im Fachjargon Identit\xe4tsstiftung nennt.
Nun muss Deutschland aufgrund seiner besonderen Beziehung mit Israel allerdings vorsichtig sein.
Aber gleichzeitig glaube ich, dass es auch nicht die amerikanische Position unterst\xfctzt.
Erschwerend kommt hinzu, dass die Europ\xe4er keine koh\xe4rente und einheitliche Politik haben.
Aber es spielt auf jeden Fall eine wichtige Rolle in deutschen \xdcberlegungen.
So gesehen ist Deutschland in einer viel schwierigeren Position als die USA.
Dennoch genie\xdft sie so lange Schutz, wie die eigentlichen Namensgeber nicht klagen.
So wird aus Gucci einfach Lu-Gucci, statt Prada l\xe4sst man Prada-Kny eintragen.
Bis zu neun Jahre kann sich das Verfahren hinziehen, mit ungewissem Ausgang.
Seit mehr als sieben Jahren k\xe4mpft der Konzern gegen einen chinesischen Plagiator.
F\xfcr 15 oder 20 Euro im Monat kann man eine Patenschaft \xfcbernehmen.
Ohne Schulabschluss hat man in einem armen Land erst recht keine Chance.
Kondome k\xf6nnen das Risiko einer Ansteckung mindern, bieten aber keinen hundertprozentigen Schutz.
Die Temperatur auf dem Merkur kann bis zu 426 Grad Celsius erreichen.
Diese schillernde Glut eines sterbenden Sternes hat das Spitzer-Teleskop der Nasa aufgenommen.
Der Donut-f\xf6rmige Ring besteht aus Material, das der Stern im Sterbeprozess herausschleuderte.
Eine Kombination aus normalem und infrarotem Foto sorgt f\xfcr die spektakul\xe4re Farbgebung.
In diesem Sternennebel befindet sich die hellste Gruppe junger Sterne unserer Milchstra\xdfe.
Blick auf das Observatorium der Europ\xe4ischen Sternwarte (ESO) in den Chilenischen Anden.
Ebenfalls auf dem chilenischen ESO-Observatorium wird das European Extremely Large Telescope geplant.
Sie bieten gleich zwei Spiegel mit je einem Durchschnitt von zehn Metern.
Seit dem 24. April 1990 liefert es bereits Bilder von fernen Welten.
Wissenschaftler gehen davon aus, dass auch am S\xfcdpol des Merkur Eis existiert.
Eine Spurensuche in dem Land, in dem 97-J\xe4hrige noch vergleichsweise jung sind.
Eine Spurensuche in dem Land, in dem 97-J\xe4hrige noch vergleichsweise jung sind.
Mit ihren 97 Jahren ist sie f\xfcr diese Breiten noch vergleichsweise jung.
Denn sie alle, bisher hoffnungslos zerstritten in einer konfusen Opposition, haben Angst.
Nach dem Sturz des Diktators sa\xdfen bis zu 11.000 Zivilisten in Milit\xe4rhaft.
Kein Artikel \xfcbrigens schreibt ausdr\xfccklich die Gleichstellung von M\xe4nnern und Frauen fest.
Ebenso dubios mutet die Formulierung an, die "Beleidigung von Menschen" sei verboten.
Mursi Machtausweitung auf alle drei Gewalten im Staat lie\xdfen den Anwalt resignieren.
Er geh\xf6rt zu den teureren Gerichten, die man sich hier kaufen kann.
Doch genau diese, so die Familie, habe man ihr bis jetzt verwehrt.
Die Beh\xf6rden haben mich behandelt, als sei ich eine Schw\xe4tzerin, Unruhestifterin, N\xf6rglerin.
Sie m\xf6chten, dass man ihr Urteil einfach akzeptiert und den Mund h\xe4lt.
Die Staatsanwaltschaft widerspricht Bradley Mannings Vorw\xfcrfen, er sei im Gef\xe4ngnis misshandelt worden
Die Anh\xf6rung befasst sich mit Mannings Zeit im Milit\xe4rgef\xe4ngnis in Quantico, Virginia
Die Verteidigung strebt eine Abweisung der Anklage aufgrund zu harter Haftbedingungen an
Dem Gefreiten der US-Armee wird vorgeworfen, tausende vertrauliche Dokumente entwendet zu haben
Im Januar 2011 erhob Mannings Anwalt formell Einspruch gegen die Behandlung Mannings.
Navarrette ist der Ansicht, dass mexikanische Amerikaner zwischen zwei Welten gefangen sind
Wenn unsere Familien nicht in Mexiko gescheitert w\xe4ren, w\xe4ren sie nicht gegangen.
W\xe4hrend sie US-amerikanische Staatsb\xfcrgerin ist, sieht sie sich als Teil zweier L\xe4nder.
Man genie\xdft das Beste beider Welten, doch ist in keiner davon verwurzelt.
Die neuesten blutigen Ereignisse scheinen eine solche Hoffnung im Keim zu ersticken.
Warum auch diese hinterlistigen Pal\xe4stinenser verh\xe4tscheln und ihnen einen eigenen Staat \xfcberlassen?
Der Verteidigungsetat Israels ist gr\xf6\xdfer als der seiner vier arabischen Nachbarn zusammen.
Auch Obama muss seinen Teil dazu beitragen, Israel zu Verhandlungen zu bewegen.
Die Vereinigten Staaten haben ein wesentliches Interesse an einem stabilen Nahen Osten.
Aber immer mehr Akademiker und Kindesentwicklungsexperten f\xfchren Langeweile als etwas Positives an.
Und dann ist da noch die Frage, wie wir Langeweile eigentlich definieren.
"Wir haben keinen echten Pr\xe4zedenzfall, dem wir folgen k\xf6nnen", f\xfcgt er hinzu.
In meinen ersten Wochen in Oxford geh\xf6rte ich einer solchen Minderheit an.
Sollte ich mich der Labour-Partei zuwenden und meine nat\xfcrlichen Neigungen unterdr\xfccken m\xfcssen?
"Aber es ist der beste Ort auf der Welt", sagte er kleinlaut.
Ersch\xf6pft durch meine h\xe4ufigen Reisen nach London wurde mein emotionaler Widerstand schw\xe4cher.
Zu jener Zeit schrieb er pro Woche zwei Kolumnen in der Murdoch-Presse.
Auch das argentinische Modell Valeria Mazza vergisst das Charisma des Modemachers nicht.
"Es war ein wahr gewordener Traum", sagt die Witwe von Rodrigo d'Arenberg.
Wie wird diese Definition auf seinen Alltag und die sozialen Netzwerke angewendet?
Darunter auch die Mutter, die das Passwort zu einem der Konten hat.
Dem Jungen sind Erfahrungen nicht unbekannt, die man heute als Cyberbullying kennt.
"Ihnen zu sagen, sie sollen es nicht tun, funktioniert nicht", sagt er.
"Beispielsweise das Alter, oder was man teilen oder ver\xf6ffentlichen darf" erkl\xe4rt er.
Ursache f\xfcr ein Sterben wegen Aids ist heute eine zu sp\xe4te Erkennung
Fabrizio war 21 Jahre alt, als man ihm das Untersuchungsergebnis best\xe4tigte: HIV-positiv.
- Meiner Meinung nach ist das Problem nicht der Zugang zur Behandlung.
Seine Nachricht ist eine Zusammenfassung des Kampfs gegen AIDS im Jahr 2012.
Niemand in Puerto Rico hat auf dieser Ebene so dominiert wie Picul\xedn.
Was glaubst du ist das Beste, was du im Verband erreicht hast?
Dort lernte er die junge Designerin Maj Axelsson kennen und heiratete sie.
Indiana war der erste Bundesstaat, der eine derartige Forderung erhoben hat.
Die republikanischen Beh\xf6rden beeilten sich, diese Praxis auf andere Staaten auszudehnen.
Diese Ma\xdfnahmen zielen deutlich darauf ab, die hispanischen Stimmen zu begrenzen.
Der Generalanwalt der USA hat eingegriffen, um die umstrittensten Gesetze auszusetzen.
Die Organisation empfiehlt ebenfalls, den Verzehr von rotem Fleisch zu begrenzen.
Nach der kanadischen Krebsgesellschaft sind die Studien zu Vitamin E widerspr\xfcchlich.
Davon ausgehend teilen die Physiker die Teilchen in zwei Kategorien ein.
In die Kindheitsphase zur\xfcckzukehren ist f\xfcr gewisse Personen eine unannehmbare Dem\xfctigung.
Aber durch die Krankheit habe ich meine Kinder wirklich kennen gelernt.
In Quebec kommt auf 11.700 Einwohner ein Bett f\xfcr die Palliativpflege.
Die Realisierung dieses Berichts war m\xf6glich aufgrund eines Journalismusstipendiums kanadischer Gesundheitsforschungsinstitute.
In dieser Saison haben Sie mit PSG ein neues Ausma\xdf angenommen.
Diese Elemente spornen mich tagt\xe4glich dazu an, mein Spielniveau zu verbessern.
Sie machen sich somit die von Carlo Ancelotti eingef\xfchrte Konkurrenz zunutze...
\xdcbrigens gibt mir Carlo Ancelotti viel in Bezug auf meine Spielposition.
Was denken Sie \xfcber den ersten Teil der Saison des PSG?
Kann der PSG auf kurze Sicht ein gro\xdfer europ\xe4ischer Verein werden?
Dieses Jahr liegt es uns wirklich am Herzen, diesen Titel abzusahnen.
Wie haben Sie die EM 2012 mit der franz\xf6sischen Nationalmannschaft erlebt?
Ich habe dort Dinge gesehen, aus denen ich gest\xe4rkt hervorgegangen bin.
Heute gelingt es mir, gute Spiele in der Nationalmannschaft zu verwirklichen.
Wir haben eine gute Position in der Qualifikationsgruppe f\xfcr die WM.
Ich hoffe, dass Didier Deschamps die "Bleus" nach Brasilien f\xfchren wird.
Mit 15.000 Computern im Netzwerk wurden bereits etwa 200.000 Transaktionen erfasst.
Auf diese Weise kann das Netzwerk die Authentizit\xe4t der Transaktion pr\xfcfen.
Franz\xf6sische Truppen haben ihren Verantwortungsbereich in Afghanistan (Kapisa und Surobi) verlassen.
Alles wird importiert; abgesehen von Obst und Gem\xfcse wird nichts produziert.
Welches Souvenir lassen wir nach Milit\xe4rausgaben von zwei Milliarden Euro zur\xfcck?
Es handelt sich um ein neues Pokerspiel von Pr\xe4sident Mohammed Mursi.
Vertreter von Menschenrechtsorganisationen, religi\xf6sen Minderheiten oder der Zivilgesellschaft haben gleicherma\xdfen gehandelt.
Es ist nicht \xfcberraschend, dass die Artikel meistens einstimmig verabschiedet wurden.
Denn ihnen zufolge erfolgt die Islamisierung der Verfassung \xfcber andere Artikel.
Einer alten Legende zufolge lebten angeblich heidnische G\xf6tter auf dem Berggipfel.
Abends sieht man sie sogar schlafend auf den D\xe4chern parkender Autos.
Die Katzen m\xf6gen belebte Pl\xe4tze und sagen nicht Nein zu Leckereien.
Auf Probleme sto\xdfen Migranten ohne Beruf, Bildung, Sprachkenntnisse und \xe4rztliche Begutachtung.
Das russische Innenministerium plant eine Versch\xe4rfung des Waffengesetzes f\xfcr private Waffenbesitzer.
Besonders viele Pistolen und Gewehre kommen aus armen L\xe4ndern wie Kirgisien.
Es werden weder irgendwelche Papiere ben\xf6tigt noch gibt es pers\xf6nliche Treffen.
Die Waffe wird in milit\xe4rischen Waffenlagern von Aufsehern mittleren Ranges ausgegeben.
Die Proteste werden von Gewerkschaften und mehreren linksgerichteten gemeinn\xfctzigen Organisationen unterst\xfctzt.
Das sind ca. 1,1% mehr als sie jetzt f\xfcr Lohn spenden.
- Nicht unbedingt, aber es geht hier um eine gegenseitige Ann\xe4herung.
Der neue Held von Rosbalt ist der extravagante K\xfcnstler Kirill Miller.
Als die Gruppe anfing, live zu spielen, wurde aus ihr "Leningrad".
Jetzt gibt es Mikrogemeinschaften, und es ist schwierig, allen zu gefallen.
- Zu den Auftritten von Stas Michailow kommen aber mehrere Tausend!
Jedoch werden sich auf dem Biosatelliten "Bion" nur gleichgeschlechtliche Spezies befinden.
Wird sie nach diesem Flug ein Kind zur Welt bringen k\xf6nnen?
Der BRH darf nur Bundesmittel kontrollieren, was unseren staatlichen Mitteln entspricht.
Ist es dann aber sinnvoll, das Gesetz noch strenger zu machen?
Ein solches System setzt lediglich die B\xfcrokratie unter noch gr\xf6\xdferen Druck.
Auf den Stra\xdfen herrscht vereinzelt Eisgl\xe4tte, \xfcberwiegend sind sie jedoch trocken.
Auf den K\xe4mmen des Erzgebirges liegen jedoch etwa 30 cm Schnee.
Welchem Zweck kommt der Erl\xf6s der Konzerte gegen den Weltuntergang zugute?
Wir wollten ein Programm zusammenstellen, das alle Generationen einschlie\xdflich Kinder anspricht.
Sogar in Moskau, wo wir unl\xe4ngst waren, gab es keine Probleme.
Wie viele davon waren von Anfang an, d.h. seit 1998 dabei?
Die Rakete war 1,4 m lang und wog ungef\xe4hr 11,5 kg.
Hier dr\xe4ngt sich naturgem\xe4\xdf die Frage auf, woher dieses Kapital kommt?
Denn es ist eines Menschen Zahl, und seine Zahl ist sechshundertsechsundsechzig."
Unmittelbar vor der Besetzung der Botschaft gelang sechs Botschaftsmitarbeitern die Flucht.
Diese endete nach zahlreichen Komplikationen in der Residenz des kanadischen Botschafters.
Daf\xfcr brauche ich m\xf6glichst viel Einfluss und ein m\xf6glichst starkes Mandat.
Aber best\xe4tigen Sie das nicht dadurch, was Sie gerade gesagt haben?
Und die Angesprochenen m\xfcssten dann ggf. sagen, warum sie dies ablehnen.
Die Leute wollen mich als Samariter sehen, der die Republik rettet.
Aber ich frage mich, wof\xfcr wir heute noch eine B\xfccherei brauchen.
Kein Mensch geht heute noch freiwillig in eine dieser Old-Style-Bibliotheken, oder?
Neun Jahre sp\xe4ter ist der 30 Millionen Euro teure Berg aufgesch\xfcttet.
"Nichts ist schlimmer als eine halbleere Bibliothek", sagt Architekt Winy Maas.
Ich glaube, genau das macht es so schwierig f\xfcr die Deutschen.
"Die Marke wird verw\xe4ssert, die Alleinstellung verschwindet, der Imageschaden ist enorm."
Dennoch warten in dem Amt immer noch 81.500 Einspr\xfcche auf Erledigung.
Das Markenamt CTMO wies den Einspruch der M\xfcnchner denn auch zur\xfcck.
"Daran sieht man, wie viel uns das wert ist", sagt Wentzler.
Die Geschichte einer Verbindung, die weit mehr als 8733 Kilometer \xfcberwindet.
Die Bantusprache flie\xdfend sprechen kann in diesem Raum niemand, aber singen.
H\xe4ufige virale STI sind HIV, Humane Pappilomaviren, Herpes genitalis oder Hepatitis.
Unter Jugendlichen treten Chlamydien-Infektionen wesentlich h\xe4ufiger auf als bei anderen Bev\xf6lkerungsgruppen.
Daher empfehlen Experten vor allem bei h\xe4ufig wechselnden Sexpartnern regelm\xe4\xdfige Untersuchungen.
Fr\xfch diagnostiziert k\xf6nnen die meisten STI geheilt und Sp\xe4tfolgen vermieden werden.
Aber auch den vielen Wanderarbeitern, die das Virus durchs Land tragen.
"Geht nach Esitjeni, da ist das Licht" sagen die Menschen dort.
Der Spiegel, hier im Bild, hatte einen Durchschnitt von f\xfcnf Metern.
Die wichtigsten Eindr\xfccke aus dem All liefert jedoch das Weltraumteleskop Hubble.
Zurzeit gibt es 20 Personen, die \xe4lter als 100 Jahre sind.
Dann erz\xe4hlt sie von ihrem Mann, der in der Armee war.
Am schlimmsten war es in der Zeit nach dem Zweiten Weltkrieg.
Sie leben inmitten der Gro\xdffamilie, werden geliebt, umsorgt und sind gl\xfccklich.
Die k\xfcnftige Verfassung mit der Scharia als Basis ist heftig umstritten.
Angst vor einem Gottesstaat am Nil von Gnaden der m\xe4chtigen Muslimbruderschaft.
Die Opposition formiert sich seit Wochen gegen die \xdcbermacht der Islamisten.
"Mansche Leute m\xf6gen den Aquavit mehr als den Rakfisk", sagt Havard.
Stattdessen bezieht man sich nur auf den "Vorfall vom 22. Juli".
Ihr Englisch ist genau wie das der meisten Menschen hier makellos.
Aber vielleicht ist es doch der strenge Dunst des ganzen Fischs.
Und die Probleme in der Gemeinde sind von entscheidend urbaner Natur.
Doch ihre Familie glaubt, dass sie von ihrem Lebensgef\xe4hrten ermordet wurde.
Die Staatsanwaltschaft behauptet: Bradley Manning habe sich nicht \xfcber Misshandlung beschwert
Viele Menschen seien aufgrund der fehlenden Chancen gezwungen, Mexiko zu verlassen
Mexikos Verh\xe4ltnis zu den Vereinigten Staaten ist kompliziert und voller Ressentiment.
Wir sind die Nachkommen dieser Menschen, und unsere Treue gilt ihnen.
W\xe4hrend seiner ersten Amtszeit vers\xe4umte er die Vorstellung seines eigenen Friedensplans.
Bei der Apathie hingegen gebe es keinen Drang, etwas zu tun.
Doch nur 3% der Eltern gaben an, sich gelangweilt zu f\xfchlen.
In Colorado gibt es keine klare Leitlinie f\xfcr das neue Marihuanagesetz
Und auch Regulierungsbeh\xf6rden im Bundesstaat Washington kratzen sich ratlos am Kopf.
Petronella Wyatt: Ich wurde aus Oxford gemobbt, weil ich Tory bin
W\xe4hrend seiner Zeit in den Vierzigern waren alle politischen Ansichten akzeptiert.
Selbst meine kommunistischen Freunde legten stets einwandfreie Manieren an den Tag.
"Ich liebe diesen Palast", sagt er mit seinem unverwechselbaren italienischen Akzent.
In den Adel verliebt zu sein, muss nicht von Nachteil sein.
Der schwierigste Beruf der Welt: die menschlichen Arbeitstiere von Kawah Ijen
Wer dieses Thema nicht leicht nimmt, ist die Regierung von Singapur.
Auf FB lade ich sch\xf6ne Bilder oder Bilder von Spielen hoch.
Auch wenn ihm jemand einen Fremden empf\xe4hle, w\xfcrde er dies ignorieren.
Abschluss des Gipfeltreffens der Unasur ohne Ver\xf6ffentlichung der Erkl\xe4rung von Lima
Ebenso nahm das Abschlussdokument Bezug auf die politische Lage in Paraguay.
"S\xfcdamerika muss bei der Integration der B\xfcrger lernen", sagt Rafael Correa
"Das w\xfcrde die Gesundheit von jedem Menschen beeintr\xe4chtigen", f\xfcgte er hinzu.
Heute ist es m\xf6glich, dieses Syndrom auch mit Lebensqualit\xe4t zu \xfcberleben.
Wie Sie wissen, ist Azc\xe1rraga Andrade der Hauptaktion\xe4r der Hotelkette Posadas.
Von den Jungen gef\xe4llt mir die Arbeit von Leo Arill gut.
Die Studenten ihrerseits versichern, dass der Kurs zu den Interessantesten z\xe4hlt.
Arizona war der erste Bundesstaat, der eine derartige Forderung einf\xfchrte.
Mehrere Gesetzesentw\xfcrfe wurden durch die Vetos der demokratischen Gouverneure blockiert.
Es gibt Krebsarten, die aggressiv und andere, die indolent sind.
Das Rauchen ist verantwortlich f\xfcr 85% der F\xe4lle von Lungenkrebs.
Allerdings wurden beim CERN derartige Abweichungen bis jetzt nicht gefunden.
Palliativpflege - der beste Weg zu sterben... | Le Devoir
Allerdings bleibt in diesem wichtigen Themenbereich noch viel zu tun.
"Wir helfen Angeh\xf6rigen und Patienten gleicherma\xdfen", berichtet Pflegedirektorin Nathalie Savard.
Allerdings hatte sie mir gesagt, dass ich am Ende sei!
Ich denke, dass er in Paris weitere Titel gewinnen wird.
Im Januar habe ich ein ermutigendes Gespr\xe4ch mit ihm gef\xfchrt.
Wir haben die Saison mit einer sehr starken Leistung beendet.
Denken Sie, dass die Medien zu viel vom PSG erwarten?
Das hei\xdft, dass Ibrahimovic leistungsstark ist und viele Tore schie\xdft.
Leider hat mich meine Verletzung daran gehindert, etwas Spielzeit herauszuschlagen.
Dies war seit meiner Taufe mit den "Bleus" meine Hoffnung.
Einige tausend Webseiten akzeptieren Bitcoin als Spende oder als Zahlungsmittel.
Das soziale Netzwerk Facebook hat ebenfalls ein derartiges System entwickelt.
Der Computer, der die Aufgabe gel\xf6st hat, erh\xe4lt 50 Bitcoins.
Das Leben des Netzwerks hat bereits H\xf6hen und Tiefen gehabt.
Die jungen Menschen haben den Krieg und seine Ideologien satt.
Der Abzug der franz\xf6sischen Kampftruppen wurde am 20. November abgeschlossen.
"Scheinheiligkeit" erwidern die Liberalen, die dies nur als Propagandaschlag ansehen.
Mit dieser Verfassung bleiben wir im Rahmen des b\xfcrgerlichen Staates.
Besuchen Sie den Fluss Jordan, in dem Jesus getauft wurde.
Vom Fu\xdf des Berges gelangen Sie dorthin mit einem Shuttlebus.
Bei nur einer Reise k\xf6nnen nicht alle davon besichtigt werden.
Im sorgf\xe4ltig restaurierten Theater werden heutzutage Abendkonzerte und Opern aufgef\xfchrt.
Gem\xe4\xdf j\xfcdischer Tradition wird in Israel samstags der Sabbat begangen.
In den Stra\xdfen israelischer St\xe4dte gibt es keine streunenden Hunde.
Ihre Rechte m\xfcssen jedoch bereits vor ihrer Abreise gesch\xfctzt werden.
Der Grund sind b\xfcrokratische H\xfcrden und nat\xfcrlich die sprachlichen Schwierigkeiten.
Au\xdferdem kostet die Legalisierung Geld: 12 bis 16 Tausend Rubel.
Einen Beitrag zum Schwarzmarkt leisten gem\xe4\xdf Baranez auch die Waffenhersteller.
Er bekam ein Fotoalbum, in dem "alles M\xf6gliche" abgebildet war.
"Ich f\xfchlte mich wie im Luxusladen", erinnert sich der Milit\xe4rangeh\xf6rige.
"Kaufe eine TT. Moskau", lautet die lakonische Anfrage von "Fedorenkow".
Sie forderten weiterhin die Bildung von Gewerkschaften in der Fast-Food-Branche.
- Beschreiben Sie bitte kurz, welche Forschungen Ihre Gruppe betreibt.
In einem Clown verwischt das alles und verliert seine Tragik.
- Heutzutage muss kommerzielle Kunst vorsichtig, r\xfccksichtsvoll und schmeichelhaft sein.
Konsum hat \xfcberhaupt keine Kultur, das ist etwas ganz anderes.
Doch nicht jeder von ihnen kann sich mit Kultur befassen.
Das Projekt wird aus Zusch\xfcssen der Stadt Sankt Petersburg finanziert
Bereits ein halbes Jahrhundert davor wurden Experimente mit Pflanzen durchgef\xfchrt.
Zehn Stunden sp\xe4ter stumpften die Instinkte der Neugeborenen vollst\xe4ndig ab.
Das Wertvollste, das die Menschheit besitzt, ist der weibliche Organismus.
Bisher ist die Geburt von Kindern im Weltall blo\xdfe Theorie.
Was die deutsche Gesetzgebung betrifft, ist die einfacher als unsere?
Liegt das vielleicht daran, dass dort die Pr\xfcfer besser sind?
Auf diesen Stra\xdfen verbleiben jedoch abschnittsweise vereiste oder ausgefahrene Schneereste.
Insbesondere in den h\xf6heren Lagen ist daher erh\xf6hte Aufmerksamkeit geboten.
Die Stra\xdfen I/43 und I/34 bei Svitavy sind chemisch behandelt.
Die Fahrbahnen der ersten Stra\xdfenklasse sind \xfcberwiegend trocken, jedoch durchgefroren.
In Nordb\xf6hmen melden die Stra\xdfenmeistereien gleich mehrere schlecht befahrbare Stra\xdfenabschnitte.
 \u2047 imon Ornest: Auf unseren Konzerten wollen wir positive Energie sammeln
Wir bem\xfchen uns, diese Leute intensiv in unsere Projekte einzubinden.
Es gibt noch viele Dinge, in denen wir hinterher h\xe4ngen...
Der Weg Polens in den Weltraum begann freilich viel fr\xfcher.
Beide Projekte befassten sich mit der milit\xe4rischen Nutzung des Raketenantriebs.
Die maximale Flugh\xf6he betrug bei allen drei Typen 37 km.
Die Aufhebung des Gesetzes \xfcber gemeinn\xfctzige Arbeiten ist keine L\xf6sung.
Diese Entscheidung rief in der \xd6ffentlichkeit eine lebhafte Diskussion hervor.
Diese Ideen stammten freilich nicht aus Br\xfcssel, sondern aus Prag.
Es geht mir nicht darum, Senator oder Pr\xe4sident zu sein.
Und damit kommen Sie in der Politik langfristig nicht weit.
Ich versuche, Verb\xfcndete f\xfcr meine Ansichten und Visionen zu finden.
Das klingt ein wenig, als ob Okamura Tschechien retten sollte.
Aber das h\xe4ngt nicht mit der H\xf6he des Gehalts zusammen.
So wird z.B. mein Stellvertreter im Fr\xfchjahr Gesch\xe4ftsf\xfchrer des Reiseb\xfcros.
Etwa 200.000 bis 400.000, und das ist auch weiterhin so.
Das vollst\xe4ndige Gespr\xe4ch finden Sie in der Samstagsausgabe von Pr\xe1vo.
Die 80.000-Einwohner-Gemeinde weist die niedrigste Bildungsrate der gesamten Niederlande auf.
Was bedeutet eine "normale" Au\xdfenpolitik denn konkret aus deutscher Sicht?
Vielleicht wird sich Deutschland damit sogar einen gewissen Respekt einspielen.
Es gibt in Europa verschiedene Meinungen zu der pal\xe4stinensischen Initiative.
Die USA dagegen haben sich klar f\xfcr ein Veto ausgesprochen.
Gibt es Meinungsverschiedenheiten zwischen den USA und vielen europ\xe4ischen Nationen?
"Markenschutz" in China: Wenn Puma und Armani pl\xf6tzlich chinesisch werden
Und selbst dann ist nicht klar, ob sie Recht bekommen.
Pattloch \xf6ffnet einen Ordner mit Eintragungen des Markenamts in Peking.
So sei der Bestand unbearbeiteter Einspruchsverfahren um 22 Prozent gesunken.
Oder wir werden im fraglichen Segment aus dem Markt gedr\xe4ngt.
Zu den bakteriellen STI z\xe4hlen Syphilis, Chlamydien und Tripper (Gonorrh\xf6).
Das ist etwa ein Zehntel weniger als im Jahr zuvor.
Die Eisdecke soll m\xf6glicherweise bis zu 20 Meter dick sein.
Das Spitzer-Teleskop der Nasa schoss diese Foto der galaktischen Geburtsstube.
Mit dem Teleskop kommen allerdings die Farben besser zur Geltung.
Eine der gr\xf6\xdften und sch\xe4rfsten Aufnahmen des Hubble-Teleskops: Die Whirlpool-Galaxie
Je nach Farbgebung werden Aufnahmen von Spiralgalaxien zu wahren Kunstwerken.
Diese Sternen-Geburt zeichnete das Hubble-Teleskop in der Spiralgalaxie M83 auf.
Dieses Bild wurde aus optischen und R\xf6ntgen-Aufnahmen verschiedener Teleskope zusammengef\xfcgt.
Im Bild sind die letzten Startvorbereitungen am Weltraumteleskop Kepler dokumentiert.
Der Prim\xe4rspiegel des Weltrauminfrarotteleskops hat einen Durchmesser von 6,5 Metern.
Im S\xfcden Aserbaidschans erreichen viele Menschen ein biblisch hohes Alter.
Im S\xfcden Aserbaidschans erreichen viele Menschen ein biblisch hohes Alter.
Das hier ist mein Gro\xdfvater, er wurde 120 Jahre alt.
Museumsdirektorin Fatulayeva dagegen glaubt, dass es an der Ern\xe4hrung liege.
Die Propaganda klingt seltsam aus dem Mund einer alten Frau.
Rivalisierende Kundgebungen in Kairo offenbaren die tiefe Spaltung des Landes.
Diese Gerichte dienten w\xe4hrend Mubaraks Herrschaft zur Unterdr\xfcckung von Oppositionellen.
Eine Mehrheit f\xfcr den Entwurf der Islamisten gilt als sicher.
Rakfisk aus Norwegen: Ist das der \xfcbelriechendste Fisch der Welt?
Wir sind ein - wie sagt man - umsichtiges Volk.
"Und nat\xfcrlich Rakfisk essen", f\xfcgt sie mit unbeschwertem Lachen hinzu.
Aber am Abend steht wieder der Stinkefisch auf dem Speiseplan.
Ein Mann f\xe4llt von seinem Stuhl, m\xf6glicherweise vom Aquavit \xfcberw\xe4ltigt.
Der offiziellen Version der Ereignisse zufolge beging Mariana 2010 Selbstmord.
Die Beamten stellten Manning Fragen und schrieben seine Antworten auf.
Ihrer Meinung nach ist unsere Existenz ein Symbol des Scheiterns.
Und in den Vereinigten Staaten werden wir als Mexikaner gesehen.
Und dazu geh\xf6rt ein Friedensabkommen zwischen Israel und den Pal\xe4stinensern.
Damit f\xfchrt Australien die weltweit strengsten Regelungen f\xfcr Tabakverpackungen ein.
Andere hingegen sagen, dass die Gesetze ihr Gesch\xe4ft angekurbelt haben.
Kanada war 2001 das erste Land, das fotografische Warnungen vorschrieb.
H\xe4rtere Gesetze werden in Gro\xdfbritannien, Neuseeland, S\xfcdafrika und Indien erwogen.
"Tats\xe4chlich hat die Langeweile eine sehr lange Geschichte", sagt er.
Nicht nur Universit\xe4tsstudenten von heute werden f\xfcr ihre Ansichten angegriffen
Ja, lief, denn ich litt unter systematischem Mobbing und Drohungen.
Als unglaublich sch\xfcchterne 18-J\xe4hrige war ich im September 1986 angekommen.
Der Hass auf die Konservative Partei hatte seinen H\xf6hepunkt erreicht.
Die meisten Tory-Erstsemester geben vor, Anh\xe4nger der Labour-Partei zu sein.
In einem \xf6rtlichen Pub versuchte ich sp\xe4ter, mich zu verstellen.
W\xfcrde ich Gleichgesinnte erst nach Einbruch der Dunkelheit treffen k\xf6nnen?
"Er war makellos; die Zeit hinterl\xe4sst keine Spuren an ihm".
Es handelt sich um das gr\xf6\xdfte Problem in diesem Land.
Der Bekannte einer Freundin wurde in einem sozialen Netzwerk erpresst.
Dies ist meine Meinung, und so ist in unserem Krankenhaus.
Alles ist anders, wenn du wei\xdft, dass du AIDS hast.
Einige denken, dass sie sterben werden, und m\xf6chten nichts h\xf6ren.
Es gibt 13.435 kumulierte F\xe4lle (12.158 AIDS und 1.317 HIV).
Zweibandige Karambole: ein Schlag f\xfcr Vitro und f\xfcr das Land.
Es sollte hei\xdfen "Hier ruht der ehrenwerte B\xfcrger J.R. Ewing".
Dies ist das einzige Gesch\xe4ft, das er nicht gewonnen hat.
Eine republikanische Strategie, um der Wiederwahl von Obama entgegenzutreten
Bei M\xe4nnern afro-amerikanischer Herkunft besteht ebenfalls ein h\xf6heres Risiko.
Leider gibt es kein Wundermittel zur Vorbeugung von Krebs.
Es ist auch ein Risikofaktor f\xfcr mehrere andere Krebsarten.
Sowohl auf Ebene des k\xf6rperlichen, emotionellen oder spirituellen Komforts.
Im Heim Victor-Gadbois ist kein Tag wie der andere.
Sie sagt, dass das Verfahren "schmerzhaft, aber positiv" sei.
Damals hatte ich mich gerade von einer Verletzungsserie erholt.
Was ist das Ziel des Vereins in diesem Wettbewerb?
Wir werden versuchen, so weit wie m\xf6glich zu kommen.
Um so besser, dass man von einer "Zlatan-Abh\xe4ngigkeit" spricht.
Dies spornt die Anderen an, ihr Spielniveau zu verbessern.
Es lag mir am Herzen, an dieser EM teilzunehmen.
Mit Bitcoin ist Bezahlen und Verkaufen ohne Bank m\xf6glich
Von Anderen wie der Blog-Plattform WordPress werden sie akzeptiert.
Die NATO und die USA d\xfcrften Ende 2014 folgen.
Das Ger\xfccht wurde verbreitet, dass Afghanistan immense Bodensch\xe4tze bes\xe4\xdfe.
Innerhalb von 14 Tagen sollte ein Referendum abgehalten werden.
Die Mehrheit der Liberalen ist der Aufforderung nicht nachgekommen.
Man kann hierin die ersten Anzeichen einer Theokratie sehen".
Dieses Wort war in der vorherigen Verfassung nicht enthalten.
Eben hier erschien Jesus seinen J\xfcngern nach der Auferstehung.
Nur Bergsteiger k\xf6nnen die Ruinen aus eigener Kraft erreichen.
Alle anderen bringt eine Luftseilbahn zu diesem historischen Gipfel.
Darunter ist einmal das Israel-Museum unweit der Knesset (Parlament).
Der Eintritt ist frei, und Spenden werden grunds\xe4tzlich abgelehnt.
Die Stadt wird in altgriechischen und alt\xe4gyptischen Legenden erw\xe4hnt.
Den Test m\xfcssen nur Migranten mit legalem Status ablegen.
Die gef\xe4lschten Papiere wurden mit einem gew\xf6hnlichen Farbdrucker gedruckt.
Die Waffen gelangen \xfcber mehrere Kan\xe4le auf den Schwarzmarkt.
Die Waffe wird ausgestellt und durch den Zaun \xfcbergeben.
K\xe4ufer und Verk\xe4ufer finden am h\xe4ufigsten \xfcber Bekannte zueinander.
Den Preis f\xfcr die Waffe erfuhr ich erst dort
Dort geben Benutzer Ihre Bestellungen auf und stellen Anfragen.
Bisher ist diese Branche der Wirtschaft kaum gewerkschaftlich organisiert.
Weniger als sie verdient niemand in dieser teuren Stadt.
Und zuallererst sollten wir diese bescheuerten Virtual-Reality-Helme los werden!
Mangelt es an Aufl\xf6sung, Tiefe oder noch etwas anderem?
- M\xfcsste die Anzahl der Kameras nicht erh\xf6ht werden?
Und die dritte Kamera ist tats\xe4chlich eine gew\xf6hnliche RGB-Kamera.
Oder das Problem verst\xe4rken, da mehr Berechnungen notwendig w\xe4ren.
Welche Antworten will Ihre Gruppe auf diesen Einwand geben?
Jede meiner vergangenen Provokationen war eine Einladung zum Gespr\xe4ch.
- Wann wusstest du, dass du Maler werden musst?
Trachtenberg moderierte viele Programme vor der Zeit von "Halli-Galli".
Ich liebe die Groteske, und ich habe groteske Ideen.
Jetzt musst du dir \xfcberlegen, wem du gefallen wirst.
Im Gegensatz zu Tieren k\xf6nnte der Mensch das prinzipiell.
Doch Frauen fliegen bereits seit 50 Jahren ins All.
"Schlie\xdflich beantwortete niemand diese Frage", sagt Raumfahrtveteran Wachtang Watschnadse.
Der Vater des Kindes, Andrijan Nikolajew, war ebenfalls Kosmonaut.
NK \u2047 -Chef: Kontrolle des Schwarz-Systems versagt durch Verschulden der Politik
Sagen wir zun\xe4chst einmal, welcher Weg nicht zielf\xfchrend ist.
Auf den Stra\xdfen Tschechiens besteht teilweise Schnee- und Eisgl\xe4tte.
Nach Angaben der Bezirksstra\xdfenwacht herrschte wegen Nebels eingeschr\xe4nkte Sicht.
"Im Kreis  \u2047 umperk verbleiben in den H\xf6henlagen noch Schneereste.
Eisgl\xe4tte wird insbesondere aus dem Umkreis von  \u2047 t \u2047 t\xed gemeldet.
Wie sind Sie zu der Zusammenarbeit mit beiden gekommen?
Bei jedem Konzert treten mehrere Gruppen und Interpreten auf.
Bislang sind dies nur Einzelf\xe4lle von besonders willensstarken Pers\xf6nlichkeiten.
Die Informationen hierzu stammen ausschlie\xdflich aus der zeitgen\xf6ssischen Presse.
Im Jahr 1962 jedoch wurde die weitere Entwicklung eingestellt.
Die Anzahl der Betroffenen geht bereits in die Millionen.
Der Film Argo: Wenn's am schlimmsten steht, Hollywood anrufen
"Wir sind dadurch benachteiligt, dass wir kein Meer haben.
Es missf\xe4llt Ihnen, wenn jemand Sie als Populisten bezeichnet.
Aber ohne Unterst\xfctzung im Parlament bleiben Ihnen nur Schlagw\xf6rter.
Denken Sie \xfcber die Gr\xfcndung einer eigenen Partei nach?
Mein Privatverm\xf6gen sch\xe4tze ich auf etwa 60 Mio. CZK.
Ich habe schon 2,5 Millionen in die Kampagne gesteckt.
Sagten Sie nicht, dass Sie diese Aktivit\xe4ten zur\xfcckfahren werden?
Als Pr\xe4sident w\xfcrde ich meine Unternehmungen jedoch ganz einstellen.
Jeder wei\xdf, dass sein Buch Teil dieses Geb\xe4udes ist.
Die Deutschen finden sich also zwischen den Fronten wider.
Aufgrund der amerikanischen Innenpolitik haben diese Verschiedenheiten immer existiert.
Die Deutschen werden einfach eine gr\xf6\xdfere Rolle spielen m\xfcssen.
Armani ist eine weltbekannte Marke, Polo Ralph Lauren ebenfalls.
Jede Woche landet ein neuer Fall auf meinem Schreibtisch.
Damit sind Frauen gemeint, die sich reiche M\xe4nner angeln.
"Das ist gesch\xe4ftssch\xe4digend, man muss es bek\xe4mpfen", fordert Pattloch.
Wie so oft in China sind die Zahlen beeindruckend.
2011 seien 1,8 Milliarden Yuan an Geb\xfchren eingenommen worden.
Jetzt ist die Angelegenheit vor dem Obersten Gerichtshof anh\xe4ngig.
Die Gefahren in Fernost drohen sogar nach Europa zur\xfcckzuschwappen.
Dann n\xe4mlich, wenn sich dort Imitatoren ungesch\xfctzte Marken sichern.
Sonst kann das viel teurer werden als die Registrierung.
Mehr als 40 Prozent der Bev\xf6lkerung sind inzwischen HIV-positiv.
Hierzulande kommen zudem Humane Pappilomaviren bei Jugendlichen h\xe4ufig vor.
Die Kultur ist eine andere - flesh to flesh."
Die acht Planeten unseres Sonnensystems, au\xdferdem der Zwergplanet Ceres.
Trotzdem erreicht er einen Durchmesser von etwa elf Metern.
Auch das Hobby-Eberly-Teleskop in Texas ist im H\xf6henwinkel fixiert.
T\xe4glich Butter trinken - und 168 Jahre alt werden
Die Fahrt durch das Talysch-Gebirge ist wildromantisch zu nennen.
Im Alter von 136 Jahren noch ein Kind gezeugt
Warum also leben hier im S\xfcden so viele Hochbetagte?
Auch problematisch: Die zivile Milit\xe4rgerichtsbarkeit soll weiter aufrechterhalten bleiben.
Doch ohne zivilgesellschaftliche Organisationen k\xf6nne eine Demokratie nicht funktionieren.
Man platziere sie inmitten eines Haufens schmutziger, feuchter Sportkleidung.
Wir sind nicht sehr angeberisch, wir m\xf6gen keine Prahlerei.
Aktuell ist der Verkehr in Mexiko-Stadt ganz besonders schlecht.
Das Material wurde dann von WikiLeaks im Internet ver\xf6ffentlicht.
WikiLeaks hat Manning als Quelle der Informationen nie best\xe4tigt.
Und die Kinder Montezumas begeben sich auf den Kriegspfad.
Die israelischen Hardliner hingegen lassen eine entgegengesetzte Schlussfolgerung ziehen.
Zumindest eine Weile lang wird Israel ruhiger schlafen k\xf6nnen.
Sollten wir die Langeweile also mit offenen Armen begr\xfc\xdfen?
Langeweile kann sich damit fast so anh\xf6ren wie Depression.
Aber im Allgemeinen sind Teenager ein ziemlich abgespannter Haufen.
F\xfcrsprecher der Legalisierungsbewegung hoffen, dass das Justizministerium nachgeben wird.
Ich kehrte mit h\xe4ngendem Kopf in mein Zimmer zur\xfcck.
Jeder, der verd\xe4chtigt wird, Tory zu sein, wird drangsaliert.
"Du wirst hier nicht gl\xfccklich werden", sagte er mir.
Es w\xfcrde mir das Herz brechen, wenn du gingst.
Valentino hat immer schon die Eleganz der Ber\xfchmtheit vorgezogen.
Ende der 90er Jahre kam es dann schlie\xdflich dazu.
So hat sie bereits auch Auswirkungen auf den Wohnungsmarkt.
"Er hat nie erfahren, wer es war", versichert er.
Laut Jos\xe9 hat das Opfer das Benutzerkonto nicht geschlossen.
"Aber ich wei\xdf, dass dies Cyberbullying ist" erkl\xe4rt er.
Peru hat den Vorsitz auf Zeit des regionalen Blocks.
Heute wissen seine Eltern nur, dass er Krebs hatte.
Ich lebe ein normales Leben, wie jeder andere auch.
Zu den Risikopersonen f\xfcr neue Infektionen z\xe4hlen die Jugendlichen.
Allerdings wird diese M\xf6glichkeit von den mexikanischen Gesetzen anerkannt.
Die Abstimmung w\xe4re 45 Prozent gegen 37 Prozent ausgegangen.
Die entsprechenden Investitionen liegen bei \xfcber 1,5 Milliarden Dollar.
Seine Zahlen auf Ebene der internationalen Turniere sind beeindruckend.
Heute machen die Kinder unn\xf6tig viele Reisen und Spiele.
Damit erreichte die Serie einen Zuschauerrekord in jener Zeit.
Beginn der Kurses, der das "Ende der Welt" studiert
Dies ist haupts\xe4chlich in der englischsprechenden Welt der Fall.
Prostatakrebsfr\xfcherkennung: sollte der Test gemacht werden oder nicht?
Wir haben die Meinung von zwei Fach\xe4rzten eingeholt.
Deshalb empfehle ich trotzdem die Durchf\xfchrung des Tests.
"Die Durchf\xfchrung eines Fr\xfcherkennungstest f\xfchrt nicht zu Krebs."
Sie sahen wissenschaftliche Anwendungen, aber sonst nichts weiter.
Le Devoir hat versucht, dies n\xe4her zu betrachten.
Sie haben eine maximale Lebenserwartung von drei Monaten.
Die Diabetiker m\xfcssen ihren Blutzuckerspiegel nicht mehr kontrollieren.
Kanalisationsvertr\xe4ge, deren Kosten von ihm k\xfcnstlich aufgebl\xe4ht wurden
In Montreal funktionierte das "System" der Korruption reibungslos.
Das technische Personal hat mir ebenfalls viel gegeben.
Und bei einem Spiel ist dies noch einfacher.
Sie wissen auch, dass jede Trainingseinheit ausschlaggebend ist.
Ist Ancelotti die richtige Person f\xfcr die Aufgabe?
In der letzten Saison waren wir dicht dran.
Normalerweise sollte man mit 79 Punkten Meister sein...
Ich glaube, dass dieses Jahr das richtige ist.
Man fragt sich, was die Leute noch erwarten.
Wir k\xf6nnten niemals jedes Wochenende mit 4-0 gewinnen.
Eine Mannschaft baut sich mit der Zeit auf.
In der Champions League haben wir St\xe4rke bewiesen.
Dies zeigt, dass die Ligue 1 spannend ist.
Er respektiert ebenfalls die Personen, die ihn umgeben.
Wichtige Akteure wie Wikipedia verweigern Spenden dieser Art.
"Derzeit ist kein konkretes religi\xf6ses Engagement zu erkennen.
Die meisten Heiligt\xfcmer finden sich jedoch in Jerusalem.
Die Skipisten haben eine Gesamtl\xe4nge von 45 Kilometern.
In diesem Land gibt es fast 300 Museen.
Die Versicherung kostet zus\xe4tzlich 15 Dollar pro Tag.
Eintrittskarten f\xfcr Museen kosten im Schnitt 30 Schekel.
"Es ist schwierig ohne Sprachkenntnisse", geben sie zu.
B\xfcrgerrechtler betonen bez\xfcglich des Gesetzes folgenden wichtigen Aspekt.
Lieferanten: von den Fabriken bis zu den Offizieren
Weitere illegal verkaufte Waffen stammen aus milit\xe4rischen Waffenlagern.
Bei vielen Milit\xe4rlagern kam es h\xe4ufig zu Explosionen.
Ein weiterer Kanal des Schwarzmarkts ist der Schmuggel.
Die Schemas haben sich ihm zufolge nicht ver\xe4ndert.
"Nat\xfcrlich ohne Lizenz", fragt Benutzer "Iwan" (w\xf6rtliches Zitat).
Der K\xe4ufer \xfcberweist das Geld \xfcber einen Bankautomaten.
Andererseits macht die Unternehmensf\xfchrung es ihnen nicht einfach.
"Das Gehirn l\xe4sst sich bisher nur m\xe4\xdfig \xfcberlisten"
- Was erwartet uns noch in der Zukunft?
Sie ist beliebt, aber wird sie nicht \xfcberbewertet?
- Oh, das w\xe4re sehr schwer zu erkennen.
- Haben Sie versucht, das Gehirn zu \xfcberlisten?
Ich begriff, dass ich diesen Weg gehen muss.
Auf unseren Steinen kann Kunst nur schwer heranwachsen.
Viele Auswahlm\xf6glichkeiten gibt es meiner Meinung nach nicht.
Ohne festen Untergrund \xfcberschlugen sich die K\xfcken wild.
Die K\xfcken reagierten nicht auf Licht und Laute.
Aus ethischen \xdcberlegungen werden solche Experimente nicht durchgef\xfchrt.
Na gut, umgehen wir das durch geburtseinleitende Hilfsmittel.
K\xf6nnen Sie unseren Lesern das Projekt n\xe4her vorstellen?
Alles weitere erfahren Sie auf der Internetseite www.kpks.cz.
Sind \xe4hnliche "Gro\xdfveranstaltungen" auch f\xfcr die Zukunft geplant?
Wie bew\xe4ltigen Sie diese Reisen logistisch und organisatorisch?
Im Showbusiness kopiert heute oft einer den anderen.
Danach wurden die Versionen Meteor-2H und Meteor-3 gebaut.
Dies \xe4u\xdfert sich insbesondere in \xc4nderungen geltender Gesetze.
Afflecks Film ist eine besondere Kombination mehrerer Filmgenres.
Kehren Sie dadurch nicht Ihren W\xe4hlern den R\xfccken?
F\xfcr mich ist dieses Rechts-Links-Denken aber v\xf6llig unwichtig.
Im Senat sind wir damit nur zwei Unabh\xe4ngige.
Sie sprechen von Verm\xf6genserkl\xe4rungen, wie s\xe4he Ihre aus?
Ich habe keine 15 Millionen f\xfcr die Kampagne.
Wie versprochen, habe ich meine Aktivit\xe4ten teilweise zur\xfcckgefahren.
Aber ich muss doch auch von etwas leben.
An welches Monatseinkommen waren Sie als Unternehmer gew\xf6hnt?
Der Erfolg der Bildungsoffensive hielt sich in Grenzen.
Nach 105 Stufen ist man am Gipfel angelangt.
So jung und ungebildet sie auch sein mag.
Das ist endlich mal ein Ansatzpunkt f\xfcr Identit\xe4t.
Eine Au\xdfenpolitik, wie sie Frankreich oder Gro\xdfbritannien haben.
Das machen sie ja gerade mit dem Euro.
Oder f\xe4llt Deutschland die F\xfchrungsrolle noch immer schwer?
Die Chinesen nennen das "Bang Mingpai", eine Beifahrermarke.
Die chinesischen Beh\xf6rden sind sich keiner Schuld bewusst
Die chinesischen Beh\xf6rden sind sich keiner Schuld bewusst.
23,5 Millionen Menschen davon leben im S\xfcden Afrikas.
Imbongi bedeutet auf Zulu Geschichtenerz\xe4hler oder auch Lobpreiser.
Filzl\xe4use und Kr\xe4tze geh\xf6ren zu den parasit\xe4ren STI.
Wie hat sich die Zahl der Infektionen entwickelt?
Die Zahl der HIV-Neuinfektionen geht seit 2007 zur\xfcck.
Er befindet sich 700 Lichtjahre entfernt im Aquarius-Sternbild.
In Arizona, USA, steht das Large Binocular Telescope.
Das Radioteleskop hat einen Durchmesser von 305 Metern.
Mit Bildern ist aber fr\xfchestens 2018 zu rechnen.
Hier ist es auf einer Illustration zu bestaunen.
"Shampoo habe ich auch nie benutzt", sagt Mirzayeva.
Immerhin gibt es keine Not unter Aserbaidschans Alten.
Im Klartext bedeutet das nichts anderes als Zensur.
Das wollten Mursis Anh\xe4nger ganz offensichtlich nicht riskieren.
Mexikos Enrique Pena Nieto steht vor schwierigem Start
Ich dachte, ich w\xfcrde in diesem K\xe4fig sterben.
Ich f\xfcrchte, da m\xfcsst ihr alleine durch, Amigos.
Vielleicht wird dies nur zu mehr Blutvergie\xdfen f\xfchren.
Ein Krieg, der weder verloren noch gewonnen wird
Milit\xe4risch gesehen ist die Hamas keine Gefahr mehr.
Australische Gesetze f\xfcr einheitliche Zigarettenverpackungen treten in Kraft
Aber einige Personen langweilen sich leichter als andere.
Zur\xfcck also zu meiner Ursprungsfrage: Ist Langeweile gesund?
Ich glaube nicht, dass wir Langeweile zelebrieren sollten.
Auch sollten wir sie nicht zu kritisch sehen.
"Ich wei\xdf, wer du bist", sagte er freundlich.
Gerne k\xf6nnen Sie mich einen weinerlichen Schlappschwanz nennen.
Valentino ist ein spektakul\xe4rer, gro\xdfz\xfcgiger und eleganter Gastgeber.
Also warum bekommen die Singapurer nicht mehr Kinder?
Was ist privat f\xfcr jemanden unter 16 Jahren?
Ich vertreibe mir auch meine Zeit mit Bekannten.
Wei\xdft du, was die anderen \xfcber dich ver\xf6ffentlichen?
- Warum sterben also noch immer Menschen daran?
Wer war der beste Spieler von Puerto Rico?
Wer war der beste Trainer aus Puerto Rico?
"Anderenorts denken die Leute nicht so", sagt er.
Sollte der Test gemacht werden oder nicht?
Es sch\xe4digt stark die Gesundheit der Menschen.
Ihre Untersuchungen sind aber derzeit nicht schl\xfcssig.
"Ich habe gute Kinder", f\xfcgt sie hinzu.
Und der Tod ist Teil des Alltags.
Eine 2011 ins Leben gerufene, permanente Antikorruptionseinheit
T\xe4glich mache ich an ihrer Seite Fortschritte.
Aber ich breche nicht in Begeisterung aus.
Was er geleistet hat, ist wirklich au\xdfergew\xf6hnlich.
Jeder hat sich f\xfcr alle anderen eingesetzt.
Allerdings weist Bargeld ebenfalls diesen M\xe4ngel auf.
Der privaten Initiative wird der Vorrang gelassen.
Eine Verfassung mit der Brechstange in \xc4gypten
Ein weiterer Streitpunkt: die Befugnisse der Armee.
Die Bef\xfcrworter des Staatsoberhauptes werden Samstag aufmarschieren.
Dort gibt es weder Museumsf\xfchrer noch Souvenirl\xe4den.
Beim Betreten des Raumes herrscht v\xf6llige Dunkelheit.
Genau genommen ist es eine unterirdische Standseilbahn.
Und Fahrradverleih kostet 15 Schekel pro Tag.
Uns erreichen viele Beschwerden von unseren Migranten.
"Herzlich willkommen" oder "Zutritt f\xfcr Unbefugte verboten"
"Blo\xdf keine Kosten f\xfcr falsche Papiere scheuen"
Anteil legaler Waffen an Straftaten \xe4u\xdferst gering
Neulinge suchen nach Waffen auf verschiedenen Wegen.
Man muss warten bis zu eineinhalb Monaten.
In den USA streiken Fast-Food- und Supermarkt-Besch\xe4ftigte
Jumaane Williams, Mitglied des New Yorker Stadtrats
Der wichtigste Grund ist die hohe Personalfluktuation.
Sie sagen es und deuten gleichzeitig darauf.
- Normalerweise sage ich es einfach nur.
Sie dient nicht zur Berechnung der Objekttiefe.
Mehr Kameras k\xf6nnten m\xf6glicherweise das Problem l\xf6sen...
- Deine Arbeiten haben einen unverkennbaren Stil.
- Kann auch kommerzielle Kunst sch\xf6n sein?
Ich bin keine Einhundert-Dollar-Note, die jedem gef\xe4llt.
Jetzt hat jeder Kultstar ungef\xe4hr 100 Anh\xe4nger.
Das ist die Kultur, die ich bef\xfcrworte.
In Moskau gibt es gegenw\xe4rtig gute Berater.
Es entwickelt sich ein ganz normales K\xfcken.
Vier Tage sp\xe4ter starben sie dann einfach.
Im Fr\xfchjahr 2013 werden die Experimente fortgesetzt.
Nach der Landung bekamen die Weltraumratten Nachwuchs.
Das gr\xf6\xdfte Risiko gab es bei Tereschkowa.
Andererseits braucht das Kind ebenfalls k\xfcnstliche Schwerkraft.
Ist das Schwarz-System nun verboten oder erlaubt?
Nach welchen Kriterien haben Sie diese ausgesucht?
Wie haben Sie diese Dinge bisher erlebt?
Dies ist meines Erachtens aber v\xf6llig normal.
Derzeit hat The Tap Tap zwanzig Mitglieder.
Diese Gesetzentw\xfcrfe werden anschlie\xdfend im Bundestag verabschiedet.
Terroristische Angriffe gab es auf beiden Seiten.
Zu viel Handlung an zu vielen Orten
Kuriose Einf\xe4lle gibt es auch zu Hause
Ich hatte keine Ambitionen, Politiker zu werden.
F\xfcr mich ist wichtig, dass wir weiterkommen.
Und wenn es nur zur Zierde ist.
Diese wurde schlie\xdflich von der NATO durchgesetzt.
Das spielt auf jeden Fall eine Rolle.
Das war immer schon ein empfindliches Thema.
Das macht es den Deutschen nicht einfach.
Das Wort orientiert sich an "Bang Dakuan".
Manchmal herrscht hier das Gesetz des Dschungels.
70 von ihnen besuchen eine weiterf\xfchrende Schule.
Was sind die wichtigsten sexuell \xfcbertragbaren Krankheiten?
Nicht alle sexuell \xfcbertragbaren Krankheiten sind meldepflichtig.
Welche Symptome weisen auf eine Geschlechtskrankheit hin?
Messenger: NASA entdeckt Eis auf dem Merkur
Die gr\xf6\xdfere Spiralgalaxie nennen Wissenschaftler UGC 1810.
Unsere Einblicke ins All: Die wichtigsten Teleskope
Es gibt sogar ein Museum f\xfcr Langlebigkeit.
Es gibt sogar ein Museum f\xfcr Langlebigkeit.
Das Wort "Menschenrecht" fehlt in der Verfassung
Der \xe4gyptische Pr\xe4sident sparte nicht mit Pathos.
"Das Wort Menschenrechte kommt nicht einmal vor"
Das Spektakel \xe4hnelt dem Eurovision Song Contest.
In Mexiko werden wir als Amerikaner gesehen.
Vielleicht sind wir "mexikanischer", als ich dachte.
Beide Seiten ben\xf6tigen einen Ansto\xdf von au\xdfen
Doch das ist eine bedauerliche, kurzsichtige Perspektive.
Die Tabaklobby k\xe4mpfte hart gegen die Gesetze.
F\xfcr uns ist das ein gutes Gesch\xe4ft.
Eine WTO-Entscheidung wird f\xfcr Mitte 2013 erwartet.
"Wir werden wie Kriminelle behandelt", so Orozco.
Unsere Gemeinde hat gegen diese Gesetzes\xe4nderung gestimmt.
Die Atmosph\xe4re h\xe4tte sogar Stalinisten aufschrecken lassen.
Dieser Trick sollte sich als erfolglos erweisen.
"Wie haben Tories Sex?", fragte mich einer.
Ich bin sicher, man neckt dich nur.
Valeria Mazza, in einem Kleid von Valentino
Singapur braucht Babys zur Rettung der Wirtschaft
Das offline Private offline ist online privat
Der Fall des 14-j\xe4hrigen Jos\xe9 liegt anders.
Es soll nicht die Promiskuit\xe4t gef\xf6rdert werden.
H\xe9ctor "Hetin" Reyes: "Basketball war mein Leben"
Er machte allen Freude, die ihn kannten.
Studenten und Professoren nehmen dieses Datum leicht.
Diese Einschr\xe4nkungen sind nicht ohne Folgen.
Gleiches gilt f\xfcr die hispanische Bev\xf6lkerung.
Sie konnten die Sch\xe4den teilweise begrenzen.
Um das Sterben angenehmer zu gestalten.
"PSG ist nicht der FC Barcelona!"
Im Fu\xdfball geht alles sehr schnell.
Ancelotti fl\xf6\xdft allen Technikern Respekt ein.
Er hatte Kontakt mit gro\xdfen Spielern.
Von nun an ist alles m\xf6glich.
Er hat bereits das Budget daf\xfcr...
Dies ist heute nicht der Fall.
Nat\xfcrlich w\xe4re dies eine gro\xdfe Entt\xe4uschung.
Wir haben mit 79 Punkten abgeschlossen.
Wir sind nicht der FC Barcelona!
Wie es auch Laurent Blanc war.
Aber ich m\xf6chte keinen Vergleich anstellen.
Dieses Spiel hat uns Zuversicht gegeben.
Im November wurde ein "Mega-Schlussverkauf" gestartet.
Einige stehen den Moslembr\xfcdern sehr nahe.
Eine Reise in die H\xf6he unternehmen
Auch die Ukraine wird dort erw\xe4hnt.
Die umliegende Landschaft ist unbeschreiblich sch\xf6n.
Und am Sonntagmorgen beginnt die Arbeitswoche.
Sinn, Problematik und Schutz der Rechte
"Du f\xfchlst dich erniedrigt und minderwertig."
Screenshot einer Webseite, die Waffenbestellungen annimmt
Milit\xe4rkommentator und ehemaliger Milit\xe4rangeh\xf6riger Viktor Baranez
Die Verantwortlichen nehmen die Bestellungen an.
- Was denken Sie \xfcber Sprachsteuerung?
Eigener Geschmack statt Kultur - rosbalt.ru
Dorthin gingen unsere Mitarbeiter und Stammg\xe4ste.
Die T\xe4uschung verschwindet durch das Verkleiden.
Wir sehen den Zerfall der Kulturen.
Es hei\xdft: geistige Kultur und Konsumkultur.
Jetzt z\xe4hlt nur der eigene Geschmack.
- Was ist f\xfcr dich Petersburg?
Bei uns sind das viel weniger.
Prinzipiell wurde dabei nichts Besonderes festgestellt.
Das Wasser stellt die Schwerelosigkeit dar.
Wie funktioniert das Kontrollsystem in Deutschland?
Meines Erachtens nicht auf diese Weise.
Diese Angaben stammen von den Bezirksstra\xdfenmeistereien.
Bezirk  \u2047 st\xed nad Labem, Bezirk Liberec
Hier ist die eindeutige Antwort: Ja.
Viel wird nicht \xfcber sie geschrieben.
Begeisterung weckt er jedoch nur schwer.
Bananen m\xfcssen 14 cm lang sein
EU: Bizarre Verordnungen sind die Ausnahme
Wie wollen Sie dieses Problem l\xf6sen?
Und diesem m\xf6chten Sie sich n\xe4hern.
Alle haben Internet, iPad und E-Books.
Der erste Eindruck: B\xfcchereldorado unter K\xe4seglocke.
Optik, Haptik und Geruch sind fremd.
Geheizt und gek\xfchlt wird mit Erdw\xe4rme.
Auch Lisette Verhaig war schon da.
Die Regale sind bis obenhin gef\xfcllt.
Szabo: "Deutsche m\xfcssen gr\xf6\xdfere Rolle spielen"
Ber\xfchmte F\xe4lle betreffen auch grafische Elemente.
"Man muss h\xf6llisch aufpassen", sagt Wentzler.
2011 gab es rund 2700 F\xe4lle.
Die Sternenwiege produziert immer neue Youngster.
Eine Geburtsurkunde gibt es allerdings nicht.
Die Revolution ist nach Kairo zur\xfcckgekehrt.
Daf\xfcr wurde er verpr\xfcgelt, verurteilt, inhaftiert.
Man nehme eine Auswahl \xfcberreifer K\xe4sesorten.
Und belasse sie dort eine Woche.
Die Spirituose kann den Geruch verdr\xe4ngen.
Er steht vor einer komplexen Aufgabe.
Sp\xe4ter entschied ich mich f\xfcr "Mexikanisch-Amerikanisch".
Diese gilt eindeutig den Vereinigten Staaten.
Viele australische Raucher zeigen sich trotzig.
Darauf komme ich noch einmal zur\xfcck.
Mein Vater brach in Tr\xe4nen zusammen.
Die Wahrheit aber war weniger am\xfcsant.
Warum erw\xe4hne ich dies gerade jetzt?
In meinen Augen wallten Tr\xe4nen auf.
Leider ist es, wie es ist.
Die Erleichterung dauerte nur kurz an.
"Valentino zieht Eleganz der Ber\xfchmtheit vor"
Und dennoch ist er ein Star.
Naty Abascal und der Modemacher, 2006
Ich kann mich noch perfekt erinnern.
"Die Bev\xf6lkerung von Singapur muss wachsen."
Aber alles hatte bisher wenig Erfolg.
Sie bedrohten ihn und verlangten Geld.
"Er hat es nur privat gemacht."
Gegenw\xe4rtig wird dieses Urteil nicht umgesetzt.
Dies gilt auch, wenn wir verlieren.
Er versteckte es vor seiner Familie.
Damals war AIDS Synonym f\xfcr Tod.
Und das Wichtigste ist die Vorbeugung.
Dies wird vom Berufungsgericht nicht ber\xfccksichtigt.
Reyes \xfcbertreibt mit dieser Aussage nicht.
Das war ohne Zweifel Picul\xedn Ortiz.
Was bleibt dir noch zu tun?
Das Internet hat diese Spekulationen erh\xf6ht.
Wir haben eine Begnadigung vom Papst.
Mehrere bleiben auch v\xf6llig ungekl\xe4rt.
Wurstwaren sollten ebenfalls gemieden werden.
Der Mut des gew\xf6hnlichen Todes.
Problem des Zugangs zur Palliativpflege
Immobilienskandale gro\xdfen Ausma\xdfes in Quebec
70% Schwarzgeld in den Wahlkampagnen
Wie erkl\xe4ren Sie diesen Fortschritt?
Wir lauern aber im Hinterhalt.
Wir versuchen, ein Spielkonzept aufzustellen.
Er hat vielversprechende Ergebnisse erreicht.
Wir sind aus Afghanistan abgezogen.
Eine Armee ist jetzt vorhanden.
Vor den heiligen St\xe4tten verbeugen
Etwas f\xfcr die Gesundheit tun
Die Geheimnisse des Altertums ber\xfchren
Wird auch an Minderj\xe4hrige verkauft?
Eine Makarow f\xfcr 100 US-Dollar
Die H\xe4nde sp\xfcren \xfcberhaupt nichts!
Sie nimmt Druck hervorragend wahr!
Heutzutage gibt es oft Missverst\xe4ndnisse.
- Kirill, was fehlt Petersburg?
Man sagt: Diener der Kultur.
Erderw\xe4rmung oder Zusammensto\xdf mit Killerasteroid.
Doch dann beginnt das Problem.
Worum ging es da konkret?
Wo ist hier der Ausweg?
Bezirke Pardubice und Hradec Kr\xe1lov\xe9
Bislang sind keine Verkehrsst\xf6rungen gemeldet.
Von wem stammt diese Idee?
Nur ein einziger: L\xe1 \u2047 a Angelovi \u2047 .
Dieser Trend ist daher systembedingt.
Sprechen wir \xfcber Ihre Visionen.
Dazu m\xfcssen Sie Gesetze \xe4ndern.
Ich habe keine andere M\xf6glichkeit.
Das ist nicht gerade \xfcberzeugend.
Soll ich etwa Schulden machen?
Der lange Weg zum Buch
Das urbane Ambiente ist perfekt.
Und \xfcberall B\xfccher, B\xfccher, B\xfccher.
Das ist billig und zeiteffizient.
Spenden f\xfcr die neue Seele
Das Raumklima ist sehr angenehm.
Den Rest erledigen vollautomatische Rollos.
Dann aber enthielt sich Berlin.
Was aber ist Armani Polo?
In Swasiland leben 245000 Aidswaisen.
Fakten zu sexuell \xfcbertragbaren Infektionen
Wie kann man sich sch\xfctzen?
Ein K\xf6nig mit 14 Ehefrauen
Seine Besonderheit: die hohe Lichtsammelkraft.
Jeden Tag becherweise geschmolzene Butter
Auch zwei Kleinkinder springen herum.
Monatliche Rente reicht zum Leben
Wir m\xfcssen den \xdcbergang schaffen.
Soll die Judikative entmachtet werden?
Vieles im Verfassunsgsentwurf ist Auslegungssache
"Der Koran ist unsere Verfassung"
"Hier sind unsere Punkte, Havard".
Aber das hier war Mexiko.
Ich war einfach nur Amerikaner.
Lust, \xfcber Ressentiments zu sprechen?
Es gibt mehr als genug.
Alte Gefechte, neuer Naher Osten
Auch Israelis sollten langfristiger denken.
Die Bilder beeinflussen mich nicht.
Professor Eastwood stimmt dem zu.
Aber ist er auch einer?
Noch sind viele Fragen offen.
Andere Studenten teilten seine Meinung.
Ich war pervers und dreckig.
Die schlagen sich gegenseitig, oder?
Er war nur selten da.
Seine feuchten Augen tr\xfcbten sich.
Gib dem Ganzen eine Chance.
Und dies sagt eine Prinzessin...
Die Kinder k\xf6nnen andere bekommen.
"Das ist entschieden", erkl\xe4rte er.
Das ist eine schwierige Frage.
Er wurde 81 Jahre alt.
Die Kurse waren sehr beliebt.
Dies reicht noch weiter.
Stellen Sie sich vor...
Wie man sauber macht.
Gro\xdfartige Spieler sind gekommen.
Wir akzeptieren das vollkommen.
Wie funktioniert dieses Netzwerk?
Innenministerium ignoriert illegalen Waffenmarkt
Woher stammen die Waffen?
Einkaufen vom Sofa aus
46 Cents im Jahr?
Wer, wenn nicht ich?
Die Aufgabe ist schwierig.
Trotzdem bleibt ein Risiko.
Polen und der Weltraum.
Dies betrifft ganz Lateinamerika.
Israel: Labor des Chaos.
Ich bin kein Retter.
Sie haben kein Geld?
Das Konzept ist aufgegangen.
Spijkenisse hat Literaturgeschichte geschrieben.
Dagegen anzugehen kostet viel
Man muss h\xf6llisch aufpassen
Weltaidstag: Stampfen, singen, helfen
Vierzig Prozent sind infiziert
Wer sind die Hauptbetroffenengruppen?
Doch was hei\xdft "Prinzipien"?
"Die Revolution ist zur\xfcckgekehrt"
Das k\xf6nnte sich r\xe4chen.
Ich koste einige H\xe4ppchen.
Man klatscht und lacht.
Dies beruht auf Gegenseitigkeit.
Das wird nicht passieren.
Zu viele verletzte Gef\xfchle.
Ich ignoriere sie einfach.
Ich will nicht l\xfcgen.
Meine Freunde waren verwirrt.
Die anderen Studenten kicherten.
Meine T\xfcr war verschlossen.
Ich kehrte nie zur\xfcck.
Die Proportionen sind perfekt.
Der "K\xf6nig" der Mode
Singapur ist ein Stadtstaat.
Die meisten sind Verwandte.
Es sind dieselben Regeln.
Kondome hinter dem Ladentisch
Dragon Mart ist umzingelt
"Basketball war mein Leben."
Darauf bin ich stolz.
Was machst Du heute?
Larry Hagman ist tot
Vorbeugen der Krankheit
Das Higgs-Boson analysiert
Keine omnipotente Pflege
Wie eine Entt\xe4uschung.
Einzigartige Museen besuchen
Merkliste f\xfcr Touristen
Nicht schimpfen, Chef!
"Wie im Luxusladen"
Milit\xe4rkommentator Viktor Baranez
- Wie das?
Clowns sind zeitlos.
- Gute Kulturexperten.
Geburt im Weltall
Erde in Gefahr.
Kombination der Genres
Ja, das stimmt.
Hilfe zur Selbsthilfe
Polygamie statt Demokratie.
Endstation ist Lerik.
Ein direkter Mann
Meine mexikanisch-amerikanische Identit\xe4tskrise.
Das ist fair.
Ich lief weg.
Ich stolperte dabei.
Du bist verschmutzt.
Er schien ungl\xe4ubig.
Modenschau der Herkunft
Zu viel Stress
Schl\xfcsseldaten von Jalisco
ACTA ist tot
Gr\xfcndung von Competival
Bayam\xf3n im Herzen
M\xf6chtest Du ihn?"
Ich genie\xdfe es.
Das Gewicht
Die Ern\xe4hrung
Stabileres Feld
Und danach?
Sterne funkeln.
In Zahlen
"Freie Kasse!"
Bezirk Pilsen
Bezirk Olomouc
Nicht Mexiko.
Und nein.
1,2 Kinder
Unerwartete Folgen
Allgemeine Bilanz
Homex langfristig
Vitamine
Auswirkungen
Regelm\xe4\xdfig.
Selbstverst\xe4ndlich.
Unzufriedene
Karlsbad
Verst\xe4ndlicherweise.
Warum?
Eins-zwei-drei-vier.
Nun.
Hmmm.
Ja.
Privatsph\xe4re
Schl\xfcsselfragen
\xdcberwachung


==> tables/qualitiative_analysis/emb1.14_deen_outputs_cvt.tex <==
\textbf{Corr}\underline{up}tion was \textbf{ramp}\underline{ant}, and the people \textbf{went} to the \textbf{poll}\underline{s} with \textbf{votes} already \textbf{bought}\underline{"} ... "P\textbf{eo}\textbf{\underline{ple}} of character did not apply for office, so that the state had no \textbf{cons}\underline{ul} for \textbf{eight} months as a result of this \textbf{decline}\underline{"} ... "\textbf{You} really began to talk about the only \textbf{medicine} in this difficult situation being an \textbf{exclusive} rule and that a strong man had to be \textbf{elected}\underline{"}...
Israel u2019s current \textbf{prime} \textbf{minister}\underline{,} \textbf{Falk}\underline{e} \textbf{Net}\underline{an}yahu, is a \textbf{typical} example of a fa\textbf{sc}\underline{ism}-prone \textbf{politician} \textbf{loyal} to international \textbf{bankers} who is doing all he can to \textbf{trigger} a war with Iran, which, with Iran u2019s \textbf{membership} of the \textbf{Shanghai} \textbf{Cooperation} Organisation (\textbf{China}\underline{,} India, Russia, Pakistan\textbf{...)}\underline{,} could \textbf{rapidly} develop into a global conflict and could lead to the \textbf{destruction} of the world economy because of Iran u2019s control of the only 2 \textbf{mile}\underline{-}\textbf{wide} \textbf{Stra}\underline{it} of \textbf{Hor}\textbf{\underline{mus}}\underline{,} which \textbf{accounts} for \textbf{20\%} of world oil \textbf{supplies}\underline{.}
In order to \textbf{facilitate} World War II, the \textbf{bankers} allowed \textbf{politics} to create a latent conflict situation by \textbf{imposing} \textbf{giganti}\underline{c} war \textbf{repair}\underline{s} on Germany; by doing so, they created the \textbf{precondition}\underline{s} for impover\textbf{ished} masses, so that they only had to rejoice the Germans with a \textbf{sufficiently} strong \textbf{leader} who offered the \textbf{guilty} to name and simple solutions; another \textbf{factor} was the creation of the multi-\textbf{ethnic} state of Czechos\textbf{lov}\underline{ak}ia with a strong German \textbf{minority}\underline{,} which was to take on the role of a \textbf{fifth} \textbf{column} and also took on the role of \textbf{trigger}\underline{ing} the war.
One of the \textbf{galleries} in Somer\textbf{set} House has been \textbf{transformed} into a \textbf{glorious} and 60-\textbf{metre}\underline{-}\textbf{long} \textbf{cat}\textbf{\underline{walk}} that \textbf{proposes} a re\textbf{els} exchange: the user takes the place of the model and goes along the \textbf{cat}\textbf{\underline{walk}} to \textbf{admire} a \textbf{fantastic} "\textbf{audi}\underline{ence}" \textbf{carrying} \textbf{masterpiece}\underline{s} of \textbf{Valentin}\underline{o}, such as the \textbf{dress} that \textbf{Jack}\underline{ie} \textbf{Kennedy} \textbf{chose} for her \textbf{wedding} with Arist xf3teles On\textbf{assi}\underline{s}, the \textbf{costume}\underline{s} that \textbf{Mon}\underline{ica} Vi\textbf{tti} wore in "La Notte", or a \textbf{coat} of \textbf{wool} and \textbf{leather} that \textbf{belong}\underline{ed} to the \textbf{Em}\underline{press} \textbf{Far}\underline{ah} Diba.
The first war was aimed at \textbf{eliminating} the great \textbf{monarch}\underline{ist} states of Europe, the second war was intended to break \textbf{Britain}\underline{'}s \textbf{colonial} rule in particular, and the third war is intended to reduce the world's population to \textbf{approximately} \textbf{0.5} to 1 billion people (a number that would provide their comfort and \textbf{luxury} and would not \textbf{consume} so many resources), to create a \textbf{universal} \textbf{religion} (e\textbf{cum}\underline{en}ism is nothing more than the pre\textbf{cur}\underline{s}or), and finally to take over \textbf{absolute} power.
The \textbf{experts} and civil \textbf{servant}\underline{s} of the Consejo Estatal de Prevenci xf3n del S\textbf{ida} en Ja\textbf{lis}\underline{co} (\textbf{Co}\underline{es}\textbf{ida}\underline{)} (\textbf{Stat}\underline{e} Committee on \textbf{AIDS} \textbf{Prevention} in Ja\textbf{lis}\underline{co}) and also \textbf{patients} such as \textbf{Fabr}\underline{i}\textbf{zio}\underline{,} who carried out his test at a private \textbf{laboratory}\underline{,} agree with this proposal for the \textbf{sole} reason that he had made a \textbf{friend} of him who, despite his young age, was already in the \textbf{AIDS} \textbf{phase} and even had the casssari comb (a \textbf{cancer}\underline{ous} \textbf{tu}\textbf{\underline{mor}}\underline{),} which is one of the \textbf{usual} \textbf{complications}\underline{.}
The \textbf{infectious} \textbf{disease} and \textbf{HIV}\underline{/}\textbf{AIDS} \textbf{expert}\underline{,} Andrade Villa\textbf{nu}\textbf{\underline{eva}}\underline{,} commented that since 2008, \textbf{scientists} have \textbf{concluded} that \textbf{AIDS} was not a death \textbf{sentence}\underline{,} but that the years of \textbf{survival} and quality of life depended on the level of im\textbf{pair}\underline{ment} of the \textbf{immune} system of people at the beginning of treatment, and that those who are not \textbf{drug}\underline{-}\textbf{dependent} would have greater chances: up to 30 years at 200 CD4 \textbf{count}\underline{s} and 50 years at 500 CD4 \textbf{count}\underline{s}.
The most serious \textbf{aspect} of this case is that the Court has set \textbf{aside} a document sent by the Government of \textbf{Mexico} under \textbf{Figur}\underline{a} a\textbf{mic}\underline{us} \textbf{cur}\underline{ia}e (\textbf{Fri}\underline{end} of the Court), which \textbf{describes} the procedure carried out by Vitro under the \textbf{Trade} Con\textbf{cur}\underline{r}\textbf{ency} \textbf{Act} and which states that it had \textbf{adhere}\underline{d} \textbf{strictly} to the agreements \textbf{signed} by both countries in order to \textbf{comply} with \textbf{Chapter} 15 of the \textbf{bankruptcy} law of the United States.
The \textbf{Roth}\textbf{\underline{schild}}\underline{s} are involved in almost all of the world u2019s central banks, and against the countries in which they are not \textbf{participating} in the central banks, they \textbf{wage} wars or \textbf{arm} themselves against them (before the attack on Afghanistan, there were 7 countries, there were 5 after the attack on Iraq, and only four were left after the fall of Ghaddafi, with Russia in the \textbf{meantime} subjecting its central bank to the Russian government).
31 years after \textbf{AIDS} \textbf{appeared} in the world, that is to say after the first \textbf{reported} cases \textbf{appeared}\underline{,} 'the great success today means that the \textbf{survival} of a \textbf{patient} who receives treatment in good time and the \textbf{survival} of the general population are exactly the same', stated the head of the \textbf{HIV} \textbf{unit} of the HCG, Ja\textbf{ime} Andrade Villa\textbf{nu}\textbf{\underline{eva}}\underline{,} saying that this information was supported by a \textbf{respected} scientific \textbf{publication} in April this year.
Cor\textbf{rea} stated that the solution to \textbf{asylum} \textbf{granted} by Ass\textbf{ange} at the \textbf{Ecuador}\underline{ian} \textbf{embassy} in London in June was to \textbf{grant} a \textbf{licence} to travel to \textbf{Ecuador}\underline{,} and that this would be in the \textbf{hands} of \textbf{Britain}\underline{,} \textbf{Sweden} and the European legal authorities, underlining that there had been \textbf{talks} with London to find a solution for the \textbf{imprisoned} \textbf{founder} of \textbf{Wiki}\textbf{\underline{Le}}\underline{ak}s.
There he \textbf{earned} 7\textbf{5,000} rupees (\textbf{6.2} \textbf{euros}\underline{)} a day, and the work was not so hard, but Anto has \textbf{returned} with his family to \textbf{Ban}\textbf{\underline{yu}}\textbf{\underline{wang}}\underline{i}, a village \textbf{nearby}\underline{,} for a reason as important as \textbf{sulphur} in \textbf{Indonesia}\underline{:} 'I \textbf{married} a \textbf{girl} from \textbf{Bali}\underline{,} where they are \textbf{Hindu}\underline{s}, and I have brought her to \textbf{Java} to \textbf{convert} them to \textbf{Islam}\underline{'}.
Even if the \textbf{sulphur} \textbf{burn}\underline{s} the \textbf{thro}\underline{at} and the \textbf{eyes} it\textbf{ches} when the \textbf{wind} \textbf{suddenly} \textbf{turns} and the \textbf{mine}\textbf{\underline{work}}\underline{ers} are \textbf{stuck} in the \textbf{thick} \textbf{column}\underline{s} that rise out of the \textbf{cra}\underline{ter}, the men are so hard that \textbf{nobody} \textbf{complain}\underline{s} about serious \textbf{diseases} ... of course, \textbf{apart} from the \textbf{usual} \textbf{respiratory} problems, arthr\textbf{osis}\underline{,} \textbf{pain}\underline{s} in the \textbf{knee}\underline{s} and b\textbf{list}\underline{ers} on the shoulders that have deformed from the \textbf{weight} of the \textbf{basket}\underline{s}.
In her study "The Unenga\textbf{ged} \textbf{Mind}\underline{:} \textbf{Defin}\underline{ing} \textbf{Bor}\underline{e}\textbf{dom} in \textbf{Terms} of At\textbf{tention}\underline{"} - in German for example: "The \textbf{idle} mind: The \textbf{definition} of \textbf{bo}\underline{re}\textbf{dom} under the \textbf{aspect} of attention", which \textbf{appeared} in September in the \textbf{journal} "\textbf{Per}\textbf{\underline{spect}}\underline{ive}s on \textbf{Psycho}\textbf{\underline{logical}} \textbf{Science}\underline{",} \textbf{Professor} East\textbf{wood} and his colleagues point to an earlier \textbf{experiment} in which \textbf{participants} \textbf{listened} to a \textbf{band} on which a person read a \textbf{magazine} \textbf{article}\underline{.}
Since \textbf{2009,} a service of "ci\textbf{vil}\underline{-}\textbf{military} actions" of the \textbf{Ministry} of \textbf{Defence} (Cimic), which was \textbf{discontinu}\underline{ed} in \textbf{2012}\underline{,} has carried out in \textbf{dozen}\underline{s} of mountain \textbf{villages} numerous \textbf{char}\underline{it}able works and measures for agricultural \textbf{rehabilitation} and has been carried out by a small French non-\textbf{governmental} \textbf{organisation} to try to \textbf{win} the "hearts and spirits" and to achieve the \textbf{impossible} task of \textbf{reco}\underline{n}\textbf{cil}\underline{ing} aid and \textbf{offensive} actions.
There is no doubt that the \textbf{austerity} measures of \textbf{virtually} all EU-\textbf{South} countries will end up in the same situation where people are \textbf{forced} to \textbf{emigr}\underline{ate} under the pressure of a \textbf{catastrophic} \textbf{decline} in their social level (as was the case in the 19th century), or for a starvation \textbf{wage} on the \textbf{margin}\underline{s} of society, \textbf{hoping} that private investment capital will \textbf{eventually} \textbf{flow} into the country.
Even if \textbf{mortality} has \textbf{decline}\underline{d} \textbf{significantly} in recent years (in \textbf{Mexico}\underline{,} the number of people \textbf{dying} from \textbf{AIDS} has \textbf{decline}\underline{d} from 6,\textbf{67}\underline{8} in 2007 to 4,\textbf{86}\underline{2} in \textbf{2011} (A\textbf{nnual} \textbf{Report} of \textbf{ON}\underline{US}\textbf{ID}\underline{A}), it is \textbf{nonetheless} true that 60 \textbf{percent} of \textbf{patients} \textbf{recorded} in the national \textbf{database} have died since the \textbf{advent} of \textbf{AIDS}\underline{.}
In \textbf{Prague} I have a property \textbf{worth} 25 million, an apartment \textbf{worth} about 10 million, another for 8 million, an art collection \textbf{worth} about 10 million, as well as an Aston \textbf{Martin} for \textbf{3.5} million and a   u20\textbf{47} \textbf{ko}\underline{du} Superb \textbf{worth} about a million, and then I have a few million in my account.
"\textbf{For} my life I have put up many hats in \textbf{basketball}\underline{,} even several at the same time, when I was President of the BSN, head of the national team and \textbf{president} of the \textbf{association} in the 1990s," \textbf{Rey}\underline{es} \textbf{remembered} when he \textbf{visited} \textbf{Prime}\underline{ra} \textbf{Hor}\underline{a} at home in \textbf{Bay}\underline{am} xf3n, where he lives with \textbf{Isabel}\underline{,} his \textbf{faithful} \textbf{wife} for more than 50 years.
In addition to a 9\textbf{3-}\textbf{\underline{year}}\underline{-}\textbf{old} man who \textbf{enjoys} the last family meeting in the \textbf{court} and is well supported by his \textbf{pil}\textbf{\underline{low}}\underline{s} while in\textbf{dig}\underline{n}ant in his \textbf{honour}\underline{,} a \textbf{36}\underline{-}\textbf{year}\underline{-}\textbf{old} man who is \textbf{surrounded} by his \textbf{parents}\underline{,} his \textbf{wife} and his two little children dies \textbf{tragic}\underline{ally} after trying to \textbf{survive}\underline{.}
For even if p\textbf{article} \textbf{physics} is a really \textbf{strange} world, it \textbf{turns} out that such a law also applies to them: the \textbf{Paul}\underline{i}ian principle of \textbf{exclusion}\underline{,} which states that two p\textbf{article}\underline{s} cannot \textbf{occupy} the same space at the same time when they are in the same "\textbf{qu}\underline{ant}ity state", with this "\textbf{state}\underline{"} \textbf{generally} \textbf{consist}\underline{ing} of some of their \textbf{characteristics}\underline{.}
So far, we have \textbf{felt} more of an impact in the \textbf{preparato}\underline{ry} \textbf{phase} of future \textbf{controls} - for example, we have introduced the new control instrument 'Re\textbf{cognit}\underline{ion} of \textbf{risks} of in\textbf{eff}\textbf{\underline{ici}}\underline{en}\textbf{cies}\underline{'} and with this almost 1\textbf{4,000} public \textbf{contracts} \textbf{checked} and \textbf{analysed} - here, of course, the changes will have an impact, because the \textbf{threshold}\underline{s} are \textbf{changing}\underline{,} the conditions for certain types of \textbf{tender} have been modified, and so on.
The \textbf{Second} World War \textbf{broke} out, and whether \textbf{Hitler} was torn \textbf{apart} from the \textbf{chain} at which the international \textbf{bankers} had \textbf{initially} \textbf{kept} him, or whether everything was \textbf{planned}\underline{,} it is difficult to \textbf{estimate}\underline{.} In any case, the \textbf{suffering} of the European \textbf{Jews} in the \textbf{concentration} \textbf{camps} created the \textbf{precondition} for the international community's \textbf{recognition} of the \textbf{Jewish} state.
D\textbf{espite} the fact that \textbf{rocket}\underline{s} from \textbf{Gaza} have \textbf{killed} around 30 \textbf{Israelis} since 2004, the country has \textbf{remained} relatively free of \textbf{suicide} \textbf{bomb}\underline{ers}, not least thanks to the \textbf{closure}\underline{s} that have \textbf{flow}\underline{ed} into the West Bank and thus into the \textbf{bulk} of a possible \textbf{Palestinian} state, which are \textbf{protecting} \textbf{Jewish} \textbf{settlements}\underline{,} which have been \textbf{declared} \textbf{contrary} to international law but are being developed.
He stated that measures would be taken 'to improve cooperation in the fight against in\textbf{security} in cities and against \textbf{organised} cross-\textbf{border} crime, as well as measures to improve access to \textbf{medicines} and the Internet at low prices in all parts of South America and to act \textbf{jointly} and effectively in the event of natural \textbf{disasters}\underline{'}.
In fact, the late \textbf{phy}\underline{s}icist \textbf{Will}\underline{ard} \textbf{Boy}\underline{le} - who worked in the \textbf{Bell} \textbf{Lab}\underline{s} where the \textbf{laser} was \textbf{invented} in the \textbf{1960}\underline{s}, and who in \textbf{1962} developed the first permanent\textbf{strich} \textbf{laser} (the first were \textbf{pulse}\underline{d}) - has already \textbf{told} us that the \textbf{laser} was \textbf{initially} \textbf{regarded} as a "\textbf{bor}\underline{e}-\textbf{play}\underline{ing}" \textbf{laser}\underline{.}
Here lies another task that we will have to \textbf{contend} with for a long time to come: to make a person \textbf{physically} in a closed space believe that he is instead in an open, \textbf{virtually} \textbf{infinite} space; here we are working on \textbf{concepts} with \textbf{tre}\underline{ad}\textbf{mill}\underline{s} (\textbf{other} than in \textbf{fitness} \textbf{studios}\underline{),} \textbf{moving} \textbf{platforms} and large \textbf{ball}\underline{s}.
\textbf{Sand}\underline{ra} Ha of \textbf{Zi}\underline{co} \textbf{Import} Pty \textbf{Ltd}\underline{,} a small family company, \textbf{notes} that demand for \textbf{cigarette} cases and \textbf{silicon}\underline{e} \textbf{lid}\underline{s} to cover \textbf{unbe}\textbf{\underline{arable}} \textbf{packaging} has increased \textbf{enormous}\underline{ly} since British American To\textbf{bac}\underline{co}, \textbf{Britain}\underline{'}s \textbf{Imperial} To\textbf{bac}\underline{co}, \textbf{Philip} \textbf{Morris} and Japan To\textbf{bac}\underline{co} \textbf{failed} at the \textbf{Australian} \textbf{Supreme} Court to challenge the law two months ago.
Efe \textbf{repeatedly} \textbf{tried} to \textbf{gain} access to the \textbf{signed} document at the \textbf{VI}\underline{th} Or\textbf{din}\underline{ary} \textbf{Meeting} of the \textbf{Heads} of State and Government of the Unasur.
"\textbf{And} it makes that the small and the big, the rich and the poor, the free and the \textbf{servant}\underline{s} all give a \textbf{paint}\underline{mark} to their right hand or to their fore\textbf{head} that \textbf{nobody} can buy or \textbf{sell}\underline{,} they have the \textbf{paint}\underline{mark}, namely the name of the animal or the number of its name.
\textbf{Among} the \textbf{controversial} EU regulations are, for example, the \textbf{mandatory} addition of \textbf{bio}\underline{e}\textbf{than}\underline{ol} to \textbf{fuels} that cause natural damage, the ban on \textbf{reliable} \textbf{mercury} \textbf{thermo}\textbf{\underline{meter}}\underline{s}, just because they \textbf{contain} a relatively small amount of this \textbf{dangerous} \textbf{substance}\underline{,} and also the directive on the size of \textbf{chicken} ca\textbf{ges}\underline{,} which made \textbf{eggs} much more \textbf{expensive} this year.
However, there are also technologies that are actually aimed at giving something \textbf{tangible} to the '\textbf{pic}\underline{ture}s in the air', for example, the \textbf{interference} of some directional \textbf{ultra}\underline{s}\textbf{onic} \textbf{ray}\underline{s} in a particular point where the \textbf{finger} is located \textbf{creates} a \textbf{feeling} that is still so \textbf{weak} at the moment, as if \textbf{someone} were \textbf{pu}\underline{st}ling over the hand\textbf{ball}\underline{s}.
The best \textbf{scenes} of the film play in the \textbf{streets} and show the \textbf{reconstruction} of events that have actually taken place - the entry \textbf{sequence} of the first \textbf{storm}\underline{ing} of the message is very \textbf{impressive} in its \textbf{clarity}\underline{,} yet \textbf{convey}\underline{s} the sense of \textbf{confusion} and un\textbf{pre}\textbf{\underline{dic}}\underline{t}ability that \textbf{happens} when history \textbf{moves} \textbf{somewhere}\underline{.}
However, he is working very \textbf{successfully} with the little, sometimes \textbf{helping} the reality - which does not always \textbf{seem} so elegant (the \textbf{scenes} in which the im\textbf{pending} crisis at Te\textbf{hra}\underline{n} airport is a\textbf{vert}\underline{ed} from a telephone call in America, or even the follow-up \textbf{hunt} on the runway are \textbf{somewhat} \textbf{artificial}\underline{).}
In the first room of this \textbf{exhibition}\underline{,} which will be on display until 3 March, there are a number of private \textbf{letters} and \textbf{photos} with the \textbf{signature} of the most \textbf{prestigious} a\textbf{risto}\textbf{\underline{cracy}}\underline{,} from \textbf{Prince}\underline{s}s Sal\textbf{ima}\underline{h} Aga \textbf{Khan} to \textbf{Prince}\underline{s}s \textbf{Marie}\underline{-}\textbf{Cha}\underline{n}tal of Greece and Margar\textbf{ita} of \textbf{England} to \textbf{Lord} \textbf{Snow}\textbf{\underline{don}}\underline{.}
It is only \textbf{250} metres from the summit of the \textbf{volcano}\underline{,} which rises up to 2\textbf{386} metres, but the \textbf{exhaust}\underline{ed} \textbf{carriers} take more than 40 minutes to \textbf{climb} at the tortoise speed, \textbf{keeping} the balance and taking \textbf{precaution}\underline{s} to prevent them from \textbf{slip}\underline{ping} and \textbf{falling}\underline{.}
In this respect, before he began his participation in the regional meeting, the President of \textbf{Colombia}\underline{,} \textbf{Juan} \textbf{Manuel} \textbf{Santo}\underline{s}, said that he was \textbf{expecting} a meeting with his \textbf{counterpart} from \textbf{Nicaragua}\underline{,} \textbf{Daniel} \textbf{Ortega}\underline{,} on \textbf{Saturday} in \textbf{Mexico}\underline{,} in order to respect the \textbf{maritime} conflict following a \textbf{judgment} questioned by the I\textbf{CC} by Bo\textbf{got} xe\textbf{1.}
\textbf{According} to The P\textbf{article} \textbf{Adventure} website, these \textbf{Bos}\underline{ons} are \textbf{divided} into two groups by the \textbf{Ber}\underline{ke}ley \textbf{Labor}\textbf{\underline{atori}}\underline{es} (\textbf{which}\underline{,} by the way, is absolutely \textbf{amazing}\underline{):} the mesons we will not \textbf{treat} here and the "\textbf{power} p\textbf{article}\underline{s}" through which the great forces of nature \textbf{spread} and with which the \textbf{Hi}\textbf{\underline{gg}}\underline{s}\textbf{Bo}\underline{son} is \textbf{somehow} related.
\textbf{According} to the \textbf{Ministry} of the \textbf{Interior}\underline{'}s official \textbf{statistics}\underline{,} the number of illegal \textbf{weapons} \textbf{offences} across Russia \textbf{fell} by \textbf{7\%} to \textbf{22.}\underline{9} \textbf{thousand} between January and October \textbf{2011}\underline{,} while the number of cases of theft and blackmail \textbf{exposed} in connection with \textbf{weapons}\underline{,} am\textbf{muni}\underline{tion}, \textbf{explosive}\underline{s} and \textbf{explosive}\underline{s} \textbf{fell} by \textbf{7.}\textbf{\underline{8\%}}\underline{.}
The only reason that so many people of \textbf{Mexican} origin live in cities like \textbf{Los} \textbf{Angeles}\underline{,} \textbf{Las} \textbf{Vegas}\underline{,} \textbf{Phoenix}\underline{,} Denver or San \textbf{Antonio} is because at one point in our family \textbf{tree}\underline{,} a person - perhaps a \textbf{parent} or \textbf{grand}\textbf{\underline{parent}} - was not offered a chance in \textbf{Mexico} and \textbf{migrate}\underline{d} \textbf{north}\textbf{\underline{ward}}\underline{.}
Re\textbf{stall} \textbf{pointed} out that many days were \textbf{discussed} by the last \textbf{court} over the years, and said that if nothing \textbf{happened} on 21 December, "\textbf{people} immediately think of a new date" or \textbf{phil}\textbf{\underline{oso}}\underline{ph}ized that 21 December was the beginning of a \textbf{seven}\underline{-}\textbf{year} period of coming to the end of the world.
Sebe\textbf{lev} is \textbf{convinced} that a future \textbf{migrant} who has no knowledge of languages will \textbf{inevitably} meet people with bad \textbf{intentions} who, on the \textbf{pretext} of aid, are \textbf{putting} him in a \textbf{dark}\underline{,} \textbf{narrow} bar\textbf{rack} where he will \textbf{endure} \textbf{dozen}\underline{s} of unfam\textbf{ili}\underline{ar} months without food and documents and who will have worked 12 to 14 hours a day.
What is particularly \textbf{disastrous} is the fact that today's \textbf{elite}\underline{s} are completely \textbf{ignor}\underline{ant} of the possible future loss of \textbf{hundreds} of thousands of lives, of the \textbf{humanitarian} and social \textbf{disasters} that we are already \textbf{witness}\underline{ing} today and of the \textbf{crimes} against \textbf{humanity} that we know from old and modern history.
The \textbf{patient} must be made \textbf{genuinely} aware of the extent of the risk of \textbf{cancer} by \textbf{showing} the possible options for which pro\textbf{state} \textbf{cancer}\underline{s} can remain untreated if they do not \textbf{affect} the quality of life in the long term and, in these cases, \textbf{opt} for active monitoring of the \textbf{disease}\underline{.}
\textbf{Parti}\textbf{\underline{cip}}\textbf{\underline{ants}} of the \textbf{protests} that began on \textbf{Thursday} at \textbf{6.}\underline{30} a.m. in front of \textbf{McDonald}\underline{'}s on 40th \textbf{Street} and \textbf{Madison} \textbf{Avenue} \textbf{demanded} that the \textbf{cash}\textbf{\underline{iers}} and \textbf{cook}\underline{s} of fast-\textbf{food} restaurants receive a minimum \textbf{wage} of \$15 an \textbf{hour}\underline{,} more than a doubling of the current minimum \textbf{wage}\underline{.}
The \textbf{culminat}\underline{ion} of the \textbf{protests} was a \textbf{mid}\underline{day} meeting in front of \textbf{McDonald}\underline{'}s on \textbf{Times} \textbf{Square} where some local \textbf{democrat}\underline{s} \textbf{spoke}\underline{,} including \textbf{council}\textbf{\underline{lor}} \textbf{Ju}\underline{ma}\textbf{ane} \textbf{William}\underline{s}, who said: 'Mc\textbf{Don}\underline{al}d's \textbf{says} it \textbf{sell}\underline{s} billions of \textbf{portion}\underline{s}, and yet you are not allowed \textbf{sick} days and you are not paid for your \textbf{honest} work!'
\textbf{Samuel} \textbf{Robert}\underline{s}, 21 and \textbf{Histori}\underline{c} \textbf{student} in \textbf{Corp}\underline{us} \textbf{Christi}\underline{,} who \textbf{initiated} the request for greater protection, \textbf{believes} that such a climate is "in\textbf{conv}\underline{en}\textbf{ient}\underline{.}
The \textbf{confirmation} by both \textbf{president}\underline{s} that they would \textbf{submit} to the I\textbf{CC} came after \textbf{Colombia} had brought an action against the Bo\textbf{got} xe1 Agreement following a decision on the \textbf{maritime} borders with \textbf{Nicaragua}\underline{,} which it considered to be a serious \textbf{mistake}\underline{,} in which it agreed to \textbf{submit} to the \textbf{judgment}\underline{s} of this international \textbf{court}\underline{.}
Cor\textbf{rea} also supported the decision to maintain the \textbf{veto} against \textbf{Paraguay} in Unasur at least until its next elections, \textbf{arguing} that the \textbf{organism} must remain '\textbf{hard} and must not give way to \textbf{opportun}\underline{ism} or a \textbf{coup} d' xe9\textbf{tat} that is \textbf{legally} \textbf{disguise}\underline{d}' because it 'de\textbf{stro}\underline{y}ed the \textbf{legitimacy} of democracy in \textbf{Paraguay}\underline{'}.
"I work, do a lot, have an active but responsible \textbf{sex} life, I pay attention to my health and that of the other person", \textbf{count}\underline{s} \textbf{Fabr}\underline{i}\textbf{zio}\underline{,} who agreed to share his \textbf{intimate} details with M\textbf{IL}\underline{EN}\textbf{IO} JALIS\textbf{CO} in order to animate with his \textbf{testimony} those who are \textbf{afraid} today within the global \textbf{AIDS} \textbf{Day}\underline{.}
Afghanistan, the country of \textbf{mountains} with strong local \textbf{identities}\underline{,} should have benefited from a certain de\textbf{central}\underline{ization} of the Western \textbf{nations}\underline{,} but by \textbf{abolish}\underline{ing} the \textbf{prime} \textbf{minister} u2019s office, which has \textbf{existed} since the \textbf{constitution} of \textbf{1964}\underline{,} the US wanted to make it a centralized state with a strong \textbf{presidential} power.
When it comes from another EU country, poverty simply \textbf{migrate}\underline{s} from one country to another; or capital \textbf{leaves} completely, because in China, India, \textbf{Brazil}\underline{,} Turkey, \textbf{Morocco} or \textbf{Egypt}\underline{,} or Africa, workers work for a \textbf{fraction} of European \textbf{wages}\underline{.}
The \textbf{CIA}\underline{,} in cooperation with the \textbf{Canadian} authorities, managed to bring the \textbf{refugees} from Iran, \textbf{helping} them an extra\textbf{vag}\underline{ant} \textbf{story} to cover up their true \textbf{identity} - they traveled \textbf{disguise}\underline{d} with \textbf{Canadian} \textbf{passport}\underline{s} as members of a film staff who \textbf{alleged}\underline{ly} \textbf{visited} \textbf{locations} for a \textbf{science} \textbf{fiction} film in the country.
\textbf{Because} the government has not \textbf{complied} with a \textbf{Senat}\underline{e} request to \textbf{explain} under what conditions and circumstances the \textbf{Mexican} \textbf{ambassador} to Japan \textbf{signed} the Anti-\textbf{Co}\textbf{\underline{unter}}\underline{fe}iting \textbf{Trade} Agreement, known as \textbf{AC}\textbf{\underline{TA}}\underline{,} the matter has already been \textbf{archive}\underline{d} under the \textbf{Mexican} \textbf{Institute} of \textbf{Intel}\textbf{\underline{lect}}\textbf{\underline{ual}} \textbf{Property}\underline{.}
It recommends a complete \textbf{revision} of the system for public \textbf{procurement} and the \textbf{financing} of parties: '\textbf{We} cannot fall \textbf{deeper}\underline{;} by getting to the \textbf{bottom} of things with \textbf{courage}\underline{,} we can \textbf{rebuild} the house on a more \textbf{solid} basis with more \textbf{controls} and laws'.
Some support Israel and \textbf{argue} with its right to self-de\textbf{fence} while \textbf{calling} the \textbf{Palestinians} \textbf{terrorists}\underline{;} others support the \textbf{Palestinians}\underline{,} \textbf{argue} with the \textbf{racism} of the \textbf{Israeli} state, with the \textbf{genocide} committed against the \textbf{Palestinian} \textbf{Arab}\underline{s} and call the State of Israel \textbf{terrorist}\underline{.}
In the \textbf{midst} of the \textbf{usual} re\textbf{cri}\underline{min}ations, \textbf{countless} \textbf{buildings} have been \textbf{laid} in \textbf{ruins}\underline{,} more than \textbf{140} \textbf{Palestinians}\underline{,} most of them \textbf{civilians}\underline{,} and six \textbf{Israelis} - and for the first time \textbf{rocket}\underline{s} from \textbf{Gaza} have been \textbf{launched} near the \textbf{Israeli} \textbf{metropolis} of \textbf{Tel} A\textbf{viv} and the holy city of \textbf{Jerusalem}\underline{.}
\textbf{Ju}\textbf{\underline{bil}}\underline{ant} \textbf{Hamas} followers believe that an \textbf{Islamist} \textbf{cre}\underline{s}\textbf{cent} is \textbf{forming} around Israel - from \textbf{Lebanon} in the \textbf{north}\underline{,} where \textbf{militant} \textbf{Hezbollah} has power, to \textbf{Syria}\underline{,} where \textbf{rebel}\underline{s} of an increasingly \textbf{Islamist} \textbf{shape} may be \textbf{facing} \textbf{Bas}\textbf{\underline{har}} Assad's \textbf{storm}\underline{,} to \textbf{Jordan}\underline{,} where \textbf{Hamas} \textbf{allies} \textbf{threaten} the \textbf{king}\underline{.}
It was not only \textbf{Min}\underline{cy}, Ga\textbf{usse}\underline{,} \textbf{Ram}\underline{on} \textbf{Riva}\underline{s}, Fico L xf3pez and \textbf{Pic}\underline{ul} xedn (\textbf{Or}\underline{t}iz), but also the young players (\textbf{Ja}\textbf{\underline{vier}}\underline{)} "\textbf{To}  u20\textbf{47} ito" \textbf{Col} xf3n and \textbf{James} Carter, the \textbf{brother}\underline{s} Le xf3n (\textbf{Fran}\underline{ci}sco and \textbf{Ed}\underline{gar}) and \textbf{Mario} "\textbf{Qu}\textbf{\underline{ij}}\textbf{\underline{ote}}\underline{"} \textbf{Moral}\underline{es}, who could not be there because of a \textbf{knee} \textbf{injury} in 1990.
\textbf{Egypt} must now, together with Turkey and \textbf{Qatar}\underline{,} stop \textbf{arms} \textbf{supplies} to \textbf{Gaza} and is better placed than ever to \textbf{convince} \textbf{Hamas} of the idea of a \textbf{Jewish} state based on the \textbf{1967} borders, \textbf{supplement}\underline{ed} by \textbf{territorial} \textbf{exchanges} and a common \textbf{Jerusalem}\underline{.}
In this sense, he congratulated \textbf{himself} on the fact that \textbf{Ecuador} is no longer \textbf{dominated} by such \textbf{journalists} 'and not by \textbf{bankers} or hegem\textbf{onic} and \textbf{spi}\underline{es}-citizen countries', and \textbf{anticipated} that, in re-el\textbf{ection}\underline{,} he '\textbf{will} deepen the \textbf{revolution} to continue on the path in this right direction'.
It is also true that, after \textbf{withdraw}\underline{ing} the \textbf{votes} of the \textbf{branches}\underline{,} the creditors of Vitro, the creditors who \textbf{tried} Vitro in the \textbf{courts} of the United States, i.e. the \textbf{vul}\underline{ture} funds such as \textbf{Aureli}\underline{os} \textbf{Capital}\underline{,} \textbf{Aureli}\underline{os} Convergencia, El\textbf{lio}\underline{t} Intern\textbf{acion}\underline{al} and \textbf{Liverpool} \textbf{Limited}\underline{,} would not have \textbf{obtained} a majority.
\textbf{Before} being \textbf{tied} to the \textbf{wheelchair} by a \textbf{stroke} in 2008, Rexes was part of this sport for 6 years, be it as a lower-\textbf{class} player, first national \textbf{league} player, BSN \textbf{agent} and \textbf{manager} with the \textbf{Va}\textbf{\underline{quer}}\underline{os} de \textbf{Bay}\underline{am} xf3n or \textbf{president} of the \textbf{basketball} \textbf{association}\underline{.}
We have \textbf{compared} all of these with each other, and although the \textbf{examination} has not yet been \textbf{completed}\underline{,} we have been able to establish very interesting \textbf{differences}\underline{.}
I do not want to \textbf{write} at this point about who is \textbf{guilty} and who is the \textbf{victim} in these re\textbf{current} \textbf{waves} of \textbf{killing}\underline{;} at the end of the day, the current \textbf{residents} of Israel, including the self-governing \textbf{territories}\underline{,} have been \textbf{born} into the current political situation and have not \textbf{experienced} the beginning of violence.
It is also relatively \textbf{absurd} to have a directive that \textbf{affects} European \textbf{officials} themselves - \textbf{anyone} who has an official role in the EU must not use the name \textbf{Macedonia} because of the \textbf{sensitivity} of the issue for Greece and must instead say FY\textbf{ROM} (former \textbf{Yugoslav} Republic of \textbf{Macedonia}\underline{).}
On \textbf{Friday}\underline{,} \textbf{Jud}\underline{ge} Manning also questioned an \textbf{accus}\underline{ation} that he made in his statement on \textbf{Thursday} - so he had to \textbf{sleep} \textbf{naked} in his \textbf{cell} in \textbf{Qua}\underline{n}\textbf{tico} and have to stand \textbf{naked} before \textbf{guard}\underline{s} and other \textbf{prisoners} at a morning \textbf{count}\underline{.}
My \textbf{wife}\underline{,} \textbf{born} in \textbf{Gua}\textbf{\underline{dal}}\textbf{\underline{aja}}\underline{ra} and who, as a child, \textbf{legally} \textbf{migrate}\underline{d} to the United States, reminds me that there is \textbf{tension} between \textbf{Mexican}\underline{s} and \textbf{Mexican} \textbf{Americans}\underline{,} because \textbf{Mexican}\underline{s} have a \textbf{clearer} idea of who they are - and \textbf{Mexican} \textbf{Americans} do not like that.
If at least some \textbf{Mexican}\underline{s} are not yet ready to \textbf{award} the United States for dealing with \textbf{Mexico} a century and a half ago, they must also accept that some \textbf{Mexican} \textbf{Americans} have a \textbf{res}\underline{ent}ment about how their family members were \textbf{treated} not so long ago.
After a long reading of research \textbf{literature} and the \textbf{presentation} of the idea in front of a focus group of about 100 people \textbf{Professor} East\textbf{wood} and his colleagues \textbf{concluded} that \textbf{bo}\underline{re}\textbf{dom} can be \textbf{defined} as the experience "to do a \textbf{satisfactory} job but not to be able to do it".
The \textbf{president}\underline{s} of \textbf{Peru}\underline{,} Oll\textbf{anta} \textbf{Hum}\textbf{\underline{ala}}\underline{,} and \textbf{Chile}\underline{,} Seba\textbf{sti} xe1n Pi  u20\textbf{47} \textbf{era}\underline{,} met during the regional meeting and \textbf{confirmed} that they would accept the decision of the I\textbf{GH}\underline{,} which \textbf{begins} on \textbf{Monday} in The \textbf{Hague}\underline{,} in the process that \textbf{Lima} \textbf{launched} against \textbf{Santiago}\underline{,} to \textbf{listen} to the \textbf{plea}\underline{s} of both \textbf{sides}\underline{.}
With regard to the possibility of \textbf{standing} as a \textbf{candidate} for the next \textbf{presidential} elections in \textbf{Ecuador} in order to achieve his third \textbf{consecutive} \textbf{mandate}\underline{,} he stated that he sees this possibility '\textbf{with} much \textbf{optimism} and \textbf{joy}\underline{,} although it is sometimes very difficult'.
In certain places, "the distribution of con\textbf{dom}\underline{s} was actually increased; \textbf{previously} they were \textbf{handed} out \textbf{individually}\underline{,} now they give us \textbf{packages} with a \textbf{hundred} \textbf{pieces}\underline{,} which is good, but there are still people who have no access to a con\textbf{dom}\underline{,}" he said.
At a \textbf{weekend} meeting at a \textbf{forum} of the University of the \textbf{Caribbean}\underline{,} a group of national and foreign environmentalists, \textbf{academic}\underline{s}, \textbf{entrepreneurs} and general members of civil society decided to create a broad front to \textbf{oppose} the opening of the Chinese \textbf{Dragon} Mart in \textbf{Canc}  u20\textbf{47} n.
\textbf{Every} \textbf{semester}\underline{,} when the \textbf{religious} \textbf{professor} decided to hold a course on the end of the world, he \textbf{knew} that he had an \textbf{irre}\underline{s}ist\textbf{ible} \textbf{hook}\underline{:} the end of the "\textbf{long} \textbf{backward} \textbf{count}\underline{"} of the \textbf{Maya}\underline{n} \textbf{calendar} on December 21, which many people \textbf{believed} was the end of the world.
"\textbf{This} \textbf{experiment} that we are \textbf{carrying} out together, namely the \textbf{birth} of a child in a foreign environment, will lead us to create a \textbf{disabled} person, a completely uns\textbf{uit}\underline{ed} person," \textbf{says} I\textbf{gor} \textbf{Pest}\underline{ov}, head of the \textbf{Bio}\textbf{\underline{eth}}\textbf{\underline{ics}} Commission of the \textbf{Institute} for \textbf{Medical}\underline{-}bi\textbf{ological} \textbf{Problems}\underline{.}
The world u2019s first laws on \textbf{uniform} \textbf{cigarette} and \textbf{tobacco} \textbf{packaging} have \textbf{entered} into force in \textbf{Australia}\underline{,} \textbf{replacing} brand \textbf{logo}\underline{s} and \textbf{colours} with \textbf{neutral} \textbf{olive}\underline{-}\textbf{green} \textbf{lid}\underline{s}, which are also \textbf{printed} with \textbf{drastic} images \textbf{showing} \textbf{sick} body parts and \textbf{infant}\underline{s} and children \textbf{suffering} from \textbf{cigarette} \textbf{smoke}\underline{.}
"\textbf{One} can already see in children of young age that they understand the message that \textbf{tobacco} companies are trying to promote with their brand image," \textbf{says} \textbf{Federal} Minister of \textbf{Health} \textbf{Tan}\underline{ya} P\textbf{lib}\underline{ers}ek.
You will also not receive a share of the 3\textbf{0,000} rupees \textbf{(2}\underline{.}5 \textbf{euros}\underline{)} \textbf{supplement} per camera, which the \textbf{guardian}\underline{s} of this nature park, together with the entry \textbf{fee} of 1\textbf{5,000} rupees \textbf{(1}\underline{.}2 \textbf{euros}\underline{),} demand from the \textbf{tourists} who come to \textbf{photograph} the \textbf{volcano} and the human \textbf{carrying}\underline{.}
The President of \textbf{Ecuador} also \textbf{considers} the desire of his \textbf{Colombia}\underline{n} \textbf{counterpart}\underline{,} \textbf{Juan} \textbf{Manuel} \textbf{Santo}\underline{s}, to be 'ab\textbf{solut}\underline{e}ly \textbf{justified}\underline{'} now and after the \textbf{ruling} of the International Court of \textbf{Justice} in The \textbf{Hague}\underline{,} which favoured the \textbf{maritime} \textbf{sovereignty} of \textbf{Nicaragua} to \textbf{negotiate} \textbf{maritime} borders between the two countries with \textbf{Nicaragua}\underline{.}
He also trusted in a good conclusion to the \textbf{disputes} over the \textbf{maritime} borders between \textbf{Peru} and \textbf{Chile} before the same Court of \textbf{Justice}\underline{,} saying that 'it is right for \textbf{Latin} America to call international authorities if both countries \textbf{commit} to \textbf{adopting} the \textbf{judgment}\underline{,} even if it is very \textbf{harsh}\underline{'}.
After the U.S. Court of \textbf{App}\underline{e}al has \textbf{confirmed} a \textbf{ruling} that does not \textbf{recognise} the \textbf{restructuring} of the \textbf{liabilities} of the Vitro Group, which has been achieved through a commercial exchange rate in \textbf{Mexico}\underline{,} an \textbf{om}\underline{in}ous \textbf{precedent} is set for any national company with \textbf{subsidiaries} in \textbf{neighbouring} countries that has payment problems.
Former construction \textbf{engineer} \textbf{Gill}\underline{es} \textbf{Sur}\textbf{\underline{pre}}\underline{n}ant \textbf{described} this in detail before the Commission: in ten years he received \textbf{gift}\underline{s}, \textbf{invitation}\underline{s} to travel, \textbf{golf} \textbf{tournaments}\underline{,} restaurants and \textbf{ice} \textbf{hoc}\textbf{\underline{key}} games from the construction company, as well as \textbf{bri}\textbf{\underline{bes}} of \$\textbf{76}\textbf{\underline{6,000}} in return for se\textbf{wer}\underline{age} \textbf{contracts}\underline{,} the cost of which he \textbf{artificial}\underline{ly} in\textbf{flat}\underline{ed}.
After \textbf{Bit}\underline{co}in reached a \textbf{peak} of \$30 (\textbf{23} Euro) in June \textbf{2011}\underline{,} it \textbf{fell} to \textbf{\$2} five months later before \textbf{recover}\underline{ing} to about \textbf{\$10} today (the prices are listed on the bitcoin\textbf{chart}\underline{s}.com website).
The \textbf{demonstrators} were also supported by other \textbf{prominent} New York \textbf{democrat}\underline{s}, for example, \textbf{mayor} \textbf{candidate} \textbf{Bill} De \textbf{Bla}\underline{s}io, who said that 'we should \textbf{jointly} support fast-\textbf{food} workers so that they can get a fair \textbf{wage} and achieve the economic \textbf{prosperity} that every New Yorker \textbf{deserves}\underline{!}'
\textbf{Ap}\textbf{\underline{parent}}\underline{ly}, the \textbf{liberal} \textbf{democracies} are \textbf{rapidly} getting into a situation like that \textbf{described} by \textbf{App}\underline{ian} in his work on the crisis of the Roman Republic in the times of \textbf{Caesar} and Pompe\textbf{ius}\underline{:} "The state had long been in dis\textbf{integration} and the \textbf{offices} were \textbf{occupied} by violence.
In order to promote cultural exchange, the Im\textbf{bon}\underline{gi}-C\textbf{hor} travels through \textbf{southern} Africa every two or three years and \textbf{sing}\underline{s} \textbf{songs} full of woes, \textbf{fighting} spirit, confidence and black self-\textbf{conf}\underline{id}ence that many on the \textbf{southern} \textbf{tip} of the black \textbf{continent} still know from the \textbf{era} of \textbf{apart}\textbf{\underline{heid}}\underline{.}
I was ha\textbf{rass}\underline{ed} for just one reason - a reason that \textbf{seemed} all the more \textbf{narrow} and \textbf{cruel} in this \textbf{supposed} \textbf{cra}\textbf{\underline{dle}} of enlightenment: my late \textbf{father} \textbf{Wood}\textbf{\underline{row}} Wy\textbf{att} had been an important \textbf{advise}\underline{r} to \textbf{Margaret} Thatcher and I support the \textbf{Conservative} Party.
"The daily \textbf{wage} of \textbf{mine} workers here, where the \textbf{coffee} \textbf{harvest} \textbf{pays} 1\textbf{5,000} rupees \textbf{(1}\underline{.}2 \textbf{euros}\underline{)} a day and the \textbf{average} \textbf{monthly} income is 2 million rupees \textbf{(16}\underline{7} \textbf{euros}\underline{),} is very high," \textbf{explains} the \textbf{bear}\underline{er} who \textbf{previously} worked as a \textbf{brick}\textbf{\underline{lay}}\underline{er} on the tourist island of \textbf{Bali}\underline{.}
"I wouldn't \textbf{reveal} my deepest \textbf{secret}\underline{s} in a post" \textbf{says} 10-\textbf{year}\underline{-}\textbf{old} \textbf{Jorge} trying to \textbf{explain} the \textbf{meaning} of "\textbf{private}\underline{"} in \textbf{websites} like \textbf{Facebook}\underline{,} \textbf{Twitter}\underline{,} \textbf{Hot}\underline{mail} and Windows \textbf{Live} \textbf{Messenger} where he has had \textbf{accounts} for two years.
"\textbf{Chi}\underline{le} was, is and will continue to be a country that \textbf{abide}\underline{s} by international laws, \textbf{seeks} \textbf{peaceful} solutions to \textbf{disputes}\underline{,} \textbf{conclude}\underline{s} agreements and \textbf{submit}\underline{s} to international \textbf{courts}\underline{,}" Pi  u20\textbf{47} \textbf{era} \textbf{adds}\underline{,} and \textbf{greet}\underline{ed} \textbf{Hum}\textbf{\underline{ala}} with a \textbf{hands}\textbf{\underline{hak}}\underline{e} in front of the \textbf{flag}\underline{s} of both countries.
"\textbf{We} have decided to give priority to a number of 31 \textbf{emblemati}\underline{c} projects aimed at improving \textbf{geographical} links in South America and, in particular, in rural and border areas...to \textbf{unite} our countries and open up new economic forms," said the \textbf{Peru}\textbf{\underline{via}}\underline{n} President in a read-out statement.
He also \textbf{criticised} the \textbf{Swedish} \textbf{judiciary}\underline{,} which asked him to be inter\textbf{rog}\underline{ated} on his \textbf{territory} for a \textbf{alleged} \textbf{sexual} of\textbf{fence}\underline{,} while 'S\textbf{wed}\underline{es}' case law allowed this to be done by means of a video conference which could have been carried out via the \textbf{Ecuador} \textbf{Embassy} in London'.
He makes a \textbf{striking} statement: 'Nine out of ten \textbf{patients} come to us if they already have an \textbf{accompanying} \textbf{infection}\underline{;} in order to influence global \textbf{mortality}\underline{,} more early \textbf{diagnosis} is required, and so all those who need it must be offered \textbf{massive} \textbf{detection} \textbf{tests}\underline{'}.
In practice, \textbf{Jud}\underline{ge} \textbf{Har}\underline{lin} \textbf{Hal}\underline{e} u2019s \textbf{recognition} of the \textbf{ruling} in \textbf{Ban}\underline{car}\textbf{rot}\underline{as} on 15 June for the \textbf{northern} \textbf{district} of \textbf{Texas} \textbf{leads} \textbf{Mexican} companies to be help\textbf{lessly} \textbf{exposed} to confi\textbf{sc}\underline{ation} of their property beyond the \textbf{river} \textbf{Bra}\underline{vo}.
But \textbf{Char}\underline{m} xe9 had no idea what he should expect in the following two months: the \textbf{destructive} H\textbf{urri}\textbf{\underline{can}}\underline{e} \textbf{Sand}\underline{y}, which some have called "de\textbf{uda}\underline{r}ma\textbf{gged}\underline{on}," and a growing conflict \textbf{involving} Israel, the place that \textbf{Christian} theorists believe the apocal\textbf{yp}\underline{se} is beginning.
I had \textbf{looked} at \textbf{websites} and \textbf{blog}\underline{s} when \textbf{someone} \textbf{drew} my attention and proposed to come to the "B\textbf{ego}\underline{wa}ja" station where a person would \textbf{wait} for me to take me to a certain place where we could then \textbf{negotiate} the price.
- Of course it is not pleasant to always keep a \textbf{smart}\textbf{\underline{phone}} in your hand on the road, but I think that the best way to do this would be to have a '\textbf{change}\underline{d}' \textbf{extended} reality where we could \textbf{switch} from a \textbf{cloud} of \textbf{glass}\underline{es} to a \textbf{smart}\textbf{\underline{phone}}\underline{,}
"A law must be valid, and if something is \textbf{forbidden} by law, it cannot simply come from the President of the Government, and the control office, whose duty is to control \textbf{compliance} with the law, \textbf{hinder}\underline{s} its activities," \textbf{Kal}\underline{a} states.
\textbf{Temperatur}\underline{es} will remain below \textbf{zero} even in lower \textbf{locations}\underline{,} so that \textbf{snow} and \textbf{ice} will remain on the \textbf{roads}\underline{.}
The \textbf{reck}\underline{less} practice of private capital \textbf{creates} a situation in individual \textbf{economies} in which governments are \textbf{forced} to \textbf{compete} with each other in order to \textbf{artificial}\underline{ly} reduce the social level of their own people and thus \textbf{attract} foreign capital.
We must \textbf{admit} that we are living in a time when the \textbf{wealth} of the world is \textbf{concentrated} in the \textbf{hands} of a few \textbf{individuals}\underline{,} and that this \textbf{concentration} of money and the power that \textbf{emerge}\underline{s} from it has not been created within the life\textbf{span} of a \textbf{generation}\underline{.}
The first press \textbf{agency} (Re\textbf{uter}\underline{s}) was \textbf{bought} by the \textbf{Roth}\textbf{\underline{schild}}\underline{s} as long ago as the 1990s in order to prevent the connection of their name with highly criminal \textbf{acts}\underline{,} whose \textbf{background} was always the \textbf{consolidation} of their power, the increase of their \textbf{wealth} or both.
The EU \textbf{apparatus} often decides under the pressure of this or that commercial and industrial \textbf{lobby} whose \textbf{claims} are usually \textbf{represented} in \textbf{Brussels} by one or more Member States (for example, the Czech Republic is currently trying to \textbf{impose} the demands of Czech banks even with a \textbf{veto} \textbf{threat}\underline{).}
In the official list of products \textbf{registered} in the EU, there are now also \textbf{Karl}\underline{ov}y Vary Zwie\textbf{back}\underline{,} Poho  u20\textbf{47} elice and T  u20\textbf{47} ebo  u20\textbf{47}  carp and Sa\textbf{az} hops in the company of world-\textbf{famous} \textbf{cheese}\underline{s} such as \textbf{Fe}\underline{ta} and \textbf{Gor}\textbf{\underline{gon}}\underline{z}ola, L xfcbeck \textbf{mar}\textbf{\underline{zip}}\underline{an} or \textbf{Par}\underline{ma} \textbf{ham}\underline{.}
On 21 November, \textbf{Chief} O\textbf{ates} sent an e-mail to his staff in Aur\textbf{ora} de\textbf{cla}\underline{ring} that the public \textbf{prosecutor} would no longer \textbf{prosecut}\underline{e} \textbf{minor} \textbf{mar}\underline{i}juana \textbf{offences} against persons over 21 years of age, and that the police would not "as of now" \textbf{seek} criminal \textbf{charges} for these \textbf{offences}\underline{.}
\textbf{Once} you have \textbf{arrived}\underline{,} you will find a path between the \textbf{tourists} \textbf{photograph}\underline{ing} them like \textbf{circus} apes and you will walk three \textbf{kilometres} with the \textbf{tir}\underline{ing}ly \textbf{heavy} \textbf{basket}\underline{s} to the \textbf{scale} that a \textbf{mine} company has placed a little further down at an \textbf{altitude} of 1850 \textbf{meters}\underline{.}
While the \textbf{judge} of the case points out that creditors must be subject to the \textbf{bankruptcy} law of the United States, the New \textbf{Orleans}\underline{-}based \textbf{Fifth} \textbf{Circ}\textbf{\underline{uit}} Court of \textbf{App}\underline{e}al \textbf{initially} \textbf{says} that the main \textbf{proceedings} are the trade exchange rate \textbf{treated} in \textbf{Mexico}\underline{.}
The company's \textbf{spoke}\underline{s}man, \textbf{Dan} \textbf{Fo}\underline{gel}man, \textbf{claimed} in an \textbf{interview} on the website of the left-\textbf{wing} H\textbf{uff}\textbf{\underline{ington}} Post that all "less than five" \textbf{Wal}\underline{mar}t employees \textbf{laid} down the work and the \textbf{protest} action was only "an additional \textbf{PR} \textbf{trick}\underline{"} of the \textbf{union} that \textbf{organized} the \textbf{protests}\underline{.}
This is a state of \textbf{affairs} in which the \textbf{manufacturer} \textbf{tries} to \textbf{compete} \textbf{economically} by \textbf{import}\underline{ing} \textbf{cheap} goods by '\textbf{under}\textbf{\underline{cut}}\underline{ting}' competition in order to \textbf{gain} a greater market share and increase its \textbf{profits}\underline{.}
While the rest of the \textbf{Arab} world is taking \textbf{tim}\underline{id} steps towards \textbf{democratisation}\underline{,} \textbf{Palestinians} are still being \textbf{deprived} of their right to self-\textbf{determination} - a \textbf{powder} k\textbf{eg} that will \textbf{undoubtedly} one day \textbf{explode} in \textbf{Israeli}\underline{-}o\textbf{ccupied} \textbf{territories}\underline{,} just as a bus \textbf{explode}\underline{d} in \textbf{Tel} A\textbf{viv} this week.
\textbf{Kevin} A. Sa\textbf{bet}\underline{,} a former \textbf{Obama} administration \textbf{drug} policy \textbf{advise}\underline{r}, \textbf{believes} that while criminal \textbf{officers} are \textbf{unlikely} to open \textbf{doors} to confi\textbf{sc}\underline{ate} small \textbf{quantities} of \textbf{drugs}\underline{,} they are likely to be \textbf{reluctant} to \textbf{tolerate} legal, state-\textbf{reg}\textbf{\underline{ulate}}\underline{d} \textbf{mar}\underline{i}juana \textbf{deals} under new legislation.
It states that this is a complex issue 'because we are \textbf{asking} them to have a \textbf{defined} \textbf{criterion} on what can be \textbf{disseminat}\underline{ed}, published or said, and this at an age when the \textbf{maturity} is not \textbf{sufficient}\underline{'}.
Cor\textbf{rea}\underline{,} who took part in the \textbf{Sixth} \textbf{Summit} of Presidents of the Union of South American Nations (Una\textbf{sur}\underline{)} held in \textbf{Lima}\underline{,} \textbf{explained} to \textbf{Peru}\underline{'}s state \textbf{television} that Europeans were '\textbf{kill}\underline{ed} in the \textbf{Second} World War and in other \textbf{clash}\underline{es}' and 'today are \textbf{practically} a \textbf{father} country'.
In \textbf{Lima} today, the \textbf{Ecuador}\underline{ian} \textbf{Head} of State took part in the \textbf{Sixth} \textbf{Summit} of \textbf{Heads} of State or Government of the Union of South American Nations (Una\textbf{sur}\underline{),} which \textbf{ended} with the call for greater regional integration to ensure sustainable progress, \textbf{equality} and security.
At the University of \textbf{Pennsylvania} u2019s main \textbf{campus}\underline{,} the \textbf{professor} of \textbf{Latin} American history \textbf{Matthew} Re\textbf{stall} and his \textbf{colleague} Am\textbf{ara} \textbf{Solar}\underline{i}, a \textbf{professor} in art history and anthrop\textbf{ology}\underline{,} have \textbf{formed} a team to offer a course called  u201cThe End of the World u201d.
And in the other, the \textbf{Bos}\underline{ons}, an \textbf{evil} gang of an\textbf{arch}\underline{ists} to whom nothing is \textbf{sacred} - certainly not this principle, which means that they can actually be in the same place at the same time.
It is said that 7\textbf{7\%} of \textbf{Canadian}\underline{s} do not have access to \textbf{pal}\underline{li}ative care, that is to say, care to \textbf{relieve} the \textbf{suffering} of \textbf{patients} when they have reached the final stage of their lives, both at home, in \textbf{hospital} or in a nursing home.
It is my \textbf{intention} to open the \textbf{reader} u2019s \textbf{gaze} behind the \textbf{scenes}\underline{,} to look at who the \textbf{95}\underline{-}\textbf{year} \textbf{tension} (since the \textbf{Bal}\textbf{\underline{four}} \textbf{Declaration} in November \textbf{1917}\underline{)} in the small region of the Middle East is especially useful.
One \textbf{candidate} for the \textbf{victory} in this \textbf{poll} may be last year's EU regulation, which, according to \textbf{balloon}\underline{s}, must be \textbf{accompanied} by a \textbf{notice} that children under the age of \textbf{eight} may not in\textbf{flat}\underline{e} the \textbf{balloon} without the \textbf{supervision} of an \textbf{adult}\underline{.}
\textbf{Win}\underline{y} Maas of the \textbf{Rotterdam} \textbf{architectural} office \textbf{MV}\underline{R}DV, \textbf{master} of \textbf{fantastic} bar \textbf{chart}\underline{s} and \textbf{producer} of \textbf{funny}\underline{,} often \textbf{cynical} \textbf{buildings}\underline{,} took the matter with \textbf{usual} \textbf{ser}\underline{en}ity and \textbf{appeared} to the competition-hearing anno 2003 with five \textbf{books} under your \textbf{arm} and a \textbf{gr}\underline{in} in your face.
"Om'O\textbf{ban}\underline{i}" is not a simple \textbf{piece}\underline{,} each \textbf{chor}\underline{al} voice has a different text and this one is also in a very foreign language: Zulu, which is \textbf{spoken} by \textbf{eleven} million people in South Africa, \textbf{Bot}\underline{s}\textbf{wan}\underline{a}, \textbf{Les}\underline{ot}ho, Mala\textbf{wi}\underline{,} \textbf{Mozambique} and in parts of Swaziland.
The \textbf{judge}\underline{,} \textbf{Colon}\underline{el} Denise \textbf{Lind}\underline{,} also asked Manning why he did not \textbf{complain} about his treatment when he met with a committee in January \textbf{2011} to \textbf{investigate} the \textbf{suicide} ideas he mentioned a few months earlier on a form.
During \textbf{Friday} u2019s \textbf{interview}\underline{,} Manning stated that he had closed from a \textbf{guard} order that he should \textbf{drop} the \textbf{ceiling} with which he could have covered \textbf{himself}\underline{,} but he \textbf{admitted} that no one had asked him to do so.
It has even \textbf{gone} so far as to pay Ukraine, \textbf{Honduras} and the \textbf{Dominican} Republic to challenge the new rules - those countries \textbf{complain} to the World \textbf{Trade} Organisation about \textbf{unfair} trade \textbf{restrictions}\underline{,} even though \textbf{none} of the countries trade more with \textbf{Australia}\underline{.}
If you try to focus on a difficult or ard\textbf{uous} task, attention \textbf{disorder} can lead to \textbf{bo}\underline{re}\textbf{dom}\underline{,} \textbf{says} \textbf{Mark} J. Fenske, \textbf{Associate} \textbf{Professor} of \textbf{Neuro}\textbf{\underline{science}}\underline{s} at University of \textbf{Gu}\underline{el}ph in \textbf{Ontario} and one of the \textbf{authors} of the study.
And \textbf{unpleasant} practical issues need to be \textbf{clarified} at this time - for example, how to agree on the state \textbf{requirement} of 'appro\textbf{pri}\underline{ate} access' to \textbf{licensed} \textbf{mar}\underline{i}juana with the ban on canna\textbf{bis} sales within a \textbf{radius} of 300 metres around \textbf{schools}\underline{,} \textbf{parks}\underline{,} \textbf{playground}\underline{s} and \textbf{childcare} facilities.
\textbf{Both} my \textbf{father} and my \textbf{older} \textbf{brother} had \textbf{visited} what I once thought was the largest \textbf{temple} of knowledge in the world, a modern \textbf{Greek} \textbf{sy}\underline{m}\textbf{pos}\underline{ium} that \textbf{promoted} the great \textbf{pillars} of \textbf{civilisation} - free thought and \textbf{tolerance}\underline{.}
Last October, \textbf{Peru} \textbf{hosted} the \textbf{Third} \textbf{Summit} between South America and \textbf{Arab} States (\textbf{AS}\textbf{\underline{PA}}\underline{),} and even on that \textbf{occasion} the so-called \textbf{Lima} \textbf{Declaration}\underline{,} which had been \textbf{announced} \textbf{previously}\underline{,} was not published, despite the press's strong call.
After several months of no progress has been made in \textbf{advertisement}\underline{s} by \textbf{Mexican} air transport \textbf{unions} against former \textbf{owner} Gast xf3n \textbf{Az}\underline{c} xe1rr\textbf{aga} Andrade, \textbf{accused} of \textbf{fraudulent} administration, the Asociaci xf3n \textbf{Sind}\underline{ical} de \textbf{Pilot}\underline{os} \textbf{Avi}\textbf{\underline{adores}} has finally made progress.
\textbf{Born} on September 21, 19\textbf{31} in Forth Worth (Texas), La\textbf{rry} \textbf{Hag}\underline{man} became world famous for his role as John \textbf{Ros}\underline{s} E\textbf{wing}\underline{,} better known as "J.R.
When the answer became known in a \textbf{chapter} in November 1990, it was seen by an \textbf{average} of \textbf{41} million viewers who \textbf{transformed} "\textbf{Da}\textbf{\underline{lla}}\underline{s}" into the second most \textbf{visible} \textbf{entertainment} program since the end of "\textbf{MA}\textbf{\underline{SH}}\underline{"} in \textbf{1983}\underline{,} which had 50 million viewers.
\textbf{Jacques} Du\textbf{ches}\underline{n}\textbf{eau}\underline{,} for his part, \textbf{notes} that "\textbf{office}\underline{rs} have \textbf{stolen} \textbf{hundreds} of \textbf{millions} of \textbf{dollars}\underline{",} but above all he is concerned about the role of the "\textbf{sign}\textbf{\underline{atori}}\underline{es} who are aware of the \textbf{ta}\textbf{\underline{ctic}}\underline{s}" if they were not involved in the \textbf{fraud}\underline{!}
In fact, the \textbf{Bit}\underline{co}in \textbf{invented} by Sato\textbf{shi} Naka\textbf{moto} (a \textbf{pseudo}\underline{n}\textbf{ym}\underline{)} is both a \textbf{virtual} currency (\textbf{but} \textbf{convert}\textbf{\underline{ible}} in \textbf{dollars}\underline{,} \textbf{euros}\underline{,} etc.) and a \textbf{protocol} for safe exchange such as \textbf{Bit}\textbf{\underline{Torrent}}\underline{,} which allows for the direct exchange of files.
If a user \textbf{wants} to \textbf{cheat} \textbf{twice} very quickly (less than 10 minutes) with the same money, only one of the two \textbf{transactions} would be validated by the network and the other would not be linked because they have different \textbf{fingerprint}\underline{s}.
The comment\textbf{ators}\underline{,} \textbf{incidentally}\underline{,} found it \textbf{entertaining} that the only \textbf{difference} of opinion of the day... was expressed at the time of \textbf{prayer}\underline{,} because some members of the body \textbf{felt} that the \textbf{clock} of the \textbf{constituent} \textbf{assembly} was not \textbf{accurate}\underline{.}
A law must be valid, and if something is \textbf{forbidden} by law, then it cannot simply be the President of the government and the control office, whose duty is to \textbf{monitor} \textbf{compliance} with the law, that \textbf{hinder}\underline{s} its activities.
\textbf{Thus}\underline{,} the faceless small town \textbf{rescue} station, which has so far had no more to offer than a post-\textbf{modern} \textbf{pedestrian} \textbf{zone} and a \textbf{sta}\textbf{\underline{gger}}\underline{ing}ly ugly town \textbf{hall} behind whose white fa  u20\textbf{47} ades one would be \textbf{inclined} to \textbf{assume} a \textbf{dairy} \textbf{factory} to \textbf{enrich} a \textbf{piece} of \textbf{contemporary} \textbf{architecture}\underline{.}
"But oil is not the only reason why we are so good," \textbf{says} \textbf{Anna}\underline{,} our \textbf{wait}\underline{er} who \textbf{distribute}\underline{s} round tablets with \textbf{rip}\underline{e} \textbf{rak}\underline{fi}sk and e\textbf{mbo}\textbf{\underline{dies}} the \textbf{Nordic} ideal with her long \textbf{blo}\textbf{\underline{nde}} \textbf{hair} and \textbf{st}\underline{ing}ing \textbf{blue} \textbf{eyes}\underline{.}
On \textbf{Friday}\underline{,} the Public \textbf{Prosecutor} \textbf{tried} to find that the \textbf{army}\underline{-}\textbf{lib}\underline{er}ated \textbf{Brad}\underline{ley} Manning - in\textbf{dic}\underline{ted} for the \textbf{greatest} \textbf{disclosure} of \textbf{confidential} information in American history - \textbf{missed} several opportunities to \textbf{complain} about the \textbf{ill}\underline{-}treatment he \textbf{alleged}\underline{ly} \textbf{suffered} in military \textbf{detention}\underline{.}
One day before the cross-ex\textbf{ami}\textbf{\underline{nation}}\underline{,} which was held as a result of a \textbf{defense} request to deport the in\textbf{dic}\underline{t}ment - mening had already been \textbf{sufficiently} \textbf{punished} by the \textbf{harsh} period of \textbf{detention} - Manning said that he had considered \textbf{suicide} in \textbf{prison}\underline{.}
In the \textbf{hearing} on \textbf{Friday}\underline{,} \textbf{Fein} \textbf{went} through with Manning the forms that \textbf{officials} had \textbf{filled} out after meeting with Manning during his \textbf{detention} in the \textbf{Qua}\underline{n}\textbf{tico} military \textbf{prison}\underline{,} where he had been under \textbf{stronger} \textbf{prison} conditions from July 2010 to April \textbf{2011}\underline{.}
Most \textbf{Americans} probably never waste a single thought that the United States inva\textbf{ded} \textbf{Mexico} in 18\textbf{48} and \textbf{forced} the country u2019s leaders to hand over more than half of their \textbf{territory}\underline{.}
The people who \textbf{watch}\underline{ed} the \textbf{scarce}\underline{ly} aud\textbf{ible} \textbf{television} \textbf{indicated} that they \textbf{felt} more \textbf{bo}\underline{re}\textbf{dom} than the other two groups - they had problems \textbf{concentrating}\underline{,} could not find any reason for them and \textbf{admitted} their \textbf{difficulties} to \textbf{bo}\underline{re}\textbf{dom}\underline{.}
The 19-\textbf{year}\underline{-}\textbf{old} Community \textbf{College} \textbf{student} and \textbf{football} player \textbf{Anthony} O\textbf{roz}\underline{co} is on \textbf{trial} in south-\textbf{east} \textbf{Color}\textbf{\underline{ados}} for an of\textbf{fence} that will soon be legal in that state: the \textbf{possession} of a few \textbf{mar}\underline{i}juana \textbf{bro}\underline{ok}s and a \textbf{pipe} with which he \textbf{ra}\textbf{\underline{ged}} them.
This was \textbf{recognized} by the \textbf{designer} at the opening of "\textbf{Val}\underline{en}\textbf{tino} - \textbf{Master} of \textbf{Cou}\underline{ture}", a \textbf{grandiose} \textbf{retro}\textbf{\underline{spect}}\underline{ive} for which more than \textbf{130} \textbf{skin} \textbf{cou}\underline{ture} \textbf{clothes} were \textbf{assembled}\underline{,} created by his "Ma\textbf{ison}\underline{"} over the last 50 years.
"\textbf{It} is \textbf{incomprehensible} that the Inter-\textbf{American} Commission on Human Rights is based in \textbf{Washington} and is \textbf{funded} by the United States," he said as an allusion to the political \textbf{asylum} that \textbf{Ecuador} has \textbf{granted} to the \textbf{founder} of \textbf{Wiki}\textbf{\underline{Le}}\underline{ak}s, \textbf{Julian} Ass\textbf{ange}\underline{.}
I have just \textbf{spoken} to the \textbf{Vice}\underline{-}\textbf{President} of \textbf{Venezuela}\underline{,} \textbf{Nico}\underline{l} xe1s \textbf{Mad}\textbf{\underline{uro}}\underline{,} who has \textbf{told} me that he has been there for \textbf{planned} \textbf{routine} treatment and that he is expected to be able to return to \textbf{Cuba} after the \textbf{election} \textbf{campaign}\underline{.}
It also points out that the country has been subject to the principles of the United Nations Commission on International \textbf{Trade}\underline{,} that is to say, to the rules \textbf{laid} down for cases of cross-\textbf{border} in\textbf{sol}\underline{v}\textbf{ency}\underline{,} which guarantee \textbf{equality} between debtors and creditors.
Prev\textbf{ious}\underline{ly}, Canacintra (the National \textbf{Chamber} of \textbf{Process}\underline{ing} \textbf{Industry}\underline{)} managed to \textbf{unite} the \textbf{governor}\underline{s} in the south-\textbf{east} in order to \textbf{resist} the \textbf{monumental} \textbf{institution} that \textbf{destroyed} some of the protected areas and was the \textbf{mother} of all the industrial \textbf{threats}\underline{.}
For several years, he has paid \textbf{3\%} of the value of the \textbf{contracts} received in \textbf{Montreal} to a mediator \textbf{associated} with the \textbf{Mafia} who \textbf{transferred} the money to the Union of \textbf{Montreal}\underline{,} the party of \textbf{mayor} G xe9\textbf{ral}\underline{d} \textbf{Tre}\underline{mb}\textbf{lay}\underline{.}
The \textbf{Quebec} Government \textbf{proposes} to limit \textbf{contributions} to parties to \$\textbf{100}\underline{,} which, according to it, would not change the situation: '\textbf{For} as long as \textbf{electoral} \textbf{spending} is not \textbf{strictly} limited, black money will be in \textbf{circulation} in \textbf{politics}\underline{.}'
The \textbf{glass}\underline{es} are a personal \textbf{ga}\underline{d}\textbf{get} and therein lies their \textbf{strength} (\textbf{private}\underline{s} can only see you), but at the same time their \textbf{weakness}\underline{,} because an \textbf{extended} reality through \textbf{glass}\underline{es} prevents you from working with others on \textbf{virtual} \textbf{objects}\underline{.}
As far as the authorities are concerned, the German \textbf{counterpart} to the \textbf{NK}  u20\textbf{47}  is the \textbf{Bundes}\textbf{\underline{rechnung}}\underline{s}hof, which is similar to our own and also has a \textbf{college} which is only \textbf{formed} \textbf{slightly} \textbf{differently}\underline{,} but in principle both authorities work in a similar way.
\textbf{Next} year we would also like to appear in the Czech House in New York, and I \textbf{personally} - if we are in the USA - would like to \textbf{combine} this with \textbf{appearance}\underline{s} in \textbf{Washington} and \textbf{Chicago}\underline{.}
Last week, at a meeting of the Council of \textbf{Ministers} of the Member States of the European \textbf{Space} \textbf{Agency} (ESA), \textbf{Poland} was accepted as the 20th member of this space \textbf{agency}\underline{,} making it the second member country from the former \textbf{Eastern} \textbf{bloc} (\textbf{after} the Czech Republic, which became an ESA member on 12 November 2008).
\textbf{Who} is the \textbf{cul}\textbf{\underline{pri}}\underline{t} and who is the \textbf{victim} of the conflict between \textbf{Palestinians} and \textbf{Israeli}\underline{tes}, where \textbf{injustice} only \textbf{causes} \textbf{injustice} in an \textbf{endless} \textbf{spiral} of violence, with the \textbf{gre}\underline{ed} of \textbf{individuals} and their desire for global power \textbf{initially}\underline{?}
As a result, the \textbf{mood} levels in the film change - on the one hand, the \textbf{documentary} \textbf{scenes} from Te\textbf{hra}\underline{n} (in the title \textbf{sequence}\underline{,} \textbf{icon}\underline{ic} \textbf{contemporary} \textbf{photographs} are shown, and there are no big \textbf{differences} in the film version of the same \textbf{situations} either).
And while the \textbf{jury} was still \textbf{tired} of looking around and \textbf{cla}\textbf{\underline{pping}} with the axes, the n\textbf{aught}\underline{y} Maas \textbf{stack}\underline{ed} his \textbf{exquisite} bringr of size into a \textbf{pyramid} and \textbf{ended} his actionist-\textbf{back}\underline{ed} \textbf{speech} with the words '\textbf{lov}\underline{e} town community!'
During a joint trip to Africa in the \textbf{spring} of 2005, the \textbf{choir} \textbf{discovered} the village, but above all the Im\textbf{bon}\underline{gi}s \textbf{saw} many children on the \textbf{streets} who were not only \textbf{lacking} in \textbf{parent}\underline{al} care, but also in everything: food, \textbf{clothing}\underline{,} education.
However, it does not \textbf{seem} \textbf{plausible} from a \textbf{nutrition}\underline{al} point of view that it is precisely the high-cal\textbf{ori}\underline{e} diet of the Talytes that should be so \textbf{healthy}\underline{,} which love \textbf{meat}\underline{,} \textbf{bread} and especially \textbf{dairy} products and many of which \textbf{drink} a \textbf{glass} of \textbf{mel}\underline{ted} \textbf{butter} every day.
During \textbf{Governor} \textbf{Pen}\underline{a} \textbf{Nie}\underline{to}'s term of office, over \textbf{1,000} women were \textbf{murdered} in the state of \textbf{Mexico} - a \textbf{statistic} that even \textbf{exceed}\underline{s} that of the city of \textbf{Ciudad} \textbf{Ju}\underline{are}z, which is \textbf{notorious} for its violence and the \textbf{murder}\underline{s} of \textbf{innocent} women.
During a cross-ex\textbf{ami}\textbf{\underline{nation}} of Manning during a pre-ju\textbf{dic}\underline{ial} \textbf{hearing} in Ft. Me\textbf{ade}\underline{,} \textbf{Mary}\underline{land}, \textbf{Maj}\underline{.} \textbf{Ash}\underline{den} \textbf{Fein} stated that there were no \textbf{complaints} about his treatment in respect of \textbf{weekly} \textbf{visits} made by civil \textbf{servant}\underline{s} during Manning u2019s \textbf{nine}\underline{-}\textbf{month} \textbf{detention} in \textbf{Qua}\underline{n}\textbf{tico}\underline{,} \textbf{Virgin}\underline{ia}.
Some groups heard a \textbf{loud} TV from the \textbf{adjacent} room, which had nothing to do with the content; others heard it at low \textbf{volume}\underline{,} so it was \textbf{bare}\underline{ly} per\textbf{cept}\textbf{\underline{ible}}\underline{,} while the third group did not hear it at all.
In \textbf{1991} \textbf{Reed} Larson, a \textbf{professor} of human and community development at the University of \textbf{Illinois}\underline{,} carried out an \textbf{experiment} in which he contacted almost \textbf{400} \textbf{teenagers} and their \textbf{parents} \textbf{seven} to \textbf{eight} times a day with a pager.
\textbf{District} \textbf{prosecutor}\underline{s} are a "\textbf{cultural} \textbf{barrier}\underline{,}" \textbf{says} Sean \textbf{Mc}\textbf{\underline{All}}\textbf{\underline{ister}}\underline{,} a Denver \textbf{lawyer} who represents \textbf{defend}\textbf{\underline{ants}} in \textbf{court} for \textbf{mar}\underline{i}juana \textbf{offences} and \textbf{acts} on the ground as \textbf{spoke}\underline{s}\textbf{person} for the national \textbf{organisation} for the reform of \textbf{mar}\underline{i}juana laws.
But within two weeks of my \textbf{arrival} at \textbf{Wor}\underline{s}cester \textbf{College} at the end of the \textbf{1980}\underline{s} - where I had \textbf{planned} to study history - I \textbf{packed} my \textbf{suit}\textbf{\underline{case}}\underline{s} again, \textbf{causing} the first \textbf{scandal} of my life.
At least in the last 12 years, we have not had problems with the supply of \textbf{medicines}\underline{,} and the problem is that people are in an \textbf{advanced} state because they do not know their \textbf{infectious} state, that is to say at very late \textbf{stages} of the \textbf{disease}\underline{.}
The \textbf{sooner} they know if they are \textbf{HIV} positive, the better, and if they already know the \textbf{diagnosis}\underline{,} they should learn how to live in a responsible way like all people.
Secondly, the \textbf{judgment} \textbf{stipulat}\underline{es} that, without the \textbf{votes} of the companies, the necessary majority for the \textbf{restructuring} of \textbf{liabilities} would not have been achieved without the \textbf{recognition} of the \textbf{liabilities} in the \textbf{bankrupt} mass that the Vitro \textbf{branches} had with their \textbf{parent} company.
In fact, \textbf{25\%} of \textbf{African}\underline{-}\textbf{American}\underline{s}, \textbf{15\%} of those with an income of less than \$3\textbf{5,000}\underline{,} 18\% of citizens over \textbf{65}\underline{,} and \textbf{20\%} of \textbf{voters} between 18 and 29 do not have the required photo \textbf{identification}\underline{.}
As \textbf{mayor} of the \textbf{district} of Rivi xe8re-des-Prairies, in the \textbf{east} of the island, she \textbf{opposed} the \textbf{sale} of a \textbf{municipal} property from 2010 \textbf{onwards} that was \textbf{bought} for \$5 million and \textbf{sold} on to \textbf{1.6} million \textbf{developers} in the \textbf{boom}\underline{ing} property market.
They have \textbf{transformed} themselves into business \textbf{makers} by confi\textbf{sc}\underline{ating} government land to \textbf{sell} them as land to \textbf{refugees} from Iran and Pakistan, thus benefiting from \textbf{massive} American sub\textbf{contract}\underline{ing}.
With this \textbf{recourse} to a hasty vote, the \textbf{Egyptian} people are being given an u\textbf{ltima}\textbf{\underline{tum}}\underline{:} '\textbf{You} either vote in favour of my draft or I \textbf{retain} \textbf{unlimited} power', which should \textbf{supposedly} end after \textbf{adoption} of the \textbf{Constitution}\underline{.}
The path \textbf{begins} at the Roman \textbf{fortress} \textbf{Antoni}\underline{a}, Pre\textbf{torium} where the \textbf{court} was, and \textbf{leads} through the \textbf{streets} of the old town to the \textbf{Church} of the Tomb on the \textbf{hill} \textbf{Gol}\underline{go}\textbf{tha}\underline{,} where there is the \textbf{cru}\underline{ci}\textbf{fix}\underline{ion}, the ano\textbf{int}\underline{ment} \textbf{stone} and the tomb of \textbf{Jesus}\underline{.}
"At home you are \textbf{promised} one thing, and on \textbf{arrival} you will be deceived, your \textbf{passport}\underline{s} will be taken off and you will not get the \textbf{promised} pay," \textbf{confirm}\underline{s} To\textbf{lib} \textbf{Schw}\underline{ari}pov, head of the \textbf{Department} of \textbf{Labour} \textbf{Migration} of Ta\textbf{ji}\underline{k}\textbf{istan}\underline{.}
It may even be that, in this way, we only \textbf{burden} the system with \textbf{excessive} 'paper\textbf{work}\underline{'}, and those who \textbf{seek} \textbf{gap}\underline{s} in the system will have it much \textbf{easier} to \textbf{exploit} the system than if the \textbf{threshold}\underline{s} are higher.
J.F. \textbf{Kennedy} began to issue his own bank\textbf{note}\underline{s} and wanted to \textbf{abolish} the F\textbf{ED} - he was \textbf{murdered} in \textbf{1963}\underline{;} \textbf{Louis} \textbf{Mc} Fadden was \textbf{poison}\underline{ed} in 19\textbf{36} after he \textbf{tried} to sue the F\textbf{ED} for \textbf{trigger}\underline{ing} the Great \textbf{Depression} in \textbf{1929}\underline{.}
Israel was \textbf{founded} in \textbf{1948}\underline{,} and just as war re\textbf{par}\underline{ations} against Germany provided the ground for the \textbf{Second} World War, the \textbf{declaration} of the State of Israel is the \textbf{focal} point for the \textbf{Third} World War.
If international \textbf{bankers} \textbf{succeed} in \textbf{unleash}\underline{ing} this war, the \textbf{Jewish} people will become victims in the front line, this time along with the \textbf{Arab} or \textbf{Muslim} population of the Middle East, as they did in the \textbf{Second} World War.
There was no positive way out of this situation for the American Government - it could not \textbf{afford} to \textbf{throw} the \textbf{Sha}\underline{h} overboard, as it would have \textbf{greatly} \textbf{damaged} the confidence of its \textbf{allies} in other countries.
"The EU's recent plan to introduce \textbf{40\%} of women in the management of large European companies brought us this idea," said \textbf{Patri}\underline{k} Nacher, who is responsible for \textbf{organising} this \textbf{survey}\underline{,} to the \textbf{newspaper} \textbf{Pr} xe1vo.
And although we may now have \textbf{lived} the American \textbf{dream}\underline{,} \textbf{visited} good \textbf{schools} and had good jobs, we must never \textbf{lose} \textbf{sight} of the fact that it is the American \textbf{dream} we are living - not the \textbf{Mexican} \textbf{dream}\underline{.}
\textbf{Us}\underline{ing} such \textbf{scale}\underline{s}, \textbf{researchers} have \textbf{discovered} that \textbf{boys} become \textbf{bo}\underline{ring} more often than \textbf{girls}\underline{,} according to \textbf{Stephen} \textbf{Vo}\underline{da}\textbf{nov}\underline{ich}, \textbf{Professor} of \textbf{Psycho}\textbf{\underline{logy}} at the University of West\textbf{flo}\underline{r}\textbf{ida} - especially as regards the need for more and a greater variety of external \textbf{stimuli}\underline{.}
It then \textbf{sell}\underline{s} it for \textbf{10,000} rupees (\textbf{83} euro \textbf{cent}\underline{s}) to the petro\textbf{chemical} industry, because this \textbf{mineral} is \textbf{widely} used in \textbf{everyday} life and is used for the \textbf{manufacture} of \textbf{string}\underline{-}\textbf{wood}\underline{s}, \textbf{fire}\textbf{\underline{work}}\underline{s}, \textbf{cosmetic}\underline{s}, \textbf{dynamic}\underline{s} and even for \textbf{ble}\underline{ach}ing \textbf{sugar}\underline{.}
He is able to carry up to \textbf{110} \textbf{kg} and \textbf{assure}\underline{s} that he will continue "as long as possible" because he needs the money to \textbf{raise} his three children a\textbf{ged} between 10 and \textbf{18.}
"The free movement of citizens and workers in all South American countries must be achieved, as is already the case in the Andean Community, but there are still \textbf{reaction}\underline{ary} sectors \textbf{seeking} a return to the past," he \textbf{warned}\underline{.}
Then came the 1990 World \textbf{Cup}\underline{,} where we took \textbf{fourth} place, which should have been \textbf{bronze} had it not been for this \textbf{Canadian} referee who had us \textbf{repeat} the last \textbf{match} for the second time, \textbf{Rey}\underline{es} said.
In addition, these laws also reduce the time\textbf{scale}\underline{s} for early \textbf{votes}\underline{,} \textbf{declare} in\textbf{valid} the right to \textbf{register} as \textbf{voters} on \textbf{election} day, and deny citizens the right to vote for which \textbf{court} \textbf{acts} are available.
Finally, this is the last p\textbf{article} whose \textbf{existence} has been \textbf{predicted} by the standard model - our best or least \textbf{false} \textbf{explanation} of nature and the \textbf{conduct} of matter - but not yet \textbf{observed} \textbf{empirical}\underline{ly}.
However, the \textbf{Hi}\textbf{\underline{gg}}\underline{s} field is much more \textbf{stable} than the \textbf{electromagnetic} field; the \textbf{pathogen} must achieve very high energy levels, a bit like a \textbf{frozen} \textbf{pond}\underline{,} whose \textbf{surface} could only be \textbf{crack}\underline{ed} by a very large \textbf{rock}\underline{.}
Mr \textbf{Za}\underline{mb}\textbf{ito} had his hand in the 2000s \textbf{everywhere} by giving more than 8\textbf{8,000} \textbf{Canadian} \textbf{dollars} (\textbf{about} EUR 6\textbf{8,000}\underline{)} to \textbf{provincial} parties, especially to the \textbf{liberal}\underline{s} who were in power at the time.
From the \textbf{investigation} that is finally carried out, it \textbf{says} that it '\textbf{dra}\underline{w}s on a \textbf{thread} that makes it possible to understand the \textbf{functioning} of the system sub\textbf{vert}\underline{ed} by \textbf{ants} in order to stop the \textbf{evil} and \textbf{denounce} the \textbf{guilty}\underline{'}.
In order for farmers to free themselves from the ins\textbf{urg}\textbf{\underline{ency}} led by foreign groups, which they say they want, it would be necessary to continue with low, well-\textbf{controlled} and directly related \textbf{civilian} aid in their favour.
In the city you usually get by bus, but in \textbf{Jerusalem} there is also a \textbf{tram}\underline{way} and in \textbf{Hai}\underline{fa} the only \textbf{subway} line in the country with six \textbf{stations} that \textbf{connect} the lower city with the \textbf{upper} city.
\textbf{Nevertheless}\underline{,} many citizens of the Central \textbf{Asian} \textbf{republic}\underline{s} who want to make their money in Russia \textbf{admit} that not only do they not know the language of the \textbf{destination} country, but they are also \textbf{unable} to express themselves in writing in their own language.
In recent days there have been \textbf{massive} \textbf{protests} across the US against low \textbf{wages} at \textbf{Wal}\underline{mar}t \textbf{stores} and restaurants of popular fast-\textbf{food} \textbf{chain}\underline{s} such as \textbf{Mc} \textbf{Donald}\underline{'}s, \textbf{Burg}\underline{er} \textbf{King}\underline{,} Taco \textbf{Bell}\underline{,} Wendy's and Kent\textbf{uck}\underline{y} \textbf{Fried} \textbf{Chi}\underline{cken}.
Even under the previous rules, the persons under \textbf{examination} are \textbf{accountable} to the \textbf{carrier} (for example, in the case of an \textbf{operational} regional policy programme, to the \textbf{Regional} Council) in such a way that any failure to \textbf{comply} with the \textbf{procurement} law is \textbf{tan}\underline{ta}\textbf{mount} to a \textbf{violation} of budgetary \textbf{discipline}\underline{.}
\textbf{Another} stage of development should already be able to do real scientific work - the \textbf{RM}\underline{-}\textbf{34} \textbf{rocket} should reach an \textbf{altitude} of up to \textbf{14.}\underline{5} km and be used to \textbf{observe} high-al\textbf{titude} \textbf{wind}\underline{s}.
On a large \textbf{scale}\underline{,} this means for most companies to \textbf{relocate} their production \textbf{abroad} or buy it \textbf{cheap}\underline{ly}, or to \textbf{abandon} their business, \textbf{resulting} in high unemployment in countries with \textbf{comparable} labour costs.
The only solution is \textbf{targeted} political and social reforms that increase the state u2019s participation in the economy, increase citizens u2019 influence on the government, and \textbf{weaken} the \textbf{monopoly} of private capital in society for the benefit of the state.
What is less \textbf{apparent} is the question of whether it really was always these personalities who \textbf{determined} their actions \textbf{autonomous}\underline{ly}, or whether behind their \textbf{thro}\underline{ne} there was \textbf{someone} who \textbf{directed} their actions towards a prede\textbf{termin}\underline{ed} goal.
Israel is like a huge \textbf{laboratory}\underline{,} a source of conflict and \textbf{chaos}\underline{,} not only in the country itself, but also \textbf{internationally} (re\textbf{member} how \textbf{sharply} the people \textbf{divide} into \textbf{supporters} and \textbf{opponents} of Israel).
\textbf{Regulation}\underline{s} are easily subject to \textbf{criticism} in the Member States, but, in the opinion of some \textbf{experts}\underline{,} the EU's efforts to \textbf{regulate} and thus also to make the whole of the European Union more effective and developing \textbf{deserve} more \textbf{recognition}\underline{.}
After a six-\textbf{year} \textbf{struggle} with Germany and Austria, the Czech Republic was able to \textbf{defend} the name "Olomo\textbf{uck} xe9 \textbf{tv}\underline{ar}  u20\textbf{47} \textbf{ky}\underline{",} the national\textbf{rum} (T\textbf{uz}\underline{em}sk  u20\textbf{47}  \textbf{rum}\underline{),} whose \textbf{tradition} goes back to the 19th century, but our \textbf{manufacturers} had to re\textbf{name} it "T\textbf{uz}\underline{em} xe1k".
\textbf{Pen}\underline{a} \textbf{Nie}\underline{to} was also very interested in talking about the growth of the \textbf{Mexican} economy, which is one reason why \textbf{Mexican}\underline{s} are just as likely to stay in \textbf{Mexico} today rather than \textbf{emigr}\underline{ate} to the United States.
\textbf{Among} these projects, there are also five \textbf{Peru}\textbf{\underline{via}}\underline{n}s on the axes of his \textbf{territory} from the \textbf{coast} to \textbf{Brazil}\underline{,} two of which are intended to provide a better link with \textbf{Ecuador}\underline{,} although he did not give any further details.
As part of the summit, the \textbf{defence} \textbf{ministers} of the \textbf{bloc} on the \textbf{adoption} of the \textbf{2013} action plan also met in advance, in order to strengthen dialogue and \textbf{consensus} on the \textbf{defence} of the region.
The President of \textbf{Ecuador} also supported the re\textbf{organiz}\underline{ation} of the Organisation of American States (O\textbf{EA}\underline{),} with the aim of \textbf{reducing} the influence of An\textbf{glo}\underline{-}\textbf{Saxon} countries and taking into account those who have \textbf{signed} the San Jos xe9 Agreement on Human Rights.
However, there are still many people in the \textbf{clinic} who know nothing about their \textbf{disease}\underline{,} who have already \textbf{suffered} damage and have \textbf{exhaust}\underline{ed} their \textbf{immune} system and who are victims of \textbf{opportun}\textbf{\underline{istic}} \textbf{infection}\underline{s}.
After that, the \textbf{supervisory} \textbf{authority} \textbf{systematically} \textbf{refused} to inform the main administration of the Republic of a \textbf{transaction} carried out by the \textbf{entrepreneur} in order to de\textbf{duct} from Bank IXE u2019s trust account F\textbf{/5}\textbf{\underline{89}} to the name \textbf{Mexican}\underline{a} de A\textbf{via}\underline{ci} xf3n 198 million pesos.
With players such as "\textbf{Can}\textbf{\underline{ito}}\underline{"} \textbf{Nie}\textbf{\underline{ves}}\underline{,} \textbf{Pablo} \textbf{Ali}\textbf{\underline{cea}} and the young \textbf{Roland}\underline{o} \textbf{Hour}\underline{ru}\textbf{iti}\underline{ner} as a \textbf{replacement} for the \textbf{locked} players because of the events at the \textbf{Pan} American \textbf{Games} in Mar del \textbf{Pla}\underline{ta}, we won the \textbf{gold} \textbf{medal} against any \textbf{prediction}\underline{.}
\textbf{Instead}\underline{,} you can choose between different \textbf{dishes} with ha\textbf{mmel} and \textbf{beef}\underline{,} soups and desserts (\textbf{prepared} with coconut \textbf{milk}\underline{),} traditional \textbf{Jewish} \textbf{hum}\underline{us} paste, different \textbf{sauce}\underline{s}, \textbf{fried} \textbf{ball}\underline{s} made of \textbf{sausage}\underline{d} be\textbf{ans} and peas (\textbf{fal}\underline{con}) as well as \textbf{fruits} and \textbf{vegetables}\underline{.}
On that day, some \textbf{Wal}\underline{mar}t workers, of which there are \textbf{2.2} million worldwide, \textbf{stopped} their work and, together with trade \textbf{unions} and left-\textbf{wing} \textbf{activists}\underline{,} \textbf{went} to \textbf{chain} \textbf{stores} that target low- and \textbf{middle}\underline{-}\textbf{income} \textbf{individuals}\underline{.}
The selected list has already included high-\textbf{rank}\underline{ing} representatives of the \textbf{Petersburg} art \textbf{scene}\underline{,} whose \textbf{successes} \textbf{extend} beyond the borders of the city and are often \textbf{recognized} in Europe without being known in the rest of Russia.
It is this kind of joint control that could help us to stop \textbf{constantly} trying to improve the law and reduce and \textbf{offset} \textbf{threshold}\underline{s} if this does not \textbf{seem} to have a particularly positive effect.
The powers are also to some extent \textbf{comparable}\underline{,} but Germany is a \textbf{federal} state, i.e. that these \textbf{courts} of \textbf{auditor}\underline{s} also exist in the individual \textbf{federal} states - that is where the German system \textbf{differ}\underline{s} from ours.
With our \textbf{band} The \textbf{Tap} \textbf{Tap} we are rather \textbf{funny} about it and say that we are the only \textbf{band} in the world that can \textbf{collect} enough positive energy to stop or prevent the world's end.
Some come to us with \textbf{romantic} ideas, and when they then find that they have rehe\textbf{ars}\textbf{\underline{als}} \textbf{twice} a week, have to go through \textbf{preparato}\underline{ry} \textbf{phase}\underline{s} and spend a lot of time on \textbf{concert} \textbf{tours}\underline{,} the \textbf{enthusiasm} of many will soon \textbf{disappear}\underline{.}
In \textbf{1937}\underline{,} the design of a photo\textbf{electric} \textbf{hunting} \textbf{rocket}\underline{,} which was produced by Ing. \textbf{Roh}\underline{o}zi  u20\textbf{47} ski, \textbf{appeared} in the press, and in the following year the work "R\textbf{aki}\textbf{\underline{eta}} - tor\textbf{ped}\underline{a} powie\textbf{tr}\underline{z}na i \textbf{ra}\textbf{\underline{kie}}\underline{to}\textbf{bomb}\underline{a} lot\textbf{nic}\underline{za}" by the \textbf{author} Leliwa-Kr\textbf{zy}\textbf{\underline{wo}}\textbf{\underline{block}}\underline{y} \textbf{appeared}\underline{.}
\textbf{Already} in its beginnings in \textbf{1956} the \textbf{Polish} space company P\textbf{TA} \textbf{tried} to join the International \textbf{Federation} for \textbf{Space}\underline{,} \textbf{founded} in \textbf{1951}\underline{,} and in fact the P\textbf{TA} became a regular member as early as the \textbf{autumn} of \textbf{1956}\underline{.}
My \textbf{thoughts} are based in part on \textbf{accessible} historical \textbf{facts}\underline{;} others are \textbf{derived} from them and \textbf{arise} from my own understanding of who or which group of people have a significant influence on the events of modern history.
\textbf{Among} these astro\textbf{nom}\textbf{\underline{ically}} rich families, one is particularly \textbf{striking}\underline{,} which could be called the head of the \textbf{oc}\textbf{\underline{top}}\underline{us} (I do not know if there is \textbf{anyone} above them, but I do not rule this out) - the \textbf{Roth}\textbf{\underline{schild}}\underline{s}.
The way in which the group of the \textbf{richest} families works with the \textbf{Roth}\textbf{\underline{schild}}\underline{s} at the top is to \textbf{trigger} a crisis and then offer a solution (\textbf{order} from \textbf{cha}\underline{o} - order out of \textbf{chaos}\underline{).}
\textbf{Sub}\textbf{\underline{sid}}\underline{ies} for applications for funding were offered to the \textbf{municipalities} by the \textbf{Ministry} of \textbf{Regional} Development under the direction of Minister Pa\textbf{vel} N  u20\textbf{47} mec (US-DEU).
In the opinion of these \textbf{experts}\underline{,} a more serious problem is EU funding for projects which have absolutely nothing to do with \textbf{deepening} European integration, but which were \textbf{forced} on by individual Member States in the budget negotiations.
So, as soon as a US government official levels even the \textbf{slightest} \textbf{criticism} of \textbf{Mexico}\underline{,} \textbf{complaints} are heard - in the \textbf{Mexican} press and among the country's \textbf{elite}\underline{s} - about how \textbf{Americans} depress the \textbf{sovereignty} of their \textbf{neighbouring} country.
A number of \textbf{Australian} laws have ban\textbf{ished} \textbf{tobacco} companies from TV \textbf{advertising}\underline{,} \textbf{banned} them from \textbf{acting} as sports \textbf{sponsor}\underline{s} and \textbf{forced} most \textbf{traders} to stop \textbf{selling} \textbf{cigarette}\underline{s} in \textbf{shops}\underline{.}
After the police \textbf{officer} \textbf{Mari}\underline{hu}ana was found in the car, O\textbf{roz}\underline{co} was \textbf{charged} for \textbf{possession} of \textbf{drugs} and \textbf{drug} \textbf{uten}\underline{s}ils - ca\textbf{val}\underline{ier} \textbf{offences}\underline{,} each with a fine of \textbf{USD} 100 - and received a \textbf{court} \textbf{appointment}\underline{.}
In \textbf{Washington}\underline{,} it is \textbf{believed} that \textbf{Color}\underline{ado} is in any case \textbf{ahead} of most states in \textbf{regulating} \textbf{mar}\underline{i}juana, where the \textbf{drug} was legalised first for medical purposes and then for self-con\textbf{sumption}\underline{.}
"None\textbf{where} will it be \textbf{harder} to find a location for a \textbf{licensed} canna\textbf{bis} business than in \textbf{urban} areas, especially in the \textbf{Seattle} \textbf{metropolitan} area," \textbf{says} \textbf{Ben} \textbf{Living}\underline{s}ton, \textbf{spoke}\underline{s}\textbf{person} for the Center for \textbf{Legal} Canna\textbf{bis}\underline{,} a recently \textbf{formed} research group.
Although 5\textbf{5\%} of \textbf{voters} in \textbf{Color}\underline{ado} supported the measure, it was clear from the \textbf{outset} that it would not be easy to \textbf{reconcile} personal \textbf{consumption} of \textbf{mar}\underline{i}juana with the complexities of government and legal systems.
While \textbf{advocate}\underline{s} and state \textbf{officials} are \textbf{preparing} for an age of legal sales, they are also \textbf{nervous}\underline{ly} \textbf{awaiting} \textbf{instructions} from the \textbf{Federal} Government, which \textbf{wants} to continue to \textbf{treat} the \textbf{sale} and \textbf{cultivation} of \textbf{mar}\underline{i}juana at \textbf{federal} level as a criminal of\textbf{fence}\underline{.}
The 27-\textbf{year}\underline{-}\textbf{old} Anto has been risking his life at Kawah Ijen for three years, whose \textbf{sulphur} has already left his first \textbf{trace}\underline{s} in his \textbf{eyes}\underline{,} even though he \textbf{covers} his face with a \textbf{mask} and special \textbf{glass}\underline{es}.
Then the \textbf{Peru}\textbf{\underline{via}}\underline{n} Presidency sent an e-mail to the media with the 'con\textbf{cl}\underline{us}ive \textbf{declaration}\underline{'} of the summit, but this was the \textbf{Hum}\textbf{\underline{ala}} \textbf{declaration} and not the official document for \textbf{concluding} the summit.
"\textbf{Si}\textbf{\underline{nce}} he has been in our message, I have not \textbf{spoken} to him, but the \textbf{ambassador} has \textbf{informed} me that he has a \textbf{slight} problem with the lungs, but not a serious one," said \textbf{Ecuador}\underline{'}s \textbf{Head} of State.
"The solution to this problem is in the \textbf{hands} of the UK, \textbf{Sweden} and the European legal authorities because the \textbf{lawyer} of Ass\textbf{ange}\underline{,} \textbf{Bal}\underline{t}\textbf{azar} \textbf{Gar}\underline{z} xf3n, \textbf{leads} a number of \textbf{proceedings} at various European \textbf{bodies}\underline{,}" he \textbf{explained}\underline{.}
Cor\textbf{rea} took the opportunity to \textbf{confirm} \textbf{himself} as \textbf{defend}\underline{er} of freedom of the press and said that what he does not \textbf{tolerate} is 'the me\textbf{dio}\textbf{\underline{crit}}\underline{y}, the \textbf{evil} \textbf{intent} and the lies that de\textbf{tract} from freedom of \textbf{expression}\underline{'}.
In Ja\textbf{lis}\underline{co} alone, 255 people died in \textbf{2011}\underline{,} and by May this year there are already 187 \textbf{deaths}\underline{,} but it is \textbf{assured} that \textbf{universal} access to antiretro\textbf{vir}\underline{al} \textbf{medicines} has been available since \textbf{2005.}
As you know, we are talking about a huge sales and distribution centre in \textbf{Mexico}\underline{,} Central America and the \textbf{Caribbean} with products from the country beyond the \textbf{wall}\underline{,} \textbf{supplement}\underline{ed} by a living area for the employees of 150 companies.
The most e\textbf{motive} \textbf{memories} are those that remember his time at the \textbf{Va}\textbf{\underline{quer}}\underline{os} from the \textbf{mid}\textbf{\underline{-19}}\underline{50}s as a player until \textbf{1982}\underline{,} when he \textbf{celebrated} his 15th \textbf{anniversary} as a co-\textbf{chair} or \textbf{manager} of the \textbf{club}\underline{.}
However, my \textbf{favourite} is the \textbf{pan}\underline{-}\textbf{American} team in \textbf{Cuba} in \textbf{1991}\underline{,} where we won \textbf{gold} and offered the US team a fight, as they did when they won \textbf{bronze} against us at the World \textbf{Cup}\underline{.}
The \textbf{ad}\underline{age} "Who \textbf{shot} on J.R.?", which was \textbf{supposed} to create an \textbf{episode} full of \textbf{emotions} where \textbf{Hag}\underline{mann}'s \textbf{figure} was almost \textbf{killed}\underline{,} led to international \textbf{speculation}\underline{,} and \textbf{millions} of \textbf{dollars} were \textbf{bet}\underline{s} in be\textbf{tting} \textbf{houses}\underline{.}
A \textbf{manifest}\underline{o} has been in \textbf{circulation} since October, \textbf{signed} by \textbf{prominent} \textbf{figures} of \textbf{pal}\underline{li}ative care such as Dr \textbf{Bal}\textbf{\underline{four}} \textbf{Mount} and Dr \textbf{Bernard} La\textbf{point}\underline{e}, to \textbf{demonstrate} their \textbf{opposition} to such an initiative.
\textbf{Civil} \textbf{servant}\underline{s} of the \textbf{Road} \textbf{Building} Office, companies of the construction industry, money \textbf{creator}\underline{s} of political parties and \textbf{specialists} of the Italian \textbf{mafia} tell every day what they know about a great 'system' \textbf{involving} construction, civil \textbf{servant}\underline{s}, \textbf{politicians}\underline{,} trade \textbf{union}\underline{ists} and mafi\textbf{oso}\underline{.}
The Chinese have almost left Mes \textbf{Ay}\underline{n}ak u2019s \textbf{copper} \textbf{mine}\underline{s}, \textbf{leaving} the international \textbf{arch}\underline{a}e\textbf{ologist}\underline{s} (\textbf{finance}\underline{d} by the World Bank) to \textbf{excavat}\underline{e} the huge \textbf{Buddhist} site and remain the \textbf{province} u2019s most important \textbf{employers}\underline{.}
Most \textbf{lawyers} who have worked on this text are not \textbf{Ul}\underline{e}ma, but \textbf{academic}\underline{s} who have been \textbf{partially} \textbf{trained} in the French system," a\textbf{ppe}\textbf{\underline{ase}}\underline{s} \textbf{Alex}\underline{is} \textbf{Blo}\underline{ue}t, who \textbf{write}\underline{s} a \textbf{doctor}\underline{al} thesis on \textbf{Egypt}\underline{'}s \textbf{constitutional} \textbf{transition}\underline{.}
From January to October \textbf{2012}\underline{,} 1\textbf{18}\underline{.}8 \textbf{thousand} \textbf{Ukrainian} \textbf{tourists} \textbf{entered} the \textbf{promised} country, an increase of 5\textbf{1\%} \textbf{compared} with the same period in \textbf{2010,} before \textbf{visa} \textbf{waiver} on 9 February \textbf{2011}\underline{.}
"The police, of course, know all about it and therefore, if they cannot \textbf{comply} with the crime \textbf{detection} plan, carry out periodic \textbf{checks} on dealers who offer illegal \textbf{weapons}\underline{,}" \textbf{adds} the sales \textbf{advisor}\underline{.}
The \textbf{protests} \textbf{continued} this week in New York, where their goal was not \textbf{Wal}\underline{mar}t \textbf{stores} (\textbf{which} are not \textbf{desirable} in this \textbf{progressive} city and are therefore not there), but \textbf{McDonald}\underline{'}s and other low-\textbf{cost} restaurants.
Not only do we want to \textbf{collect} enough positive energy to prevent the end of the world, but we also want to think with the public about the state of our handing over this world to our children.
The global desire for power of the \textbf{Roth}\textbf{\underline{schild}}\underline{s} led in the years 18\textbf{59} - 18\textbf{71} to the \textbf{formulation} of a plan to \textbf{unleash} three world wars by \textbf{Albert} Pik, a freemason of the \textbf{33}\textbf{\underline{rd}} and thus the highest degree of knowledge.
At the end of the 19th century, the \textbf{Roth}\textbf{\underline{schild}}\underline{s} \textbf{initiated} the \textbf{founding} of the \textbf{Zion}\underline{ist} movement in which a \textbf{branch} \textbf{sought} to establish a \textbf{Jewish} state, \textbf{preferably} in the historical area of \textbf{Jud}\underline{e}a with \textbf{Jerusalem} as capital (re\textbf{turn} to \textbf{Zion}\underline{).}
Af\textbf{fleck} u2019s film thus \textbf{lose}\underline{s} a bit of tra\textbf{ction}\underline{,} it is a film that can be \textbf{watch}\underline{ed} with a certain interest and can gout the design and the \textbf{retro}\underline{-}\textbf{style} \textbf{reminiscent} of a \textbf{thrill}\underline{er} from the 70 u2019s.
The \textbf{organize}\underline{rs} of the \textbf{survey} were also \textbf{impressed} by the idea that certain countries should receive money for not having a sea, or by the idea of providing funding for applications for funding.
This \textbf{suggests} at least one new \textbf{article}\underline{:} in all \textbf{Sha}\textbf{\underline{ria}} \textbf{affairs}\underline{,} Al-As\textbf{har} University, the country u2019s most important \textbf{Islamic} \textbf{institution}\underline{,} must be \textbf{consulted} with great \textbf{vig}\textbf{\underline{our}} throughout \textbf{Sunni} \textbf{Islam}\underline{.}
Even on better days, this is an ever-c\textbf{hallen}\textbf{\underline{ged}} city, but on \textbf{Monday} a \textbf{steel} \textbf{ring} was built that \textbf{shut}\underline{s} down several important \textbf{routes} to the capital and \textbf{creates} \textbf{chaos} on the \textbf{streets}\underline{.}
Manning commented on \textbf{Thursday} on his \textbf{arrest} and transfer to \textbf{Kuwait}\underline{,} where he was held for about two months before being \textbf{transferred} to the \textbf{Qua}\underline{n}\textbf{tico} \textbf{naval} base in \textbf{Virgin}\underline{ia} in July \textbf{2010.}
Although several \textbf{Hamas} leaders have been \textbf{killed} and the 1.7 million \textbf{inhabitants} of \textbf{Gaza} are \textbf{pl}\textbf{\underline{uck}}\underline{ed} into one of the most desolate and densely \textbf{populated} \textbf{corner}\underline{s} of the \textbf{planet}\underline{,} Israel has so far \textbf{failed} to \textbf{destroy} \textbf{Hamas}\underline{.}
In particular, the rise of the \textbf{Muslim} \textbf{Brot}\underline{her}\textbf{hood} under President \textbf{Muhammad} \textbf{Mor}\underline{si} in \textbf{Egypt} - the most in\textbf{habit}\underline{ant} and important \textbf{Arab} country by far - on Israel's \textbf{southern} \textbf{flank} has changed the region's balance on a \textbf{lasting} basis.
\textbf{Cava}\textbf{\underline{lier}}\underline{e} di \textbf{Gran} \textbf{Cro}\underline{ce} (the highest \textbf{award} in Italy), \textbf{Cava}\textbf{\underline{lier}}\underline{e} del Lavoro, \textbf{Command}\textbf{\underline{eur}} de L'\textbf{Or}\textbf{\underline{dre}} des \textbf{Arts} et des Lettres, \textbf{awarded} with the \textbf{honour} of \textbf{honour}\underline{,} \textbf{cum}\textbf{\underline{ulate}}\underline{s} \textbf{Gar}\textbf{\underline{ava}}\underline{ni} as many \textbf{honour}\underline{s} as any of the \textbf{husband}\underline{s} of his clients.
Even if these new rules could \textbf{pave} the way for an increase in the national \textbf{birth} rate, \textbf{discussions} with the \textbf{Singapore}\textbf{\underline{ans}} working in the financial \textbf{district} show that they will not have much effect.
The \textbf{Sixth} \textbf{Summit} of Presidents of the Union of South American Nations (Una\textbf{sur}\underline{)} \textbf{ended} today in \textbf{Peru} without the \textbf{publication} of the \textbf{Lima} \textbf{Declaration}\underline{,} which was \textbf{announced} earlier and was \textbf{theoretical}\underline{ly} to be \textbf{signed} by the \textbf{seven} leaders present.
To put it simply, the above \textbf{statements} mean that who\textbf{ever} is \textbf{diagnose}\underline{d} with \textbf{HIV} positive at the age of 25 can "be \textbf{75} years old without any problems as long as he is under control," he \textbf{explained}\underline{.}
A team that was perhaps not the best in terms of personalities, but with which we won a \textbf{gold} \textbf{medal} and which \textbf{gave} us great \textbf{pleasure}\underline{,} was that of the pre-Olym\textbf{pic} \textbf{tournament} in Neu\textbf{qu} xe9n, \textbf{Argentina} in 1995.
\textbf{Hag}\underline{man}, who \textbf{returned} this year in a new season of "\textbf{Da}\textbf{\underline{lla}}\underline{s}", died on \textbf{Friday} \textbf{afternoon} due to \textbf{cancer} \textbf{complications} in a family press release to The \textbf{Associate}\underline{d} \textbf{Press} by \textbf{Warn}\underline{er} \textbf{Bro}\underline{s}., \textbf{producer} of "\textbf{Da}\textbf{\underline{lla}}\underline{s}".
\textbf{Hag}\underline{man} \textbf{interpreted} the role of E\textbf{wing} as a \textbf{corrupt}\underline{,} ins\textbf{ati}\underline{able} man with a \textbf{charisma}\underline{tic} \textbf{smile}\underline{:} a deceitful businessman and un\textbf{trust}\underline{ed} \textbf{husband} who \textbf{sought} to in\textbf{struct} his \textbf{alcohol}\underline{-}ind\textbf{uc}\underline{ed} \textbf{wife} Sue E\textbf{llen} (\textbf{Li}\underline{n}da \textbf{Gra}\underline{y}).
In addition, this \textbf{appears} to be \textbf{confirmed} by new data presented this week at a major \textbf{physics} \textbf{congress} in \textbf{Kyoto}\underline{,} but there is still a lack of data to be absolutely certain about this.
After all, if a p\textbf{article} with an \textbf{electric} charge \textbf{accelerate}\underline{s} or changes direction, the \textbf{electromagnetic} field is "\textbf{dis}\textbf{\underline{tur}}\textbf{\underline{bed}}\underline{"} in this very place, almost like a pe\textbf{bble} \textbf{thrown} into a \textbf{pond}\underline{.}
"They \textbf{gave} me five years to live, I have managed \textbf{seven} years," he half-heartedly said, \textbf{lying} in his bed in the home for \textbf{pal}\underline{li}ative care \textbf{Victor}\underline{-}\textbf{Ga}\textbf{\underline{db}}\textbf{\underline{ois}} in Beloeil, where he had \textbf{arrived} the previous day.
Dr. Martel \textbf{believes} that \textbf{90\%} of \textbf{patients} who have asked to die thank the nursing staff for not \textbf{allowing} this desire after their \textbf{pain} has been \textbf{alleviate}\underline{d} by a team of \textbf{pal}\underline{li}ative care.
All the \textbf{examination} \textbf{bodies} will be under the a\textbf{eg}\underline{is} of the P\textbf{ush}\textbf{\underline{kin}} \textbf{Institute} for the Russian \textbf{Language}\underline{,} the Russian University of \textbf{Friend}\underline{ship} of Nations, the \textbf{Moscow} State University, the St. \textbf{Petersburg} State University and other Russian \textbf{universities}\underline{.}
"The problem is that the \textbf{chic}\underline{k} has to stop; it has to be able to stand on its \textbf{feet} and begin to move," \textbf{explains} \textbf{Vladimir} \textbf{Sy}\underline{che}v, head of the \textbf{Institute} for \textbf{Medical} and Bi\textbf{ological} \textbf{Problems}\underline{.}
"Twice we let \textbf{chic}\textbf{\underline{ks}} \textbf{slip} and then put it in, because it is simply \textbf{impossible} to work with them there," \textbf{says} \textbf{Vladimir} \textbf{Sy}\underline{che}v for a \textbf{failed} \textbf{experiment} with \textbf{chic}\textbf{\underline{ks}} in space.
Generally \textbf{speaking}\underline{,} I would not like to \textbf{compare} this without specific information, but Germany is, in a certain sense, often called a model, but it is certainly not possible to say that Germany is better on the whole.
On some \textbf{roads} in East \textbf{Bohemia} there is a risk of \textbf{ice}\underline{-}smoothing, in higher \textbf{locations} and in the \textbf{mountains} there is sometimes still an \textbf{extended} \textbf{snow} \textbf{layer} on the \textbf{roads}\underline{,} informs the road and \textbf{motorway} \textbf{director}\underline{ate} on their website.
However, it is not exactly \textbf{custom}\underline{ary} for a larger group of \textbf{disabled} people to take an active part in social events there, in which we are a little \textbf{ahead} of the West with The \textbf{Tap} \textbf{Tap}\underline{!}
The First World War \textbf{ended} with the \textbf{sudden}\underline{,} military and economic un\textbf{founded} \textbf{surrender} of Germany (\textbf{war} was no longer necessary for the \textbf{destruction} of the Russian T\textbf{sar} \textbf{Empire}\underline{),} followed by the dis\textbf{solut}\underline{ion} of the Central European great power of Austria-Hungary.
E\textbf{motion}\underline{s} in this country also give rise to the fact that the Czech Republic, like other Member States in \textbf{Brussels}\underline{,} has to fight for the right to use specific designations of traditional products and does not always \textbf{win} this \textbf{battle}\underline{.}
Some of them have received up to 14 \textbf{orphan}\underline{s}, give them a \textbf{roof} over their \textbf{heads} and make sure that the children appear in their \textbf{uniform}\underline{s} on time for school \textbf{lessons} every day.
The hotel in which I stay is one of several \textbf{venue}\underline{s} that \textbf{organize} a Rakfisk \textbf{dinner} where guests can vote for the best - or perhaps the most \textbf{challenging} - fish.
To reach the city you can go on one of the \textbf{motorway}\underline{s} that built \textbf{Pen}\underline{a} \textbf{Nie}\underline{to}, which is a great \textbf{improvement} over the \textbf{broken}\underline{,} p\textbf{uff}\underline{y} \textbf{roads} that once \textbf{existed} here.
When \textbf{Fein} asked him about the forms on \textbf{Friday}\underline{,} Manning \textbf{admitted} that he had \textbf{judged} the treatment by his \textbf{guard}\underline{s} "ex\textbf{cell}\underline{ent}" and the treatment by the \textbf{institution} as a whole "\textbf{very} professional".
On \textbf{Thursday}\underline{,} Manning had said that he was \textbf{forced} to \textbf{sleep} \textbf{naked} on the previous night and had \textbf{tried} to show an official that he was not a \textbf{danger} to \textbf{himself}\underline{.}
His \textbf{lawyers} hope that the \textbf{judge} will at least take his experience of \textbf{detention} into account and \textbf{drastically} reduce his \textbf{detention} if he is \textbf{tried} before the military \textbf{court}\underline{,} which is \textbf{scheduled} for early next year.
The question must be asked: is this just a private person who likes Mar\textbf{lb}\textbf{\underline{oro}} \textbf{cigarette}\underline{s} so much that it even takes a video for it - or does a marketing \textbf{agency} have to do with it?
They are \textbf{waiting} for \textbf{guidance} on the establishment of a \textbf{licensing} system for the production, production, distribution and \textbf{sale} of \textbf{drugs} - with a \textbf{deadline} of 1 December \textbf{2013} in mind.
The \textbf{Washington} \textbf{Law}\underline{,} called I\textbf{-5}\underline{02}, enters into force on 6 December, and thus also forms the end point of a \textbf{grey} area where the state \textbf{licensing} system does not yet exist but property is legalised.
\textbf{Organis}\underline{ed} and \textbf{rising} hatred for Tory students in \textbf{Oxford} has now developed to such an extent that a group of them last week called for equal rights protection for \textbf{gay}\underline{s}, \textbf{disabled} people and \textbf{ethnic} \textbf{minorities}\underline{.}
It \textbf{divide}\underline{s} up a \textbf{dirty} \textbf{wooden} \textbf{hut} with other \textbf{carriers} and \textbf{stands} up every morning at two o'\textbf{clock} because the \textbf{sulphur} also \textbf{flows} out at night, where its \textbf{characteristic} \textbf{yellow} \textbf{colour} \textbf{shine}\underline{s} \textbf{blu}\underline{ish} in the \textbf{dark}\underline{.}
\textbf{Every} day he and his \textbf{companion}\underline{s} break 15 tons of \textbf{sulphur} from the \textbf{volcano}\underline{,} which are \textbf{transported} by three \textbf{truck}\underline{s} through a goat path between the bush and the \textbf{camp} in \textbf{Tam}\textbf{\underline{ans}}\underline{ari} 18 \textbf{kilometres} away.
In \textbf{Singapore}\underline{,} there are Web sites where the \textbf{bare}\underline{ly} \textbf{ve}\underline{il}ed \textbf{xenophobia} is \textbf{flourish}\underline{ing} against many new \textbf{immigrants}\underline{,} especially the Chinese, who are \textbf{criticised} for \textbf{keeping} \textbf{wages} low and not \textbf{integrating}\underline{.}
He proposed re\textbf{orient}\underline{ing} this in\textbf{efficient} distribution; the con\textbf{dom}\underline{s} should not be just behind the \textbf{shop} table, but in public \textbf{toilet}\underline{s} in institutions often \textbf{visited} by young people.
"\textbf{Our} first project \textbf{dealt} with the \textbf{prop}\underline{he}cy of the \textbf{Maya}\underline{s}, and in a certain way we \textbf{discredit} them," said Julie \textbf{Ze}\textbf{\underline{gl}}\underline{en}, \textbf{student} last year in \textbf{Temple}\underline{,} 21 years old and from West \textbf{Che}\underline{ster}.
However, he \textbf{notes} that there is an apocaly\textbf{ptic} \textbf{fear} in Western society that goes back several \textbf{centuries} when people \textbf{react}\underline{ed} to changes in their \textbf{surroundings} by \textbf{predict}\underline{ing} the end of the world.
\textbf{Nevertheless}\underline{,} let us \textbf{assume} that it is actually \textbf{Hi}\textbf{\underline{gg}}\underline{s}, because there seems to be only a small risk of being deceived, and let us look at what is at \textbf{stake}\underline{.}
It has to be said that the \textbf{latter} still has great \textbf{shortcomings}\underline{,} as it does not provide an \textbf{explanation} of \textbf{gravity} (ups!) and \textbf{dark} matter, which is about \textbf{80\%} of the matter of the \textbf{universe} (re\textbf{new}\underline{ed} ups!).
"\textbf{Si}\textbf{\underline{nce}} the study began in \textbf{2010,}\underline{"} he \textbf{emphasize}\underline{s}, "the \textbf{Ministry} of Transport alone \textbf{saved} a billion \textbf{dollars} in \textbf{contracts}\underline{,}" because some of them \textbf{narrow}\underline{ed} their in\textbf{stinct}\underline{s} to maintain their share!
The new cooperation agreement provides for the \textbf{continuation} of traditional aid: \textbf{girls}\underline{'} and \textbf{boys}\underline{'} \textbf{Gy}\underline{m}n\textbf{asia}\underline{,} \textbf{institute} of French \textbf{universities}\underline{,} French \textbf{institute}\underline{,} cooperation in the military, legal, medical and agricultural sectors, support for the \textbf{archaeological} \textbf{delegation}\underline{.}
\textbf{Stephen} \textbf{Bet}\underline{ish}es developed in our \textbf{laboratory} in Red\textbf{mond} a contact \textbf{sensor} with a \textbf{variable} processing \textbf{delay} between 1 and 100 \textbf{mill}\underline{i}\textbf{second}\underline{s}, with today's commercial \textbf{sensors} being \textbf{closer} to the second (60 to 100).
\textbf{Recently} he \textbf{grab}\textbf{\underline{bed}} an \textbf{organ} and became a St. \textbf{Petersburg} \textbf{organ} player, because he \textbf{felt} ready for this difficult role in terms of his \textbf{artistic} \textbf{existence}\underline{,} \textbf{philosophy} and image.
There is a link between the fact that a child is in the ab\textbf{dom}\underline{en} of the \textbf{mother} in \textbf{fruit} water for about 9 months and that it is \textbf{easier} to get used to water.
At the end of the \textbf{Maya}\underline{n} \textbf{Cal}\underline{en}\textbf{dar} we have also developed a unique collection of \textbf{shoes}\underline{,} t-\textbf{shirt}\underline{s}, \textbf{bags} and key \textbf{ring}\underline{s} against the end of the world with which people can also support us by \textbf{purchasing} them through www.e-tap.\textbf{cz} .
As the German economy improves its \textbf{competitiveness}\underline{,} there are regular cases where workers receive such low \textbf{wages} that the state has to increase their incomes to the minimum level of subsistence.
\textbf{Abraham} \textbf{Lincoln} \textbf{refused} to \textbf{renew} \textbf{Roth}\textbf{\underline{schild}} u2019s Bank of America u2019s central bank status, began \textbf{issuing} his own bank\textbf{note}\underline{s} during the \textbf{Civil} War, and was \textbf{murdered} in a \textbf{theater} in 18\textbf{65}\underline{.}
For their release, they called for the \textbf{extradition} of the \textbf{overthrow}\underline{n} \textbf{Sha}\underline{h} Mo\textbf{ham}\textbf{\underline{mad}} Reza P\textbf{ahl}\textbf{\underline{avi}}\underline{,} who had \textbf{fled} to the US after the \textbf{revolution}\underline{,} who had \textbf{maintained} \textbf{patron}\underline{age} of his regime for \textbf{decades}\underline{.}
\textbf{Alan} Ar\textbf{kin} and John \textbf{Good}\underline{man} are very \textbf{charming} in their roles as \textbf{Hollywood} staff, but their \textbf{characters} \textbf{deserve} more room, and they are not alone in the film.
However, it is \textbf{sufficient} to remember a \textbf{piece} of history that is still \textbf{alive} in some way to this day and to \textbf{prove} how over-ex\textbf{pen}\underline{s}ive the \textbf{notion}\underline{s} of the \textbf{om}\underline{ni}\textbf{pot}\underline{ent} and \textbf{om}\textbf{\underline{nis}}\underline{ci}ent \textbf{secret} services are.
And as I am already over 40, independent and part\textbf{isa}\underline{n}, I have no other way of in\textbf{flu}\underline{en}cing things than to stand as a senator or \textbf{president}\underline{.}
But \textbf{Pat}\underline{t}\textbf{loch} u2019s cases are different: on behalf of his clients, he \textbf{oppose}\underline{s} the official right of Chinese companies to use a designation that is already protected \textbf{elsewhere}\underline{.}
\textbf{Who}\textbf{\underline{ever}} no longer has one comes to the \textbf{shelter} of \textbf{Khan}\underline{y}isile, a single \textbf{woman} who is paid just as much by the \textbf{club} as the two \textbf{chef}\underline{s} who \textbf{cook} every day for more than 200 \textbf{hungry} children.
A bus full of whites \textbf{singing} \textbf{songs} in a black language - not only does it bring \textbf{mood} and \textbf{joy}\underline{,} but it has also \textbf{sm}\textbf{\underline{ash}}\underline{ed} a few \textbf{tear}\underline{s} on some \textbf{fierce} border \textbf{soldiers}\underline{.}
\textbf{Under} the outgoing \textbf{Felipe} \textbf{Cal}\underline{der}on government, \textbf{Mexico} has been able to \textbf{prove} its \textbf{worth} \textbf{economically}\underline{,} but it is under control of a \textbf{drug} war that has already cost 60 000 lives in the last six years.
Even if the \textbf{Islamist}\underline{s} now in power in \textbf{Egypt} and other countries have little left for Israel, they will focus first on \textbf{domestic} \textbf{difficulties}\underline{.}
The right answer is that \textbf{represented} by the more \textbf{sensible} representatives of both \textbf{sides}\underline{,} by most of the rest of the world and by this \textbf{newspaper}\underline{:} two states where Israel is \textbf{leaving} for security purposes.
But \textbf{Professor} East\textbf{wood} \textbf{believes} that, although these two conditions may be related, \textbf{bo}\underline{red} people see the problem in their \textbf{surroundings} or in the world, while depressed people see the problem in themselves.
On the \textbf{scale} are \textbf{statements} like "\textbf{Man}\underline{y} things I have to do \textbf{repeat} themselves and are \textbf{mono}\underline{ton}ous" and "I have so many interests that I do not have enough time for everything".
If an iPad is enough for his \textbf{bo}\underline{red} child, it can be used to stop the \textbf{bo}\underline{re}\textbf{dom}\underline{,} but it has not \textbf{learnt} to talk or control itself, \textbf{says} \textbf{Professor} Fenske.
"\textbf{We} were all pleased when we were \textbf{invited} to his house in Gstaad," \textbf{explains} the ex-\textbf{wi}\underline{fe} of "\textbf{He}\underline{ini}" \textbf{Thyssen}\underline{,} close friends with \textbf{forgotten} \textbf{beauties} such as Mar\textbf{ella} \textbf{Ag}\underline{n}\textbf{elli} or \textbf{Eugen}\underline{ie} \textbf{Ni}\textbf{\underline{arch}}\underline{os}.
The company is PT Candi N\textbf{gri}\underline{m}bi, which since \textbf{1960} has been \textbf{exploit}\underline{ing} the \textbf{deposit}\underline{s} in the \textbf{volcano} and (n\textbf{ear}\underline{ly}) its workers, to which it \textbf{pays} 6\textbf{62} \textbf{Indonesia}\underline{n} rupees \textbf{(5} euro \textbf{cent}\underline{s}) for each \textbf{kilo} of \textbf{sulphur}\underline{.}
It seems \textbf{incredible} that the \textbf{vers}\underline{es} are part of an \textbf{ad}\textbf{\underline{vert}} for \textbf{min}\underline{z}\textbf{bon}\underline{s}, but \textbf{nevertheless} - or precisely because of this - at the beginning of this year in \textbf{Singapore} they became a vi\textbf{ral} video on \textbf{YouTube}\underline{.}
However, he \textbf{admit}\underline{s} that the new standards give \textbf{developers} \textbf{clearer} \textbf{orientation}\underline{s}, which were \textbf{previously} \textbf{obstruct}\underline{ed} if they wanted to build too many small \textbf{housing} \textbf{units} within a project.
\textbf{Marie}\underline{los} \textbf{Por}\textbf{\underline{ras}}\underline{,} a \textbf{teacher} of English with a degree in education and \textbf{learning}\underline{,} \textbf{believes} that to \textbf{orient}\underline{ate} children and a\textbf{dol}\underline{es}\textbf{cent}\underline{s}, it must be \textbf{understood} that it is the purpose of social networks to inform.
The head of state read the final document, in which it stated that 16 decisions were taken and that the lines of action for 31 projects between the South American countries were set at an investment total of \$\textbf{17} billion.
With the crisis in Europe, "\textbf{economic} \textbf{consolidation} (in \textbf{Latin} America) must not take on \textbf{triumph}\underline{ant} tra\textbf{its}\underline{,} but should serve to \textbf{expand} our \textbf{output} and show our \textbf{peoples} a better future," \textbf{Hum}\textbf{\underline{ala}} added.
I still know that \textbf{Gene} Bartow, who worked here as a trainer and \textbf{employed} at the University of Alab\textbf{ama} (\textbf{Bi}\textbf{\underline{rm}}\underline{ing}\textbf{ham}\underline{),} said to me: "I have a very strong and 2 m big player.
In \textbf{Pen}\underline{n} State, the final \textbf{exam} is carried out on the eve of the apocal\textbf{yp}\underline{se}, so students have no other chance than "to continue working until night where the world is \textbf{supposed} to end," said Re\textbf{stall}\underline{.}
\textbf{Joseph} D\textbf{ough}\underline{er}ty, a \textbf{religious} \textbf{professor} at the University of La S\textbf{alle}\underline{,} who is \textbf{teaching} in the \textbf{Philippines} this year, quickly \textbf{answers} the question whether he would know a course about the "end of the world" there.
A report by the \textbf{Brenn}\underline{an} Center in \textbf{2011} shows that those states that \textbf{passed} these laws make up 171 of the 270 \textbf{votes} that are required in the Ele\textbf{ctor}\underline{al} Committee to \textbf{win} the \textbf{presidency}\underline{.}
There are, by the way, many \textbf{phy}\underline{s}icists who \textbf{fer}\textbf{\underline{vent}}\underline{ly} hope that such \textbf{deviation}\underline{s} will be found, as the \textbf{slightest} \textbf{difference} could open a \textbf{door} to a "\textbf{new} \textbf{physics}\underline{"} and \textbf{plug} some \textbf{holes} in the model.
It is precisely this great in\textbf{adequacy} in \textbf{Quebec}\underline{'}s health care system that is \textbf{causing} concern among a number of \textbf{doctors} specialising in \textbf{pal}\underline{li}ative care to see the \textbf{adoption} of a law \textbf{regulating} \textbf{eu}\textbf{\underline{than}}\textbf{\underline{asia}} and \textbf{assisted} \textbf{suicide}\underline{.}
\textbf{Bit}\underline{co}in \textbf{differ}\underline{s} from other types of \textbf{virtual} \textbf{currencies} such as "\textbf{credit}\underline{s}" that are used to make progress in a video game that can be won or \textbf{bought} (and sometimes exchanged) by \textbf{playing}\underline{.}
"The \textbf{vulnerability} that has been used does not \textbf{affect} the actual \textbf{protocol}\underline{,}" \textbf{says} \textbf{Pierre} No\textbf{iza}\underline{t}, who has just introduced \textbf{Pay}\underline{m}ium, which is a company for real money payment and \textbf{uses} \textbf{Bit}\underline{co}in network.
The \textbf{Sala}\underline{f}ist parties, for which the establishment of \textbf{Islamic} law is an important \textbf{requirement}\underline{,} had \textbf{hoped} to \textbf{replace} '\textbf{pri}\underline{n}\textbf{cip}\underline{les}' with 'rules', which would have made it possible to apply them more \textbf{rigorous}\underline{ly}.
\textbf{Gali}\textbf{\underline{lee}} is the place where \textbf{Jesus} did his \textbf{miracle}\underline{s}: the \textbf{transformation} of water into wine at a \textbf{wedding}\underline{,} walking on the water, the \textbf{silence} of the seastorm and fishing.
\textbf{According} to the \textbf{Ministry} of the \textbf{Interior}\underline{'}s \textbf{statistics}\underline{,} 142 \textbf{crimes} were committed with the use of \textbf{registered} \textbf{weapons} over six months in \textbf{2012}\underline{,} while for the same period a total of \textbf{1.1}\textbf{\underline{68}} \textbf{thousand} \textbf{offences} were \textbf{recorded}\underline{.}
There are \textbf{traders} in the markets, but there you have to go and \textbf{arrange} with a code like "by \textbf{Ivan} \textbf{Ivan}\textbf{\underline{ovi}}\underline{ch}, who can tell that the \textbf{daughter} has lost a tooth".
In \textbf{conversation} with the head of the \textbf{interactive} 3D technologies group at the Microsoft \textbf{Lab} in \textbf{Cambridge} \textbf{Sha}\underline{h}\textbf{ram} Izadi, it is clear, however, that the \textbf{glass}\underline{es} were only a \textbf{transit} station for the company u2019s \textbf{scientists}\underline{.}
\textbf{Simpl}\underline{y} put, it is a question of European legislation \textbf{defining} how public \textbf{procurement} is to be \textbf{handled}\underline{,} on which national legislation is based, and, finally, on the actual practical application.
After \textbf{Madrid}\underline{,} \textbf{Luxembourg}\underline{,} London and other cities where everything works better than ours, we have just seen in Russia that everything is still in its beginnings in the East.
Re\textbf{spect} for the public and \textbf{accessibility} is one thing, but only when important sportsmen, \textbf{artists}\underline{,} \textbf{actors}\underline{,} \textbf{politicians} or \textbf{lawyers} come from our \textbf{rank}\underline{s} will things really start to change.
\textbf{Poland} also \textbf{participated} in space research with \textbf{Soviet} \textbf{satellite}\underline{s} under the Inter\textbf{cos}\textbf{\underline{mos}} programme and in \textbf{1978} \textbf{Polish} \textbf{pilot} \textbf{Mir}\underline{os}\textbf{law} Her\textbf{mas}\underline{ze}wski became second inter\textbf{kos}\underline{mon}\textbf{aut} after Czech V\textbf{lad}\underline{im} xedr Remek.
In what light do \textbf{David} \textbf{Rock}\textbf{\underline{ef}}\textbf{\underline{eller}}\underline{'}s words from \textbf{1994} appear: 'The only thing we need is an all-encompassing crisis and people will welcome the new world order'.
The standards on \textbf{fruit} and \textbf{vegetables} have already been \textbf{soft}\underline{en}ed by the EU against \textbf{opposition} from some countries, with the \textbf{indication} that the previous \textbf{directives} would lead to a waste of food.
As President, it would not be a problem for me to call on the \textbf{chair}\underline{men} of Parliament's political parties, live on \textbf{television}\underline{,} to make the \textbf{substantive} and criminal \textbf{liability} of \textbf{politicians}\underline{,} \textbf{officials}\underline{,} \textbf{judges} and public \textbf{prosecutor}\underline{s} \textbf{legally} \textbf{binding}\underline{.}
For almost ten years, the \textbf{chor}\underline{us} has been \textbf{performing} \textbf{songs} in this foreign \textbf{soft} language and \textbf{brings} them back from time to time where they \textbf{originally} came from: to \textbf{southern} Africa.
In the con\textbf{stell}\underline{ation} of \textbf{ser}\textbf{\underline{pen}}\underline{t} \textbf{carriers}\underline{,} \textbf{astronomer}\underline{s} have \textbf{photograph}\underline{ed} the fore\textbf{runner}\underline{s} of a cos\textbf{mic} cara\textbf{mbo}\underline{lage}: \textbf{400} million light years away from \textbf{Earth}\underline{,} the \textbf{nu}\textbf{\underline{cle}}\underline{us} of two \textbf{merge}\underline{d} \textbf{galaxies} \textbf{ra}\underline{ge} at each other and will \textbf{inevitably} co\textbf{lli}\underline{de} with each other.
When the \textbf{dark}\underline{ness} comes over the country in \textbf{Norway} and the \textbf{weather} \textbf{gets} \textbf{cold}\underline{er}, \textbf{Norwegian}\underline{s} \textbf{pour} into a \textbf{festival} here in Fagernes, which is \textbf{dedicated} to this speciality, which is now really very \textbf{impressive}\underline{.}
"\textbf{You} \textbf{eat} it \textbf{raw} and then wash it down with a \textbf{glass} of \textbf{Aqua}\textbf{\underline{vit}}\underline{",} \textbf{says} Ha\textbf{var}\underline{d} \textbf{Hal}\textbf{\underline{var}}\underline{s}en, who actually works in the local \textbf{fire} \textbf{guard}\underline{,} but as a so-called "Rakfisk general" also \textbf{organize}\underline{s} the \textbf{festival}\underline{.}
Manning \textbf{replied} that he had expressed his concerns orally and that the \textbf{officials} had \textbf{discussed} them with him and \textbf{indicated} that they were dealing with them, but they had not been \textbf{recorded}\underline{.}
"I wanted to \textbf{convince} employees that I was doing well and get \textbf{rid} of the \textbf{observation} status to prevent \textbf{injuries} (\textbf{...)} in order to achieve what I see as a higher quality of life," said Manning.
When he was \textbf{moved} to \textbf{Qua}\underline{n}\textbf{tico}\underline{,} Manning \textbf{spent} most of his days in a small \textbf{cell} - at least 21 hours and often more than 23 hours - and without society.
"\textbf{If} you market \textbf{tobacco} and only have a small area left to \textbf{advertise} your products, you will not get around the Internet," \textbf{says} \textbf{Beck}\underline{y} Freeman, health researcher at the University of \textbf{Sydney}\underline{.}
But \textbf{Peter} Toohey, \textbf{professor} of \textbf{Greek} and Roman history at the University of \textbf{Cal}\underline{g}ary in \textbf{Canada} and \textbf{author} of "B\textbf{ore}\textbf{\underline{dom}}\underline{:} A \textbf{Live}\underline{ly} \textbf{History}\underline{"} (Yale University \textbf{Press}\underline{,} \textbf{2011}\underline{)} does not see this.
\textbf{Sometimes} not, because in \textbf{extreme} cases it \textbf{causes} people to take \textbf{extreme} \textbf{physical} \textbf{risks} and to resort to \textbf{gambling} or \textbf{drugs} in order to \textbf{relieve} them - \textbf{studies} have shown this.
\textbf{According} to the \textbf{journalist} Su\textbf{zy} \textbf{Men}\textbf{\underline{kes}}\underline{,} the \textbf{supreme} \textbf{authority} of the trade press, this \textbf{dress} was a \textbf{milestone} in the \textbf{Haut}\underline{e} \textbf{Cou}\underline{ture} at the end of the 20th century, "the return to the customers of the highest society".
This is the case with Anto Wijaya, one of the \textbf{400} \textbf{mine} workers who \textbf{earn} their lives by \textbf{extract}\underline{ing} \textbf{sulphur} from the Kawah Ijen \textbf{Vol}\underline{ca}no in the \textbf{east} of the \textbf{Indonesia}\underline{n} island of \textbf{Java}\underline{.}
D\textbf{espite} its great \textbf{profits}\underline{,} the \textbf{mining} company has not me\textbf{chan}\underline{ised} \textbf{sulphur} de\textbf{ple}\underline{tion} in order to save costs and does not supply any equipment to those \textbf{carriers} who work on their own account and are paid for by \textbf{weight}\underline{.}
The \textbf{sentence}\underline{s} are part of a \textbf{ra}\textbf{\underline{pper}} \textbf{song}\underline{,} the local sayings such as "\textbf{bla}\underline{de} will be a "bao" (\textbf{lay}\underline{er}) in the \textbf{oven} to make fun of the low \textbf{birth} rate in \textbf{Singapore}\underline{.}
\textbf{Por}\textbf{\underline{ras}} \textbf{explains} that the \textbf{academic} \textbf{Marc} Pren\textbf{sky}\underline{,} \textbf{owner} of a \textbf{master} u2019s title in \textbf{ped}\textbf{\underline{ago}}\textbf{\underline{gy}} at \textbf{Ya}\underline{le} University and \textbf{author} of the work \textbf{Digital} Natives and \textbf{Immigrant}\underline{s}, \textbf{formed} these terms to \textbf{explain} the \textbf{phenomenon}\underline{.}
The only document \textbf{distributed} during the day was the list of \textbf{participating} \textbf{president}\underline{s}, which caused discom\textbf{fort} among the \textbf{hundreds} of \textbf{journalists} from different national and international media who were \textbf{calling} for more information.
And when \textbf{Sweden} inter\textbf{rog}\underline{ated} Mr Ass\textbf{ange} at the \textbf{Ecuador}\underline{ian} \textbf{embassy} in London or via \textbf{Skype}\underline{,} as \textbf{Swedish} case law allows and has been done in other cases, the problem is \textbf{solved}\underline{.}
Con\textbf{struct}\underline{ed} from \textbf{NY}\textbf{\underline{CE}}\underline{,} e-\textbf{Qu} xe1lity and Kernet, leading information technology companies, a group of companies has been established under the name \textbf{Comp}\underline{et}\textbf{ival}\underline{,} the aim of which is the service market of software \textbf{cluster}\underline{s} in Central and South America.
There he played the as\textbf{tron}\textbf{\underline{aut}} \textbf{Tony} \textbf{Nelson}\underline{,} whose life is \textbf{turned} upside down when he \textbf{encounter}\underline{s} an \textbf{attractive} "\textbf{ji}\underline{n}n" (\textbf{play}\underline{ed} by \textbf{Barbara} \textbf{Eden}\underline{)} who will live with him at home.
\textbf{Student}\underline{s} who are \textbf{regarded} as \textbf{voters} who are increasingly \textbf{casting} their \textbf{votes} for democratic \textbf{candidates} are not allowed in several states to use their photo \textbf{ID} \textbf{issued} by their \textbf{institution}\underline{.}
If you are able to read this \textbf{chronic}\underline{le}, it is only thanks to a \textbf{boss} of \textbf{extraordinary} ban\textbf{ality}\underline{:} the photon or the "light p\textbf{article}\underline{"} that is the "\textbf{bot}\underline{"} of \textbf{electromagnetic} force.
At the very end of their lives, \textbf{doctors} often resort to \textbf{terminal} sedation, which \textbf{amounts} to \textbf{dorm}\underline{ating} the \textbf{patient} either \textbf{sp}\textbf{\underline{ora}}\textbf{\underline{dic}}\underline{ly} or \textbf{permanently} until the time of his death.
In recent weeks, it has carried out a number of house \textbf{survey}\underline{s} and has made \textbf{allegations} of \textbf{fraud} and \textbf{corruption} against local \textbf{officials} such as \textbf{Frank} Tampino and \textbf{Richard} \textbf{Marco}\textbf{\underline{tte}}\underline{,} who are \textbf{mayor}\underline{s} of a \textbf{suburb}\underline{an} town.
The \textbf{monastery} of the \textbf{Holy} \textbf{Cross} in \textbf{Jerusalem} \textbf{stands} in the place where, according to a \textbf{Christian} \textbf{legend}\underline{,} the \textbf{tree} from which the cross was made for the \textbf{cru}\underline{ci}\textbf{fix}\underline{ion} of \textbf{Jesus} \textbf{grew}\underline{.}
The fact that the most important \textbf{immediate} task is to protect the system against \textbf{corruption} so that \textbf{certificates} cannot be \textbf{bought} is agreed by both \textbf{officials} and civil rights \textbf{activists}\underline{.}
\textbf{Parti}\textbf{\underline{cip}}\textbf{\underline{ants}} in the "B\textbf{lack} \textbf{Friday}\underline{"} \textbf{protests} called for \textbf{wage} \textbf{increases} and expressed their anger that the contribution to company health \textbf{insurance} had risen from \$30 to \$\textbf{100} a month.
There was a time when \textbf{nearly} a \textbf{quarter} of all American \textbf{youth}\underline{s} were behind the \textbf{counter} after school at \textbf{McDonald}\underline{'}s, but they were still living with their \textbf{parents}\underline{.}
On the other hand, there is a comment in the \textbf{forum} of the \textbf{newspaper} \textbf{Wall} \textbf{Street} \textbf{Journal}\underline{,} whose \textbf{author} states that it is \textbf{irresponsible} to have children if we do not know how to \textbf{feed} them.
In 1995 I \textbf{occupied} a room in P\textbf{ush}\textbf{\underline{kin}}\underline{s}\textbf{kaya} 10 and there was a \textbf{musical}\underline{-}art\textbf{istic} \textbf{club} for Bo\textbf{hem}\underline{e}, the house of the \textbf{Petersburg} Bo\textbf{hem}\underline{e} until the \textbf{renovation} work.
In \textbf{Petersburg}\underline{,} we have those who could be \textbf{experts}\underline{,} but they are being \textbf{blocked} by the need for more high-\textbf{level} \textbf{experts} to \textbf{evaluate} the former properly and open the way for them.
The end of the \textbf{concerts} should be about at the time when the \textbf{Maya} \textbf{calendar} \textbf{ends} on the \textbf{Pacific} island of \textbf{Kir}\textbf{\underline{ib}}\textbf{\underline{ati}}\underline{,} which is in a 12 \textbf{hour} time \textbf{zone} before us.
The aim of the \textbf{concert} is to \textbf{raise} the funds for \textbf{fur}\underline{n}ishing a multi-\textbf{function}\underline{al} education centre for people with \textbf{disabilities}\underline{,} which will be called S\textbf{TU}\underline{DE}O at the Jedli  u20\textbf{47} \textbf{ka} \textbf{Institute} in \textbf{Prague}\underline{.}
However, the ideas of the young \textbf{engineer} (\textbf{born} \textbf{190}\textbf{\underline{5)}} left the \textbf{audience} \textbf{cold} and after years   u20\textbf{47} \textbf{tern}\underline{feld} still \textbf{remembered} that only Dr. \textbf{Jan} Ga\textbf{dom}\underline{ski} had shown interest in his work.
This situation is \textbf{exacerbat}\underline{ed} by the fact that the \textbf{employers} are completely \textbf{unwilling} to pay their \textbf{taxes} and \textbf{thereby} to \textbf{compensate} for the social and economic damage they have caused.
\textbf{"...}\textbf{\underline{that}} nothing comes out of violence or could ever \textbf{arise}\underline{"} \textbf{sing}\underline{s} Sting in the \textbf{song} \textbf{Fra}\textbf{\underline{gil}}\underline{e}, whose most important \textbf{verse} in the \textbf{chor}\underline{us} is: \textbf{"...}\textbf{\underline{that}}\underline{'}s not to \textbf{forget} how \textbf{fragile} we are" .
A \textbf{distinction} must be made here between the \textbf{residents} of Israel and their leaders, because the international \textbf{bankers} in Israel, like us, the people, only choose their own \textbf{candidates}\underline{.}
The server Bankovn xedpoplat\textbf{ky}\underline{.}com, in cooperation with the \textbf{Association} of \textbf{Liberal} \textbf{Economist}\underline{s} La\textbf{isse}\underline{z} \textbf{Fair}\underline{e}, \textbf{nominated} the EU regulation on the \textbf{volume} of food \textbf{stocks} in the \textbf{territory} of a member country in addition to the \textbf{aforementioned} \textbf{absurd}\underline{ities}.
The problem is small-\textbf{minded} policy - if \textbf{someone} from the right or from the left comes up with a good proposal, it is \textbf{deliberately} \textbf{rejected}\underline{,} and that is something that the public only \textbf{stops}\underline{.}
By the way, Aston \textbf{Martin} was a child's \textbf{dream} - \textbf{James} \textbf{Bond} always \textbf{liked} how he \textbf{drove} in the car, was \textbf{ga}\textbf{\underline{lant}} to women and at the same time \textbf{fought} against \textbf{evil}\underline{.}
At the end of the \textbf{nearly} 500-\textbf{metre}\underline{-}\textbf{long} \textbf{hike} you will be \textbf{rewarded} not only with a \textbf{fantastic} view of the city, but also with \textbf{Dutch} \textbf{crown}\underline{s} and \textbf{fried} \textbf{fi}\textbf{\underline{cus}} \textbf{trees}\underline{.}
Is it difficult for Germany to \textbf{reconcile} its close relations with Israel and the USA on the one hand and the position of the main partners in the EU on the other?
In addition, "Voices for Africa" has set up a \textbf{secondary} school, built two \textbf{chicken} \textbf{houses} and, together with the American health \textbf{organisation} P\textbf{SI}\underline{,} \textbf{organized} that many people in the village had an \textbf{HIV} test.
"Remark\textbf{ably} many high-al\textbf{titude} people are also present in some parts of China, in Japan or in the Hunza \textbf{Valley} in Pakistan," \textbf{says} \textbf{Sc}\textbf{\underline{holz}}\underline{,} "\textbf{ther}\underline{e} are also extremely many very old men living in \textbf{Sardinia}\underline{".}
But what the \textbf{61}\underline{-}\textbf{year}\underline{-}\textbf{old} \textbf{engineer}\underline{,} who has a \textbf{doctor}\underline{ate} from the American University of South \textbf{California}\underline{,} really \textbf{wants} to save is something the \textbf{Egyptian}\underline{s} are aware of.
This was and is an \textbf{interpretation} and it is to be \textbf{fear}\underline{ed} that the \textbf{Islamist}\underline{s} will use the \textbf{mud}\underline{d}led \textbf{wording} and the legal leeway that goes with it for a \textbf{stricter} \textbf{interpretation} of \textbf{Sha}\textbf{\underline{ria}} law.
\textbf{Ten}\underline{s} of thousands of \textbf{Mexican} families have been affected by \textbf{violent} \textbf{crimes} over the past six years, and the new \textbf{president} has \textbf{promised} to address this problem in particular during his term of office.
As I should learn during my trip, there is something that makes this relationship even more \textbf{complicated}\underline{:} some \textbf{Mexican} leaders and \textbf{sections} of the \textbf{educational} community want to \textbf{resume} their links with the \textbf{dia}\underline{sp}\textbf{ora}\underline{.}
The leaders of \textbf{Hamas}\underline{,} the \textbf{Islamist} movement that has been in control of \textbf{Gaza} since 2007, will \textbf{claim} to have \textbf{pushed} back the \textbf{Israelis}\underline{,} even though its group has \textbf{suffered} huge \textbf{losses}\underline{.}
Turkey, a re\textbf{sur}\textbf{\underline{gent}} regional power that was once \textbf{regarded} as Israel's \textbf{closest} \textbf{Muslim} ally, has taken over \textbf{Hamas} - just like \textbf{Qatar}\underline{,} one of the \textbf{richest} and most \textbf{dynamic} \textbf{Gulf} states.
In doing so, the government is starting from \textbf{studies} that have shown that people who have not started \textbf{smoking} at the age of 26 are 9\textbf{9\%} likely to stop \textbf{smoking} after that.
The problem, according to John D. East\textbf{wood}\underline{,} an \textbf{associated} \textbf{professor} of \textbf{psychology} at the University of York in \textbf{Ontario}\underline{,} \textbf{Canada}\underline{,} is that \textbf{bo}\underline{re}\textbf{dom} has been \textbf{defined} and \textbf{discussed} in many ways.
He found that 3\textbf{2\%} of a\textbf{dol}\underline{es}\textbf{cent}\underline{s} were \textbf{bo}\underline{red} in school and in doing their home\textbf{work}\underline{,} \textbf{whereas} 2\textbf{3\%} \textbf{indicated} that they were \textbf{bo}\underline{red} when they were not in school.
In the \textbf{uncertain} weeks following the state u2019s decision to legalize small \textbf{amounts} of \textbf{mar}\underline{i}juana for its own use, the answer to \textbf{hundreds} of \textbf{smaller} \textbf{drug} \textbf{offences} \textbf{depends} less on the law than on the location.
It \textbf{showed}\underline{,} among other things, \textbf{graduate} Joe \textbf{Cook}\underline{e}, former \textbf{president} of \textbf{Oxford} University u2019s \textbf{conservative} \textbf{student} \textbf{association}\underline{,} who \textbf{drove} in a \textbf{Roll}\underline{s}-\textbf{Ro}\underline{y}ce and used \textbf{silver}\underline{-}\textbf{colour}\underline{ed} \textbf{suit}\underline{s} and \textbf{silver}\underline{-}\textbf{plate}\underline{d} walking \textbf{stick}\underline{s}.
What is even more \textbf{tragic} is that it was \textbf{Oxford} - a \textbf{university} that not only produced 14 Tory \textbf{prime} \textbf{ministers}\underline{,} but still \textbf{hide}\underline{s} behind an undis\textbf{put}\underline{ed} \textbf{reputation} for \textbf{equality} and freedom of thought.
\textbf{Four} months of work and 25 "R\textbf{aga}\textbf{\underline{zz}}\underline{e}" (as the \textbf{fashion}\textbf{\underline{maker}} called his se\textbf{wing}\underline{s}) were necessary to make this  \textbf{elf}\underline{-}le\textbf{gged} \textbf{silk} \textbf{dress} with beads, 12 different \textbf{embr}\textbf{\underline{oid}}\textbf{\underline{erie}}\underline{s} and a four-and-a-\textbf{half}\underline{-}\textbf{metre} \textbf{tail}\underline{.}
"\textbf{This} work is for animals and not for humans" \textbf{protests} \textbf{Mad}\textbf{\underline{rus}}\underline{in}, a \textbf{stra}\underline{te}gist, \textbf{42}\underline{-}\textbf{year}\underline{-}\textbf{old} \textbf{bear}\underline{er} who works three \textbf{decades} since \textbf{leaving} school at Kawah Ijen.
"I will not \textbf{retire}\underline{,} I will die here because the \textbf{volcano} was my whole life" \textbf{explains} Un\textbf{ain}\underline{ik}, opening his \textbf{mouth} wide, with some \textbf{teeth} \textbf{missing}\underline{.}
In four of the cases they linked the term to "s\textbf{omething} very own" at a personal level and "to the \textbf{password} and the user" when they applied it to social networks.
It could therefore be said that the procedures for \textbf{survival} of the companies that allow \textbf{Mexican} laws have no \textbf{validity} in the country of \textbf{stars} and \textbf{strip}\underline{es}, \textbf{contrary} to international agreements.
For this reason, the Gonz xe1lez Sada family \textbf{appeal}\underline{s} to the same Court of \textbf{App}\underline{e}al for the vote to be held in \textbf{plenary}\underline{,} that is to say by all the \textbf{judges}\underline{,} because only three of them voted.
"\textbf{Th}\textbf{\underline{ose}} were the best years I have \textbf{enjoyed} most because I have been part of \textbf{eight} \textbf{Va}\textbf{\underline{quer}}\underline{os} \textbf{championship}\underline{s} since \textbf{1967}\underline{,} be it as a \textbf{manager}\underline{,} co-\textbf{chair}\underline{man} or trainer.
"\textbf{It} is \textbf{fascinating} to see what people are doing to comfort themselves," said \textbf{Bri}\underline{d}gid \textbf{Robinson}\underline{,} a 23-\textbf{year}\underline{-}\textbf{old} \textbf{student} in Rutgers-Camden for \textbf{religion} and \textbf{socio}\textbf{\underline{logy}} from \textbf{Had}\textbf{\underline{don}}\textbf{\underline{field}}\underline{,} New \textbf{Jersey}\underline{.}
This study has also shown that after 12 years of monitoring, the \textbf{probability} of \textbf{meta}\underline{sta}ses \textbf{forming} is 30 to \textbf{40\%} higher if early \textbf{detection} is not carried out.
This "\textbf{inter}\underline{r}uption" \textbf{creates} an \textbf{electromagnetic} \textbf{wave} (light, \textbf{infrared} or \textbf{ultra}\textbf{\underline{violet}} \textbf{ray}\underline{s}, etc. \textbf{),} and this \textbf{wave} is nothing more than a photon and therefore one of the \textbf{Bos}\underline{ons} of \textbf{Power}\underline{.}
That is why a huge p\textbf{article} \textbf{acc}\underline{e}lerator such as C\textbf{ERN} is needed - the \textbf{Large} \textbf{Had}\underline{ron} \textbf{Coll}\underline{id}er is a 27 km \textbf{ring}\underline{!} - to achieve this kind of energy.
For \textbf{science}\underline{,} they are used to test the standard model (\textbf{SM}\underline{),} and they also allow \textbf{phy}\underline{s}icists to study \textbf{carefully} all \textbf{deviation}\underline{s} between the \textbf{observations} and the \textbf{prediction}\underline{s} of the \textbf{SM}\underline{.}
The \textbf{scandal} was \textbf{revealed} by a detailed \textbf{investigation} into the \textbf{mis}\underline{ap}pro\textbf{pri}\underline{ation} of \textbf{contracts} for road construction in \textbf{Quebec}\underline{,} which the then \textbf{Prime} Minister \textbf{reluctant}\underline{ly} agreed to.
It is time for the \textbf{Afghan} \textbf{army} to take \textbf{possession} of its \textbf{territory} again and for the \textbf{Afghan} people to decide their future without \textbf{expecting} anything from us.
The \textbf{Taliban} are made up of foreign extremists, former leaders who have \textbf{fled} to Pakistan, but often also farmers who \textbf{refuse} to have an \textbf{armed} foreign \textbf{presence}\underline{,} as was the case at the time of the \textbf{Soviet}\underline{s}.
Just before the \textbf{constitutional} \textbf{declaration} in \textbf{mid}\underline{-}\textbf{No}\underline{ve}\textbf{mber}\underline{,} they \textbf{turned} their backs on their view that they were not able to make their views heard.
Finally, Article 2, which has \textbf{attracted} all attention, remains the same as that of the \textbf{1971} \textbf{Constitution} and states that 'the principles of \textbf{Sha}\textbf{\underline{ria}} law are the main source of justice'.
For \textbf{Islamist}\underline{s}, the fact that this \textbf{article} has not been \textbf{amended} is \textbf{proof} of their good will and respect for the other members of \textbf{Egyptian} society.
They are particularly concerned with Article \textbf{220}\underline{,} which gives Al-Az\textbf{har} University a \textbf{consult}\underline{ative} role, particularly with regard to the \textbf{verification} of \textbf{conformity} with \textbf{Sha}\textbf{\underline{ria}} law.
\textbf{Visitors} come here for \textbf{treatments} using \textbf{salt} water (\textbf{natural} \textbf{salt}\underline{s}\textbf{ole}\underline{)} and \textbf{cur}\underline{ative} \textbf{mud} as well as for treatment of \textbf{skin} in\textbf{flamm}\underline{ation}, aller\textbf{gie}\underline{s}, asthma, eczema, arthr\textbf{itis}\underline{,} \textbf{bro}\underline{n}ch\textbf{itis}\underline{,} \textbf{sugar} \textbf{disease} and to \textbf{calm} \textbf{stressed} \textbf{nerve}\underline{s}.
The money in the trip is not taken in \textbf{euros}\underline{,} but in \textbf{dollars} that can easily be changed into she\textbf{lves} (\textbf{current} exchange rate: 1 \textbf{dollar} to 3.8 she\textbf{lves}\underline{).}
"\textbf{To}\underline{day}, there are \textbf{countless} private \textbf{arm}\textbf{\underline{ament}}\underline{s} \textbf{factories} that do not stand up to international competition and therefore waste their \textbf{weapons} under their \textbf{hands} on the black market, for example in \textbf{Moscow}\underline{,}" reports the \textbf{expert}\underline{.}
\textbf{Black} \textbf{Friday} lasted in its \textbf{store} from 8 a.m. on \textbf{Thursday} to \textbf{midnight} the next day, and during that time \textbf{Wal}\underline{mar}t \textbf{sold} about \textbf{5000} \textbf{items} per second.
- And all this \textbf{united} in your art \textbf{clinic}\underline{...} - It was important for me to be at the center of the \textbf{Petersburg} culture, where the best \textbf{creative} \textbf{artists} should \textbf{gather}\underline{.}
Today it is easy to become famous, but culture and \textbf{popularity} are not the same: you can be famous without making a cultural contribution.
The same is true of Erarta, but with the \textbf{difference} that they are \textbf{honest} in saying that they do not accept all \textbf{contemporary} art and that some \textbf{painter}\underline{s} therefore have to look for other \textbf{museums}\underline{.}
The system must \textbf{exclude} those who want to attack and \textbf{abuse} the system and not \textbf{punish} those who have made a \textbf{formal} \textbf{error} that does not \textbf{affect} the actual decision-\textbf{making} process.
I would like to \textbf{recall}\underline{,} for example, the \textbf{lecture} by A.   u20\textbf{47} \textbf{tern}\underline{feld} on 6 December \textbf{1933} at the ob\textbf{serv}\textbf{\underline{atory}} in \textbf{Warsaw}\underline{,} where the \textbf{author} presented ideas from his \textbf{pioneering} work "In\textbf{put} to Cosmon\textbf{aut}\textbf{\underline{ics}}\underline{".}
However, these solutions are wrong and always lead to an \textbf{aggravat}\underline{ion} of the situation (see the \textbf{founding} of the \textbf{Federal} \textbf{Reserve} so that \textbf{crises} like the \textbf{ones} they caused in 19\textbf{07} do not re\textbf{cur}\underline{).}
But I can no longer see how the Republic has been \textbf{pl}\textbf{\underline{under}}\underline{ed} for 20 years, how \textbf{th}\textbf{\underline{ieve}}\underline{s} are running around \textbf{freely}\underline{,} while people are being raised in \textbf{taxes} and \textbf{retirement} ages.
In order to \textbf{counter} this \textbf{stupid} situation, a few years ago it was decided to contribute to general education and to \textbf{rebuild} the \textbf{seven} \textbf{fi}\textbf{\underline{ct}}\underline{it}\textbf{ious} \textbf{bridge}\underline{s} \textbf{displayed} on the euro \textbf{notes} as \textbf{pretty} \textbf{brush}\underline{ed} \textbf{concrete}\textbf{\underline{mini}}\textbf{\underline{atur}}\underline{es}.
\textbf{Stephen} Szabo is \textbf{deputy} \textbf{director} of the \textbf{Transatlanti}\underline{c} \textbf{Academy} in \textbf{Washington}\underline{,} an \textbf{institute} where \textbf{academic}\underline{s} and policy \textbf{experts} from Europe and North America carry out joint research on the challenges \textbf{facing} the \textbf{transatlanti}\underline{c} community.
\textbf{Initial}\underline{ly}, it was the private commitment of \textbf{individuals} to send a child to school for a \textbf{couple} of \textbf{euros} a year and to allow him a warm \textbf{meal} a day.
This section of an \textbf{infrared} image of the \textbf{Spitze}\underline{r} \textbf{Tele}\textbf{\underline{scope}} shows a "\textbf{family} \textbf{portrait}\underline{"} of un\textbf{count}\underline{ed} \textbf{generation} of \textbf{stars}\underline{:} the \textbf{oldest} \textbf{stars} are \textbf{visible} as \textbf{blue} dots, the \textbf{pink} "\textbf{new}\textbf{\underline{born}}\underline{s}" in the star \textbf{circle} are \textbf{harder} to \textbf{identify}\underline{.}
While her \textbf{mother} \textbf{tells} her \textbf{story}\underline{,} from the \textbf{wall} a picture of \textbf{Maria}\underline{na} \textbf{looks} down on us.
The fact that \textbf{pragmatic} President \textbf{Mor}\underline{si} met \textbf{Barack} \textbf{Obama} to achieve a \textbf{ceasefire} could be a \textbf{promising} sign - and perhaps \textbf{symbol}\underline{ize} the beginning of a new \textbf{era}\underline{.}
Although \textbf{Australia} has one of the \textbf{lowest} \textbf{smoking} rates in the world and the changes will have a \textbf{slight} impact on the \textbf{profits} of \textbf{multinational}\underline{s}, other countries are already \textbf{considering} similar steps.
If, on the other hand, you carry out a one-\textbf{week} activity - "as well as \textbf{searching} for \textbf{fault}\underline{y} products on a \textbf{conveyor} \textbf{belt}\underline{,} music can \textbf{distract} and help you not feel \textbf{bo}\underline{red}".
The police authorities no longer \textbf{prosecut}\underline{e} \textbf{adults} over 21 for \textbf{possession} on a small \textbf{scale}\underline{,} which is \textbf{permitted} by law as soon as the new laws enter into force in the next few weeks.
At the same time, several cities, from the \textbf{suburb}\underline{s} of Den\textbf{vers} to the Western \textbf{Mountains}\underline{,} are voting to prevent new state-licensed \textbf{mar}\underline{i}juana \textbf{stores} from opening in their \textbf{communities}\underline{.}
"\textbf{This} situation is developing so quickly that I do not know what will happen next," \textbf{says} \textbf{Daniel} J. O\textbf{ates}\underline{,} \textbf{chief} of police in Aur\textbf{ora}\underline{,} \textbf{east} of Denver.
\textbf{Their} situation was \textbf{aggravat}\underline{ed} by a recent \textbf{documentary} on political students on \textbf{BBC} \textbf{Two}\underline{,} "\textbf{Wo}\textbf{\underline{nder}}\underline{land}: \textbf{Young}\underline{,} B\textbf{right} and on the \textbf{Right}\underline{",} which Tories \textbf{portray}\underline{ed} as an e\textbf{cc}\underline{en}\textbf{tric} and \textbf{neo}\underline{-}\textbf{Na}\underline{zi}.
"I suggest that they take some French \textbf{lessons} in your free time - so if you are not too \textbf{busy} with your social activities," \textbf{Pit}\underline{t} \textbf{jump}\underline{ed} at me.
On the \textbf{occasion} of the \textbf{exhibition} "\textbf{Val}\underline{en}\textbf{tino} - \textbf{Master} of \textbf{Cou}\underline{ture}", which was \textbf{opened} this week in London, \textbf{ABC} \textbf{talks} with Naty Abascal, Fi\textbf{ona} \textbf{Thyssen}\underline{-}Borne\textbf{mis}\underline{za} and other famous customers of the Italian \textbf{fashion}\textbf{\underline{maker}}\underline{.}
After \textbf{breaking} out large \textbf{sulphur} \textbf{stones}\underline{,} which can \textbf{weigh} up to 70 \textbf{kilo}\underline{s} in total, he transports them in two \textbf{ba}\textbf{\underline{mbo}}\underline{o} \textbf{basket}\underline{s} on his shoulders over the sheer path of \textbf{stone}\underline{.}
These changes in social conditions have \textbf{contributed} to the increase in the number of single people and to the \textbf{delay} in \textbf{marriage} and \textbf{birth}\underline{s}, the result of which is a reduction in the \textbf{birth} rate in \textbf{Singapore}\underline{.}
The \textbf{Municipal} Development \textbf{Authority} has started to control the number of small apartments known as "sho\textbf{uld}\underline{ard}s" that can be built in certain areas of the city.
As regards the decisions made, he said that the countries of Unasur '\textbf{will} take significant steps towards the goal of South American \textbf{citizenship}\underline{,} to which we \textbf{extend} the decisions on \textbf{residence} rights'.
The need for \textbf{Latin} America to continue to be an integrated region for \textbf{prosperity} and peace and with good \textbf{neighbour}\underline{ly} relations was another \textbf{aspect} \textbf{highlighted} at the summit.
\textbf{Santo}\underline{s} and \textbf{Ortega} would meet in \textbf{Mexico} on \textbf{Saturday}\underline{,} when they \textbf{intend} to be present at the \textbf{inaugura}\underline{tion} of the new President of that country, Enr\textbf{ique} Pe  u20\textbf{47} a \textbf{Nie}\underline{to}.
As you know, these measures were carried out despite the fact that the \textbf{Senat}\underline{e} had \textbf{ignored} the possibility because it considered them to be a \textbf{violation} of freedom of \textbf{expression} in social networks.
"\textbf{We} \textbf{analyze} why these ideas \textbf{spread} over time," he said, as well as the way in which \textbf{hypothe}\underline{t}ical \textbf{scenario}\underline{s} are offered that lead to a certain human \textbf{behavior}\underline{.}
However, the \textbf{Brenn}\underline{an} Center \textbf{considers} the \textbf{latter} a \textbf{myth} by \textbf{affirm}\underline{ing} that \textbf{fraud} in the US is \textbf{rare}\underline{r} than the number of people \textbf{killed} by the lightning \textbf{strike}\underline{.}
The democratic \textbf{critics} \textbf{denounce} the part\textbf{isa}\underline{n} nature of the laws \textbf{passed} and see them as a clear objective to influence the results in the countries that will decide for \textbf{2012}\underline{.}
It is too early to \textbf{confirm} with \textbf{certainty} that these changes to the legislation on the \textbf{electoral} system will have a significant impact on the \textbf{outcome} of the \textbf{2012} \textbf{presidential} \textbf{election}\underline{.}
He even manages \textbf{brave}\underline{ly} to \textbf{smile} and talk to the \textbf{strange}\underline{rs} who are \textbf{busy} around him, bring his \textbf{medicines} to him and offer him a bath.
\textbf{According} to Dr \textbf{Christian}\underline{e} Martel, \textbf{Quebec}\underline{'}s health system is not powerful enough to ensure that everyone has the right to high-\textbf{quality} \textbf{pal}\underline{li}ative care before it is accepted to \textbf{switch} to \textbf{eu}\textbf{\underline{than}}\textbf{\underline{asia}}\underline{.}
\textbf{Recently}\underline{,} she \textbf{says}\underline{,} I have seen a \textbf{patient} who has been in the \textbf{emergency} room for 14 days with great \textbf{pain}\underline{,} without taking any measures to \textbf{alleviate} it.
On the basis of a \textbf{70\%} black money share in the funding of \textbf{electoral} \textbf{campaigns} in \textbf{Quebec}\underline{,} he \textbf{joke}\underline{s}: 'I have been \textbf{told} that this is only a \textbf{slight} di\textbf{spar}\underline{ity} in reality.'
If this \textbf{story} \textbf{damages} \textbf{Quebec}\underline{'}s international \textbf{reputation} and that of \textbf{Montreal}\underline{,} Mr Du\textbf{ches}\underline{n}\textbf{eau} calls on those who \textbf{laugh} to take a look at their own back\textbf{yard}\underline{...}
This is done by means of a \textbf{mathematical} task that is started on \textbf{computers}\underline{,} with the \textbf{winner}\underline{,} who is a kind of \textbf{temporary} central banker, having the \textbf{privilege} of \textbf{adding} this additional line.
This work, which required a large number of local workers, has \textbf{helped} to \textbf{suppress} the ins\textbf{urg}\textbf{\underline{ency}}\underline{:} \textbf{irrigation}\underline{,} wells, \textbf{drinking} water, refore\textbf{station}\underline{,} \textbf{fruit} \textbf{trees}\underline{,} \textbf{soil} protection and increased agricultural land.
A much more \textbf{modest} budget will contribute to improving local living conditions, which are very hard in these \textbf{valley}\underline{s}, which are often more than 2000 metres high.
While \textbf{Egypt} remains more \textbf{divided} than ever with regard to the \textbf{constitutional} \textbf{declaration}\underline{,} which gives it \textbf{temporary} \textbf{unlimited} powers, it has decided to put everything on a card.
\textbf{Jerusalem} is also the most \textbf{sacred} place of the \textbf{Jews} - the W\textbf{ailing} \textbf{Wall}\underline{,} the remains of a \textbf{temple} \textbf{destroyed} by the Romans in 70 A.D.
\textbf{Half} of all \textbf{weapons} on the black market are there because of 'the debt of those responsible for their work with \textbf{weapons}\underline{'}, the report states.
A sales \textbf{advisor} to an \textbf{arms} \textbf{shop} who does not want to be \textbf{named}\underline{,} \textbf{assure}\underline{s} that \textbf{weapons} found in illegal \textbf{excavat}\textbf{\underline{ions}} have long since not been \textbf{bought} because they are \textbf{outdated}\underline{.}
The \textbf{protests} began last week after \textbf{Thanks}\underline{g}\textbf{iving}\underline{,} on the so-called \textbf{Black} \textbf{Friday}\underline{,} when sales were being made in the USA, \textbf{attract}\underline{ing} \textbf{millions} of customers, which sometimes led to hand masses.
For example, in the field of \textbf{controlling} \textbf{objects} in public places, we worked on a project in which we \textbf{experiment}\underline{ed} with short and short, instead of with \textbf{loading} \textbf{gesture}\underline{s}.
- \textbf{Imagine} for a moment that the \textbf{manipulation} of \textbf{virtual} \textbf{holo}\textbf{\underline{gram}}\underline{s} in the air is not only \textbf{accessible} to \textbf{Tony} Stark from \textbf{Iron} Man, but also to \textbf{ordinary} \textbf{mor}\underline{tal}s.
He is also a man of the city and makes a \textbf{smile} to his fellow citizens through his \textbf{presence} on the street and makes them feel good.
\textbf{Under} pressure from global and European economic competition, the Czech Republic will be \textbf{forced} to continue to \textbf{seek} ways of lowering the social level of the population.
\textbf{Having} \textbf{succeeded} in \textbf{trigger}\underline{ing} World War I by \textbf{murder}\underline{ing} the \textbf{Habsburg} \textbf{successor} \textbf{Ferdinand} in \textbf{Sarajevo}\underline{,} they \textbf{destroyed} the Russian T\textbf{sar} by the \textbf{Bol}\underline{sh}\textbf{evi}\underline{k} \textbf{Revolution}\underline{.}
On the one hand he is a \textbf{realistic} \textbf{polit}\underline{th}r\textbf{iller}\underline{,} but at the same time a so-called "\textbf{Ca}\underline{per} \textbf{Movie}\underline{",} i.e.
I believe that German foreign policy is \textbf{motivated} by economic policy, that is, by \textbf{exports} and its relations with certain regions, such as Russia, China or the Middle East.
"\textbf{It} is becoming more and more difficult for \textbf{foreigners} to protect their \textbf{brands} in China," \textbf{says} \textbf{Thomas} \textbf{Pat}\underline{t}\textbf{loch}\underline{,} \textbf{attorney} at \textbf{Taylor} Wessing, who special\textbf{ises} in property rights \textbf{violations} in \textbf{Far} East.
And if you return the \textbf{87}\textbf{\underline{33}} km air line to \textbf{Heidelberg}\underline{,} to the \textbf{stamp}\underline{ing} \textbf{singer}\underline{s} in the rehe\textbf{ars}\underline{al} room on Bergheimer \textbf{Stra} xdfe, you can see it \textbf{shine} there as well.
\textbf{Ten}\underline{s} of thousands \textbf{gathered} in \textbf{unusual} \textbf{harmony} on \textbf{Friday} evening in Tahrir \textbf{Square} in \textbf{Cairo} and \textbf{promised} to \textbf{overthrow} the \textbf{Charter} before it can enter into force.
As \textbf{Mexico} u2019s future \textbf{president}\underline{,} Enr\textbf{ique} \textbf{Pen}\underline{a} \textbf{Nie}\underline{to}, \textbf{prepare}\underline{s} to take office, \textbf{BBC} \textbf{Will} \textbf{Grant} \textbf{analyze}\underline{s} the challenges and \textbf{mixed} \textbf{feelings} of his people.
"\textbf{We} expect real and \textbf{lasting} changes from him," \textbf{says} his \textbf{friend} and political ally \textbf{Gabriel} \textbf{Ol}\underline{ver}a Hernandez, who is a member of the \textbf{Congress} for the \textbf{Pen}\underline{a} \textbf{Nie}\textbf{\underline{tos}} party, the \textbf{PRI}\underline{.}
The \textbf{charges} against Manning include \textbf{favor}\underline{ing} the \textbf{enemy}\underline{,} \textbf{il}\underline{leg}\textbf{iti}\textbf{\underline{mate}} \textbf{publication} of \textbf{intelligence} on the Internet, the transfer of national \textbf{defence} information and the theft of public property or documents.
And, in view of the \textbf{unfair} distribution of income, un\textbf{bri}\underline{d}led \textbf{corruption} and \textbf{drug} violence, many of us are not so sure that this is really a great country.
\textbf{Apart} from the different health \textbf{warning}\underline{s} and \textbf{pictures}\underline{,} there will be the only \textbf{difference} between the \textbf{pack}\underline{s} in the brand \textbf{names}\underline{,} which are \textbf{printed} in \textbf{identical}\underline{,} small \textbf{font}\underline{s}.
"\textbf{You} just take a \textbf{til}\underline{t} and put the \textbf{box} away," \textbf{says} \textbf{Victor} El Hage when you buy a \textbf{cigarette} \textbf{box} where a photo is \textbf{printed} with a \textbf{mouth} \textbf{tu}\textbf{\underline{mor}}\underline{.}
D\textbf{espite} a number of \textbf{arrest}\underline{s} by consumers and \textbf{seller}\underline{s} of \textbf{medicinal} \textbf{mar}\underline{i}juanas, the \textbf{Federal} Government has \textbf{largely} allowed the \textbf{sale} of \textbf{medicinal} \textbf{mar}\underline{i}juana in \textbf{Color}\underline{ado}, \textbf{Washington} and 16 other states.
\textbf{Conservative} members of \textbf{Corp}\underline{us} \textbf{Christi} \textbf{College}\underline{'}s \textbf{Junior} \textbf{Common} Room (J\textbf{CR}\underline{)} \textbf{claim} that they are "often \textbf{actively} \textbf{isolated}\underline{,} \textbf{personally} \textbf{attacked} and \textbf{declared} \textbf{undesirable}\underline{"} because of their political views.
Somer\textbf{set} House, the former \textbf{residence} of \textbf{Isabel} I of \textbf{England}\underline{,} is the only place in the British capital \textbf{worthy} of \textbf{hosting} an \textbf{exhibition} on \textbf{Valentin}\underline{o} \textbf{Gar}\textbf{\underline{ava}}\underline{ni}.
\textbf{Name}\underline{s} such as S\textbf{ib}\textbf{\underline{illa}} de \textbf{Luxembourg}\underline{o}, \textbf{Glo}\textbf{\underline{ria}} de \textbf{Thu}\underline{r}n and \textbf{Taxi}\underline{s}, M\textbf{ette}\underline{-}\textbf{Mar}\underline{it} of \textbf{Norway}\underline{,} \textbf{Ros}\textbf{\underline{ario}} of \textbf{Bulgaria} or Sof xeda of \textbf{Habsburg} \textbf{ra}\underline{di}ate in this \textbf{audience} of \textbf{fashion} dolls.
"\textbf{Si}\textbf{\underline{nce}} we usually carry 70 \textbf{kg}\underline{,} we get about 4\textbf{6,000} rupees \textbf{(3}\underline{.}8 \textbf{euros}\underline{)} for each way," \textbf{explains} Anto, who usually does three \textbf{routes} a day.
This friendly and \textbf{intelligent}\underline{,} but life-s\textbf{trick}\underline{en} young man could work as a tourist \textbf{guide}\underline{,} \textbf{wait}\underline{er} or at the reception of a hotel, but instead he does the work of a carryer.
\textbf{Time} \textbf{passes}\underline{,} but poverty \textbf{persist}\underline{s} on \textbf{generation} in one of the hardest \textbf{profession}\underline{s} in the world: those who work as a human \textbf{burden} on Kawah Ijen.
"\textbf{This} has made it possible for people \textbf{except} to \textbf{mar}\underline{ry} and make a family much more options in terms of life \textbf{goals} and to set priorities," she \textbf{explains}\underline{.}
The \textbf{teenage}\underline{r} has user \textbf{accounts} in \textbf{Hot}\underline{mail}, \textbf{Facebook}\underline{,} My \textbf{Space} and \textbf{Ask}\underline{,} and in \textbf{Ask} he \textbf{admit}\underline{s} not to know 20 of the people he has added to his \textbf{friend} list.
However, there is a risk that he will \textbf{suffer} \textbf{physical} and \textbf{psychological} damage because he is tra\textbf{pped} in a \textbf{narrow} space and cannot carry out \textbf{physical} exercises \textbf{outdoor}\underline{s}.
He decided to take care of his \textbf{illness} alone and began to find out about it with such commitment that he just \textbf{celebrated} his \textbf{43}\underline{th} \textbf{birthday}\underline{.}
\textbf{Fabr}\underline{i}\textbf{zio} has been living with the human \textbf{immun}\underline{o}\textbf{def}\textbf{\underline{ici}}\textbf{\underline{ency}} \textbf{virus} (H\textbf{IV}\underline{)} for 22 years.
"W\textbf{hy} do you need it?" is a common m\textbf{ock}\underline{ing} question of social workers, \textbf{orientation} staff in \textbf{schools}\underline{,} employees in \textbf{pharma}\textbf{\underline{cies}} and in the health system that young people do not want to \textbf{expose}\underline{,} \textbf{insure}\underline{d} the \textbf{correspond}\underline{ent}.
There are half a \textbf{dozen} \textbf{examples}\underline{,} including \textbf{Ag}\textbf{\underline{rem}}\underline{ex} and Comer\textbf{cial} \textbf{Mexican}\underline{a}, whose \textbf{liabilities} among companies of the group have been \textbf{confirmed} by the \textbf{Institut}\underline{o} \textbf{Federal} de Con\textbf{cur}\underline{s}os \textbf{Mer}\textbf{\underline{can}}\textbf{\underline{tile}}\underline{s} (Federal \textbf{Institute} for \textbf{Trade} Con\textbf{solid}\underline{ations}).
If this is not accepted, the \textbf{Cer}\underline{ci}orare \textbf{appeal} will be filed, \textbf{calling} for a higher body to review the \textbf{proceedings}\underline{,} in this case by the United States \textbf{Supreme} Court.
\textbf{Lind}\underline{a} \textbf{Gra}\underline{y}, who played the role of his \textbf{wife} in the original and \textbf{subsequent} series, was with \textbf{Hag}\underline{man} when he died in \textbf{Dal}\textbf{\underline{las}} \textbf{hospital}\underline{,} said her publicist \textbf{Jeff}\underline{re}y \textbf{Lan}\underline{e}.
J.R. had \textbf{sw}\underline{or}n and \textbf{threatened} to \textbf{portray} her as a prost\textbf{itu}\underline{te} if she did not leave the city.
It is unique and \textbf{irre}\textbf{\underline{place}}\underline{able} for \textbf{millions} of \textbf{lovers} in the world and remains in our hearts for those who were \textbf{lucky} enough to know and love it.
On the other hand, the same states allow members of fishing or \textbf{hunting} \textbf{associations} who vote more for the \textbf{Republican} side to use the \textbf{cards} \textbf{issued} by these \textbf{clubs} for elections.
For example, in the 2008 general \textbf{election} in \textbf{Florida}\underline{,} 3\textbf{3\%} of pre-el\textbf{ection} \textbf{voters} were Afro-\textbf{American}\underline{s}, even though they account for only 13\% of the state u2019s \textbf{electorate}\underline{.}
Today, many men who have \textbf{recognized} \textbf{cancer} do not receive treatment because their \textbf{cancer} is not \textbf{aggressive} and does not \textbf{pose} a \textbf{threat} to their lives.
And several \textbf{organizations}\underline{,} such as the \textbf{Victor}\underline{-}\textbf{Ga}\textbf{\underline{db}}\textbf{\underline{ois}} Home and the \textbf{Montreal} \textbf{Char}\underline{ity} \textbf{Society}\underline{,} are more or less \textbf{specialised} in caring for \textbf{cancer} \textbf{patients}\underline{.}
In addition, an \textbf{organise}\underline{r} of the \textbf{Mayor}\underline{'}s Party, \textbf{Martin} Du\textbf{mont}\underline{,} has \textbf{accused} Mr \textbf{Tre}\underline{mb}\textbf{lay} of \textbf{deliberately} \textbf{ignor}\underline{ing} a \textbf{shadow} budget that was \textbf{pour}\underline{ing} black money into his co\textbf{ffer}\underline{s}.
But if we \textbf{win} a home \textbf{match} against \textbf{Tro}\textbf{\underline{yes}} 4-0 and you still find something you can reproach us for, that is certainly a bit \textbf{fru}\underline{st}\textbf{rating}\underline{.}
\textbf{Its} \textbf{Pay}\textbf{\underline{tun}}\underline{ia} system is \textbf{equivalent} to a credit card (\textbf{with} real money) or a contactless payment with a mobile phone, but \textbf{uses} \textbf{Bit}\underline{co}in to validate \textbf{transactions}\underline{,} which are therefore \textbf{cheaper}\underline{.}
You just have to \textbf{specify} an address that can be " \textbf{photograph}\underline{ed} and \textbf{recognized}\underline{"} by a phone, \textbf{says} \textbf{Pierre} No\textbf{iza}\underline{t}, who \textbf{assure}\underline{s} that he has thousands of users.
The \textbf{withdrawal} of French \textbf{troops} from the base in \textbf{Ni}\underline{j}rab, which I \textbf{observed} from a \textbf{hill} planted with al\textbf{mond} \textbf{trees}\underline{,} \textbf{financed} by French \textbf{loans}\underline{,} was carried out properly.
\textbf{Its} \textbf{supporters} are \textbf{assured} that it is a way to end the institutional and political crisis as quickly as possible and to \textbf{accelerate} the \textbf{transition} process.
The \textbf{ruins} of the For\textbf{tress} of \textbf{Mass}\underline{ada} are the remains of the \textbf{secret} \textbf{hide}\textbf{\underline{away}} from \textbf{enemies} who had herodes of the Great built for his family in 25 A.D.
\textbf{Old} \textbf{Qu}\underline{m}ran \textbf{manuscript}\underline{s} or \textbf{scroll}\underline{s} from the Dead Sea found in \textbf{cave}\underline{s} in the \textbf{Jud}\underline{a}ean \textbf{Desert} are \textbf{kept} there, as well as about 500 \textbf{thousand} \textbf{archaeological} and anthrop\textbf{ological} \textbf{exhibit}\underline{s}.
The most \textbf{striking} section is the \textbf{monument} for the children, built to \textbf{commemorat}\underline{e} the \textbf{1.5} million children who were \textbf{destroyed} in the \textbf{concentration} \textbf{camps} and gas \textbf{chamber}\underline{s}.
Am\textbf{az}\underline{ing}ly, the Red Sea is also bathed in the winter months, as the water \textbf{temperature} does not fall below 21   u20\textbf{47} C and the air warms up to 23   u20\textbf{47} C.
\textbf{According} to \textbf{tradition}\underline{,} it was here that Noah built his a\textbf{rk}\underline{,} and \textbf{Pers}\underline{e}us \textbf{saved} the beautiful And\textbf{rome}\underline{da} with which he had a long and happy life.
In many caf xe9s, restaurants and restaurants only \textbf{ko}\underline{s}her food is served, which \textbf{exclude}\underline{s} \textbf{por}\underline{k}, sea products, fish without \textbf{scale}\underline{s} and food \textbf{containing} both \textbf{milk} and \textbf{meat} products.
The \textbf{Chair} of the \textbf{Duma} Committee on Security and Com\textbf{bat} \textbf{Corr}\underline{up}tion, I\textbf{rina} \textbf{Jar}\textbf{\underline{ova}}\underline{ja}, supported the proposal and \textbf{promised} that the amendments to the \textbf{arms} law would be submitted \textbf{shortly} to the \textbf{Duma}\underline{.}
Researchers from \textbf{California} University in \textbf{Ber}\underline{ke}ley show that if the company increased its \textbf{average} \textbf{wage} to 12 \textbf{dollars} an \textbf{hour}\underline{,} it would cost \textbf{Wal}\underline{mar}t \$3.2 billion.
In fast-\textbf{food} restaurants, the minimum \textbf{wage} is \textbf{gradually} \textbf{rising}\underline{,} but not too high, and on \textbf{average}\underline{,} their \textbf{ordinary} New York employees receive \textbf{USD} \textbf{8.}\underline{90} per \textbf{hour}\underline{.}
Now, in \textbf{interview}\underline{s} with \textbf{McDonald}\underline{'}s employees, I am \textbf{constantly} \textbf{hearing} people \textbf{complain}\underline{ing} that they are living on this \textbf{wage} and sometimes even \textbf{feeding} their children.
I think that in the near future we will have to work, above all, on developing new types of \textbf{sensors} that will enable us to measure people's \textbf{reactions} more closely.
The whole city \textbf{knows} \textbf{Kir}\textbf{\underline{ill}} \textbf{Mill}\underline{er}, the red \textbf{bear} that you can see at the Russian Museum, at the summer garden, at \textbf{scene} \textbf{meetings} or at openings.
I am a man of the past culture and \textbf{grew} up with \textbf{artists} who \textbf{lived} in poverty and died in poverty and \textbf{rejected} money to \textbf{paint}\underline{.}
"A law is never perfect, but it must be applied \textbf{correctly} - and I do not think this is the case with us," \textbf{Kal}\underline{a} commented on the current situation.
At the meeting of the \textbf{Supervisor}\underline{y} Committee of the \textbf{Chamber} of De\textbf{put}\underline{ies}, you \textbf{spoke} about a joint Czech-\textbf{German} project in which the laws of both countries on public \textbf{contracts} were \textbf{compared}\underline{.}
Even their colleagues in Jesen xedk had to leave at night, according to their data, the \textbf{roads} are free and wet up to the \textbf{altitude}\underline{s} after \textbf{chemical} treatment.
\textbf{Nevertheless}\underline{,} it has always worked without any problems,   u20\textbf{47} \textbf{SA} and British \textbf{Airways} have always been very well prepared for us, that I have sometimes \textbf{wonder}\underline{ed}.
In London and \textbf{Madrid} it is absolutely \textbf{custom}\underline{ary} for people with serious \textbf{disabilities} to be able to move \textbf{freely} in public space, go to the \textbf{museum}\underline{,} use \textbf{toilet}\underline{s}, etc.
\textbf{Liberal} \textbf{theories} and the media \textbf{claim} all too well that the state must not take part in its own economy with capital, and that \textbf{planned} economy \textbf{leads} to economic \textbf{disaster}\underline{.}
The server www.\textbf{bank}\underline{ov}nipop\textbf{lat}\textbf{\underline{ky}}\underline{.}com, which draws up an annual \textbf{survey} on the most \textbf{absurd} bank \textbf{charges}\underline{,} has decided this year to \textbf{organise} the competition "\textbf{Ab}\textbf{\underline{sur}}\underline{de}ste Verordnung bzw.
Finally, the European Commission met the Czech Republic so far that it \textbf{organised} a \textbf{tender} for the purchase of \textbf{ce}\textbf{\underline{real}}\underline{s} from countries which do not have access to the sea.
I always \textbf{publicly} support any good solution approach, even if it comes from the KS  u20\textbf{47} M or the O\textbf{DS}\underline{,} and I will also \textbf{oppose} bad ideas.
I think this can be called \textbf{pop}\underline{ul}ism, but all the proposals I have \textbf{spoken} about are already working in the world or have been \textbf{discussed} by important \textbf{experts}\underline{.}
The so-called Land\textbf{bou}\underline{w}\textbf{plastic} (K\textbf{LP}\underline{)} is a \textbf{dark}\underline{,} \textbf{homogen}\textbf{\underline{eous}}\underline{,} \textbf{load}\underline{-}bearing material that \textbf{smell}\underline{s} of a bissl after a new car and a bissl after a sports \textbf{shoe}\underline{.}
This is because it is \textbf{shift}\underline{ing} its foreign policy from a policy that was managed, so to speak, by the US to a German foreign policy.
Germany is still not used to it, it is still \textbf{unpleasant} and, for \textbf{obvious} reasons, it is still difficult for it to play a greater role.
I was \textbf{thinking} about that moment this week when \textbf{Mexican} President Enr\textbf{ique} \textbf{Pen}\underline{a} \textbf{Nie}\underline{to} \textbf{visited} the \textbf{White} House to meet President \textbf{Obama}\underline{.}
Let us tell our American colleagues how great a visit to that country is and how much pressure it \textbf{puts} on the political \textbf{leadership} to step up their \textbf{ties} with \textbf{Mexico}\underline{.}
\textbf{Wa}\underline{it}ing half a day at the airport for a \textbf{flight} is quite \textbf{nervous} - even if \textbf{books}\underline{,} \textbf{magazine}\underline{s} and \textbf{iPhone}\underline{s} (and, of course, tax-\textbf{free} shopping) are available.
"\textbf{We} do not want to get into a position where we \textbf{license} \textbf{someone} and then face a major problem at \textbf{federal} level," \textbf{says} \textbf{Bob} \textbf{Nicholson}\underline{,} a member of the City Council.
\textbf{Political} issues such as the \textbf{mining} \textbf{strike}\underline{,} the \textbf{privatisation} and the \textbf{rejection} of the government of \textbf{sanctions} against the \textbf{apart}\textbf{\underline{heid}} regime of South Africa found their way into the \textbf{wood}\underline{-}\textbf{pan}\underline{ell}ed rooms of the \textbf{Tu}\textbf{\underline{torium}}\underline{.}
At my first of these events, I was \textbf{supposed} to \textbf{translate} 18th-\textbf{century} French \textbf{texts} into English; I had not been able to understand what was to come.
A new \textbf{student} in \textbf{philosophy}\underline{,} \textbf{politics} and economics who, \textbf{iron}\textbf{\underline{ically}}\underline{,} had \textbf{visited} Eton \textbf{College} as \textbf{conservative}\underline{,} said to me: '\textbf{You} are the \textbf{daughter} of a \textbf{fascist} \textbf{pig}\underline{'}.
During a \textbf{tutorial} the following week, when another \textbf{historian} \textbf{seriously} \textbf{claimed} that I was 'an \textbf{enemy} of the people', I decided to do the same.
For four \textbf{euros}\underline{,} the \textbf{bear}\underline{ers} of the \textbf{Indonesia}\underline{n} \textbf{volcano} risk their lives and health by \textbf{carrying} 70 \textbf{kilo}\underline{s} of \textbf{sulphur} over the \textbf{steep}\underline{,} \textbf{rocky} \textbf{paths}\underline{.}
To do this, he must \textbf{climb} down to the \textbf{bottom} of his \textbf{cra}\underline{ter} every day, where the \textbf{sulphur}\underline{-}con\textbf{tain}\underline{ing} gas coming out of the \textbf{earth} \textbf{solid}\textbf{\underline{ifies}} in contact with the air.
"I will work here for another two years because I want to open a \textbf{shop} or learn Spanish or French," he \textbf{promises} in more than \textbf{acceptable} English.
While the \textbf{falling} \textbf{birth} rate has the well-\textbf{known} impact on a \textbf{nation} u2019s economic growth, tax \textbf{revenues}\underline{,} health costs and \textbf{immigration} policy, \textbf{Singapore} u2019s example also shows \textbf{unexpected} consequences.
\textbf{Men} and women use their \textbf{career}\underline{s}, the stress and the cost of property and education as reasons for not having children.
\textbf{According} to the \textbf{dictionary}\underline{,} this is the property of private or '\textbf{thos}\underline{e} areas of private life where you have a right to protection from any kind of \textbf{interference}\underline{'}.
\textbf{According} to the \textbf{expert}\underline{,} the most effective way to \textbf{teach} children and a\textbf{dol}\underline{es}\textbf{cent}\underline{s} what \textbf{privacy} is is to ask them questions that make them think.
At both international \textbf{meetings}\underline{,} the \textbf{Peru}\textbf{\underline{via}}\underline{n} authorities \textbf{stressed} that the information systems were available to \textbf{journalists}\underline{,} but they \textbf{greatly} \textbf{restricted} access to information.
The summit also \textbf{ended} with the joint commitment of \textbf{Chile} and \textbf{Peru} to adopt a \textbf{judgment} by the \textbf{Hague} Court which \textbf{resolve}\underline{s} a border \textbf{dispute} between the two countries.
Cor\textbf{rea} \textbf{assured} us that he did not \textbf{regret} this decision because he had not \textbf{betray}\underline{ed} his principles, but had \textbf{complied} with his 'de\textbf{ep} democratic values and views on human rights'.
They should not be paid the beer and motel, as \textbf{Governor} \textbf{Emil}\underline{io} Gonz xe1lez \textbf{answered} when he asked whether \textbf{conservative}\underline{s} would be \textbf{distributed} under his administration.
"Sex\textbf{ual}\underline{ity} does not look like this; it is best to bring the con\textbf{dom}\underline{s} \textbf{closer} to those who already \textbf{practise} \textbf{sexual} activity," he \textbf{summ}\underline{ed} it up.
I was part of the most successful \textbf{era} of the national team from \textbf{1988} to 1995, which at the beginning of the 1990s included up to 17 \textbf{teams} in one season.
In the years before "\textbf{Da}\textbf{\underline{lla}}\underline{s}" \textbf{Hag}\underline{man} became known on TV as a nice \textbf{guy} between \textbf{1965} and \textbf{1970} with the \textbf{sit}\underline{com} "A\textbf{chan}\underline{ting} \textbf{Jean}\textbf{\underline{nie}}\underline{"} of the TV company N\textbf{BC}\underline{.}
He also played two come\textbf{dies}\underline{,} which were only aired for a short time, such as The \textbf{Good} \textbf{Life} (N\textbf{BC}\underline{,} \textbf{1971}\underline{-}\textbf{72}\underline{)} and "\textbf{Her}\underline{e} We Go \textbf{Again}\underline{"} (A\textbf{BC}\underline{,} \textbf{1973}\underline{).}
"I have not \textbf{noticed} that this will be the most apocaly\textbf{ptic} \textbf{semester} ever," \textbf{Char}\underline{m} xe9 said this week to students at Rutgers-Camden University (\textbf{New} \textbf{Jersey}\underline{).}
"\textbf{We} do not take up \textbf{2012} so that we can always keep the option of \textbf{holding} the course again in case the world does not \textbf{sink}\underline{,}" said Re\textbf{stall}\underline{.}
In the \textbf{studies} carried out in the United States, there have been many \textbf{disrupt}\underline{ive} \textbf{factors} between control groups, so it is difficult to \textbf{interpret} these data and make clear \textbf{recommendations}\underline{.}
That is why I recommend the test from the age of 50 or 40 if you have a direct relative who has already had pro\textbf{state} \textbf{cancer}\underline{.}
In cooperation with the International \textbf{Society} for \textbf{Ur}\textbf{\underline{ology}}\underline{,} \textbf{Move}\textbf{\underline{mber}} has developed an instrument for \textbf{assessing} the \textbf{advantages} and \textbf{disadvantage}\underline{s} of the PSA test.
Indeed, it is \textbf{believed} that this Boson is involved in nothing less than the \textbf{mechanism} responsible for the mass of all \textbf{objects} in the \textbf{universe}\underline{.}
And \textbf{equally}\underline{,} not all p\textbf{article}\underline{s} \textbf{interact} with the \textbf{Hi}\textbf{\underline{gg}}\underline{s} field: those who do so have a mass, while others (\textbf{like} photon, by the way) do not have a mass.
When I \textbf{told} my onc\textbf{ologist} that I would stop the treatment, she \textbf{told} me that she \textbf{regret}\underline{s} that I would end the fight.
"\textbf{It} is \textbf{strange} how the system is dis\textbf{integr}\underline{ating} since \textbf{drastic} measures have been taken," \textbf{says} \textbf{Jacques} Du\textbf{ches}\underline{n}\textbf{eau}\underline{,} a \textbf{Quebec} Member and former head of the \textbf{Montreal} police.
We are in the process of \textbf{cleaning} up the \textbf{wound}\underline{,} but we need an \textbf{invest}\underline{ig}ative \textbf{unit} for \textbf{Montreal} only, as well as a \textbf{supervisor} to prevent a return to \textbf{dubious} \textbf{practices}\underline{.}
\textbf{Us}\underline{ing} the content of the file, it is also possible to ensure that the bitcoins traded are present in the public \textbf{accounts} \textbf{accounting} book \textbf{spread} throughout the network.
\textbf{Afghan} women have paid the price for the obs\textbf{cur}\underline{ant}ism of farmers overw\textbf{helm}\underline{ed} by Al \textbf{Qaeda}\underline{,} but their situation has not improved to this day.
\textbf{According} to the \textbf{Egyptian} \textbf{specialist} \textbf{Sophie} Pommier, this is \textbf{worrying} because 'the people who are asked to give an opinion have not been \textbf{elected} and have no democratic \textbf{legitimacy}\underline{.}
The \textbf{facts} of \textbf{bla}\underline{sp}\textbf{hem}\underline{y} are being \textbf{maintained} and \textbf{insult}\underline{s} are now \textbf{banned}\underline{,} which could have serious consequences for freedom of \textbf{expression}\underline{,} especially for the press.
Of course, this is not so much their \textbf{fault} as the \textbf{evil}\underline{:} few \textbf{Turk}\underline{men}, Uz\textbf{bek}\underline{s}, and Ta\textbf{ji}\textbf{\underline{ks}} can \textbf{afford} even proper \textbf{primary} education.
The \textbf{authors} of the open \textbf{letter} are \textbf{convinced} that \textbf{tight}\underline{en}ing up the law on private \textbf{arms} \textbf{owners} will not prevent criminals from using the black market.
"I can then \textbf{shoot} there, and if I am \textbf{convinced} that the \textbf{weapon} has a good \textbf{shot}\underline{,} we \textbf{negotiate} with each other," the \textbf{expert} \textbf{describes} the procedure.
However, only a few \textbf{hundred} people were there, far from all of them \textbf{employed} in the fast-\textbf{food} industry, which \textbf{employ}\underline{s} \textbf{tens} of thousands of people in New York.
- It is certainly not an all-\textbf{purpose} solution because it \textbf{raises} questions about \textbf{privacy}\underline{,} because you do not always want to inform everyone around about your actions and \textbf{intentions}\underline{.}
It would be nice to have a flexible \textbf{Ki}\underline{n}\textbf{ect}\underline{-}\textbf{like} system where we could play with different camera \textbf{angle}\underline{s} to see how this \textbf{helps} us to \textbf{determine} a position three-\textbf{dimensional}\underline{ly}.
At some point, however, it \textbf{becomes} a reality when the \textbf{Earth}\underline{'}s \textbf{inhabitants} break up in their spaceships into a \textbf{distant} \textbf{planet} that \textbf{becomes} the home of their \textbf{descendants} \textbf{born} in space.
\textbf{Road}\underline{s} in \textbf{Ol}\underline{o}mo\textbf{uc} \textbf{county} can be \textbf{accessed} without any \textbf{restrictions}\underline{,} but in   u20\textbf{47} \textbf{tern}\underline{ber}k \textbf{county} \textbf{drivers} have to drive \textbf{carefully} in \textbf{forest} \textbf{sections}\underline{,} as \textbf{tracks} here are still wet.
The \textbf{Tap} \textbf{Tap} is very popular at the moment, but if we go back a few years, what \textbf{motivated} you in 1998 to set up a \textbf{band}\underline{?}
We have \textbf{realised} that if you do something and you do not see it out\textbf{ward}\underline{,} your own performance does not exist in a way.
All three \textbf{venue}\underline{s} are \textbf{connected} to each other by a live \textbf{circuit} and there is a common \textbf{interpretation} of the anthem "\textbf{Welt}\textbf{\underline{unter}}\underline{gang} aus" of The \textbf{Tap} \textbf{Tap}\underline{.}
Ga\textbf{dom}\underline{ski}'s \textbf{globally} \textbf{recognized} contribution to the development of space was \textbf{recognized} by the fact that one of the \textbf{cra}\textbf{\underline{ters}} on the \textbf{earth}\textbf{\underline{ward}} side of the \textbf{moon} was \textbf{named} after him.
\textbf{Met}\underline{e}or\textbf{-2} had a starting \textbf{weight} of \textbf{380} \textbf{kg} and was able to carry a pay\textbf{load} of 10 \textbf{kg} to an \textbf{altitude} of about 60 km.
It is also \textbf{worth} noting that \textbf{Poland} \textbf{joined} the \textbf{COS}\textbf{\underline{PAR}} (\textbf{Com}\textbf{\underline{mitte}}\underline{e} for \textbf{Space} Research) in \textbf{1960}\underline{,} after which a national \textbf{COS}\textbf{\underline{PAR}} committee was established two years later.
It is \textbf{evident} that today's society, as in \textbf{ancient} times, is \textbf{founded} on the \textbf{reck}\underline{less} \textbf{preference} of one's own advantage, without \textbf{paying} attention to the interests of society as a whole.
From today u2019s point of view, the demise of these \textbf{regimes} in favour of \textbf{liberal} \textbf{democracies} can be \textbf{regarded} as a certain \textbf{pause}\underline{,} with the next round already \textbf{lo}\underline{om}ing.
The \textbf{weakness} of Argo is that it is too broad, due to the need to show too much action in too many places.
The \textbf{difficulty}\underline{,} however, is not just that we, as a people, are in the \textbf{pub} and in front of the \textbf{television}\underline{,} but that we are \textbf{closing} down \textbf{anyone} who \textbf{wants} to make a \textbf{difference}\underline{.}
You have taken up the \textbf{battle} for the \textbf{castle} with the thesis of the \textbf{substantive} and criminal \textbf{liability} of \textbf{politicians} and with \textbf{retro}\textbf{\underline{active}} \textbf{declarations} of \textbf{assets} of more than 20 million \textbf{crown}\underline{s}.
I have not thought about this yet, because I do not have time to review the past of any potential party member, nor do I have the money to do so.
The \textbf{MV}\underline{R}DV \textbf{architect}\underline{s} \textbf{prove} that the real \textbf{adventure}\underline{s} are not just in the head - with the example of \textbf{Sp}\textbf{\underline{ijk}}\underline{en}\textbf{isse} and the recently built bookberg - 2 \textbf{photos}\underline{.}
\textbf{According} to the market research company \textbf{CL}\underline{SA}, China is the third largest market for \textbf{luxury} products and the \textbf{fastest} growing market with a \textbf{volume} of EUR 15 billion per year.
This was \textbf{missed} because in Germany \textbf{sur}\textbf{\underline{name}}\underline{s} could not be protected, \textbf{says} \textbf{Han}\underline{no} Wen\textbf{tz}\underline{ler}, \textbf{Chairman} of the Management Board of \textbf{Freud}\textbf{\underline{enberg}} \textbf{Chemical} \textbf{Special}\underline{ities} in \textbf{Munich}\underline{.}
It is not enough to \textbf{rely} on international \textbf{trademark} rights. \textbf{Instead}\underline{,} \textbf{foreigners} should 'enter\textbf{tain} everything that is \textbf{somehow} \textbf{worth} \textbf{protecting} in China', as Wen\textbf{tz}\underline{ler} \textbf{says}\underline{.}
For 8,\textbf{73}\underline{3} \textbf{kilometres} from \textbf{Heidelberg}\underline{,} in the \textbf{northwest} of the \textbf{Kingdom} of Swaziland, there is the village of Esitjeni, which \textbf{depends} on the voice of the German \textbf{choir}\underline{.}
The well-\textbf{organis}\underline{ed} \textbf{Muslim} \textbf{Brot}\underline{her}\textbf{hood}\underline{,} for its part, \textbf{fle}\underline{w} to the regional \textbf{demonstration}\underline{,} for the \textbf{sake} of it, but not in Tahrir \textbf{Square}\underline{,} but after a mass \textbf{prayer} on the other bank of the \textbf{Nil}\underline{e} in front of \textbf{Cairo} University.
Rakfisk is a \textbf{salt}\underline{y} \textbf{trou}\underline{t} that is \textbf{fer}\underline{ment}ed in water for up to one year depending on how \textbf{st}\textbf{\underline{ink}}\underline{ing} your fish is.
If you avoid \textbf{bringing} Rakfisk \textbf{closer} to your nose, it is not bad - like Su\textbf{shi}\underline{,} who has a very long bus \textbf{ride} behind him.
Rakfisk is the product of a very different, much \textbf{poorer} \textbf{Norwegian} \textbf{ep}\textbf{\underline{och}}\underline{,} when there were no re\textbf{fr}\textbf{\underline{iger}}\underline{ation} facilities and fish was \textbf{drinks}\underline{ed} in air-t\textbf{ight} \textbf{salt} water casks in \textbf{autumn}\underline{.}
The military said that it had \textbf{assigned} this \textbf{restrictive} status - one level at risk of \textbf{suicide} - to him and to the protection of others.
On a recent trip to \textbf{Mexico} City, I had just crossed the \textbf{hall} and \textbf{arrived} at \textbf{passport} control when there was \textbf{confusion} in me.
\textbf{Yet} \textbf{Mexico} u2019s \textbf{greatest} challenge is in fact its relationship with more than 35 million \textbf{Mexican} \textbf{Americans} living in the United States.
Indeed, he \textbf{says}\underline{,} we now know that hu\textbf{mming} and \textbf{cri}\underline{pp}ling, often \textbf{interpreted} as a sign of \textbf{bo}\underline{re}\textbf{dom}\underline{,} can even fight them by \textbf{keeping} people \textbf{physically} more \textbf{attentive}\underline{.}
On the other hand, many \textbf{philosopher}\underline{s} and \textbf{authors} study the relationship between \textbf{bo}\underline{re}\textbf{dom} and \textbf{creativity}\underline{,} an opinion that \textbf{Professor} \textbf{Vo}\underline{da}\textbf{nov}\underline{ich} has been \textbf{studying} for more than two \textbf{decades}\underline{.}
"\textbf{Co}\textbf{\underline{lor}}\underline{ado} has a more \textbf{regulated} market, so the state is well \textbf{suited} for \textbf{guidance}\underline{,}" \textbf{says} \textbf{Brian} E. \textbf{Smith}\underline{,} \textbf{Spe}\underline{ak}er of the \textbf{Washington} State \textbf{Spirit}\textbf{\underline{ual}}\underline{s} \textbf{Authority}\underline{.}
At the moment, 119 people are being \textbf{tried} for \textbf{possession} of about 50 \textbf{gram}\underline{s} or less \textbf{mar}\underline{i}juana, even though many have been \textbf{accused} for other \textbf{offences}\underline{.}
"They have \textbf{spent} so much of their lives \textbf{prosecut}\underline{ing} people that they still cannot accept legalisation," he \textbf{believes}\underline{.}
\textbf{Prince}\underline{s}s D'\textbf{Ar}\textbf{\underline{enberg}} "because a \textbf{dress} is not only a \textbf{dress}\underline{,} but also the \textbf{associated} \textbf{memories}\underline{".}
The \textbf{advertising} company BBH, which made the video, maintains the hope that the \textbf{advertisement} will reach in a \textbf{funny} way to draw attention to the problem.
The rise in \textbf{immigration} is also seen as one of the reasons why \textbf{Singapore} u2019s \textbf{ruling} party achieved its \textbf{worst} \textbf{election} result since \textbf{independence} last year.
The \textbf{boy} is aware that it is wrong to \textbf{write} ob\textbf{sc}\underline{en}e \textbf{photos}\underline{,} \textbf{nu}\underline{de} \textbf{photos}\underline{,} crime or \textbf{insult}\underline{ing} or \textbf{violent} comments.
"\textbf{You} should also be \textbf{elect}\underline{ive} when it is most important for them to be popular, to have thousands of friends without \textbf{thinking} about the consequences," he \textbf{adds}\underline{.}
The little information \textbf{circulate}\underline{d} among \textbf{journalists} was received by the press \textbf{spoke}\underline{s}\textbf{person}\underline{s} of some of the governments of Unasur present at the meeting, but not by the \textbf{Peru}\textbf{\underline{via}}\underline{n} press \textbf{spoke}\underline{s}\textbf{person}\underline{.}
\textbf{Argentina}\underline{,} \textbf{Bolivia}\underline{,} \textbf{Colombia}\underline{,} \textbf{Ecuador}\underline{,} \textbf{Peru}\underline{,} \textbf{Brazil}\underline{,} \textbf{Uruguay}\underline{,} \textbf{Venezuela}\underline{,} \textbf{Chile}\underline{,} \textbf{Guy}\underline{ana}, \textbf{Sur}\underline{in}am and \textbf{Paraguay} are members of UN\textbf{AS}\textbf{\underline{UR}}\underline{,} even if the \textbf{latter} country is currently \textbf{excluded}\underline{.}
"\textbf{It} was as if a \textbf{bomb} \textbf{hit}\underline{,}" he \textbf{says} about the moment he received the \textbf{diagnosis} that the \textbf{doctor} \textbf{tried} to "de\textbf{fuse}\underline{"} without any \textbf{apparent} success.
In fact, the United Nations \textbf{Model} \textbf{Law} for the Un\textbf{ification} of International \textbf{Trade} \textbf{Law} was created for this purpose, with the American \textbf{Law} \textbf{Institute} being used as a mediator.
On the other hand, Vitro is to \textbf{blame} for his difficult situation as of 2008, in the context of the major economic crisis in the United States, which \textbf{struck} the country.
That the \textbf{guy}\underline{s} in Po\textbf{nce}\underline{,} for example, only play in their area and only meet \textbf{teams} from other \textbf{corner}\underline{s} of the island in the national playoffs.
He \textbf{tried} his \textbf{luck} on the \textbf{theater} \textbf{stages} in New York at the beginning of the \textbf{1950}\underline{s}, then served in the air forces in \textbf{England} from \textbf{1952} to \textbf{1956}\underline{.}
And he is not the only \textbf{professor} who offers this \textbf{semester}\underline{,} which should be the last in history, \textbf{courses} on the "end of the world".
In fact, the PSA test sometimes shows \textbf{fault}\underline{y} results, with \textbf{false} negative or \textbf{false} positive results that lead to \textbf{unnecessary} medical \textbf{interventions}\underline{.}
Although it was not the original purpose, this \textbf{sensor} now \textbf{serves} as a "\textbf{ey}\underline{e}" for all digital \textbf{cameras} worldwide and has won the \textbf{Nobel} \textbf{Prize} for \textbf{Physi}\textbf{\underline{cs}} in \textbf{2009.}
"\textbf{Si}\textbf{\underline{nce}} six months, three to five beds have always been \textbf{occupied} with \textbf{cancer} \textbf{patients} a\textbf{ged} less than \textbf{45}\underline{,}" \textbf{says} Dr. \textbf{Christian}\underline{e} Martel \textbf{worried}\underline{.}
The \textbf{Char}\textbf{\underline{bon}}\underline{n}\textbf{eau} Commission '\textbf{has} already brought down two \textbf{mayor}\underline{s}', he \textbf{adds}\underline{,} in the hope that it will manage 'to show the \textbf{ta}\textbf{\underline{ctic}}\underline{s} behind the individual'.
Even if the big \textbf{teams} such as \textbf{Marseille}\underline{s}, \textbf{Lyon} or \textbf{Bordeaux} fight for the title, I believe that we have the \textbf{stuff} to \textbf{win} it.
\textbf{Consider} \textbf{Manchester} City, a two-season \textbf{club} that has not managed to \textbf{qualify} for the \textbf{eight}\underline{h} final and has also made huge \textbf{expenditure}\underline{!}
We have \textbf{learned} our \textbf{lesson} from what has \textbf{happened} in Ukraine, and today we must show \textbf{exemplary} \textbf{behaviour}\underline{.}
Moreover, as so often in these technologies, a political \textbf{vision} is \textbf{tangible}\underline{:} the \textbf{conviction} that the current \textbf{monetary} system, \textbf{shaped} by bank \textbf{monopolies}\underline{,} \textbf{leads} to financial \textbf{crises}\underline{.}
\textbf{Recently}\underline{,} Adi \textbf{Sha}\textbf{\underline{mir}} and \textbf{Dor}\underline{it} Ron of the Weizmann \textbf{Institute} in Israel \textbf{analysed} the \textbf{accounting} book and \textbf{showed} that almost \textbf{80\%} of the bitcoins are not in \textbf{circulation}\underline{.}
For almost two years now, \textbf{Egypt} has been \textbf{bas}\underline{ing} itself on a \textbf{provisional} text that has been \textbf{amended} several times, which \textbf{weaken}\underline{s} institutional stability and \textbf{leads} to legal \textbf{confusion}\underline{.}
In the \textbf{north} of the country, between \textbf{1600} and 2040 metres high, there is the famous ski resort of Hermon, which \textbf{attract}\underline{s} \textbf{countless} \textbf{tourists} during the winter months.
In \textbf{Ak}\underline{ko} you can visit the Museum in the Bad Al \textbf{Bas}\underline{ha}, which \textbf{houses} several rooms of old \textbf{Turkish} baths with \textbf{sculpture}\underline{s} from then visitors and bath \textbf{attend}\textbf{\underline{ants}}\underline{.}
For there is not even money in their families to \textbf{feed} the children, let alone to buy \textbf{decent} \textbf{clothes}\underline{,} \textbf{shoes} and school materials.
Of course, the new \textbf{owners} did not get it for free: every \textbf{migrant} who \textbf{hoped} to avoid the \textbf{tests} paid 7 000 \textbf{rub}\underline{les} for the document.
The police want to ban the \textbf{wearing} of non-de\textbf{ath} \textbf{weapons} in public and \textbf{raise} the age for \textbf{possession} of \textbf{fire}\textbf{\underline{arm}}\underline{s} from 18 to 21 years.
\textbf{According} to data from the \textbf{researchers}\underline{,} 17\% of \textbf{weapons} come from conflict \textbf{zones}\underline{,} 14\% derive from thefts in \textbf{weapons} production and \textbf{5\%} from illegal \textbf{excavat}\textbf{\underline{ions}}\underline{.}
"In order to get a \textbf{weapon}\underline{,} I need a \textbf{friend} who has \textbf{contacts}\underline{,}" \textbf{says} the sales \textbf{advisor}\underline{.}
First, Google presented a working model at its annual conference in the summer, and in November it became known that Microsoft had also applied for a \textbf{patent}\underline{.}
I was friendly with the new \textbf{generation} \textbf{painter}\underline{s}, that is to say with the representatives of the "\textbf{Ga}\textbf{\underline{zone}}\underline{v}schina"; from this came "P\textbf{usch}\textbf{\underline{kin}}\underline{s}\textbf{kaya} 10" and then it was over.
In \textbf{1988}\underline{,} the second \textbf{woman} in space, S\textbf{vet}\textbf{\underline{lan}}\underline{a} Sa\textbf{wi}\underline{z}kaja, who was in orbit \textbf{twice} and even carried out work outside the space \textbf{vehicle}\underline{,} left a \textbf{son}\underline{.}
This \textbf{confirm}\underline{s} that it is not enough to draw up new and more \textbf{precise} rules time and time again, and we must also look at the actual application of the law.
Economics means \textbf{buying} something at a \textbf{reasonable} price (\textbf{which} is not always the \textbf{lowest} price) and \textbf{excluding} illegal \textbf{enrichment} or even criminal activity.
Ice \textbf{smooth}\underline{ing} can be achieved especially on second and third class \textbf{roads} in \textbf{Lan}  u20\textbf{47} \textbf{kro}\underline{un},   u20\textbf{47} \textbf{st} xed \textbf{nad} Orlic xed, \textbf{Poli}  u20\textbf{47} \textbf{ka}\underline{,} S\textbf{vita}\textbf{\underline{vy}} and V\textbf{ys}\underline{ok} xe9 M  u20\textbf{47} to.
On the   u20\textbf{47} erveno\textbf{hor}\underline{sk} xe9 sedlo pass, \textbf{drivers} in the direction of Jesen xedk have to \textbf{count} on \textbf{snow} jams," said a member of the   u20\textbf{47} umperk road management team to the   u20\textbf{47} TK \textbf{agency} today.
\textbf{According} to meteor\textbf{ologist}\underline{s} there were ideal conditions for this during the night - \textbf{rain} and \textbf{melting} \textbf{snow} during the day, \textbf{cloud}\underline{less} \textbf{sky} and \textbf{fro}\underline{st} at night.
The \textbf{Tap} \textbf{Tap} has also \textbf{recorded} the so-called anthem against the end of the world with the title "\textbf{Welt}\textbf{\underline{unter}}\underline{gang} f xe4llt aus".
In May we will \textbf{perform} for the first time at the \textbf{Prague} \textbf{Spring}\underline{,} and for this \textbf{concert} we are also \textbf{preparing} an interesting programme with interesting guests.
Since \textbf{1956}\underline{,} P\textbf{TA} has been \textbf{instrumental} in the development of the extremely successful meteor\textbf{ological} \textbf{missile} (R\textbf{aki}\textbf{\underline{eta}} \textbf{Met}\underline{e}or\textbf{ologic}\underline{z}na), the first \textbf{Polish} \textbf{rocket} for scientific research.
In Germany, there have been public food le\textbf{vie}\underline{s} for a number of years now for poor people who are no longer able to \textbf{feed} themselves through their own work.
Then one must ask \textbf{oneself} whether private capital does not influence or even direct \textbf{politics} and therefore the entire state in its own selfish sense.
We must therefore find the cause of the rise of fa\textbf{sc}\underline{ism} and \textbf{communism} in the \textbf{ruthless} \textbf{liberalisation} of the \textbf{economies} of the 19th and 20th \textbf{centuries}\underline{.}
It was a serious \textbf{blow} to the \textbf{reputation} of the United States, and the \textbf{subsequent} \textbf{fi}\underline{as}co in the \textbf{violent} \textbf{attempt} to \textbf{lib}\underline{er}ate \textbf{hostage}\underline{s} only made matters \textbf{worse}\underline{.}
I know that I will not achieve anything on my own; that is why I have \textbf{spoken} to a number of well-\textbf{known} \textbf{figures} about whether they do not want to stand for the \textbf{Senat}\underline{e} as well.
"I find the building \textbf{funny}\underline{,} it \textbf{looks} \textbf{fut}\underline{ur}\textbf{istic}\underline{,} and at last there is something interesting to see," \textbf{says} Lis\textbf{ette} Verhaig, a passer-by on the side of the road.
" \textbf{Normal}\underline{ly}, the \textbf{books}\underline{h}\textbf{elf}\underline{s} are \textbf{standing} along the fa  u20\textbf{47} ade, and in the \textbf{middle} there is a large \textbf{dark} room, which is \textbf{mostly} \textbf{uncomfortable} and im\textbf{personal}\underline{,}" \textbf{says} \textbf{Win}\underline{y} Maas.
\textbf{Deutsche} \textbf{Welle}\underline{:} \textbf{Earl}\underline{ier} this week, Germany \textbf{signal}\underline{led} that it would vote against the request for \textbf{Palestinian} \textbf{observe}\underline{r} status at the United Nations.
The United States' influence in European \textbf{politics} is \textbf{constantly} \textbf{diminish}\underline{ing}, but at the moment the EU is not \textbf{filling} this \textbf{vacuum}\underline{,} so who else is there?
On September 14, \textbf{2010,} a Chinese company had the \textbf{Ze}\textbf{\underline{gna}} \textbf{DF} \textbf{Pu}\underline{ma} \textbf{trademark} protected there, an art name that was also used by the Ermene\textbf{gil}\underline{do} \textbf{Ze}\textbf{\underline{gna}} \textbf{fashion} house.
In fact, if \textbf{Freud}\textbf{\underline{enberg}} is subject to \textbf{license} \textbf{fees} for his own name in the last act of his brand \textbf{drama}\underline{,} then one would probably have to pay the other side \textbf{license} \textbf{fees} for his own name, \textbf{explains} Wen\textbf{tz}\underline{ler}.
This is where the Ca\textbf{uc}\textbf{\underline{asia}}\underline{n} \textbf{Tal}\textbf{\underline{yan}} people live, of which not much is known, \textbf{except} that they speak \textbf{perfectly} \textbf{Persian} and Asean and are very long-\textbf{lasting}\underline{.}
"\textbf{Ba}\underline{ku} became famous in May with the Euro\textbf{vision} \textbf{song} \textbf{festival} - and next year we will have a \textbf{festival} of the \textbf{oldest} people in the world," \textbf{says} Fatu\textbf{lay}\textbf{\underline{eva}}\underline{.}
It is a matter of \textbf{interpretation}\underline{,} as much in the draft that \textbf{Mor}\underline{si} has for his \textbf{signature} and will, in his words, '\textbf{very} soon' be presented to the \textbf{Egyptian}\underline{s} for a \textbf{referendum}\underline{.}
The \textbf{48}\underline{-}\textbf{year}\underline{-}\textbf{old} human rights \textbf{lawyer} and \textbf{president} of the \textbf{Egyptian} Human Rights Organisation (EO\textbf{HR}\underline{)} \textbf{defended} the \textbf{Muslim} \textbf{Brot}\underline{her}\textbf{hood} when they were in \textbf{prison} or on \textbf{trial} under \textbf{Mubarak}\underline{.}
Just a \textbf{generation} ago, thousands of \textbf{Norwegian}\underline{s} were \textbf{forced} to leave their country in search of work and \textbf{migrate}\underline{d} mainly to the US.
There is still hatred to call a spade a spade a spade - that \textbf{racist} right-\textbf{wing} extremist who \textbf{shot} \textbf{77} men, women and children last year.
\textbf{Earl}\underline{ier} this year, the military was \textbf{deployed} to combat \textbf{drug} gangs operating in \textbf{quarter}\underline{s}, and violence against women is a particularly \textbf{acute} problem.
Manning \textbf{told} the civil \textbf{servant} that he could have used the \textbf{union} of his \textbf{trouser}\underline{s} or f\textbf{lip} \textbf{flo}\underline{ps} to injure \textbf{himself} but not.
The \textbf{defence} has \textbf{indicated} that Manning will be \textbf{guilty} of lesser \textbf{offences}\underline{,} while other \textbf{charges} that are considered too \textbf{extreme} are to be challenged.
The \textbf{Pen}\underline{t}\textbf{agon} maintains its position that Manning has been held in accordance with the provisions that apply to all \textbf{prisoners} held under the highest security provisions in \textbf{Qua}\underline{n}\textbf{tico}\underline{.}
And then we would not now be \textbf{caught} behind the \textbf{silk} \textbf{curtain} - with a pleasant life in the United States, but \textbf{somehow} lost.
The \textbf{Arab} \textbf{Spring} has created a new, \textbf{uncertain} situation, and, whether they like it or not, \textbf{Palestinians} and \textbf{Israelis} have become part of that \textbf{turmoil}\underline{.}
"The government should simply have \textbf{banned} \textbf{cigarette}\underline{s} completely - then we would have said to ourselves \textbf{ok}\underline{ay}, that's it, we're going to close," he \textbf{adds}\underline{,} \textbf{vis}\textbf{\underline{ib}}\underline{ly} in\textbf{dig}\underline{n}antly.
And because most of us today are almost \textbf{constantly} staring on one or other screens, we no longer benefit from \textbf{bo}\underline{re}\textbf{dom}\underline{.}
The key experience of \textbf{bo}\underline{re}\textbf{dom}\underline{,} he \textbf{says}\underline{,} is a "\textbf{dis}\textbf{\underline{tur}}\textbf{\underline{bing}} the attention process, \textbf{coupled} with a bad \textbf{mood} and a \textbf{feeling} that time is only \textbf{passing} \textbf{slowly}\underline{".}
However, he is certain that "\textbf{yo}\underline{ung} people are \textbf{regarded} as particularly \textbf{bo}\underline{ring}," mainly because children and \textbf{teenagers} have no great influence on their daily life.
"\textbf{With} \textbf{bo}\underline{re}\textbf{dom}\underline{,} the \textbf{brain} \textbf{wants} to tell you that you should do something different," \textbf{says} Gary \textbf{Marcus}\underline{,} \textbf{Professor} of \textbf{Psycho}\textbf{\underline{logy}} at New York University.
\textbf{According} to O\textbf{roz}\underline{co}, on a September day he and some friends were \textbf{travelling} by car in \textbf{Lama}\underline{r} near the \textbf{Kan}\underline{s}as border when they were \textbf{stopped}\underline{.}
The only \textbf{tut}\underline{or} who \textbf{openly} \textbf{recognized} Tory was \textbf{Norman} \textbf{Stone}\underline{,} \textbf{professor} of \textbf{contemporary} history, who was in my \textbf{college}\underline{.}
He was hated not only for being a \textbf{conservative}\underline{,} but also for \textbf{advising} Thatcher on foreign policy and writing \textbf{speeches} for her.
This \textbf{exhibition} is the conclusion of a \textbf{story} whose only \textbf{protagonist} is "il sign\textbf{ore}\underline{"} \textbf{Gar}\textbf{\underline{ava}}\underline{ni}, but which could not have been written without his \textbf{distinguished} client\textbf{ele}\underline{.}
"I \textbf{prefer} him to everyone else because of his great love for women and because he \textbf{emphasize}\underline{s} our \textbf{beauty}\underline{,}" \textbf{adds} the ex-du\textbf{ches}\underline{s} of F\textbf{eria}\underline{.}
They know that every step can cost their lives, as \textbf{happened} to a French tourist who \textbf{crash}\underline{ed} years ago on the \textbf{steep} \textbf{slopes} of Kawah Ijen.
For each \textbf{route} it takes three hours, after which it has been completely \textbf{accomplished}\underline{,} but at the end of the day it has 13\textbf{8,000} rupees (11,5 \textbf{euros}\underline{).}
But what \textbf{looks} like a \textbf{mis}\underline{er}able \textbf{reward} for such an in\textbf{human} effort is three times what it would \textbf{earn} from field work.
\textbf{Def}\underline{y}ing the \textbf{shadow}\underline{s}, it rises into the \textbf{cra}\underline{ter} in light of a small fore\textbf{head} lamp on its \textbf{helmet}\underline{,} which it \textbf{bought} from its own money.
However, there is concern that they can promote the way of life of the \textbf{isolated} and that they deter construction companies from building large \textbf{housing} for families.
If they understand all \textbf{sections}\underline{,} they have \textbf{solid} \textbf{foundations} to talk to their children about the importance of opening a user account on the Internet.
The President of \textbf{Ecuador}\underline{,} \textbf{Raf}\underline{a}el Cor\textbf{rea}\underline{,} today \textbf{confirmed} that the creation of common \textbf{citizenship} is an objective, with '\textbf{South} America \textbf{genuinely} \textbf{learning} something from Europe'.
I have never been \textbf{personally} interested in power, but under such \textbf{unfair} circumstances as in \textbf{Ecuador}\underline{,} this \textbf{socio}\underline{-}\textbf{economic} poverty can only be \textbf{corrected} by political power.
The request made by \textbf{Carlos} D xed\textbf{az} \textbf{Ch} xe1vez \textbf{Mor}\underline{ine}au has now brought criminal \textbf{proceedings} against the National Bank and \textbf{Securities} Commission, which is \textbf{accused} of \textbf{obstruct}\underline{ing} the \textbf{judiciary}\underline{.}
He was \textbf{granted} the \textbf{Va}\textbf{\underline{quer}}\underline{os} \textbf{Championship} with Ga\textbf{usse}\underline{,} but from a distance, because he was already at the top of the \textbf{association} in \textbf{1988}\underline{.}
\textbf{Born} in \textbf{Fort} Worth, \textbf{Texas}\underline{,} he was the \textbf{son} of the \textbf{actress} and \textbf{singer} \textbf{Mary} \textbf{Martin}\underline{,} who played \textbf{classical} works such as "\textbf{South} \textbf{Pacific}\underline{"} and "\textbf{Peter} \textbf{Pan}\underline{".}
"I have not written anything that I thought could \textbf{harm} or \textbf{affect} \textbf{anyone} \textbf{wise}\underline{ly}," said the \textbf{Associate}\underline{d} \textbf{Press} at the time.
I would like to give them some comfort, such as 'no \textbf{fear}\underline{,} it is a bit in\textbf{conv}\underline{en}\textbf{ient} the first time, but it will be good for you'.
In this sense, since \textbf{2009,} the majority of American governments have \textbf{announced} new laws that make the \textbf{registration} or \textbf{ballot} procedure more difficult.
This \textbf{phenomenon} became more important after the November 2010 elections, with 6\textbf{75} new \textbf{Republican} representatives in 26 countries.
\textbf{Another} study, this time from Europe, \textbf{concluded} that there is a \textbf{difference} in the \textbf{mortality} of \textbf{patients} with and without early \textbf{detection}\underline{.}
D\textbf{espite} progress in research, \textbf{adopting} a \textbf{healthy} \textbf{lifestyle} remains the best way to reduce the risk of \textbf{falling} \textbf{ill}\underline{.}
We know without a \textbf{shadow} of doubt that we have a real new p\textbf{article} and that it is very similar to the \textbf{Hi}\textbf{\underline{gg}}\underline{s}-\textbf{Bo}\underline{son} \textbf{predicted} by the standard model.
By the way: in the early \textbf{1960}\underline{s}, the \textbf{pioneer}\underline{s} of the \textbf{laser} in the \textbf{Bell} \textbf{laboratories} did not \textbf{assume} that their work would \textbf{trigger} such a \textbf{revolution}\underline{.}
Of course, this does not mean that LHC u2019s activities will \textbf{necessarily} change our lives, but it does mean that you really can never know...
I hope that in May we will be the s\textbf{mil}\underline{ing} \textbf{winner} and tell us that, despite all the \textbf{difficulties}\underline{,} we have finally won it.
Moreover, in its report, the \textbf{ECB} \textbf{intends} to re-\textbf{eval}\underline{u}ate the various \textbf{risks} that are now \textbf{regarded} as high if this currency were to be successful.
\textbf{Jobs} will have to be made available to these young people who do not want to return to the obs\textbf{cur}\underline{ant}ism of the former parties or to the \textbf{corruption} of certain leaders.
Former commanders of the anti-S\textbf{ovi}\underline{et} \textbf{struggle} are already trying to \textbf{restore} the \textbf{provincial} \textbf{militia}\underline{s} that will \textbf{escape} the power of the central government.
\textbf{Min}\underline{ing} is not possible without energy to process \textbf{iron} or \textbf{copper} ore on site or without means of transport for export over the \textbf{mountains}\underline{.}
One day it will also be necessary for Afghanistan and Pakistan, on which \textbf{imports} and \textbf{exports} are \textbf{largely} \textbf{dependent}\underline{,} to \textbf{restore} normal relations.
\textbf{Liberal} \textbf{fears} are also \textbf{fuel}\underline{led} by the fact that the next re\textbf{ctor} of this \textbf{university} should be much less \textbf{moderate} than the current one.
It \textbf{admit}\underline{s}, however, that there may be ambi\textbf{gu}\underline{ity} with regard to Article \textbf{220}\underline{,} as the terms used are \textbf{borrow}\underline{ed} from \textbf{religious} \textbf{vocabulary}\underline{.}
As early as the day on which the law \textbf{entered} into force, it became clear that it was not only \textbf{immigrants}\underline{'} \textbf{registration} documents that could be f\textbf{als}\textbf{\underline{ified}}\underline{.}
For the moment, the authorities can only \textbf{promise} guest workers who fall through the test for the first time that they will have time for a basic language course.
An open \textbf{letter} has been published on the Internet, the \textbf{authors} of which - representatives of various \textbf{arms} \textbf{associations} - call on the authorities to \textbf{refrain} from 's\textbf{ense}\underline{less} \textbf{tight}\underline{en}ings'.
The \textbf{experts} \textbf{analyze}\underline{d} reports by the \textbf{Ministry} of the \textbf{Interior} and the \textbf{Federal} Service for State \textbf{Stat}\textbf{\underline{istic}}\underline{s}, criminal \textbf{literature} and \textbf{publicly} \textbf{accessible} data on \textbf{weapons} \textbf{portal}\underline{s}.
"As a response he receives a photo and a \textbf{description} of the \textbf{hide}\textbf{\underline{away}} of the \textbf{weapon}\underline{,}" reports the press \textbf{spoke}\underline{s}man of the non-\textbf{profit} \textbf{organization} "Pravo na ory\textbf{zh}\underline{ie}" Dmitr\textbf{ij} \textbf{Ki}\underline{s}\textbf{lov}\underline{.}
For example, the \textbf{Xbox} \textbf{console} and the \textbf{Ki}\underline{n}\textbf{ect} \textbf{sensors} are a step forward and today no more \textbf{Xbox} is \textbf{sold} without \textbf{Ki}\underline{n}\textbf{ect} because everyone is interested in motion control.
This is what makes the work on \textbf{virtual} reality so \textbf{attractive} to a researcher: on many issues we are only just starting.
Then the time of the old free but not \textbf{officially} \textbf{recognised} \textbf{painter}\underline{s} came to an end, and new and free \textbf{painter}\underline{s} like me were \textbf{incomprehensible}\underline{.}
It is not easy to work in new times according to old rules; I am a man of \textbf{truth}\underline{,} \textbf{honest}\underline{y} and culture of the last century.
In my \textbf{youth} I have \textbf{painted} such images, which even \textbf{hang}\underline{ed} in a \textbf{row} with the works of \textbf{Falk} and La\textbf{rio}\textbf{\underline{nov}} by a \textbf{collect}\underline{or}.
The real T\textbf{sar} was different, because Ts\textbf{ars} may not understand much about culture, but they \textbf{understood} that proper \textbf{experts} were needed.
"The more \textbf{dangerous} it is even on \textbf{flights} in orbit", \textbf{conclude}\underline{s} Kosmon\textbf{aut} \textbf{Wal}\underline{er}i \textbf{Pol}\underline{ja}\textbf{kov}\underline{,} hero of the \textbf{Soviet} Union and hero of the Russian \textbf{Federation}\underline{.}
He can say: '\textbf{We} are \textbf{changing} the law and \textbf{allowing} the matter', but he cannot say that we are \textbf{acting} as if nothing were.
The \textbf{procurement} law \textbf{lay}\underline{s} down relatively \textbf{strict} rules on the \textbf{formal} \textbf{execution} of certain \textbf{transactions} - and that is right to protect public competition.
By \textbf{travelling} \textbf{abroad}\underline{,} you have a \textbf{comparison} of what is \textbf{happening} in the individual countries with \textbf{accessibility}\underline{,} how people are being \textbf{treated} with \textbf{disabled} people and so on.
At that time I started as a care\textbf{take}\underline{r} at the Jedli  u20\textbf{47} \textbf{ka} \textbf{Institute}\underline{,} where I met many young people who were interested in getting involved with something \textbf{intensive}\underline{.}
I always say that if people with \textbf{disabilities} are successful, it is not just a step forward for them, it is a step forward for society as a whole.
The result is a \textbf{desperate} situation in the area of \textbf{corruption}\underline{,} \textbf{mutual} \textbf{preference}\underline{,} legislation in which \textbf{virtually} everything is criminal but nothing is criminal.
In Germany, the situation is that a \textbf{Ministry} of State is in\textbf{struct}\underline{ing} private law companies that are closely intert\textbf{win}\underline{ed} with industry to draft legislation because of a lack of \textbf{finance}\underline{.}
All violence then no longer comes from the people, as the Western \textbf{constitution}\underline{s} pro\textbf{claim}\underline{,} but from strong financial groups that \textbf{prefer} their own interests.
The \textbf{Bal}\textbf{\underline{four}} \textbf{Declaration}\underline{,} which has already been mentioned, created the conditions for mass \textbf{immigration} of \textbf{Jews} into \textbf{Palestine}\underline{;} there were first \textbf{clash}\underline{es} with the local \textbf{Arab} population.
At the same time, it was \textbf{unable} to secure the release of the \textbf{hostage}\underline{s} in Iran, where the \textbf{revolution} \textbf{resulted} in the establishment of a theo\textbf{cra}\underline{tic} regime.
In order to make the camo\textbf{uf}\underline{lage} \textbf{credible}\underline{,} \textbf{articles} on this film project were published in \textbf{specialist} \textbf{magazine}\underline{s}, press \textbf{conferences} were held and the \textbf{fi}\textbf{\underline{ct}}\underline{it}\textbf{ious} production company had a real office.
Then there are the \textbf{scenes} from the \textbf{CIA} \textbf{headquarters} and other institutions - men in \textbf{suit}\underline{s} at the meeting table, on the official \textbf{hall}\underline{s}, on the telephone...
My advantage is that I can take away from any party what is best for our country without drawers and party \textbf{dogma}\underline{s}.
Or do you think that, if you only talk to people long enough, you will be able, for example, to \textbf{impose} material and criminal \textbf{liability}\underline{?}
I always try to \textbf{judge} things for \textbf{myself}\underline{;} and if it does not work, I will return to the private sector in six years' time.
But I couldn u2019t live on the senator u2019s \textbf{salary} alone; for example, I couldn u2019t \textbf{finance} my \textbf{son} u2019s English school, which costs 3\textbf{0,000} a month.
\textbf{Has} Germany \textbf{damaged} its relations with the US by \textbf{abstain}\underline{ing} on important decisions, such as the vote on \textbf{Palestine}\underline{?}
It would, of course, be a little \textbf{easier} for the Germans if there were a \textbf{coherent} and \textbf{unified} European policy, which is not the case at present.
This is a record, and it means that China is for the tenth time in succession leading the list of new applications around the world.
A year later, however, the \textbf{choir} \textbf{founded} the \textbf{association} "Voices for Africa", which since then has been dealing almost professionally with the \textbf{AIDS} \textbf{orphan}\underline{s} in Esitjeni.
\textbf{According} to the \textbf{Robert} \textbf{Koch} \textbf{Institute}\underline{,} the number of \textbf{Sy}\textbf{\underline{phil}}\underline{is} \textbf{infection}\underline{s} has more than doubled from 16\textbf{97} in 2001 to \textbf{36}\textbf{\underline{98}} in \textbf{2011}\underline{.}
Although it is \textbf{closest} to the sun, there is also \textbf{frozen} water there, as \textbf{indicated} by three \textbf{studies} published on \textbf{Thursday} in the \textbf{magazine} "Science".
No one related the \textbf{discovery} of \textbf{ice} but to the \textbf{existence} of life on the \textbf{planet}\underline{,} said the \textbf{chief} \textbf{scientist} of the \textbf{Messenger} \textbf{probe}\underline{,} Sean \textbf{Solo}\underline{mon}.
This star-forming region - called W5 by \textbf{scientists} un\textbf{roman}\underline{tic} - has been \textbf{discovered} by the \textbf{telescope} \textbf{Spitze}\underline{r} in the star image C\textbf{assi}\underline{op}eia, at a distance of 6\textbf{500} light years.
The man had been \textbf{married} three times and had 23 children.
\textbf{Mir}\underline{za}y\textbf{eva} u2019s white \textbf{teeth} are perfect in Re\textbf{ih} and \textbf{Gli}\underline{ed}, under her \textbf{heads}\underline{car}f she \textbf{hide}\underline{s} long, \textbf{dark}\underline{-}\textbf{blo}\textbf{\underline{od}}\underline{ed} \textbf{pot}\underline{s} that her \textbf{son} \textbf{proud}\underline{ly} \textbf{reveals} before us.
\textbf{230} Manat (a\textbf{round} the same amount in \textbf{euros}\underline{),} receives \textbf{Mir}\underline{za}y\textbf{eva} a \textbf{monthly} \textbf{pension}\underline{,} for local circumstances an amount from which you can live well.
In fact, the 234 \textbf{articles} that were \textbf{pushed} through by the \textbf{Islamic}\underline{-}d\textbf{ominated} 100-\textbf{member} \textbf{constitution}\underline{-}\textbf{making} \textbf{assembly} in a 15-\textbf{hour} par\textbf{ody} at night are sometimes \textbf{worrying}\underline{.}
Saeda feels left alone, including by the international community, which sees the \textbf{ideological} \textbf{struggle} for direction on the \textbf{Nil}\underline{e} with a \textbf{mixture} of \textbf{curiosity} and \textbf{tension}\underline{.}
\textbf{Norway} has been very \textbf{careful} with its oil \textbf{wealth} - a large part of its industry income is being \textbf{invested} in a special \textbf{fund} for the benefit of future \textbf{generations}\underline{.}
When, in the years leading up to the global economic crisis, everyone was \textbf{throw}\underline{ing} around with money that they did not have, \textbf{Norway} \textbf{kept} its \textbf{pur}\underline{se} \textbf{firmly} closed.
"\textbf{My} government is \textbf{strongly} committed to \textbf{reducing} violence," \textbf{Pen}\underline{a} \textbf{Nie}\underline{to} said earlier this week in the O\textbf{val} Office to US President \textbf{Barack} \textbf{Obama}\underline{.}
\textbf{Congress}\underline{man} \textbf{Ol}\underline{ver}a \textbf{admit}\underline{s} that after 12 years outside the Presidential \textbf{Palace} of \textbf{Los} \textbf{Pin}\underline{os}, the party has high \textbf{expectations} of Enr\textbf{ique} \textbf{Pen}\underline{a} \textbf{Nie}\underline{to}.
Irinea \textbf{Bu}\underline{en}\textbf{dia} \textbf{struggle}\underline{s} with \textbf{tear}\underline{s} in a \textbf{concrete} construction, \textbf{typical} of the decayed \textbf{quarter}\underline{,} when she shows me \textbf{photos} of her late \textbf{daughter} \textbf{Maria}\underline{na} Luna.
Hosni \textbf{Mubarak}\underline{,} the \textbf{secular} des\textbf{pot} that \textbf{ruled} \textbf{Egypt} for 30 years until his fall in \textbf{2011}\underline{,} had little time left for \textbf{Hamas}\underline{.}
On a \textbf{diplomatic} level, the United States remains \textbf{ste}\underline{ad}\textbf{fast} in its position, and many European countries have \textbf{blame}\underline{d} \textbf{Hamas} for the latest \textbf{escalation}\underline{s} of violence.
\textbf{Net}\underline{an}yahu is doing well, and his Likud party, under A\textbf{vig}\textbf{\underline{dor}} \textbf{Liebe}\underline{r}man, has allied itself with an even more combative group in the run-up to the 22 January elections.
On social media such as \textbf{YouTube}\underline{,} \textbf{Twitter} and \textbf{Facebook}\underline{,} Freeman has seen an increase in brand experience reports written by "\textbf{normal} people" .
\textbf{James} \textbf{Yu}\underline{,} the \textbf{tobacco} trade's "King of the \textbf{Pack}\underline{"} in \textbf{downtown} \textbf{Sydney}\underline{,} \textbf{says} that standard \textbf{packaging} has made it difficult to \textbf{fill} up his she\textbf{lves}\underline{.}
This \textbf{Thanks}\underline{g}\textbf{iving} I \textbf{spent} \textbf{unexpected}\underline{ly} five hours at the airport when our \textbf{plane} \textbf{failed} because of \textbf{mechanical} problems and we had to \textbf{wait} for another \textbf{aircraft}\underline{.}
"\textbf{Studie}\underline{n} haben gezeigt, dass Kinder, die \textbf{herum}\underline{ha}\textbf{mpel}\underline{n} d xfcr\textbf{fen}\underline{,} mehr \textbf{lernen} und mehr Informationen \textbf{behalten} als die, die zum \textbf{Still}\textbf{\underline{sitz}}\underline{en} \textbf{gezwungen} werden", so \textbf{Professor} Fenske.
\textbf{Chief} O\textbf{ates} added that the police would continue to \textbf{impose} \textbf{urban} regulations on \textbf{mar}\underline{i}juana \textbf{growers} and that \textbf{drug} \textbf{traffickers} would continue to be \textbf{prosecut}\underline{ed}.
\textbf{Valentin}\underline{o} shows these personal \textbf{memories} as \textbf{troph}\underline{ies} of his social rise from the \textbf{modest} \textbf{fashion}\textbf{\underline{maker}} in the city of \textbf{Vo}\textbf{\underline{gh}}\textbf{\underline{era}} in \textbf{northern} Italy to the i\textbf{dol} of the international \textbf{jet} set.
"At least they do not appear on your beautiful \textbf{carpet}\underline{,} as some beautiful \textbf{celebrities} from \textbf{pop} music do," \textbf{says} Bar\textbf{oni}\underline{n} Fi\textbf{ona} \textbf{Thyssen}\underline{-}Borne\textbf{mis}\underline{za}.
"\textbf{All} \textbf{invite}\underline{es} \textbf{felt} important and \textbf{loved}\underline{,}" remembers the "\textbf{Top} \textbf{Model}\underline{",} which started her \textbf{career} at the week of \textbf{Haut}\underline{e} \textbf{Cou}\underline{ture} in Paris in 1995.
"\textbf{Val}\underline{en}\textbf{tino} does not depend on \textbf{fashion}\underline{,} his ob\textbf{session} is timeless," \textbf{explains} this Italian a\textbf{risto}\textbf{\underline{cra}}\underline{t} who lives between \textbf{Par} xeds, New York and \textbf{Bueno}\underline{s} \textbf{Aires}\underline{.}
The \textbf{grand} finale of the \textbf{exhibition} in Somer\textbf{set} House is \textbf{Marie}\underline{-}\textbf{Cha}\underline{n}tal \textbf{Mill}\underline{er}'s \textbf{wedding} \textbf{dress} for her \textbf{wedding} with \textbf{Pablo} de \textbf{Gre}\underline{cia} in 1995.
The \textbf{Singapore}\textbf{\underline{ans}} are b\textbf{lam}\underline{ing} them for not having children on \textbf{career}\underline{s}, stress and the cost of property and child-\textbf{rea}\underline{ring}.
\textbf{Their} \textbf{creative} \textbf{director} \textbf{Douglas} \textbf{Hamilton} \textbf{says} that he wanted to use the power of music to get people to \textbf{fulfil} their "\textbf{national} duty".
We are the \textbf{worst} in the world when it comes to planting, so we \textbf{realised} that this was an issue we had to deal with.
We \textbf{knew} that the government had \textbf{tried} a lot, such as marketing \textbf{perfume}\underline{s} with ph\textbf{ero}\underline{mon}es or \textbf{organizing} speed \textbf{dating} evenings (\textbf{fast} flirts).
\textbf{Meanwhile}\underline{,} an \textbf{immigration} policy aimed at a \textbf{dramatic} increase in \textbf{immigration} in order to \textbf{counter}\textbf{\underline{act}} the reduction of the population has led to \textbf{res}\underline{ent}ment among the local population.
When asked about the text, they \textbf{indicated} that the content was presented by the President of \textbf{Peru}\underline{,} Oll\textbf{anta} \textbf{Hum}\textbf{\underline{ala}}\underline{,} in \textbf{brief} \textbf{statements} to the press.
"\textbf{We} will follow and implement the \textbf{judgment} on the \textbf{differences} that we are currently \textbf{presenting} to this international \textbf{court}\underline{,}" \textbf{Hum}\textbf{\underline{ala}} said, together with his \textbf{Chile}\underline{an} \textbf{counterpart}\underline{.}
'\textbf{We} will review all these \textbf{paths} - they are not \textbf{exclusive}\underline{,} and the agreement with \textbf{Nicaragua} also requires \textbf{talks} with \textbf{Nicaragua}\underline{'} he \textbf{stressed}\underline{.}
There are huge \textbf{gap}\underline{s} between health programs and \textbf{ordinary} citizens, \textbf{explains} \textbf{Rica}\underline{r}do Sal\textbf{azar}\underline{,} \textbf{Gua}\textbf{\underline{dal}}\textbf{\underline{aja}}\underline{ra} \textbf{journalist}\underline{,} who has \textbf{tackled} the \textbf{HIV} issue.
It is \textbf{estimated} that \textbf{50,000} people live with \textbf{HIV} because for each \textbf{registered} case there are 4 or 5 people who do not know.
In an effort to pay long-term \textbf{liabilities} without im\textbf{pair}\underline{ing} short-term \textbf{liabilities}\underline{,} the construction company Homex \textbf{puts} more than 500 million pesos on the market.
I like to \textbf{listen} to music, \textbf{watch} \textbf{videos} of my time in \textbf{YouTube}\underline{,} enjoy my \textbf{grand}\textbf{\underline{child}}\underline{ren} and from time to time I go to a \textbf{basketball} game.
La\textbf{rry} \textbf{Hag}\underline{man}, whose role as the oil magnate J.R. E\textbf{wing} in the \textbf{television} series "\textbf{Da}\textbf{\underline{lla}}\underline{s}" became a \textbf{symbol} of the \textbf{gre}\underline{ed} of the \textbf{1980}\underline{s}, is \textbf{dead}\underline{.}
The \textbf{couple} had two children, Preston and Heidi, and they \textbf{lived} for a long time in the \textbf{California}\underline{n} town of \textbf{Mali}\textbf{\underline{bu}}\underline{,} where many \textbf{celebrities} live.
If \textbf{someone} were to \textbf{analyse} what has \textbf{happened} in the world today as if we were \textbf{thirty} days away from it, this would be a very good period.
"In two hours there were no more places" said Re\textbf{stall} about his high \textbf{average} \textbf{student} course, which was \textbf{filled} with 35 students.
The measures adopted since 2009 have reduced the number of newcomers \textbf{registered} by 17\% in 2010 \textbf{compared} with \textbf{2006.}
At this stage, the \textbf{doctors} and nurses who take care of them no longer overw\textbf{helm} them with so-called "\textbf{cur}\underline{ative}" care.
"I no longer have any desires in life," she \textbf{says} before \textbf{accepting} that a \textbf{mask} should be set up to help her \textbf{breath}\underline{e}.
\textbf{According} to El\textbf{sie} \textbf{Mon}\underline{er}\textbf{eau}\underline{,} head of \textbf{pal}\underline{li}ative care of the company of \textbf{domestic} \textbf{pal}\underline{li}ative care of the \textbf{Montreal} area, \textbf{8\%} of \textbf{patients} do not address \textbf{pain} treatment.
In addition, the police of the '\textbf{Mar}\textbf{\underline{teau}} force', which since 2009 has \textbf{meant} that the '\textbf{Can}\underline{al}isation Cartel' of \textbf{Montreal} has been more \textbf{cautious} in \textbf{artificial}\underline{ly} in\textbf{flat}\underline{ing} \textbf{contracts}\underline{...}
The next on the list would be \textbf{Gill}\underline{es} \textbf{Va}\textbf{\underline{illa}}\underline{n}\textbf{court}\underline{,} who has just \textbf{resign}\underline{ed} from his position as \textbf{mayor} of La\textbf{val}\underline{,} the third largest city in \textbf{Quebec}\underline{.}
Since my beginnings at the centre of the \textbf{preparato}\underline{ry} training of \textbf{IN}\underline{F} \textbf{Cla}\textbf{\underline{ire}}\textbf{\underline{fo}}\underline{n}\textbf{tain}\underline{e} up to my \textbf{playing} time at \textbf{Saint}\underline{-}Et\textbf{ienne}\underline{,} I have made \textbf{progressive} progress.
\textbf{Would} it be a great failure not to \textbf{win} the title in Li\textbf{gue} 1, as was the case in the last season?
It \textbf{describes} \textbf{Bit}\underline{co}in as "the \textbf{virtual} currency with the \textbf{greatest} success", "in competition with the \textbf{dollar} or euro" and "si\textbf{mil}\underline{ar} to \textbf{conventional} \textbf{currencies}\underline{".}
Many young people want to leave the country, as did those who have benefited from American \textbf{subsidies}\underline{:} capital \textbf{flight} is \textbf{considerable}\underline{.}
All, including \textbf{armed} parties, are obsessed with mobile \textbf{phones}\underline{;} \textbf{television}\underline{,} with its \textbf{Turkish} series, which are a modern world, is being \textbf{watch}\underline{ed} \textbf{everywhere}\underline{.}
A very short period that forces the \textbf{brother}\underline{s} to for\textbf{ego} their \textbf{intention} to \textbf{explain} to the \textbf{Egyptian}\underline{s} the text section by section.
It is also a way for the President to \textbf{regain} his public and democratic \textbf{legitimacy} as the \textbf{protest} \textbf{ra}\textbf{\underline{ges}} throughout the country.
\textbf{Following} \textbf{affirm}\underline{ations} in an \textbf{interview} with the American \textbf{weekly} show \textbf{Time}\underline{,} \textbf{Mohammed} \textbf{Mor}\underline{si} seems \textbf{convinced} that the \textbf{Egyptian}\underline{s} will vote favour\textbf{ably}\underline{.}
A \textbf{journey} within the city costs 6 \textbf{bars} \textbf{regardless} of the means of transport, which includes a transfer for a \textbf{journey} of up to \textbf{1.5} hours.
The Russian police know that most of our documents are for\textbf{ged} and we are not \textbf{registered}\underline{,} and this \textbf{leads} to blackmail.
In this way, the authorities are \textbf{react}\underline{ing} to recent events: \textbf{wound}\underline{ed} in \textbf{shot}\underline{s} at \textbf{wedding}\underline{s} and \textbf{seven} \textbf{dead} in \textbf{Moscow}\underline{'}s \textbf{ju}\underline{r}ist Dmitri \textbf{Win}\underline{o}\textbf{grad}\underline{ov}'s amok \textbf{race}\underline{.}
"\textbf{There} is \textbf{evidence} that some cases were arson in order to cover up the \textbf{absence} of \textbf{weapons}\underline{,}" \textbf{says} former military member.
As a potential customer, I do not just buy but go into the \textbf{forest} with the \textbf{seller}\underline{,} where we set a target.
\textbf{Viktor} Baranez \textbf{emphasize}\underline{s} that when you place a request on a website, you can end up being \textbf{empty} and coming behind \textbf{bars}\underline{.}
\textbf{McDonald}\underline{'}s \textbf{says} that the company \textbf{sell}\underline{s} billions of \textbf{portion}\underline{s}, and yet you are not given \textbf{sick} days and you are not paid for your \textbf{honest} work!
The \textbf{theme} of the \textbf{enlarged} reality, which is popular among \textbf{adher}\textbf{\underline{ents}} of modern technologies, is usually \textbf{perceived} recently by a \textbf{lens} of a special \textbf{spectacle}\underline{.}
\textbf{Until} now, human\textbf{kind} has \textbf{largely} \textbf{remained} \textbf{stuck} in the \textbf{phase} of working with \textbf{pixels} on \textbf{flat} screens that are sometimes touched.
- \textbf{Does} that mean you want the user to \textbf{adapt} to what a machine can and cannot do at the time?
- \textbf{Ki}\underline{n}\textbf{ect} currently works with three "\textbf{cam}\textbf{\underline{era}}\underline{s}", one of which is actually an \textbf{infrared} \textbf{transmit}\underline{ter} and the other a \textbf{receiver} for the \textbf{reflected} \textbf{signal}\underline{.}
- In my \textbf{lecture}\underline{s} I often speak of the fact that the \textbf{enlarged} reality is the \textbf{seventh} \textbf{breakthrough} in the \textbf{interaction} between man and machine.
\textbf{cord} and his friends sang simple \textbf{songs} for play-\textbf{back}\underline{,} \textbf{wearing} \textbf{tight} jer\textbf{sey}\underline{s} and including today's \textbf{trendy} \textbf{composer} I\textbf{gor} W\textbf{dow}\underline{in}.
"\textbf{This} was just the case with the \textbf{bio}\textbf{\underline{satellit}}\underline{es}, but once again it was only a single \textbf{experiment}\underline{,} and research must continue," \textbf{says} \textbf{Vladimir} \textbf{Sy}\underline{che}v.
In the state of \textbf{gravity}\textbf{\underline{lessness}}\underline{,} the ab\textbf{dom}\underline{en} and pool \textbf{muscle}\underline{s} \textbf{rapidly} \textbf{shrink} and thus the ability to press out the child \textbf{decrease}\underline{s}.
\textbf{Recently}\underline{,} the \textbf{Prime} Minister said that the O\textbf{DS} would not ha\textbf{rass} \textbf{entrepreneurs} with \textbf{controls} - is the system now \textbf{banned} or allowed?
The law will never be perfect, but it must be applied \textbf{correctly} - and that is what I believe we lack.
\textbf{Road}\underline{s} in the \textbf{Pil}\underline{s}en area are now easily \textbf{accessible}\underline{,} but there is a need for increased attention to be paid to the local area and the way of \textbf{driving} must be \textbf{adapted} to the \textbf{weather}\underline{.}
The road from \textbf{Tel}\underline{n}ice to Kn xednice is closed in   u20\textbf{47} \textbf{st} xed n.K., according to traffic police.
The road between \textbf{Tel}\underline{n}ice and Kn xednice was closed because of \textbf{branches} \textbf{pressed} from the \textbf{snow} to the road.
\textbf{Five} of our members are \textbf{wheelchair} users, i.e. the \textbf{wheelchair}\underline{s} must be carried in the \textbf{luggage} room, and of course we must carry many instrument cases and other \textbf{luggage}\underline{...}
At that time there were already the first \textbf{satellite} technology projects and it was to be expected that space \textbf{exploration} would have a future.
\textbf{Three} types of this \textbf{missile} were developed (\textbf{Me}\underline{te}or-1A, -1B and -1C) which \textbf{differ}\underline{ed} from each other in the size of the transport space for scientific instruments.
This is caused by the principle of free trade and free, \textbf{unrest}\textbf{\underline{ric}}\underline{ted} movement of private capital, which goes hand in hand with un\textbf{bri}\underline{d}led financial \textbf{speculation}\underline{.}
\textbf{Lobby} interests also supported the idea that \textbf{banana}\underline{s} of the highest trade class in the EU must be at least 14 \textbf{cm} long and must not have a '\textbf{cur}\underline{r}\textbf{ency} an\textbf{oma}\underline{ly}'.
The EU thus set the maximum \textbf{volume} of food \textbf{stocks} that was allowed to be on the \textbf{territory} of the Czech Republic on the day of our accession to the EU.
It is part of a re\textbf{vit}\underline{al}ization project that also includes \textbf{underground} parking, \textbf{supermarket}\underline{,} post office and a \textbf{couple} of \textbf{neighbouring} \textbf{houses} with a total of 50 apartments.
Although there is a \textbf{lift} that \textbf{leads} through the mountain massif, the true \textbf{delight}\underline{s} of space and reading are \textbf{revealed} by walking up the top\textbf{ography}\underline{.}
\textbf{Like} \textbf{Plu}\underline{to}, who \textbf{circle}\underline{s} around the sun behind Ne\textbf{pt}\underline{un}, \textbf{Cer}\underline{es} is not a "planet" according to the new \textbf{definition} of the International \textbf{Astronom}\underline{ical} Union of \textbf{2006.}
The \textbf{inner} life of \textbf{Gran} \textbf{Tele}\textbf{\underline{sc}}\underline{op}io \textbf{Canaria} on the \textbf{Canary} \textbf{Island} of La \textbf{Palma} is huge - only the \textbf{mirror} is \textbf{10.}\underline{4} \textbf{meters} in \textbf{diameter}\underline{.}
Or is it the original way of life that \textbf{keeps} people young?
But the \textbf{cult} of the \textbf{father} of the \textbf{nation}\underline{,} who \textbf{ruled} his country like a \textbf{dictator}\underline{,} \textbf{knows} little borders in \textbf{Azerbaijan}\underline{.}
As \textbf{Mohammed} \textbf{Mor}\underline{si} almost apologized, he had \textbf{temporarily} \textbf{curtail}\underline{ed} the powers of the \textbf{Constitutional} Court and \textbf{extended} his powers 'to save the \textbf{revolution}\underline{'}.
That does not have to be the case, but it may mean that \textbf{cl}\underline{er}\textbf{gy} \textbf{supervise}\underline{s} legislation, which would de \textbf{facto} lead to the \textbf{judiciary} being \textbf{strip}\textbf{\underline{ped}} of its powers.
The state should also "prot\textbf{ect} the true \textbf{essence} of the \textbf{Egyptian} family" and promote its \textbf{moral}\underline{s} and values.
The aim, however, was not to \textbf{disrupt} com\textbf{mut}\underline{ers} on their way to work, but to prevent \textbf{demonstrators} from \textbf{reaching} Parliament.
In the last two years alone, \textbf{dozen}\underline{s} of \textbf{murdered} women have been left behind on a \textbf{spot} of set-aside land near a large \textbf{landfill} site.
The US \textbf{Army} \textbf{intelligence} analyst, \textbf{arrested} in June \textbf{2010,} is \textbf{accused} of \textbf{steal}\underline{ing} thousands of \textbf{confidential} documents during his service in Iraq.
Manning said that he had \textbf{tried} to stay on the move, because on the day it was \textbf{forbidden} to \textbf{sleep} or even \textbf{sit} down.
If he had \textbf{turned} around at night and \textbf{guard}\underline{s} could no longer see his face, he was woken up to turn back.
As \textbf{Islamist}\underline{s} have \textbf{gained} influence in the \textbf{Arab} world, \textbf{Hamas} has been able to draw powerful and rich friends on its side.
In future \textbf{diplomatic} negotiations, \textbf{Hamas} could \textbf{prove} to be a player that even Israel and the United States cannot \textbf{push} out.
No, it is better to keep them in check and \textbf{punish} them behind the \textbf{wall} if they dare to \textbf{lift} their \textbf{heads}\underline{.}
The \textbf{repression} is already und\textbf{ermining} democracy in the \textbf{Jewish} state, and with the growth of the \textbf{Arab} population this situation will only \textbf{worse}\underline{n}.
\textbf{Like} many people, I have always \textbf{assumed} that \textbf{bo}\underline{re}\textbf{dom} is a relatively current \textbf{phenomenon} that has developed with increasing \textbf{leisure} time.
"\textbf{Our} \textbf{authority} has a duty to \textbf{prosecut}\underline{e} \textbf{offences} that were criminal at the time of the crime," B\textbf{uck} stated in a statement.
And the conflicting \textbf{responses} across the state \textbf{revealed} a deep \textbf{division} among local \textbf{officials} about the great green \textbf{experiment}\underline{.}
\textbf{Color}\underline{ado} and \textbf{Washington} are the first countries to \textbf{treat} \textbf{smaller} \textbf{amounts} of \textbf{mar}\underline{i}juana like \textbf{alcohol} as national \textbf{models} for the legalisation of \textbf{drugs}\underline{.}
The 20-\textbf{year}\underline{-}\textbf{old} Luke \textbf{Black}\underline{,} \textbf{vice}\underline{-}\textbf{pre}\underline{s}\textbf{ident} of the \textbf{conservative} \textbf{student} \textbf{association} of the University of \textbf{Nottingham}\underline{,} said in a \textbf{Sunday} \textbf{newspaper}\underline{:} "\textbf{There} is a growing \textbf{trend} towards links in \textbf{universities}\underline{.}
Last year, the University voted not to \textbf{grant} an \textbf{honor}\underline{ary} \textbf{diploma} to \textbf{Margaret} Thatcher, a former \textbf{student}\underline{,} because of \textbf{cuts} in higher education.
In the first days of the first \textbf{semester} week, when new students get to know each other and the \textbf{tut}\underline{ors}, I received a fore\textbf{taste} of what will happen in the future.
It is bad enough for me, but they know that your \textbf{father} is close to \textbf{Margaret} Thatcher, so it will be \textbf{worse} for you.
Even the \textbf{prince}\underline{s}s and opinion-\textbf{lea}\underline{der} at the \textbf{fashion} \textbf{Patri}\underline{cia} \textbf{della} Giovampaola d'\textbf{Ar}\textbf{\underline{enberg}} cannot \textbf{forget} for the first time when she wore a \textbf{Valentin}\underline{o}.
When I was a \textbf{teenage}\underline{r} in Italy, I \textbf{dream}\underline{ed} of finally having the age and the opportunity to \textbf{wear} one of his evening \textbf{clothes}\underline{...}
We therefore thought: why not do something as \textbf{creative}\underline{ly} as possible to \textbf{tackle} this problem, such as \textbf{comp}\underline{os}ing a \textbf{rap}\underline{?}
\textbf{Singapore} is a rich, high-\textbf{tech} city-\textbf{state} in south-\textbf{east} Asia known for its \textbf{rulers} u2019 \textbf{conserv}\underline{at}ism and \textbf{strict} social \textbf{controls}\underline{.}
\textbf{Tan} Wei Ming, \textbf{Director} of Mar\textbf{ria}\underline{ge} and \textbf{Family} Policy of the National \textbf{Pop}\textbf{\underline{ulation}} \textbf{Authority}\underline{,} \textbf{says} that this is due to '\textbf{bett}\underline{er} education' and '\textbf{gre}\underline{at}er \textbf{career} opportunities'.
"P\textbf{eo}\textbf{\underline{ple}} are very \textbf{stressed}\underline{,} the apartments and also the up\textbf{bring}\underline{ing} are \textbf{expensive}\underline{,} which is why it is being \textbf{pushed} out by many" \textbf{says} a young \textbf{manager}\underline{.}
That is why the \textbf{Singapore}\textbf{\underline{ans}} have the last word when it comes to having children - the government can do so much.
Is he aware of the \textbf{dangers} he is \textbf{exposed} to when he \textbf{announce}\underline{s} on the Internet \textbf{situations} he would not share in real life?
"The Internet was created as a medium for \textbf{searching} for information, but with the \textbf{publication} of these pages the rules of the game changed," she \textbf{says}\underline{.}
The summit was \textbf{attended} by the Presidents of \textbf{Brazil}\underline{,} Dilma \textbf{Rou}\underline{s}\textbf{eff}\underline{,} \textbf{Venezuela}\underline{,} Hugo \textbf{Ch} xe1vez, \textbf{Bolivia}\underline{,} Evo \textbf{Moral}\underline{es}, and \textbf{Argentina}\underline{,} \textbf{Cristina} \textbf{Kirch}\underline{ner}.
'\textbf{We} hope that the \textbf{electoral} process in that country will serve to re-\textbf{establish} it in the Union of South American Nations', from which it is currently \textbf{excluded}\underline{.}
"I hope to be able to say to President \textbf{Ortega} that we will \textbf{treat} this matter as civilised and respectful as possible," \textbf{Santo}\underline{s} added.
"The \textbf{greatest} \textbf{enemies} of press freedom are not \textbf{evil} and \textbf{perverse} \textbf{politicians}\underline{,} but bad \textbf{journalists} who \textbf{seek} \textbf{profit} and blackmail," he said.
"\textbf{My} political movement had the \textbf{belief} that it was I who \textbf{guaranteed} this likely \textbf{victory}\underline{,} so I must \textbf{assume} that responsibility," he said.
He is \textbf{undoubtedly} one of the \textbf{oldest} \textbf{patients} of the \textbf{HIV} \textbf{unit} of the \textbf{Hospital} \textbf{Civil} de \textbf{Gua}\textbf{\underline{dal}}\textbf{\underline{aja}}\underline{ra} (HCG), which he came to after several fights in \textbf{1994}\underline{.}
However, the decision \textbf{opens} the \textbf{door} to the largest \textbf{glass} \textbf{manufacturer} in \textbf{Mexico} to refer three inconsisten\textbf{cies} to the United States \textbf{Supreme} Court.
"La\textbf{rry} was back in his \textbf{beloved} \textbf{birth} town of \textbf{Dal}\textbf{\underline{las}}\underline{,} where he again played the \textbf{icon}\underline{ic} role he \textbf{liked} most," said the family.
The \textbf{dramatic} series of the C\textbf{BS} TV \textbf{chain} about the E\textbf{wing}\underline{-}C\textbf{lan} and other \textbf{figures} in its \textbf{surroundings} was aired from April \textbf{1978} to May \textbf{1991}\underline{.}
Moreover, \textbf{Republican} \textbf{legislators} in five other states have \textbf{passed} laws aimed at shortening the period for early voting.
There is an \textbf{inevitable} law in this world that prevents two \textbf{objects} from being in the same place at the same time.
It is not possible to \textbf{violate} this rule - and do not try too hard because you will \textbf{hurt}\underline{.}
The same is true for the \textbf{Hi}\textbf{\underline{gg}}\underline{s}\textbf{Bo}\underline{son}, with the \textbf{difference} that another field, the \textbf{Hi}\textbf{\underline{gg}}\underline{s} field, must be "\textbf{cor}\underline{r}\textbf{ect}\underline{ed}" for this \textbf{bo}\underline{son} to appear.
The \textbf{disease} does its job: an immeasurable \textbf{weakness} prevents it from going to the \textbf{toilet} alone and even \textbf{eating} itself.
\textbf{Other} civil \textbf{servant}\underline{s} of the road construction \textbf{authority} have \textbf{admitted} that they have been \textbf{gre}\underline{as}ed by \textbf{artificial}\underline{ly} in\textbf{flat}\underline{ing} the \textbf{bill}\underline{s} by 30-40\% with \textbf{false} additional services.
\textbf{Given} what has been \textbf{invested} and the players we have, it is normal that much is expected of us.
The \textbf{Bit}\underline{co}ins that are in \textbf{circulation} are therefore limited to 21 million, but can be \textbf{divided} up to one \textbf{hundred} millionth, which \textbf{leaves} some room for \textbf{manoeuvre}\underline{...}
For his \textbf{opponents}\underline{,} the President \textbf{persist}\underline{s} in his "\textbf{auto}\textbf{\underline{cra}}\underline{tic} deli\textbf{rium}\underline{"} by \textbf{continuing} to "\textbf{break} his word" and "re\textbf{fu}\underline{ge} the law".
In addition to its \textbf{religious} \textbf{aspect}\underline{,} the text adopted \textbf{yesterday} is highly \textbf{criticised} for the far-\textbf{reaching} powers it \textbf{grants} to the President of the Republic.
While \textbf{parliamentarian}\underline{s} and civil rights \textbf{activists} are \textbf{discussing} the benefits of the law on \textbf{compulsory} language \textbf{tests} for \textbf{migrants}\underline{,} criminals are already \textbf{trading} with fake \textbf{certificates}\underline{.}
On 1 December, a law \textbf{entered} into force \textbf{requiring} every \textbf{immigrant} worker to carry out a test \textbf{cert}\textbf{\underline{ifying}} knowledge of the Russian language.
Also \textbf{excluded} from this law are people who received their \textbf{certificates} and \textbf{diploma}\underline{s} before the \textbf{USS}\underline{R} dis\textbf{integr}\underline{ated} in \textbf{1991}\underline{.}
"\textbf{Man}\underline{y} people are now talking about \textbf{protecting} the rights of \textbf{migrant} workers," \textbf{says} \textbf{Viktor} Sebe\textbf{lev}\underline{,} head of the \textbf{federal} \textbf{immigration} \textbf{agency} in Ta\textbf{ji}\underline{k}\textbf{istan}\underline{.}
Baranez \textbf{explains} that this includes \textbf{weapons} \textbf{stolen} both from police \textbf{chamber}\underline{s} and directly from law \textbf{enforcement} staff.
"The dealer \textbf{brings} the \textbf{weapon} to the city and \textbf{sell}\underline{s} it there for \textbf{900} Euros per \textbf{piece} with two \textbf{magazine}\underline{s}," he \textbf{says}\underline{.}
Former military member \textbf{Viktor} Baranez \textbf{tried} to buy illegal \textbf{weapons} in the \textbf{mid}\textbf{\underline{-19}}\underline{90} u2019s when he \textbf{wrote} an \textbf{article} on the subject.
\textbf{According} to Dmitry \textbf{Ki}\underline{s}\textbf{lov} of the \textbf{organization} "Pravo na ory\textbf{zh}\underline{ie}" one can buy a \textbf{Mak}\underline{a}\textbf{row} \textbf{gun} for 100 to 300 \textbf{dollars}\underline{.}
Ad\textbf{voca}\underline{tes} of \textbf{Wal}\underline{mar}t are pleased to note that \textbf{protests} have only \textbf{occurred} in \textbf{nine} states and have not caused any \textbf{losses} to the company.
- Although \textbf{Ki}\underline{n}\textbf{ect} has brought \textbf{interaction} to a \textbf{physical} level, much still takes place on the \textbf{flat} screen, sometimes in 3D.
Do you not think that \textbf{glass}\underline{es} have the best \textbf{prospects} in day-to-day life with regard to the application of the technology of \textbf{extended} reality?
In order to save \textbf{humanity}\underline{,} the important question \textbf{arises} as to how we can \textbf{prop}\underline{a}\textbf{gate} ourselves in \textbf{weight}\textbf{\underline{lessness}} or on the \textbf{replacement} \textbf{planet}\underline{?}
In view of the fact that this amendment is only in force for a short time, it has not yet had an impact on our \textbf{tests}\underline{.}
The \textbf{Prime} Minister recently said that the O\textbf{DS} would not ha\textbf{rass} \textbf{entrepreneurs} with \textbf{controls} on the so-called '\textbf{black} system' - what exactly does that mean?
On the other hand, it is also \textbf{tragic} if the \textbf{bid}\underline{der} with the best offer is \textbf{excluded} \textbf{solely} because of \textbf{fault}\underline{s} in form.
The text of the anthem comes from \textbf{Tom} xe1  u20\textbf{47}  \textbf{Han} xe1k, who also \textbf{plays} the main character of \textbf{Jesus} in the video \textbf{clip}\underline{,} also \textbf{Xi}\underline{nd}l X \textbf{sing}\underline{s} with...
It is still \textbf{unusual} for people \textbf{travelling} in \textbf{wheelchair}\underline{s} alone in the city centre.
The first mention of this company was made in \textbf{1954} in the November issue of the \textbf{magazine} Problemy, in which four comprehensive \textbf{articles} are \textbf{devoted} to space.
Since private capital has no social responsibility and therefore no responsibility for the unemployment it \textbf{causes}\underline{,} public \textbf{spending} is \textbf{necessarily} increasing.
\textbf{Private} capital, by its very nature, is not in a position to \textbf{recognise} and \textbf{enforce} the benefit for the whole of society.
"\textbf{If} my \textbf{son}\underline{s} \textbf{didn}\underline{'}t want wars, there wouldn't be wars," \textbf{says} Mayer Ams\textbf{chel} \textbf{Roth}\textbf{\underline{schild}}\underline{'}s \textbf{dying} good-sn\textbf{ake}\underline{,} \textbf{wife}\underline{,} in 18\textbf{49}\underline{.}
A \textbf{laugh}\underline{ing} \textbf{actor} has become a respectable \textbf{director}\underline{,} and even as an \textbf{actor} he is no longer the target of \textbf{iron}\underline{ic} comments.
The \textbf{feeling} for the atmosphere of the place was one of the features that \textbf{distinguished} this \textbf{director} u2019s previous \textbf{films} from \textbf{Hollywood} u2019s standard.
The European Commission \textbf{defended} itself by \textbf{arguing} that it would only \textbf{harmonise} the un\textbf{even} national standards that would \textbf{hinder} trade.
As an \textbf{argument}\underline{,} he \textbf{argued} that the \textbf{grain} \textbf{harvest} was very high and that the state \textbf{stock} had been overc\textbf{row}\textbf{\underline{ded}} as a result of the so-called \textbf{intervention} purchases.
\textbf{Later}\underline{,} I made this clear and I said that I would stand for the office of President if I were \textbf{elected} as a senator.
In addition, there are the media who want to \textbf{deprive} you of \textbf{honour} and who \textbf{confuse} the freedom of the word with freedom to \textbf{lie}\underline{.}
\textbf{Six}\underline{ty} per \textbf{cent} of those \textbf{entitled} to vote did not go to the elections at all, and those who have \textbf{gone} have \textbf{mostly} \textbf{elected} representatives of the establishment.
The fully \textbf{gla}\underline{z}ed \textbf{interior} is \textbf{bright} and well-\textbf{structure}\underline{d}, the \textbf{burn}\underline{ed} K\textbf{link}\underline{er} floor and the elegant street lamps speak unmistak\textbf{ably} the language of a public \textbf{square}\underline{.}
During the March \textbf{2011} \textbf{uprising} in \textbf{Libya}\underline{,} Germany also \textbf{abstained} on \textbf{establishing} a no-fly \textbf{zone}\underline{.}
If you look at \textbf{Obama} u2019s relations with \textbf{Prime} Minister \textbf{Net}\underline{an}yahu, \textbf{Obama} is not so \textbf{enthusiastic} about \textbf{Net}\underline{an}yahu u2019s policies.
If we look at the euro crisis, for example, every time Germany takes on a greater role, a variety of anti-\textbf{German} \textbf{sentiment}\underline{s} are \textbf{released}\underline{.}
\textbf{Pat}\underline{t}\textbf{loch} reports of cases in which the Court \textbf{rejected} \textbf{claims} because, after the long period of time, the \textbf{dispute}\underline{d} name had become "\textbf{market} reality".
The \textbf{fashion} \textbf{manufacturer} La\textbf{cost}\underline{e} lost in China against \textbf{counterfeit}\underline{s} from \textbf{Hong} \textbf{Kong} and \textbf{Singapore}\underline{,} who led the famous \textbf{cro}\underline{co}dile to look the other way.
The \textbf{Robert} \textbf{Koch} \textbf{Institute} \textbf{assume}\underline{s} that at least four out of five of all \textbf{Sy}\textbf{\underline{phil}}\underline{is} cases \textbf{reported} in Germany are \textbf{transmitted} through \textbf{sexual} \textbf{contacts} between men.
The \textbf{spread} of \textbf{HIV} is \textbf{comparative}\underline{ly} low among \textbf{het}\textbf{\underline{ero}}\textbf{\underline{sexual}} \textbf{adults} in this country - \textbf{nevertheless}\underline{:} \textbf{approximately} 20 \textbf{percent} of new \textbf{HIV} \textbf{infection}\underline{s} are caused by this group.
This state-\textbf{san}\textbf{\underline{ction}}\underline{ed} way of life is one of the reasons why the \textbf{HI} \textbf{virus} has \textbf{spread} so \textbf{rapidly} in recent \textbf{decades}\underline{.}
However, the \textbf{findings} could help to \textbf{clarify} how water and other building \textbf{blocks} of life have \textbf{moved} to other areas of the \textbf{solar} system.
The \textbf{telescope} is said to have been \textbf{invented} by \textbf{Hans} Li\textbf{pper}\underline{he}y in 16\textbf{08} - even before \textbf{Galileo} \textbf{Gali}\textbf{\underline{lei}} used it for star \textbf{observation} a year later.
This is where the \textbf{vita} of about \textbf{eight} \textbf{dozen} \textbf{ta}\underline{ly}\textbf{ches} from the area is \textbf{documented}\underline{.}
His \textbf{speech} was \textbf{addressed} to the whole people, but above all to the \textbf{Christian} \textbf{Cop}\underline{ts}, the \textbf{liberal}\underline{s}, enlightened \textbf{Muslims} and \textbf{secular}\underline{s}.
This is so \textbf{blu}\underline{nt}ly \textbf{formulated} \textbf{legally} that state institutions could even control the content of film art and \textbf{literature} with the help of this \textbf{article}\underline{.}
Hafez \textbf{Abu} Saeda is \textbf{fur}\textbf{\underline{ious}} about this \textbf{forced} \textbf{constitutional} process, which should have \textbf{gone} to February and involved all social forces.
\textbf{Norway}\underline{'}s five million \textbf{inhabitants} enjoy one of the highest standards of living, not only in Europe but throughout the world.
Today, the population is growing \textbf{rapidly} - more than 13\% are \textbf{immigrants}\underline{,} \textbf{attracted} by a \textbf{thriving} labour market, high \textbf{wages} and comprehensive health care.
Since the early \textbf{1970} u2019s, \textbf{Norway} u2019s \textbf{wealth} today has been \textbf{driven} by the growth of one of the world u2019s largest oil and gas \textbf{industries}\underline{.}
The agenda included all the issues that are expected when the \textbf{heads} of these two countries meet: \textbf{immigration}\underline{,} \textbf{drugs} and trade.
If they really had control of the West Bank, would they not \textbf{fire} \textbf{rocket}\underline{s}, just like their \textbf{Gaza} \textbf{rival}\underline{s}?
The hope - small for the near future - is that the \textbf{cease}\underline{-}\textbf{fire} will give more influence to outsiders in order to implement this solution.
"\textbf{It} \textbf{sounds} as if we need to be \textbf{bo}\underline{ring} more often than not, but \textbf{bo}\underline{re}\textbf{dom} is the tormenting, un\textbf{rel}\underline{en}ting desire to do something \textbf{meaningful}\underline{,}" he \textbf{says}\underline{.}
In the Evening Standard it was said that I had \textbf{gone} because I had a problem with the fact that com\textbf{ili}\underline{ton}s had \textbf{sex} in the \textbf{neighbouring} room.
The \textbf{author} A N \textbf{Wilson} \textbf{gle}\underline{an}ed that I had left the \textbf{university} because I was \textbf{forced} to \textbf{drink} from \textbf{damaged} \textbf{cup}\underline{s}.
I started com\textbf{mut}\underline{ing} between \textbf{Oxford} and my \textbf{parents} u2019 house and found \textbf{refuge} with more open-\textbf{minded} friends and family members in the city.
Although I was \textbf{secret}\underline{ly} \textbf{sh}\textbf{\underline{atter}}\underline{ed} in \textbf{shame}\underline{,} I \textbf{admitted} that my \textbf{parents} had undergoed a \textbf{brain}\textbf{\underline{wash}} and called it "\textbf{old} \textbf{tr}\textbf{\underline{ough}}\underline{".}
A government package for \textbf{couples} and \textbf{parents} \textbf{grants} up to \textbf{\$1}\textbf{\underline{5,000}} per child, \textbf{extends} \textbf{maternity} leave, and \textbf{distribute}\underline{s} tax benefits.
But \textbf{Lim} Y\textbf{ew} Soon, \textbf{Director}\underline{-}\textbf{General} of \textbf{EL} \textbf{Developer}\underline{s}, \textbf{says} that his "s\textbf{hoe} \textbf{boxes}\underline{"} can be \textbf{sold} much \textbf{faster} than larger \textbf{housing} \textbf{units}\underline{.}
\textbf{Por}\textbf{\underline{ras}} then mentions some options: There are things you wouldn't tell a \textbf{strange}\underline{r}, so why do you do it on the Internet?
\textbf{Paraguay}\underline{,} which has been \textbf{excluded} from the United States since \textbf{2011} after the \textbf{removal} of its President \textbf{Fernando} Lugo, has not \textbf{participated} in the meeting.
He added that '\textbf{ther}\underline{e} were \textbf{reasonable} \textbf{assumption}\underline{s} at the time that Ass\textbf{ange} would be extradited to a third country and that his procedure would not be \textbf{complied} with'.
This month, students \textbf{analyze}\underline{d} \textbf{films} with apocaly\textbf{ptic} content and \textbf{studied} how to \textbf{compare} them with real life.
But \textbf{none} of the students \textbf{survey}\underline{ed} - and not so much a \textbf{professor} - stated that they \textbf{believed} in the last date of 21 December.
\textbf{Over} the past two years, they have \textbf{promoted} \textbf{bill}\underline{s} in \textbf{34} states that force \textbf{voters} to show a photo \textbf{ID}\underline{.}
In fact, 11\% of US citizens, that is to say 21 million \textbf{voters}\underline{,} do not have a photo \textbf{ID} \textbf{issued} by a government \textbf{authority} in their state.
Moreover, \textbf{Republican} \textbf{legislators} \textbf{promoted} laws in \textbf{eight} states in \textbf{2011} that \textbf{abolished} \textbf{voters} u2019 \textbf{registration} on \textbf{election} day.
Of course, democratic \textbf{legislators} and their \textbf{supporters} have \textbf{strongly} \textbf{opposed} the \textbf{adoption} of laws that \textbf{restrict} the \textbf{registration} of \textbf{voters}\underline{.}
This document (\textbf{current}\underline{ly} only in English but a \textbf{translation} will be available \textbf{shortly}\underline{)} can be \textbf{downloaded} at http://ca.\textbf{mov}\underline{e}\textbf{mber}\underline{.}com/\textbf{fr}\underline{/}mens-\textbf{health}\underline{/}pro\textbf{state}\underline{-}\textbf{can}\textbf{\underline{cer}}\underline{-}\textbf{screen}\underline{ing} .
Encour\textbf{aging} data: 10 years after \textbf{smoking}\underline{,} the risk of \textbf{cancer} is reduced by half.
In addition, Mr \textbf{Beau}\textbf{\underline{lie}}\underline{u} \textbf{emphasise}\underline{s} the importance of talking to his \textbf{doctor} about his concerns and his family pre\textbf{oc}\textbf{\underline{cup}}\underline{ation}.
\textbf{Establish}\underline{ed} in \textbf{2011}\underline{,} the permanent anti-\textbf{cor}\underline{r}uption \textbf{unit} is also making great efforts with its \textbf{troops} to government \textbf{auditor}\underline{s}, \textbf{invest}\underline{ig}\textbf{ators}\underline{,} and analysts.
It is a \textbf{fragment} of the file, i.e. \textbf{convert}\underline{ing} a large file into a \textbf{shorter} and unique electronic \textbf{fingerprint}\underline{.}
There is a collection of works by \textbf{impression}\underline{ists} and \textbf{expression}\underline{ists} \textbf{Mon}\underline{et}, P\textbf{issa}\underline{ro}, Renoir, C xe9z\textbf{anne}\underline{,} Sisley, \textbf{Mat}\textbf{\underline{isse}}\underline{,} \textbf{Mod}\textbf{\underline{iglia}}\underline{ni}, \textbf{Cha}\underline{ga}ll and \textbf{Picasso}\underline{.}
By the way, this \textbf{unusual} sea, with a \textbf{altitude} of 4\textbf{17} metres below sea level, is the deepest sea in the world.
\textbf{Migrant}\underline{s} can test in all cities; already more than \textbf{160} \textbf{centres} have been \textbf{opened} in Russia.
The \textbf{percentage} of \textbf{crimes} with \textbf{registered} \textbf{weapons} is very low, said the criminal , Was\textbf{ili}\underline{y} \textbf{Les}\underline{ni}\textbf{kov}\underline{,} the Russian service of the \textbf{BBC}\underline{.}
There are five such main \textbf{channels}\underline{,} \textbf{says} a former \textbf{Colon}\underline{el} \textbf{Viktor} Baranez, who worked for ten years in the \textbf{Ministry} of \textbf{Education} and the General \textbf{Staff}\underline{.}
"P\textbf{eo}\textbf{\underline{ple}} come like \textbf{hungry} fish to \textbf{feed} and then land in the \textbf{Siberia}\underline{n} labour \textbf{camp} and are allowed to snatch \textbf{coal}\underline{,}" he \textbf{says}\underline{.}
In addition to \textbf{raising} the \textbf{modest} \textbf{wages} of \textbf{ordinary} \textbf{Wal}\underline{mar}t and fast-\textbf{food} workers, the \textbf{protest} \textbf{organize}\underline{rs} are \textbf{aiming} to establish trade \textbf{unions}\underline{.}
The \textbf{gesture}\underline{s} were not \textbf{recorded} by the \textbf{object} camera, but by a \textbf{bra}\underline{ce}let that \textbf{recorded} the \textbf{movements} of the \textbf{bone}\underline{s} and \textbf{muscle}\underline{s}.
There are also \textbf{ri}\textbf{\underline{bb}}\underline{ons} for the wrist that influence the \textbf{nerve} \textbf{ending}\underline{s} in the \textbf{finger}\underline{s}, which is also a potential direction.
- \textbf{Kir}\textbf{\underline{ill}}\underline{,} why are you always in red and not in \textbf{yellow} or \textbf{tur}\textbf{\underline{qu}}\textbf{\underline{ois}}\underline{e} in the city?
Many were \textbf{born} there: N.O.M., Tequilajaz\textbf{zz}\underline{,} and I also remember how \textbf{cord} came there with his project "U\textbf{cho} Van Goga".
We need a cultural \textbf{breeding} ground because, for example, we now have more \textbf{writer}\underline{s} than \textbf{readers}\underline{,} and that is not right.
However, while the conditions on \textbf{Mars} are relatively friendly to life, the \textbf{surface} of \textbf{Venus} has a \textbf{temperature} of 500 \textbf{degrees}\underline{.}
In \textbf{1979}\underline{,} \textbf{qua}\underline{il} \textbf{eggs} were sent into space to \textbf{explore} how \textbf{gravity} \textbf{affects} the development of \textbf{embr}\textbf{\underline{yo}}\underline{s}.
The main \textbf{routes} as well as the I/\textbf{13} road at the border of   u20\textbf{47} \textbf{st} xed n.L.
For the establishment of the \textbf{barrier}\underline{-}\textbf{free} \textbf{Education} Centre \textbf{Stu}\underline{de}o, which we have been working on for six years with the \textbf{Tap} \textbf{Association} in the Jedli  u20\textbf{47} \textbf{ka} \textbf{Institute}\underline{.}
It is true that cooperation with well-\textbf{known} \textbf{singer}\underline{s} has \textbf{helped} us; we have also started to promote us \textbf{actively}\underline{.}
If we want to do something well, we cannot compromise on many things and we must also demand a certain \textbf{discipline}\underline{.}
\textbf{Poland} began a close cooperation with the ESA in \textbf{1994} and \textbf{participated} in several ESA projects over the following years.
\textbf{Further} \textbf{articles} on space \textbf{appeared} in the \textbf{Polish} press after the war thanks to the work of the \textbf{Polish} \textbf{Space} \textbf{Society} (\textbf{Pol}\underline{ski}e To\textbf{war}\textbf{\underline{zy}}\underline{s}\textbf{two} \textbf{Astro}\textbf{\underline{nau}}\underline{ty}\textbf{cz}\underline{ne}).
The \textbf{liberal} \textbf{economies} in the EU and in the globalised world are \textbf{founded} on the principle of un\textbf{reg}\textbf{\underline{ulate}}\underline{d} economic competition.
A world in which each new\textbf{born} is \textbf{implant}\underline{ed} at \textbf{birth} a \textbf{chip} to subject this being to total control.
The film Argo by \textbf{director} and \textbf{actor} \textbf{Ben} Af\textbf{fleck} \textbf{describes} an \textbf{episode} of this \textbf{story} that brought a small \textbf{partial} \textbf{victory} to the US.
Argo is his third feature film after the \textbf{Krim}\underline{i} \textbf{Kein} Kinderspiel (Gone \textbf{Baby} Gone, 2007) and the \textbf{Th}\underline{r}\textbf{iller} Stadt ohne \textbf{Gnade} (\textbf{2010}\underline{).}
\textbf{Among} the \textbf{absurd}\underline{ities} \textbf{nominated} is, for example, the \textbf{ruling} of the European Court of \textbf{Justice} on the \textbf{uniform}\underline{ity} of \textbf{insurance} \textbf{tariffs} for men and women.
In the past, there has also been \textbf{criticism} of the fact that there has been a ban on the use of the term 'b\textbf{utter} \textbf{spread}\underline{'} or even the ban on \textbf{selling} \textbf{conventional} light \textbf{bulb}\underline{s}.
I have been \textbf{telling} \textbf{myself} all the time that I will start the \textbf{battle} for the \textbf{castle} after the \textbf{outcome} of the \textbf{Senat}\underline{e} elections.
I started my can\textbf{dida}\underline{cy} on the \textbf{condition} that people are \textbf{deeply} diss\textbf{ati}\underline{s}fied, but now I am no longer sure.
And so the city \textbf{father}\underline{s} \textbf{recognized} that there was only one way to \textbf{master} the \textbf{statistics}\underline{:} a \textbf{library} had to go!
"\textbf{You} wouldn't believe it, but despite the many \textbf{glass} \textbf{surface}\underline{s} this house is a model project for \textbf{eco}\textbf{\underline{logy}}\underline{,}" \textbf{says} \textbf{Tro}\underline{ub}orst.
For the time being, this is intended to \textbf{fill} the \textbf{optical} \textbf{gap}\underline{s} in the \textbf{library} that has not yet been fully equipped - currently 7\textbf{0,000} \textbf{pieces}\underline{.}
It shows a \textbf{willingness} to take \textbf{positions} on national interests that are independent from those of the United States or European partners.
Germany u2019s economic interests are to some extent different from those of the other major powers, and that is why Germany must protect its interests.
It must therefore be \textbf{careful} not to up\textbf{set} the public, but also the \textbf{elite}\underline{s}, in the \textbf{Arab} countries.
Szabo is also a member of the German \textbf{Marshall} Fund, where he \textbf{specialize}\underline{s} in German \textbf{politics}\underline{,} US foreign policy and \textbf{transatlanti}\underline{c} relations.
If the \textbf{plain}\underline{t}\textbf{iff} is un\textbf{luck}\underline{y}, he even has to pay money to the \textbf{pla}\textbf{\underline{gia}}\underline{r} because he \textbf{broke} his brand in China, \textbf{says} \textbf{Pat}\underline{t}\textbf{loch}\underline{.}
The CTMO \textbf{Trade}\underline{mark} Office in \textbf{Beijing} \textbf{admit}\underline{s} that there were \textbf{bottle}\underline{n}\textbf{eck}\underline{s} there in 2010 due to \textbf{insufficient} \textbf{personnel} and room equipment.
The internal costs could \textbf{hardly} be \textbf{quant}\textbf{\underline{ified}}\underline{;} the company u2019s \textbf{archive} even had to look through a \textbf{hundred}\underline{-}\textbf{year}\underline{-}\textbf{old} file to produce \textbf{evidence}\underline{.}
Then the \textbf{voices} of the \textbf{singer}\underline{s} \textbf{slowly} \textbf{grow} up - old, \textbf{bass}\underline{,} tenor and so\textbf{pra}\underline{no} - \textbf{crowd}\underline{,} be\textbf{gui}\underline{le} and \textbf{pursue} themselves.
And Fi\textbf{ete} Ho\textbf{pf}\underline{,} the 29-\textbf{year}\underline{-}\textbf{old} \textbf{conductor}\underline{,} almost \textbf{lift}\underline{s} it out of his \textbf{clothes} when he \textbf{brings} them together with his \textbf{smoothly} \textbf{wild} \textbf{gesture}\underline{s}.
More than forty per \textbf{cent} of Swaziland u2019s people carry the \textbf{immun}\underline{o}\textbf{def}\textbf{\underline{ici}}\textbf{\underline{ency}} \textbf{virus}\underline{,} and \textbf{dying} in the \textbf{middle} of \textbf{thirty} is not \textbf{rare}\underline{.}
The \textbf{probe} \textbf{Messenger}\underline{s} have found \textbf{evidence} that there is an \textbf{ice} \textbf{blanket} in the \textbf{permanently} \textbf{shadow}\underline{ed} region of the \textbf{planet}\underline{.}
For 30 years, from \textbf{1947} to \textbf{1975}\underline{,} \textbf{Hal}\underline{e} \textbf{Teleskop} was the largest \textbf{telescope} in the world in the \textbf{Pal}\underline{o}mar ob\textbf{serv}\textbf{\underline{atory}} near San Diego.
This small town \textbf{boasts} an unduly er\textbf{od}\underline{ed} \textbf{Soviet}\underline{-}\textbf{era} \textbf{architecture} that does not \textbf{fit} into the \textbf{picturesque} mountain \textbf{landscape}\underline{.}
"\textbf{We} are not \textbf{tired}\underline{,} the \textbf{blood} of our \textbf{brother}\underline{s} has not yet atoned," the \textbf{Egyptian} media \textbf{quoted} the \textbf{opposition} \textbf{politician} \textbf{Cha}\underline{led} \textbf{Ali}\underline{.}
'\textbf{And} now the word human rights does not even appear in the new \textbf{constitution}\underline{'}, he \textbf{complain}\underline{s} in \textbf{conversation} with the '\textbf{World} on \textbf{Sunday}\underline{'}.
In the deepest winter it was taken out after a long \textbf{fer}\underline{ment}ation and \textbf{consumed} - no doubt with the help of \textbf{alcohol} \textbf{temper}\underline{ed} senses.
In particular, as far as security and economics are concerned, we hope for an interesting and real change that our country so \textbf{urgently} needs.
In Nezahualco\textbf{yo}\underline{t}l, also known as \textbf{Ciudad} Neza, the \textbf{contrast} with the co\textbf{bble}\underline{d} \textbf{streets} of \textbf{Valle} del \textbf{Bra}\underline{vo} could not be greater.
\textbf{Pen}\underline{a} \textbf{Nie}\underline{to}'s \textbf{critics} believe that he has at least not \textbf{adequately} \textbf{addressed} the problem of \textbf{female} \textbf{murder} during his term of office.
"They \textbf{wrote} "\textbf{No} problems" (\textbf{after} meeting the concerns) and that did not \textbf{necessarily} mean that I said nothing at all," Manning said.
An \textbf{ethnic} abbreviation - just as my friends in \textbf{Boston} call themselves "Iren" or my friends in New York "Italy".
Israel has done well in recent years, especially under \textbf{Prime} Minister \textbf{Bin}\underline{ya}min \textbf{Net}\underline{an}yahu, who has \textbf{largely} \textbf{ignored} the peace process.
'In an environment in which we are \textbf{constantly} over-\textbf{sti}\textbf{\underline{mul}}\underline{ated}, it is difficult to get involved when the \textbf{noise} has been \textbf{mu}\underline{ted}.'
But \textbf{Smith} also \textbf{admit}\underline{s} that no place or system can do more than serve as a \textbf{rough} \textbf{guide}\underline{.}
After the vote, he stated that his \textbf{authority} would continue to \textbf{pursue} cases of \textbf{mar}\underline{i}juana \textbf{ownership}\underline{,} mainly to encourage consumers to \textbf{withdraw}\underline{.}
Even before the \textbf{election} day, some local \textbf{municipalities} approved \textbf{mor}\underline{a}\textbf{toria} for new \textbf{mar}\underline{i}juana \textbf{stores}\underline{,} although they could only open in about a year.
We are \textbf{guided} by what the \textbf{municipality} has \textbf{chosen} and not by what the state has \textbf{chosen}\underline{.}
The last time this rate \textbf{exceeded} 2 - also known as the \textbf{replacement} rate - was in \textbf{1976}\underline{.}
"\textbf{It} is important for me to have my own money and time" \textbf{says} another man, about \textbf{twenty} years old.
Or: \textbf{Would} you like to \textbf{publish} a photo of you like the one you published by a \textbf{friend}\underline{?}
"Jemand outside the Internet \textbf{acts} with respect, \textbf{moral}\underline{ity} and other principles, and the same must apply to social networks," he \textbf{explains}\underline{.}
Estu\textbf{ardo} \textbf{Guard}\underline{ia}, \textbf{university} \textbf{professor}\underline{,} \textbf{primary} school \textbf{teacher} and ed\textbf{uc}\underline{ator}, comments that it is essential that \textbf{parents} \textbf{carefully} read the \textbf{guidelines} of social networks.
During the day only the picture of the Presidential \textbf{Meeting} without sound was \textbf{transmitted} in the press room with the message "\textbf{private} \textbf{session}\underline{,} limited \textbf{audio}\underline{".}
We are not dealing with human rights; we do not use that word in this case, but there have been \textbf{constant} \textbf{discussions}\underline{.}
In order to properly \textbf{assess} this progress, it is important to remember that \textbf{Mexican}\underline{s} have an \textbf{average} life expect\textbf{ancy} of \textbf{76} years today.
The first point would mean that international cooperation on in\textbf{sol}\underline{v}\textbf{ency} procedures for companies with a cross-\textbf{border} \textbf{profile} is \textbf{unknown}\underline{.}
The world \textbf{champion} of \textbf{basketball}\underline{,} H xe9\textbf{ctor} "\textbf{He}\underline{tin}" \textbf{Rey}\underline{es}, has been \textbf{associated} with \textbf{basketball} for more than 60 years and has \textbf{visited} the whole world.
\textbf{Fe}\underline{w} in \textbf{Puerto} \textbf{Rico} have such a great \textbf{intellectual} collection of the country's \textbf{basketball} history as H xe9\textbf{ctor} "\textbf{He}\underline{tin}" \textbf{Rey}\underline{es}.
I still know, as he said, that if \textbf{Min}\underline{cy} had allowed a \textbf{championship} for \textbf{Bay}\textbf{\underline{amo}}\underline{n}, Ga\textbf{usse} would make for another.
The \textbf{recording} of five \textbf{chapter}\underline{s} for the second season was \textbf{completed}\underline{,} and a \textbf{sixth} \textbf{chapter} was just \textbf{shot}\underline{,} the \textbf{broadcast}\underline{er} \textbf{informed}\underline{.}
There was no \textbf{immediate} \textbf{explanation} from \textbf{Warn}\underline{er} or T\textbf{NT} about how \textbf{Hag}\underline{mann}'s loss would be \textbf{treated} in the series.
It is important to note that, \textbf{unlike} \textbf{Quebec}\underline{,} US citizens do not have a \textbf{universal} card such as a health \textbf{insurance} card.
You have also \textbf{restricted} the right of \textbf{individuals} and groups to provide assistance to those \textbf{voters} who wish to \textbf{register}\underline{.}
By \textbf{contrast}\underline{,} the whites, which \textbf{represented} 7\textbf{6\%} of the \textbf{electorate}\underline{,} accounted for only 4\textbf{6\%} of the \textbf{voters} who voted in advance.
Most important, however, is to talk to his \textbf{doctor} to \textbf{determine} whether or not he should be carried out.
"\textbf{If} there were no more \textbf{smokers}\underline{,} this would be at least \textbf{50\%} higher," \textbf{emphasized} Andr xe9 \textbf{Beau}\textbf{\underline{lie}}\underline{u}, \textbf{spoke}\underline{s}\textbf{person} for the \textbf{Canadian} \textbf{Canc}\underline{er} \textbf{Society}\underline{.}
The \textbf{announcement} last summer of the \textbf{probable} \textbf{discovery} of the \textbf{Hi}\textbf{\underline{gg}}\underline{s}\textbf{Bo}\underline{son} caused a certain \textbf{stir}\underline{,} and with good reason.
The \textbf{analog}\underline{y} with the \textbf{electromagnetic} field is helpful again to \textbf{explain} the relationship between the \textbf{Hi}\textbf{\underline{gg}}\underline{s} and the mass.
Some, such as \textbf{magnet}\underline{s}, do this, but others do not - for example, a \textbf{piece} of paper would never keep itself on the \textbf{fridge}\underline{.}
\textbf{Where}\underline{ver} he has played, he has \textbf{demonstrated} that he is a great player and a world star.
\textbf{Pierre} No\textbf{iza}\underline{t}, who is also the \textbf{author} of a book about this currency, \textbf{firmly} \textbf{believes} in the potential of this technology as a \textbf{transaction} network.
They want to \textbf{defend} their \textbf{centuries}\underline{-}\textbf{old} and \textbf{arch}\underline{a}ic \textbf{traditions}\underline{,} even if they have been \textbf{joined} by \textbf{j}\textbf{\underline{ih}}\underline{ad}ists, Pakistani, \textbf{Arab}\underline{s}, Uz\textbf{bek}\underline{s} and Ta\textbf{ji}\textbf{\underline{ks}}\underline{.}
Former \textbf{Mu}\underline{ja}\textbf{hed}\underline{in}, the \textbf{Afghan} Government and current \textbf{Taliban} all share a common desire to keep women in a \textbf{subordinate} position.
As I have heard in the \textbf{campaigns}\underline{,} people want a government that is not made up of \textbf{th}\textbf{\underline{ieve}}\underline{s}.
\textbf{About} 6\textbf{5\%} of the population is under 25 years old; Ka\textbf{bul} now has 5 million \textbf{inhabitants}\underline{,} which is one \textbf{fifth} of the total population.
To everyone's \textbf{surprise}\underline{,} he \textbf{announced} on \textbf{Wednesday} that the \textbf{constituent} \textbf{assembly} would adopt its final version the next day.
In line with the military's desire, the \textbf{defence} budget is not submitted to Parliament but to a national \textbf{defence} \textbf{council}\underline{.}
\textbf{Similarly}\underline{,} there will be no ban on civil \textbf{proceedings} in military \textbf{courts}\underline{,} as called for by human rights \textbf{associations}\underline{.}
The \textbf{fifth} \textbf{museum}\underline{,} the \textbf{Holocaust} Museum or \textbf{Ya}\underline{d} \textbf{Va}\underline{s}\textbf{hem} in \textbf{Tel} A\textbf{viv}\underline{,} \textbf{tells} about one of the most \textbf{shock}\underline{ing} \textbf{chapter}\underline{s} in history.
In \textbf{Caesar}\underline{e}a, the city of \textbf{King} \textbf{Hero}\underline{des}, you can walk through the Roman \textbf{theatre} and \textbf{conquer} the \textbf{fortress} of the \textbf{cru}\underline{s}aders.
If you travel to Israel, don u2019t \textbf{worry} about your poor knowledge of English: \textbf{approximately} \textbf{30\%} of \textbf{Israelis} speak Russian.
A \textbf{rental} car costs between \$ \textbf{37} per day (Hyundai \textbf{Get}\underline{z}) and \$ 188 (A\textbf{udi} A6, \textbf{Volvo} S80).
That is more than \textbf{twice} the cost of the official test: it costs a work \textbf{immigrant} three \textbf{thousand} \textbf{rub}\underline{les}.
The first \textbf{channel} is the \textbf{army} or the military, that is, \textbf{weapons} \textbf{stolen} during the \textbf{fighting} in the \textbf{Caucasus}\underline{.}
The \textbf{Federal} Security Service has recently \textbf{launched} a number of fake \textbf{websites}\underline{,} and \textbf{buyer}\underline{s} who want to buy \textbf{weapons} are getting into the network.
The \textbf{Federal} Security Service has recently \textbf{launched} a number of fake \textbf{websites}\underline{,} and \textbf{buyer}\underline{s} who want to buy \textbf{weapons} are getting into the network.
No one can \textbf{predict} yet whether the \textbf{protests} will increase even further or whether they will soon be out of the air.
The \textbf{movements} of human \textbf{beings} are extremely \textbf{dynamic} and \textbf{frankly}\underline{,} the current 30 fps are not enough, especially for \textbf{gesture}\underline{s}.
In 2000 there was a press \textbf{survey} about the "\textbf{Per}\underline{son}alities of our City" \textbf{award}\underline{.}
- \textbf{Recently} we \textbf{saw} you in the role of the \textbf{urban} \textbf{organ} player - A cultural city should have such a hero.
For cultural reasons there are 300 people and not 10 \textbf{thousand}\underline{,} so there is less management, money, and everything is \textbf{dying}\underline{.}
While for a new\textbf{born} child, \textbf{gravity}\textbf{\underline{lessness}} is a much more natural state, the \textbf{woman} cannot do without \textbf{gravity}\underline{.}
In this respect, it should be \textbf{noted} that those countries that are a model for us also have problems to \textbf{contend} with.
As far as Czech legislation is concerned, how important it was for your \textbf{authority} to \textbf{revise} the \textbf{procurement} law, do you already feel any impact?
I think that this law is certainly a step in the right direction and I hope that it will be \textbf{confirmed}\underline{.}
The D5 \textbf{motorway} can be reached \textbf{practically} without any \textbf{restrictions}\underline{.}
The second and third class \textbf{tracks} are \textbf{hum}\underline{id} and therefore there is also a reference to possible \textbf{blocked} \textbf{sections}\underline{.}
After the use of \textbf{sc}\textbf{\underline{atter}}\underline{ing} \textbf{vehicles} \textbf{snow} \textbf{mat}\underline{s} remain on the   u20\textbf{47} erveno\textbf{hor}\underline{sk} xe9 sedlo pass and on the road in the direction of Videlsk  u20\textbf{47}  k  u20\textbf{47}  xed  u20\textbf{47} .
For this we want to take advantage of the marketing potential of the \textbf{Maya}\underline{n} \textbf{Cal}\underline{en}\textbf{dar}\underline{,} which is projected to end at 11:10 a.m. on 21 December.
The day before, that is, on 20 December, three \textbf{concerts} will take place \textbf{simultaneously} from 21:00 in \textbf{Prague}\underline{,} \textbf{Brno} and \textbf{Ost}\underline{r}\textbf{ava}\underline{.}
Since the students themselves do not have the resources to visit the \textbf{teachers}\underline{,} we want to help them in this way.
In \textbf{Prague}\underline{,} for example, Chinaski, support \textbf{Les}\textbf{\underline{bian}}\underline{s}, \textbf{Il}\textbf{\underline{lust}}\underline{r}\textbf{ato}\textbf{\underline{sphere}} with \textbf{Dan} B xe1rta, The \textbf{Tap} \textbf{Tap}\underline{,} \textbf{Mari} xe1n \textbf{Ban}\underline{go} and \textbf{Ji}  u20\textbf{47}  xed Such  u20\textbf{47}  appear.
\textbf{Well}\underline{,} and over time, as our \textbf{mode}\underline{r}ator, L xe1  u20\textbf{47} a \textbf{Angel}\textbf{\underline{ovi}}  u20\textbf{47} , used to say, this is something out of control (la\textbf{ugh}\underline{s}).
However, this compassion is absolutely \textbf{unnecessary}\underline{,} because people with \textbf{disabilities} are not lonely and \textbf{abandoned} \textbf{beings} that we should \textbf{regret}\underline{.}
Even before the \textbf{Second} World War, \textbf{Polish} cos\textbf{mos}\underline{-}\textbf{lov}\underline{ers} were already \textbf{engaged} in space, but they did not always understand it.
In \textbf{1934}   u20\textbf{47} \textbf{tern}\underline{feld} won the \textbf{Prix} \textbf{RE}\underline{P}-Hirsch donated by \textbf{Robert} Esn\textbf{ault}\underline{-}Pel\textbf{terie} and Andr xe9 \textbf{Louis} \textbf{Hirsch}\underline{.}
\textbf{Short}\underline{ly} before the war, all projects for military use of \textbf{missile} technology were \textbf{coordinated} by the \textbf{Ty}\underline{m}\textbf{cz}\underline{as}owy Committee of Dorad\textbf{cz}\underline{o}-Nau\textbf{kow}\underline{y}.
The \textbf{missile} with a maximum \textbf{altitude} of \textbf{1800} m was about 80 \textbf{cm} long and \textbf{weigh}\underline{ed} not quite 5 \textbf{kg}\underline{.}
The aim of these measures is to force its own people to accept the \textbf{dictate}\underline{s} of private capital, particularly in the area of \textbf{wages}\underline{.}
The result, as it was then, is an \textbf{unprecedented} \textbf{decade}\textbf{\underline{nce}} of the \textbf{elite}\underline{s} who are not at all committed to \textbf{deeper} reform.
In November \textbf{1979}\underline{,} a mob of \textbf{demonstrating} \textbf{Islamist} students \textbf{occupied} the US \textbf{embassy} in Te\textbf{hra}\underline{n} and held \textbf{52} \textbf{diplomats} \textbf{hostage}\underline{.}
The deba\textbf{cle} in Iran \textbf{contributed} \textbf{significantly} to \textbf{Jim}\textbf{\underline{my}} Carter u2019s \textbf{defeat} against \textbf{Ronald} \textbf{Reagan} in the \textbf{1980} \textbf{presidential} \textbf{election}\underline{.}
Af\textbf{fleck} and his team also have a similar effect on \textbf{fi}\textbf{\underline{ct}}\underline{it}\textbf{ious} \textbf{scenes} (the wrong film \textbf{wand} on a \textbf{ba}\underline{za}ar in Te\textbf{hra}\underline{n}).
The EU called for an American study which, according to air \textbf{balloon}\underline{s}, is the leading cause of child s\textbf{uff}\textbf{\underline{oc}}\underline{ation}.
As a simple \textbf{citizen}\underline{,} I have worked to ensure that the travel \textbf{guide} remains a free trade, and this has been achieved.
\textbf{Poli}\underline{tic}\textbf{ians}\underline{,} \textbf{journalists} and the public to \textbf{convince} and try to get them on our side in order to achieve these objectives.
I believe they are still \textbf{playing} their part, but they are on the way to a more '\textbf{normal}\underline{'} foreign policy.
Even if they do not like it, it is \textbf{unpleasant} to them and makes them much more unpop\textbf{ular} - c'est la vie!
The \textbf{Volvo} \textbf{buyer} Geely \textbf{originally} used a \textbf{blue}\underline{-}\textbf{white} \textbf{logo} that \textbf{reminded} \textbf{BMW}\underline{;} the \textbf{dispute} was \textbf{settled}\underline{,} Geely had to change it.
Last year CTMO received more than \textbf{1.4} million \textbf{trademark} protection applications, almost a third more than in \textbf{2010.}
Fifty \textbf{singer}\underline{s} have \textbf{arrived}\underline{,} between 23 and \textbf{69} years old, from the human \textbf{genetic}\underline{ist} to the houseman.
This is not a for\textbf{ego}\underline{ne} conclusion, because as \textbf{obvious} as the \textbf{disease} is throughout the country, it is \textbf{prefer}\underline{able} to keep it \textbf{silent}\underline{.}
The name Trifid derives from the \textbf{Latin} word \textbf{tri}\underline{fi}dus (three \textbf{divided}\underline{,} three-\textbf{col}\underline{um}ns), because \textbf{dark} \textbf{dust} \textbf{strip}\underline{s} three-\textbf{part} the \textbf{glo}\textbf{\underline{wing}} heart of the \textbf{starb}\underline{ur}st.
The K\textbf{eck}\underline{-}T\textbf{ele}\textbf{\underline{sko}}\underline{pe} are part of the Ma\textbf{una}\underline{-}Kea ob\textbf{serv}\textbf{\underline{atory}}\underline{,} which \textbf{looks} out into the \textbf{sky} with the \textbf{Sub}\underline{ar}u \textbf{Tele}\textbf{\underline{scope}} and the I\textbf{RT}\textbf{\underline{TF}}\underline{.}
The \textbf{legendary} \textbf{wealth} that the country \textbf{owe}\underline{s} to its oil in the Caspian Sea has not yet \textbf{arrived} here in the \textbf{province}\underline{.}
Many \textbf{ve}\underline{il}ed women and \textbf{Sala}\underline{f}ists took part in it and \textbf{shout}\underline{ed}: 'The people are \textbf{calling} for the application of God's law.'
A \textbf{battle} for \textbf{sovereignty} over the \textbf{symbolic} Tahrir \textbf{Square}\underline{,} where everything began, would have \textbf{provoke}\underline{d} civil war-\textbf{like} conditions.
Even from \textbf{Sweden}\underline{,} the old \textbf{rival} who was not so long ago much richer than \textbf{Norway}\underline{,} \textbf{immigrants} are \textbf{flow}\underline{ing}.
\textbf{Op}\underline{in}\textbf{ions} on the new \textbf{Head} of State are \textbf{divided} in this densely \textbf{populated} and extensive part of the country \textbf{surrounding} the capital.
"I hope that as \textbf{president} he is as he was as \textbf{governor}\underline{,}" \textbf{says} the \textbf{PRI} \textbf{Congress}\underline{man} \textbf{Ol}\underline{ver}a in \textbf{Valle} del \textbf{Bra}\underline{vo}.
It \textbf{wants} to \textbf{unite} with the United States and \textbf{Canada} and create a North American trade \textbf{bloc} modelled on the European Union.
\textbf{Mexico} has \textbf{winners} and losers, people for whom it offers opportunities and others for whom it does not.
\textbf{Expert}\underline{s} say that the \textbf{catch} in the \textbf{popularity} of social media lies with the very population to which the plan is \textbf{directed}\underline{.}
British American To\textbf{bac}\underline{co} \textbf{Australia} \textbf{says} that, instead of marketing, industry is \textbf{concentrating} on dealing with the new laws.
\textbf{Professor} Larson \textbf{says} today, 21 years later, that he does not know if the \textbf{percentage} of \textbf{bo}\underline{re}\textbf{dom} has risen or fallen.
\textbf{Hund}\underline{red}s of \textbf{irregularities} around \textbf{mar}\underline{i}juana are already being \textbf{dropped} here and in the State of \textbf{Washington}\underline{,} which approved similar measures.
The police in Grand \textbf{Ju}\underline{n}\textbf{ction}\underline{,} the largest city in the \textbf{county}\underline{,} no longer show \textbf{adults} for \textbf{holding} \textbf{smaller} \textbf{quantities}\underline{.}
I \textbf{experienced} that the \textbf{tut}\underline{ors} not only du\textbf{ped} the m\textbf{ock}\underline{ing} of Tory students, but also \textbf{enjoyed} \textbf{participating} in it.
The three years that were before me \textbf{stretch}\underline{ed} before my \textbf{mental} \textbf{eye} into a fencing \textbf{fire} of \textbf{ost}\textbf{\underline{rac}}\underline{ism} and \textbf{isolation}\underline{.}
Many years ago we \textbf{went} home for \textbf{dinner} after a \textbf{fashion} show in \textbf{Piazza} di Spa\textbf{gna} in \textbf{Rome}\underline{.}
It was a red \textbf{dress} with \textbf{flying} skirt and a covered \textbf{upper} with a de\textbf{col}\underline{let} xe9 that \textbf{honour}\underline{s} his name.
Anto has asthma, \textbf{breath}\underline{es} with \textbf{difficulty}\underline{,} husts \textbf{frequently} and his \textbf{eyes} are \textbf{ir}\textbf{\underline{rit}}\underline{ated} by \textbf{toxic} \textbf{gases} from the \textbf{volcano}\underline{.}
With the \textbf{basket} on its back, Un\textbf{ain}\underline{ik} with its \textbf{53} years is only able to carry 50 \textbf{kg}\underline{.}
"The social networks are \textbf{entertaining}\underline{,} I can talk quickly with relatives in the distance or with friends" he \textbf{says}\underline{.}
The \textbf{hosting} President Oll\textbf{anta} \textbf{Hum}\textbf{\underline{ala}} \textbf{opened} the morning \textbf{discussions} and \textbf{ended} the summit in \textbf{Lima} \textbf{shortly} after \textbf{lunch}\underline{.}
If I were to \textbf{win}\underline{,} it would be my last term as President, after which I \textbf{withdraw} from public life.
The state is in the \textbf{fourth} place in national terms of new and \textbf{accumulate}\underline{d} cases of \textbf{AIDS}\underline{,} and in the 13th place in relation to \textbf{HIV}\underline{.}
\textbf{Victoria} \textbf{Principal}\underline{,} co-\textbf{present}\underline{er} of the original series, \textbf{remembered} \textbf{Hag}\underline{man} on \textbf{Friday} as an "e\textbf{norm}\underline{ous} \textbf{personality} on and outside the screen".
After the liver trans\textbf{plant} he worked for liver \textbf{donation}\underline{s} and worked as a \textbf{volunteer} in a \textbf{hospital} to help \textbf{scar}\underline{ed} \textbf{patients}\underline{.}
"I \textbf{advise} them, give them \textbf{courage}\underline{,} I meet with them when their \textbf{operations} are about to take place and after," he \textbf{explained} in 1996.
\textbf{Every} week, students \textbf{investigate} apocaly\textbf{ptic} issues such as nuclear war, \textbf{zo}\underline{mb}ies, \textbf{virus} and ge\textbf{rm}\underline{s}, and global \textbf{warming}\underline{.}
\textbf{Every} week, students \textbf{investigate} apocaly\textbf{ptic} issues such as nuclear war, \textbf{zo}\underline{mb}ies, \textbf{virus} and ge\textbf{rm}\underline{s}, and global \textbf{warming}\underline{.}
The \textbf{Maya}\underline{s} never \textbf{predicted} the end of the world; it is only a key point in the \textbf{calendar}\underline{,} said Re\textbf{stall}\underline{.}
"I may call a \textbf{couple} of friends so that we can \textbf{laugh} together," said \textbf{Sam}\textbf{\underline{ira}} \textbf{Ford}\underline{,} a 20-\textbf{year}\underline{-}\textbf{old} \textbf{student} of communication.
For example, \textbf{electoral} \textbf{registration} \textbf{campaigns} in the 2004 general \textbf{election} \textbf{helped} to \textbf{register} some 10 million citizens.
It is \textbf{estimated} that \textbf{30\%} of \textbf{cancer}\underline{s} could be \textbf{prevented} if everyone \textbf{eat}\underline{s} well and \textbf{moved} \textbf{sufficiently}\underline{.}
For the \textbf{Canadian} \textbf{cancer} society, the fight against \textbf{tobacco} \textbf{dependence} remains a priority, despite the \textbf{decline} in the number of \textbf{smokers}\underline{.}
However, it is important to point out that these \textbf{Bos}\underline{ons} are not all as \textbf{exotic} \textbf{creature}\underline{s} as one might think.
The impact of this research on the general public is more difficult to \textbf{predict}\underline{,} but it would be wrong to \textbf{assume} that there are \textbf{none}\underline{.}
"In the course of our lives, we learn that a man is \textbf{standing} \textbf{pink}\underline{,}" \textbf{says} \textbf{Pierre} \textbf{Bro}\underline{de}ur, \textbf{psycho}\textbf{\underline{logist}} at \textbf{Victor}\underline{-}\textbf{Ga}\textbf{\underline{db}}\textbf{\underline{ois}} Home.
But that does not \textbf{necessarily} mean 'I want you to \textbf{sleep} me', but 'I want my \textbf{pain} to be \textbf{ease}\underline{d}'.
By the way, there have been strong \textbf{charges} against \textbf{engineers} from the \textbf{Montreal} \textbf{Road} Transport \textbf{Authority}\underline{,} as well as \textbf{entrepreneurs} of Italian origin, such as \textbf{Tony} \textbf{Ac}\textbf{\underline{cur}}\underline{so} and Lino \textbf{Za}\underline{mb}\textbf{ito}\underline{.}
The \textbf{latter} has caused a \textbf{stir} by de\textbf{cla}\underline{ring} to the Commission the \textbf{functioning} of the 'system' for \textbf{obtaining} public \textbf{contracts}\underline{.}
First of all, we want to be the first of our group before \textbf{Porto}\underline{,} so that we can take the return of the \textbf{eight}\underline{h} final as a home game.
The \textbf{transaction} is therefore \textbf{permanently} linked to the \textbf{chain} of all other \textbf{transactions}\underline{,} and any \textbf{modification} would change the \textbf{fingerprint}\underline{.}
"T\textbf{hir}\underline{d} \textbf{thousand} \textbf{dollars} have been exchanged," \textbf{says} Jon \textbf{Hol}\underline{m}quist, who works for Coina\textbf{bul}\underline{,} which \textbf{convert}\underline{s} \textbf{Bit}\underline{co}ins into \textbf{gold}\underline{.}
Tolerated, sometimes supported by local in\textbf{sur}\textbf{\underline{gent}}\underline{s}, the \textbf{latter} will no longer be there if Western countries become more \textbf{discreet}\underline{.}
During their \textbf{exile} in Iran or Pakistan, they have had contact with the modern world and \textbf{enjoyed} its benefits.
In a country \textbf{ruin}\underline{ed} by 30 years of war, state control of infrastructure would have been necessary.
In addition, no more \textbf{article} \textbf{refers} to the protection of women, unders\textbf{core}\underline{s} Heba \textbf{Mora}\underline{y}\textbf{ef} of Human Rights \textbf{Watch}\underline{.}
In \textbf{Caesar}\underline{e}a you should visit the unique private Ra\textbf{lli} Museum where you can \textbf{admire} \textbf{sculpture}\underline{s} by Dali and \textbf{Rod}\underline{in}.
In Roman times, \textbf{Caesar}\underline{e}a was the most important city of \textbf{Jud}\underline{e}a and \textbf{residence} of the Roman \textbf{governor}\underline{s}, including \textbf{Pont}\textbf{\underline{ius}} \textbf{Pil}\underline{at}us.
\textbf{Up} to now, this regulation only applies to \textbf{migrants} who want to work in the services sector, in local \textbf{housing} and in the \textbf{retail} sector.
It is not only language \textbf{tests} that must be carried out, but also \textbf{tests} in Russian history and the \textbf{foundations} of legislation.
On the other hand, before the law enters into force, civil rights \textbf{activists} asked the following question several times in the press: what is the point?
In addition, newcomers without knowledge of languages are offered places where there is no need for active understanding with people.
"\textbf{There} is an own, sometimes hand\textbf{craft}\underline{ed} production as well as a \textbf{mafia} that \textbf{organize}\underline{s} the \textbf{smuggling}\underline{,}" \textbf{explains} the former military member.
"\textbf{You} only need the right amount of money," \textbf{says} the \textbf{ad} on the website "\textbf{Bu}\underline{y} \textbf{gun} or \textbf{ri}\textbf{\underline{fle}}\underline{".}
I have heard about the following \textbf{scheme}\underline{:} the website is \textbf{normally} \textbf{registered} \textbf{abroad} and Russian laws are not \textbf{applicable}\underline{.}
The U.S. law for\textbf{bid}\underline{s} \textbf{corporate} \textbf{governance} from \textbf{standing} in the way of this objective and from \textbf{warning} or s\textbf{ack}\underline{ing} \textbf{union} members.
It encourages the possibility of \textbf{manipulat}\underline{ing} \textbf{virtual} \textbf{objects} in the air with simple \textbf{hands} and creating \textbf{virtual} open \textbf{spaces}\underline{.}
- We deal with the \textbf{interaction} of man and machine, but want to \textbf{expand} the \textbf{limits} of this \textbf{interaction}\underline{.}
This can be \textbf{laser} \textbf{sensors}\underline{,} for example, because they offer a good resolution in \textbf{depth}\underline{,} which is very important.
From this point of view, all current technologies are not good enough for us, as the \textbf{developers} of the \textbf{algorithm}\underline{s} have more work.
Not only the resolution along the X and Y \textbf{axis} but also along the Z \textbf{axis} must be taken into account.
\textbf{Ros}\textbf{\underline{bal}}\underline{t} \textbf{continues} the "\textbf{Peter}\textbf{\underline{sburg}} a\textbf{vant}\underline{-}\textbf{garde}\underline{"} project \textbf{dedicated} to \textbf{urban} \textbf{residents} who make up the a\textbf{vant}\underline{-}\textbf{garde} of art and culture.
We have very few cosmon\textbf{aut}\underline{s} who, after long \textbf{flights}\underline{,} have all \textbf{gone} well and had \textbf{healthy} young people.
\textbf{Yet} \textbf{humanity} must look for new \textbf{paths} in \textbf{biotechnology}\underline{,} \textbf{radiation} protection and \textbf{artificial} \textbf{gra}\textbf{\underline{vit}}\underline{ation}.
Even if \textbf{adults} feel that water is pleasant, it is a foreign environment, but \textbf{infant}\underline{s} feel that water is a natural \textbf{element}\underline{.}
The Czech Republic has good \textbf{supervisory} authorities and \textbf{adequate} laws in connection with public \textbf{contracts}\underline{,} but falls behind in their application.
Noc\textbf{turn}\underline{al} \textbf{snow}\underline{s}torms \textbf{forced} the road \textbf{rid}\underline{ers} to use it. \textbf{According} to information from the road authorities about 3 \textbf{cm} of new \textbf{snow} \textbf{fell} in   u20\textbf{47} umperk \textbf{County}\underline{.}
We also \textbf{cooperate} with other personalities of the Czech cultural \textbf{scene}\underline{,} which is related to the fact that we \textbf{organize} many \textbf{charity} events and \textbf{concerts}\underline{...}
As part of the \textbf{completion} of the Jedli  u20\textbf{47} \textbf{ka} \textbf{Institute}\underline{,} a separate building is to be created, which we will then move into with this project.
And since I am a musician \textbf{myself} and play saxo\textbf{phone}\underline{,} among other things, I \textbf{founded} a music company with a \textbf{colleague}\underline{.}
This is \textbf{logical} in its own way, because everything new is considered with \textbf{caution} and will only be accepted after a long time.
They are people who can live a full life and develop if they have the means to do so.
Was it also helpful for this success that you are a \textbf{strict} \textbf{boss}\underline{,} as many people say?
It is not even clear whether the \textbf{rocket} should be used to \textbf{launch} or \textbf{brake} the \textbf{Dra}\underline{is}ine.
The following year the first P\textbf{TA} \textbf{chairman}\underline{,} Kazimierz \textbf{Za}\textbf{\underline{rank}}\underline{ie}\textbf{wi}\textbf{\underline{cz}} (1902 - \textbf{1959}\underline{),} became \textbf{Deputy} \textbf{Chairman} of the International \textbf{Federation} for \textbf{Space}\underline{.}
\textbf{Later} an improved version, the \textbf{RM}\underline{-1}A, was built, and in \textbf{1959} \textbf{flight} \textbf{tests} with the \textbf{RM}\textbf{\underline{-2}} two-stage \textbf{rocket} began in the B  u20\textbf{47} d xf3w \textbf{desert}\underline{.}
The \textbf{Met}\underline{e}or-1A \textbf{rocket} had a transport room with \textbf{0.4} \textbf{lit}\underline{res} capacity, meteor-1B with 0.\textbf{34} \textbf{lit}\underline{res} and meteor-1C with 0.\textbf{62} \textbf{lit}\underline{res}.
The \textbf{Met}\underline{e}or 2 \textbf{rocket} was developed in the \textbf{aviation} \textbf{institute} between \textbf{1965} and \textbf{1968}\underline{.} The first \textbf{flight} \textbf{tests} began in October \textbf{1970}\underline{.}
After the last \textbf{wave} of violence between Israel and \textbf{Gaza}\underline{,} there were, as always, \textbf{countless} \textbf{reactions}\underline{.}
The \textbf{diplomats} \textbf{arrested} were finally \textbf{released} after 4\textbf{44} days after negotiations were mediated by the \textbf{Algeria}\underline{n} Government.
The \textbf{director} also had to face up to the fact that history does not actually offer many \textbf{exciting} \textbf{scenes} in the \textbf{cinema}\underline{tic} sense.
As the Czech Republic has another way to reach sea \textbf{ports}\underline{,} \textbf{Pala}\underline{s} \textbf{says} that the EU should pay us \textbf{hundreds} of \textbf{millions} of \textbf{euros}\underline{.}
But when I see something that I do not like, I try to \textbf{propose} a solution to change that.
But my goal is not the function; it is an instrument with which I can \textbf{realize} my \textbf{vision}\underline{s}.
As an independent partyless, I have much greater potential to \textbf{gain} support from all the parties \textbf{represented} in Parliament.
It is not a question of whether \textbf{someone} \textbf{belongs} to the left or right \textbf{camp}\underline{;} I want to \textbf{connect} people.
I have just started with \textbf{politics} and I am trying to get the support of the majority for my programme.
The reason: At the opening a few weeks ago, each \textbf{resident} was \textbf{invited} to donate a book from his own personal collection.
So they cannot be part of a \textbf{broader} line and must instead take things forward from their own position.
This \textbf{conceal}\underline{s} an official designation in China, which has nothing to do with the original companies.
\textbf{Both} he and \textbf{Pat}\underline{t}\textbf{loch} \textbf{advise} German companies to be very \textbf{careful} when dealing with China.
First of all there is \textbf{st}\textbf{\underline{ump}}\underline{ing}: \textbf{cow}\textbf{\underline{boy}} \textbf{boot}\underline{s}, \textbf{basketball} \textbf{shoes}\underline{,} ladies \textbf{pump}\underline{s} and men's \textbf{li}\textbf{\underline{pper}}\underline{s} are looking for the \textbf{clock} on the par\textbf{quet} floor, they find it quickly.
It is \textbf{Monday} evening, in the music room of the \textbf{Institute} for \textbf{Medical} \textbf{Psycho}\textbf{\underline{logy}} in \textbf{Heidelberg}\underline{,} the \textbf{choir} Im\textbf{bon}\underline{gi} is trying a new \textbf{song}\underline{.}
There are around \textbf{34} million people \textbf{infected} with \textbf{HIV} worldwide, \textbf{estimated} by Un\textbf{aid}\underline{s}, the United Nations programme to combat \textbf{AIDS}\underline{.}
\textbf{Through} \textbf{sponsor}\underline{ship}s, \textbf{donation}\underline{s} and, not least, the \textbf{ga}\underline{g}s that the \textbf{choir} \textbf{sing}\underline{s} all over Germany, a lot of things come together.
Although it is difficult to find the small village on \textbf{maps}\underline{,} it is more than known in the \textbf{valley} of the Ezul\textbf{wen}\underline{i} \textbf{river}\underline{.}
Unn\textbf{otic}\underline{ed} by \textbf{Earth}\underline{'}s citizens, pro\textbf{bes}\underline{,} \textbf{telescope}\underline{s} and small \textbf{robots} like \textbf{Phoenix} are \textbf{exploring} the \textbf{depth}\underline{s} of space.
Even this star \textbf{cloud}\underline{,} \textbf{connected} with the \textbf{Rose}\underline{t} Ne\textbf{bul}\underline{a}, \textbf{constantly} \textbf{produces} new \textbf{infant} \textbf{stars} - \textbf{5000} light years away from the \textbf{Earth}\underline{.}
Researchers suggest that it was created only \textbf{shortly} after the \textbf{Big} Bang, when \textbf{hydrogen} was \textbf{predominant}\underline{ly} found in the \textbf{universe}\underline{.}
One of the \textbf{tasks} of the \textbf{telescope} is to search for light from the first \textbf{stars} and \textbf{galaxies} for the big bang.
\textbf{Sc}\textbf{\underline{ient}}\underline{ists} now have \textbf{certainty} with the \textbf{Messenger} \textbf{probe} \textbf{launched} in \textbf{2004.}
\textbf{Mir}\underline{za}y\textbf{eva}\underline{,} who \textbf{claims} to have 143 \textbf{descendants}\underline{,} lives in a simple \textbf{wooden} house \textbf{typical} of the whole \textbf{Caucasus} region.
\textbf{Eight} people live here under one \textbf{roof}\underline{,} including one of \textbf{Mir}\underline{za}y\textbf{eva} u2019s \textbf{son}\underline{s} and a \textbf{daughter}\underline{,} both of whom have long been \textbf{grand}\textbf{\underline{parent}}\underline{s}.
"When he calls the \textbf{referendum}\underline{,} we will go to his \textbf{palace} and over\textbf{turn} him," said the \textbf{opposition}\underline{ist} Ja\textbf{sser} Said.
Now is the time to let the people decide at the \textbf{ballot} \textbf{box} which direction the country should go.
There are \textbf{snow}\underline{,} \textbf{spectacular} \textbf{landscapes} - and this \textbf{st}\underline{ub}\textbf{born} \textbf{smell} in the air that simply does not want to \textbf{disappear}\underline{.}
But in fact everything here is \textbf{expensive} - a small \textbf{glass} of beer or a \textbf{sandwich} costs a \textbf{proud} 10 \textbf{euros}\underline{.}
\textbf{Norwegian}\underline{s} find it difficult to accept that \textbf{someone} in their peace-\textbf{lov}\underline{ing} country is \textbf{capable} of such \textbf{brutal} \textbf{murder}\underline{s}.
The forms, he said, did not \textbf{contain} \textbf{complaints} about maltreatment, even though \textbf{officials} had questioned Manning directly about his treatment.
Manning \textbf{replied} that his \textbf{intention} during this meeting was to down\textbf{grade} his \textbf{observation} status to '\textbf{pre}\textbf{\underline{vention}} of \textbf{injuries}\underline{'}.
But for \textbf{Mexican}\underline{s} who think in \textbf{centuries} and not minutes, \textbf{memories} of this event cannot be \textbf{overlooked}\underline{.}
They see us as a reme\textbf{mbra}\textbf{\underline{nce}} of a \textbf{hum}\textbf{\underline{ili}}\underline{ating} \textbf{defeat} and look down on us because we are not \textbf{Mexican} enough.
But many \textbf{Mexican} \textbf{Americans} I know have the \textbf{feeling} that they are not part of either country.
But, while \textbf{Israelis} and \textbf{Palestinians} \textbf{seem} tra\textbf{pped} in their historical conflict, the Middle East around them is \textbf{changing}\underline{.}
Even if the \textbf{cease}\underline{-}\textbf{fire} agreed on 21 November lasts, this week's \textbf{fighting} has \textbf{strengthened} the hard people on both \textbf{sides}\underline{.}
\textbf{Hard}\underline{lin}ers may be able to \textbf{win} the day, but the \textbf{Arab} \textbf{Spring} may be a \textbf{stroke} for them.
If it is up to them, it is \textbf{ok} for us - and our children - to be sometimes \textbf{bo}\underline{red}.
If you are \textbf{bo}\underline{ring} and you use this energy to play and \textbf{cook} \textbf{guitar}\underline{,} you will be happy.
But \textbf{prosecutor}\underline{s} in \textbf{Color}\textbf{\underline{ados}} u2019 more \textbf{conservative} \textbf{districts} have \textbf{announced} that they will continue to \textbf{pursue} existing \textbf{mar}\underline{i}juana \textbf{offences} and still \textbf{quote} people in \textbf{court}\underline{.}
It was an English \textbf{student} from the second year called \textbf{James} who \textbf{imagine}\underline{d} \textbf{himself} as a member of the \textbf{conservative} \textbf{student} \textbf{association}\underline{.}
\textbf{Every} detail of his apartment, \textbf{decoration}\underline{,} food and music \textbf{recognized} and \textbf{felt} his influence.
Since the elections, an \textbf{attempt} has been made to correct the problem by increasing \textbf{contributions} and le\textbf{vie}\underline{s} on foreign workers.
They are so popular, and \textbf{units} are \textbf{sold} out by days and even weeks \textbf{faster} than larger \textbf{units}\underline{.}
"I wouldn't share a photo that isn't \textbf{mine}\underline{,} or of \textbf{someone} who makes a \textbf{stupid} head," he \textbf{says}\underline{.}
"\textbf{If} \textbf{someone} \textbf{har}\textbf{\underline{asse}}\underline{s} me or asks me to \textbf{remove} it from my user account," he \textbf{admit}\underline{s}.
\textbf{Another} point is to make them understand that they must act online, as they do \textbf{offline}\underline{.}
On the official website of the \textbf{ASP}\underline{A} you can see that the document was published last \textbf{Tuesday}\underline{.}
Cor\textbf{rea} \textbf{assured} that if he lost the February \textbf{2013} elections, he would \textbf{withdraw} from political life.
At that time, even the \textbf{director} of a \textbf{IM}\textbf{\underline{SS}} \textbf{clinic} \textbf{avoided} saying goodbye 'because it led to a \textbf{dead} end'.
His \textbf{films} included well-re\textbf{garde}\underline{d} roles in "The Group", "\textbf{Har}\underline{ry} and \textbf{Ton}\underline{to}" and "\textbf{Pri}\underline{m}ary \textbf{Color}\underline{s}".
\textbf{Ten} \textbf{episode}\underline{s} of the new issue of "\textbf{Da}\textbf{\underline{lla}}\underline{s}" were aired a few months ago with great success in the TV \textbf{channel} T\textbf{NT}\underline{.}
"The \textbf{Philippines} do not \textbf{participate} at the end of the world," he \textbf{wrote} as an allusion to an \textbf{exception} of a higher instance.
In 10 years, \textbf{Republican} \textbf{lawyers} have only \textbf{recorded} 300 cases of \textbf{electoral} \textbf{fraud} in the United States.
As a result, \textbf{180} legislative proposals were introduced in \textbf{2011} alone, \textbf{restrict}\underline{ing} the exercise of the right to vote in \textbf{41} states.
Since \textbf{2011}\underline{,} a \textbf{dozen} states have \textbf{passed} laws \textbf{requiring} \textbf{voters} to \textbf{prove} their US \textbf{citizenship}\underline{.}
"The research shows that regular \textbf{physical} activity protects against w\textbf{rath} \textbf{cancer} throughout life," he \textbf{adds}\underline{.}
But for \textbf{phy}\underline{s}icists it is still not \textbf{entirely} certain that it is really the \textbf{Hi}\textbf{\underline{gg}}\underline{s}.
In one \textbf{corner} are the good citizens, who are called \textbf{Fer}\underline{mi}one, and who follow the \textbf{Paul}\underline{i} principle.
In fact, not all p\textbf{article}\underline{s} and not all materials \textbf{interact} with the \textbf{electromagnetic} field.
There is currently no \textbf{comparable} person in Li\textbf{gue} 1 and he is one of the best trainers in Europe.
One of our most important \textbf{goals} is the \textbf{Champion}\underline{s} \textbf{League}\underline{:} in this way we \textbf{qualified} for the 8th final.
The \textbf{opposite} of the current \textbf{monetary} exchange based on central banks, \textbf{identified} \textbf{transactions} and processing \textbf{fees} between the parties.
\textbf{Nevertheless}\underline{,} the European Central Bank (ECB) has shown an interest in this in a report on \textbf{virtual} \textbf{currencies} published in October.
With the \textbf{difference} that the user can choose a different address for each payment, which \textbf{ensures} \textbf{anonym}\underline{ity}.
The system can be easily implemented by the \textbf{vendor}\underline{s} and the \textbf{latter} do not need to \textbf{install} new \textbf{terminal}\underline{s} or computer programs.
There is a general \textbf{trend} in reviewing hier\textbf{arch}\underline{ical} systems in favour of more \textbf{horizontal} systems.
They have brought themselves into disre\textbf{put}\underline{e} and most of them have not been involved in the \textbf{fighting}\underline{.}
This \textbf{reinforce}\underline{s} the \textbf{impression} that the Western countries were only there to \textbf{seize} it.
Just a week ago, the \textbf{Head} of State \textbf{gave} this \textbf{plenary} two additional months to complete his work.
Israel u2019s three main \textbf{recreational} areas are on the \textbf{shores} of the Mediterranean, the Red Sea and the Dead Sea.
\textbf{Fort}\textbf{\underline{una}}\underline{,} according to \textbf{legend}\underline{,} should be held by all who touch the \textbf{walls} in the alley with their sign.
What changes does the \textbf{requirement} to have language \textbf{skills} mean, both for Russians and for \textbf{migrant} workers?
"They want one or two \textbf{hundred} \textbf{rub}\underline{les} for \textbf{cigarette}\underline{s} and \textbf{tea}\underline{,}" \textbf{says} the Ta\textbf{ji}\underline{k} Umed Hu\textbf{zh}\underline{k}ada\textbf{mov} to \textbf{journalists}\underline{.}
\textbf{Expert}\underline{s} \textbf{calculated} how much each of the five \textbf{channels} has about to \textbf{deliver} illegal \textbf{weapons} to the black market.
People come like \textbf{hungry} fish to \textbf{feed} and then land in \textbf{Siberia} and are allowed to snatch \textbf{coal}\underline{.}
\textbf{According} to \textbf{critics}\underline{,} \textbf{Wal}\underline{mar}t can \textbf{sell} the goods so \textbf{cheap}\underline{ly} only because the employees are \textbf{badly} paid.
If \textbf{Wal}\underline{mar}t were to \textbf{shift} all \textbf{wage} \textbf{increases} \textbf{entirely} to customers, each purchase would cost them only \textbf{46} \textbf{cent}\underline{s} more in the future.
The \textbf{input} of information (the system receives more data) has been improved, the \textbf{output} has not been \textbf{decisive}\underline{.}
- The current \textbf{generation} is \textbf{basically} a good starting point for our work in the field of three-\textbf{dimensional} \textbf{recognition}\underline{.}
For my work I needed just such a \textbf{device}\underline{,} only without touch control and with more images per second.
- Many of my images are real \textbf{pearl}\underline{s} and clearly express the \textbf{topical}\underline{ity} and \textbf{sharp}\underline{ness} of the \textbf{thoughts}\underline{.}
Our \textbf{gu}\underline{ll} \textbf{fle}\underline{w} away and no one on \textbf{earth} could have \textbf{answered} the following question: does it \textbf{survive} the space \textbf{flight}\underline{?}
In June \textbf{1964}\underline{,} just one year after her space \textbf{flight}\underline{,} the first \textbf{female} cosmon\textbf{aut}\underline{,} \textbf{Valentin}\underline{a} \textbf{Ter}\underline{es}h\textbf{kov}\underline{a}, \textbf{gave} \textbf{birth} to a \textbf{daughter}\underline{.}
It is as if the little Ichty\textbf{ander}\underline{s} were \textbf{bearing} \textbf{witness} that life on the land \textbf{escape}\underline{d} the \textbf{ocean}\underline{.}
In principle, this is \textbf{logical}\underline{,} since only two weeks pass from \textbf{birth} to first swimming.
Public funds, which are \textbf{administer}\underline{ed} by our \textbf{districts} and \textbf{municipalities}\underline{,} are subject to the control of our national account\textbf{ants}\underline{.}
There is no more \textbf{snow} in the region and only a \textbf{thin} \textbf{snow} cover remains in the lower \textbf{altitude}\underline{s}.
As it has \textbf{snow}\underline{ed} in the past and then \textbf{fell}\underline{,} the \textbf{streets} can be \textbf{chill}\underline{ed} out.
It \textbf{turned} out that most people are interested in working with us and have fun with it.
Your foreign plans are not exactly small, so far you have already \textbf{appeared} in \textbf{Madrid}\underline{,} \textbf{Brussels}\underline{,} London or \textbf{Moscow}\underline{.}
The research was carried out by the \textbf{Kom} xf3rka \textbf{Technik}\underline{i} Uz\textbf{bro}\underline{je}\textbf{nia} \textbf{Institute} in cooperation with \textbf{Prof}\underline{.} \textbf{Mi}\underline{e}\textbf{czy}\underline{s}\textbf{law} \textbf{Wolf}\underline{ke} and \textbf{Prof}\underline{.} \textbf{Gu}\underline{sta}w Mokr\textbf{zy}\underline{ck}iegi.
The first type, the \textbf{RM}\underline{-1}, was \textbf{completed} in \textbf{1957} and its first \textbf{launch} was on 10 October \textbf{1958}\underline{.}
In other words, governments spend their own people on private capital without regard for the social consequences.
The details of this operation were \textbf{kept} \textbf{secret} for a long time.
\textbf{Until} then, women \textbf{enjoyed} an advantage in life \textbf{insurance} because, objectively, they represent a lower risk for \textbf{insurance} companies.
You managed to get to the \textbf{Senat}\underline{e} and then set out on your way to the \textbf{castle}\underline{.}
I have been \textbf{told}\underline{,} for example, that I would \textbf{bri}\underline{be} \textbf{journalists} or that I was \textbf{advise}\underline{r} to \textbf{Ji}  u20\textbf{47}  xed \textbf{Par}\underline{ou}\textbf{bek}\underline{.}
As President, you have no powers in this respect, and only the \textbf{Senat}\underline{e} as a whole can \textbf{submit} legislative proposals.
I also supported \textbf{invest}\underline{ig}ative \textbf{journalist} \textbf{Jan}\underline{a} \textbf{Lor}\underline{en}cov xe\textbf{1,} who \textbf{revealed} \textbf{fraud} in the trade in light \textbf{fuel} oil.
You drive an Aston \textbf{Martin}\underline{,} have a \textbf{fortune} of 60 million and have no money for your \textbf{campaign}\underline{?}
"\textbf{We} wanted to work with \textbf{recycling} materials here," \textbf{explains} Joop \textbf{Tro}\underline{ub}orst, project \textbf{manager} at the \textbf{municipality} of \textbf{Sp}\textbf{\underline{ijk}}\underline{en}\textbf{isse}\underline{,} on demand of the standard.
In a \textbf{Fri}\underline{es}ian \textbf{farm} we found a suitable waste product from agriculture one day.
For many years now, a \textbf{mill}\textbf{\underline{imeter}} \textbf{thin} \textbf{plastic} \textbf{flee}\underline{ce} has been used as a base in the \textbf{Netherlands} in \textbf{greenhouse}\underline{s} and fields.
For the \textbf{library}\underline{,} for the first time in these \textbf{quantities}\underline{,} the non\textbf{woven} was \textbf{pressed} into four \textbf{cent}\underline{i}\textbf{metre} \textbf{thick} \textbf{plates}\underline{.}
Although the bookberg is under a \textbf{drop} of \textbf{glass}\underline{,} even on \textbf{sunny} days the sun \textbf{shine}\underline{s} only \textbf{briefly} into the \textbf{interior}\underline{.}
The wide \textbf{wood} \textbf{glue} binders \textbf{standing} right across the \textbf{glass} fa  u20\textbf{47} ade serve as a \textbf{sha}\underline{ding} and \textbf{capture} much of the \textbf{solar} \textbf{radiation}\underline{.}
It \textbf{signals} that it must be taken \textbf{seriously} as an international player and that its interests must be \textbf{respected}\underline{.}
\textbf{Does} Germany see itself as an important international player - does Germany want to play a leading role at all?
The financial \textbf{losses} and process costs of the affected \textbf{industries} are in the \textbf{millions}\underline{,} especially for \textbf{expensive} \textbf{flagship} products.
In \textbf{2009,} \textbf{Daimler} lost a legal \textbf{dispute} with the construction \textbf{machinery} \textbf{manufacturer} Sany, the company that recently took over the German \textbf{concrete} \textbf{pump} \textbf{manufacturer} \textbf{Put}\underline{z}\textbf{meister}\underline{.}
The population \textbf{hardly} \textbf{accepts} \textbf{ci}\underline{r}\textbf{cum}\underline{ci}sion of the \textbf{male} fores\textbf{kin}\underline{,} which has been \textbf{proven} to reduce the risk of contagion by half.
In heteros\textbf{sexual} \textbf{adults}\underline{,} \textbf{chlor}\underline{ine} \textbf{infection}\underline{s}, \textbf{tri}\textbf{\underline{cho}}\underline{mon}ads, candi\textbf{dos}\underline{e} (\textbf{pill}\underline{),} tripper and human \textbf{pap}\textbf{\underline{pil}}\textbf{\underline{oma}} \textbf{viruses} are common \textbf{sexual}\underline{ly} \textbf{transmitted} \textbf{diseases}\underline{.}
"In total, we have already sent around 200 000 \textbf{euros} to Esitjeni," \textbf{says} \textbf{Anne}\textbf{\underline{tte}} Len\textbf{nar}\textbf{\underline{tz}}\underline{,} \textbf{president} of the \textbf{association}\underline{.}
The 2,\textbf{400} light years away \textbf{fo}\underline{g} is made up of \textbf{dust} \textbf{grain}\underline{s} 10 to 100 times \textbf{smaller} than \textbf{ordinary} house \textbf{dust}\underline{.}
Since then, the \textbf{mirror}\underline{s} of \textbf{optical} \textbf{telescope}\underline{s} have become ever larger - and the \textbf{insight}\underline{s} they provide have become ever \textbf{deeper}\underline{.}
\textbf{Dis}\underline{ad}\textbf{vant}\underline{age} of the \textbf{favourable} design: The \textbf{telescope} is \textbf{fixed} in its \textbf{height} \textbf{angle} - and thus limited in its \textbf{mobility}\underline{.}
A huge new \textbf{telescope} is also to be built on the Ma\textbf{una} \textbf{Ke}\underline{a} - with a \textbf{mirror} \textbf{average} of \textbf{thirty} metres.
However, there is no \textbf{reliable} data for this, as the \textbf{Messenger}\underline{s} are much \textbf{closer} to the \textbf{north} \textbf{pole} around the \textbf{planet}\underline{.}
But this is the deepest south of \textbf{Azerbaijan}\underline{,} the border with Iran is only a few \textbf{kilometres} away.
I always was\textbf{hed} my \textbf{hair} with \textbf{milk}\underline{,} so they never \textbf{went} out of me and \textbf{kept} their \textbf{color}\underline{.}
"\textbf{And} that he \textbf{succeed}\underline{s} is my responsibility, before the people and before God," he said on state \textbf{television}\underline{.}
As in previous \textbf{constitution}\underline{s}, the draft states that \textbf{ju}\textbf{\underline{ris}}\textbf{\underline{pru}}\underline{d}ence is based on the '\textbf{pri}\underline{n}\textbf{cip}\underline{les} of \textbf{Islamic} law'.
The \textbf{Muslim} \textbf{Brot}\underline{her}\textbf{hood} stated that both \textbf{opponents} of the draft \textbf{Constitution} and \textbf{supporters} had \textbf{spoken} out \textbf{loud} and clear.
Rakfisk is \textbf{regarded} as something important - an essential, if \textbf{strictly} \textbf{smell}\underline{ing} part of \textbf{Norwegian} history.
I stand in the \textbf{snow} and stand up for another \textbf{dish} - I have had enough of Rakfisk.
On \textbf{Saturday}\underline{,} \textbf{Mexico} u2019s new \textbf{president}\underline{,} Enr\textbf{ique} \textbf{Pen}\underline{a} \textbf{Nie}\underline{to}, will be \textbf{elected} \textbf{president} and take over the \textbf{leadership} of the \textbf{nation}\underline{.}
"When I \textbf{arrived} at her home, it \textbf{seemed} that her body had been was\textbf{hed}\underline{,}" \textbf{Sen}\textbf{\underline{ora}} \textbf{Bu}\underline{en}\textbf{dia} remembers.
Manning had said that he had never had the opportunity to cover \textbf{himself} with his \textbf{blanket} during this \textbf{count}\underline{.}
This night, Manning said, his under\textbf{wear}\underline{,} f\textbf{lip} \textbf{flo}\underline{ps} and \textbf{glass}\underline{es} were \textbf{removed} from his \textbf{cell}\underline{.}
The \textbf{hearing} is \textbf{scheduled} to continue this \textbf{weekend} and the public \textbf{prosecutor} is expected to \textbf{justify} the conditions of \textbf{detention}\underline{.}
I speak Spanish, at least good enough, to \textbf{assert} \textbf{myself} in this language at both \textbf{ends} of an \textbf{interview}\underline{.}
But I do not have the \textbf{vocabulary} of a \textbf{native} \textbf{speaker} and I will not get \textbf{rid} of my American \textbf{accent} either.
And \textbf{Pen}\underline{a} \textbf{Nie}\underline{to} \textbf{vo}\textbf{\underline{wed}} to continue \textbf{Mexico} u2019s war against \textbf{drug} \textbf{carte}\textbf{\underline{ls}}\underline{,} even if he did not give any details.
And in most cases this person \textbf{correspond}\underline{ed} to a \textbf{profile} - \textbf{dark}\underline{-}s\textbf{kin}\textbf{\underline{ned}}\underline{,} uned\textbf{uc}\underline{ated}, from a poor village, etc.
They want to use \textbf{Mexican} \textbf{Americans} as \textbf{provisional} "\textbf{mes}\underline{s}\textbf{ages}\underline{"} for \textbf{Mexico}\underline{,} \textbf{representing} their interests in the United States.
A war with the local super\textbf{power} will \textbf{hardly} help the new \textbf{Arab} governments to \textbf{repair} their \textbf{economies}\underline{.}
It was said that the laws would encourage black market trade, which would lead to \textbf{cheaper} and more \textbf{accessible} \textbf{cigarette}\underline{s}.
The \textbf{Australian} Government has \textbf{banned} Internet \textbf{advertising} by local companies and sites but has no influence on international sites.
\textbf{District} \textbf{prosecutor} \textbf{Pet}\underline{e} \textbf{Haut}\underline{z}\textbf{inger} supported this decision, but also decided not to \textbf{drop} all \textbf{outstanding} \textbf{ownership} procedures.
"I do not think I am wasting my time \textbf{enforcing} the law until it changes," he \textbf{says}\underline{.}
This evening I \textbf{sat} in \textbf{college} alone for \textbf{dinner}\underline{,} when \textbf{someone} \textbf{slightly} \textbf{tip}\textbf{\underline{ped}} me on the shoulder.
I \textbf{bought} my first \textbf{Valentin}\underline{o} \textbf{girl} for a party in the \textbf{castle} of my cousin, \textbf{Prince} \textbf{Ed}\underline{ou}ard de L\textbf{igne}\underline{.}
I am a \textbf{patri}\textbf{\underline{otic}} \textbf{husband}\underline{,} you are my \textbf{patri}\textbf{\underline{otic}} \textbf{wife}\underline{:} let us \textbf{fulfil} our civil duty and let us create lives.
\textbf{Every} year it spends \textbf{USD} 1 300 on policy measures to encourage citizens to have more children.
El Peri xf3d\textbf{ico} \textbf{interview}\underline{ed} five young people a\textbf{ged} between 10 and 15 who are often on the \textbf{net}\underline{.}
In this sense, he \textbf{defended} the project to create a South American \textbf{citizenship} that promotes the member states of the Unasur.
\textbf{Those} who \textbf{teach} never \textbf{commit} to anything, and in return we always sign everything to the South American people.
Cor\textbf{rea} also referred to the treatment of the health problems of \textbf{Venezuela}\underline{n} President Hugo \textbf{Ch} xe1vez in \textbf{Cuba}\underline{.}
The \textbf{walls} of his house are almost all \textbf{decorated} with \textbf{photos} and \textbf{memories} of his long \textbf{career} and \textbf{testify} to them.
And then I left with a \textbf{championship} in \textbf{1981}\underline{,} the year of the \textbf{debut} of Je\textbf{rome} \textbf{Min}\underline{cy} at BSN.
At that time he \textbf{preferred} to enjoy his \textbf{execution}\underline{s} and those of \textbf{Min}\underline{cy} in the national team.
She is one of the best, as well as the one who won against the \textbf{Dream} Team at the 2004 \textbf{Olympic}\underline{s}.
The family of La\textbf{rry} and his \textbf{closest} friends were with him in \textbf{Dal}\textbf{\underline{las}} for the \textbf{celebration}\underline{s} of the \textbf{harvest} \textbf{grateful}\underline{.}
\textbf{Unlike} \textbf{Canada}\underline{,} the US states are responsible for \textbf{holding} national elections.
They are proposed active monitoring and are offered treatment as the \textbf{disease} progresses.
The criteria for \textbf{deciding} who should and should not be \textbf{treated} are increasingly being \textbf{determined}\underline{.}
While one study found the reduction in the risk of pro\textbf{state} \textbf{cancer}\underline{,} another \textbf{showed} an increase.
\textbf{Quebec} has recently \textbf{discussed} the \textbf{delicate} question of the end of life with its Committee on \textbf{Death} in \textbf{dignity}\underline{.}
Si\textbf{tting} at the table in front of a \textbf{tasty} \textbf{lunch}\underline{,} he \textbf{resign}\underline{ed} to be \textbf{helped} with food.
"\textbf{My} \textbf{greatest} wish is to heal my diarrhea, as this is \textbf{hum}\textbf{\underline{ili}}\underline{ating}," he \textbf{says}\underline{.}
In the view of several people working in \textbf{pal}\underline{li}ative care, major events are taking place in the \textbf{middle} of these \textbf{decline}\underline{s}.
In the next few days, however, she is still \textbf{awaiting} a last visit by her \textbf{son}\underline{,} who comes from Italy.
In the \textbf{Victor}\underline{-}\textbf{Ga}\textbf{\underline{db}}\textbf{\underline{ois}} Home, a group of \textbf{volunteer}\underline{s} is offered body care and help with food in\textbf{take}\underline{.}
This is where life \textbf{continues} under the best possible conditions, \textbf{explains} Dr. \textbf{Christian}\underline{e} Martel, one of the \textbf{doctors} of the Home.
An 'indus\textbf{try}\underline{'} that was very \textbf{expensive} for \textbf{Quebec}\underline{'}s \textbf{taxpayers}\underline{,} especially in the 1990s and 2000s.
This means that a player like me has to stand up and do his best.
In order to become a great European \textbf{club}\underline{,} Paris must \textbf{win} titles and make a name for itself in the long term.
\textbf{Lyon} and \textbf{Marseille}\underline{,} which weren't good in the last season, were "\textbf{fuel}\underline{ed}" by this new \textbf{PS}\underline{G}.
\textbf{Thi}\textbf{\underline{ago}} \textbf{Silva}\underline{,} one of the best \textbf{defend}\underline{ers} in the world, also enables everyone else to make progress.
A number of data related to this \textbf{transaction} is \textbf{electronically} \textbf{signed} by a double \textbf{encryption} system.
The \textbf{computers} "\textbf{take}\underline{"} the new \textbf{transaction} and add a number to it before it is "\textbf{hack}\underline{ed}".
The goal is to find the number that gives a special \textbf{fingerprint} (many \textbf{zero}\underline{s} at the beginning).
"\textbf{It} will take some time for \textbf{Bit}\underline{co}in to \textbf{prevail}\underline{,} but \textbf{2013} could be a \textbf{turning} point," he \textbf{predict}\underline{s}.
At that time, Ka\textbf{bul} was \textbf{empty} and the country was overw\textbf{helm}\underline{ed} by war because of the \textbf{fighting} of the various in\textbf{sur}\textbf{\underline{gent}} groups.
While the \textbf{Egyptian} President had to speak on \textbf{television} last night, \textbf{demonstrations} are \textbf{planned} for this \textbf{afternoon}\underline{.}
From \textbf{Friday} evening to the \textbf{sunset} on \textbf{Saturday}\underline{,} markets and \textbf{shops} are closed and public transport rests.
Most \textbf{adventure}\underline{rs} and \textbf{recreational} \textbf{seekers} came from Russia, France, Germany, Italy, \textbf{England}\underline{,} the USA and Ukraine.
\textbf{Their} only aim is to make money for the \textbf{maintenance} of the families left in their \textbf{homes}\underline{.}
However, over time, according to the \textbf{Federal} \textbf{Migration} \textbf{Authority}\underline{,} the \textbf{tests} will become \textbf{compulsory} for all guest workers.
The initiative to introduce the \textbf{tests} was supported by members of the State \textbf{Duma} and the \textbf{Federal} \textbf{Migration} \textbf{Authority}\underline{.}
Some fake \textbf{certificates} \textbf{cert}\textbf{\underline{ifying}} the \textbf{completion} of the language test have already been confi\textbf{sc}\underline{ated} by members of the \textbf{Federal} \textbf{Migration} \textbf{Authority}\underline{.}
Not all of them are \textbf{satisfied} that the Russian authorities want to combat the problems by 're\textbf{tract}\underline{ing} \textbf{screw}\underline{s}'.
\textbf{Wal}\underline{mar}t \textbf{sell}\underline{s} all products, from \textbf{dia}\textbf{\underline{pers}}\underline{,} \textbf{hunting} \textbf{gun}\underline{s} and car \textbf{batteries} to \textbf{vacuum} cleaners, \textbf{eggs} and \textbf{milk}\underline{.}
The products in \textbf{Wal}\underline{mar}t \textbf{stores} are on \textbf{average} between 8 and 2\textbf{7\%} \textbf{cheaper} than in large \textbf{supermarket}\underline{s}.
A \textbf{typical} \textbf{Wal}\underline{mar}t \textbf{employee} who \textbf{earn}\underline{s} \$9.5 an \textbf{hour} cannot \textbf{afford} this increase, they said.
\textbf{According} to the New York \textbf{Times}\underline{,} this was the \textbf{biggest} action of its kind in the history of the US fast-\textbf{food} industry.
We try to change this, work on real three-\textbf{dimensional} display systems based on different technologies, including \textbf{projection}\underline{s}.
- If I remember \textbf{correctly}\underline{,} Microsoft, \textbf{unlike} Google, did not present its \textbf{glass}\underline{es} to the public.
I have \textbf{chosen} the \textbf{color} red as a \textbf{fashion} \textbf{designer} who \textbf{deals} with the \textbf{opt}\textbf{\underline{ics}} and image.
We \textbf{gave} them \textbf{Tra}\textbf{\underline{chten}}\underline{berg}, and his great \textbf{career} began, but he \textbf{learned} the basics with us.
Now everyone \textbf{pays} attention to the \textbf{clothes} and \textbf{focuses} on the outer and not on the \textbf{inner}\underline{.}
In the past, people \textbf{formed} large groups: the \textbf{Bohemia}\underline{n}s \textbf{loved} one thing and the simple people \textbf{loved} the other.
I have \textbf{supporters}\underline{,} and the most important thing is not to \textbf{cheat} them and not to \textbf{destroy} what has been achieved.
- \textbf{Petersburg} is not the capital of culture; in \textbf{Moscow} there is much more culture and a \textbf{breeding} ground.
The \textbf{fourth} \textbf{generation} of peas \textbf{br}\underline{ed} in orbit did not \textbf{differ} in any way from \textbf{earth}\underline{ly} \textbf{species}\underline{.}
A new\textbf{born} child cannot be put into a stress \textbf{suit} in orbit like an \textbf{adult}\underline{.}
In the discussion for \textbf{Akt}\underline{u} xe1ln  u20\textbf{47} .\textbf{cz} this is said by the \textbf{Vice}\underline{-}\textbf{President} of the \textbf{Supreme} \textbf{Control} Office (N\textbf{ej}\textbf{\underline{vy}}  u20\textbf{47}  xed \textbf{kon}\underline{tro}ln xed   u20\textbf{47} \textbf{ad}\underline{,} \textbf{NK}  u20\textbf{47} \textbf{),} \textbf{Mil}\underline{o}\textbf{slav} \textbf{Kal}\underline{a}.
It is a \textbf{parallel} test that we started about two years ago.
However, the problem may \textbf{arise} that the rules are becoming 'ser\textbf{ious}\underline{'} and can no longer be \textbf{complied} with.
It should be \textbf{noted}\underline{,} however, that improving the situation always \textbf{depends} on the efforts of those affected.
There are only a few \textbf{truly} unique things, and I dare to say that \textbf{Tap} \textbf{Tap} is part of it.
Entrance costs \textbf{400} \textbf{CZK}\underline{,} children under 12 years free of charge, \textbf{tickets} are available for pre-sale at \textbf{Bohemia}\textbf{\underline{ticket}}\underline{.}
The first \textbf{RM} \textbf{rocket}\underline{s} were \textbf{succeeded} by the \textbf{Met}\underline{e}or-1 \textbf{rocket} developed between \textbf{1962} and \textbf{1965}\underline{.}
The \textbf{missile} was designed as a two-stage \textbf{rocket}\underline{,} its total \textbf{length} was 510 \textbf{cm} and its starting \textbf{weight} was \textbf{32}\underline{.}5 \textbf{kg}\underline{.}
This is done, on the one hand, through economic coer\textbf{cion} in the case of long-term unemployment and, on the other, by \textbf{curtail}\underline{ing} workers' rights.
\textbf{Private} capital \textbf{st}\underline{ub}\textbf{born}\underline{ly} \textbf{insist}\underline{s} on its view that the state must not be allowed to \textbf{intervene} in the economy in a direct way.
We are going to apply for a \textbf{refund} from the EU," \textbf{explained} the then Minister of \textbf{Agriculture} Jaro\textbf{slav} \textbf{Pala}\underline{s} (  u20\textbf{47} S\textbf{SD}\underline{)} in \textbf{autumn} \textbf{2004.}
If you set up a business plan in a company, you also have an ideal goal and a \textbf{vision}\underline{.}
I say quite clearly that I am an \textbf{amateur}\underline{;} I am \textbf{neither} a \textbf{genius} nor an \textbf{intellectual}\underline{.}
I do not even have money for the \textbf{presidential} \textbf{campaign}\underline{;} on my transparent account there are only 2\textbf{0,000} \textbf{CZK}\underline{.}
You say that you want to change the Republic, but you do not want to \textbf{invest} your own money in it.
The fact that I do not have \textbf{sponsor}\underline{s} shows that my programme does not \textbf{arouse} too much interest.
We have \textbf{turned} the \textbf{classic} room \textbf{configuration} on its head and \textbf{fold}\underline{ed} the reading area from the inside to the outside.
The \textbf{interior} of the bookberg is well used: \textbf{offices}\underline{,} Internet \textbf{library}\underline{,} chess \textbf{club}\underline{,} environmental centre and house technology centre are in the centre.
But I would not want to place too much \textbf{emphasis} on this either; it is not a completely one-\textbf{sided} relationship.
I believe that the \textbf{Obama} administration \textbf{secret}\underline{ly} has quite a lot of understanding for the European position.
I believe that in future Germany will take a leading role in \textbf{pressing} Europe into a European position.
Wen\textbf{tz}\underline{ler} is \textbf{confident} to bring the matter to a successful conclusion and \textbf{commend}\underline{s} the \textbf{professionalism} of the \textbf{courts}\underline{.}
But he also \textbf{says}\underline{:} 'The process is extremely complex and costs us a lot of time, money and \textbf{nerve}\underline{s}'.
Some 2 000 people live there, some still living in simple \textbf{mud} and \textbf{stra}\underline{w} \textbf{huts}\underline{,} most of which are children.
In Esitjeni, the little one shows what is \textbf{sick} of Swaziland: the highest \textbf{HIV} \textbf{infection} rate, the \textbf{lowest} life expect\textbf{ancy} in the world according to Unicef.
Some of the \textbf{pathogen}\underline{s} of \textbf{sexual}\underline{ly} \textbf{transmitted} \textbf{diseases} can also be \textbf{passed} on through \textbf{lub}\textbf{\underline{ric}}\underline{ation} \textbf{infection}\underline{s} and close body contact.
The \textbf{photograph} published by the European \textbf{Southern} \textbf{Observatory} shows the Trifid ne\textbf{bul}\underline{a}, which is several \textbf{thousand} light years away, in the con\textbf{stell}\underline{ation} Sch xfc\textbf{tze}\underline{.}
In this \textbf{bright}\underline{ly} \textbf{illumin}\underline{ated} \textbf{galaxy} with a small black \textbf{hole}\underline{,} there is no \textbf{dust} but only gas.
It allows you to look into space over two \textbf{mirror}\underline{s}, each with a \textbf{diameter} of \textbf{8.}\underline{4} \textbf{meters}\underline{.}
In the "\textbf{Se}\textbf{\underline{arch}} for \textbf{Extra}\textbf{\underline{terre}}\textbf{\underline{stri}}\underline{al} \textbf{Intelligence}\underline{"} (\textbf{SET}\underline{I}), any computer \textbf{owner} can help by providing \textbf{computing} power.
\textbf{Until} 2007, the two K\textbf{eck} \textbf{telescope}\underline{s} on the \textbf{Hawaii}\underline{an} \textbf{volcano} Ma\textbf{una} \textbf{Ke}\underline{a} were considered the largest in the world.
Since March \textbf{2009,} the \textbf{Ke}\underline{pl}er space \textbf{telescope} has been \textbf{searching} for extra\textbf{sol}\underline{ar} \textbf{planet}\underline{s} - especially those that are \textbf{habit}\underline{able}.
The \textbf{mini}\underline{bus} \textbf{ro}\underline{am}s over the \textbf{wind}\underline{ing} road, past densely \textbf{wood}\underline{ed} \textbf{hills}\underline{,} \textbf{tear}\underline{ing} \textbf{rivers} and simple \textbf{farmhouse}\underline{s}.
However, a \textbf{controversial} star of the \textbf{museum} is the shepherd   u20\textbf{47} \textbf{ir}\textbf{\underline{ali}} M xf\textbf{cs}\underline{l} xfc\textbf{mov}\underline{,} who is said to have become 168 years old.
And, in view of the \textbf{oldest} \textbf{documented} man who was 122 years old, M xf\textbf{cs}\underline{l} xfc\textbf{mov} u2019s age seems extremely questionable.
The fact is, however, that the people of the region around Le\textbf{rik} \textbf{cons}\textbf{\underline{pic}}\textbf{\underline{uous}}\underline{ly} often reach a \textbf{bi}\textbf{\underline{bli}}\underline{cal} age.
\textbf{Perhaps} \textbf{Mir}\underline{za}y\textbf{eva}\underline{'}s long-s\textbf{uff}\underline{er}ing \textbf{son} is right: 'The \textbf{elderly} enjoy great respect in our culture'.
\textbf{Nobel} \textbf{Peace} \textbf{Prize} \textbf{winner} and former \textbf{leader} of the International \textbf{Atom}\underline{ic} \textbf{Energy} \textbf{Agency} Mo\textbf{ham}\underline{ed} El-\textbf{Bar}\textbf{\underline{ade}}\underline{i} \textbf{declared} that the draft \textbf{Constitution} \textbf{belongs} "to the \textbf{dust}\textbf{\underline{bin}} of history".
\textbf{Could} the country's \textbf{secret} of success have something to do with the local \textbf{appetite} for \textbf{pretty} \textbf{od}\textbf{\underline{ious}} fish?
\textbf{Norway} does not manage to do so often in the world press, and most people do not \textbf{seem} to be \textbf{disturb}\underline{ed}.
"As long as we can ski in winter and \textbf{hike} in summer, we are happy," \textbf{says} \textbf{Anna}\underline{.}
There is a live TV \textbf{circuit} to a \textbf{fly}\underline{-}d\textbf{ress}\underline{ed} show\textbf{master} \textbf{surrounded} by \textbf{plates} with \textbf{rak}\underline{fi}sk.
\textbf{Before} he was on an equal \textbf{footing} with the US President, \textbf{Pen}\underline{a} \textbf{Nie}\underline{to} served as \textbf{Governor} of his home state, \textbf{Mexico}\underline{.}
\textbf{Pla}\textbf{\underline{ques}} with its name also \textbf{lie} outside a modern sports centre and an \textbf{impressive} \textbf{interactive} \textbf{museum} on climate change.
But, on the other side of the state, not many people share this view about their former \textbf{governor}\underline{.}
\textbf{Hi}\underline{d}den under \textbf{motorway} \textbf{transfers}\underline{,} it is in many ways a \textbf{suburb} of \textbf{Mexico} City itself.
He said that he had considered \textbf{suicide} in \textbf{Kuwait} and that, for once, he had become un\textbf{conscious} because of the \textbf{heat}\underline{.}
\textbf{Mexican}\underline{s} \textbf{tend} to \textbf{accus}\underline{e} \textbf{emigr}\textbf{\underline{ants}} - they remind them of difficult times, he \textbf{says}\underline{.}
By \textbf{contrast}\underline{,} the \textbf{Brot}\underline{her}\textbf{hood} with \textbf{Hamas} has become obsessed and its leaders more \textbf{dependent} on popular views.
\textbf{Blood}\underline{y} \textbf{missions} to \textbf{rep}\textbf{\underline{atri}}\underline{ate} \textbf{Hamas} in \textbf{Gaza} will increasingly take their \textbf{diplomatic} \textbf{toll} over the years.
This would do more to create a \textbf{Palestinian} state than with the \textbf{forthcoming} application for UN \textbf{observe}\underline{r} status.
The \textbf{Australian} \textbf{federal} government \textbf{wants} to deter young people from \textbf{smoking} by \textbf{removing} the \textbf{gla}\textbf{\underline{mor}}\underline{ous} image of \textbf{smoking}\underline{.}
\textbf{Frank}\underline{ly}, there is only one reason I would stop, and that is my little \textbf{girl}\underline{.}
So \textbf{bo}\underline{re}\textbf{dom} \textbf{differ}\underline{s} from a\textbf{path}\underline{y} in that the person is not \textbf{employed} but \textbf{wants} to be.
We all get \textbf{bo}\underline{red} at some point - my late \textbf{flight}\underline{,} a \textbf{loud} \textbf{speaker}\underline{,} a particularly \textbf{tir}\underline{ing} film.
He \textbf{believes} that in reality people are only looking for a way to turn off and \textbf{relax}\underline{.}
The \textbf{reactions} are \textbf{ambiguous} even in places like rural Mesa \textbf{County}\underline{,} where \textbf{voters} \textbf{rejected} the \textbf{Mari}\underline{hu}ana initiative.
Last week, \textbf{Mont}\textbf{\underline{rose}}\underline{,} a city in the West, decided on a six-\textbf{month} ban, which will probably be adopted next week.
They are \textbf{calling} for a place in their \textbf{college} \textbf{equality} committee to ensure that their \textbf{opinions} can be \textbf{freely} expressed.
"\textbf{This} \textbf{pose}\underline{s} a \textbf{threat} to \textbf{intellectual} \textbf{discourse} and to the well-\textbf{being} of members," she \textbf{says}\underline{.}
I \textbf{felt} as if \textbf{homosexual}\underline{s} had \textbf{felt} like the more \textbf{liberal} legislation of the United States.
He hated the place, found it \textbf{provincial} and \textbf{pet}\underline{ty} and \textbf{rejected} it for his \textbf{Marx}\underline{ist}-de\textbf{termin}\textbf{\underline{istic}} \textbf{perspective} of history.
It was a p\textbf{ants}\underline{,} a \textbf{shirt}\underline{,} a \textbf{wa}\underline{ist}coat type "G\textbf{ill}\textbf{\underline{ette}}\underline{"} and a \textbf{jacket} from the \textbf{autumn}\underline{/}w\textbf{inter} collection \textbf{1971}\textbf{\underline{-19}}\textbf{\underline{72}}\underline{.}
I \textbf{saw} him last time a month ago at a g\textbf{ala} \textbf{dinner} in the Museum de Orsay.
There are people for whom their work is \textbf{hell}\underline{,} and others are \textbf{literally} working in \textbf{hell}\underline{.}
Anto has asthma, \textbf{breath}\underline{es} with \textbf{difficulty}\underline{,} husts \textbf{frequently} and his \textbf{eyes} are \textbf{ir}\textbf{\underline{rit}}\underline{ated} because of \textbf{toxic} \textbf{gases}\underline{.}
I will not \textbf{retire}\underline{,} I will die here because the \textbf{volcano} was my whole life.
"\textbf{Th}\textbf{\underline{ose}} are very \textbf{confidential} \textbf{secret}\underline{s}, my \textbf{mother} may know them, but not the whole world," he \textbf{confirm}\underline{s}.
\textbf{According} to the \textbf{boy}\underline{,} no one made any \textbf{suggestion} or asked him for his address or telephone number.
"\textbf{We} are the digital \textbf{immigrants} they are \textbf{supposed} to \textbf{teach} when we still learn for ourselves," he \textbf{says}\underline{.}
Cor\textbf{rea} stated that there was a risk that Ass\textbf{ange}\underline{'}s health and \textbf{mental} \textbf{condition} would be affected.
These funds were used for the \textbf{acquisition} of \textbf{shares} of the \textbf{Admin}\underline{ist}rad\textbf{ora} \textbf{Prof}\underline{es}\textbf{ional} de Hoteles (\textbf{Pro}\underline{fe}ss\textbf{ional} Hotel Management).
Bartow then \textbf{recommended} \textbf{Ray}\textbf{\underline{mond}} Ga\textbf{usse}\underline{,} who was one of our best \textbf{throw}\underline{ers}.
I still know when we won against the United States for the first time at the pre-Olym\textbf{pic} \textbf{tournament} in \textbf{Mexico}\underline{.}
We had a number of good trainers like Julio Toro, \textbf{Flor} \textbf{Mel} xe9\textbf{nde}\underline{z}, \textbf{Carlos} \textbf{Moral}\underline{es}, \textbf{Ray}\textbf{\underline{mond}} \textbf{Dal}\underline{m}au, \textbf{Arm}\underline{and}\textbf{ito} \textbf{Torre}\underline{s}.
"\textbf{He} was an original person and \textbf{lived} life to the full," \textbf{Gra}\underline{y} \textbf{explained} in a communication.
\textbf{Hag}\underline{man} was \textbf{diagnose}\underline{d} with liver \textbf{ci}\underline{r}rhosis in \textbf{1992}\underline{,} and he \textbf{admitted} that he had \textbf{dr}\textbf{\underline{unk}} a lot for years.
In \textbf{Temple}\underline{,} the \textbf{assistant} \textbf{Professor} Barry \textbf{Va}\underline{cker} gives the course '\textbf{Media}\underline{s}, \textbf{Culture} and the End of the World'.
"I \textbf{tried} to inform the students about what is possible, probably, \textbf{credible} and \textbf{impossible}\underline{,}" \textbf{Va}\underline{cker} said.
The United States \textbf{Supreme} Court \textbf{confirmed} in 2008 the \textbf{constitutional}\underline{ity} of the \textbf{Indian}\underline{a} law.
The new \textbf{restrictions} have \textbf{disproportionate}\underline{ly} affected young people, \textbf{minorities} and people on low incomes.
It is \textbf{obvious} that two out of three His\textbf{pan}\underline{ic} \textbf{voters} \textbf{prefer} the democratic party.
The \textbf{latter} accounted for only 11\% of the \textbf{electorate}\underline{,} but 2\textbf{4\%} of the citizens who voted in advance.
For example, in \textbf{1969} \textbf{Will}\underline{ard} \textbf{Boy}\underline{le} developed a small light \textbf{sensor} during his work in \textbf{opt}\textbf{\underline{ics}}\underline{.}
Last night we served Mr X a beer who died during the night.
5\textbf{3\%} of \textbf{patients} \textbf{admitted} to the \textbf{Victor}\underline{-}\textbf{Ga}\textbf{\underline{db}}\textbf{\underline{ois}} home come from their \textbf{homes}\underline{,} 4\textbf{7\%} from the \textbf{hospital}\underline{.}
The '\textbf{Du}\textbf{\underline{ches}}\underline{n}\textbf{eau} report' established a direct link between industry, \textbf{secret} \textbf{financing} of parties and \textbf{bri}\underline{ber}y of \textbf{officials}\underline{.}
He also \textbf{admitted} that he had \textbf{organised} an illegal \textbf{fund}\textbf{\underline{raising}} for former \textbf{liberal} \textbf{Vice}\underline{-}\textbf{President} Na\textbf{thal}\underline{ie} \textbf{Norman}\underline{de}au.
As a result of these \textbf{revelation}\underline{s}, Mr \textbf{Tre}\underline{mb}\textbf{lay} \textbf{resign}\underline{ed} at the beginning of November, which \textbf{plunge}\underline{d} \textbf{Montreal} into a serious crisis.
It can be \textbf{explained} by a personal \textbf{insight}\underline{,} but also by the new \textbf{dimension} of \textbf{PS}\underline{G}.
What do you think about the first months of \textbf{Did}\underline{ier} Deschamps at the top of the "Bleus"?
I have never seen a similar game in my \textbf{career} before this meeting in Spain.
\textbf{Every} \textbf{transaction} between two users actually takes place between two e-mail \textbf{addresses} in the form of an e-mail.
\textbf{Once} this number has been found, the other nodes can easily check if it is the right one.
However, his country has been \textbf{dependent} on foreign aid since the \textbf{1950}\underline{s} and long before.
\textbf{Industry} has not been \textbf{rebuilt}\underline{,} there are no \textbf{functional} \textbf{res}\underline{er}\textbf{voir}\underline{s} and important \textbf{irrigation} systems have not been \textbf{repair}\underline{ed}.
The \textbf{embassy} received \textbf{dozen}\underline{s} of written \textbf{requests} from small agricultural projects from \textbf{communities} in the \textbf{province} of \textbf{Kap}\textbf{\underline{isa}}\underline{.}
\textbf{85} \textbf{largely} \textbf{Islamist} members of this \textbf{constituent} \textbf{assembly} adopted the text \textbf{yesterday} in a \textbf{strange} atmosphere.
The \textbf{latter} also share their concerns about the text that they see as \textbf{threatening} freedom.
In Israel \textbf{Ukrainian} \textbf{tourists} expect \textbf{sacred} sites, the um\textbf{bil}\underline{ical} of the world and a sea of \textbf{salt}\textbf{\underline{water}}\underline{.}
The Promised Land \textbf{unite}\underline{s} the \textbf{sp}\underline{len}d\textbf{our} of \textbf{bi}\textbf{\underline{bli}}\underline{cal} \textbf{truth}\underline{s}, modern comfort and \textbf{untouched} nature.
In \textbf{Christian} view, this is where the um\textbf{bil}\underline{ical} world is located, \textbf{symbol}\underline{ising} the \textbf{sal}\underline{v}ation of \textbf{humanity}\underline{.}
\textbf{Its} \textbf{tur}\textbf{\underline{qu}}\textbf{\underline{ois}}\underline{e}-\textbf{blue} water has a high \textbf{salt} content and therefore \textbf{carrie}\underline{s} even non-w\textbf{immer}\underline{s} easily on the \textbf{surface}\underline{.}
In J\textbf{aff}\underline{a} you can meet \textbf{newly} \textbf{married} \textbf{couples} from all over Israel and even other countries on photo \textbf{appointment}\underline{s}.
"The \textbf{weapons} have been \textbf{stolen} by both Russian \textbf{officers} and the Cau\textbf{cas}\textbf{\underline{ians}} themselves," \textbf{says} Baranez.
The \textbf{vast} majority of illegal \textbf{weapons}\underline{,} according to the \textbf{invest}\underline{ig}\textbf{ators}\underline{,} come from the \textbf{army} and the \textbf{judicial} authorities.
He also gives me the \textbf{ring}\underline{s} just because he \textbf{knows} that I am not \textbf{whi}\textbf{\underline{pping}} it.
Internet search \textbf{engines} show search results for \textbf{websites} and groups in \textbf{contacts} where \textbf{weapons} are offered "for different purposes".
\textbf{Expert}\underline{s} say that the price of illegal \textbf{fire}\textbf{\underline{arm}}\underline{s} is \textbf{USD} 100 to \textbf{USD} \textbf{900}\underline{.}
However, this requires not only the user but also his environment to be \textbf{recognized}\underline{.}
- What are your demands on modern \textbf{cameras} based on your work with \textbf{Xbox} \textbf{Ki}\underline{n}\textbf{ect} \textbf{sensors}\underline{?}
But the main thing is not the \textbf{Megapixel}\underline{s} themselves, but the quality of the \textbf{mat}\underline{r}ix and \textbf{depth}\underline{.}
There is a problem that \textbf{critics} of this idea often point out: there is no \textbf{tangible} \textbf{reaction}\underline{!}
Let it think that it feels what it should feel when it sees something?
So far, the \textbf{brain} is only \textbf{moderate}\underline{ly} outperformed, and we have many years of work \textbf{ahead} of us.
\textbf{Kir}\textbf{\underline{ill}} \textbf{Mill}\underline{er} is a \textbf{lumin}\underline{ous} \textbf{personality} of the \textbf{Petersburg} a\textbf{vant}\underline{-}\textbf{garde} at the end of the \textbf{1980}\underline{s} or the beginning of the 1990s.
In society, anything that de\textbf{via}\underline{tes} from the \textbf{grey} standard \textbf{causes} \textbf{aggression} and bad \textbf{behaviour}\underline{.}
Let us save the world, for example, by pres\textbf{cri}\textbf{\underline{bing}} that everyone must \textbf{dress} up completely.
But perhaps we should not give a person a hand, but we should give him a face.
\textbf{Life} would only be possible in great \textbf{height} or in the orbit of \textbf{Venus}\underline{,} in other words in space.
How can the project help you?
Do you consider the \textbf{adoption} of this law to be more positive or will the system be \textbf{burden}\underline{ed} with more \textbf{bureaucracy}\underline{?}
The R6 \textbf{motorway} and the first-\textbf{class} \textbf{roads} in the region are currently fully \textbf{accessible}\underline{.}
However, attention must be paid, for example, to \textbf{bridge}\underline{s} where the \textbf{tracks} are sometimes \textbf{frozen} and \textbf{smooth}\underline{.}
\textbf{Road} \textbf{champion}\underline{s} warn \textbf{drivers} against \textbf{ice}\underline{-}smoothing, especially in higher \textbf{locations} in the \textbf{district} of \textbf{Par}\underline{du}\textbf{bic}\underline{e}.
An \textbf{extended} \textbf{snow} \textbf{layer} is located at \textbf{altitude}\underline{s} on the \textbf{streets} of \textbf{Ry}\underline{ch}\textbf{nov} \textbf{nad} Kn  u20\textbf{47} nou and \textbf{Tru}\underline{t}\textbf{nov}\underline{.}
There is also \textbf{fo}\underline{g} on the local side, but the \textbf{visibility} will improve during the day.
\textbf{Snow} \textbf{mat}\underline{s} can be \textbf{count}\underline{ed} on today by \textbf{drivers} who are on their way to the high \textbf{altitude}\underline{s} in the \textbf{district} of \textbf{Ol}\underline{o}mo\textbf{uc}\underline{.}
\textbf{Original}\underline{ly} from me, then we developed the idea together with our \textbf{graphic} \textbf{artist} Honza Augusta.
Today the anthem on \textbf{YouTube} is already very popular, and will it be heard at the benefit \textbf{concert}\underline{?}
Dr. \textbf{Jan} Ga\textbf{dom}\underline{ski} \textbf{(18}\textbf{\underline{99}} - \textbf{1966}\underline{)} later became an important \textbf{advocate} of astro\textbf{nom}\underline{y} and space travel.
In \textbf{Polish} \textbf{magazine}\underline{s} he published \textbf{hundreds} of \textbf{articles} and \textbf{wrote} several \textbf{books} on these scientific \textbf{discipline}\underline{s}.
As long ago as 1925, a \textbf{railway} \textbf{tunnel} was built in \textbf{Poland} for which a \textbf{rocket} \textbf{engine} was \textbf{planned}\underline{.}
It is \textbf{evident} from the documents that have been \textbf{passed} on that research had reached the stage of practical \textbf{tests}\underline{.}
On the other hand, the \textbf{loose} \textbf{passage}\underline{s} from \textbf{Hollywood}\underline{,} which are \textbf{iron}\underline{ic} and \textbf{slightly} \textbf{exaggerate}\underline{d}.
\textbf{Rum} must be used only for products made from \textbf{sugar} cane di\textbf{still}\underline{ate} and not for products made from \textbf{sugar} beet.
"P\textbf{eo}\textbf{\underline{ple}} want me to save the \textbf{republic}\underline{,} but I am just an \textbf{amateur}\underline{,}" O\textbf{kam}\textbf{\underline{ura}} \textbf{claims}\underline{.}
Just take the direct \textbf{election} of the President, which was a \textbf{tribute} to public pressure.
And \textbf{Stefan} \textbf{Sp}\underline{er}mon, IT \textbf{technic}\underline{ian} in a \textbf{nearby} large-\textbf{scale} company, \textbf{says}\underline{:} 'But, it is nice already, the house'.
\textbf{Above} all, \textbf{Sp}\textbf{\underline{ijk}}\underline{en}\textbf{isse} now has the first public cultural building in its history.
\textbf{Stefan} \textbf{Sp}\underline{er}mon, the first IT \textbf{sceptic}\underline{,} has already dared to go into the new \textbf{library}\underline{.}
And also the T\textbf{CM} \textbf{teacher} \textbf{Cy}\underline{n}thia Bo\textbf{garde}\underline{,} who even calls the Boek\textbf{enberg} a \textbf{sp}\textbf{\underline{ijk}}\underline{en}\textbf{isse}\underline{s} "\textbf{long}\underline{-}overdue \textbf{soul}\underline{".}
"I think thanks to our \textbf{invitation}\underline{,} now every \textbf{resident} has a certain relationship with this new house.
They are expected to play a more independent role, but they are not used to it.
\textbf{Have} these economic interests \textbf{influenced} the \textbf{attitude} in the Middle East conflict and the UN vote?
I believe that there is a great deal of understanding in Europe and even in the USA for the German position.
That is why I do not believe that this was such a \textbf{dramatic} break as in the \textbf{Libya}\underline{n} question.
\textbf{Freud}\textbf{\underline{enberg}} was right in the next two instances, but his \textbf{opponent} \textbf{continues} to fight.
For \textbf{180} \textbf{AIDS} \textbf{orphan}\underline{s} in the village of Esitjeni the \textbf{association} \textbf{Voice}\underline{s} for Africa has found \textbf{sponsor}\underline{s} in Germany.
In\textbf{fec}\underline{t}\textbf{ious} \textbf{diseases} can cause ul\textbf{cer}\underline{s} in the \textbf{genital} area, \textbf{ur}\underline{in}ary \textbf{disorder}\underline{s}, out\textbf{flow}\underline{s}, sub\textbf{cut}\underline{an}\textbf{eous} \textbf{pain}\underline{s} as well as \textbf{ve}\underline{s}icles or warts.
There are free con\textbf{dom}\underline{s} at every \textbf{corner}\underline{,} \textbf{says} \textbf{Anne}\textbf{\underline{tte}} Len\textbf{nar}\textbf{\underline{tz}}\underline{,} "\textbf{but} they are \textbf{hardly} used.
The water was \textbf{presumably} coming from comets or \textbf{possibly} aster\textbf{oid}\underline{s} on the mesh.
In the huge Trifid Ne\textbf{bul}\underline{a}, 5\textbf{400} light years from \textbf{Earth}\underline{,} new \textbf{stars} are created from gas and \textbf{dust}\underline{.}
The \textbf{mirror} of the \textbf{Southern} \textbf{African} \textbf{Large} \textbf{Tele}\textbf{\underline{scope}} in South Africa is \textbf{segment}\underline{ed} - to save money.
D\textbf{espite} the \textbf{comparative}\underline{ly} low \textbf{mirror} \textbf{diameter}\underline{,} this is \textbf{comparable} to that of the world's largest \textbf{mirror} \textbf{telescope}\underline{s}.
\textbf{Us}\underline{ing} a \textbf{radio} \textbf{telescope} in \textbf{Are}\underline{ci}bo (\textbf{Pu}\underline{er}to \textbf{Rico}\underline{),} \textbf{researchers} \textbf{listen} to space after \textbf{alien} \textbf{signals}\underline{.}
\textbf{Its} main \textbf{mirror} is \textbf{supposed} to be a full \textbf{42} m long - and \textbf{composed} of \textbf{nearly} \textbf{1000} \textbf{mirror} elements.
On 2 February \textbf{2011}\underline{,} Nasa \textbf{announced} that 12\textbf{35} \textbf{planet} \textbf{candidates} have been \textbf{identified} since the start of the \textbf{mission}\underline{.}
The \textbf{James} We\textbf{bb} \textbf{Space} \textbf{Tele}\textbf{\underline{scope}} (JWST) will be \textbf{launched} on board an \textbf{Ariane}\underline{5} \textbf{rocket} at the \textbf{earliest} in 20\textbf{18}\underline{.}
But also Rem\textbf{brand}\underline{t} \textbf{Sc}\textbf{\underline{holz}}\underline{,} an old-age researcher at the \textbf{Max} \textbf{Planck} \textbf{Institute} in Ro\textbf{stock}\underline{,} has heard of the \textbf{senior}\underline{s} in Central Asia.
However, due to a lack of documents, no scientific \textbf{proof} of age should be provided, especially since there was no \textbf{register} of persons.
In the kitchen, guests can enjoy \textbf{tea} served in the \textbf{typical}\underline{,} bau\textbf{chy} \textbf{Arm}\underline{a}du \textbf{glass}\underline{es}.
\textbf{Through} short-term \textbf{Twitter}\underline{,} he \textbf{accused} \textbf{Mor}\underline{si}'s followers of wanting to lead a "p\textbf{unch} against democracy."
And several \textbf{judges} \textbf{announced} that they would not \textbf{monitor} the \textbf{referendum}\underline{,} which would in\textbf{valid}\underline{ate} it.
These measures are \textbf{flag}\textbf{\underline{rant}} \textbf{violations} of democratic rules of play and will lead \textbf{Egypt} into a new \textbf{dictatorship}\underline{.}
A demon\textbf{str}\underline{ator} on the Tahrir warns: "\textbf{You} fight a \textbf{monster} you can't control."
For example, one has to \textbf{imagine} the wet-absor\textbf{bing} \textbf{smell} of Rakfisk, one of \textbf{Norway} u2019s great \textbf{delicacies}\underline{.}
\textbf{Around} us, people \textbf{consume} small fish \textbf{cu}\textbf{\underline{bes}} and \textbf{drink} large \textbf{amounts} of \textbf{alcohol}\underline{.}
After \textbf{81} years in power, the \textbf{PRI} was \textbf{replaced} by \textbf{Vice}\textbf{\underline{nte}} \textbf{Fox} in \textbf{2000.}
When President \textbf{Pen}\underline{a} \textbf{Nie}\underline{to} receives the Presidential \textbf{Assembly} on \textbf{Saturday}\underline{,} he also \textbf{assume}\underline{s} a great responsibility.
Our \textbf{identity} may sometimes be \textbf{blu}\underline{r}red, but as far as our \textbf{loyalty} is concerned, this is not the case.
The \textbf{ceasefire} between Israel and \textbf{Hamas} may \textbf{prove} to be an \textbf{unexpected} \textbf{cornerstone} of peace.
Indeed, \textbf{Hamas} in the West Bank is \textbf{winning}\underline{,} \textbf{controlled} by the \textbf{rival}\underline{,} \textbf{moderate} \textbf{Palestinian} group \textbf{Fatah}\underline{.}
The \textbf{Israeli} \textbf{missile} \textbf{defence} system, the 'Iron \textbf{Dom}\underline{e}', has \textbf{proved} its \textbf{worth} and many of the \textbf{Hamas} \textbf{rocket}\underline{s} have been \textbf{destroyed}\underline{.}
"The laws will have serious, unin\textbf{tended} consequences," \textbf{says} \textbf{Scott} \textbf{Mc}\underline{In}tyre of British American To\textbf{bac}\underline{co} \textbf{Australia}\underline{.}
These have now been \textbf{extended} to more than 40 countries, including \textbf{Brazil}\underline{,} Turkey and Ukraine.
"I used to take an \textbf{hour} to sort a delivery, now I need four," \textbf{Yu} \textbf{says}\underline{.}
This forces the \textbf{brain} to get lost in interesting \textbf{thoughts}\underline{,} which may encourage \textbf{creativity}\underline{.}
\textbf{Sometimes} we believe that we are \textbf{bo}\underline{ring}, even if we have only \textbf{difficulty} in \textbf{concentrating}\underline{.}
The child not only learns to talk but also \textbf{gains} more self-\textbf{control} in other areas.
My \textbf{biggest} \textbf{dream} has always been to get a \textbf{seat} at \textbf{Oxford} University.
\textbf{Well}\underline{,} according to current reports, a new \textbf{generation} of \textbf{moderate} right-\textbf{wing} students \textbf{suffer} similar \textbf{persecution}\underline{.}
In other \textbf{universities}\underline{,} \textbf{conservative} students say that they are \textbf{regarded} as '\textbf{scape}\underline{go}\textbf{ats} for \textbf{introducing} higher \textbf{tu}\textbf{\underline{ition}} \textbf{fees}\underline{'}.
In the six\textbf{ties} and \textbf{seven}\textbf{\underline{ties}} the two \textbf{lived} in the \textbf{Alps} and were good friends.
I like the \textbf{colors} he \textbf{uses} very much; they have a lot of light and \textbf{highlight} the face.
"I have always \textbf{noticed} his \textbf{refine}\underline{ment}, his \textbf{calm}\underline{ness}, his well-\textbf{kept} and perfect \textbf{appearance}\underline{",} D'\textbf{Ar}\textbf{\underline{enberg}} \textbf{admit}\underline{s}.
\textbf{Jorge} \textbf{assure}\underline{s} to know 35 friends he has in FB and \textbf{nine} followers in \textbf{Twitter}\underline{.}
\textbf{Unlike} \textbf{Jorge}\underline{,} this \textbf{boy} would \textbf{upload} \textbf{photos} of \textbf{acquaint}\underline{ance}s in \textbf{uncomfortable} or \textbf{embarrassing} \textbf{situations}\underline{.}
\textbf{Yes}\underline{,} I would do that if he is uns\textbf{ym}\textbf{\underline{path}}\textbf{\underline{etic}} to me or if I want to \textbf{wipe} him out.
\textbf{Have} you asked the other people for \textbf{permission} before \textbf{labelling} \textbf{photos} of \textbf{celebration}\underline{s}?
\textbf{According} to \textbf{Guard}\underline{ia} the children must be \textbf{reminded} of the \textbf{lesson} "\textbf{You} should not talk to \textbf{strange}\underline{rs}".
"I may meet President \textbf{Daniel} \textbf{Ortega} tomorrow (S\textbf{atur}\underline{day})," \textbf{Santo}\underline{s} said.
The change was for \textbf{improvement}\underline{,} I \textbf{feed} \textbf{myself} well, drive sport and take the \textbf{medicines}\underline{.}
E\textbf{mission} is the first of four \textbf{equivalent} emissions that \textbf{promise} interest \textbf{payments} every 28 days.
This was the beginning of \textbf{Min}\underline{cy}, one of the best players \textbf{Puerto} \textbf{Rico} has ever had.
And this without taking into account his \textbf{career} in the different \textbf{league}\underline{s} in which he played.
But it was his \textbf{master}\underline{ly} \textbf{interpretation} of the \textbf{magical}\underline{ly} des\textbf{pic}\underline{able} J.R. that made \textbf{Hag}\underline{man} a superstar.
\textbf{Martin} was still a young man when she got La\textbf{rry} during her \textbf{marriage} with Bar \textbf{Ben} \textbf{Hag}\underline{man}.
25-\textbf{year}\underline{-}\textbf{old} \textbf{student} \textbf{Will} We\textbf{kes}\underline{a} for \textbf{Psycho}\textbf{\underline{logy}} and Nursing \textbf{explains} that he has seen all apocaly\textbf{ptic} \textbf{films}\underline{.}
The new \textbf{electoral} laws require \textbf{voters} to present a photo \textbf{ID} and \textbf{proof} of US \textbf{citizenship}\underline{.}
\textbf{Before} the 2006 elections, no US state required the \textbf{electorate} to show a photo \textbf{ID}\underline{.}
However, more than a \textbf{hundred} \textbf{dollars} are often to be paid in order to \textbf{obtain} the necessary card.
For example, only 16 out of \textbf{34} states have \textbf{passed} laws \textbf{requiring} a photo \textbf{identification} card.
However, the new rules introduced in \textbf{2012} will \textbf{undoubtedly} make it more difficult to exercise the right to vote.
Too much \textbf{increases} the risk of a w\textbf{rath} or \textbf{fat}\underline{ten}ing \textbf{cancer}\underline{.}
Con\textbf{serv}\underline{ation} of \textbf{meat} by \textbf{smokers}\underline{,} \textbf{dry}\underline{ing} or \textbf{salt}\underline{s} can lead to carcin\textbf{ogen}\underline{s}.
A few weeks ago Mr L. \textbf{lived} alone in his apartment in \textbf{Mont} xe9r xe9\textbf{gie}\underline{.}
\textbf{Patient}\underline{s} \textbf{admitted} to \textbf{Victor}\underline{-}\textbf{Ga}\textbf{\underline{db}}\textbf{\underline{ois}} \textbf{Pal}\underline{li}ative \textbf{Care} Home \textbf{suffer} from \textbf{cancer}\underline{.}
For Mrs A., \textbf{89} years, the \textbf{worst} \textbf{fear} is to die '\textbf{conscious}\underline{ly} and by s\textbf{uff}\textbf{\underline{oc}}\underline{ation}'.
I \textbf{fear} that \textbf{patients} want to die only because they do not receive \textbf{adequate} \textbf{healthcare}\underline{.}
And at the same time, despite the \textbf{worst} \textbf{prediction}\underline{s}, several onc\textbf{ologist}\underline{s} are \textbf{treating} their \textbf{patients} with obsessiveness until the last day.
The chances of \textbf{survival} of H xe9l xe8ne \textbf{Richard} were already \textbf{minimal} when she \textbf{stopped} an ard\textbf{uous} chemo\textbf{therapy}\underline{.}
It must be made clear, however, that \textbf{pal}\underline{li}ative care is not \textbf{om}\underline{ni}\textbf{pot}\underline{ent} in \textbf{pain} treatment.
We can no longer \textbf{pretend} that we do not see this side of \textbf{suffering}\underline{.}
He is supported by co-\textbf{train}\underline{ers} like \textbf{Claude} \textbf{Make}\underline{le}le, who played in the same position as me.
He has a \textbf{wealth} of experience and has won many titles with \textbf{prestigious} \textbf{clubs}\underline{.}
The confidence he has placed in me is also an \textbf{explanation} for my \textbf{achievements}\underline{.}
With regard to the \textbf{sums} \textbf{invested}\underline{,} you were \textbf{believed} to be 15 points \textbf{ahead} of the game.
That is why he has come and \textbf{prove}\underline{s} that he is the star of Li\textbf{gue} 1.
With \textbf{Bit}\underline{co}in, all network nodes are \textbf{simultaneously} \textbf{deposit}\underline{ors} of the \textbf{invoice} book, \textbf{auditor}\underline{s}, money issuers as well as \textbf{buyer}\underline{s} and \textbf{seller}\underline{s}.
To achieve the \textbf{quo}\textbf{\underline{rum}}\underline{,} 11 people, \textbf{deputy} members, were added \textbf{yesterday} morning in a \textbf{hurry}\underline{.}
And in the future the question could be raised as to the extent to which civil \textbf{judges} are \textbf{competent} to decide.'
In your view, the only positive point is the ban on \textbf{torture} under Article \textbf{36}\underline{.}
They are located on a \textbf{rock} \textbf{wall} in the \textbf{mountains} at \textbf{450} \textbf{meters} above sea level.
And there are the \textbf{names} of the \textbf{Jewish} children and the lands in which they died.
The \textbf{dead} sea is even warmer and bathed all year round.
The \textbf{secret}\underline{s} are the old town of \textbf{Tel} A\textbf{viv}\underline{,} J\textbf{aff}\underline{a} on the Mediterranean \textbf{coast}\underline{.}
The famous sea \textbf{route} that \textbf{connect}\underline{s} \textbf{Egypt}\underline{,} \textbf{Syria}\underline{,} \textbf{Anatol}\underline{ia} and Meso\textbf{pot}\textbf{\underline{ami}}\underline{a} \textbf{ran} through this city.
In particular, responds \textbf{spoke}\underline{s}\textbf{person} of the \textbf{immigration} \textbf{authority}\underline{,} it is a question of \textbf{reducing} the number of \textbf{forced} labourers.
If you do not have this status, there is no \textbf{examination} and therefore no official work.
Many \textbf{migrants} \textbf{confirm} that it is not easy to \textbf{obtain} official status in Russia.
At the moment, according to the \textbf{authors}\underline{,} it is possible to find any \textbf{weapon} for little money in \textbf{Moscow}\underline{.}
\textbf{Price}\underline{s} and products made \textbf{Wal}\underline{mar}t one of the largest companies in the USA.
For them, this would be a yearly increase in \textbf{spending} of only \textbf{USD} \textbf{12.}\textbf{\underline{39}} \textbf{compared} to today.
At present, \textbf{federal} and New York legislation \textbf{puts} the minimum \textbf{wage} at \$7.25 an \textbf{hour}\underline{.}
How it is possible to spend so little money in New York is \textbf{incomprehensible} to me.
In fact, any kind of \textbf{interaction} with \textbf{computers} is good, but each in its particular \textbf{ni}\textbf{\underline{ches}}\underline{.}
It is still relatively large but could \textbf{theoretical}\underline{ly} be reduced to the size of a wrist\textbf{watch}\underline{.}
\textbf{Where}\underline{ver} \textbf{Kir}\textbf{\underline{ill}} \textbf{Mill}\underline{er}'s images are \textbf{displayed}\underline{,} they \textbf{attract} huge \textbf{crowd}\underline{s} of people.
I love \textbf{theatre}\underline{,} \textbf{fashion}\underline{,} music, in fact everything \textbf{except} \textbf{literature}\underline{.}
The \textbf{gallery} "D \textbf{137}\underline{"} or the \textbf{club} "Griboedov" also have their origins in art \textbf{clinic}\underline{.}
I won in the \textbf{category} "artists of the year" and so I was at the \textbf{cli}\textbf{\underline{max}}\underline{.}
\textbf{Caravan}\underline{s} of spaceships with \textbf{Earth} \textbf{residents} on board are looking for a \textbf{replacement} \textbf{planet}\underline{.}
The question of \textbf{reproduction} in space was first \textbf{discussed} by \textbf{researchers} with regard to \textbf{flora}\underline{.}
\textbf{Homo} sapiens is \textbf{capable} of \textbf{abstract} \textbf{thinking} and can create a similar \textbf{emotional} \textbf{background}\underline{.}
The body cannot develop the s\textbf{kel}\underline{e}ton and the \textbf{muscle}\underline{s} without \textbf{feeling} it.
A similar \textbf{outcome} \textbf{appears} to have been achieved by joint control by Czech and German \textbf{auditor}\underline{s}.
As a negative example of practice, he \textbf{refers} to the \textbf{attitude} of \textbf{Prime} Minister \textbf{Petr} Ne  u20\textbf{47} as to the so-called '\textbf{black} system'.
But lowering \textbf{threshold}\underline{s} for \textbf{contracts} does not guarantee that we will achieve this objective.
In the \textbf{district} of \textbf{Karl}\underline{ov}y Vary this morning, the \textbf{streets} were easily \textbf{accessible}\underline{,} with some \textbf{smooth} \textbf{snow} and \textbf{ice}\underline{.}
This is \textbf{fro}\underline{s}ty in the morning, with \textbf{temperatures} between 3 and 9 \textbf{degrees} below the \textbf{freezing} point.
It goes without saying that, at the end of the day, everything will work and the world will not end...
The students of the Jedli  u20\textbf{47} \textbf{ka} \textbf{Institute} are \textbf{regularly} \textbf{supervise}\underline{d} by \textbf{lecture}\underline{rs} who help them with various \textbf{leisure} activities.
It is not even self-\textbf{evident} there that a \textbf{wheelchair} user is left in the \textbf{lift}\underline{,} for example.
\textbf{Fortunately}\underline{,} \textbf{clubs} are also being set up there trying to draw attention to the problems of people with \textbf{disabilities}\underline{.}
From the very beginning, I have \textbf{felt} the potential for a different approach.
The first \textbf{impression} the viewer usually has is of course compassionate; that is only natural...
This is how it works \textbf{everywhere}\underline{,} in every \textbf{band} that is \textbf{seriously} working and \textbf{wants} to achieve something.
We are an open group; people come and go, and that cannot be \textbf{prevented}\underline{.}
The committee was set up in \textbf{1937}\underline{,} but after two years of work its work was \textbf{completed} from the beginning of the war.
The \textbf{proof} of this is the \textbf{existence} of a \textbf{lobby} that is \textbf{virtually} \textbf{om}\underline{ni}\textbf{pot}\underline{ent} and \textbf{om}\underline{ni}\textbf{present} in all states.
The history of \textbf{humanity} is first and \textbf{foremost} a history of \textbf{fighting} for power.
\textbf{Who}\textbf{\underline{ever}} \textbf{tried} to \textbf{oppose} this family had to pay with his life for it.
A world where the rest of the human population \textbf{serves} a small group of financial a\textbf{risto}\underline{c}\textbf{rats}\underline{.}
The \textbf{fate} of the \textbf{hostage}\underline{s} created a \textbf{wave} of solidarity and anti-Iranian \textbf{sentiment}\underline{s} at home.
The plan developed by the \textbf{expert} for "\textbf{Ex}\textbf{\underline{filtration}}\underline{",} \textbf{Tony} Mendez, also required \textbf{Hollywood}\underline{'}s cooperation.
A similar \textbf{restriction} already applies to children up to 14 years of age when using annual market \textbf{roast}\underline{ing}.
The Czech Republic, for example, \textbf{exceeded} the \textbf{volume} set for can\textbf{ned} \textbf{mushroom}\underline{s}, for which we were \textbf{threatened} with a \textbf{heavy} fine.
Mr \textbf{Senator}\underline{,} how do you think of \textbf{standing} for President?
People have \textbf{chosen} such a senate that changes will be very difficult to implement.
\textbf{Nevertheless}\underline{,} I will fight for my \textbf{vision}\underline{s}, e.g. for the direct \textbf{election} of \textbf{mayor}\underline{s} and \textbf{district} leaders.
The cost of the \textbf{campaign} is \textbf{basically} covered by my \textbf{salary} as a senator.
So that is my proposal for the \textbf{Sp}\textbf{\underline{ijk}}\underline{en}\textbf{isse} \textbf{Book}\underline{berg}, for the so-called Boek\textbf{enberg}\underline{!}
In early November the Buchberg was \textbf{awarded} the second \textbf{prize} "\textbf{Best} \textbf{Library} of \textbf{NL} \textbf{2012}\underline{".}
A special \textbf{pleasure} are the black \textbf{books}\underline{h}\textbf{elf}\underline{s}, which are sometimes \textbf{wall} \textbf{covering}\underline{s}, sometimes \textbf{bra}\underline{ces}, sometimes \textbf{pole} \textbf{bal}\underline{us}\textbf{trade}\underline{s}.
\textbf{According} to \textbf{Stephen} Szabo, an \textbf{expert} on US-\textbf{European} relations, Berlin is \textbf{balancing} on a \textbf{narrow} \textbf{diplomatic} level.
But because of the political situation here, the government cannot, of course, \textbf{defend} this position \textbf{publicly}\underline{.}
I believe that the actual \textbf{differences} are not as great as they always \textbf{seem}\underline{.}
But I believe that the Germans know that they must play a more independent role.
\textbf{Five} years ago \textbf{Freud}\textbf{\underline{enberg}} offered the other side in \textbf{va}\underline{in} a "\textbf{high} six-\textbf{figur}\underline{e} euro" for \textbf{settlement}\underline{.}
For example, a Chinese \textbf{manufacturer} in Germany wanted to \textbf{register} the name \textbf{Freud}\textbf{\underline{enberg}} for \textbf{shoes} and \textbf{leather}\underline{.}
More than 300 of them no longer have \textbf{parents} because they have \textbf{suc}\textbf{\underline{cum}}\textbf{\underline{bed}} to the \textbf{HI} \textbf{virus}\underline{.}
\textbf{According} to European \textbf{survey}\underline{s}, three \textbf{quarter}\underline{s} of all \textbf{infection}\underline{s} \textbf{affect} young people a\textbf{ged} between 15 and \textbf{25.}
In the village itself, \textbf{Zo}\underline{d}wa Dla\textbf{mini}\underline{,} a \textbf{confident} and \textbf{assert}\underline{ive} \textbf{woman}\underline{,} manages the funds from Germany.
She also takes care that the \textbf{orphan}\underline{s} get well, for example with one of the \textbf{grand}\underline{m}\textbf{other}\underline{s}.
The Gogos, as the old women in Zulu are called, are the support of the village.
'Aids is an \textbf{absolute} \textbf{taboo}\underline{'}, \textbf{says} \textbf{Anne}\textbf{\underline{tte}} Len\textbf{nar}\textbf{\underline{tz}}\underline{,} 'because it has to do with \textbf{sexual}\underline{ity}'.
The \textbf{probe} \textbf{Messenger} has found \textbf{evidence} that there is \textbf{ice} on the \textbf{planet} \textbf{Mer}\textbf{\underline{kur}}\underline{.}
The Pleyad \textbf{Cluster}\underline{,} also called "The \textbf{Seven} S\textbf{ister}\underline{s}", can be seen with the \textbf{naked} \textbf{eye} at night.
This \textbf{baby} star in its full \textbf{beauty} was only \textbf{absorb}\underline{ed} by the \textbf{infrared} \textbf{detect}\underline{ors} of the \textbf{tip}\underline{r} \textbf{telescope}\underline{.}
Sa\textbf{turn} and his \textbf{ring}\underline{s}: How they were created is one of the great \textbf{rid}\textbf{\underline{dle}}\underline{s} of astro\textbf{nom}\underline{y}.
This group of \textbf{galaxies}\underline{,} called Arp 273, took up the Hu\textbf{bble} space \textbf{telescope} for the Nasa.
\textbf{Tourist}\underline{s} from Europe do not come here, it is difficult to get to \textbf{Azerbaijan}\underline{'}s capital Baku.
She has always only \textbf{eat}\underline{en} what came from her own \textbf{farm}\underline{,} to\textbf{mato}\underline{es}, \textbf{potatoes}\underline{,} peas.
For this, another for\textbf{bid}\underline{s} \textbf{insult}\underline{ing} or slandering the \textbf{Prophet} \textbf{Mohammed} and his \textbf{messenger}\underline{s}.
"Instead of \textbf{strengthening} civil society, the President de \textbf{facto} \textbf{suspend}\underline{s} it," Saeda \textbf{complain}\underline{s}.
In\textbf{habit}\textbf{\underline{ants}} of the resort \textbf{attribute} to it the development of tourism and the construction of infrastructure.
He is a very direct man, very committed and has great plans for the country.
He is an excellent statesman, but above all he is \textbf{someone} who can \textbf{listen}\underline{.}
"But this is not possible if there were so many \textbf{formal} \textbf{errors} and \textbf{omission}\underline{s}," she \textbf{says}\underline{.}
Not to know what \textbf{happened} to him or to the outside world was \textbf{burden}\textbf{\underline{some}}\underline{.}
We are also aware that many members of the \textbf{Mexican} \textbf{leadership} do not like us.
But there are reasons to believe that the \textbf{dead}\underline{ly} \textbf{sta}\underline{le}\textbf{mate} may finally end.
And \textbf{Hamas} leaders may \textbf{conclude} that they have time on their side.
Chinese and \textbf{Indonesia}\underline{n} \textbf{counterfeit}\underline{ers} will offer much larger \textbf{quantities} of these products on \textbf{Australia}\underline{'}s \textbf{roads}\underline{.}
The house \textbf{walls} of Pompe\textbf{ji} a\textbf{dor}\underline{n} a \textbf{Latin} \textbf{gra}\textbf{\underline{ffi}}\underline{ti} with \textbf{bo}\underline{re}\textbf{dom} \textbf{dating} back to the first century.
To measure these \textbf{differences}\underline{,} \textbf{researchers} developed a "scala to \textbf{bo}\underline{re}\textbf{dom}\underline{"} in the \textbf{1980}\underline{s}.
\textbf{Instead}\underline{,} our aim should be to feel comfortable even outside the \textbf{constant} activity and technology requi\textbf{site}\underline{s}.
Not because of my very \textbf{unusual} name or because I had come from a private school.
People believe we are like the \textbf{Bull}\underline{ing}\textbf{don} Club without even getting to know us".
"\textbf{Mi}\underline{s}s Wy\textbf{att}\underline{,}" said the \textbf{tut}\underline{or} \textbf{Harry} \textbf{Pit}\underline{t} (\textbf{now} \textbf{dead}\underline{),} "\textbf{ple}\textbf{\underline{ase}} \textbf{translate} the first \textbf{paragraph}\underline{.}
"\textbf{Do}\underline{es} Thatcher followers \textbf{refuse} to learn French, or are they just \textbf{stupid}\underline{?}" he asked me.
I \textbf{insisted} that I did not agree with Mrs Thatcher on all points.
In 1997 he accepted a \textbf{professor}\underline{ship} at the University of Bi\textbf{lk}\underline{ent} in \textbf{Ankara}\underline{,} Turkey.
But no 18-\textbf{year}\underline{-}\textbf{old} should ever \textbf{suffer} such \textbf{intimidation} and malice in an \textbf{educational} \textbf{institution}\underline{.}
He \textbf{sat} at the table of the \textbf{Count}\underline{es}s Jacqueline de Ri\textbf{bes}\underline{,} a very good \textbf{friend} of \textbf{mine}\underline{.}
Kawah Ijen \textbf{mine}\textbf{\underline{work}}\underline{ers} \textbf{earn} 5 euro \textbf{cent}\underline{s} for each \textbf{kilo} of \textbf{sulphur} they de\textbf{ple}\underline{te}.
"I do not know if \textbf{someone} \textbf{answers} me, I only \textbf{upload} them" he \textbf{adds}\underline{.}
"\textbf{This} does not f\textbf{right}\underline{en} me because we have something in common, for example music," he \textbf{says}\underline{.}
The digital \textbf{native}\underline{s} are they, the children and young people who have \textbf{grown} up with this technology.
"\textbf{If} I have to die, then I \textbf{prefer} to \textbf{burst} three times," they say in my case.
There are things I would have introduced, such as regionalisation of the lower \textbf{categories}\underline{.}
At least I see the result of the \textbf{prescribed} training and \textbf{courses} for trainers, table \textbf{officials} and referees.
And of course I enjoy the company of my \textbf{wife} \textbf{Isabel}\underline{,} who has always been with me.
He was \textbf{creative}\underline{,} \textbf{generous}\underline{,} \textbf{funny}\underline{,} \textbf{funny}\underline{,} \textbf{loving} and \textbf{talented} and I will \textbf{miss} him very much.
In 1995 a m\textbf{align}\underline{ant} \textbf{tum}\textbf{\underline{our}} was found in his liver and he was \textbf{subjected} to a trans\textbf{plant}\underline{.}
In 2001 he \textbf{named} his memoirs "H\textbf{ello} \textbf{Dar}\underline{lin}: Tall (and \textbf{Absolut}\underline{e}ly \textbf{Tru}\underline{e}) \textbf{Tal}\underline{es} about My \textbf{Life}\underline{".}
For weeks before the beginning of the \textbf{semester} we received e-mails from students who asked if there were still places available.
The apocaly\textbf{ptic} \textbf{sec}\underline{t} or \textbf{religious} \textbf{mental}\underline{ity} is actually only a question of con\textbf{sol}\underline{ation} or its \textbf{absence}\underline{.}
"N\textbf{ever} have I heard of any \textbf{lessons} where this is \textbf{taught}\underline{,}" he said.
\textbf{Republican} leaders \textbf{justify} their policies by the need to combat \textbf{electoral} \textbf{fraud}\underline{.}
Moreover, five million new \textbf{voters} in \textbf{2012} do not have such a card.
But one thing is certain: these new provisions will have a negative impact on turnout.
This \textbf{leads} to greater \textbf{hesitation} on the part of men who are already indecisive about \textbf{carrying} out early \textbf{detection} \textbf{tests}\underline{.}
"\textbf{To}\underline{day} there are still \textbf{1.5} million \textbf{smokers} in \textbf{Quebec}\underline{,}" \textbf{complain}\underline{s} \textbf{spoke}\underline{s}\textbf{person} Andr xe9 \textbf{Beau}\textbf{\underline{lie}}\underline{u}.
They appear to increase the risk of \textbf{breast}\underline{,} w\textbf{rath}\underline{,} in\textbf{test}\underline{ine}, oeso\textbf{pha}\textbf{\underline{gus}}\underline{,} \textbf{pan}\textbf{\underline{cre}}\textbf{\underline{atic}} and \textbf{uter}\underline{ine} \textbf{cancer}\underline{.}
In recent years, several \textbf{scientists} have \textbf{studied} the link between \textbf{vitamin} \textbf{additives} and \textbf{cancer}\underline{.}
The effect of \textbf{vitamin} D on \textbf{cancer} has also not been clearly \textbf{demonstrated}\underline{.}
In addition, applications can also be \textbf{derived} from all the instruments \textbf{surrounding} research.
"\textbf{It} is always a \textbf{shock}\underline{,} you cannot be prepared for it," he \textbf{says}\underline{.}
"\textbf{Th}\underline{at} \textbf{depends} on the ability of the person," he \textbf{notes}\underline{,} to accept a \textbf{backward} step.
This is very little if we take into account the fact that one day we will all die.
\textbf{Patient}\underline{s} without \textbf{pain} alleviation will increasingly be able to use this \textbf{terminal} sedation.
In May we were \textbf{disappointed} because we were strong enough to \textbf{win}\underline{.}
We have \textbf{punished} \textbf{Afghan} farmers in particular by \textbf{seeing} them as \textbf{terrorists}\underline{.}
The convo\textbf{ys} of \textbf{truck}\underline{s} and \textbf{tank}\underline{s} \textbf{flow}\underline{n} by \textbf{helicopter}\underline{s} have reached Ka\textbf{bul} without being \textbf{attacked}\underline{.}
President \textbf{Kar}\underline{za}  u20\textbf{47}  does not want foreign \textbf{controls}\underline{,} especially in the elections \textbf{planned} for April \textbf{2014}\underline{.}
\textbf{Traditional}\underline{ly}, people of different \textbf{faith}\underline{s} leave their \textbf{mark} there with \textbf{wishes} that can be \textbf{fulfilled}\underline{.}
For this there are many well-n\textbf{our}\textbf{\underline{ished}} \textbf{cat}\underline{s}, who \textbf{scattered} through the \textbf{streets} in a comfortable and uncon\textbf{tamin}\underline{ated} way.
In \textbf{2012}\underline{,} more than three million \textbf{tourists} from all over the world \textbf{visited} Israel.
\textbf{Language} \textbf{skills} must be \textbf{proven} both for \textbf{obtaining} and for \textbf{extending} work \textbf{permits}\underline{.}
In \textbf{2011}\underline{,} a report was \textbf{drafted} by the Centre for Problem \textbf{Analysis} and Government \textbf{Administration}\underline{.}
\textbf{According} to him, it is more common for \textbf{traders} to \textbf{obtain} \textbf{supplies} in a \textbf{stock}\textbf{\underline{pil}}\underline{e}.
A \textbf{weapon}\underline{,} for example a \textbf{gun} of the type \textbf{TT}\underline{,} is \textbf{bought} by means of an \textbf{attachment}\underline{.}
\textbf{According} to Baranez, the \textbf{buyer} does not get the \textbf{cat} in the \textbf{bag}\underline{,} but can try it out.
But it is also difficult for objective reasons to set up trade \textbf{unions} in the fast-\textbf{food} sector.
There were \textbf{loud} \textbf{protests} that day before many other fast-\textbf{food} restaurants in \textbf{Manhattan}\underline{.}
An interesting method is currently the use of the second hand as a \textbf{somewhat} \textbf{unusual} \textbf{projection} document.
I used to be social, but now it \textbf{hurt}\underline{s} and is \textbf{afraid} to be so.
In fact, there are only two real \textbf{planet}\underline{s} that we could at least in\textbf{habit} \textbf{hypothe}\underline{t}\textbf{ically}\underline{.}
\textbf{Animal}\underline{s} taken out of their natural \textbf{habitat} simply cannot follow their \textbf{prop}\underline{ag}ation.
Here in a \textbf{suspended} state the cosmon\textbf{aut}\underline{s} \textbf{win} \textbf{routine} for work in open space.
For example, \textbf{birth} could also take place in a special \textbf{chamber} to blackmail the child.
Is there a similar \textbf{authority} here to our \textbf{NK}  u20\textbf{47} , or does the system work \textbf{differently}\underline{?}
\textbf{Temperatur}\underline{es} have fallen to -5 to -10   u20\textbf{47} C. During the day it is to be warmer.
In East \textbf{Bohemia} it is \textbf{mostly} \textbf{sunny} or \textbf{ser}\underline{en}e today and it remains \textbf{largely} free of \textbf{rain}\underline{.}
The \textbf{temperature} \textbf{varies} between -3 and \textbf{+1}   u20\textbf{47} C, there is a \textbf{weak} \textbf{wind}\underline{.}
In the south of the \textbf{Pil}\underline{s}en and Tachov \textbf{circle}\underline{s}, however, there may be a \textbf{phase}\underline{d} \textbf{smooth}\underline{ing} of the \textbf{ice}\underline{.}
\textbf{Drive}\underline{rs} should be particularly \textbf{careful} on the less \textbf{frequent}\underline{ed} \textbf{roads} in the   u20\textbf{47} um\textbf{ava} area.
What do you think the world will end in less than a month?
In December you will also \textbf{realize} a unique project with three \textbf{concerts} against the end of the world.
The \textbf{Tap} \textbf{Tap} is, however, a group of people with \textbf{disabilities}\underline{.}
But the \textbf{band} only became known in recent years, or am I \textbf{mistake}\underline{n}?
\textbf{Thanks} to EU funding, we can also \textbf{afford} good \textbf{readers}\underline{,} high-\textbf{quality} equipment and so on.
We always welcome those who have the will and want to \textbf{participate}\underline{.}
\textbf{Make}\underline{s} take place the day before the \textbf{predicted} end of the world, \textbf{Thursday} \textbf{20.}\underline{12}.2012 at 21 o'\textbf{clock}\underline{.}
It is certainly interesting to look at the problem from a \textbf{broader} \textbf{perspective}\underline{.}
\textbf{Ultimate}\underline{ly}, this means that the different \textbf{economies} are in permanent conflict with each other.
This situation is well known, so there is no need for specific \textbf{statistics} here.
Such a \textbf{scandal} has also been \textbf{exposed} in the case of aid workers \textbf{employed} in the German \textbf{Bundestag}\underline{.}
The \textbf{repeal} of the law on \textbf{voluntary} work is not a solution here, at least not a permanent one.
At the same time, it is Af\textbf{fleck} u2019s first film that does not play in the \textbf{director} u2019s home\textbf{town} \textbf{Boston}\underline{.}
Af\textbf{fleck} also shows this \textbf{feeling} in Argo, where Te\textbf{hra}\underline{n} is "\textbf{play}\underline{ed}" by \textbf{Canada}\underline{.}
With an EU brand, the \textbf{Par}\underline{du}\textbf{bic} gingerb\textbf{read} or the Ho  u20\textbf{47} \textbf{ice}\underline{r} \textbf{roll}\underline{s} can \textbf{boast}\underline{.}
A strong person who points to mal\textbf{administration} can put pressure on the political \textbf{scene}\underline{.}
The \textbf{thin} \textbf{fabric} lasts one or two seasons, after which it is \textbf{rip}\underline{e} for waste.
Germany \textbf{abstained} in the vote on the \textbf{admission} of \textbf{Palestine}\underline{.}
Germany wanted to \textbf{demonstrate} its \textbf{independence} without being too critical of Israel.
That is the old problem: you do not want to be \textbf{surrounded} by \textbf{hostile} countries.
It must be \textbf{recep}\textbf{\underline{tive}} to different \textbf{neighbours} and \textbf{opinions}\underline{,} and that is not easy.
The imit\textbf{ators} are already able to use a few additional \textbf{letters} to \textbf{register} their \textbf{trademarks}\underline{.}
We know that the Chinese are world \textbf{champion}\underline{s} in \textbf{copy}\underline{ing} and injuring \textbf{intellectual} property.
However, \textbf{delete}\underline{s} of \textbf{dubious} \textbf{entries} in the \textbf{trademark} \textbf{register} are difficult to reach and go into money.
Last year, however, we had \textbf{returned} from the 'em\textbf{erg}\textbf{\underline{ency}} situation in the \textbf{workflow} to normality'.
\textbf{Simpl}\textbf{\underline{ified}}\underline{,} this means that each \textbf{registration} costs an \textbf{average} of 1280 \textbf{yu}\underline{an} or \textbf{160} \textbf{euros}\underline{.}
In \textbf{Heidelberg}\underline{,} the \textbf{Chor} Im\textbf{bon}\underline{gi} is \textbf{testing} - and \textbf{Aid}\underline{s}waisen are pleased about this in Swaziland.
\textbf{Sy}\textbf{\underline{phil}}\underline{is} and Tri\textbf{pper} are especially common in men who have \textbf{sex} with men.
\textbf{Actually} \textbf{strange} in a country where the \textbf{king} \textbf{officially} \textbf{holds} 14 \textbf{wi}\textbf{\underline{ves}}\underline{.}
The last \textbf{absolute} \textbf{monarch} of \textbf{Sub}\underline{-}\textbf{Saharan} Africa, \textbf{King} Msw\textbf{ati} \textbf{III}\underline{,} is famous for his \textbf{excessive} \textbf{lifestyle}\underline{.}
It should be at least 30 \textbf{cent}\underline{i}\textbf{metre}\underline{s} \textbf{thick} and perhaps even up to 20 metres \textbf{thick}\underline{.}
From time to time, they send images to the \textbf{earth}\underline{:} small \textbf{hole}\textbf{\underline{hole}}\underline{s} in \textbf{endless} \textbf{exp}\textbf{\underline{ans}}\underline{es}.
They may be the remains of a Sa\textbf{turn} \textbf{moon} that \textbf{disappeared} without \textbf{trace} some 4.5 billion years ago.
If you don't have technical abbreviations, you may call them the \textbf{southern} \textbf{fire} \textbf{wheel}\underline{.}
The photo of the Hu\textbf{bble} space \textbf{telescope} shows a section from the I\textbf{ris}\underline{ne}bel in the con\textbf{stell}\underline{ation} \textbf{Ke}\underline{ph}eus.
It shows a \textbf{ring} of black \textbf{holes}\underline{,} 430 million light years from the \textbf{Earth}\underline{.}
It takes \textbf{eight} hours for the 3\textbf{23} km because the road is only one lane.
But \textbf{Pil}\textbf{\underline{ata}} Fatu\textbf{lay}\textbf{\underline{eva}} (\textbf{48}\underline{)} is \textbf{convinced} that Le\textbf{rik} has the \textbf{stuff} for the tourist \textbf{attraction}\underline{.}
She is the \textbf{director} of the Museum of \textbf{Long}\textbf{\underline{ev}}\underline{ity}, probably the only one in the world.
She \textbf{sit}\underline{s} on the floor with a \textbf{butter} k\textbf{eg} that \textbf{roll}\underline{s} her \textbf{rel}\underline{ent}\textbf{lessly} back and \textbf{forth}\underline{.}
\textbf{Through}\underline{out} my life I have not \textbf{bought} food in the \textbf{supermarket} once.
He was in power until \textbf{2003,} and later his \textbf{son} \textbf{Il}\textbf{\underline{ham}} took over.
Is it enough for a \textbf{presidential} caricature or a \textbf{joke} at the \textbf{expense} of a \textbf{lawyer}\underline{?}
"The \textbf{revolution} has \textbf{returned} and we will \textbf{win}\underline{,}" said \textbf{Ham}\textbf{\underline{din}} Sabbahi, third-\textbf{place}\underline{d} in the \textbf{presidential} \textbf{election}\underline{.}
They called on \textbf{Mor}\underline{si} to clean up the country and say: 'The \textbf{Kor}\underline{an} is our \textbf{Constitution}\underline{'}.
Not because he \textbf{shares} their world view, but because human rights are indivis\textbf{ible} to him.
I am in the small town of Fagernes, about three hours from \textbf{Oslo}\underline{.}
In any case, such an elk \textbf{bull} is something different.
'\textbf{What} do you have up there in the \textbf{mountains} for the best fish, \textbf{Thor}\underline{-}J xfcrgen?'
In the \textbf{remote} little town of \textbf{Valle} del \textbf{Bra}\underline{vo}, for example, one likes to remember him.
He \textbf{reject}\underline{s} the \textbf{opposition}\underline{'}s \textbf{accus}\underline{ations} that the new \textbf{president} lacks \textbf{substance}\underline{.}
But that is what the victims u2019 families in \textbf{Ciudad} Neza \textbf{fear} most.
"\textbf{My} world \textbf{sh}\underline{r}\textbf{unk} at \textbf{Camp} Ar\textbf{af}\textbf{\underline{jon}}\underline{,} on this cage \textbf{combined}\underline{,}" Manning said on \textbf{Thursday}\underline{.}
Only one \textbf{mattress}\underline{,} \textbf{blanket}\underline{,} f\textbf{lip} \textbf{flo}\underline{ps}, \textbf{clothes} and \textbf{glass}\underline{es} were allowed.
He always had to \textbf{sleep} with light that \textbf{penetrate}\underline{d} into his \textbf{cell} from the outside.
\textbf{Sign}\underline{s} refer to two \textbf{queue}\underline{s}: one for "\textbf{Me}\textbf{\underline{xi}}\textbf{\underline{can}}\underline{os}" \textbf{("}\textbf{\underline{Me}}\textbf{\underline{xi}}\textbf{\underline{can}}\underline{os}\textbf{")}\underline{,} the other for "\textbf{Ex}\underline{tra}nje\textbf{ros}\underline{"} \textbf{("}\textbf{\underline{Aus}}\underline{l} xe4\textbf{nder}\textbf{\underline{").}}
And there was no need for shortenings or \textbf{hy}\textbf{\underline{phen}}\underline{s} in my \textbf{grand}\underline{fa}\textbf{ther}\underline{'}s home country.
So I took my American \textbf{passport} and put me in the sn\textbf{ake} for \textbf{Extra}\underline{n}je\textbf{ros}\underline{.}
Our Spanish will never be good enough, our \textbf{ties} with \textbf{Mexico} will never be strong enough.
At first \textbf{sight}\underline{,} \textbf{optimism} seems to be far from appropriate in view of the current situation.
\textbf{Far} from the white house, it seems as if he is just as \textbf{reluctant} to \textbf{participate}\underline{.}
\textbf{Health} \textbf{Warn}\underline{ing}s and \textbf{Disease}\underline{d} \textbf{Body} \textbf{Part}\underline{s} on \textbf{neutral} green \textbf{pack}\underline{s} that are the same for all \textbf{tobacco} \textbf{brands}\underline{.}
\textbf{Zi}\underline{co} has \textbf{sold} up to \textbf{6,000} \textbf{units} to \textbf{wholesale} \textbf{shops} and is \textbf{awaiting} new \textbf{stocks}\underline{.}
\textbf{According} to P\textbf{lib}\underline{ers}ek, the government has held \textbf{talks} with other countries \textbf{considering} similar \textbf{packaging} laws.
So I had enough time to think about \textbf{bo}\underline{re}\textbf{dom}\underline{.}
But, while \textbf{television} can create \textbf{feelings} of \textbf{happiness} in the short term, they \textbf{eva}\underline{po}rate in the long term.
\textbf{Pit}\underline{t} was a small man with a face like \textbf{cake} do\textbf{ugh}\underline{,} and quite ugly.
\textbf{Would} I ever be able to lead a normal life at \textbf{Oxford} University?
One of my \textbf{male} friends, also Tory \textbf{supporters}\underline{,} \textbf{gave} in to the pressure and \textbf{denied} his \textbf{conviction}\underline{s}.
It was my \textbf{father} who \textbf{hit} the last \textbf{nail} in the co\textbf{ffi}\underline{n} of my \textbf{Oxford} \textbf{career}\underline{.}
I \textbf{hi}\underline{d} in my room and after five minutes my \textbf{eggs} \textbf{gave} up.
When they \textbf{went}\underline{,} I \textbf{packed} a \textbf{suit}\textbf{\underline{case}} and took the first train to London.
"\textbf{He} never comes out of \textbf{fashion} because his \textbf{designs} are works of art" she \textbf{conclude}\underline{s}.
He likes people with good education and the highest titles, and they love him.
"\textbf{It} was a \textbf{gift} from him," \textbf{says} Naty Abascal, one of the \textbf{designer}\underline{'}s \textbf{Mus}\underline{es}.
\textbf{About} \textbf{400} \textbf{stra}\underline{ps} are \textbf{loaded} \textbf{onto} their shoulders on the \textbf{cra}\underline{ter} floor with \textbf{sulphur}\underline{.}
Of his five children, the elder with his 30 years also works as a \textbf{sulphur} \textbf{bear}\underline{er}.
This is just for the Internet, so we had to make it \textbf{funny} and \textbf{funny}\underline{.}
Poss\textbf{ible} that many of these ideas were \textbf{creative}\underline{,} but they did not \textbf{necessarily} lead to success.
I \textbf{signed} up to \textbf{Twitter} to express \textbf{myself} and \textbf{write} interesting twe\textbf{ets}\underline{.}
\textbf{Journalist}\underline{s}' access to information on the summit was limited at all times.
\textbf{Conflict}\underline{s} are \textbf{inevitable}\underline{,} but they must be \textbf{overcome} in the \textbf{pursuit} of a common path.
They must be \textbf{dealt} with comprehensively so that they can be \textbf{overcome} and \textbf{looked} forward.
"In no case does it mean a relapse in President \textbf{Ch} xe1vez's state of health," he commented.
There were many \textbf{fulfilling} years, including five \textbf{successive} \textbf{championship}\underline{s} from \textbf{1971} to \textbf{1975}\underline{.}
Was this group of the 1990 World \textbf{Cup} the best national team you have ever seen?
It was \textbf{Krist}\underline{in} who had \textbf{shot} the \textbf{sister}\underline{-}in-\textbf{law} of J.R. (\textbf{interpret}\underline{ed} by \textbf{Mary} \textbf{Cro}\underline{s}by).
He also \textbf{fought} against \textbf{smoking} and \textbf{participated} in several \textbf{campaigns}\underline{.}
And he \textbf{recall}\underline{s} that the bad is good for those with an apocaly\textbf{ptic} \textbf{mental}\underline{ity}.
For example, if nuclear material comes into the \textbf{hands} of \textbf{terrorists}\underline{,} war could break out.
D\textbf{espite} the "before death" the students have to study, create projects and take part in final \textbf{examination}\underline{s}.
One thing is certain: these new provisions will have a negative impact on turnout.
\textbf{Before} 2004, no state asked for \textbf{proof} of \textbf{citizenship} to vote.
The most important thing is to make the right decision as soon as a \textbf{cancer} has been \textbf{identified}\underline{.}
However, it is \textbf{estimated} that \textbf{approximately} \textbf{10\%} of \textbf{cancer}\underline{s} are caused by hereditary \textbf{disease}\underline{.}
\textbf{According} to the \textbf{Canadian} \textbf{Canc}\underline{er} \textbf{Society}\underline{,} obesity and obesity also promote the \textbf{outbreak} of the \textbf{disease}\underline{.}
"The \textbf{latter} can damage the body's \textbf{cells} and lead to the development of \textbf{cancer}\underline{,}" he \textbf{explains}\underline{.}
The debate must \textbf{resume} \textbf{shortly}\underline{,} even though a draft law is being prepared.
The pro\textbf{state} \textbf{cancer} that \textbf{consumed} him left him a two-\textbf{year} period.
You can give the \textbf{dying} person a \textbf{mouth} care with brandy or pepsi.
\textbf{Patient}\underline{s} whose \textbf{pain}\underline{s} are not \textbf{alleviate}\underline{d} say the same thing: 'I want to die'.
He is \textbf{suspected} of \textbf{repeatedly} \textbf{receiving} \textbf{bri}\textbf{\underline{bes}} in exchange for public \textbf{contracts}\underline{.}
\textbf{Financial}\underline{ly}, the \textbf{PS}\underline{G} is giving itself the resources to make this project take \textbf{concrete} \textbf{shape}\underline{.}
But another team, that of \textbf{Mont}\textbf{\underline{pell}}\underline{ier}, has achieved an even better season.
This would mean \textbf{ignor}\underline{ing} our \textbf{opponents} and the French \textbf{championship}\underline{.}
The \textbf{PS}\underline{G} seems to be \textbf{entirely} \textbf{dependent} on the performance of Z\textbf{lat}\underline{an} I\textbf{bra}\underline{hi}m\textbf{ovic}\underline{.}
The national trainer is \textbf{strict}\underline{,} close to the players and encourages \textbf{victory}\underline{.}
\textbf{Blanc} had achieved his goal by \textbf{qualify}\underline{ing} us for the European \textbf{Championship}\underline{.}
Is the \textbf{tie} \textbf{forced} on 16 October in Spain \textbf{(1}\underline{:}\textbf{1)} a prelude?
However, every time trade is \textbf{controlled} and \textbf{processed} by a central \textbf{authority}\underline{.}
To prevent \textbf{inflation}\underline{,} this \textbf{reward} is \textbf{regularly} \textbf{halv}\underline{ed}, probably before the end of \textbf{2012}\underline{.}
In addition, the \textbf{difficulty} of the task is increased with any \textbf{improvement} in \textbf{computing} power.
The web pages that provide services for \textbf{Bit}\underline{co}in have been \textbf{attacked} and the \textbf{Bit}\underline{co}in in\textbf{sol}\underline{es} \textbf{stolen}\underline{.}
The \textbf{ECB} also reports on the \textbf{possibilities} of money \textbf{laundering} through this \textbf{anonymous} service.
And us ourselves with our \textbf{88} \textbf{soldiers} \textbf{killed}\underline{,} as well as the \textbf{injured} and the \textbf{injured}\underline{.}
From the end of \textbf{2014}\underline{,} there will be no more in\textbf{flow}\underline{s} of the \textbf{Taliban} in Ka\textbf{bul}\underline{.}
\textbf{Conditions} have changed since their \textbf{irre}\underline{s}ist\textbf{ible} advance from \textbf{1994} to 1996.
\textbf{Their} takeover was then \textbf{regarded} as a kind of \textbf{liberation} and return to security.
The most important \textbf{figures} of the anti-S\textbf{ovi}\underline{et} war \textbf{returned} to power in 2001.
This new initiative has only led to an even greater \textbf{division} of the country.
The text that was adopted last night \textbf{consists} of 234 \textbf{articles}\underline{.}
This \textbf{refers} in particular to the "Fi\textbf{q}\underline{h}" [Is\textbf{lam}\underline{ic} \textbf{ju}\textbf{\underline{ris}}\textbf{\underline{pru}}\underline{d}ence, \textbf{Note} d. Red.].
The \textbf{Muslim} \textbf{Brot}\underline{her}\textbf{hood}\underline{s} \textbf{argue} that these are \textbf{considerably} reduced \textbf{compared} with the former regime.
It is here that believers take the ordeal or \textbf{cru}\underline{s}\textbf{ade} of \textbf{Jesus} \textbf{Christ} (in \textbf{Latin}\underline{:} \textbf{Via} \textbf{Dol}\underline{or}\textbf{osa}\underline{).}
\textbf{Every} year 13 million guest workers come to \textbf{Moscow}\underline{,} St. \textbf{Petersburg} and other Russian cities.
Most of them are the citizens of Central Asia: \textbf{Uzbekistan}\underline{,} Ta\textbf{ji}\underline{k}\textbf{istan} and \textbf{Turkmenistan}\underline{.}
In the second \textbf{channel} there are illegal \textbf{weapons} \textbf{stolen} by criminals.
I even get to some \textbf{ring}\underline{s} about a \textbf{friend} I trust.
It is not yet clear whether the \textbf{spark} of these \textbf{protests} will \textbf{mobil}\underline{ize} entire masses.
However, we want to look \textbf{ahead} for 5\textbf{-10} years and \textbf{anticipate} the \textbf{radical} changes in this \textbf{interaction}\underline{.}
We must release the computer world into our \textbf{physical} world and make it more \textbf{tangible}\underline{.}
- We would ask you, for example, to give you this \textbf{bubble} can?
Not everyone understands how much this influences the \textbf{interaction} between man and machine.
I think that the \textbf{eight}\underline{h} \textbf{breakthrough} could well become the integration of \textbf{ta}\underline{c}\textbf{tile} \textbf{perception}\underline{.}
- This is a good idea, we have not \textbf{tried} it.
\textbf{Kir}\textbf{\underline{ill}} \textbf{Mill}\underline{er} is one of the \textbf{typical} \textbf{Petersburg} social-\textbf{phil}\textbf{\underline{oso}}\underline{ph}ical \textbf{artists} who create new \textbf{myth}\underline{s}.
- At an \textbf{exhibition} in the Newskiy \textbf{Cultural} \textbf{Palace} where my works were \textbf{exhibit}\underline{ed}.
I will have an \textbf{exhibition} with the \textbf{theme} "The Russian Museum as C\textbf{low}\underline{n}s".
- To him come \textbf{abandoned} women, where the \textbf{sexual}\underline{-}\textbf{social} \textbf{sphere} \textbf{plays} a role.
"In other words \textbf{Mars} and \textbf{Venus}\underline{",} \textbf{says} the scientific \textbf{assistant} of the \textbf{Astronom}\underline{ical} \textbf{Stern}\underline{berg} \textbf{Institute} \textbf{Vladimir} \textbf{Sur}\textbf{\underline{din}}\underline{.}
It was followed by the \textbf{breeding} of \textbf{insect}\underline{s}, more precisely of \textbf{tiny} \textbf{fruit} \textbf{fly}\underline{s} (\textbf{Dr}\textbf{\underline{oso}}\textbf{\underline{phil}}\underline{a}), in orbit.
There has been an \textbf{experiment} with \textbf{rats}\underline{,} which have already been \textbf{fer}\textbf{\underline{til}}\underline{ized} into space.
The \textbf{hydro}\textbf{\underline{labor}}\textbf{\underline{atory}} in the \textbf{preparation} center of the cosmon\textbf{aut}\underline{s} is a \textbf{mandatory} station during \textbf{flight} \textbf{preparation}\underline{.}
"\textbf{Th}\underline{at} is not enough time to \textbf{forget} something," \textbf{says} \textbf{baby} swimming \textbf{instructor} \textbf{Marina} \textbf{Ak}\underline{s}enowa.
He will simply \textbf{miss} what is essential for his life.
This is certainly not the case, but as I said, I do not like such \textbf{comparison}\underline{s}.
\textbf{Otherwise}\underline{,} they would have nothing to do with cooperation with our \textbf{authority}\underline{,} would they not?
As our \textbf{controls} are carried out after the event, there is a certain \textbf{delay} here.
It is also possible to use all the second and third class \textbf{roads}\underline{,} including mountain \textbf{roads}\underline{.}
\textbf{Snow} is mainly on the \textbf{streets} of the \textbf{Gian}\underline{t} \textbf{Mountains} and Or\textbf{lick} xe9 \textbf{hor}\underline{y}.
This is one of the \textbf{disaster} reports to which we human \textbf{beings} are so \textbf{keen} to \textbf{jump}\underline{.}
It is a national benefit event that we have been planning for two years.
The anthem is to be sung \textbf{simultaneously} by all the \textbf{perform}\underline{ers} on all three \textbf{concerts}\underline{.}
The anthems are also \textbf{broadcast} live on Czech \textbf{television} in a direct connection.
Was it your goal to bring it so far with The \textbf{Tap} \textbf{Tap}\underline{?}
In \textbf{1933}\underline{,} the \textbf{Polish} \textbf{infant}\underline{ry} began to deal with \textbf{rocket}\underline{-}\textbf{power}\underline{ed} \textbf{bullet}\underline{s}.
The \textbf{article} by \textbf{Prof}\underline{.} M. \textbf{Sub}\underline{ot}owicz contains the proposal to establish a space company.
Last week, the \textbf{Constitutional} Court \textbf{repeal}\underline{ed} the non-\textbf{profit} law.
\textbf{Due} to the big \textbf{differences} in the value of work (s\textbf{ans}\underline{)} there are price \textbf{tensions}\underline{.}
The result is growing poverty, as well as growing \textbf{differences} between rich and poor.
In every \textbf{era} we can make an \textbf{Alexander} the Great or a \textbf{Napoleon}\underline{.}
In its \textbf{conception}\underline{,} the new world order is a world of \textbf{master}\underline{s} and \textbf{slave}\underline{s}.
"\textbf{Mor}\underline{e} \textbf{incredible} in\textbf{vention}\underline{s} from the EU \textbf{workshop} can be \textbf{nominated} by the end of this year.
If everything worked in our country without any problems, I would not stand \textbf{anywhere}\underline{.}
We are already looking for park \textbf{bench}\underline{,} \textbf{dog} and \textbf{football}\underline{-}\textbf{play}\underline{ing} \textbf{boys} and \textbf{girls}\underline{.}
They provide an atmosphere, but above all for the right \textbf{hum}\underline{id}ity in the \textbf{literature} \textbf{mountains}\underline{.}
\textbf{Stephen} Szabo: Germany does not support what the \textbf{Israelis} did in \textbf{Gaza}\underline{.}
Is it difficult for Germany to take a clear position on important international issues?
\textbf{Firstly}\underline{,} Germany has large markets in the Middle East, especially in the \textbf{Gulf} States.
This is not easy for Germany, of course, because of its relationship with Israel.
German companies are also being \textbf{legally} \textbf{copied} in this way, for example the sports goods \textbf{manufacturer} \textbf{Pu}\underline{ma}.
In the big cities there are multi-\textbf{storey} \textbf{department} \textbf{stores} \textbf{selling} almost \textbf{exclusively} \textbf{counterfeit}\underline{s}.
The Chinese are therefore still allowed to use an \textbf{em}\textbf{\underline{ble}}\underline{m} similar to the \textbf{Mercedes}\underline{-}star.
\textbf{Almost} 5\textbf{7,000} such cases have been closed, \textbf{75\%} more than last year.
This also applies to the \textbf{inventory} of all valid \textbf{trademarks}\underline{,} a total of \textbf{5.5} million \textbf{pieces}\underline{.}
To combat this costs many times as the case of the German family company \textbf{Freud}\textbf{\underline{enberg}} shows.
It is true that the Germans were able to get \textbf{rid} of their illegal \textbf{manufacture} of imitated car parts.
But the imitator \textbf{continued} to secure Chinese rights to the \textbf{Freud}\textbf{\underline{enberg}} brand.
The Group has long since \textbf{abandoned} this business area, but it was able to avoid \textbf{registration}\underline{.}
It \textbf{guarantees} children school \textbf{fees}\underline{,} school \textbf{uniform}\underline{s} and a warm \textbf{meal} daily in the Gogo Center.
\textbf{Often}\underline{,} however, they do not cause any \textbf{pain} or other \textbf{symptom}\underline{s} and therefore remain unn\textbf{otic}\underline{ed}.
The \textbf{journey} also \textbf{leads} to Esitjeni, where the \textbf{singer}\underline{s} visit their children.
The U.S. \textbf{Space} \textbf{Agency} \textbf{NAS}\underline{A} has \textbf{demonstrated} the \textbf{existence} of \textbf{ice} on the \textbf{planet} \textbf{Mer}\textbf{\underline{kur}}\underline{.}
The picture comes from a camera developed by German \textbf{researchers} at the \textbf{Max} \textbf{Planck} \textbf{Institute}\underline{.}
\textbf{Like} a red age, the \textbf{Heli}\underline{x} ne\textbf{bul}\underline{a} \textbf{looks} towards the viewer on this \textbf{infrared} photo.
His \textbf{resembl}\underline{ance} to an \textbf{earth}\underline{ly} \textbf{continent} \textbf{gave} this \textbf{fo}\underline{g} the title of North America.
Here \textbf{stands} the \textbf{Very} \textbf{Large} \textbf{Tele}\textbf{\underline{scope}} - which \textbf{honour}\underline{s} its name.
With a total of four \textbf{mirror}\underline{s}, the \textbf{telescope} can also \textbf{illumin}\underline{ate} the medium \textbf{infrared} \textbf{spectrum}\underline{.}
For \textbf{decades}\underline{,} \textbf{radar} \textbf{measurements} have \textbf{indicated} that there is \textbf{ice} on \textbf{Mer}\textbf{\underline{kur}}\underline{.}
\textbf{Everything} is green and \textbf{ju}\underline{ic}y, you might think you are in the \textbf{Black} \textbf{Forest}\underline{.}
"\textbf{He} was \textbf{born} here in the region in 18\textbf{05}\underline{,} he died in \textbf{1973}\underline{,}" \textbf{explains} Fatu\textbf{lay}\textbf{\underline{eva}}\underline{.}
\textbf{Has}   u20\textbf{47} \textbf{ir}\textbf{\underline{ali}} M xf\textbf{cs}\underline{l} xfc\textbf{mov} \textbf{rec}\underline{kon}ed with a few \textbf{decades} at his age?
\textbf{Far}\underline{id} Mugimzadeh \textbf{explains} this with the special \textbf{gene}\underline{s} of the \textbf{Tal}\textbf{\underline{yan}}\underline{s}.
But everything was better than the "\textbf{lov}\underline{ed} \textbf{father}\underline{"} Hey\textbf{dar} \textbf{Ali}\underline{y}\textbf{ev} took over.
If that is not a reason to stay \textbf{alive} for as long as possible.
But what is an \textbf{insult} and how it should be \textbf{punished} remains \textbf{unclear}\underline{.}
I will \textbf{propose} a new security strategy that will enable us to achieve this objective.
But, at \textbf{worst}\underline{,} his government closed its \textbf{eyes} to the problem.
There were \textbf{signs} that it was \textbf{beat}\underline{en}, and the starvation of \textbf{corps}\underline{es} had already started.
In April \textbf{2011}\underline{,} Manning was \textbf{transferred} to the military \textbf{prison} of \textbf{Fort} Le\textbf{av}\underline{en}\textbf{worth}\underline{,} \textbf{Kan}\underline{s}as.
If he is found \textbf{guilty} in all \textbf{charges}\underline{,} he \textbf{faces} a life \textbf{sentence}\underline{.}
I was there for a few \textbf{seconds}\underline{,} \textbf{uncertain} to which I should go.
I \textbf{grew} up in Central \textbf{California} and was called "\textbf{Me}\textbf{\underline{xi}}\textbf{\underline{kan}}\underline{"} all my life.
We love the \textbf{Mexican} \textbf{band} \textbf{Los} \textbf{Ti}\textbf{\underline{gre}}\underline{s} del \textbf{Nor}\underline{te}, but also \textbf{Bru}\underline{ce} \textbf{Spring}\underline{ste}en.
Can there ever be \textbf{lasting} peace between \textbf{Arab}\underline{s} and \textbf{Jews} in the Middle East?
\textbf{Out}\textbf{\underline{standing}} \textbf{Arab} \textbf{nations} should also \textbf{persuade} \textbf{Hamas} and \textbf{Fatah} to agree.
In a \textbf{constantly} \textbf{elect}\underline{r}\textbf{ified} world it is nice to be \textbf{bo}\underline{red} at times.
But the \textbf{brain} does not always know what to do best.
And he \textbf{adds}\underline{:} 'S\textbf{elf}\underline{-}\textbf{control} \textbf{transfers} from one situation to another'.
In We\textbf{ld} \textbf{County} in \textbf{northern} \textbf{Color}\textbf{\underline{ados}}\underline{,} \textbf{District} Attor\textbf{ney} Ken B\textbf{uck} has a \textbf{stronger} view.
S\textbf{everal} cities in \textbf{Color}\underline{ado} are not even \textbf{waiting} for the \textbf{federal} authorities to act.
I \textbf{told} my \textbf{father} that I hated \textbf{Oxford} and why I did it.
They would never do that, not in my city of \textbf{dream}\underline{ing} \textbf{tower} \textbf{peak}\underline{s}.
\textbf{Valentin}\underline{o} has always \textbf{felt} \textbf{fascination} for the \textbf{stick}\underline{y} and \textbf{distant} world of the no\textbf{bil}\underline{ity}.
We were about 20 people, including \textbf{Sharon} \textbf{Stone} and John \textbf{Kennedy} Jr.
The life of \textbf{Gar}\textbf{\underline{ava}}\underline{ni} is not a \textbf{story} of ob\textbf{session}\underline{,} rather of \textbf{mutual} love.
Many of these customers say that the first \textbf{Valentin}\underline{o} is like the first love, "un\textbf{forge}\textbf{\underline{table}}\underline{".}
For years with the "sa\textbf{voir}\underline{-}  u20\textbf{47} \textbf{tre}\underline{"} of the \textbf{elite}\underline{,} \textbf{Valentin}\underline{o} is now her best \textbf{copy}\underline{.}
This is the price he has to pay to achieve his \textbf{dream}\underline{.}
\textbf{According} to its national population \textbf{authority}\underline{,} the \textbf{birth} rate is currently \textbf{1.2} children per \textbf{woman}\underline{.}
The government is trying to ensure that not so many small \textbf{houses} are built.
These apartments have a living area of \textbf{46} \textbf{square} metres and show great sales success.
As a result, they are much better for our \textbf{cash} \textbf{flow}\underline{.}
When asked, he \textbf{answered} that he would never accept an \textbf{invitation} from an \textbf{unknown} person.
Jos xe9 contacted \textbf{Ask} after reading a \textbf{recommendation} in \textbf{Twitter}\underline{.}
Then he \textbf{explains} a number of steps to securely \textbf{configure} a user account.
And one more question: must everyone know what you are doing at any moment?
And 'if \textbf{Britain} gives this \textbf{carte} \textbf{blanc}\underline{he} tomorrow, I think it will be done'.
It is a problem between a South American and a Central American state.
9\textbf{2\%} of cases of contagion \textbf{occur} through \textbf{sexual} inter\textbf{course}\underline{,} \textbf{6\%} through \textbf{blood} and \textbf{2\%} perinatal.
In fact, Vitro is not the first case where this \textbf{scheme} has been allowed.
From then on, "Cuco" Ortiz, who was a very good \textbf{manager}\underline{,}" \textbf{says} \textbf{Rey}\underline{es}.
"I know what should be on the \textbf{grave}\textbf{\underline{stone}} of J.R.," \textbf{Hag}\underline{man} said in \textbf{1988}\underline{.}
S\textbf{everal} have said that they want to go to \textbf{celebration}\underline{s} about "the end of the world".
In this sense, these measures \textbf{partly} \textbf{undermine} the US democratic system.
In this sense, these measures \textbf{partly} \textbf{undermine} the US democratic system.
What can all these research be '\textbf{good}\underline{'}, Mrs \textbf{Pla}\textbf{\underline{mond}}\underline{on} asks?
A few hours later the team found a \textbf{cure} for this \textbf{evil}\underline{.}
\textbf{Pal}\underline{li}ative care is used when there are no other options.
This morning his \textbf{son} will \textbf{drink} the beer at the foot of the de\textbf{cea}\underline{s}ed.
\textbf{Chan}\underline{tal} \textbf{Rou}\underline{le}au was one of the first Members of \textbf{Montreal} to sound the \textbf{alarm}\underline{.}
This summer's newcomers are used to \textbf{playing} high-\textbf{level} games.
In Li\textbf{gue} 1 \textbf{Lyon} took us the place of \textbf{leader}\underline{.}
However, against very good European \textbf{teams} we will have our say.
\textbf{Within} the team we respect both the player and the person.
\textbf{Nothing} particularly \textbf{impressive} \textbf{compared} to world trade in real \textbf{currencies} or financial products.
The \textbf{decisive} step is to enter this new \textbf{transaction} into this book.
Moreover, the \textbf{owner} manages his \textbf{identity} and can therefore remain \textbf{anonymous}\underline{.}
In cities, state \textbf{schools} are full of \textbf{girls} and \textbf{boys}\underline{.}
\textbf{Will} the authorities under whose \textbf{authority} it will be under its command be considered \textbf{legitimate}\underline{?}
A\textbf{IF} gives you the five main reasons for \textbf{visiting} Israel.
It is said that all who bathe in this \textbf{river} receive God u2019s \textbf{blessing}\underline{.}
But at least the five most interesting of them should be \textbf{visited}\underline{.}
The Museum of Art in \textbf{Tel} A\textbf{viv} is also well \textbf{worth} a visit.
In each of the three places there are swimming \textbf{pools}\underline{,} water \textbf{parks}\underline{,} \textbf{dolphin}\underline{s} and \textbf{ocean}\textbf{\underline{aries}}\underline{.}
\textbf{Tourist}\underline{s} like to \textbf{stroll} through the \textbf{narrow} alle\textbf{ys} \textbf{named} after the sign.
"The big and powerful" \textbf{leads} to \textbf{Moscow}\underline{:} \textbf{migrants} save money for language.
\textbf{Except}\textbf{\underline{ions}} apply only to citizens of countries where Russian is an official language.
Only \textbf{organised} \textbf{recruitment} will \textbf{resolve} \textbf{90\%} of the problems of foreign workers.
As a \textbf{teenage}\underline{r}, these children immediately take the first opportunity to make money.
\textbf{Meanwhile}\underline{,} most of the guest workers remain \textbf{illegally} in Russia.
\textbf{Fal}\underline{s}\textbf{ified} \textbf{registration} can be made quickly and only for one and a half \textbf{thousand}\underline{.}
\textbf{Meanwhile}\underline{,} the \textbf{Ministry} of the \textbf{Interior} \textbf{stresses} that the \textbf{proliferation} of illegal \textbf{weapons} is under control.
One in four American \textbf{youth}\underline{s} will be behind \textbf{Mc} \textbf{Donald}\underline{'}s co\textbf{ffer}\underline{s} sometime.
That is why many of the low paid \textbf{Wal}\underline{mar}t workers only buy in their own \textbf{workplace}\underline{.}
The \textbf{latter} also \textbf{complain} about difficult working conditions, such as a lack of fork\textbf{lift} \textbf{truck}\underline{s} or hand \textbf{scanner}\underline{s}.
In total, the \textbf{Wal}\underline{mar}t \textbf{Cast}\underline{s} carried out almost 100 million \textbf{transactions} on \textbf{Black} \textbf{Friday}\underline{.}
\textbf{Hard}\underline{ly} one \textbf{saw} it as the main source of income or \textbf{planned} to stay there for longer.
Then we could add \textbf{virtual} \textbf{objects} to the real world much more easily.
But overall, the future \textbf{belongs} to \textbf{mixed} control types, such as \textbf{gesture} and language.
Of course, 8 \textbf{Megapixel}\underline{s} with a speed of \textbf{1000} fps would not be bad.
The speed and the number of images per second are also important.
In this world, Red is the compromise between \textbf{artists}\underline{,} image \textbf{consultants} and society.
But I want to talk to people through my \textbf{provocation}\underline{s}.
I am a hero of the last century when culture \textbf{meant} something.
I started with images that usually only come at the end of the \textbf{career}\underline{.}
In Europe there are many \textbf{curious} people who visit \textbf{exhibitions} or \textbf{concerts}\underline{.}
Art must be modern again, as it was at the beginning of the last century.
The last \textbf{breeding} cage with animals \textbf{fle}\underline{w} into orbit 16 years ago.
The problem of \textbf{reproduction} directly in space has not been \textbf{solved}\underline{.}
"But what \textbf{happens}\underline{?}" is \textbf{Wal}\underline{er}i \textbf{Pol}\underline{ja}\textbf{kov}\underline{'}s not \textbf{insignificant} question.
You talk about the problems with the practical implementation of the Czech \textbf{procurement} law.
However, the \textbf{roads} are \textbf{mostly} easy to drive, and sometimes there is a need for greater \textbf{caution}\underline{.}
In the other areas of the \textbf{district}\underline{,} the \textbf{tram}\underline{s} are usually fully \textbf{accessible}\underline{.}
It is not as bad as it \textbf{appears} at first \textbf{sight}\underline{.}
And in what way must we \textbf{catch} up with the more developed countries?
The \textbf{venue}\underline{s} are: Incheba-\textbf{Ar}\textbf{\underline{ena}}\underline{/}P\textbf{rag}\underline{,} \textbf{Fl} xe9da/Brno and Plynojem/O\textbf{stra}\underline{va}; 12 Czech \textbf{bands} and other \textbf{musicians}\underline{.}
The \textbf{author} of the draft and the details of this project were \textbf{unfortunately} \textbf{unknown}\underline{.}
However, research was then \textbf{interrupt}\underline{ed} by the \textbf{invasion} of the German Wehr\textbf{macht}\underline{.}
He held this position until his death in \textbf{1959}\underline{.}
For \textbf{bri}\textbf{\underline{bes}}\underline{,} by \textbf{unlawful}\underline{ly} \textbf{covering} up \textbf{advantages} or with \textbf{stone} and \textbf{sword}\underline{.}
Here is \textbf{wisdom}\underline{,} and \textbf{anyone} who has reason to think about the number of animals.
\textbf{Ben} Af\textbf{fleck} has made a \textbf{remarkable} start to his \textbf{career} with this film.
\textbf{Guidelines} for \textbf{balloon}\underline{ing}, \textbf{banana}\underline{s} and \textbf{circus}\underline{es}
The actual vote will then take place by the end of February \textbf{2013}\underline{,}" he stated.
Do you see yourself as a human in \textbf{politics} more right or left?
From a Czech point of view, it seems to me that people are looking to the left.
I have \textbf{spoken} to Radim \textbf{Jan}  u20\textbf{47} \textbf{ura}\underline{,} for example, but he \textbf{refused} because of work \textbf{congestion}\underline{.}
And I am not \textbf{obliged} to deny the \textbf{campaign} by my own means.
If I just wanted to make money, I would stand for nothing.
So do you continue to work as an \textbf{entrepreneur} to make a living?
\textbf{Sp}\textbf{\underline{ijk}}\underline{en}\textbf{isse}\underline{,} a \textbf{sleep}\underline{y} town just outside \textbf{Rotterdam}\underline{,} is a \textbf{strange} record \textbf{holder}\underline{.}
The project is also \textbf{nominated} for the \textbf{Dutch} National \textbf{Wood} \textbf{Award} \textbf{2012}\underline{.}
Even hard-\textbf{working} \textbf{architect}\underline{s} and construction \textbf{engineers} \textbf{shake} their \textbf{heads} over the \textbf{unknown} building material.
In this way, \textbf{MV}\underline{R}DV has achieved the \textbf{royal} \textbf{discipline} called the \textbf{Ident}\underline{ity} \textbf{Foundation} in the jar\textbf{gon}\underline{.}
Now, however, Germany must be \textbf{careful} because of its special relationship with Israel.
At the same time, however, I believe that it does not support the American position either.
To make matters \textbf{worse}\underline{,} Europeans do not have a \textbf{coherent} and \textbf{coherent} policy.
But it certainly \textbf{plays} an important role in German \textbf{considerations}\underline{.}
In this respect, Germany is in a much more difficult position than the US.
However, it is protected for as long as the actual \textbf{names} do not \textbf{complain}\underline{.}
This way G\textbf{ucci} is simply Lu-G\textbf{ucci}\underline{,} instead of \textbf{Pra}\underline{da} you can \textbf{insert} \textbf{Pra}\underline{da}-Kny.
The procedure can last up to \textbf{nine} years, with \textbf{uncertain} \textbf{outcome}\underline{s}.
For more than \textbf{seven} years, the Group has been \textbf{fighting} a Chinese \textbf{pla}\textbf{\underline{gia}}\underline{r}ator.
For 15 or 20 \textbf{euros} a month you can take over a \textbf{sponsor}\underline{ship}.
\textbf{Without} a school \textbf{leaving} \textbf{certificate}\underline{,} a poor country has no chance.
Con\textbf{dom}\underline{s} can reduce the risk of contagion but do not provide \textbf{100\%} protection.
The \textbf{temperature} on the \textbf{Mer}\textbf{\underline{kur}} can reach up to 4\textbf{26} \textbf{degrees} \textbf{Celsius}\underline{.}
This da\textbf{zz}\underline{ling} \textbf{glu}\underline{t} of a \textbf{dying} star has taken up the \textbf{spe}\underline{ar} \textbf{telescope} of Nasa.
The \textbf{Don}\underline{ut}-\textbf{shaped} \textbf{ring} \textbf{consists} of material that the star \textbf{extract}\underline{ed} in the \textbf{dying} process.
A combination of normal and in\textbf{fra}\underline{-}red photo provides a \textbf{spectacular} \textbf{color}\underline{ing}.
In this ne\textbf{bul}\underline{a} you will find the \textbf{bright}\underline{est} group of young \textbf{stars} of our \textbf{Mil}\textbf{\underline{ky}} \textbf{Way}\underline{.}
\textbf{View} of the \textbf{Observatory} of the European \textbf{Observatory} (ESO) in the \textbf{Chile}\underline{an} Andes.
The European \textbf{Extreme}\underline{ly} \textbf{Large} \textbf{Tele}\textbf{\underline{scope}} is also \textbf{planned} at the \textbf{Chile}\underline{an} E\textbf{SO} ob\textbf{serv}\textbf{\underline{atory}}\underline{.}
They offer two \textbf{mirror}\underline{s} with an \textbf{average} of ten metres.
Since April 24, 1990 it has already \textbf{delivered} images of \textbf{distant} worlds.
\textbf{Sc}\textbf{\underline{ient}}\underline{ists} \textbf{assume} that \textbf{ice} also \textbf{exists} at the \textbf{southern} \textbf{pole} of \textbf{Mer}\textbf{\underline{kur}}\underline{.}
A \textbf{trace} search in the country where \textbf{97}\underline{-}\textbf{year}\underline{-}\textbf{old}\underline{s} are still relatively young.
A \textbf{trace} search in the country where \textbf{97}\underline{-}\textbf{year}\underline{-}\textbf{old}\underline{s} are still relatively young.
With her \textbf{97} years she is still relatively young for these la\textbf{titude}\underline{s}.
All of them, so far hope\textbf{lessly} \textbf{divided} into a \textbf{confused} \textbf{opposition}\underline{,} are \textbf{afraid}\underline{.}
After the \textbf{dictator} u2019s fall, up to 11,\textbf{000} \textbf{civilians} were in military \textbf{detention}\underline{.}
Moreover, no \textbf{article} \textbf{explicitly} \textbf{stipulat}\underline{es} \textbf{equality} between men and women.
It is also \textbf{dubious} to say that 'inf\textbf{uri}\underline{ation} of people' is \textbf{prohibited}\underline{.}
\textbf{Mor}\underline{si} u2019s \textbf{expansion} of power to all three powers in the state led the \textbf{lawyer} to \textbf{resign}\underline{.}
It is one of the more \textbf{expensive} \textbf{dishes} you can buy here.
But this is exactly what the family \textbf{says} it has been \textbf{denied} up to now.
The authorities have \textbf{treated} me as if I were a \textbf{mother}\underline{-}in-\textbf{law}\underline{,} a \textbf{trouble}\textbf{\underline{maker}}\underline{,} a \textbf{nu}\underline{is}ance.
They want their \textbf{judgment} simply to be accepted and \textbf{kept} quiet.
The Public \textbf{Prosecutor}\underline{'}s Office \textbf{contradict}\underline{s} \textbf{Brad}\underline{ley} Manning's \textbf{accus}\underline{ations} that he had been \textbf{mis}\underline{tre}ated in \textbf{prison}\underline{.}
The \textbf{hearing} \textbf{deals} with Manning u2019s time in the military \textbf{prison} in \textbf{Qua}\underline{n}\textbf{tico}\underline{,} \textbf{Virgin}\underline{ia}.
The \textbf{defense} \textbf{seeks} to \textbf{reject} the in\textbf{dic}\underline{t}ment for overly \textbf{harsh} \textbf{prison} conditions.
The \textbf{lib}\underline{er}ated US \textbf{army} is \textbf{accused} of ab\textbf{using} thousands of \textbf{confidential} documents.
In January \textbf{2011}\underline{,} Manning u2019s \textbf{attorney} \textbf{formally} \textbf{appeal}\underline{ed} against the treatment of mening.
\textbf{Nav}\textbf{\underline{arre}}\textbf{\underline{tte}} \textbf{believes} that \textbf{Mexican} \textbf{Americans} are tra\textbf{pped} between two worlds.
If our families had not \textbf{failed} in \textbf{Mexico}\underline{,} they would not have \textbf{gone}\underline{.}
While she is an American \textbf{citizen}\underline{,} she sees \textbf{herself} as part of two countries.
You enjoy the best of both worlds, but \textbf{none} of them is \textbf{root}\underline{ed} in.
The latest \textbf{blood}\underline{y} events \textbf{seem} to \textbf{ni}\underline{p} such hope in the \textbf{bud}\underline{.}
Why \textbf{hide} these in\textbf{sid}\textbf{\underline{ious}} \textbf{Palestinians} and leave them with their own state?
Israel u2019s \textbf{defense} budget is greater than that of its four \textbf{Arab} \textbf{neighbor}\underline{s} \textbf{combined}\underline{.}
\textbf{Obama} must also play his part in \textbf{encouraging} Israel to \textbf{negotiate}\underline{.}
The United States has a vital interest in a \textbf{stable} Middle East.
But more and more \textbf{academic}\underline{s} and children's development \textbf{experts} are leading to \textbf{bo}\underline{re}\textbf{dom} as something positive.
Then there is the question of how we actually \textbf{define} \textbf{bo}\underline{re}\textbf{dom}\underline{.}
"\textbf{We} do not have a real \textbf{precedent} to follow," he \textbf{adds}\underline{.}
In my first weeks in \textbf{Oxford} I \textbf{belong}\underline{ed} to such a \textbf{minority}\underline{.}
\textbf{Should} I have to turn to the \textbf{Labour} Party and \textbf{suppress} my natural \textbf{prop}\underline{en}sities?
"But it is the best place in the world," he said.
Exhausted by my \textbf{frequent} travels to London, my \textbf{emotional} \textbf{resistance} became \textbf{weak}\underline{er}.
At that time he \textbf{wrote} two \textbf{column}\underline{s} per week in the \textbf{Mur}\underline{d}\textbf{och} press.
The \textbf{Argent}\underline{ine} model Val\textbf{eria} Ma\textbf{zza} does not \textbf{forget} the \textbf{charm} of the \textbf{fashion}\textbf{\underline{maker}}\underline{.}
"\textbf{It} was a true \textbf{dream}\underline{,}" \textbf{says} \textbf{Rod}\textbf{\underline{rig}}\underline{o} d'\textbf{Ar}\textbf{\underline{enberg}}\underline{'}s \textbf{wi}\textbf{\underline{dow}}\underline{.}
How is this \textbf{definition} applied to its \textbf{everyday} life and social networks?
This includes the \textbf{mother} who has the \textbf{password} to one of the \textbf{accounts}\underline{.}
The \textbf{boy} is not \textbf{unaware} of what is now known as \textbf{cyber}\textbf{\underline{bul}}\underline{ly}ing.
"\textbf{To} say they should not do it does not work," he \textbf{says}\underline{.}
" For example, the age or what one may share or \textbf{publish}\underline{"} he \textbf{explains}\underline{.}
The cause of \textbf{AIDS} \textbf{deaths} today is too late \textbf{detection}\underline{.}
\textbf{Fabr}\underline{i}\textbf{zio} was 21 years old when he was \textbf{confirmed} that he was \textbf{HIV} positive.
- In my opinion, the problem is not access to treatment.
His \textbf{news} is a \textbf{summary} of the fight against \textbf{AIDS} in \textbf{2012}\underline{.}
No one in \textbf{Puerto} \textbf{Rico} has \textbf{dominated} this area as much as \textbf{Pic}\underline{ul} xedn.
What do you think is the best you have achieved in the \textbf{Association}\underline{?}
There he met young \textbf{designer} \textbf{Maj} \textbf{Axel}\textbf{\underline{sson}} and \textbf{married} her.
\textbf{Indian}\underline{a} was the first state to make such a demand.
The \textbf{Republican} authorities \textbf{rush}\underline{ed} to \textbf{extend} this practice to other states.
These measures are clearly aimed at \textbf{limiting} his\textbf{pan}\underline{ic} \textbf{voices}\underline{.}
The US Ad\textbf{voca}\underline{te} General \textbf{intervene}\underline{d} to \textbf{suspend} the most \textbf{controversial} laws.
The \textbf{organisation} also recommends \textbf{limiting} the \textbf{consumption} of red \textbf{meat}\underline{.}
\textbf{According} to the \textbf{Canadian} \textbf{cancer} society, \textbf{studies} on \textbf{vitamin} E are \textbf{contradictory}\underline{.}
\textbf{Based} on this, \textbf{phy}\underline{s}icists \textbf{divide} the p\textbf{article}\underline{s} into two \textbf{categories}\underline{.}
\textbf{Return}\underline{ing} to \textbf{childhood} is an \textbf{unacceptable} \textbf{hum}\textbf{\underline{ili}}\underline{ation} for some people.
But I really got to know my children through the \textbf{disease}\underline{.}
In \textbf{Quebec} there is a bed for \textbf{pal}\underline{li}ative care for 11,\textbf{700} \textbf{inhabitants}\underline{.}
The implementation of this report was possible thanks to a \textbf{journal}\underline{ism} \textbf{grant} from \textbf{Canadian} health research \textbf{institute}\underline{s}.
This season you have taken on a new \textbf{dimension} with \textbf{PS}\underline{G}.
These elements encourage me every day to improve my level of play.
You will take advantage of the competition introduced by \textbf{Carlo} An\textbf{cel}\textbf{\underline{otti}}\underline{...}
Moreover, \textbf{Carlo} An\textbf{cel}\textbf{\underline{otti}} gives me a lot about my \textbf{playing} position.
What do you think about the first part of the \textbf{PS}\underline{G} season?
Can \textbf{PS}\underline{G} become a large European \textbf{club} in the short term?
This year it is really important for us to have this title.
How did you experience the European \textbf{Championship} in \textbf{2012} with the French national team?
I \textbf{saw} things there from which I \textbf{emerged} \textbf{stronger}\underline{.}
Today I am able to make good \textbf{matches} in the national team.
We have a good position in the \textbf{qualify}\underline{ing} group for the World \textbf{Cup}\underline{.}
I hope that \textbf{Did}\underline{ier} Deschamps will lead the 'Bleus' to \textbf{Brazil}\underline{.}
With 1\textbf{5,000} \textbf{computers} on the network, some 20\textbf{0,000} \textbf{transactions} have already been \textbf{recorded}\underline{.}
In this way, the network can \textbf{verify} the \textbf{authentic}\underline{ity} of the \textbf{transaction}\underline{.}
French \textbf{troops} have left their \textbf{responsibilities} in Afghanistan (Kap\textbf{isa} and \textbf{Sur}\underline{o}bi).
\textbf{Everything} is \textbf{imported}\underline{;} nothing is produced \textbf{apart} from \textbf{fruit} and \textbf{vegetables}\underline{.}
What \textbf{souvenir} are we \textbf{leaving} after military \textbf{expenditure} of EUR 2 billion?
This is a new \textbf{poker} game by President \textbf{Mohammed} \textbf{Mor}\underline{si}.
\textbf{Representative}\underline{s} of human rights organisations, \textbf{religious} \textbf{minorities} or civil society have \textbf{acted} \textbf{equally}\underline{.}
It is not \textbf{surprising} that most of the \textbf{articles} were adopted \textbf{unanimously}\underline{.}
\textbf{According} to them, the \textbf{Islamic}\underline{isation} of the \textbf{Constitution} takes place through other \textbf{articles}\underline{.}
\textbf{According} to an old \textbf{legend}\underline{,} \textbf{pag}\underline{an} \textbf{god}\underline{s} were living on the summit.
In the evening you can even see them \textbf{sleeping} on the \textbf{roof}\underline{s} of parking \textbf{cars}\underline{.}
The \textbf{cat}\underline{s} like \textbf{lively} places and do not say no to \textbf{delicacies}\underline{.}
There are problems with \textbf{migrants} without jobs, education, language \textbf{skills} and medical assessment.
The Russian \textbf{Ministry} of the \textbf{Interior} is planning to \textbf{tight}\underline{en} up the \textbf{arms} law for private \textbf{arms} \textbf{owners}\underline{.}
\textbf{Especially} many pistols and \textbf{ri}\textbf{\underline{fle}}\underline{s} come from poor countries such as \textbf{Ky}\underline{r}\textbf{gy}\underline{z}\textbf{stan}\underline{.}
There is no need for any \textbf{papers} or personal \textbf{meetings}\underline{.}
The \textbf{weapon} is \textbf{distributed} in military \textbf{weapons} \textbf{camps} by \textbf{middle}\underline{-}\textbf{class} wardens.
The \textbf{protests} are supported by trade \textbf{unions} and several left-\textbf{wing} \textbf{char}\underline{ities}.
That is about 1.\textbf{1\%} more than they are now donating to pay.
- Not \textbf{necessarily}\underline{,} but this is about \textbf{mutual} \textbf{convergence}\underline{.}
The new hero of \textbf{Ros}\textbf{\underline{bal}}\underline{t} is the extra\textbf{vag}\underline{ant} \textbf{artist} \textbf{Kir}\textbf{\underline{ill}} \textbf{Mill}\underline{er}.
When the group began to play live, it became out of its "Leningrad".
There are now \textbf{micro}\underline{com}\textbf{muni}\textbf{\underline{ties}} and it is difficult to please everyone.
- To the \textbf{performances} of \textbf{Sta}\underline{s} \textbf{Mich}\underline{ai}\textbf{low} come several \textbf{thousand}\underline{!}
However, the \textbf{bio}\textbf{\underline{satellit}}\underline{e} "Bion" will only \textbf{contain} the same-sex \textbf{species}\underline{.}
\textbf{Will} it be able to bring a child into the world after this \textbf{flight}\underline{?}
The \textbf{BR}\underline{H} can only control \textbf{federal} funds, which \textbf{correspond}\underline{s} to our state funds.
But does it make sense to make the law even \textbf{stricter}\underline{?}
Such a system only places \textbf{bureaucracy} under even greater pressure.
On the \textbf{streets} there are some \textbf{smooth} \textbf{ice}\underline{,} but \textbf{mostly} they are \textbf{dry}\underline{.}
However, there are about 30 \textbf{cm} of \textbf{snow} on the \textbf{cre}\underline{st}s of the Ore \textbf{Mountains}\underline{.}
What is the purpose of the \textbf{proceed}\underline{s} of the \textbf{concerts} against the end of the world?
We wanted to set up a programme that would address all \textbf{generations}\underline{,} including children.
Even in \textbf{Moscow}\underline{,} where we were recently, there were no problems.
How many of them have been there since the beginning, that is, since 1998?
The \textbf{missile} was \textbf{1.4} m long and \textbf{weigh}\underline{ed} about \textbf{11.}\underline{5} \textbf{kg}\underline{.}
Of course, this \textbf{raises} the question of where this capital comes from.
For it is a man number and his number is six \textbf{hundred} sixty-six.'
Im\textbf{media}\underline{te}ly before the \textbf{occupation} of the \textbf{embassy}\underline{,} six \textbf{embassy} staff were able to \textbf{escape}\underline{.}
It \textbf{ended} after many \textbf{complications} in the \textbf{residence} of the \textbf{Canadian} \textbf{ambassador}\underline{.}
For this I need as much influence as possible and as strong a \textbf{mandate} as possible.
But do you not \textbf{confirm} this by what you have just said?
The people concerned would have to say, if necessary, why they \textbf{refuse} to do so.
People want to see me as a \textbf{Sam}\underline{ari}tan who is \textbf{saving} the Republic.
But I \textbf{wonder} what we still need a \textbf{library} for today.
No one is still going to go to one of these old style \textbf{libraries}\underline{,} is it?
\textbf{Nine} years later, the 30 million euro mountain has been \textbf{thrown} up.
"\textbf{No}\underline{th}ing is \textbf{worse} than a half-\textbf{empt}\underline{y} \textbf{library}\underline{,}" \textbf{says} \textbf{architect} \textbf{Win}\underline{y} Maas.
I believe that this is what makes it so difficult for the Germans.
'The brand will be watered down, the \textbf{attitude} will \textbf{disappear}\underline{,} the image damage will be \textbf{enormous}\underline{'}.
However, \textbf{81}\underline{,}\textbf{500} \textbf{appeal}\underline{s} are still \textbf{pending} in office.
CTMO \textbf{rejected} the \textbf{opposition} from \textbf{Munich}\underline{.}
"\textbf{There} you can see how much this is \textbf{worth} to us," \textbf{says} Wen\textbf{tz}\underline{ler}.
The history of a link that crosses well over \textbf{87}\textbf{\underline{33}} \textbf{kilometres}\underline{.}
The \textbf{Ban}\underline{tu} language \textbf{flu}\underline{ent}ly speaks in this room no one can, but \textbf{sing}\underline{.}
\textbf{Common} vi\textbf{ral} S\textbf{TI}\underline{s} are \textbf{HIV}\underline{,} human \textbf{pap}\textbf{\underline{pil}}\textbf{\underline{oma}} \textbf{viruses}\underline{,} herpes \textbf{genital}\underline{is} or he\textbf{pat}\textbf{\underline{itis}}\underline{.}
\textbf{Ch}\textbf{\underline{lam}}\underline{y}\textbf{dia} \textbf{infection}\underline{s} are much more common among young people than in other population groups.
This is why \textbf{experts} recommend regular \textbf{examination}\underline{s}, especially for often \textbf{changing} \textbf{sex} partners.
Most S\textbf{TI}\underline{s} can be healed early and can be \textbf{avoided} late.
But also the many \textbf{migrant} workers who carry the \textbf{virus} through the country.
"\textbf{Go}\underline{ing} to Esitjeni, there is light" say the people there.
The \textbf{mirror}\underline{,} here in the picture, had an \textbf{average} of five \textbf{meters}\underline{.}
However, the Hu\textbf{bble} space \textbf{telescope} provides the most important \textbf{impression}\underline{s} from space.
There are currently 20 people over 100 years old.
Then she \textbf{tells} about her \textbf{husband} who was in the \textbf{army}\underline{.}
It was \textbf{worst} in the period after the \textbf{Second} World War.
They live in the \textbf{middle} of the big family, are \textbf{loved}\underline{,} cared for and are happy.
The future \textbf{constitution} with \textbf{Sha}\textbf{\underline{ria}} law as its basis is highly \textbf{controversial}\underline{.}
F\textbf{ear} of a state of God on the \textbf{Nil}\underline{e} of \textbf{grace}\underline{s} of the powerful \textbf{Muslim} \textbf{Brot}\underline{her}\textbf{hood}\underline{.}
The \textbf{opposition} has been \textbf{forming} for weeks against the \textbf{sup}\textbf{\underline{rem}}\textbf{\underline{acy}} of the \textbf{Islamist}\underline{s}.
"\textbf{Man}\underline{y} people like \textbf{Aqua}\textbf{\underline{vit}} more than Rakfisk," \textbf{says} Ha\textbf{var}\underline{d}.
\textbf{Instead}\underline{,} we only refer to the '\textbf{oc}\textbf{\underline{cur}}\underline{r}ence of 22 July'.
Her English is just like most people here \textbf{spot}\underline{less}.
But perhaps it is the \textbf{strict} \textbf{dark}\underline{ness} of all the fish.
And the problems in the community are of a crucial \textbf{urban} nature.
But her family \textbf{believes} that she was \textbf{murdered} by her \textbf{companion}\underline{.}
The Public \textbf{Prosecutor} \textbf{claims} that \textbf{Brad}\underline{ley} Manning has not \textbf{complain}\underline{ed} about \textbf{mis}\underline{tre}atment.
Many people are \textbf{forced} to leave \textbf{Mexico} because of a lack of opportunities.
\textbf{Mexico} u2019s relationship with the United States is complex and full of \textbf{res}\underline{ent}ment.
We are the \textbf{descendants} of these people, and our \textbf{faithful}\underline{ness} is with them.
During his first term, he \textbf{failed} to present his own peace plan.
In a\textbf{path}\underline{y}, however, there is no \textbf{urge} to do something.
But only \textbf{3\%} of \textbf{parents} said they \textbf{felt} \textbf{bo}\underline{red}.
There is no clear \textbf{guideline} for the new \textbf{mar}\underline{i}juana law in \textbf{Color}\underline{ado}.
\textbf{Regulator}\underline{s} in the state of \textbf{Washington} are also \textbf{sh}\textbf{\underline{atter}}\underline{ing} their \textbf{heads}\underline{.}
\textbf{Petro}\underline{n}\textbf{ella} Wy\textbf{att}\underline{:} I was \textbf{promoted} from \textbf{Oxford} because I am Tory.
During his time in the for\textbf{ties}\underline{,} all political views were accepted.
Even my \textbf{communist} friends have always been f\textbf{law}\underline{less}.
"I love this \textbf{palace}\underline{,}" he \textbf{says} with his \textbf{distinctive} Italian \textbf{accent}\underline{.}
\textbf{Being} in love with the no\textbf{bil}\underline{ity} does not have to be \textbf{disadvantage}\underline{ous}.
The most difficult \textbf{profession} in the world: the human work animals of Kawah Ijen
\textbf{Those} who do not take this issue lightly are the Government of \textbf{Singapore}\underline{.}
On FB I \textbf{upload} nice \textbf{pictures} or \textbf{pictures} of games.
Even if \textbf{someone} \textbf{suggested} a \textbf{strange}\underline{r}, they would \textbf{ignore} it.
Con\textbf{cl}\underline{ud}ing the Unasur \textbf{Summit} without \textbf{publishing} the \textbf{Lima} \textbf{Declaration}
The final document also referred to the political situation in \textbf{Paraguay}\underline{.}
"\textbf{South} America must learn how to \textbf{integrate} its citizens," \textbf{says} \textbf{Raf}\underline{a}el Cor\textbf{rea}\underline{.}
"\textbf{Th}\underline{at} would \textbf{affect} everyone's health," he added.
Today it is possible to \textbf{survive} this \textbf{syndrome} with quality of life.
As you know, \textbf{Az}\underline{c} xe1rr\textbf{aga} Andrade is the main \textbf{shareholder} of the hotel \textbf{chain} Posadas.
I like the work of Leo Ar\textbf{ill}\underline{.}
\textbf{Student}\underline{s}, for their part, \textbf{assure} that the course is one of the most interesting.
Ariz\textbf{ona} was the first state to introduce such a \textbf{requirement}\underline{.}
S\textbf{everal} legislative proposals have been \textbf{blocked} by the \textbf{veto}\underline{es} of democratic \textbf{governor}\underline{s}.
There are \textbf{cancer}\underline{s} that are \textbf{aggressive} and others that are in\textbf{dol}\underline{ent}.
\textbf{Smoking} is responsible for 8\textbf{5\%} of cases of \textbf{lung} \textbf{cancer}\underline{.}
However, C\textbf{ERN} has not yet found such \textbf{deviation}\underline{s}.
\textbf{Pal}\underline{li}ative care - the best way to die... | Le De\textbf{voir}
However, much remains to be done in this important area.
"\textbf{We} help families and \textbf{patients} \textbf{alike}\underline{,}" reports nursing \textbf{director} Na\textbf{thal}\underline{ie} \textbf{Sav}\underline{ard}.
However, she had \textbf{told} me that I was at the end!
I think he will \textbf{win} more titles in Paris.
I had an \textbf{encouraging} \textbf{conversation} with him in January.
We have \textbf{finished} the season with a very strong performance.
Do you think that the media expect too much from \textbf{PS}\underline{G}?
This means that I\textbf{bra}\underline{hi}m\textbf{ovic} is powerful and \textbf{score}\underline{s} many \textbf{goals}\underline{.}
\textbf{Unfortunately}\underline{,} my \textbf{injury} \textbf{prevented} me from \textbf{playing} some time.
This has been my hope since my \textbf{baptism} with the "Bleus".
A few \textbf{thousand} \textbf{websites} accept \textbf{Bit}\underline{co}in as a \textbf{donation} or as a means of payment.
The social network \textbf{Facebook} has also developed such a system.
The computer that has done the job \textbf{gets} 50 bit\textbf{ches}\underline{.}
The life of the network has already had ups and downs.
\textbf{Young} people are \textbf{fed} up with war and its ide\textbf{ologie}\underline{s}.
The \textbf{withdrawal} of French combat \textbf{troops} was \textbf{completed} on 20 November.
'\textbf{Ho}\underline{pe}' responds to \textbf{liberal}\underline{s} who see this as a \textbf{propaganda} \textbf{strike}\underline{.}
With this \textbf{Constitution}\underline{,} we remain within the civil state.
\textbf{Visit} the \textbf{river} \textbf{Jordan} where \textbf{Jesus} was \textbf{ba}\textbf{\underline{pt}}\underline{ized}.
There is a \textbf{shuttle} bus from the foot of the mountain.
Not all of them can be \textbf{visited} in just one trip.
In the \textbf{carefully} \textbf{restored} \textbf{theatre}\underline{,} evening \textbf{concerts} and \textbf{opera}\underline{s} are \textbf{performed} today.
\textbf{According} to \textbf{Jewish} \textbf{tradition}\underline{,} the Sab\textbf{bath} is committed in Israel on \textbf{Saturday}\underline{s}.
There are no \textbf{stra}\underline{y} \textbf{dogs} in the \textbf{streets} of \textbf{Israeli} cities.
However, their rights must be protected before they leave.
The reason for this is \textbf{bureaucratic} \textbf{obstacles} and, of course, \textbf{linguistic} \textbf{difficulties}\underline{.}
Moreover, legalisation costs money: 12 to 16 \textbf{thousand} \textbf{rub}\underline{les}.
\textbf{According} to Baranez, \textbf{weapons} \textbf{manufacturers} also contribute to the black market.
He received a photo \textbf{album} that \textbf{depict}\underline{ed} "e\textbf{very}\underline{th}ing possible".
"I \textbf{felt} like a \textbf{luxury} \textbf{shop}\underline{,}" he remembers.
"\textbf{Bu}\underline{y} a \textbf{TT} \textbf{Moscow}\underline{",} reads the laconic question from "Fed\textbf{oren}\textbf{\underline{kov}}\underline{".}
They also called for the \textbf{formation} of trade \textbf{unions} in the fast-\textbf{food} sector.
- Please \textbf{describe} \textbf{briefly} what research your group is doing.
In a \textbf{cl}\textbf{\underline{own}} all this is \textbf{blu}\underline{r}red and \textbf{lose}\underline{s} its \textbf{tragedy}\underline{.}
- Today, commercial art must be \textbf{careful}\underline{,} \textbf{careful} and \textbf{flat}\underline{ter}ing.
Con\textbf{sumption} has no culture at all; that is quite different.
But not all of them can deal with culture.
The project is \textbf{financed} by \textbf{grants} from the City of \textbf{Saint} \textbf{Petersburg}\underline{.}
Even half a century earlier, \textbf{experiment}\underline{s} with \textbf{plants} were carried out.
\textbf{Ten} hours later, the in\textbf{stinct}\underline{s} of the new\textbf{born}\underline{s} were completely \textbf{mu}\underline{ted}.
The most \textbf{valuable} thing that human\textbf{kind} \textbf{possess}\underline{es} is the \textbf{female} \textbf{organism}\underline{.}
\textbf{Up} to now, the \textbf{birth} of children in space has been \textbf{mere} \textbf{theory}\underline{.}
As far as German legislation is concerned, is it \textbf{easier} than ours?
Is it perhaps because the \textbf{auditor}\underline{s} are better there?
On these \textbf{roads}\underline{,} however, there are still some \textbf{scrap}\underline{s} of \textbf{snow} \textbf{falling} or \textbf{stretch}\underline{ed} out.
Greater attention is therefore required, especially in the higher areas.
\textbf{Road}\underline{s} I/\textbf{43} and I/\textbf{34} at S\textbf{vita}\textbf{\underline{vy}} are \textbf{chemical}\underline{ly} \textbf{treated}\underline{.}
The first class of \textbf{roads} are \textbf{mostly} \textbf{dry} but \textbf{frozen}\underline{.}
In \textbf{northern} \textbf{Bohemia}\underline{,} road \textbf{hau}\underline{lage} \textbf{centres} report several difficult \textbf{sections} of the road.
  u20\textbf{47} imon Ornest: At our \textbf{concerts} we want to \textbf{collect} positive energy.
We make every effort to \textbf{involve} these people in our projects.
There are still many things in which we are \textbf{lag}\underline{ging} behind...
But \textbf{Poland} u2019s path to space began much earlier.
\textbf{Both} projects were concerned with the military use of \textbf{rocket} \textbf{engines}\underline{.}
The maximum \textbf{altitude} for all three types was \textbf{37} km.
The \textbf{repeal} of the \textbf{Non}\underline{-}\textbf{profit} \textbf{Work}\underline{s} \textbf{Act} is not a solution.
This decision \textbf{provoke}\underline{d} a \textbf{lively} public debate.
These ideas did not come from \textbf{Brussels}\underline{,} however, but from \textbf{Prague}\underline{.}
I am not about being a senator or \textbf{president}\underline{.}
You will not get far in \textbf{politics} in the long term.
I try to find \textbf{allies} for my views and \textbf{vision}\underline{s}.
This \textbf{sounds} a bit like O\textbf{kam}\textbf{\underline{ura}} \textbf{saving} the Czech Republic.
But that does not \textbf{relate} to the level of pay.
For example, my \textbf{vice}\underline{-}\textbf{pre}\underline{s}\textbf{ident} will be \textbf{managing} \textbf{director} of the travel \textbf{agency} in \textbf{spring}\underline{.}
A\textbf{pproximately} 20\textbf{0,000} to 40\textbf{0,000}\underline{,} and this is still the case.
You will find the complete discussion in the \textbf{Saturday} issue of \textbf{Pr} xe1vo.
The 8\textbf{0,000}\underline{-}in\textbf{habit}\underline{ant} community has the \textbf{lowest} level of education in the \textbf{Netherlands}\underline{.}
What does a '\textbf{normal}\underline{'} foreign policy actually mean from a German point of view?
It may even show some respect for Germany.
There are different \textbf{opinions} in Europe on the \textbf{Palestinian} initiative.
The United States, on the other hand, has clearly \textbf{declared} itself in favour of a \textbf{veto}\underline{.}
\textbf{Are} there any \textbf{differences} between the US and many European \textbf{nations}\underline{?}
"\textbf{Marke}\underline{t} protection" in China: When \textbf{Pu}\underline{ma} and \textbf{Arm}\textbf{\underline{ani}} \textbf{suddenly} become Chinese.
Even then, it is not clear whether they are right.
\textbf{Pat}\underline{t}\textbf{loch} \textbf{opens} a \textbf{folder} with \textbf{registration}\underline{s} of the \textbf{Trade}\underline{mark} Office in \textbf{Beijing}\underline{.}
For example, the number of un\textbf{process}\underline{ed} \textbf{appeal}\underline{s} \textbf{fell} by 2\textbf{2\%}\underline{.}
Or we are being \textbf{forced} out of the market in the \textbf{segment} in question.
The \textbf{bacteria}\underline{l} S\textbf{TI}\underline{s} include \textbf{sy}\textbf{\underline{phil}}\underline{is}, \textbf{ch}\textbf{\underline{lam}}\underline{y}\textbf{dia} and tripper (\textbf{Go}\underline{n}orrh xf\textbf{6)}\underline{.}
That is about one tenth less than in the previous year.
The \textbf{ice} cover may be up to 20 metres \textbf{thick}\underline{.}
The Nasa \textbf{tip} \textbf{telescope} \textbf{shot} this photo of the \textbf{Gala}\textbf{\underline{ctic}} \textbf{Bir}\underline{th}\textbf{place}\underline{.}
However, with the \textbf{telescope}\underline{,} the \textbf{colours} are better applied.
One of the largest and \textbf{sharp}\underline{est} \textbf{shot}\underline{s} of the Hu\textbf{bble} \textbf{telescope}\underline{:} The \textbf{Jacuzzi} \textbf{galaxy}\underline{.}
\textbf{Depend}\underline{ing} on the \textbf{colour}\underline{ing}, \textbf{photographs} of \textbf{spiral} \textbf{galaxies} become true works of art.
This \textbf{starb}\underline{ur}st \textbf{recorded} the Hu\textbf{bble} \textbf{telescope} in the \textbf{spiral} \textbf{galaxy} M\textbf{83}\underline{.}
This image was \textbf{assembled} from \textbf{optical} and X-\textbf{ray} images of different \textbf{telescope}\underline{s}.
In the picture you can see the latest \textbf{launch} \textbf{preparations} at the \textbf{Ke}\underline{pl}er space \textbf{telescope}\underline{.}
The \textbf{primary} \textbf{mirror} of the space \textbf{infrared} \textbf{telescope} has a \textbf{diameter} of \textbf{6.}\underline{5} \textbf{meters}\underline{.}
In \textbf{southern} \textbf{Azerbaijan}\underline{,} many people are \textbf{reaching} a \textbf{bi}\textbf{\underline{bli}}\underline{cal} age.
In \textbf{southern} \textbf{Azerbaijan}\underline{,} many people are \textbf{reaching} a \textbf{bi}\textbf{\underline{bli}}\underline{cal} age.
This is my \textbf{grand}\underline{fa}\textbf{ther}\underline{,} who was \textbf{120} years old.
Museum \textbf{director} Fatu\textbf{lay}\textbf{\underline{eva}}\underline{,} on the other hand, \textbf{believes} that it lies at the diet.
The \textbf{propaganda} \textbf{sounds} \textbf{strange} from the \textbf{mouth} of an old \textbf{woman}\underline{.}
\textbf{Riva}\underline{l} \textbf{demonstrations} in \textbf{Cairo} \textbf{reveal} the deep \textbf{division} of the country.
These \textbf{courts} were used to \textbf{op}\underline{press} \textbf{opponents} during \textbf{Mubarak} u2019s rule.
A majority in favour of the \textbf{Islamist}\underline{s} u2019 draft is \textbf{deemed} safe.
Rakfisk from \textbf{Norway}\underline{:} Is this the most \textbf{od}\textbf{\underline{ious}} fish in the world?
We are, as they say, a \textbf{prudent} people.
"\textbf{And} of course \textbf{eat} Rakfisk," she \textbf{adds} with care\textbf{free} \textbf{laugh}\underline{ter}.
But in the evening the \textbf{ham}\textbf{\underline{fish}} is on the menu.
A man falls from his \textbf{chair}\underline{,} \textbf{possibly} overw\textbf{helm}\underline{ed} by the \textbf{Aqua}\textbf{\underline{vit}}\underline{.}
\textbf{According} to the official version of the events, \textbf{Maria}\underline{na} committed \textbf{suicide} in \textbf{2010.}
The \textbf{officials} asked mening questions and \textbf{wrote} his \textbf{answers}\underline{.}
In their view, our \textbf{existence} is a \textbf{symbol} of failure.
And in the United States we are seen as \textbf{Mexican}\underline{s}.
This includes a peace agreement between Israel and the \textbf{Palestinians}\underline{.}
In this way, \textbf{Australia} is \textbf{introducing} the most \textbf{stringent} rules for \textbf{tobacco} \textbf{packaging} in the world.
\textbf{Other}\underline{s}, on the other hand, say that the laws have \textbf{boost}\underline{ed} their business.
\textbf{Canada} was the first country to pre\textbf{scribe} \textbf{photographic} \textbf{warning}\underline{s} in 2001.
\textbf{Hard}\underline{er} laws are being considered in Great \textbf{Britain}\underline{,} New \textbf{Zealand}\underline{,} South Africa and India.
"In fact, \textbf{bo}\underline{re}\textbf{dom} has a very long history," he \textbf{says}\underline{.}
It is not only today u2019s \textbf{university} students who are being \textbf{attacked} for their views.
\textbf{Yes}\underline{,} I \textbf{ran} because I \textbf{suffered} \textbf{systematic} \textbf{harassment} and \textbf{threats}\underline{.}
As an \textbf{incredibly} \textbf{sh}\underline{y} 18-\textbf{year}\underline{-}\textbf{old}\underline{,} I \textbf{arrived} in September \textbf{1986}\underline{.}
The hatred of the \textbf{Conservative} Party had reached its \textbf{cli}\textbf{\underline{max}}\underline{.}
Most Tory first \textbf{semester}\underline{s} \textbf{claim} to be \textbf{Labour} \textbf{supporters}\underline{.}
In a local \textbf{pub}\underline{,} I \textbf{tried} to get my way.
\textbf{Would} I be able to meet like-\textbf{minded} people only after \textbf{dark}\underline{ness} \textbf{broke} down?
"\textbf{He} was im\textbf{pec}\underline{c}able; time \textbf{leaves} no \textbf{trace} of him".
This is the \textbf{biggest} problem in that country.
A \textbf{friend}\underline{'}s \textbf{acquaint}\underline{ance} was blackmailed in a social network.
This is my opinion, and so is in our \textbf{hospital}\underline{.}
\textbf{Everything} is different when you know that you have \textbf{AIDS}\underline{.}
Some think that they will die and want nothing.
There are 13,4\textbf{35} \textbf{cu}\textbf{\underline{mul}}\underline{ative} cases \textbf{(12}\underline{,}158 \textbf{AIDS} and 1,1\textbf{17} \textbf{HIV}\underline{).}
\textbf{Two}\underline{-}\textbf{band}\underline{ed} \textbf{Kara}\textbf{\underline{mbo}}\underline{le}: a \textbf{blow} for Vitro and for the country.
It should read '\textbf{Her}\underline{e} is the \textbf{honourable} \textbf{citizen} J.R. E\textbf{wing}\underline{'}.
This is the only business he has not won.
A \textbf{Republican} strategy to \textbf{counter} \textbf{Obama} u2019s re-el\textbf{ection}
\textbf{Men} of \textbf{African}\underline{-}\textbf{American} origin also run a higher risk.
\textbf{Unfortunately}\underline{,} there is no \textbf{miracle} \textbf{cure} for \textbf{cancer} \textbf{prevention}\underline{.}
It is also a risk \textbf{factor} for several other types of \textbf{cancer}\underline{.}
\textbf{Both} at the level of \textbf{physical}\underline{,} \textbf{emotional} or \textbf{spiritual} comfort.
In the \textbf{Victor}\underline{-}\textbf{Ga}\textbf{\underline{db}}\textbf{\underline{ois}} home, no day is like the other.
She \textbf{says} that the procedure is 'a \textbf{painful} but positive'.
At that time I just \textbf{recovered} from a series of \textbf{injuries}\underline{.}
What is the goal of the \textbf{association} in this competition?
We will try to get as far as possible.
This makes it all the better that we are talking about 'Z\textbf{lat}\underline{an} \textbf{dependence}\underline{'}.
This encourages others to improve their level of play.
It was my heart to take part in this European \textbf{Championship}\underline{.}
With \textbf{Bit}\underline{co}in you can pay and \textbf{sell} without a bank.
\textbf{Other}\underline{s} like the \textbf{WordPress} \textbf{blog} \textbf{platform} accept them.
NATO and the US are expected to follow at the end of \textbf{2014}\underline{.}
The \textbf{rumour} has been \textbf{spread} that Afghanistan \textbf{possess}\underline{es} \textbf{immense} natural resources.
A \textbf{referendum} should be held within 14 days.
The majority of \textbf{Liberal}\underline{s} have not \textbf{complied} with the request.
You can see here the first \textbf{signs} of theo\textbf{cracy}\underline{".}
That word was not in the previous \textbf{Constitution}\underline{.}
It is here that \textbf{Jesus} \textbf{appeared} to his dis\textbf{cip}\underline{les} after the \textbf{resurrect}\underline{ion}.
Only mountaineers can reach the \textbf{ruins} by their own effort.
All the others take a \textbf{cable} car to this historic summit.
\textbf{Among} them is the Israel Museum near the Knesset (\textbf{par}\textbf{\underline{lia}}\underline{ment}).
Entrance is free and \textbf{donation}\underline{s} are \textbf{rejected}\underline{.}
The city is mentioned in \textbf{ancient} \textbf{Greek} and \textbf{ancient} \textbf{Egyptian} \textbf{legend}\underline{s}.
Only \textbf{migrants} with legal status have to pass the test.
The fake \textbf{papers} were \textbf{printed} with an \textbf{ordinary} \textbf{colour} \textbf{printer}\underline{.}
The \textbf{weapons} enter the black market through several \textbf{channels}\underline{.}
The \textbf{weapon} is \textbf{issued} and \textbf{handed} over by the \textbf{fence}\underline{.}
\textbf{Purchas}\underline{ers} and \textbf{seller}\underline{s} most often find each other through \textbf{acquaint}\underline{ance}s.
Only there did I get the price for the \textbf{weapon} there.
There users place their \textbf{orders} and make \textbf{requests}\underline{.}
\textbf{Up} to now, this sector of the economy has \textbf{hardly} been \textbf{organized} by trade \textbf{unions}\underline{.}
No one \textbf{earn}\underline{s} less than them in this \textbf{expensive} city.
First of all, we should get \textbf{rid} of these \textbf{scar}\underline{ed} \textbf{virtual} reality h\textbf{ym}\underline{n}s!
Is there a lack of resolution, \textbf{depth} or something else?
- \textbf{Should} the number of \textbf{cameras} not be increased?
And the third camera is an \textbf{ordinary} R\textbf{GB} camera.
Or \textbf{worse}\underline{n} the problem because more \textbf{calculation}\underline{s} would be needed.
What \textbf{answers} do your group \textbf{intend} to give to this \textbf{objection}\underline{?}
Each of my past \textbf{provocation}\underline{s} was an \textbf{invitation} to talk.
- When did you know that you need to become a \textbf{painter}\underline{?}
\textbf{Tra}\textbf{\underline{chten}}\underline{berg} \textbf{moderate}\underline{d} many programs before the time of "\textbf{Ha}\textbf{\underline{lli}}\underline{-}\textbf{Ga}\textbf{\underline{lli}}\underline{".}
I love the \textbf{gro}\underline{tes}que and I have \textbf{gro}\underline{tes}que ideas.
Now you have to consider who you like.
\textbf{Unlike} animals, humans could do so in principle.
But women have been \textbf{flying} into space for 50 years.
"N\textbf{ever} \textbf{answered} this question," \textbf{says} space \textbf{veteran} \textbf{Wach}\textbf{\underline{tang}} Vuchnadze.
The \textbf{father} of the child, Andri\textbf{jan} \textbf{Nikola}\textbf{\underline{ev}}\underline{,} was also Kosmon\textbf{aut}\underline{.}
\textbf{NK}  u20\textbf{47}  \textbf{chief}\underline{:} control of the black system failures through political \textbf{cu}\textbf{\underline{lp}}\underline{ability}
First of all, let us say which way is not effective.
There are some \textbf{smooth} \textbf{snow} and \textbf{ice} on the \textbf{streets} of the Czech Republic.
\textbf{According} to the \textbf{district} road \textbf{guard}\underline{,} the view was limited due to \textbf{fo}\underline{g}.
"In the area of   u20\textbf{47} umperk there are still \textbf{snow} \textbf{residue}\underline{s} in the \textbf{altitude}\underline{s}.
Ice \textbf{smooth}\underline{ing} is \textbf{reported} especially from the   u20\textbf{47} t  u20\textbf{47} t xed area.
How did you get to work with both?
In each \textbf{concert} there are several groups and \textbf{perform}\underline{ers}.
So far, these are only individual cases of particularly \textbf{willing} personalities.
The information is only available in the \textbf{contemporary} press.
In \textbf{1962}\underline{,} however, further development \textbf{cease}\underline{d}.
The number of people affected is already in the \textbf{millions}\underline{.}
The film Argo: If it's the \textbf{worst}\underline{,} \textbf{Hollywood} \textbf{Call} \textbf{Call}
"\textbf{We} are \textbf{disadvantaged} by not having a sea.
You do not like \textbf{someone} \textbf{calling} you \textbf{populist}\underline{s}.
But without Parliament's support, you will have no more than keywords.
\textbf{Are} you \textbf{thinking} about creating your own party?
My private \textbf{assets} are \textbf{estimated} at about \textbf{CZK} 60 million.
I have already \textbf{invested} \textbf{2.5} million in the \textbf{campaign}\underline{.}
\textbf{Did} you not say that you are going to reduce these activities?
However, as President, I would stop my business \textbf{entirely}\underline{.}
\textbf{Everyone} \textbf{knows} that his book is part of this building.
So the Germans find themselves between the fronts.
\textbf{Because} of American \textbf{domestic} \textbf{politics}\underline{,} these \textbf{differences} have always \textbf{existed}\underline{.}
The Germans will simply have to play a greater role.
\textbf{Arm}\textbf{\underline{ani}} is a world-\textbf{famous} brand, \textbf{Polo} Ralph \textbf{Lauren} as well.
\textbf{Every} week a new case \textbf{ends} up on my \textbf{desk}\underline{.}
This means women who fish for rich men.
"\textbf{This} is \textbf{harmful} to business, you have to fight it," \textbf{says} \textbf{Pat}\underline{t}\textbf{loch}\underline{.}
As so often in China, the \textbf{figures} are \textbf{impressive}\underline{.}
In \textbf{2011}\underline{,}   u20\textbf{47} \textbf{1.8} billion was \textbf{collected} in \textbf{charges}\underline{.}
The matter is now \textbf{pending} before the \textbf{Supreme} Court.
The \textbf{dangers} in the \textbf{Far} East are even in \textbf{danger} of \textbf{falling} back to Europe.
Then when imit\textbf{ators} secure un\textbf{protected} \textbf{brands} there.
\textbf{Otherwise} this can be much more \textbf{expensive} than \textbf{registration}\underline{.}
More than \textbf{40\%} of the population is now \textbf{HIV}\underline{-}\textbf{positive}\underline{.}
Human \textbf{pap}\textbf{\underline{pil}}\textbf{\underline{oma}} \textbf{viruses} are also common in this country.
\textbf{Culture} is different - \textbf{flesh} to \textbf{flesh}\underline{.}'
The \textbf{eight} \textbf{planet}\underline{s} of our \textbf{solar} system, as well as the d\textbf{war}\underline{f} \textbf{planet} \textbf{Cer}\underline{es}.
\textbf{Nevertheless} it \textbf{reaches} a \textbf{diameter} of about 11 \textbf{meters}\underline{.}
The \textbf{hobby} Eberly \textbf{Tele}\textbf{\underline{scope}} in \textbf{Texas} is also \textbf{fixed} at \textbf{elevation} \textbf{angle}\underline{.}
\textbf{Drink} \textbf{butter} every day - and get 168 years old.
The trip through the Talysch \textbf{mountains} is \textbf{wild}\underline{ly} \textbf{romantic}\underline{.}
At the age of 1\textbf{36}\underline{,} still one child test\textbf{ified}
So why do so many people in the south live here?
Also \textbf{problematic}\underline{:} \textbf{civilian} military justice should be \textbf{maintained}\underline{.}
But democracy cannot work without civil-so\textbf{cie}\underline{ty} \textbf{organizations}\underline{.}
\textbf{Place} them a\textbf{mid} a b\textbf{unch} of \textbf{dirty}\underline{,} wet sports\textbf{wear}\underline{.}
We are not very \textbf{attractive}\underline{,} we do not like lauding.
The current traffic in \textbf{Mexico} City is particularly bad.
The material was then published by \textbf{Wiki}\textbf{\underline{Le}}\underline{ak}s on the Internet.
\textbf{Wiki}\textbf{\underline{Le}}\underline{ak}s has never \textbf{confirmed} Manning as a source of information.
And \textbf{Monte}\underline{zu}ma u2019s children go on the war \textbf{trail}\underline{.}
The \textbf{Israeli} hardliners, on the other hand, have the \textbf{opposite} conclusion.
For at least a while, Israel will be able to \textbf{sleep} more \textbf{calm}\underline{ly}.
So should we welcome the \textbf{bo}\underline{re}\textbf{dom} with open \textbf{arms}\underline{?}
\textbf{Bor}\underline{e}\textbf{dom} can \textbf{listen} to it almost as much as \textbf{depression}\underline{.}
But, in general, \textbf{teenagers} are a rather \textbf{narrow} \textbf{cluster}\underline{.}
Pro\textbf{ponent}\underline{s} of the legalization movement hope that the \textbf{Ministry} of \textbf{Justice} will \textbf{yield}\underline{.}
I \textbf{returned} with \textbf{hanging} head to my room.
\textbf{Anyone} \textbf{suspected} of being Tory is ha\textbf{rass}\underline{ed}.
"\textbf{You} will not be happy here," he \textbf{told} me.
It would break my heart if you \textbf{went}\underline{.}
\textbf{Valentin}\underline{o} has always \textbf{preferred} the \textbf{elegance} of \textbf{ce}\textbf{\underline{leb}}\underline{r}ity.
In the late 1990s, this was \textbf{eventually} achieved.
It already has an impact on the \textbf{housing} market.
"\textbf{He} never \textbf{knew} who it was," he \textbf{assure}\underline{s}.
\textbf{According} to Jos xe9, the \textbf{victim} has not closed the user account.
"But I know that this is \textbf{cyber}\textbf{\underline{bul}}\underline{ly}ing," he \textbf{explains}\underline{.}
\textbf{Peru} is \textbf{chair}\underline{ed} by the regional \textbf{bloc}\underline{.}
Today, his \textbf{parents} only know that he had \textbf{cancer}\underline{.}
I live a normal life, like everyone else.
\textbf{Young} people are at risk for new \textbf{infection}\underline{s}.
However, \textbf{Mexican} law \textbf{recognize}\underline{s} this possibility.
The vote would have \textbf{gone} 4\textbf{5\%} to 3\textbf{7\%}\underline{.}
\textbf{Investment} is more than \textbf{\$1}\underline{.}5 billion.
His \textbf{figures} at the level of international \textbf{tournaments} are \textbf{impressive}\underline{.}
Today the children make \textbf{unnecessary} \textbf{journey}\underline{s} and games.
This made the series a record viewer at that time.
Beginning of \textbf{courses} that study the "end of the world" study.
This is mainly the case in the English-\textbf{speaking} world.
Pro\textbf{state} \textbf{cancer} early \textbf{detection}\underline{:} should the test be made or not?
We have \textbf{sought} the opinion of two \textbf{specialists}\underline{.}
I therefore recommend that the test be carried out.
'The \textbf{conduct} of an early \textbf{detection} test does not lead to \textbf{cancer}\underline{'}.
They \textbf{saw} scientific applications, but nothing else.
Le De\textbf{voir} has \textbf{tried} to look at this in more detail.
They have a maximum life expect\textbf{ancy} of three months.
The diab\textbf{etic}\underline{s} no longer need to control their \textbf{blood} \textbf{sugar} level.
Se\textbf{wer}\underline{age} \textbf{contracts}\underline{,} the costs of which were \textbf{artificial}\underline{ly} in\textbf{flat}\underline{ed} by it.
In \textbf{Montreal}\underline{,} the "system" of \textbf{corruption} worked \textbf{smoothly}\underline{.}
The technical staff also \textbf{gave} me a great deal.
This is even \textbf{easier} with a game.
You also know that each training \textbf{unit} is crucial.
Is An\textbf{cel}\textbf{\underline{otti}} the right person for the job?
In the last season we were very close.
\textbf{Normal}\underline{ly} you should be \textbf{master} with \textbf{79} points...
I believe that this year is the right one.
One \textbf{wonder}\underline{s} what people still expect.
We could never \textbf{win} 4-0 every \textbf{weekend}\underline{.}
A team builds up over time.
In the \textbf{Champion}\underline{s} \textbf{League} we have \textbf{proved} strong.
This shows that Li\textbf{gue} 1 is \textbf{exciting}\underline{.}
It also \textbf{respects} the people \textbf{surrounding} it.
\textbf{Important} \textbf{actors} like \textbf{Wikipedia} \textbf{refuse} \textbf{donation}\underline{s} of this kind.
"The present is not a \textbf{concrete} \textbf{religious} commitment.
However, most \textbf{san}\underline{c}tu\textbf{aries} are in \textbf{Jerusalem}\underline{.}
The ski \textbf{runs} have a total \textbf{length} of \textbf{45} \textbf{kilometres}\underline{.}
There are almost 300 \textbf{museums} in this country.
The \textbf{insurance} costs an additional \$15 per day.
\textbf{Tickets} for \textbf{museums} cost an \textbf{average} of 30 \textbf{tickets}\underline{.}
"\textbf{It} is difficult without language \textbf{skills}\underline{,}" they \textbf{admit}\underline{.}
\textbf{Citizens}\underline{'} rights \textbf{activists} \textbf{emphasise} the following important \textbf{aspect} of the law.
\textbf{Supplier}\underline{s}: from \textbf{factories} to \textbf{officers}
\textbf{Other} \textbf{illegally} \textbf{sold} \textbf{weapons} come from military \textbf{weapons} \textbf{camps}\underline{.}
Many military \textbf{camps} have often \textbf{suffered} \textbf{explosion}\underline{s}.
\textbf{Another} black market \textbf{channel} is \textbf{smuggling}\underline{.}
\textbf{According} to him, the \textbf{schemes} have not changed.
"Of course without \textbf{license}\underline{",} asks user "\textbf{wan}\underline{"} (\textbf{liter}\underline{al} \textbf{quote}\underline{).}
The \textbf{buyer} \textbf{transfers} the money via a \textbf{cash} machine.
On the other hand, \textbf{corporate} \textbf{governance} does not make it easy for them.
'The \textbf{brain} is so far only \textbf{moderate}\underline{ly} \textbf{superior}\underline{'}.
- What can we expect in the future?
It is popular, but is it not over\textbf{value}\underline{d}?
- Oh, that would be very difficult to see.
- \textbf{Have} you \textbf{tried} to out\textbf{rid}\underline{e} the \textbf{brain}\underline{?}
I \textbf{understood} that I had to go down that road.
It is difficult for art to \textbf{grow} up on our \textbf{stones}\underline{.}
I do not think there are many \textbf{choices}\underline{.}
\textbf{Without} a \textbf{solid} base, the \textbf{chic}\textbf{\underline{ks}} \textbf{flood}\underline{ed} \textbf{wild}\underline{.}
The \textbf{chic}\textbf{\underline{ks}} did not \textbf{react} to light and sound.
Such \textbf{experiment}\underline{s} are not carried out for \textbf{ethical} reasons.
\textbf{Well}\underline{,} let us bypass this by giving \textbf{birth} \textbf{guidance}\underline{.}
Can you introduce the project to our \textbf{readers}\underline{?}
For more information please visit www.kp\textbf{ks}\underline{.}\textbf{cz}\underline{.}
\textbf{Are} similar big events \textbf{planned} for the future?
How do you manage these \textbf{journey}\underline{s} \textbf{logistical}\underline{ly} and \textbf{organisational}\underline{ly}?
In show business today often \textbf{copies} one to another.
Then the \textbf{Met}\underline{e}or\textbf{-2}\underline{H} and \textbf{Met}\underline{e}or\textbf{-3} \textbf{versions} were built.
This is particularly \textbf{reflected} in changes to current laws.
Af\textbf{fleck}\underline{s} Film is a special combination of several film \textbf{genre}\underline{s}.
Do you not turn your back on your \textbf{voters}\underline{?}
For me, however, this right-\textbf{wing} \textbf{thinking} is completely un\textbf{import}\underline{ant}.
In the \textbf{Senat}\underline{e} we are therefore only two independent.
You talk about \textbf{declarations} of \textbf{assets}\underline{,} what would your opinion be?
I do not have 15 million for the \textbf{campaign}\underline{.}
As \textbf{promised}\underline{,} I have \textbf{partly} reduced my activities.
But I have to live on something.
\textbf{Which} \textbf{monthly} income were you used to as an \textbf{entrepreneur}\underline{?}
The success of the education \textbf{offensive} was limited.
After \textbf{105} steps you have \textbf{arrived} at the summit.
However young and uned\textbf{uc}\underline{ated} it may be.
This is finally a starting point for \textbf{identity}\underline{.}
A foreign policy like France or \textbf{Britain}\underline{.}
That is what they are doing with the euro.
Or does Germany still find \textbf{leadership} difficult?
The Chinese call it "Bang Mingpai", a front-passenger brand.
The Chinese authorities are not aware of any \textbf{guilt}\underline{.}
The Chinese authorities are not aware of any \textbf{blame}\underline{.}
\textbf{23.}\underline{5} million people live from it in \textbf{southern} Africa.
Im\textbf{bon}\underline{gi} on Zulu means \textbf{story}\underline{t}\textbf{eller} or also \textbf{praise}\underline{r}.
\textbf{Fil}\underline{t}\textbf{lass}\underline{s} and \textbf{crack}\underline{ers} are part of the parasitic S\textbf{TI}\underline{.}
How has the number of \textbf{infection}\underline{s} developed?
The number of new \textbf{HIV} \textbf{infection}\underline{s} has been \textbf{falling} since \textbf{2007.}
It is \textbf{700} light years away from the \textbf{Aqua}\underline{r}\textbf{ius} star.
In Ariz\textbf{ona}\underline{,} USA, \textbf{stands} the \textbf{Large} \textbf{Bin}\textbf{\underline{oc}}\textbf{\underline{ular}} \textbf{Tele}\textbf{\underline{scope}}\underline{.}
The \textbf{radio} \textbf{telescope} has a \textbf{diameter} of 305 \textbf{meters}\underline{.}
\textbf{Image}\underline{s} can only be \textbf{rec}\underline{kon}ed with in 20\textbf{18} at the \textbf{earliest}\underline{.}
Here you can see an \textbf{illustration}\underline{.}
"I have never used\textbf{ham}\underline{po}o," \textbf{says} \textbf{Mir}\underline{za}y\textbf{eva}\underline{.}
After all, there is no need for \textbf{Azerbaijan} u2019s old.
To put it \textbf{plain}\underline{ly}, this means nothing other than \textbf{censorship}\underline{.}
\textbf{Clearly}\underline{,} \textbf{Mor}\underline{si} u2019s \textbf{supporters} did not want to risk that.
\textbf{Mexico} u2019s Enr\textbf{ique} \textbf{Pen}\underline{a} \textbf{Nie}\underline{to} \textbf{faces} a difficult start.
I thought I would die in this cage.
I am \textbf{afraid} you have to go through it alone, am\textbf{igo}\underline{s}.
\textbf{Perhaps} this will only lead to more \textbf{blood}\underline{s}\textbf{hed}\underline{.}
A war that is \textbf{neither} lost nor won
From a military point of view, \textbf{Hamas} is no longer a \textbf{danger}\underline{.}
\textbf{Australian} \textbf{uniform} \textbf{cigarette} \textbf{packaging} laws come into force.
But some people get \textbf{bo}\underline{red} more easily than others.
To return to my question of origin: is \textbf{bo}\underline{re}\textbf{dom} \textbf{healthy}\underline{?}
I do not think we should \textbf{celebrate} \textbf{bo}\underline{re}\textbf{dom}\underline{.}
\textbf{Nor} should we be too critical of them.
"I know who you are," he said friendly.
If you like, you can call me a white \textbf{cock}\underline{.}
\textbf{Valentin}\underline{o} is a \textbf{spectacular}\underline{,} \textbf{generous} and elegant \textbf{host}\underline{.}
So why do the \textbf{Singapore}\textbf{\underline{ans}} not have more children?
What is private for \textbf{someone} under 16?
I also spend my time with \textbf{acquaint}\underline{ance}s.
Do you know what others \textbf{publish} about you?
- So why are people still \textbf{dying}\underline{?}
\textbf{Who} was the best player in \textbf{Puerto} \textbf{Rico}\underline{?}
\textbf{Who} was the best \textbf{coach} from \textbf{Puerto} \textbf{Rico}\underline{?}
"P\textbf{eo}\textbf{\underline{ple}} \textbf{elsewhere} do not think so," he \textbf{says}\underline{.}
\textbf{Should} the test be made or not?
It \textbf{seriously} \textbf{damages} people's health.
However, their \textbf{investigations} are not con\textbf{cl}\underline{us}ive at the moment.
"I have good children," she \textbf{adds}\underline{.}
And death is part of \textbf{everyday} life.
A permanent anti-\textbf{cor}\underline{r}uption \textbf{unit} created in \textbf{2011}
\textbf{Every} day I make progress at their side.
But I am not \textbf{breaking} out with \textbf{enthusiasm}\underline{.}
What he has done is \textbf{truly} \textbf{extraordinary}\underline{.}
\textbf{Everyone} has worked for everyone else.
However, \textbf{cash} also has these \textbf{shortcomings}\underline{.}
The private initiative is given priority.
A \textbf{Constitution} with \textbf{Egypt} u2019s \textbf{Bre}\underline{ach} Bar
\textbf{Another} point of contention is the powers of the \textbf{army}\underline{.}
Pro\textbf{ponent}\underline{s} of the head of state will \textbf{march} on \textbf{Saturday}\underline{.}
There are no \textbf{museum} \textbf{guides} or \textbf{souvenir} \textbf{shops}\underline{.}
There is a total \textbf{dark}\underline{ness} when \textbf{entering} the room.
In fact, it is an \textbf{underground} fun\textbf{icular}\underline{.}
And \textbf{bicycle} \textbf{rental} costs 15 she\textbf{kel}\underline{s} per day.
We receive many \textbf{complaints} from our \textbf{migrants}\underline{.}
'\textbf{Her}\underline{e} welcome' or '\textbf{access} for un\textbf{authorised} persons \textbf{prohibited}\underline{'}
'\textbf{Do} not \textbf{sh}\underline{y} away from the cost of \textbf{false} \textbf{papers}\underline{'}
The share of legal \textbf{weapons} in criminal \textbf{acts} is very low.
Newcomers are looking for \textbf{weapons} in different ways.
You have to \textbf{wait} up to a month and a half.
In the US, fast-\textbf{food} and \textbf{supermarket} workers \textbf{strike}\underline{.}
\textbf{Ju}\underline{ma}\textbf{ane} \textbf{William}\underline{s}, Member of New York City Council
The most important reason is the high \textbf{personnel} \textbf{turnover}\underline{.}
You say it and at the same time you \textbf{interpret} it.
- \textbf{Normal}\underline{ly} I just say it.
It is not used to \textbf{calculate} the \textbf{depth} of the \textbf{object}\underline{.}
More \textbf{cameras} may \textbf{solve} the problem...
- Your work has an unmistakable style.
- Can commercial art also be beautiful?
I am not a one \textbf{hundred} \textbf{dollar} note that everyone likes.
Now every \textbf{cult} star has about 100 followers.
That is the culture I support.
There are currently good \textbf{advise}\underline{rs} in \textbf{Moscow}\underline{.}
A normal \textbf{chic}\underline{k} is developing.
\textbf{Four} days later they simply died.
The \textbf{experiment}\underline{s} will continue in \textbf{spring} \textbf{2013}\underline{.}
After \textbf{landing}\underline{,} the \textbf{Space} Councils were given off\textbf{spring}\underline{.}
The \textbf{greatest} risk was at \textbf{Ter}\underline{es}h\textbf{kov}\underline{a}.
On the other hand, the child also needs \textbf{artificial} \textbf{gravity}\underline{.}
Is the black system now \textbf{forbidden} or \textbf{permitted}\underline{?}
What criteria have you \textbf{chosen}\underline{?}
How have you \textbf{experienced} these things so far?
I think that is quite normal.
\textbf{Currently}\underline{,} The \textbf{Tap} \textbf{Tap} has \textbf{twenty} members.
These draft laws are then \textbf{passed} in the \textbf{Bundestag}\underline{.}
There have been \textbf{terrorist} \textbf{attacks} on both \textbf{sides}\underline{.}
Too much action in too many places
\textbf{Cur}\textbf{\underline{ious}} in\textbf{vention}\underline{s} are also available at home.
I had no \textbf{ambition} to become a \textbf{politician}\underline{.}
For me, it is important that we make progress.
And if it is just \textbf{decorative}\underline{.}
This was \textbf{eventually} \textbf{enforced} by NATO.
That is certainly important.
This has always been a \textbf{sensitive} issue.
This does not make it easy for the Germans.
The word is \textbf{derived} from "Bang Dakuan".
\textbf{Sometimes} the law of the \textbf{jungle} \textbf{reign}\underline{s} here.
70 of them go to \textbf{secondary} school.
What are the most important \textbf{sexual}\underline{ly} \textbf{transmitted} \textbf{diseases}\underline{?}
Not all \textbf{sexual}\underline{ly} \textbf{transmitted} \textbf{diseases} are subject to \textbf{reporting}\underline{.}
What are the \textbf{symptom}\underline{s} of a \textbf{sexual} \textbf{illness}\underline{?}
\textbf{Messenger}\underline{:} \textbf{NAS}\underline{A} \textbf{discovered} Ice on the \textbf{Mer}\textbf{\underline{kur}}
The larger \textbf{spiral} \textbf{galaxy} are called \textbf{scientists} \textbf{UG}\underline{C} 1810.
Our \textbf{insight}\underline{s} into space: The most important \textbf{telescope}\underline{s}
There is even a \textbf{museum} for long\textbf{ev}\underline{ity}.
There is even a \textbf{museum} for long\textbf{ev}\underline{ity}.
The word '\textbf{human} rights' is \textbf{missing} from the \textbf{Constitution}\underline{.}
The \textbf{Egyptian} \textbf{president} did not save on pathos.
'The word human rights does not even exist'
The \textbf{spectacle} is similar to the Euro\textbf{vision} \textbf{Song} \textbf{Contest}\underline{.}
In \textbf{Mexico} we are seen as \textbf{Americans}\underline{.}
\textbf{Perhaps} we are more "me\textbf{xi}\textbf{\underline{can}}\underline{"} than I thought.
\textbf{Both} \textbf{sides} need external \textbf{impetus}\underline{.}
But that is an \textbf{unfortunate} short-\textbf{sighted} \textbf{prospect}\underline{.}
The \textbf{tobacco} \textbf{lobby} \textbf{fought} hard against the laws.
For us this is a good business.
A WTO decision is expected in \textbf{mid} \textbf{2013}\underline{.}
"\textbf{We} are \textbf{treated} like criminals," \textbf{says} O\textbf{roz}\underline{co}.
Our community has voted against this amendment.
The atmosphere would have f\textbf{right}\underline{en}ed even \textbf{Stalin}\underline{ists}.
This \textbf{trick} should \textbf{prove} \textbf{unsuccessful}\underline{.}
"\textbf{How} have Tories \textbf{sex}\underline{?}" one asked me.
I am sure you will just be \textbf{neck}\underline{ed}.
Val\textbf{eria} Ma\textbf{zza}\underline{,} in a \textbf{dress} by \textbf{Valentin}\underline{o}
\textbf{Singapore} \textbf{Need}\underline{s} \textbf{Baby}\underline{s} to \textbf{Sav} the \textbf{Economy}
The \textbf{offline} \textbf{Private} \textbf{offline} is online privately.
The case of 14-\textbf{year}\underline{-}\textbf{old} Jos xe9 is different.
Pro\textbf{mis}\textbf{\underline{cu}}\underline{ity} should not be \textbf{promoted}\underline{.}
H xe9\textbf{ctor} "\textbf{He}\underline{tin}" \textbf{Rey}\underline{es}: "\textbf{Ba}\underline{s}\textbf{ket}\textbf{\underline{ball}} was my life"
He \textbf{enjoyed} all those who \textbf{knew} him.
\textbf{Student}\underline{s} and \textbf{professor}\underline{s} take this date easily.
These \textbf{restrictions} are not without consequences.
The same is true of the His\textbf{pan}\underline{ic} population.
They were able to \textbf{partially} limit the damage.
To make \textbf{dying} more pleasant.
'\textbf{PS}\underline{G} is not the \textbf{FC} Barcelona!'
\textbf{Everything} goes very quickly in \textbf{football}\underline{.}
An\textbf{cel}\textbf{\underline{otti}} \textbf{respects} all \textbf{technicians}\underline{.}
He had contact with big players.
\textbf{Everything} is possible from now on.
He already has the budget for this...
That is not the case today.
Of course, this would be a great \textbf{disappointment}\underline{.}
We have \textbf{concluded} with \textbf{79} points.
We are not the \textbf{FC} Barcelona!
Just as \textbf{Lauren}\underline{t} \textbf{Blanc} was.
But I do not want to make a \textbf{comparison}\underline{.}
This game has given us confidence.
In November a "\textbf{Me}\underline{ga} final \textbf{sale}\underline{"} was started.
Some are very close to the \textbf{Mos}\underline{elle} \textbf{brother}\underline{s}.
Going up\textbf{wards}
Ukraine is also mentioned there.
The \textbf{surrounding} \textbf{landscape} is indes\textbf{cri}\underline{b}\textbf{ably} beautiful.
And the working week \textbf{begins} on \textbf{Sunday} morning.
S\textbf{ense}\underline{,} problem and protection of rights
'\textbf{You} feel \textbf{hum}\textbf{\underline{ili}}\underline{ated} and \textbf{inferior}\underline{.}'
\textbf{Screenshot} of a website that \textbf{accepts} \textbf{weapons} \textbf{orders}
\textbf{Military} commentator and former military member \textbf{Viktor} Baranez
The responsible persons accept the \textbf{orders}\underline{.}
- What do you think about voice control?
Own \textbf{taste} instead of culture - \textbf{ro}\underline{s}\textbf{bal}\underline{t}.ru.
Our employees and regular guests \textbf{went} there.
The de\textbf{ception} \textbf{disappear}\underline{s} through the \textbf{dress}\underline{ing}.
We see the dis\textbf{integration} of \textbf{cultures}\underline{.}
It is called \textbf{intellectual} culture and consumer culture.
Now only your own \textbf{taste} \textbf{count}\underline{s}.
- What is \textbf{Petersburg} for you?
We have much less of that.
In principle, nothing special has been established.
The water is \textbf{gravity}\textbf{\underline{lessness}}\underline{.}
How does the control system work in Germany?
I do not think so.
This information comes from the \textbf{District} \textbf{Road} \textbf{Master}\underline{s}.
\textbf{District}   u20\textbf{47} \textbf{st} xed \textbf{nad} \textbf{Lab}\underline{em}, \textbf{Lib}\underline{er}ec \textbf{District}
The clear answer here is \textbf{yes}\underline{.}
\textbf{Much} is not written about them.
However, it is difficult to \textbf{inspire} \textbf{enthusiasm}\underline{.}
\textbf{Ban}\underline{ana}s must be 14 \textbf{cm} long.
EU: Bi\textbf{zar}\underline{re} regulations are the \textbf{exception}\underline{.}
How do you \textbf{intend} to \textbf{resolve} this problem?
And that is what you want to approach.
All have Internet, iPad and e-\textbf{book}\underline{s}.
The first \textbf{impression}\underline{:} \textbf{Book} El\textbf{dor}\underline{ado} under \textbf{cheese} \textbf{bell}\underline{.}
The look, feel and \textbf{smell} are foreign.
\textbf{Warm}\underline{ed} and \textbf{cool}\underline{ed} with \textbf{earth} \textbf{heat}\underline{.}
Lis\textbf{ette} Verhaig was also there.
The she\textbf{lves} are \textbf{filled} up\textbf{wards}\underline{.}
Szabo: '\textbf{German}\underline{s} must play a greater role'.
Famous cases also concern \textbf{graphic} elements.
"\textbf{You} have to be very \textbf{careful}\underline{,}" \textbf{says} Wen\textbf{tz}\underline{ler}.
In \textbf{2011} there were about 2\textbf{700} cases.
The star \textbf{cra}\textbf{\underline{dle}} always \textbf{produces} new youngsters.
However, there is no \textbf{birth} \textbf{certificate}\underline{.}
The \textbf{revolution} has \textbf{returned} to \textbf{Cairo}\underline{.}
He was \textbf{beat}\underline{en} up for this, \textbf{sentenced} and \textbf{imprisoned}\underline{.}
\textbf{Take} a selection of \textbf{rip}\underline{e} \textbf{cheese}\underline{s}.
And leave it there for a week.
\textbf{Spirit}\textbf{\underline{ual}}\underline{ism} can \textbf{replace} the \textbf{smell}\underline{.}
It \textbf{faces} a complex task.
\textbf{Later} I decided to \textbf{opt} for \textbf{Mexican}\underline{-}\textbf{American}\underline{.}
This clearly applies to the United States.
Many \textbf{Australian} \textbf{smokers} are defiant.
I will come back to that.
My \textbf{father} \textbf{collapsed} in \textbf{tear}\underline{s}.
But the \textbf{truth} was less am\textbf{using}\underline{.}
Why do I mention this right now?
In my view, \textbf{tear}\underline{s} were \textbf{brew}\underline{ing} up.
\textbf{Unfortunately}\underline{,} it is as it is.
The \textbf{relief} lasted only \textbf{briefly}\underline{.}
'\textbf{Val}\underline{en}\textbf{tino} \textbf{prefer}\underline{s} \textbf{elegance} to \textbf{fame}\underline{'}
And yet he is a star.
Naty Abascal and the \textbf{fashion}\textbf{\underline{maker}}\underline{,} 2006
I remember \textbf{perfectly}\underline{.}
'The population of \textbf{Singapore} must \textbf{grow}\underline{'}.
But everything has had little success so far.
They \textbf{threatened} him and asked for money.
'\textbf{He} only made it private.'
This \textbf{judgment} is not being implemented at the moment.
This also applies if we \textbf{lose}\underline{.}
He \textbf{hi}\underline{d} it from his family.
\textbf{Back} then, \textbf{AIDS} was \textbf{synonymous} with death.
The most important thing is \textbf{prevention}\underline{.}
The Court of \textbf{App}\underline{e}al does not take this into account.
\textbf{Rey}\underline{es} is not exa\textbf{gger}\underline{ating} with this statement.
That was \textbf{undoubtedly} \textbf{Pic}\underline{ul} xedn Ortiz.
What remains for you to do?
The Internet has increased these \textbf{speculation}\underline{s}.
We have a par\textbf{don} from the \textbf{Pope}\underline{.}
S\textbf{everal} remain completely \textbf{unresolved}\underline{.}
Meat products should also be \textbf{avoided}\underline{.}
The \textbf{courage} of \textbf{ordinary} death.
\textbf{Access} to \textbf{pal}\underline{li}ative care
\textbf{Large}\underline{-}\textbf{scale} property \textbf{scandal}\underline{s} in \textbf{Quebec}
\textbf{70\%} unde\textbf{cla}\underline{red} money in \textbf{electoral} \textbf{campaigns}
How do you \textbf{explain} this progress?
We are \textbf{lu}\underline{r}\textbf{king} in ambush.
We are trying to create a game concept.
It has achieved \textbf{promising} results.
We have left Afghanistan.
An \textbf{army} now \textbf{exists}\underline{.}
Faith to the holy places
Doing something for health
\textbf{Touch}\underline{ing} the \textbf{Secret}\underline{s} of Anti\textbf{qu}\underline{ity}
Is it also \textbf{sold} to \textbf{minor}\underline{s}?
A \textbf{Mak}\underline{a}\textbf{row} for \$\textbf{100}
The \textbf{hands} do not feel at all!
It is taking great \textbf{notice} of pressure!
Today there are often \textbf{misunderstanding}\underline{s}.
- \textbf{Kir}\textbf{\underline{ill}}\underline{,} what is \textbf{missing} \textbf{Petersburg}\underline{?}
It is said to be the \textbf{servant}\underline{s} of culture.
\textbf{Global} \textbf{warming} or \textbf{clash} with \textbf{Kill}\textbf{\underline{era}}\underline{ster}\textbf{oid}\underline{.}
But then the problem \textbf{begins}\underline{.}
What exactly was this about?
\textbf{Where} is the way out here?
\textbf{District}\underline{s} \textbf{Par}\underline{du}\textbf{bic}\underline{e} and Hradec Kr xe1\textbf{lov} xe9
So far no traffic \textbf{disruption} has been \textbf{reported}\underline{.}
\textbf{Who} \textbf{inspired} this idea?
Only one: L xe1  u20\textbf{47} a \textbf{Angel}\textbf{\underline{ovi}}  u20\textbf{47} .
This \textbf{trend} is therefore systemic.
Let us talk about your \textbf{vision}\underline{s}.
To do so, you need to change laws.
I have no other option.
That is not exactly \textbf{convincing}\underline{.}
\textbf{Should} I be in debt?
The \textbf{Long} \textbf{Road} to \textbf{Book}
The \textbf{urban} atmosphere is perfect.
And \textbf{everywhere} \textbf{books}\underline{,} \textbf{books}\underline{,} \textbf{books}\underline{.}
This is \textbf{cheap} and time-\textbf{efficient}\underline{.}
\textbf{Don}\underline{ations} for the New \textbf{Soul}
The room climate is very pleasant.
The rest is done by fully \textbf{automatic} \textbf{scooter}\underline{s}.
Then Berlin \textbf{abstained}\underline{.}
But what is \textbf{Arm}\textbf{\underline{ani}} \textbf{Polo}\underline{?}
There are 245000 \textbf{AIDS} \textbf{orphan}\underline{s} in Swaziland.
\textbf{Fact}\underline{s} on \textbf{sexual}\underline{ly} \textbf{transmitted} \textbf{infection}\underline{s}
How can we protect ourselves?
A \textbf{king} with 14 \textbf{wi}\textbf{\underline{ves}}
\textbf{Its} special feature is the high light collection power.
\textbf{Every} day \textbf{mel}\underline{ted} \textbf{butter}
\textbf{Two} \textbf{infant}\underline{s} also \textbf{jump} around.
\textbf{Mon}\underline{th}ly \textbf{pension} is enough to live.
We must make the \textbf{transition}\underline{.}
\textbf{Should} the \textbf{judiciary} be \textbf{strip}\textbf{\underline{ped}} of power?
\textbf{Much} of what is in the draft text is a matter of \textbf{interpretation}\underline{.}
'The \textbf{Kor}\underline{an} is our \textbf{Constitution}\underline{'}
"\textbf{Her}\underline{e} are our points, Ha\textbf{var}\underline{d}".
But that was \textbf{Mexico}\underline{.}
I was simply American.
\textbf{Want} to talk about \textbf{res}\underline{ent}\textbf{ments}\underline{?}
There is more than enough.
\textbf{Old} \textbf{Battle}\underline{s}, New Middle East
\textbf{Israelis} should also think more long-term.
The images do not \textbf{affect} me.
\textbf{Professor} East\textbf{wood} \textbf{agrees}\underline{.}
But is it one?
There are still many questions to be asked.
\textbf{Other} students \textbf{shared} his view.
I was per\textbf{vert}\underline{ed} and \textbf{dirty}\underline{.}
They \textbf{beat} each other, are they not?
It was \textbf{rare}\underline{.}
His wet \textbf{eyes} were \textbf{cloud}\underline{ed}.
Give it a chance.
And this is what a \textbf{prince}\underline{s}s \textbf{says}\underline{...}
The children can have other children.
"\textbf{This} is decided," he \textbf{explained}\underline{.}
This is a difficult question.
He was \textbf{81} years old.
The \textbf{courses} were very popular.
This goes even further.
\textbf{Imagine}\underline{...}
How to clean up.
Great players have come.
We fully accept that.
How does this network work?
\textbf{Interior} \textbf{Ministry} \textbf{ignore}\underline{s} illegal \textbf{arms} markets
\textbf{Where} do the \textbf{weapons} come from?
\textbf{Shopping} from \textbf{Sofa}
\textbf{46} \textbf{cent}\underline{s} a year?
\textbf{Who} if not me?
The task is difficult.
\textbf{Nevertheless}\underline{,} there is still a risk.
\textbf{Poland} and space.
This concerns the whole of \textbf{Latin} America.
Israel: \textbf{Labor}\textbf{\underline{atory}} of \textbf{Chaos}\underline{.}
I am not a \textbf{rescue}\underline{r}.
You do not have money?
The concept has started.
\textbf{Sp}\textbf{\underline{ijk}}\underline{en}\textbf{isse} has written \textbf{literary} history.
To combat this costs a great deal of money.
We must be extremely \textbf{careful}\underline{.}
World\textbf{aid} \textbf{Day}\underline{:} \textbf{Stop}\underline{,} \textbf{sing}\underline{,} help.
Forty per \textbf{cent} are \textbf{infected}\underline{.}
\textbf{Who} are the main groups affected?
But what does '\textbf{pri}\underline{n}\textbf{cip}\underline{les}' mean?
'The \textbf{revolution} has \textbf{returned}\underline{'}
That could take \textbf{rev}\underline{en}ge.
I cost some bits.
People \textbf{laugh} and \textbf{laugh}\underline{.}
This is \textbf{reciprocal}\underline{.}
That will not happen.
Too many \textbf{injured} \textbf{feelings}\underline{.}
I simply \textbf{ignore} them.
I do not want to \textbf{lie}\underline{.}
My friends were \textbf{confused}\underline{.}
The other students \textbf{jump}\underline{ed}.
My \textbf{door} was closed.
I never \textbf{returned}\underline{.}
The \textbf{proportion}\underline{s} are perfect.
The \textbf{King} of \textbf{Mode}
\textbf{Singapore} is a city state.
Most are relatives.
They are the same rules.
Con\textbf{dom}\underline{s} behind the \textbf{Shop} \textbf{Table}
\textbf{Dragon} Mart is \textbf{surrounded}
'\textbf{Ba}\underline{s}\textbf{ket}\textbf{\underline{ball}} was my life'.
I am \textbf{proud} of this.
What are you doing today?
La\textbf{rry} \textbf{Hag}\underline{man} is Dead
Pre\textbf{vent}\underline{ing} the \textbf{disease}
The \textbf{Hi}\textbf{\underline{gg}}\underline{s} Boson \textbf{analyze}\underline{s}
No \textbf{om}\underline{ni}\textbf{pot}\underline{ent} care
It is a \textbf{disappointment}\underline{.}
\textbf{Visit} unique \textbf{museums}\underline{.}
\textbf{List} of \textbf{tourists}
Do not peel, \textbf{boss}\underline{!}
'As in a \textbf{luxury} \textbf{shop}\underline{'}
\textbf{Military} \textbf{Comment}\underline{ator} \textbf{Viktor} Baranez
- How?
C\textbf{low}\underline{n}s are timeless.
- \textbf{Good} cultural \textbf{experts}\underline{.}
\textbf{Bir}\underline{th} in space
\textbf{Earth} at risk.
\textbf{Combin}\underline{ation} of \textbf{genre}\underline{s}
\textbf{Yes}\underline{,} that is true.
\textbf{Help}\underline{ing} \textbf{Self}\underline{-}\textbf{hel}\underline{p}
\textbf{Poly}\textbf{\underline{gam}}\underline{y} instead of democracy.
End station is Le\textbf{rik}\underline{.}
A \textbf{Direct} Man
My \textbf{Mexican}\underline{-}\textbf{American} \textbf{identity} crisis.
That is fair.
I \textbf{ran} away.
I \textbf{st}\textbf{\underline{umble}}\underline{d}.
You are \textbf{poll}\underline{ut}ed.
He \textbf{seemed} unfaithful.
\textbf{Mode}\textbf{\underline{ration}} of \textbf{Origin}
Too much stress
\textbf{Key} \textbf{Data} from Ja\textbf{lis}\underline{co}
\textbf{AC}\textbf{\underline{TA}} is Dead
\textbf{Foundation} of \textbf{Comp}\underline{et}\textbf{ival}
\textbf{Bay}\underline{am} xf3n in the \textbf{Heart}
\textbf{Want} it?'
I enjoy it.
The We\textbf{ight}
\textbf{Food}
More \textbf{stable} field
And after that?
Stars \textbf{gli}\textbf{\underline{tter}}\underline{.}
In \textbf{numbers}
'\textbf{Free} \textbf{cash}\underline{!}'
\textbf{Pil}\underline{s}en \textbf{district}
\textbf{District} \textbf{Ol}\underline{o}mo\textbf{uc}
Not \textbf{Mexico}\underline{.}
And no.
\textbf{1.2} \textbf{Children}
Unex\textbf{pec}\underline{ted} consequences
General balance \textbf{sheet}
Homex long-term
\textbf{Vitamin}\underline{s}
\textbf{Effect}\underline{s}
\textbf{Regular}\underline{ly}.
Of course.
\textbf{Dis}\underline{s}\textbf{ati}\underline{s}fied
\textbf{Karl}\underline{ov}y Vary
\textbf{Under}\underline{stand}\textbf{ably}\underline{.}
Why?
One-\textbf{two}\underline{-}three-\textbf{four}\underline{.}
\textbf{Well}\underline{.}
Hmmm.
\textbf{Yes}\underline{.}
\textbf{Privacy}
\textbf{Key} questions
\textbf{Monitoring}


==> tables/qualitiative_analysis/emb32_deen_outputs_cvt.tex <==
Corr\underline{up}tion was ramp\underline{ant}, and the people went to the poll\underline{s} with already bought votes ... "Peo\underline{ple} of character did not apply for office, so that the state had no cons\underline{ul} for eight months as a result of this decline\underline{"} ... "You really started to talk about the fact that the only medicine in this difficult situation was to rule alone and that a strong man had to be elected\underline{"}...
The current Prime Minister of Israel, the Falk Net\underline{an}yahu, is a typical example of a fasc\underline{ism}-prone politician loyal to international bankers who is doing everything possible to spark a war with Iran, which, given Iran's membership of the Shanghai Cooperation Organisation (China\underline{,} India, Russia, Pakistan...)\underline{,} could rapidly spread to a global conflict, and could lead to the destruction of the world economy because of Iran's control of the only 2-\underline{mile}\underline{-}wide Stra\underline{it} of Hor\underline{mus}\underline{,} which accounts for 20\% of world oil supplies\underline{.}
In order to facilitate World War II, the bankers allowed politics to create a latent conflict situation by imposing giganti\underline{c} war repair\underline{s} on Germany, thereby creating the precondition\underline{s} for impoverished masses, so that they had to rejoice the Germans only with a sufficiently strong leader to name the guilty and offer simple solutions; another factor was the creation of the multi-ethnic state of Czechoslov\underline{ak}ia with a strong German minority\underline{,} which was supposed to take on the function of a fifth column and also took on the function of spark\underline{ing} the war.
One of the galleries in Somerset House has been transformed into a glorious and 60-metre\underline{-}long cat\underline{walk} that proposes a change of role: the user takes the place of the model and goes along the cat\underline{walk} to admire a dream\underline{like} "audi\underline{ence}" carrying masterpiece\underline{s} by Valentin\underline{o}, such as the dress chosen by Jack\underline{ie} Kennedy for her wedding with Arist xf3teles Onassi\underline{s}, the costume\underline{s} worn by Mon\underline{ica} Vitti in "La Notte", or a coat of wool and leather belonging to the Em\underline{press} Far\underline{ah} Diba.
The first war was aimed at eliminating the great monarch\underline{ist} states of Europe, and the second war was intended to break Britain\underline{'}s colonial rule in particular, and the third war was to reduce the world's population to about 0.5 - 1 billion people (such a number would provide their comfort and luxury and would not consume so much resources), create a universal religion (ecum\underline{en}ism is no more than the run-up) and ultimately lead to the takeover of absolute power.
The experts and officials of the Consejo Estatal de Prevenci xf3n del Sida en Jalis\underline{co} (Co\underline{es}ida\underline{)} (Stat\underline{e} Committee on AIDS Prevention in Jalis\underline{co}) and also patients such as Fabr\underline{i}zio\underline{,} who conducted his test at a private laboratory\underline{,} for the sole reason that he had made a friend of him who, despite his young age, was already in the AIDS phase and even had the Kap\underline{os}i-Sarkom (a cancer\underline{ous} tu\underline{mor}\underline{),} which is one of the usual complications\underline{.}
The specialist for infectious diseases and HIV\underline{/}AIDS\underline{,} Andrade Villanu\underline{eva}\underline{,} commented that since 2008, scientists have concluded that although AIDS is not a death sentence\underline{,} that the years of survival and quality of life depend on the degree of impair\underline{ment} of the immune system of people at the beginning of treatment, and that those who are not addict\underline{ed} to drugs would have greater opportunities: up to 30 years at a count of 200 CD4 and 50 years at a count of 500 CD4.
The most serious aspect of this case is that the Court left aside a document sent by the Government of Mexico under the figure of amic\underline{us} cur\underline{ia}e, which describes the proceedings carried out by Vitro under the Trade Concur\underline{r}ency Law\underline{,} pointing out that it had strictly adhere\underline{d} to the agreements signed by both countries in order to comply with Chapter 15 of the bankruptcy law of the United States.
The Roth\underline{schild}\underline{s} are involved in almost all of the world u2019s central banks, and against the countries in which they are not central banks, they wage wars or arm themselves against them (before the attack on Afghanistan, there were 7 countries, there were 5 countries after the attack on Iraq, and after the fall of Ghaddafi, there were only four, with Russia, meanwhile\underline{,} submitting its central bank to the Russian government).
31 years after the appearance of AIDS in the world, i.e. after the first reported cases, 'the great success today implies that the survival of a patient who receives treatment in time and the survival of the general population is exactly the same', said the head of the HCG HIV unit\underline{,} Jaime Andrade Villanu\underline{eva}\underline{,} saying that this information was supported by a prestigious scientific publication in April of this year.
Correa said that the solution to the asylum granted to Assange since June at the Embassy of Ecuador in London was to grant a free hand-in-hand to travel to Ecuador\underline{,} and that this would be in the hands of the United Kingdom\underline{,} Sweden and the European legal authorities, underlining that there had been talks with London to find a solution to the imprisoned founder of Wiki\underline{Le}\underline{ak}s.
There he earned 75,000 rupees (6.2 euros\underline{)} a day, and the work was not so hard, but Anto has returned with his family to Ban\underline{yu}\underline{wang}\underline{i}, a village nearby\underline{,} for a reason as important as sulphur in Indonesia\underline{:} "I married a girl from Bali\underline{,} where they are Hindu\underline{ists}, and I brought her to Java to convert them to Islam\underline{".}
Even when the sul\underline{fur} burn\underline{s} the thro\underline{at} and chews the eyes\underline{,} when the wind turns suddenly and the mine\underline{work}\underline{ers} are stuck in the thick column\underline{s} that rise out of the cra\underline{ter}, the men are so hard that no one complain\underline{s} about serious diseases ... of course, except the usual respiratory problems, arthrosis\underline{,} pain in the knee\underline{s} and bubble\underline{s} on the shoulders that have deformed from the weight of the basket\underline{s}.
In her study "The Unengaged Mind\underline{:} Defin\underline{ing} Bor\underline{e}dom in Terms of Attention\underline{"} - for example: "The idle mind: The definition of bo\underline{re}dom from the point of view of attention", published in September in the trade journal "Per\underline{spect}\underline{ive}s on Psycho\underline{logical} Science\underline{",} Professor Eastwood and his colleagues point to an earlier experiment in which participants listened to a band on which a person had read a magazine article\underline{.}
Since 2009, a civil-military service of the Ministry of Defence (Cimic), which was discontinu\underline{ed} in 2012\underline{,} has carried out in dozen\underline{s} of mountain villages numerous non-profit activities and measures for the restoration of agriculture and has been carried out by a small French non-governmental organisation to try to win the "hearts and spirits" and to achieve the impossible task of reco\underline{n}cil\underline{ing} aid and offensive actions.
The austerity measures of virtually all EU-South countries will undoubtedly end up in the same state, with people being forced to emigr\underline{ate} (as was the case in the 19th century) under pressure from a catastrophic decline in their social level, or for a starvation wage on the fringe\underline{s} of society, hoping that private investment capital will eventually flow into the country.
Even if mortality has decline\underline{d} significantly in recent years (in Mexico\underline{,} the number of people dying of AIDS has decline\underline{d} from 6,67\underline{8} cases in 2007 to 4,86\underline{2} in 2011 (Annual Report of ON\underline{US}ID\underline{A}), it is nevertheless true that 60\% of patients registered in the national database have died since AIDS appeared\underline{.}
In Prague I have a plot worth 25 million, a flat for about 10 million, another for 8 million, an art collection worth about 10 million, as well as an Aston Martin for 3.5 million and a   u2047 ko\underline{du} superb worth about one million, and then I have a few million in my account.
"For my life I have put up many hats in basketball\underline{,} even several at the same time when I was President of the BSN, chief executive of the national team and president of the association in the 1990s," Rey\underline{es} remembered when visiting Prime\underline{ra} Hor\underline{a} at his home in Bay\underline{am} xf3n, where he lives with Isabel\underline{,} his faithful wife for more than 50 years.
In addition to an old man of 93\underline{,} who enjoys the last family gathering in the courtyard and is well supported by his pil\underline{low}\underline{s} while being raised to his honor\underline{,} a young man of 36 years, surrounded by his parents\underline{,} his wife and his two little children, dies tragic\underline{ally} after having tried everything to survive\underline{.}
For even if particle physics is a really strange world, it turns out that such a law also applies to them: the Paul\underline{i} principle of exclusion\underline{,} which states that two particle\underline{s} cannot occupy the same space at the same time when they are in the same "qu\underline{ant}ity state", whereas this "state\underline{"} consists largely of some of their properties\underline{.}
So far, we have felt more of an impact in the preparato\underline{ry} phase of future controls - for example, we have introduced the new control instrument 'Recognit\underline{ion} of risks of inefficiency\underline{'}, which examine\underline{s} and analyses almost 14,000 public contracts - here, of course, the changes will have an impact, as the threshold\underline{s} change, the conditions for certain types of tender have been modified, among other things.
The Second World War broke out, and whether Hitler broke away from the chain at which the international bankers had initially kept him, or whether everything went according to plan, it is difficult to estimate\underline{,} but in any case the suffering of European Jews in the concentration camps made it necessary for the international community to recognise the Jewish state.
Although rocket\underline{s} from Gaza have killed around 30 Israelis since 2004, the country has remained relatively free of suicide bomb\underline{ers}, not least thanks to the closure\underline{s} that have flow\underline{ed} into the West Bank and thus into the main part of any Palestinian state, which protect the Jewish settlements\underline{,} which have been declared contrary to international law, but are being further and further extended\underline{.}
He said that measures would be taken to 'improve cooperation in the fight against urban insecurity and organised transnational crime, as well as measures to improve access to medicines and the Internet at low prices in all areas of South America and to act jointly and effectively in the event of natural disasters\underline{'}.
In fact, the late phy\underline{s}icist Will\underline{ard} Boy\underline{le} - who worked in the Bell Lab\underline{s} in which the laser was invented in the 1960\underline{s} and who in 1962 developed the first continuous slash laser (the first pulse\underline{d}) - has already told us that the laser was initially regarded as a "lab playback\underline{".}
This is another task that we will have to face for a long time to come, namely to make a person physically in a closed space believe that he is instead in an open, practically infinite space; here we are working on concepts with tre\underline{ad}mill\underline{s} (other than in gym\underline{s}), mobile platforms and large ball\underline{s}.
Sand\underline{ra} Ha of Zi\underline{co} Import Pty Ltd\underline{,} a small family business, notes that the demand for cigarette cases and silicon\underline{e} lid\underline{s} to cover the unbe\underline{arable} packaging has increased enormous\underline{ly} since the British American Tobac\underline{co}, Britain\underline{'}s Imperial Tobac\underline{co}, Philip Morris and Japan Tobac\underline{co}, two months ago, failed at the Australian Supreme Court to challenge the laws.
Efe repeatedly tried to gain access to the signed document at the 6th Ordin\underline{ary} Session of the Heads of State and Government of the Unasur.
And it makes it that the little ones and the big ones\underline{,} the rich and the poor, the free and the servant\underline{s} all give themselves a sign of their right hand or their forehead that no one can buy or sell\underline{,} for they have the sign, namely the name of the animal or the number of its name.
Controvers\underline{ial} EU regulations include, among other things, the mandatory ad\underline{mix}\underline{ture} of bio\underline{e}than\underline{ol} to fuels that are consequently harmful to nature, the ban on reliable mercury thermo\underline{meter}\underline{s} simply because they contain a relatively small amount of this hazardous substance\underline{,} and also the directive on the size of chicken cages\underline{,} which has made eggs much more expensive this year.
However, there are also technologies that are actually designed to give the "pic\underline{ture}s in the air" some tangible strength\underline{,} for example, the interference of some directed ultra\underline{sound} beam\underline{s} creates a feeling at a certain point where the finger is located, a feeling that is still so weak at the moment, as if someone was cry\underline{ing} over the handball\underline{s}.
The best scenes of the film play in the streets and show the reconstruction of events that have really taken place - the entrance sequence of the storm\underline{ing} of the message is very impressive in its clarity\underline{,} yet convey\underline{s} the sense of confusion and unpre\underline{dic}\underline{t}ability that occurs when history moves somewhere\underline{.}
However, with the few he works quite successfully\underline{,} sometimes helping the reality - which does not always seem so elegant (the scenes in which the imminent crisis at Tehra\underline{n} airport is turned away from a telephone call in America, or even the cha\underline{se} on the runway, seem somewhat knot\underline{ted}).
In the first hall of this exhibition\underline{,} which will be on view until March 3rd\underline{,} there are many private letters and photos with the signature of the most exquisite aristo\underline{cracy}\underline{,} from Prince\underline{s}s Salima\underline{h} Aga Khan to Prince\underline{s}s Marie\underline{-}Cha\underline{n}tal of Greece and Margarita of England to Lord Snow\underline{don}\underline{.}
It is only 250 meters to the peak of the volcano\underline{,} which rises up to 2386 meters above sea level, but the exhaust\underline{ed} beam\underline{s} take more than 40 minutes to climb at the tortoise speed, keeping the balance and taking their steps carefully so that they do not slip and fall.
In this sense, the President of Colombia\underline{,} Juan Manuel Santo\underline{s}, said before he began attending the regional meeting that he expected a meeting in Mexico on Saturday with his counterpart in Nicaragua\underline{,} Daniel Ortega\underline{,} to respect the maritime conflict following a judgment of the ICC questioned by Bogot xe1.
According to The Particle Adventure website, these bo\underline{son}s are grouped into two groups by the Ber\underline{ke}ley Labor\underline{atori}\underline{es} (which\underline{,} by the way, is absolutely amazing\underline{):} the mesons that we are not going to treat here and the "power particle\underline{s}" through which the great forces of nature spread and with which the Hi\underline{gg}\underline{s}-Bo\underline{son} would be somehow related.
According to the Ministry of the Interior\underline{'}s official statistics\underline{,} the number of illegal weapons offences throughout Russia decreased by 7\% to 22.\underline{9} thousand between January and October 2011\underline{,} while the number of cases of theft and blackmail relating to weapons\underline{,} ammuni\underline{tion}, explosive\underline{s} and explosive devices decreased by 7.\underline{8\%}\underline{.}
The only reason so many people of Mexican origin live in cities like Los Angeles\underline{,} Las Vegas\underline{,} Phoenix\underline{,} Denver or San Antonio is that at one point in our family tree\underline{,} a person - perhaps a parent or grand\underline{parent} - was not given a chance in Mexico and emigr\underline{ated} north\underline{wards}\underline{.}
Restall pointed out that many days had been spoken of by the last court over the years, and said that if nothing happened on 21 December, "people immediately thought of a new date" or phil\underline{oso}\underline{ph}ised that 21 December was the beginning of a seven\underline{-}year period, according to which the end of the world would come.
Sebelew is convinced that a future migrant without language skills will inevitably meet people with bad intentions who, on the pretext of aid, put him in a dark\underline{,} narrow barrack\underline{,} where he will endure dozen\underline{s} of unpara\underline{lle}led months without food and documents and work 12 to 14 hours a day.
What is particularly disastrous is the fact that today's elite\underline{s} are completely ignor\underline{ant} of the possible future loss of hundreds of thousands of human lives, the humanitarian and social disasters we are already witness\underline{ing}, and the crimes against humanity that we know from older and more recent history.
The patient must be made genuinely aware of the extent of the risk of his or her cancer by indicating the possible options whereby prostate cancer\underline{s} can remain untreated if they do not affect the quality of life in the long term and, in these cases, opt for active monitoring of the disease\underline{.}
Parti\underline{cip}\underline{ants} in the protests that began on Thursday at 6.\underline{30} a.m. in front of McDonald\underline{'}s on 40th Street and Madison Avenue demanded that the cash\underline{iers} and chef\underline{s} of fast food restaurants receive a minimum wage of USD 15 an hour\underline{,} which is more than a doubling of the current minimum wage\underline{.}
The culminat\underline{ion} of the protests was a lunch\underline{time} meeting outside McDonald\underline{'}s at Times Square\underline{,} where some local democrat\underline{s} spoke\underline{,} including council\underline{lor} Ju\underline{ma}ane William\underline{s}, who said: 'McDon\underline{al}d's says it sell\underline{s} billions of portion\underline{s}, yet you are not given sick days and you are not paid for your honest work!'
Samuel Robert\underline{s}, 21-year\underline{-}old history student at Corp\underline{us} Christi\underline{,} who initiated the appeal for greater protection, believes that such a climate is "uncan\underline{ny}".
The two president\underline{s} confirmed that they would submit to the ICC after Colombia took legal action against the Bogot xe1 Agreement, which it agreed to submit to the judgment\underline{s} of this international court\underline{,} following a decision on the maritime borders with Nicaragua\underline{,} which considered it to be a serious mistake\underline{.}
Correa also supported the decision to maintain the veto against Paraguay in Unasur at least until its next elections, arguing that the organism must remain "hard and must not condon\underline{e} opportun\underline{ism} and any coup d' xe9tat legally disguise\underline{d}" because it "destro\underline{y}ed the legitimacy of democracy in Paraguay\underline{.}"
"I work, do a lot, have an active but responsible sex life, I pay attention to my health and that of the other person," count\underline{s} Fabr\underline{i}zio\underline{,} who agreed to share his intimate details with MIL\underline{EN}IO JALISCO in order to encourage with his testimony those who are afraid today in the context of AIDS Day worldwide.
Afghanistan, the land of mountains with strong local identities\underline{,} should have benefited from a degree of decentral\underline{ization} based on the example of Western nations\underline{,} but by abolish\underline{ing} the post of prime minister since the constitution of 1964\underline{,} the US wanted to make it a centralized state with a strong presidential power.
When it comes from another EU country, poverty simply migrate\underline{s} from one country to another; or capital is left out completely, because in China, India, Brazil\underline{,} Turkey, Morocco or Egypt or Africa at all, workers work for a fraction of European wages\underline{.}
The CIA\underline{,} in cooperation with the Canadian authorities, managed to bring the refugees from Iran, helping them with an extravag\underline{ant} story to cover up their true identity - they traveled camouf\underline{lage}d with Canadian passport\underline{s} as members of a film crew who alleged\underline{ly} visited locations for a science fiction film in the country.
Because the government failed to comply with a request from the Senat\underline{e} to explain the conditions and circumstances under which the Mexican ambassador to Japan signed the Anti-Co\underline{unter}\underline{fe}iting Trade Agreement, known as AC\underline{TA}\underline{,} the matter has already been archive\underline{d} under the Mexican Institute of Intel\underline{lect}\underline{ual} Property\underline{.}
It recommends a complete overhaul of the public procurement system and the financing of the parties: 'We cannot fall deeper\underline{;} by getting to the bottom of things with courage\underline{,} we can rebuild the house on a more solid basis, with more controls and laws'.
Some support Israel and argue its right to self-defence while calling the Palestinians terrorists\underline{;} others support the Palestinians\underline{,} argue with the racism of the Israeli state, with the genocide perpetrated against the Palestinian Arab\underline{s}, and call the State of Israel terrorist\underline{.}
In the midst of the usual recri\underline{min}ations, countless buildings have been laid in ruins\underline{,} more than 140 Palestinians\underline{,} most of them civilians\underline{,} and six Israelis killed - and for the first time, rocket\underline{s} from Gaza have been launched near the Israeli metropolis of Tel Aviv and the holy city of Jerusalem\underline{.}
Ju\underline{bil}\underline{ant} Hamas supporters believe that Israel is an Islamist cre\underline{s}cent - from Lebanon in the north\underline{,} where Hezbollah militant\underline{s} have power, to Syria\underline{,} where rebel\underline{s} could face an increasingly Islamist face before Bas\underline{har} Assad's storm\underline{,} to Jordan\underline{,} where Hamas allies threaten the king\underline{.}
Not only Min\underline{cy}, Gausse\underline{,} Ram\underline{on} Riva\underline{s}, Fico L xf3pez and Pic\underline{ul} xedn (Or\underline{t}iz), but also the young players (Ja\underline{vier}\underline{)} "To  u2047 ito" Col xf3n and James Carter, the brother\underline{s} Le xf3n (Fran\underline{ci}sco and Ed\underline{gar}) and Mario "Qu\underline{ij}\underline{ote}\underline{"} Moral\underline{es}, who couldn't be there in 1990 because of knee injury\underline{.}
Egypt\underline{,} together with Turkey and Qatar\underline{,} must now stop the supply of arms to Gaza and is better positioned than ever to convince Hamas of the idea of a Jewish state based on the 1967 borders, supplement\underline{ed} by territorial exchanges and a common Jerusalem\underline{.}
In this sense, he congratulated himself on the fact that Ecuador is no longer dominated by such journalists 'and not by bankers or hegemonic and civic countries', and anticipated that, in a re-election\underline{,} he 'will deepen the revolution in order to continue along the path in this right direction'.
It is also true that, after deduct\underline{ing} the votes of the branches\underline{,} the creditors of Vitro, the creditors who took action against Vitro in the United States courts\underline{,} i.e. the vul\underline{ture} funds such as Aureli\underline{os} Capital\underline{,} Aureli\underline{os} Convergencia, Ellio\underline{t} Internacion\underline{al} and Liverpool Limited\underline{,} would not have obtained a majority.
Before being tied to the wheelchair by a stroke in 2008, Rexes was part of this sport for 6 years, be it as lower-class players, first national league players, BSN agents and leaders with the Va\underline{quer}\underline{os} de Bay\underline{am} xf3n or president of the Basketball Association\underline{.}
We have compared all of this and, although the review has not yet been completed\underline{,} we have seen some very interesting differences\underline{,} generally speaking\underline{,} the laws are perhaps even more 'str\underline{eng}\underline{th} and perfect' in Germany, but the actual application is better in some parameters\underline{.}
I do not want to write at this point about who is to blame in these recurring waves of killing and who is to be the victim\underline{;} in the end, the present-day inhabitants of Israel, including the self-government areas, were born into the current political situation and did not experience the beginning of violence itself.
It is also relatively absurd to have a directive that affects European officials themselves - anyone who has an official role in the EU must not use the name Macedonia because of the sensitivity of the issue to Greece and must instead say FYROM (former Yugoslav Republic of Macedonia\underline{).}
On Friday\underline{,} Jud\underline{ge} Manning also questioned an accus\underline{ation} that he made in his statement on Thursday - so he had to sleep naked in his cell in Qua\underline{n}tico and face naked guard\underline{s} and other prisoners at a morning count\underline{.}
My wife\underline{,} born in Gua\underline{dal}\underline{aja}\underline{ra}, who legally migrate\underline{d} to the United States as a child, reminds me that there is tension between Mexican\underline{s} and Mexican Americans\underline{,} because Mexican\underline{s} have a clearer idea of who they are - and Mexican Americans do not.
If at least some Mexican\underline{s} are not ready to give the United States a deal with Mexico a century and a half ago, they must also accept that some Mexican Americans have a res\underline{ent}ment about how their family members were treated not so long ago.
After a long reading of research literature and the presentation of the idea in front of a focus group of about 100 people Professor Eastwood and his colleagues concluded that bo\underline{re}dom can be defined as the experience of "to do a satisfy\underline{ing} job but not to do it".
Peru u2019s president\underline{s}, Ollanta Hum\underline{ala}\underline{,} and Chile\underline{,} Sebasti xe1n Pi  u2047 era\underline{,} met during the regional meeting and confirmed that they would accept the IGH u2019s decision, which begins on Monday in The Hague\underline{,} to listen to the plea\underline{s} of both sides in the trial that Lima launched against Santiago\underline{.}
With regard to the possibility of standing as a candidate for the next presidential elections in Ecuador in order to achieve his third consecutive mandate\underline{,} he said that he saw this possibility 'with much optimism and joy\underline{,} although sometimes it is very difficult'.
In these places, "the distribution of condom\underline{s} was actually increased; previously they were handed out individually\underline{,} now they give us packages with a hundred pieces\underline{,} which is good, but there are still people who do not have access to a condom\underline{,}" he said.
At a weekend meeting at a forum at the University of the Caribbean\underline{,} a group of national and foreign environmentalists, academic\underline{s}, entrepreneurs and general members of civil society decided to create a broad front to oppose the opening of the Chinese Dragon Mart in Canc  u2047 n.
Every semester\underline{,} when the religious professor decided to hold a course towards the end of the world, he knew that he had an irre\underline{s}istible hook\underline{:} the end of the Maya\underline{n} Cal\underline{en}dar\underline{'}s "long backward count\underline{"} on 21 December, which many people believed was the end of the world.
"This experiment we are carrying out together, namely the birth of a child in a foreign environment, will lead us to bring a disabled person, a completely unadapt\underline{ed} person," says Igor Pest\underline{ow}, head of the Bio\underline{eth}\underline{ics} Commission of the Institute for Medical and Biological Problems\underline{.}
The world's first laws on uniform packaging for cigarette\underline{s} and tobacco have come into force in Australia\underline{,} replacing brand logo\underline{s} and colours with neutral\underline{,} olive\underline{-}green lid\underline{s}, which are printed with drastic images showing sick body parts and infant\underline{s} and children suffering from cigarette smoke\underline{.}
"You can already see in children of young age that they understand the message that the tobacco companies are trying to promote their brand image," says Federal Minister of Health\underline{,} Tan\underline{ya} Plib\underline{ers}ek, who quote\underline{s} studies showing\underline{,} for example, that children associate the crown of a logo with the idea of a prince\underline{s}s.
You will also not receive a share of the 30,000 rupees (2\underline{.}5 Euro) supplement per camera that the guardian\underline{s} of this natural park, together with the entry fee of 15,000 rupees (1\underline{.}2 Euro) demand from tourists who come to photograph the volcano and the human carrying\underline{s}.
The President of Ecuador also considers the desire of his Colombia\underline{n} counterpart\underline{,} Juan Manuel Santo\underline{s}, now and following the judgment of the International Court of The Hague\underline{,} which favoured the maritime sovereignty of Nicaragua to negotiate with Nicaragua the maritime borders between the two countries, to be 'absolut\underline{e}ly justified\underline{'}.
He also trusted in a good conclusion to the disputes over the maritime borders between Peru and Chile before the same Court of Justice\underline{,} saying that 'it is right for Latin America to invoke international jurisdiction\underline{s} if both countries commit themselves to accept the judgment\underline{,} even if it is very harsh\underline{'}.
After the Court of App\underline{e}al of the United States has confirmed a ruling that does not recognise the restructuring of the liabilities of the Vitro Group, achieved through a trade agreement in Mexico\underline{,} a disastrous precedent will be created for any national company with subsidiaries in the neighbouring country that has payment problems.
Former construction engineer Gill\underline{es} Sur\underline{pre}\underline{n}ant described this in detail before the Commission: in ten years he received gift\underline{s}, invitation\underline{s} to travel, golf tournaments\underline{,} restaurants and ice hoc\underline{key} games, as well as bri\underline{bes} of \$73\underline{6,000} in exchange for sewer\underline{age} contracts\underline{,} the costs of which he artificial\underline{ly} inflat\underline{ed}.
After the Bit\underline{co}in rate reached \$30 (23 euros\underline{)} in June 2011\underline{,} it fell five months later to \$2 before recover\underline{ing} today to around \$10 (the rates are listed on the bitcoinchart\underline{s}.com website).
The demonstrators were also supported by other prominent New York democrat\underline{s}, for example, Mayor\underline{ial} candidate Bill De Bla\underline{s}io, who said that 'we should jointly support the fast-food workers so that they can earn a fair wage and achieve the economic prosperity that every New Yorker deserves\underline{!}'
Ap\underline{parent}\underline{ly}, the liberal democracies are now rapidly entering a situation as described by App\underline{ian} in his work on the crisis of the Roman Republic at the time of Caesar and Pompeius\underline{:} "The state had long been in disintegration and the offices were occupied with violence.
To promote cultural exchange, the Imbon\underline{gi} Cho\underline{ir} travels through southern Africa every two or three years together, singing songs full of woe, combat spirit, confidence and black self-conf\underline{id}ence that many people on the southern tip of the black continent still know from apart\underline{heid}\underline{.}
I was harass\underline{ed} for just one reason - a reason that seemed all the more blink\underline{er}ed and cruel in this supposed cra\underline{dle} of enlightenment: my late father Wood\underline{row} Wyatt had been an important advise\underline{r} to Margaret Thatcher and I support the Conservative Party.
"The daily salary of mine workers here, where 15,000 rupees (1\underline{.}2 euros\underline{)} are paid at the coffee harvest and the average monthly income is 2 million rupees (16\underline{7} euros\underline{),} is very high," explains the bear\underline{er} who previously worked as a brick\underline{lay}\underline{er} on the tourist island of Bali\underline{.}
"My deepest secret\underline{s} I wouldn't reveal in a post," says Jorge\underline{,} 10 years old, trying to explain the meaning of "private\underline{"} in websites like Facebook\underline{,} Twitter\underline{,} Hot\underline{mail} and Windows Live Messenger\underline{,} where he has accounts for two years.
"Chi\underline{le} was, is and will continue to be a country that adhere\underline{s} to international laws, seeks peaceful solutions to disputes\underline{,} conclude\underline{s} agreements and submit\underline{s} itself to international courts\underline{,}" adds Pi  u2047 era and greet\underline{s} Hum\underline{ala} with hands\underline{hak}\underline{e} in front of the flag\underline{s} of both countries.
"We have decided to give priority to a series of 31 emblemati\underline{c} projects aimed at improving geographical links in South America and, in particular, in rural and border areas...and thus unite our countries and open up new forms of economy," said the Peru\underline{via}\underline{n} President in a read-out statement.
He also criticised the Swedish judiciary\underline{,} which asked him to interrog\underline{ate} him on his territory for alleged sex offences\underline{,} while 'Swed\underline{ish} law allowed this through a video conference that could have been carried out via the Embassy of Ecuador in London'.
He makes a telling statement: 'Nine out of ten patients come to us when they already have accompanying infection\underline{;} in order to influence global mortality\underline{,} more early diagnosis is needed, which means that massive detection tests must be offered to all those who need it'.
In practice, the recognition of Jud\underline{ge} Har\underline{lin} Hal\underline{e}'s judgment in the Ban\underline{car}rot\underline{as} court for the northern district of Texas on 15 June has left Mexican companies helpless to seize their property beyond the River Bra\underline{vo}.
But Char\underline{m} xe9 had no idea what to expect in the next two months: the destructive Hurri\underline{can}\underline{e} Sand\underline{y}, which some have called the Deuda\underline{r}magged\underline{on}, and a growing conflict involving Israel, the place where Christian theorists believe the Apocalyp\underline{se} begins\underline{.}
I had looked at websites and blog\underline{s} when someone came to my attention and suggested coming to the "Bego\underline{wa}ja" station where a person would wait for me to bring me to a certain place where we could negotiate the price.
- Of course, it is not pleasant to keep a smart\underline{phone} in your hand on the move, but I think that the best option would be a 'change\underline{able}' enlarged reality, where we could switch from glass\underline{es} to smart\underline{phone}\underline{s} via a cloud\underline{;}
"A law must be valid, and if something is prohibited by law, then it cannot simply come to the head of government, and the control office, whose duty is to monitor compliance with the law, obstruct\underline{s} its activity," Kal\underline{a} states.
Temperatur\underline{es} remain below zero\underline{,} so that snow and ice will stay on the roads\underline{,} but no problems are reported from the depth\underline{s}, especially south-east of the Bohemia\underline{n} Central Mountains\underline{,} and the roads are usually dry\underline{.}
The reck\underline{less} practice of private capital creates a situation in individual economies in which governments are forced to compete with each other in order to artificial\underline{ly} reduce the social level of their own people and thus entice foreign capital into the country.
We have to admit that we are living in a time when the wealth of the world is concentrated in the hands of fewer individuals\underline{,} and that this concentration of money and the power resulting from it has not come about within the lifespan of a generation\underline{.}
The first press agency (Reuter\underline{s}) was bought by the Roth\underline{schild}\underline{s} back in the 1990s in order to prevent its name from being linked to highly criminal acts\underline{,} in the context of which it was always the consolidation of its power, the increase of its wealth or both.
The EU app\underline{ar}ition often decides under pressure from this or that trade and industry lobby whose demands are usually represented in Brussels by one or more member states (for example, the Czech Republic is currently trying to impose the demands of Czech banks with a veto threat\underline{).}
In the official list of products registered in the EU, the company of the world-famous cheese\underline{s} Fe\underline{ta} and Gor\underline{gon}\underline{z}ola, the L xfcbeck mar\underline{zip}\underline{an} or Par\underline{ma} ham\underline{,} also the Karl\underline{ov}y Vary onion, Carp from Poho  u2047 elice and T  u2047 ebo  u2047 , or also the Saaz\underline{er} hops, appear.
On November 21, Chief Oates sent an e-mail to his Aurora staff stating that the prosecutor would no longer prosecut\underline{e} minor mar\underline{i}juana offenses in persons over 21 years of age, and that the police would not "immedia\underline{te}ly" seek criminal prosecution\underline{s} for these offenses.
Once on the top, they will clear the way between the tourists who photograph them like circus apes and walk three kilometres with the tir\underline{ing}ly heavy basket\underline{s} to the scale that a mining company has placed a little further down at a height of 1850 meters\underline{.}
While the judge points out that creditors must be subject to bankruptcy law in the United States, the New Orleans\underline{-}based Court of App\underline{e}al initially says that the main proceedings are the trade contract dealt with in Mexico\underline{.}
The company's spoke\underline{s}man, Dan Fo\underline{gel}man, claimed in an interview on the website of the left-wing Huff\underline{ington} Post that a total of "less than five" Wal\underline{mar}t workers laid down the work and that the protest action was only "an additional trade union PR trick\underline{"} that organized the protests\underline{.}
This is a situation in which the manufacturer tries to compete economically by import\underline{ing} cheap goods by 'under\underline{bid}\underline{ing}' competition in order to gain a larger market share and increase its profits\underline{.}
While the rest of the Arab world is taking tim\underline{id} steps towards democrat\underline{ization}, Palestinians continue to be deprived of their right to self-determination - a powder keg that will undoubtedly one day explode in the Israeli\underline{-}occupied territories\underline{,} just as a bus explode\underline{d} this week in Tel Aviv\underline{.}
Kevin A. Sabet\underline{,} an Obama administration u2019s former drug policy advise\underline{r}, believes that, while criminal officials are unlikely to enter into doors to confisc\underline{ate} smaller quantities of drugs\underline{,} they are likely to resist the legal, state-reg\underline{ulate}\underline{d} mar\underline{i}juana deals that will be tolerate\underline{d} under the new legislation.
He says that this is a complex issue, 'because we require them to have a defined criterion on what can be disseminat\underline{ed}, published or said, at an age when the maturity is not sufficient\underline{'}.
Correa\underline{,} who attended the 6th Summit of Presidents of the Union of South American Nations (Unasur\underline{)} held in Lima\underline{,} declared to state television in Peru that Europeans "kill\underline{ed} themselves in World War II and other conflicts\underline{"} and "now are practically a homeland\underline{.}"
The Ecuador\underline{ian} head of state took part today in Lima in the Sixth Summit of Heads of State and Government of the Union of South American Nations (Unasur\underline{),} which ended with the call for greater regional integration to ensure sustainable progress, equality and security.
On the main campus of the University of Pennsylvania\underline{,} the professor of Latin American history Matthew Restall and his colleague Amara Solar\underline{i}, a professor of art history and anthropology\underline{,} formed a team to offer a course called "The End of the World".
And in the other, the Bos\underline{ons}, a nasty gang of anarch\underline{ists} to whom nothing is sacred\underline{,} do not move this principle, which means that they can indeed be in the same place at the same time.
It is said that 77\% of Canadian\underline{s} do not have access to pal\underline{li}ative care, that is to say care to relieve the suffering of patients when they reach the final stage of their lives, both at home, in a hospital or in a nursing home.
I am interested in giving readers a behind-the-sc\underline{en}es look, a look at who the 95\underline{-}year tension (including the Bal\underline{four} declaration in November 1917\underline{)} in the small region of the Middle East is of particular benefit.
A candidate for victory in this survey may be last year's EU regulation, which, according to balloon\underline{s} on sale\underline{,} must be accompanied by an indication that children under the age of eight may not inflat\underline{e} the balloon without an adult\underline{'}s supervision\underline{.}
Win\underline{y} Maas of Rotterdam u2019s architecture firm MV\underline{R}DV, master of brilliant bar chart\underline{s} and producer of wit\underline{ty}, often cynical buildings\underline{,} took the matter with familiar ser\underline{en}ity and appeared to the contest\underline{-}hearing anno 2003 with five books under arm and a gr\underline{in}.
"Om'Oban\underline{i}" is not a simple piece\underline{,} each choir voice has a different text and one in a very foreign language: Zulu, which is spoken by eleven million people in South Africa, Bot\underline{s}wan\underline{a}, Les\underline{ot}ho, Malawi\underline{,} Mozambique and parts of Swaziland.
The judge\underline{,} Colon\underline{el} Denise Lind\underline{,} also asked Manning why he did not complain about his treatment when, in January 2011\underline{,} he met a committee to investigate the suicide ideas he mentioned a few months earlier on a form.
During Friday u2019s interview\underline{,} Manning stated that he had closed from a command of his guard that he should drop the ceiling with which he could have covered himself\underline{,} but admitted that no one had asked him to do so.
It even went so far as to pay Ukraine, Honduras and the Dominican Republic to challenge the new rules - those countries complain to the World Trade Organisation about unfair trade restrictions\underline{,} even though none of the countries trade more with Australia\underline{.}
If you try to focus on a difficult or arduous task, attention disorder can lead to bo\underline{re}dom\underline{,} Mark J. Fenske, Associate Professor of Neuro\underline{science}\underline{s} at Gu\underline{el}ph University in Ontario\underline{,} and one of the authors of the study, says\underline{.}
And unpleasant practical issues need to be clarified during this period - such as how to agree on the state requirement for "appropri\underline{ate} access" to licensed mar\underline{i}juana by banning cannabis shops within 300 metres around schools\underline{,} parks\underline{,} playground\underline{s} and childcare facilities.
Both my father and my elder brother had visited the university that I once thought was the greatest temple of knowledge in the world, a modern Greek sy\underline{m}pos\underline{ium} that promoted the great pillars of civilisation - free thought and tolerance\underline{.}
Last October, Peru hosted the Third Summit of South America - Arab States (AS\underline{PA}\underline{),} and even on that occasion\underline{,} despite the press's insist\underline{ence}, the so-called Lima Declaration\underline{,} which had been announced earlier, was not published either.
After the announcement\underline{s} by the Mexican trade unions for air transport against the former owner Gast xf3n Az\underline{c} xe1rraga Andrade, accused of fraudulent administration, did not progress for several months, the Asociaci xf3n Sind\underline{ical} de Pilot\underline{os} Avi\underline{adores} (feder\underline{al} association of pilot\underline{s}) has finally made progress.
Born on 21 September 1931 in Forth Worth (Texas), Larry Hag\underline{man} became famous worldwide for his role as John Ros\underline{s} Ewing\underline{,} better known as "J.R.
When the answer became known in a chapter in November 1990, it was seen by an average of 41 million viewers who turned "Da\underline{lla}\underline{s}" into the second most popular entertainment program since the end of "MA\underline{SH}\underline{"} in 1983\underline{,} which had 50 million viewers.
Jacques Duches\underline{n}eau\underline{,} for his part, notes that "official\underline{s} have stolen hundreds of millions of dollars\underline{",} but above all, he is concerned about the role of "mandate\underline{ers} who are aware of ta\underline{ctic}\underline{s}" when they were not involved in the fraud\underline{!}
In fact, the Bit\underline{co}in invented by Satoshi Nakamoto (a pseudo\underline{n}ym\underline{)} is both a virtual currency (but convert\underline{ible} into dollars\underline{,} euros\underline{,} etc.) and a protocol for secure exchange such as Bit\underline{Torrent}\underline{,} which allows for the direct exchange of files.
If a user wants to cheat twice very quickly (less than 10 minutes) with the same money, only one of the two transactions would be validated by the network and the other would remain unlink\underline{ed}, since both have different fingerprint\underline{s}.
By the way, the commentators found it entertaining that the only difference of opinion of the day was expressed at the time of prayer\underline{,} as some members of the body believed that the clock of the Constitu\underline{ent} Assembly was not accurate\underline{.}
Surely a law must be valid, and if something is prohibited by law, then it cannot simply be the President of the Government who is responsible for monitoring compliance with the law and hinder\underline{ing} the work of the supervisory body.
Thus\underline{,} the faceless small town rescue\underline{s}, which until now had no more to offer than a postmodern pedestrian zone and a st\underline{ub}born\underline{ly} ugly town hall behind whose white facade\underline{s} one would be inclined to suspect a dairy factory to enrich a piece of contemporary architecture\underline{.}
"But oil is not the only reason why we are so good," says Anna\underline{,} our wait\underline{ress}\underline{,} who distribute\underline{s} round tablets with rip\underline{e} Rakfisk and embo\underline{dies} the Nordic ideal with her long blo\underline{nde} hair and the st\underline{ing} blue eyes\underline{.}
On Friday\underline{,} the prosecutor tried to find out that Brad\underline{ley} Manning, an army\underline{-}lea\underline{der} accused of reveal\underline{ing} confidential information in US history, missed several opportunities to complain about the abuses he alleged\underline{ly} suffered in military detention\underline{.}
One day before the cross-exami\underline{nation}\underline{,} which was held following a defence request to deport the indic\underline{t}ment - Manning had already been punished sufficiently by the harsh detention period - Manning had said that he had considered suicide in prison\underline{.}
At the hearing on Friday\underline{,} Fein and Manning went through the forms that officials had filled out after meeting with Manning during his detention in the Qua\underline{n}tico military prison\underline{,} where he had sat from July 2010 to April 2011 under stronger conditions of detention\underline{.}
Most Americans probably never waste a single thought that the United States invaded Mexico in 1848\underline{,} forcing the country u2019s leaders to surrender more than half of their territory\underline{.}
The people who heard the hardly audible television said they felt more bo\underline{re}dom than the other two groups - they had problems concentrating\underline{,} could not find any reason for them and admitted their difficulties of bo\underline{re}dom\underline{.}
The 19-year\underline{-}old Community College student and football player Anthony Oroz\underline{co} is on trial in the south-east of Color\underline{ados} for an offence that will soon be legal in that state: possession of a few mar\underline{i}juana bro\underline{ok}s and a pipe with which he ran them.
This was recognized by the designer at the opening of "Val\underline{en}tino - Master of Cou\underline{ture}", a grandiose retro\underline{spect}\underline{ive} for which more than 130 skin cou\underline{ture} dress\underline{es} were created by his "Maison\underline{"} in the last 50 years.
"It is incomprehensible that the Inter-American Commission for Human Rights is based in Washington and funded by the United States," he said as an allusion to the political asylum granted to Ecuador to the founder of Wiki\underline{Le}\underline{ak}s, Julian Assange\underline{.}
I have just spoken to the Vice\underline{-}President of Venezuela\underline{,} Nico\underline{l} xe1s Mad\underline{uro}\underline{,} who told me that he went there for planned\underline{,} routine treatment and that he was expected to be able to travel back to Cuba after the election campaign\underline{.}
It also points out that the country has subjected itself to the principles of the United Nations Commission for International Trade\underline{,} that is to say, the rules laid down for cases of cross-border insol\underline{v}ency that guarantee equality between debtors and creditors.
Previous\underline{ly}, the Canacintra (the national chamber of manufacturing industry) managed to unite the governor\underline{s} of the south-east in order to resist the monumental institution that destroyed some of the protected areas and was the mother of all industrial threats\underline{.}
For several years, he himself has paid 3\% of the value of the contracts received in Montreal to a mediator associated with the Mafia who transferred the money to Union Montreal\underline{,} the party of Mayor G xe9ral\underline{d} Tre\underline{mb}lay\underline{.}
The government of Quebec proposes to limit donation\underline{s} to parties to \$100\underline{,} which he says would not change the situation: 'As long as campaign spending is not strictly limited, black money will be in circulation in politics\underline{'}.
The glass\underline{es} are a personal ga\underline{d}get and that is their strength (Privat\underline{es} can only see you), but at the same time their weakness\underline{,} because an enlarged reality through glass\underline{es} prevents you from working with others on virtual objects\underline{.}
As far as the authorities are concerned, the German counterpart to the NK  u2047  of the Federal Court of Auditors\underline{,} which is similar to ours and also has a college\underline{,} which is formed only slightly differently\underline{,} but in principle both authorities work similarly.
Next year we would also like to appear in the Czech House in New York, and I personally - if we are in the USA - would like to associate this with appearance\underline{s} in Washington and Chicago\underline{.}
Last week, at a Council of Ministers meeting of the member countries of the European Space Agency (ESA), Poland was accepted as the 20th member of this Space Agency\underline{,} making Poland the second member of the former Eastern bloc (after the Czech Republic, which became a member of the ESA on 12 November 2008).
Who is the cul\underline{pri}\underline{t} and who is the victim of the conflict between Palestinians and Israeli\underline{tes}, where injustice is just causing injustice in an endless spiral of violence, starting with the gre\underline{ed} of individuals and their quest for global power?
As a result, the mood levels change in the film - on the one hand, the documentary scenes from Tehra\underline{n} (in the title sequence\underline{,} icon\underline{ic} contemporary photographs are shown, and in the film version of the same situations there are no big differences either).
And while the jury was still mud\underline{d}led around and fold\underline{ed} with the axes, the naught\underline{y} Maas pile\underline{d} his exquisite bring-away\underline{s} of size into a pyramid and ended his actionist-back\underline{ed} speech with the words: "Lo\underline{ve} City Community!"
During a joint trip to Africa in spring 2005, the choir discovered the village, but above all the Imbon\underline{gi}s saw many children on the streets who lacked not only parent\underline{al} care, but simply everything: food, clothing\underline{,} education.
However, the fact that the calor\underline{ie}-rich diet of the Tal\underline{yn} is supposed to be so healthy that it loves meat\underline{,} bread and especially dairy products, many of which drink a glass of mel\underline{ted} butter every day does not seem to be particularly plausible from a nutrition\underline{al} point of view.
During Governor Pen\underline{a} Nie\underline{to}'s term of office, more than 1,000 women were murdered in the state of Mexico - a statistic that even exceed\underline{s} that of the city of Ciudad Ju\underline{are}z, which is notorious for its violence and the murder\underline{s} of innocent women.
At a manning cross-exami\underline{nation} during a pre-judic\underline{ial} hearing in Ft. Meade\underline{,} Mary\underline{land} explained that records of weekly visits by prison officers during Manning u2019s nine\underline{-}month prison term in Qua\underline{n}tico\underline{,} Virgin\underline{ia} had no complaints about his treatment.
Some people heard a loud TV from the adjacent room, which had nothing to do with the content, others heard it at low volume\underline{,} so it was hardly percept\underline{ible}\underline{,} while the third group did not hear these noise\underline{s} at all.
In 1991\underline{,} Reed Larson, a professor of human and community development at the University of Illinois\underline{,} conducted an experiment in which he contacted almost 400 teenagers and their parents seven to eight times a day with a pager.
District prosecutor\underline{s} are a "cultural barrier\underline{,}" says Sean Mc\underline{All}\underline{ister}\underline{,} a Denver lawyer who defend\underline{s} defend\underline{ants} in court for mar\underline{i}juana offences and acts locally as spoke\underline{s}person for the national organisation for the reform of mar\underline{i}juana laws.
But within two weeks of my arrival at Wor\underline{s}cester College at the end of the 1980\underline{s} - where I had intended to study history - I had packed my suit\underline{case}\underline{s} again and brought about the first scandal of my life.
At least in the last 12 years, we have had no problems with the supply of medicines\underline{,} and the problem is that people are in a far advanced state because they do not know their condition of infection\underline{,} i.e. at very late stages of the disease\underline{.}
The sooner they know whether they are HIV positive, the better, and if they already know the diagnosis\underline{,} they should learn how to live responsibly like everyone else.
Secondly, the ruling stipulat\underline{es} that, without the votes of the companies, after recognising the liabilities in the bankrupt assets that Vitro u2019s subsidiaries had with their parent company, the required majority would not have been achieved for the restructuring of liabilities\underline{.}
Indeed, 25\% of African Americans\underline{,} 15\% of people with less than \$35,000\underline{,} 18\% of citizens over 65\underline{,} and 20\% of voters between 18 and 29 do not have the required photo ID\underline{.}
As mayor of the Rivi xe8re-des-Prairies district in the east of the island, she opposed the sale of a municipal property in 2010 that was purchased for \$5 million and sold to 1.6 million developers in the boom\underline{ing} real estate market.
They have turned into profit makers by confisc\underline{ating} government land to sell it as a land for refugees from Iran and Pakistan, thereby benefiting from massive subcontract\underline{ing} by the US.
With this recourse to a hasty vote, the Egyptian people are being given an ultima\underline{tum}\underline{:} 'either vote for my draft or I retain unlimited power', the latter should supposedly end after adoption of the Constitution\underline{.}
The path starts at the Roman fort Antoni\underline{a}, Pretorium where the court was, and leads through the streets of the old town to the tomb church on Gol\underline{go}tha Mountain\underline{,} where the cru\underline{ci}fix\underline{ion}, the Salbungsstein and the tomb of Jesus are located.
"In your home country, one is promised\underline{,} and on arrival you will be cheated, you will receive your passport\underline{s} and will not receive the promised salary\underline{,}" confirm\underline{s} Tolib Schw\underline{ari}pow, head of the Department of Labour Migration of Taji\underline{k}istan\underline{.}
Perhaps it is even the case that, in this way, we only place excessive burden\underline{s} on the system, and those who seek gap\underline{s} in the system will have much easier to exploit the system than if the threshold\underline{s} remain higher.
J.F. Kennedy began issuing his own banknote\underline{s} and wanted to abolish the FED - he was murdered in 1963\underline{;} Louis Mc Fadden, MP\underline{,} was poison\underline{ed} in 1936 after he tried to sue the FED for trigger\underline{ing} the Great Depression in 1929\underline{.}
Israel was founded in 1948 and, just as the war repar\underline{ations} against Germany laid the ground for the Second World War, the procla\underline{m}ation of the State of Israel is the creation of the focal point for the Third World War.
If international bankers succeed in unleash\underline{ing} this war, the Jewish people will become victims in the front line, this time along with the Arab or Muslim population of the Middle East, in the same way as in World War II.
There was no positive way out of this situation for the American Government - it could not afford to drop the Sha\underline{h}, as this would have severely damaged the confidence of its allies in other countries.
"This is the idea that the EU's recent plan to introduce a 40\% female rate in the management of large European companies," said Patri\underline{k} Nacher, who is responsible for organising this survey\underline{,} to the newspaper Pr xe1vo.
And although we may now live the American dream\underline{,} have visited good schools\underline{,} and have received good jobs, we must never lose sight of the fact that it is the American dream we are living - not the Mexican dream\underline{.}
With such scale\underline{s}, researchers have found that boys become more bo\underline{ring} than girls\underline{,} according to Stephen Vo\underline{da}nov\underline{ich}, Professor of Psycho\underline{logy} at the University of Westflo\underline{r}ida - especially as regards the need for more and a greater variety of external stimuli\underline{.}
It then sell\underline{s} this for 10,000 rupees (83 Eurocent\underline{s}) to the petrochemical industry, because this mineral is widely used in everyday life and is used for the production of match woods\underline{,} fire\underline{work}\underline{s}, cosmetic\underline{s}, dyn\underline{ami}\underline{te} and even for ble\underline{ach}ing sugar\underline{.}
He is able to carry up to 110 kg and assure\underline{s} that he will continue "as long as it goes" because he needs the money to raise his three children aged between 10 and 18.
"The free movement of citizens and workers in all South American countries must be achieved, as is already the case in the Andean Community; however, there are still reaction\underline{ary} sectors seeking a return to the past," he warned\underline{.}
Then came the 1990 World Cup\underline{,} where we ranked fourth\underline{,} which should have been bronze had it not been this Canadian referee who had us repeat the last move for the second time, said Rey\underline{es}.
In addition, these laws also reduce the periods for early voting, declare invalid the right to register as a voter on the day of the election and deny the right to vote for citizens for whom a court file has been submitted.
Finally, this is the last particle whose existence has been predicted by the standard model - our best or least false explanation of nature and the behavior of matter - but not yet empirical\underline{ly} observed\underline{.}
However, the Hi\underline{gg}\underline{s} field is much more stable than the electromagnetic field; the pathogen must reach very high energies\underline{,} a bit like a frozen pond whose surface could only be sh\underline{atter}\underline{ed} by a very large rock\underline{.}
Mr Za\underline{mb}ito played his hand everywhere in the 2000s by giving more than 88,000 Canadian dollars (about EUR 68,000\underline{)} to provincial parties, especially to the Liberal\underline{s} who were in power at the time.
From the investigation that is ultimately carried out, it says that it draws 'on a thread that makes it possible to understand the functioning of the system that ants infilt\underline{rate}, in order to stop the evil and denounce the cul\underline{pri}\underline{ts}'.
In order for farmers to free themselves from the insurg\underline{ency} led by foreign groups, which they say is their wish, it would be necessary to continue with low, well-controlled civilian aid which directly affects them in their favour.
In the city you usually get by bus, but in Jerusalem there is also a highway and in Hai\underline{fa} the only subway line in the country with six stations connecting the Lower City to the Upper City.
Nevertheless\underline{,} many citizens of the Central Asian republic\underline{s} who want to make their money in Russia admit that not only do they not speak the language of the target country, but they can hardly express themselves in writing in their own language.
In recent days there have been massive protests across the US against low wages at Wal\underline{mar}t stores and restaurants of popular fast-food chain\underline{s} such as Mc Donald\underline{'}s, Burg\underline{er} King\underline{,} Taco Bell\underline{,} Wendy's and Kentuck\underline{y} Fried Chi\underline{cken}.
Under the previous rules, the persons under examination are already accountable to the agency (for example, in the case of an operational programme of regional policy, the Regional Council) so that any failure to comply with the procurement law amounts to a violation of budgetary discipline\underline{.}
Another stage of development should already be able to do real scientific work - the RM\underline{-}34 rocket should reach an altitude of up to 14.\underline{5} km and be used to observe high-altitude wind\underline{s}.
On a large scale\underline{,} this means that most companies move their production abroad\underline{,} buy cheap\underline{ly} or abandon their business, resulting in high unemployment in countries with comparable labour costs.
The only solution is targeted political and social reforms that increase the state's share of capital in the economy, increase citizens' influence on the government and weaken the monopoly of private capital in society for the benefit of the state.
What is less obvious is whether it really was always these personalities who determined their actions autonomous\underline{ly}, or whether there was someone behind their thro\underline{ne} who directed their actions towards a predetermin\underline{ed} goal.
Israel is like a huge lab\underline{,} a source of conflict and chaos\underline{,} not only in the country itself, but also internationally (remember how sharply people divide into Israel u2019s followers and opponents\underline{).}
Regulation\underline{s} may well become the target of criticism in the Member States, but, in the opinion of some experts\underline{,} the EU's efforts to regulate and thus also to improve the effectiveness and development of the entire European Union deserve more recognition\underline{.}
After a six-year struggle with Germany and Austria, the Czech Republic was able to defend the name "Olomouck xe9 tv\underline{ar}  u2047 ky\underline{",} the inlandrum (Tuz\underline{em}sk  u2047  rum\underline{),} whose tradition goes back to the 19th century, but our manufacturers had to rename it "Tuz\underline{em} xe1k".
Pen\underline{a} Nie\underline{to} was also keen to talk about the growth of the Mexican economy, which is one reason that Mexican\underline{s} are just as likely to remain in Mexico today, rather than emigr\underline{ating} to the United States.
Among these projects, there are five Peru\underline{via}\underline{n}s lying on the cross-ax\underline{is} of their territory from the coast to Brazil\underline{,} two of which are supposed to provide a better link with Ecuador\underline{,} although it did not provide any further details.
As part of the summit, the bloc\underline{'}s defence ministers also met in advance to adopt the action plan for 2013\underline{,} in order to strengthen dialogue and consensus on the defence of the region.
The President of Ecuador also advocated the reorganiz\underline{ation} of the Organization of American States (OEA\underline{),} with the aim of reducing the influence of the Anglo\underline{-}Saxon states and taking into account those who signed the San Jos xe9 Convention on Human Rights.
However, there are still many people in the clinic who do not know anything about their illness\underline{,} who have already caused damage and have exhaust\underline{ed} their immune system, and who are victims of opportun\underline{istic} infection\underline{s}.
Subsequently\underline{,} the Supervisor\underline{y} Authority has systematically refused to inform the Republic u2019s Chief Administration of a transaction carried out by the entrepreneur in order to withdraw 198 million pesos from the trustee account F/5\underline{89} of Bank IXE.
With players like "Can\underline{ito}\underline{"} Nie\underline{ves}\underline{,} Pablo Ali\underline{cea} and the young Roland\underline{o} Hour\underline{ru}iti\underline{ner} as a replacement for the locked players due to the events at the Pan American Games in Mar del Pla\underline{ta}, we won the gold medal against any forecast\underline{.}
Instead\underline{,} you can choose between different dishes with hammock and beef\underline{,} soups and desserts (prepared with coconut milk\underline{),} traditional Jewish hum\underline{us} paste, various sauce\underline{s}, fried ball\underline{s} made of pure beans and peas (fal\underline{con}) as well as fruits and vegetables\underline{.}
On that day, some Wal\underline{mar}t workers, 2.2 million of whom are worldwide, laid down their jobs and, together with unions and left-wing activists\underline{,} set up chain stores targeting low- and middle\underline{-}income individuals\underline{.}
On the select list already high-rank\underline{ing} representatives of the Petersburg art scene\underline{,} whose successes go beyond the borders of the city and often find recognition in Europe without being known in the rest of Russia.
It is precisely this kind of joint control that could help us to stop constantly trying to improve the legislation and to reduce and balance threshold\underline{s} if this does not seem to have a particularly positive effect.
The competences are also to some extent comparable\underline{,} but Germany is a federal state, i.e. that these courts of auditor\underline{s} also exist in the individual federal states - that is where the German system differ\underline{s} from ours.
With our band The Tap we make fun of it and say that we are the only band in the world that can gather enough positive energy to stop or prevent the end of the world.
Some come to us with romantic ideas, and when they discover that they have to rehearse twice a week, have to complete preparato\underline{ry} phase\underline{s} and spend a lot of time on concert trips\underline{,} the enthusiasm of many quickly disappear\underline{s}.
In 1937\underline{,} the design of a photoelectric hunting rocket\underline{,} originating from Ing. Roh\underline{o}zi  u2047 ski, appeared in the trade press, and the following year the work "Raki\underline{eta} - torped\underline{a} powietr\underline{z}na i ra\underline{kie}\underline{to}bomb\underline{a} lotnic\underline{za}" by the author Leliwa-Krzy\underline{wo}\underline{block}\underline{y} appeared\underline{.}
Already in its early days in 1956\underline{,} the Polish space company PTA tried to join the International Federation for Space\underline{,} founded in 1951\underline{,} and in fact PTA became a regular member in the autumn of 1956\underline{.}
My thoughts are based partly on accessible historical facts\underline{;} others are derived from them and, from my own understanding, are based on who or which group of people have a significant influence on the events of modern history.
Among these astronom\underline{ical} rich families, one stands out, which could be called the head of the oc\underline{top}\underline{us} (I do not know if anyone is above them, but I do not rule out this) - the Roth\underline{schild}\underline{s}.
The method by which the group of richest families works with the Roth\underline{schild}\underline{s} at the top is to trigger a crisis and then offer a solution (order from cha\underline{o} - order out of chaos\underline{).}
Grant\underline{s} for applications for funding were offered to the municipalities by the Ministry of Regional Development under the direction of Minister Pavel N  u2047 mec (US-DEU), and specifically by means of funding applications to Brussels\underline{.}
In the opinion of these experts\underline{,} a more serious problem is EU funding for projects which have absolutely nothing in common with the deepening of European integration, but which were imposed by individual Member States during the budgetary negotiations.
So as soon as a US government official makes even the slightest criticism of Mexico\underline{,} complaints are heard - in the Mexican press and among the country's elite\underline{s} - about how Americans are pushing the sovereignty of their neighbor\underline{ing} country.
A number of Australian laws have banned tobacco companies from TV advertising\underline{,} banned them from acting as sports sponsor\underline{s}, and forced most dealers to stop using cigarette\underline{s} in shops\underline{.}
After the mar\underline{i}juana police officer found in the car, Oroz\underline{co} was summ\underline{on}ed for possession of drugs and drug uten\underline{s}ils - caval\underline{ier} offence\underline{,} each with a fine of USD 100 - and received a court appointment\underline{.}
In Washington\underline{,} it is believed that Color\underline{ado} is in any case ahead of most states in terms of the regulation of mar\underline{i}juana, where the drug was legalised first for medical purposes and then for self-consumption\underline{.}
"No\underline{where} will it be harder to find a location for a licensed cannabis business than in urban areas, especially in the Seattle metropolitan area," says Ben Living\underline{s}ton, spoke\underline{s}person for the "Center for Legal Cannabis\underline{",} a recently formed research group.
Although 55\% of voters in Color\underline{ado} supported the measure, it was clear from the outset that it would not be easy to reconcile the personal consumption of mar\underline{i}juana with the complexity of government and legal systems.
While advocate\underline{s} and state officials are preparing for an age of legal sales, they are also nervous\underline{ly} awaiting orders from the Federal Government, which wants to continue treating the sale and cultivation of mar\underline{i}juana at the federal level as a criminal offence\underline{.}
The 27-year\underline{-}old Anto has been jeopardising his life at Kawah Ijen for three years, whose sulphur has already left his first trace\underline{s} in his face, even though he covers his face with a mask and special glass\underline{es}.
After that, the Peru\underline{via}\underline{n} Presidency sent an e-mail to the media with the "concl\underline{us}ive declaration\underline{"} of the summit, but it was the Hum\underline{ala} Declaration and not the official document to conclude the summit.
"Si\underline{nce} he has been in our embassy\underline{,} I have not spoken to him, but the ambassador has informed me that he has a slight problem with the lungs, but no serious problem," said the head of state of Ecuador\underline{.}
"The solution to this problem is in the hands of the United Kingdom\underline{,} Sweden and the European legal authorities because the lawyer of Assange\underline{,} Bal\underline{t}azar Gar\underline{z} xf3n, conduct\underline{s} a series of proceedings in various European bodies\underline{,}" he said.
Correa took the opportunity to confirm himself as a defend\underline{er} of the freedom of the press and said that what he does not tolerate is 'the medio\underline{crit}\underline{y}, the evil intention and the lie that deny freedom of expression\underline{'}.
In Jalis\underline{co} alone, 255 people died in 2011\underline{,} and by May this year there are already 187 deaths\underline{,} but it is assured that universal access to antiretrovir\underline{al} medicines has been available since 2005.
As you know, we are talking about a huge sales and distribution centre in Mexico\underline{,} Central America and the Caribbean with products from the country beyond the Wall\underline{,} complement\underline{ed} by a living area for the staff of 150 companies.
The most emotional memories are those that recall his time at the Va\underline{quer}\underline{os} from the mid\underline{-19}\underline{50}s as a player until 1982\underline{,} when he celebrated his 15th anniversary as the club u2019s managing director or CEO\underline{.}
But my favorite is the team of the pan\underline{-}American matches in Cuba in 1991\underline{,} where we won gold and offered a fight to the US team, as when they won bronze against us in the World Cup\underline{.}
The slogan "Who shot on J.R.?", which was supposed to create expectation for an episode full of emotions\underline{,} where the figure of Hag\underline{mann} was almost killed\underline{,} led to international speculation\underline{,} and millions of dollars were wage\underline{red} in betting houses\underline{.}
A manifest\underline{o} has been circulating since October, signed by prominent Pal\underline{li}ative-care figures\underline{,} such as Dr Bal\underline{four} Mount and Dr Bernard Lapoint\underline{e}, to express their opposition to such an initiative.
Every day, road building officials\underline{,} major construction companies, political party money creator\underline{s} and Italian mafia specialists tell us what they know about a great 'system' in which construction, civil servant\underline{s}, politicians\underline{,} trade union\underline{ists} and Mafioso are involved.
The Chinese have already almost left Mes Ay\underline{n}ak u2019s copper mine\underline{,} leaving international arch\underline{a}eologist\underline{s} (finance\underline{d} by the World Bank) to excavat\underline{e} the vast Buddhist site, and remaining the province u2019s most important employers\underline{.}
Most lawyers who have worked on this text are not Ul\underline{e}ma, but academic\underline{s} who have been trained in part in the French system," notes Alex\underline{is} Blo\underline{ue}t, who write\underline{s} a doctor\underline{al} thesis on Egypt\underline{'}s constitutional transition\underline{.}
From January to October 2012\underline{,} 118\underline{.}8 thousand Ukrainian tourists entered the promised country, an increase of 51\% over the same period in 2010, before the visa waiver on 9 February 2011\underline{.}
"The police are, of course, aware of everything and therefore, if they cannot keep to the crime detection plan, they periodically carry out checks on dealers who offer illegal weapons\underline{,}" adds the sales advisor\underline{.}
The protests continued this week in New York, where their goal was not Wal\underline{mar}t stores (which are not desirable in this progressive city and therefore not yet present), but McDonald\underline{'}s and other inexpensive restaurants.
Not only do we want to collect enough positive energy to prevent the end of the world, but we also want to consider, together with the public, the state in which we hand this world over to our children.
The global lust for power of the Roth\underline{schild} led in the years 1859 - 1871 to the formulation of a plan to unleash three world wars by Albert Pik, a freemason of the 33\underline{rd} and thus the highest degree of knowledge.
At the end of the 19th century, the Roth\underline{schild}\underline{s} initiated the founding of the Zion\underline{ist} movement, in which a branch sought to establish a Jewish state, preferably in the historical area of Jud\underline{a}ea with Jerusalem as capital (return to Zion\underline{).}
Affleck\underline{'}s film lose\underline{s} a bit of traction\underline{,} it is a film that you can follow with a certain interest, while enjoying the design and retro style reminiscent of a thrill\underline{er} from the 70s.
The organise\underline{rs} of the survey were also impressed by the idea that certain countries should receive money for not having a sea, or the idea of providing funding for applications for funding.
This suggests at least one new article\underline{:} in all matters relating to Sha\underline{ria} law, it is necessary to consult al-Ashar University, the country u2019s most important Islamic institution with great vig\underline{our} throughout Sunni Islam\underline{.}
Even on better days, this is a city that is always clo\underline{gged}\underline{,} but on Monday a ring of steel was built that blocked several important traffic routes into the capital and caused chaos on the streets\underline{.}
Manning said on Thursday about his arrest and transfer to Kuwait\underline{,} where he was held nearly two months before being transferred to the Qua\underline{n}tico naval base in Virgin\underline{ia} in July 2010.
Although several Hamas leaders are killed and the 1.7 million inhabitants of Gaza are being pl\underline{ough}\underline{ed} into one of the most desolate and densely populated corner\underline{s} of the planet\underline{,} Israel has so far failed to destroy Hamas\underline{.}
And, in particular, the rise of the Muslim Brot\underline{her}hood under President Muhammad Mor\underline{si} in Egypt - the most pop\underline{ul}ous and important Arab country by far - on Israel's southern flank has profound\underline{ly} changed the region's balance.
Cava\underline{lier}\underline{e} di Gran Cro\underline{ce} (the highest award in Italy), Cava\underline{lier}\underline{e} del Lavoro, Command\underline{eur} de L'Or\underline{dre} des Arts et des Lettres, awarded with the Legion of Honour\underline{,} Gar\underline{ava}\underline{ni} cum\underline{ulate}\underline{s} as many honor\underline{s} as any of the husband\underline{s} of his customers.
Even if these new rules could pave the way for an increase in the national birth rate, talks with the Singapore\underline{ans} working in the financial district suggest that they will not have much effect.
The Sixth Summit of Presidents of the Union of South American Nations (Unasur\underline{)} ended today in Peru without the publication of the Lima Declaration\underline{,} which was announced earlier and was theoretical\underline{ly} to be signed by the seven governor\underline{s} present.
Simpl\underline{y} put, the above statements mean that anyone who receives HIV\underline{-}positive diagnosis at the age of 25 can, in this sense, become "problem\underline{atic} 75 years of age as long as he is under control," said this expert\underline{.}
A team that was perhaps not the best in terms of personalities, but with which we won a gold medal and which gave us great pleasure\underline{,} was that of the pre-Olympic tournament in 1995 in Neuqu xe9n, Argentina\underline{.}
Hag\underline{man}, who returned this year as J.R. in a new season of "Da\underline{lla}\underline{s}", died Friday afternoon due to cancer complications according to a family press release to The Associate\underline{d} Press by Warn\underline{er} Bro\underline{s}., producer of "Da\underline{lla}\underline{s}".
Hag\underline{man} interpreted the role of Ewing as a corrupt\underline{,} insati\underline{able} man with a charisma\underline{tic} smile\underline{:} a deceitful businessman and unfaithful husband who sought to have his alcoholic wife\underline{,} Sue Ellen (Li\underline{n}da Gra\underline{y}).
Moreover, this appears to be confirmed by new data presented this week at a major physics conference in Kyoto\underline{,} but there is still a lack of data to be absolutely sure about this.
If a particle accelerate\underline{s} or changes direction with an electric charge, the electromagnetic field is "dis\underline{tur}\underline{bed}\underline{"} in this very place, roughly like a pebble thrown into a pond\underline{.}
"They gave me five years to live, I managed seven years," he said half-heartedly lying in his bed in the home for pal\underline{li}ative care Victor\underline{-}Ga\underline{db}\underline{ois} in Beloeil, where he arrived the previous day.
Dr. Martel believes that 90\% of patients who have asked to die thank the nursing staff for not accepting this desire after their pain has been relieve\underline{d} by a team of pal\underline{li}ative care.
All of the examination centres will be under the aeg\underline{is} of the Push\underline{kin} Institute for the Russian Language\underline{,} the Russian University of the People's Conscious\underline{ness}, the Moscow State University, St. Petersburg State University and other Russian universities\underline{.}
"The problem is that the chic\underline{k} must stop; it must be able to stand on its leg\underline{s} and begin to move," explains RAN\underline{'}s Labor\underline{atory} Director\underline{,} Vladimir Sy\underline{che}w.
"Two times we let chic\underline{ks} slip and then put it in, because it is simply impossible to work with them there," Vladimir Sy\underline{che}w notes as a failed experiment with chic\underline{ks} in space.
Generally speaking\underline{,} I would not like to compare this with any specific information, but Germany is, in a sense, often described as a model, although it certainly cannot be said that Germany is better in all.
On some roads in eastern Bohemia there is danger because of ice\underline{-}smoothness, higher altitude\underline{s} and in the mountains there is sometimes still a snow layer on the roads\underline{,} informs the road and motorway director\underline{s} on their internet pages.
However, it is not exactly custom\underline{ary} for a large group of disabled people to actively participate in social events there, in which we are a little ahead of the West with the band The Tap\underline{!}
The First World War ended with the sudden\underline{,} militari\underline{ly} and economically unfounded cap\underline{it}ulation of Germany (the war was no longer necessary for the destruction of the Russian empire\underline{),} followed by the dissolut\underline{ion} of the Central European great power of Austria-Hungary.
Emotion\underline{s} also give rise to the fact that the Czech Republic, like other Member States in Brussels\underline{,} has to fight for the right to use specific designations of traditional products and does not always win this battle\underline{.}
Some of them have taken up to 14 orphan\underline{s}, give them a roof over their heads and ensure that the children appear in their uniform\underline{s} on time for school lessons every day.
The hotel in which I stay is one of several venue\underline{s} that organize a Rakfisk dinner where guests can vote for the best - or perhaps the most challenging - fish.
To reach the city, one can drive on one of the highway\underline{s} that built Pen\underline{a} Nie\underline{to}, which represents a great improvement over the sha\underline{ky}\underline{,} bu\underline{mp}y roads that once existed here.
When Fein asked him about the forms on Friday\underline{,} Manning admitted that he had judged the treatment by his guard\underline{s} as "excell\underline{ent}" and the treatment by the institution as a whole as "very professional".
On Thursday\underline{,} Manning had said that he was forced to sleep naked the night before, trying to show an official that he did not pose a threat to himself\underline{.}
His lawyers hope that the judge will at least take into account his detention experience and drastically reduce his detention if he is convicted in his trial before the military court\underline{,} which is scheduled for early next year.
The question must be asked: is this just a private person who likes Marlb\underline{oro} cigarette\underline{s} so much that she even takes a video for it - or does a marketing agency have to do with it?
They are waiting for guidance on establishing a licensing system for the production, production, distribution and sale of the drug - with a deadline of 1 December 2013 in mind.
The Washington Act\underline{,} known as I-5\underline{02}, enters into force on 6 December, thus forming the final point of a grey zone in which the state licensing system does not yet exist but the property is legalized.
Organiz\underline{ed} and growing hatred of Oxford\underline{-}based Tory students has now developed to such an extent that a group of them last week called for equal protection of equality for the benefit of gay\underline{s}, disabled people and ethnic minorities\underline{.}
He divide\underline{s} a dirty wooden hut with other carriers and is standing up every morning at two o'clock\underline{,} because the sulphur also flows out at night, where its characteristic yellow colour shine\underline{s} blu\underline{ish} in the dark\underline{ness}.
Every day he and his companion\underline{s} break 15 tons of sulphur from the volcano\underline{,} which are transported by three truck\underline{s} over a goat path between the bush and the camp in Tam\underline{ans}\underline{ari} 18 kilometres away.
In Singapore\underline{,} there are websites where the bare\underline{ly} disguise\underline{d} xenophobia against many new immigrants is flourish\underline{ing}, especially against the Chinese, who are criticize\underline{d} for keeping wages low and not integrating\underline{.}
He proposed reorient\underline{ing} this inefficient distribution; the condom\underline{s} should be located not only behind the counter\underline{,} but in the public toilet\underline{s} of facilities often visited by young people.
"Our first project dealt with the prop\underline{he}cy of the Maya\underline{s}, and in a certain way we discredit them," said Julie Ze\underline{gl}\underline{en}, student last year in Temple\underline{,} 21 years old and from West Che\underline{ster}.
He notes\underline{,} however, that there is an apocalyptic fear in Western society, which leads back several centuries when people responded to changes in their environment by predict\underline{ing} the end of the world.
Let us assume\underline{,} however, that this is actually the Hi\underline{gg}\underline{s}, because there seems to be only a small risk of deceiving oneself\underline{,} and let us look at what is at stake\underline{.}
It has to be said that the latter still has major flaws\underline{,} as it does not explain the gravity (ups!) and the dark matter that makes up about 80\% of the matter of the universe (renew\underline{ed} ups!).
"Si\underline{nce} the start of the investigation in 2010,\underline{"} he emphasize\underline{s}, "the Ministry of Transport alone saved \$1 billion in contracts\underline{,}" because some narrow\underline{ed} their instinct\underline{s} to retain their share!
The new cooperation agreement provides for the continuation of traditional aid: girls\underline{'} and boys\underline{'} schools\underline{,} the French Institute of Universit\underline{ies}, the French Institute\underline{,} cooperation in the military, legal, medical and agricultural fields, support for the archaeological delegation\underline{.}
Stephen Bet\underline{ish}es developed in our laboratory in Redmond a touch sensor with a regul\underline{able} processing delay of between 1 and 100 mill\underline{i}second\underline{s}, whereas today's commercial sensors are closer to the second value (60 to 100).
Recently\underline{,} he snap\underline{ped} a barrel organ and became a Petersburg\underline{or}gel player because he finally felt ready for this difficult role in terms of his artistic existence\underline{,} philosophy and image.
There is a connection between the fact that a child is in the mother\underline{'}s abdom\underline{en} in fruit water for about 9 months and the fact that it is easier to get used to water.
On the occasion of the end of the Maya\underline{n} calendar\underline{,} we also developed a unique collection of shoes\underline{,} t-shirt\underline{s}, bags and key ring\underline{s} against the end of the world, with which people can also support us through www.e-tap.cz\underline{.}
As the German economy becomes more competitive, there are regular cases where workers receive such low wages that the state must increase its income to the minimum level of subsistence.
Abraham Lincoln refused to renew Roth\underline{schild}\underline{'}s Bank of America's status as a central bank, began issuing his own (that is, state) banknote\underline{s} during the civil war, and was murdered in a theatre in 1865\underline{.}
For their release, they demanded the extradition of the fallen Sha\underline{h} Moham\underline{mad} Reza Pahl\underline{avi}\underline{,} who had fled to the US after the revolution\underline{,} who had maintained the patron\underline{age} of his regime for decades\underline{.}
Alan Arkin and John Good\underline{man} are very charming in their roles as Hollywood employees, but their characters deserve more space, and they are far from alone in the film.
However, it is sufficient to commemorat\underline{e} a piece of history that is still alive in some way to this day and to prove how exaggerate\underline{d} the notion\underline{s} of the om\underline{ni}pot\underline{ent} and om\underline{nis}\underline{ci}ent intelligence services are.
As I am more than 40, independently and impartial\underline{ly}, I have no other way of influ\underline{en}cing things than to stand for the office of a senator or president\underline{.}
But Pat\underline{t}loch u2019s cases are different: on behalf of his clients, he oppose\underline{s} Chinese companies being officially authorized by the Trade\underline{mark} Office to use a designation that is already protected elsewhere\underline{.}
If you don't have anyone any more, you will come to the shelter of Khan\underline{y}isile, a single woman who is just as well paid by the club as the two cook\underline{s} who cook every day for more than 200 hungry children.
A bus full of whites singing songs in a black language - not only does it bring mood and joy\underline{,} but it has also wrough\underline{t} tear\underline{s} to some fierce border soldiers\underline{.}
Under Felipe Cal\underline{der}on u2019s outgoing government, Mexico has been able to prove itself economically well, but it is under the grip of a drug war that has already cost 60, 000 lives in the last six years.
Even if the Islamist\underline{s} now in power in Egypt and other countries have little left for Israel, they will focus first on domestic difficulties\underline{.}
The right answer is that represented by the more sensible representatives of both sides\underline{,} the majority of the rest of the world, and by this newspaper\underline{:} two states where Israel surrender\underline{s} territories for security purposes.
But Professor Eastwood believes that although these two conditions may be related, bo\underline{red} people see the problem in their surroundings or in the world, while depressive people see the problem in themselves.
On the scale are statements like "Man\underline{y} things I have to do repeat themselves and are mono\underline{ton}ous" and "I have so many interests that I do not have enough time for everything".
So if you are able to give your bo\underline{red} child an iPad, you can stop the bo\underline{re}dom\underline{,} but it has not learned to talk or control yourself, says Professor Fenske.
"We were all delighted when we were invited to his house in Gstaad," explains the ex-wi\underline{fe} of "He\underline{ini}" Thyssen\underline{,} who is close friends with forgotten beauties such as Marella Ag\underline{n}elli or Eugen\underline{ie} Ni\underline{arch}\underline{os}.
The company is PT Candi Ngri\underline{m}bi, which since 1960 exploit\underline{s} the deposit\underline{s} in the volcano and (near\underline{ly}) its workers, to whom it pays 662 Indonesia\underline{n} rupees (5 Euro cent\underline{s}) for each kilo of sulphur\underline{.}
It seems incredible that the vers\underline{es} are part of an advertisement for Min\underline{z}bon\underline{s}, but nevertheless - or precisely because of that - they became a viral video on YouTube in Singapore earlier this year.
He admit\underline{s}, however, that the new standards give the developers clearer orientation\underline{s}, which were previously obstruct\underline{ed} when they wanted to build too many small units within a project.
Marie\underline{los} Por\underline{ras}\underline{,} a teacher of English with a university degree in education and learning\underline{,} believes that in order to orient\underline{ate} children and young people, it must be understood that the purpose of social networks is to inform them.
The Head of State read the final document, which stated that 16 decisions were taken and that the lines of action were laid down for 31 projects between South American countries, totalling \$17 billion in investment.
With the crisis in Europe, "economic consolidation (in Latin America) must not take on a triumph\underline{ant} character, but should serve to expand our output and show our peoples a better future," added Hum\underline{ala}\underline{.}
I still know that Gene Bartow, who worked here as a trainer and employed me at the University of Alabama (Bi\underline{rm}\underline{ing}ham\underline{),} said: "I have a very strong and 2 m big player.
In Pen\underline{n} State, the final exam will be held on the eve of the Apocalyp\underline{se}, which is why students have no option but to continue working until the night when the world is supposed to end," said Restall\underline{.}
Joseph Dough\underline{er}ty, a professor of religion at the University of La Salle\underline{,} who teach\underline{es} in the Philippines this year, quickly answers the question whether he would know a course there about the "end of the world".
A 2011 report by the Brenn\underline{an} Center shows that those states that passed these laws account for 171 of the 270 votes required in the Elector\underline{al} College to win the presidency\underline{.}
By the way, there are many phy\underline{s}icists who fer\underline{vent}\underline{ly} hope that such deviation\underline{s} will be found, because the slightest difference could open a door to a "new physics\underline{"} and fill some holes in the model.
It is precisely this great inadequacy in Quebec\underline{'}s health care system that is causing concern to several doctors who specialize in pal\underline{li}ative care who are awaiting the adoption of a law regulating eu\underline{than}\underline{asia} and assisted suicide\underline{.}
Bit\underline{co}in differ\underline{s} from other types of virtual currencies such as the "credit\underline{s}" used to advance in a video game that can be won or bought (and sometimes exchanged) by playing\underline{.}
"The vulnerability does not affect the protocol itself," said Pierre Noiza\underline{t}, who has just introduced Pay\underline{m}ium, which is a real money payment company and uses Bit\underline{co}in network.
The Sala\underline{f}ist parties, for which the establishment of Islamic law is an important demand, hoped to replace 'the principles' with 'the rules', which would have made it possible to apply them more strictly\underline{.}
Gali\underline{lee} is the place where Jesus performed his miracle\underline{s}: the transformation of water into wine at a wedding ceremony\underline{,} walking on the water, the sta\underline{in}ing of the storm and fishing.
According to the Ministry of the Interior statistics\underline{,} 142 crimes involving the use of registered weapons were committed over six months in 2012\underline{,} while a total of 1.1\underline{68} thousand offences were recorded for the same period.
There are dealers on the markets, but there you have to go there and agree with a code like "by Ivan Ivan\underline{ovi}\underline{ch}, who tells them that the daughter has lost a tooth".
In conversation with the head of the group for interactive 3D technologies in the Microsoft Lab in Cambridge Sha\underline{h}ram Izadi, however, it is clear that for the company u2019s scientists\underline{,} glass\underline{es} were only a transit station.
Simpl\underline{y} put, it is a question of the European legislative authority laying down how public contracts are to be dealt with, on which the national legislations are based, and, finally, the actual practical application.
After Madrid\underline{,} Luxembourg\underline{,} London and other cities where everything works better than us, we have just seen in Russia that everything is still in its early stages in the East.
Respect for the public and accessibility is one thing, but only when important sportsmen, artists\underline{,} actors\underline{,} politicians or lawyers come from our rank\underline{s} will things really start to change.
Poland also participated in space research with Soviet satellite\underline{s} as part of the Intercos\underline{mos} programme, and in 1978 the Polish pilot Mir\underline{os}law Hermas\underline{ze}wski became second intercos\underline{mon}aut after the Czech Vlad\underline{im} xedr Remek.
In what light do the words of David Rock\underline{ef}\underline{eller} in 1994 appear: 'The only thing we need is an all-round crisis and people will welcome the new world order'.
The standards on fruit and vegetables have already been relaxed by the EU, despite opposition from some countries, on the grounds that the previous directives would lead to a waste of food.
As President, it would not be a problem for me to call on the chair\underline{men} of parliamentary parties live on television to enshrine the substantive and criminal liability of politicians\underline{,} officials\underline{,} judges and prosecutor\underline{s}.
For almost ten years, the choir has been performing songs in this foreign soft language, and occasionally bringing them back to where they originally came from: to the south of Africa.
In the constell\underline{ation} of ser\underline{pen}\underline{t} carriers\underline{,} astronomer\underline{s} have photograph\underline{ed} the forerunner\underline{s} of a cosmic caroblage: 400 million light years away from Earth\underline{,} the core\underline{s} of two merge\underline{d} galaxies colli\underline{de} inevitably\underline{.}
When the dark\underline{ness} comes over the country and the weather gets cold\underline{er} in Norway\underline{,} Norwegian\underline{s} flock to a party here in Fagernes dedicated to this very speciality, now.
"You eat it raw and then rin\underline{se} it with a glass of Aqua\underline{vit}\underline{",} says Havar\underline{d} Hal\underline{var}\underline{s}en, who actually works in the local fire station, but as a so-called "Rakfisk general" also organize\underline{s} the festival\underline{.}
Manning replied that he had expressed his concerns orally and that the officials had discussed them with him and indicated that they were dealing with them, but they had not been recorded\underline{.}
"I wanted to convince employees that I was doing well and get rid of the observation status for the prevention of injuries (...) in order to achieve what I see as a better quality of life," said Manning.
When he moved to Qua\underline{n}tico\underline{,} Manning spent most of his days in a small cell - at least 21 hours and often more than 23 hours - and without society.
"If you market tobacco and only have a small area to advertise your products, you won't get around the Internet," says Beck\underline{y} Freeman, a health researcher at the University of Sydney\underline{.}
But Peter Toohey, professor of Greek and Roman history at the University of Cal\underline{g}ary, Canada\underline{,} and author of "Bore\underline{dom}\underline{:} A Live\underline{ly} History\underline{"} (Yale University Press\underline{,} 2011\underline{)} does not see this.
Sometimes not, because in extreme cases it leads to people taking extreme physical risks and falling into gambling or drugs in order to alleviate them - studies have shown this.
According to the journalist Suzy Men\underline{kes}\underline{,} the supreme authority of the specialist press, this dress was a milestone in the Haut\underline{e} Cou\underline{ture} at the end of the 20th century, "the return to the customers of the top society".
This is the case with Anto Wijaya, one of the 400 mine\underline{work}\underline{ers} who earn their lives by bringing sulphur from the Kawah Ijen volcano in the east of the Indonesia\underline{n} island of Java\underline{.}
Despite its huge profits\underline{,} the mining company has not mechan\underline{ised} the extraction of sulphur in order to save costs and does not supply any equipment to the carriers who work on their own account and are paid for by weight\underline{.}
The sentence\underline{s} are part of a ra\underline{pper} song\underline{,} the local sayings such as "Shift will be a "bao" (mor\underline{ning}) in the oven to make fun of the low birth rate in Singapore\underline{.}
Por\underline{ras} explains that the academic Marc Prensky\underline{,} holder of a master\underline{'}s title in ped\underline{ago}\underline{gy} at Ya\underline{le} University and author of the work Digital Natives and Immigrant\underline{s}, formed these terms to explain the phenomenon\underline{.}
The only document circulate\underline{d} during the day was the list of participating president\underline{s}, causing disquiet among the hundreds of journalists from various national and international media who demanded more information.
And when Sweden interrog\underline{ated} Mr Assange at the Embassy of Ecuador in London or via Skype\underline{,} as Swedish law allows and has been done in other cases, the problem is resolved\underline{.}
Construct\underline{ed} from NY\underline{CE}\underline{,} e-Qu xe1lity and Kernet, leading information technology companies, a group of companies was founded under the name of Comp\underline{et}ival\underline{,} the aim of which is the service market of software cluster\underline{s} in Central and South America.
There he played the astron\underline{aut} Tony Nelson\underline{,} whose life is turned upside down when he meets an attractive "ji\underline{n}nn" (play\underline{ed} by Barbara Eden\underline{)} who will live at home.
Student\underline{s} who are seen as voters\underline{,} who increasingly vote for democratic candidates\underline{,} are not allowed to use their photo ID issued by their institution in several states.
If you are able to read this chronic\underline{le}, it is only thanks to a bo\underline{on} of exceptional banality\underline{:} the photon or the "light particle\underline{"} that is the "Bo\underline{te}" of the electromagnetic force.
Thus\underline{,} at the very end of life, doctors often resort to terminal sedation, which amounts to either sp\underline{ora}\underline{d}ically or permanently seizing the patient until the time of his death.
In recent weeks, she has carried out a series of house searches and made accus\underline{ations} of fraud and corruption against local representatives such as Frank Tampino and Richard Marco\underline{tte}\underline{,} who is the mayor of a suburb\underline{.}
The monastery of the Holy Cross in Jerusalem stands in the place where, according to a Christian legend\underline{,} the tree from which the cross was made for the cru\underline{ci}fix\underline{ion} of Jesus grew\underline{.}
The most important immediate task is to protect the system from corruption so that certificates cannot be bought easily, and both officials and civil rights activists agree.
Parti\underline{cip}\underline{ants} of the protests at Black Friday called for wage increases and expressed their anger that the contribution to in-house health insurance had risen from \$30 to \$100 a month.
There was once a time when nearly a quarter of all American youth\underline{s} were behind the counter after McDonald\underline{'}s's school, but young people still lived with their parents\underline{.}
On the other hand, there is a comment in the forum of the Wall Street Journal\underline{,} whose authors say that it is irresponsible to have children if you do not know how to feed them.
In 1995 I occupied a room in the Push\underline{kin}\underline{s}kaya 10, where until the renovation work there was a musical\underline{-}artistic club for the Bohem\underline{e}, the house of the Petersburg Bohem\underline{e}.
In Petersburg\underline{,} we have those who might be experts\underline{,} but they are being blocked because there is a need for more high-level experts to assess the former properly and to clear the way for them.
The end of the concerts should be about at the time when the Maya calendar ends on the Pacific island of Kir\underline{ib}\underline{ati}\underline{,} which is in a time zone of 12 hours before us.
The aim of the concert is to raise funds for the equip\underline{ping} of a multifunctional educational centre for the disabled\underline{,} which will be called STU\underline{DE}O at the Jedli  u2047 ka Institute in Prague\underline{.}
However, the ideas of the young engineer (born 190\underline{5)} left the audience cold\underline{,} and after years   u2047 tern\underline{feld} still remembered that only Dr. Jan Gadom\underline{ski} had shown interest in his work.
This situation is exacerbat\underline{ed} by the fact that the entrepreneurs are absolutely unwilling to pay their taxes and thereby compensate for the social and economic damage they cause.
"...\underline{that} nothing comes from violence or could ever arise\underline{"} sing\underline{s} Sting in the song Fra\underline{gil}\underline{e}, whose most important verse in the refrain is: "...\underline{th}en we don't forget how fragile we are".
A distinction must be made here between the inhabitants of Israel and their leaders, since the international bankers in Israel, like us, the people, are only choosing their own candidates\underline{.}
Server Bankovn xedpoplatky\underline{.}com, in cooperation with the Association of Liberal Economist\underline{s} Laisse\underline{z} Fair\underline{e}, nominated not only the above-mentioned absurd\underline{ities} but also the EU regulation on the scope of food stocks in the territory of a Member State.
The problem is small-minded politics - when someone comes from the right or from the left with a good proposal, it is deliberately rejected\underline{,} and that is something that the population is holding up.
The Aston Martin was, by the way, a child's dream - James Bond always liked how he drove in the car, was ga\underline{lant} to women and at the same time fought against evil\underline{.}
At the end of the almost 500-metre walk, the Literatur\underline{ca}f xe9 reward\underline{s} you not only with a fantastic view of the city, but also with Dutch cro\underline{quet}\underline{tes} and stuff\underline{ed} fi\underline{cus} trees\underline{.}
Is it difficult for Germany to reconcile its close relations with Israel and the USA on the one hand, and the position of the most important partners in the EU on the other?
In addition, "Voices for Africa" has set up a sewing school, built two chicken houses and, together with the American health organization PSI\underline{,} organised that many people in the village had an HIV test.
"Remarkably many high-altitude people are also present in some parts of China, Japan or the Hunza Valley in Pakistan," says Sc\underline{holz}\underline{,} "even in Sardinia live extremely many very old men".
But what the 61\underline{-}year\underline{-}old engineer\underline{,} who holds a Ph\underline{D} from the American University of Southern California\underline{,} really wants to save, the Egyptian\underline{s} are unaware of that.
That was and is a matter of interpretation\underline{,} and it is to be fear\underline{ed} that Islamist\underline{s} will use the vague wording and the legal room for manoeuvre that goes with it for a stricter interpretation of Sha\underline{ria} law.
Ten\underline{s} of thousands of Mexican families have been affected by violent crimes over the last six years, and the new president has promised to address this issue in particular during his term of office.
As I should learn during my trip, there is one thing that makes this relationship even more complicated\underline{:} some Mexican leaders and parts of the education middle class want to reconnect to the dia\underline{sp}ora\underline{.}
The leaders of Hamas\underline{,} the Islamist movement that has controlled Gaza since 2007, will claim to have pushed the Israelis back, even though its group itself suffered major losses\underline{.}
Turkey, a resur\underline{gent} regional power once considered Israel's closest Muslim ally, has taken sides with Hamas - just like Qatar\underline{,} one of the richest and most dynamic Gulf states.
The government expects to do so from studies that have shown that people who have not yet started smoking at 26 will, with a 99\% probability\underline{,} no longer start smoking\underline{.}
The problem, according to John D. Eastwood\underline{,} an associate professor of psychology at the University of York, Ontario\underline{,} Canada\underline{,} is that bo\underline{re}dom has been defined and discussed in many ways.
He found that 32\% of adol\underline{es}cent\underline{s} were bo\underline{red} in school and doing homework\underline{,} whereas 23\% said they were bo\underline{red} when they were not in school.
In the uncertain weeks following the state u2019s decision to legalize small quantities of mar\underline{i}juana for personal use, the answer to hundreds of minor drug offences depends less on the law than on location.
The show included graduate Joe Cook\underline{e}, former president of Oxford University's Conservative student association\underline{,} who was driving in a Roll\underline{s}-Ro\underline{y}ce wearing a silver suit and a silver\underline{-}filled tre\underline{ad}.
More tragic\underline{ally}, it was Oxford - a university that not only produced 14 Tory prime ministers\underline{,} but still hide\underline{s} behind an undeniable reputation for equality and freedom of thought.
Four months of work and 25 "Raga\underline{zz}\underline{e}" (as the fashion designer called his sewer\underline{s}) were necessary to make this ivory\underline{-}colour\underline{ed} silk dress with beads, twelve different embr\underline{oid}\underline{ery} and a four-and-a-half\underline{-}metre\underline{-}long vo\underline{w}.
"This work is for animals and not for humans" protests Mad\underline{rus}\underline{in}, a sta\underline{unch}\underline{,} 42\underline{-}year\underline{-}old bear\underline{er} who works three decades since leaving school at Kawah Ijen.
"I will not retire\underline{,} I will die here because the volcano was my whole life," explains Unain\underline{ik}, opening his mouth wide, with some teeth missing\underline{.}
In four of the cases, they linked the term to "something very own" on a personal level and "to the password and the user" when applying it to the social networks.
One might say, then, that the procedures for the survival of the companies that allow Mexican law are not valid in the country of stars and strip\underline{es}, in contra\underline{vention} of international agreements.
That is why the Gonz xe1lez Sada family appeal\underline{s} to the same Court of App\underline{e}al so that the vote takes place in plenary\underline{,} that is to say in all the judges\underline{,} because only three of them voted.
"They were my best years, which I enjoyed most, because I was allowed to be part of eight championship\underline{s} of the Va\underline{quer}\underline{os} since 1967\underline{,} whether as managing director\underline{,} co-chair\underline{man} or trainer.
"It is fascinating to see what people are doing to comfort themselves," said Bri\underline{d}gid Robinson\underline{,} a 23-year\underline{-}old student in Rutgers-Camden for religion and socio\underline{logy} from Had\underline{don}\underline{field}\underline{,} New Jersey\underline{.}
This study has also shown that after 12 years of monitoring, meta\underline{sta}ses are likely to be formed by 30 to 40\% if early detection is not carried out.
This "dis\underline{tur}\underline{b}ation" creates an electromagnetic wave (light, infrared or ultra\underline{violet} radiation\underline{,} etc. ), and this wave is nothing more than a photon and therefore one of the bo\underline{son}s of force.
Therefore, a huge particle acc\underline{e}lerator such as CERN - the Large Had\underline{ron} Coll\underline{id}er is a ring of 27 km! - is needed to achieve this kind of energy.
For science\underline{,} they are used to test the standard model (SM\underline{),} and they also allow phy\underline{s}icists to examine in detail all deviation\underline{s} between the observations and prediction\underline{s} of the SM\underline{.}
The scandal was brought to light by him following a thorough investigation of the mis\underline{ap}propri\underline{ations} relating to the contracts for road works in Quebec\underline{,} which the then Prime Minister had reluctant\underline{ly} agreed to.
It is time for the Afghan army to regain its territory and for the Afghan people to decide their future without expecting anything from us.
The Taliban are made up of foreign extremists, former leaders who have fled to Pakistan, but often also peasant\underline{s} who refuse to have an armed foreign presence\underline{,} as in the case of the Soviet\underline{s}.
Short\underline{ly} before the Constitutional Declaration in mid\underline{-}No\underline{ve}mber\underline{,} they turned their backs on the idea that they were unable to express their views.
Finally, Article 2, which attracted all attention, remains identical to that of the 1971 Constitution and states that 'the principles of Sha\underline{ria} law are the main source of law'.
For Islamist\underline{s}, the fact that this article has not been amended is proof of their good will and of their respect for other members of Egyptian society.
In particular, they have in mind Article 220\underline{,} which grants the University of Al-Azhar a consult\underline{ative} role, particularly with regard to the verification of conformity with Sha\underline{ria} law.
Visitors come here for treatments using salt water (natural salt\underline{s}ole\underline{)} and cur\underline{ative} slu\underline{d}ge as well as for the treatment of skin inflamm\underline{ations}, allergie\underline{s}, asthma, eczema, arthritis\underline{,} bro\underline{n}chitis\underline{,} sugar sick\underline{ness} and to calm stressed nerve\underline{s}.
The money on the trip is not taken in euros\underline{,} but in dollars that can easily be exchanged in bill\underline{s} (current exchange rate: 1 dollar to 3.8 bill\underline{ets}\underline{).}
"To\underline{day}, there are countless private arm\underline{ament} factories that do not stand up to international competition and therefore squ\underline{ander} weapons under the hand of the black market, for example in Moscow\underline{,}" reports the expert\underline{.}
Black Friday lasted the next day in his store from 8 a.m. on Thursday to midnight\underline{,} during which time Wal\underline{mar}t sold about 5000 items per second.
- And all this united in your art clinic\underline{...} - It was important to me to be at the center of Petersburg culture, where the best creative artists should gather\underline{.}
Nowadays\underline{,} it is easy to become famous, but culture and popularity are not the same: you can be famous without making a cultural contribution.
The same applies to the Erarta, but with the difference that they honestly say that they do not take all contemporary art and some painter\underline{s} therefore have to look for other museums\underline{.}
The system must exclude those who want to attack and abuse the system and not penalise those who have committed a formal error that does not affect the actual decision-making process.
I would remind you, for example, of the lecture given by A.   u2047 tern\underline{feld} on 6 December 1933 at the Warsaw Observatory\underline{,} where the author presented ideas from his pioneering work "Ein\underline{gang} zur Kosmonautik\underline{".}
However, these solutions are wrong and always lead to a worsening of the situation (see the establishment of the FED\underline{,} so that crises like the ones they triggered in 1907 do not occur again).
But I can no longer see the republic being pl\underline{under}\underline{ed} for 20 years, the th\underline{ieve}\underline{s} running around freely while people are being raised taxes and retirement ages.
In order to counter\underline{act} this stupid situation, a few years ago, it was decided to contribute to general education and to rebuild the seven fi\underline{ct}\underline{it}ious bridge\underline{s} depict\underline{ed} on the euro notes as nicely brush\underline{ed} steel concrete\underline{mini}\underline{atur}\underline{es}.
Stephen Szabo is Deputy Director of the Transatlanti\underline{c} Academy in Washington\underline{,} an institute in which academic\underline{s} and policy experts from Europe and North America research the challenges of the transatlanti\underline{c} community.
Initial\underline{ly}, it was the private commitment of individuals to send a child to school for a few euros a year and to give him a warm meal a day.
This section of an infrared image of the Spitze\underline{r} telescope shows a "family portrait\underline{"} of countless generations of stars\underline{:} the oldest stars are visible as blue dots, the pink "new\underline{born}\underline{s}" in the Star Circle\underline{.}
As her mother tells her story\underline{,} a picture of Maria\underline{na} looks down on us from the wall\underline{,} placed next to a cross that has a single word: justice.
The fact that pragmatic President Mor\underline{si} met Barack Obama to achieve a ceasefire could be a promising sign - and perhaps symbol\underline{ize} the beginning of a new era\underline{.}
Although Australia has one of the lowest rates of smokers in the world, and the changes will have little impact on multinational profits\underline{,} other countries are already considering similar steps.
If, on the other hand, you do a mono\underline{ton}ous activity - "as well as searching for fault\underline{y} products on a factory conveyor belt\underline{,} music can distract and help not to feel bo\underline{red}".
The police authorities no longer prosecut\underline{e} adults over the age of 21 for possession to a small extent, which is permitted by law as soon as the new laws enter into force in the coming weeks.
At the same time, several cities, from the suburb\underline{s} of Denvers to the Western Mountains\underline{,} are voting to prevent new state-licensed mar\underline{i}juana operations from opening in their communities\underline{.}
"This situation is developing so fast that I don't know what will happen next," says Daniel J. Oates\underline{,} police chief at Aurora\underline{,} located east of Denver.
Their situation was exacerbat\underline{ed} by a recent documentary on BBC Two\underline{,} entitled 'Wo\underline{nder}\underline{land}: Young\underline{,} Bright and on the Right\underline{'}, which Tories portray\underline{ed} as ecc\underline{en}tric\underline{s} and neo\underline{-}Na\underline{zi}s.
"I suggest you take some French lessons in your free time - so if you are not too busy with your social activities," Pit\underline{t} told me.
On the occasion of the exhibition "Val\underline{en}tino - Master of Cou\underline{ture}" opened this week in London, ABC talks with Naty Abascal, Fiona Thyssen\underline{-}Bornemis\underline{za} and other famous customers of the Italian fashion\underline{maker}\underline{.}
After breaking out large sulphur stones\underline{,} weigh\underline{ing} up to 70 kilo\underline{gram}\underline{s} in total, he transports them on his shoulders in two ba\underline{mbo}\underline{o} basket\underline{s}.
These changes in social realities have contributed to the increase in the number of single-parent\underline{s} and to the delay\underline{ing} of marriage and birth\underline{s}, the result of which is a reduction in the birth rate in Singapore\underline{.}
The Municipal Development Authority has begun to control the number of small apartments known as "shoe boxes\underline{"} that can be built in certain areas of the city.
As regards the decisions taken, he said that the countries of Unasur will 'take significant steps towards the goal of South American citizenship\underline{,} to which we will extend the decisions on residence rights'.
The need for Latin America to remain an integrated region of prosperity and peace and good neighbour\underline{ly} relations was another aspect that was emphasised at the summit.
Santo\underline{s} and Ortega would meet in Mexico on Saturday\underline{,} where they intend to be present at the inaugura\underline{tion} of the country's new president\underline{,} Enrique Pe  u2047 a Nie\underline{to}.
As you know, these measures took place despite the fact that the Senat\underline{e} had disregard\underline{ed} the possibility because it considered them to be a violation of freedom of expression in social networks.
"We analyze why these ideas spread over time," he said, as well as the way hypothe\underline{t}ical scenario\underline{s} are offered that lead to a particular human behavior\underline{.}
However, the Brenn\underline{an} Center considers the latter a myth by affirm\underline{ing} that fraud in the US is less common than the number of people killed by the lightning strike\underline{.}
Democratic critics denounce the partisa\underline{n} nature of the laws passed and see them as a clear objective to influence the results in the countries that will determine 2012\underline{.}
It is too early to confirm with certainty that these changes to legislation on the electoral system will have a significant impact on the outcome of the presidential elections in 2012\underline{.}
He even managed to smile brave\underline{ly} and talk to the strange\underline{rs} who work around him, bring his medicines to him and give him a bath.
According to Dr Christian\underline{e} Martel, Quebec\underline{'}s health system is not efficient enough to ensure that everyone has the right to high-quality pal\underline{li}ative care before accepting to go on to eu\underline{than}\underline{asia}\underline{.}
Recently\underline{,} she says\underline{,} I saw a patient who was in the emergency room for 14 days with great pain\underline{,} without taking measures to relieve her.
Based on a share of 70\% of black money in the financing of the electoral campaigns in Quebec\underline{,} he joke\underline{s}: 'I have been told that this is only a slight drop in reality'.
If this story damages the international standing of Quebec and Montreal\underline{,} Mr Duches\underline{n}eau calls on those who laugh to take a look at their own backyard\underline{...}
This is done through a mathematical task that is started on the computers\underline{,} with the privilege of adding this extra line to the winner\underline{,} who is a kind of temporary central banker.
These works, which required a large number of local workers, have helped to suppress the insurg\underline{ency}\underline{:} irrigation\underline{,} wells, drinking water, reforestation\underline{,} fruit trees\underline{,} soil protection and farm\underline{land} increase.
A much more modest budget will help to improve local living conditions, which are very hard in these valley\underline{s}, which are often more than 2000 metres high.
Whereas Egypt remains more divided than ever with regard to the constitutional declaration\underline{,} which temporarily gives it unlimited power, it has decided to put everything on one card.
Jerusalem is also the most sacred place of the Jews - the Wailing Wall\underline{,} the remains of a temple destroyed by the Romans in 70 AD\underline{.}
Half of all weapons on the black market are there through the 'debt of those responsible for their work with weapons\underline{'}, says the report.
A sales advise\underline{r} to an arms shop who does not want to be named\underline{,} assure\underline{s} us that weapons found in illegal excavat\underline{ions} have long since no one bought them, since they are outdated\underline{.}
The protests started last week after Thanks\underline{g}iving\underline{,} on the so-called Black Friday\underline{,} where sales took place in the US, attract\underline{ing} millions of customers, which sometimes led to hand-wrapping\underline{.}
For example, in the field of controlling objects in public places, we worked on a project in which we experiment\underline{ed} with short and short gesture\underline{s} rather than loading them out.
- Imagine for a moment that the manipulation of virtual holo\underline{gram}\underline{s} in the air is accessible not only to Tony Stark from Iron Man, but also to normal mor\underline{tal}s.
He is also a man of the city and his presence on the street makes his fellow citizens smile and make them feel good.
Under pressure from global and European economic competition, the Czech Republic will continue to be forced to seek ways to push the social level of the population down.
After the assassination of Ferdinand of the Habsburg thro\underline{ne} in Sarajevo\underline{,} they succeeded in trigger\underline{ing} World War I, destroying the Russian empire through the Bol\underline{sh}evi\underline{ks} revolution\underline{.}
On the one hand he is a realistic Pol\underline{itt}\underline{hr}iller\underline{,} but at the same time a so-called "Ca\underline{per} Movie\underline{",} i.e.
I believe that German foreign policy is motivated by economic policy, that is, by exports and its relations with certain regions, such as Russia, China or the Middle East.
"It is becoming increasingly difficult for foreigners to protect their trademarks in China," says Thomas Pat\underline{t}loch\underline{,} Taylor Wessing attorney\underline{,} who specialize\underline{s} in property infringement\underline{s} in the Far East.
And when you return the 87\underline{33} km airline to Heidelberg\underline{,} to the stamp\underline{ing} singer\underline{s} in the rehears\underline{al} room on Bergheimer Stra xdfe, you can see it there too.
Ten\underline{s} of thousands gathered in unusual concord on Friday evening in Tahrir Square in Cairo and vo\underline{wed} to overthrow the Charter before it can enter into force.
As Mexico u2019s future president\underline{,} Enrique Pen\underline{a} Nie\underline{to}, prepare\underline{s} to take office, the BBC u2019s Will Grant analyze\underline{s} the challenges ahead and the mixed feelings of his people.
"We expect real and lasting change from him," says his friend and political ally, Gabriel Ol\underline{ver}a Hernandez, who works as a congress\underline{man} for Pen\underline{a} Nie\underline{tos}\underline{,} the PRI\underline{.}
Manning charges include favor\underline{ing} the enemy\underline{,} unlawful publication of intelligence information on the Internet, transmission of national defense information and theft of public property or documents.
And, given the unjust distribution of income, unbri\underline{d}led corruption and drug violence, many of us are not so sure that this is really a great country.
Apart from the different health warning\underline{s} and pictures\underline{,} from next Saturday the only difference between the pack\underline{s} in the brand names\underline{,} which are printed in identical\underline{,} small font\underline{s}.
"You just take a til\underline{t} and put the box away," says Victor El Hage when buying a cigarette packet on which a photo is printed with a mouth tum\underline{our}\underline{.}
Despite several arrest\underline{s} of consumers and medical mar\underline{i}juana vendor\underline{s}, the Federal Government has largely allowed the sale of mar\underline{i}juana medical products in Color\underline{ado}, Washington and 16 other states.
Conservative members of the Corp\underline{us} Christi College\underline{'}s Junior Common Room (JCR\underline{)} claim that they are "often actively isolated\underline{,} attacked\underline{,} and declared undesirable\underline{"} because of their political views.
Somerset House, the former residence of Isabel I of England\underline{,} is the only place in the British capital worthy of hosting an exhibition on Valentin\underline{o} Gar\underline{ava}\underline{ni}.
In this audience of fashion dolls, names such as those of Sib\underline{illa} de Luxembourg\underline{o}, Glo\underline{ria} of Thu\underline{r}n and Taxi\underline{s}, Mette\underline{-}Mar\underline{it} of Norway\underline{,} Ros\underline{ario} of Bulgaria or Sof xeda of Habsburg ra\underline{di}ate.
"Si\underline{nce} we normally carry 70 kg\underline{,} we get about 46,000 rupees (3\underline{.}8 Euro) for each way," explains Anto, who usually makes three tracks a day.
This kind and intelligent young man could work as a tourist guide\underline{,} wait\underline{er} or hotel reception, but instead he does the work of a carryer.
Time passes\underline{,} but poverty persist\underline{s} generation to generation in one of the tough\underline{est} profession\underline{s} in the world: those who work as human vice\underline{s} on Kawah Ijen.
"This has made it possible for people, apart from mar\underline{ry}ing and forming a family, to have much more options in terms of life goals and to set priorities," she explains\underline{.}
The teenage\underline{r} has user accounts in Hot\underline{mail}, Facebook\underline{,} My Space and Ask\underline{,} and in Ask he admit\underline{s} not to know 20 of the people he added to his friend list.
There is a danger\underline{,} however, that he would suffer physical and psychological damage because he is trapped in a narrow room and cannot carry out physical exercises outdoor\underline{s}.
He decided to take care of his illness alone and began to learn about it, with such dedication that he just celebrated his 43\underline{rd} birthday\underline{.}
Fabr\underline{i}zio has been living with the human immun\underline{o}def\underline{ici}\underline{ency} virus (HIV\underline{)} for 22 years, which was difficult to imagine at the beginning of the 1990s, when there were many doubts\underline{,} few treatments and more st\underline{ig}mat\underline{a}.
"What do you need it?
There are half a dozen examples\underline{,} including Ag\underline{rem}\underline{ex} and Comercial Mexican\underline{a}, whose liabilities among companies of the group have been confirmed by the Institut\underline{o} Federal de Concur\underline{s}os Mer\underline{can}\underline{tile}\underline{s} (Federal Institute for Trade Concur\underline{s}ors).
If this is not accepted, the Cer\underline{ci}orare appeal will be lodge\underline{d}, calling for the procedure to be reviewed by a higher court\underline{,} in this case by the Supreme Court of the United States.
Lind\underline{a} Gra\underline{y}, who played the role of his wife in the original and subsequent series, was with Hag\underline{man} when he died at Dal\underline{las} hospital\underline{,} said her journalist Jeff\underline{re}y Lan\underline{e}.
J.R. had sw\underline{or}n and threatened to portray her as a prostitu\underline{te} if she did not leave the city.
It is unforgettable and irre\underline{place}\underline{able} for millions of admire\underline{rs} in the world and remains in our hearts for those who have been fortunate enough to know and love it.
On the other hand, the same states allow members of fishing or hunting associations who vote more for the Republican side to use the cards issued by these clubs for elections.
For example, in the 2008 general election in Florida\underline{,} 33\% of pre-elected voters were African\underline{-}American\underline{s}, even though they account for only 13\% of the state u2019s voters\underline{.}
Today, many men who have been identified with cancer do not receive treatment because their cancer is not aggressive and pose\underline{s} no threat to their lives.
And several organizations\underline{,} such as the Victor\underline{-}Ga\underline{db}\underline{ois} Home and the Montreal Home Pal\underline{li}ative Care Society\underline{,} are more or less specialising in caring for cancer patients\underline{.}
In addition, an organize\underline{r} of the mayor\underline{'}s party, Martin Dumont\underline{,} has accused Mr Tre\underline{mb}lay of deliberately overlooking a shadow budget that was pour\underline{ing} black money into his coffer\underline{s}.
However, if we win in a home game against Tro\underline{yes} 4-0 and you still find something you can accus\underline{e} us of, that is certainly somewhat fru\underline{st}rating\underline{.}
Its Pay\underline{tun}\underline{ia} system correspond\underline{s} to a credit card (with real money) or a contactless payment with a mobile phone, but uses Bit\underline{co}in to validate transactions that are cheaper\underline{.}
You just have to specify an address that can be "photo\underline{graph}\underline{ed} and recognized\underline{"} by a phone, says Pierre Noiza\underline{t}, who assure\underline{s} that he has thousands of users.
The withdrawal of French troops from the base in Ni\underline{j}rab, observed by a hill planted with almond trees\underline{,} financed with French loans\underline{,} was carried out properly.
Its supporters are assured that it is a way to end the institutional and political crisis as quickly as possible and to speed up the transition process.
The ruins of the fortress Mass\underline{ada} are the remains of the secret hiding place from enemies that Hero\underline{d} the Great built for his family in 25 AD\underline{.}
There are preserved ancient Qu\underline{m}ran manuscript\underline{s} or Dead Sea scroll\underline{s} found in cave\underline{s} in the Jud\underline{e}an Desert\underline{,} as well as approximately 500 thousand archaeological and anthropological exhibit\underline{s}.
The most poignant department is the monument to the children, built to commemorat\underline{e} the 1.5 million children who were destroyed in the concentration camps and gas chamber\underline{s}.
Sur\underline{pr}\underline{ising}ly, the Red Sea is also bathed in the winter months, as the water temperature there does not fall below 21  u2047 C and the air warms up to 23  u2047 C.
According to tradition\underline{,} it was here that Noah built his ark\underline{,} and Pers\underline{e}us saved the beautiful Androme\underline{da}, with which he led a long and happy life in this place.
In many cafe\underline{s}, restaurants and restaurants only cosier food is served, excluding por\underline{k}, sea products, fish without scale\underline{s} and food containing both milk and meat products.
The Chairman of the Duma\underline{'}s Security and Corr\underline{up}tion Committee, Irina Jar\underline{ova}\underline{ja}, supported the proposal and promised that the amendments to the Arm\underline{s} Act will shortly be submitted to the Duma\underline{.}
Researchers from California University in Ber\underline{ke}ley show that if the company increased the average wage to \$1\underline{2} per hour\underline{,} it would cost Wal\underline{mar}t \$3.2 billion.
In fast-food restaurants, the minimum wage is gradually being raised, but not too high, and on average\underline{,} ordinary New York employees get \$8.90 per hour\underline{.}
Now, during interview\underline{s} with McDonald\underline{'}s staff, I see people complain\underline{ing} that they have to live with this wage and sometimes even feed their children.
I think that in the near future, we will need to work, above all, on developing new types of sensor that will enable us to better understand people's reactions\underline{.}
The whole city knows Kir\underline{ill} Mill\underline{er}, the red bear\underline{,} which is sometimes seen at the Russian Museum, at the summer garden, at scene meetings or at openings.
I am a man of the past culture and grew up with artists who lived in poverty and died in poverty and refused money to paint\underline{.}
"A law is never perfect, but it must be applied correctly - and I do not think this is the case with us", Kal\underline{a} commented on the current situation.
At the meeting of the Chamber of Deput\underline{ies}' Supervisor\underline{y} Committee, you spoke about a common Czech-German project, in which the laws of both countries regarding public contracts were compared\underline{.}
Her colleagues in the Jesen xedk district also had to leave at night, according to them the roads are free and wet up to the height\underline{s} after chemical treatment.
Nevertheless\underline{,}   u2047 SA and British Airways have always been very well prepared for us, that I have sometimes been surprised\underline{.}
In London and Madrid it is absolutely common for people with severe disabilities to be able to move independently in public areas, go to the museum\underline{,} use toilet\underline{s}, etc.
Liberal theories and the media maintain ad nauseam that the state must not participate with capital in its own economy, and that planned economy leads to economic disaster\underline{.}
The server www.bank\underline{ov}nipoplat\underline{ky}\underline{.}com, which annually collect\underline{s} a survey on the most absurd bank charges\underline{,} decided this year to hold the contest "the most absurd regulation or idea from the EU workshop\underline{".}
Finally, the European Commission approached the Czech Republic to such an extent that it organised a tender for the purchase of ce\underline{real}\underline{s} from countries which do not have access to the sea.
I always publicly support any good solution, even if it comes from the KS  u2047 M or the ODS\underline{,} and I will also oppose bad ideas.
I might call this pop\underline{ul}ism, but all the proposals I have mentioned already work in the world, or they have been discussed by important experts\underline{.}
Under heat and pressure, the so-called Landbou\underline{w}plastic (KLP\underline{)} turns into a dark\underline{,} homogen\underline{eous}\underline{,} load\underline{able} material that smell\underline{s} a bit of new cars and a bit of sports shoe\underline{.}
This is because it is precisely changing its foreign policy away from a policy that was managed, so to speak, by the United States to a German foreign policy.
Germany is not yet used to it, it is still unpleasant and, for obvious reasons, it is still difficult for it to play a greater role.
I thought about the moment this week when Mexican future President Enrique Pen\underline{a} Nie\underline{to} visited the White House to meet President Obama\underline{.}
Let us tell our American colleagues how great a visit to this country is and how pressure is exert\underline{ed} on the political leadership to strengthen its ties with Mexico\underline{.}
Wa\underline{it}ing for half a day at the airport for a flight is quite nervous - even if books\underline{,} magazine\underline{s} and iPhone\underline{s} (and of course tax-free shopping) are available.
"We do not want to get into a position where we license someone and then face a major problem at the federal level," says Bob Nicholson\underline{,} member of the City Council.
Political issues such as the min\underline{er}'s strike\underline{,} privatisation and opposition to the government of sanctions against the apart\underline{heid} regime of South Africa have found their way into the wood\underline{-}pan\underline{ell}ed rooms of the tut\underline{or}.
At my first of these events, I was supposed to translate French texts from the 18th century into English, and I was not prepared for what was to come.
A student in philosophy\underline{,} politics and economics who, iron\underline{ically}\underline{,} visited the conservative Eton College\underline{,} said to me: 'You are the daughter of a fascist pig\underline{'}.
During a tutorial the following week, when another historian seriously claimed that I was "an enemy of the people", I decided to do the same.
For four euros\underline{,} the carriers of the Indonesia\underline{n} volcano are risking their lives and health by carrying 70 kilo\underline{s} of sulphur over steep\underline{,} rocky roads\underline{.}
To do this, he must climb down to the bottom of his cra\underline{ter} every day, where the sulphur\underline{-}contain\underline{ing} gas coming out of the earth solid\underline{ifies} in contact with the air.
"I will be working here for another two years because I want to open a shop or learn Spanish or French," he promises in more than acceptable English.
While the falling birth rate has the known impact on a nation u2019s economic growth, tax revenues\underline{,} health costs, and immigration policies, the example of Singapore also shows unexpected consequences.
Men and women pursue their career\underline{s}, the stress and the cost of property and education as reasons why they cannot have children.
According to the dictionary\underline{,} it is the property of private or 'any area of private life where you are entitled to protection from any kind of interference\underline{'}.
According to the expert\underline{,} the most effective way to teach children and adol\underline{es}cent\underline{s} what privacy is is to ask them questions that make them think.
At both international meetings\underline{,} the Peru\underline{via}\underline{n} authorities stressed that the information systems were in place for journalists\underline{,} but they greatly restricted access to information.
The summit also ended with the joint commitment of Chile and Peru to adopt a judgment by the Hague Court, which resolve\underline{s} a border dispute between the two countries.
Correa assured us that he did not regret this decision, because he did not betray his principles, but he lived up to his 'deep democratic values and views on human rights'.
They should not be paid the beer and motel, as Governor Emil\underline{io} Gonz xe1lez replied to the question as to whether preserv\underline{ative}s would be distributed under his administration.
"Sexual\underline{ity} does not look like this; the best thing is to bring the condom\underline{s} closer to those who are already engaged in sexual activity," he explained\underline{.}
I was part of the most successful era of the national team from 1988 to 1995, which at the beginning of the 1990s included the BSN up to 17 teams in one season.
In the years before "Da\underline{lla}\underline{s}" Hag\underline{man} became known on television as a nice guy in the years 1965 to 1970 with the sit\underline{com} "Ador\underline{ing} Jean\underline{nie}\underline{"} of the TV company NBC\underline{.}
He was also the actor of two short-live\underline{d} comedies\underline{,} such as The Good Life (NBC\underline{,} 1971\underline{-}72\underline{)} and Here We Go Again (ABC\underline{,} 1973\underline{).}
"I have not noticed that this will be the most apocalyptic semester ever," said Char\underline{m} xe9 this week to students at Rutgers-Camden University (New Jersey\underline{).}
"We do not take up 2012 so that we can always keep the option to hold the course again, in case the world does not sink\underline{,}" said Restall\underline{.}
In the studies carried out in the United States, there were many disturbance\underline{s} between the control groups, so it is difficult to interpret these data and make clear recommendations\underline{.}
That is why I recommend testing at the age of 50 or 40 if you have a direct relative who has already had prostate cancer\underline{.}
In cooperation with the International Society for Ur\underline{ology}\underline{,} Move\underline{mber} has developed an instrument that enables us to assess the advantages and disadvantage\underline{s} of the PSA test.
Indeed, it is believed that this bo\underline{son} is involved in nothing less than the mechanism responsible for the mass of all objects in the universe\underline{.}
Similarly\underline{,} not all particle\underline{s} interact with the Hi\underline{gg}\underline{s} field: those who do have a mass, while others (like the photon, by the way) do not have a mass.
When I told my oncologist that I would stop the treatment, she told me that she regret\underline{s} that I am wa\underline{ging} the fight, she told me.
"It is strange how the system has disintegr\underline{ated} since drastic measures have been taken," joke\underline{s} Jacques Duches\underline{n}eau\underline{,} Member of Quebec and former Head of the Montreal Police\underline{.}
We are cleaning up the wound\underline{,} but we need an invest\underline{ig}ative unit only for Montreal and supervision to prevent the return of dubious practices\underline{.}
Us\underline{ing} the content of the file, it is also possible to ensure that the bitcoins traded are present in the account book of public accounts spread throughout the network.
Afghan women have paid the price for the obscur\underline{ant}ism of farmers overwhelm\underline{ed} by Al Qaeda\underline{,} but their situation has not improved to date.
According to Egyptian specialist Sophie Pommier, this is worrying because 'the people who are asked to give their opinion have not been elected and have no democratic legitimacy whatsoever\underline{.}
The bla\underline{sp}hem\underline{y} is being maintained and insult\underline{s} are now banned\underline{,} which could have serious consequences for freedom of expression\underline{,} particularly for the press.
Of course, it is not so much their fault as the evil\underline{:} only a few Turk\underline{men}s, Uzbek\underline{s} and Taji\underline{ks} can afford proper primary education.
The authors of the open letter are convinced that tight\underline{en}ing up the law on private arms owners will not prevent criminals from using the black market.
"I can shoot there, and if I am convinced that the weapon has a good shot\underline{,} we negotiate with each other," the expert describes the approach.
However, only a few hundred people were present, far from all of whom are employed in the fast-food sector, where tens of thousands of people work in New York.
- It is certainly not a universal solution, since it raises questions about privacy\underline{,} because you do not always want to inform all those around you about your actions and intentions\underline{.}
A flexible, Ki\underline{n}ect\underline{-}like system would be nice, where we could play with different camera angle\underline{s} to see how this helps us to determine a position three-dimensional\underline{ly}.
At some point, however, it becomes a reality when the Earth\underline{'}s inhabitants in their spaceships break up into a distant planet that becomes the home of their offspring born in space.
Road\underline{s} in Ol\underline{o}mouc county can be accessed without restrictions\underline{,} but in   u2047 tern\underline{ber}k the drivers have to drive carefully in forest sections\underline{,} as the roads are still wet here.
The Tap Tap is currently very popular, but if we go back a few years, what motivated you to start a band in 1998?
We have become aware that if you do something and you cannot see it outside, your own performance does not exist in a sense.
All three venue\underline{s} are finally connected by live circuit\underline{s} and a common interpretation of the anthem "World Ending is Out\underline{"} of the band The Tap Tap\underline{.}
Gadom\underline{ski}'s world-wide recognized contribution to space development was acknowledged by the fact that one of the cra\underline{ters} on the earth side of the moon was named after him.
Met\underline{e}or-2 had a starting weight of 380 kg and was able to carry a payload of 10 kg to an altitude of approximately 60 km.
It is also worth mentioning the accession of Poland to the COS\underline{PAR} (Com\underline{mitte}\underline{e} for Space Research) in 1960\underline{,} which was followed by the creation of a national COS\underline{PAR} committee two years later.
As it turns out, today's society, as in ancient times, is based on the reck\underline{less} preference of one's own advantage, without paying attention to the interests of society as a whole.
From today u2019s perspective\underline{,} the demise of these regimes for the benefit of liberal democracies can be seen as a pause in which the next round is already lo\underline{om}ing.
The weakness of Argo is its over-explo\underline{it}ation due to the need to show too much action in too many places.
The difficulty\underline{,} however, is not only that we, as a people, are shooting in the pub and in front of the television\underline{,} but are closing down anyone who wants to change something.
You entered the battle for the castle with the thesis of the material and criminal liability of politicians as well as with retro\underline{spect}\underline{ive} declarations of assets over   u2047 20 million.
I have not yet thought about this because I do not have time to review the past of any potential party member, nor do I have the money to do so.
The MV\underline{R}DV architect\underline{s} prove that the real adventure\underline{s} are not only in mind - with the example of Sp\underline{ijk}\underline{en}isse and the recently built bookberg - 2 photos\underline{.}
According to the market research company CL\underline{SA}, China is the third largest market for luxury goods and the fastest growing one, with a volume of 15 billion euros per year.
This is something that has been missed\underline{,} as family names could not be protected in Germany, says Han\underline{no} Wentz\underline{ler}, Chairman of the Management Board of Freud\underline{enberg} Chemical Special\underline{ities} in Munich\underline{.}
It is not enough to rely on international trademark rights, but rather foreigners should 'register in China anything that is somehow worth protecting\underline{'}, as Wentz\underline{ler} says\underline{.}
For 8,73\underline{3} kilometres of airline away from Heidelberg\underline{,} in the northwest of the kingdom of Swaziland, there is the village of Esitjeni, which depends on the voice of the German choir\underline{.}
The well-organiz\underline{ed} Muslim Brot\underline{her}hood in turn turned into counter\underline{-}demo\underline{n}stration\underline{,} but not in Tahrir Square\underline{,} but after a mass prayer on the other bank of the Nil\underline{e} in front of Cairo University.
Rakfisk is a trou\underline{t} sp\underline{r}inkl\underline{ed} with salt\underline{,} which is fer\underline{ment}ed in water for up to one year depending on how st\underline{ink}\underline{ing} one would like his fish to be.
If you avoid bringing Rakfisk close to the nose, it is not bad - like Sushi\underline{,} who has a long bus ride behind him.
Rakfisk is the product of a very different, much poorer Norwegian era\underline{,} when there were no cooling facilities and fish was satur\underline{ated} in air-tight salt\underline{water} barrel\underline{s} in autumn\underline{.}
The military said that it gave him this restrictive status - one stage under the risk of suicide - to protect him and others.
On a recent trip to Mexico City, I had just crossed the hall and arrived at the passport control when there was confusion in me.
Yet Mexico u2019s biggest challenge is in fact related to the more than 35 million Mexican Americans living in the United States.
Indeed, he says\underline{,} we now know that tinkering and tingling, often interpreted as a sign of bo\underline{re}dom\underline{,} can even fight them by keeping people physically more attentive\underline{.}
On the other hand, many philosopher\underline{s} and authors examine the relationship between bo\underline{re}dom and creativity\underline{,} as is Professor Vo\underline{da}nov\underline{ich}, who has been researching the subject for more than two decades\underline{.}
"Co\underline{lor}\underline{ado} has a more regulated market, so the state is well-suite\underline{d} to orientation\underline{,}" says Brian E. Smith\underline{,} spoke\underline{s}man for the regulator of spirit drinks in the State of Washington\underline{.}
At present, 119 people have to take legal proceedings for possession of about 50 gram\underline{s} or less mar\underline{i}juana, although many have also been charged for other offences\underline{.}
"They spent so much of their lives prosecut\underline{ing} people for still not being able to accept legalization," he believes\underline{.}
Prince\underline{s}s D'Ar\underline{enberg} keeps her evening dress\underline{es} of the fashion designer "with absolute care", "because a dress is not only a dress but also the memories associated with it".
The advertising company BBH, which made the video, maintains the hope that the commercial will reach the problem in a fun way.
The rise in immigration is also seen as one of the reasons why the ruling party in Singapore achieved its worst election result since independence last year.
The boy is aware that it is wrong to write obsc\underline{en}e photos\underline{,} nu\underline{de} photos\underline{,} crimes\underline{,} or offensive or violent comments.
"They should also be elected when they are most important to be popular, to have thousands of friends without thinking about the consequences," he adds\underline{.}
The little information circulate\underline{d} among journalists was received by the press spoke\underline{s}person\underline{s} of some of the Unasur governments present at the meeting, but not by the Peru\underline{via}\underline{n} press spoke\underline{s}person\underline{.}
Argentina\underline{,} Bolivia\underline{,} Colombia\underline{,} Ecuador\underline{,} Peru\underline{,} Brazil\underline{,} Uruguay\underline{,} Venezuela\underline{,} Chile\underline{,} Guy\underline{ana}, Sur\underline{in}am and Paraguay are members of UNAS\underline{UR}\underline{,} even though the latter country is currently excluded\underline{.}
"It was as if a bomb struck\underline{,}" he says about the moment when he received the diagnosis that the doctor tried "to weaken\underline{"} without disc\underline{ern}ing success.
In fact, the United Nations Model Law for the Unification of International Trade Law was created to this end, with the American Law Institute being used as a mediator.
On the other hand, Vitro is to blame for his difficult situation as of 2008, in the context of the major economic crisis in the United States, which gave the country blow\underline{s}.
That the boys in Ponce\underline{,} for example, only play in their area and only meet teams from other corner\underline{s} of the island in the national playoffs.
He tried his luck on stage in New York in the early 1950\underline{s}, then served in the air forces in England from 1952 to 1956\underline{.}
And he is not the only professor who offers courses on the "end of the world" this semester\underline{,} which should be the last in history.
In fact, the PSA test sometimes shows fault\underline{y} results, with false negative or false positive results that lead to unnecessary medical interventions\underline{.}
Although it was not the original purpose, this sensor now serves as a "ey\underline{e}" to all digital cameras worldwide and has won the Nobel Prize for Physi\underline{cs} in 2009.
"Si\underline{nce} six months three to five beds have always been occupied with cancer patients less than 45 years old," says Dr. Christian\underline{e} Martel worried\underline{.}
The Char\underline{bon}\underline{n}eau Commission "has already brought down two mayor\underline{s}," he adds\underline{,} in the hope that it will "dis\underline{cover} the ta\underline{ctic}\underline{s} behind individuals\underline{".}
Even though the great teams such as Marseille\underline{,} Lyon or Bordeaux are struggling to win the title, I believe that we have what it takes to win\underline{.}
Consider Manchester City, a club that hasn't been able to qualify for the eight\underline{h} final for two seasons, and that has also made huge expenses\underline{!}
We have learnt a lesson from what has happened in Ukraine, and today we must behave in an exemplary manner.
Moreover, as so often happens in these technologies, a political vision is tangible\underline{:} the conviction that the current monetary system, designed by bank monopolies\underline{,} is leading to financial crises\underline{.}
Recently\underline{,} Adi Sha\underline{mir} and Dor\underline{it} Ron of the Weizmann Institute in Israel analysed the accounting book and showed that almost 80\% of bitcoins are not circulating\underline{.}
For almost two years now, Egypt has been rely\underline{ing} on a provisional\underline{,} amended text, which weaken\underline{s} institutional stability and leads to legal confusion\underline{.}
In the north of the country, 1600 to 2040 meters above sea level, there is the famous ski resort Hermon, which attract\underline{s} countless tourists during the winter months.
In Ak\underline{ko} you can visit the museum in the Bad Al Bas\underline{ha}, which houses several rooms of old Turkish baths with sculpture\underline{s} by then visitors and bathers.
Their families do not even have money to feed the children, let alone buy decent clothes\underline{,} shoes and schoolware\underline{.}
Of course, the new owners did not get them in va\underline{in}: every migrant who hoped to avoid testing paid seven thousand rub\underline{les} for the document.
The police want to ban the wearing of non-lethal weapons in public and raise the age for possession of fire\underline{arm}\underline{s} from 18 to 21 years.
According to research data, 17\% of weapons originate from conflict zones\underline{,} 14\% originate from thefts in the production of weapons and 5\% originate from illegal excavat\underline{ions}\underline{.}
"In order to obtain a weapon\underline{,} I need a friend who has contacts\underline{,}" says the sales consultant\underline{.}
First, Google presented a working model at its annual conference in the summer, then in November it became known that Microsoft had applied for a patent\underline{.}
I became friends with the painter\underline{s} of the new generation\underline{,} i.e. with the representatives of the "Ga\underline{zone}\underline{v}schina"; the result was "Push\underline{kin}\underline{s}kaya 10", and then there was an end to it.
In 1988\underline{,} the second woman in space, Svet\underline{lan}\underline{a} Sawi\underline{z}kaja, who was twice in orbit and even did work outside the space vehicle\underline{,} gave birth to a son\underline{.}
This confirm\underline{s} that it is not enough to keep laying down new and more precise rules, and we also need to look at the actual application of the law.
Effi\underline{ci}ency means buying something at a reasonable price (which is not always the lowest price) and excluding illegal enrichment or even criminal acts\underline{.}
Ice smooth\underline{ing} can be achieved in the areas of Lan  u2047 kro\underline{un},   u2047 st xed nad Orlic xed, Poli  u2047 ka\underline{,} Svita\underline{vy} and Vys\underline{ok} xe9 M  u2047 to.
On the   u2047 ervenohor\underline{sk} xe9 sedlo pass, drivers in the direction of Jesen xedk have to count on snow\underline{-}making\underline{,}" said one of the   u2047 umperk Road Authority\underline{'}s employees today opposite the   u2047 TK agency\underline{.}
According to meteorologist\underline{s}, there were ideal conditions for this during the night - rain and melting snow during the day, cloud\underline{less} sky and fro\underline{st} at night.
The band The Tap\underline{,} together with other perform\underline{ers}, has also recorded the so-called Hy\underline{m}ne against the world end, entitled "Welt\underline{unter}\underline{gang} f xe4llt aus".
In May we perform for the first time in the Prague Spring\underline{,} and for this concert we prepare an interesting programme with interesting guests.
Since 1956\underline{,} the PTA has been instrumental in the development of the extremely successful meteorological missile (Raki\underline{eta} Met\underline{e}orologic\underline{z}na), the first Polish rocket for scientific research.
In Germany, there have been public food levie\underline{s} for the poor for several years now, which are no longer able to feed themselves through their own work.
Then, however, one must ask oneself whether private capital is not influ\underline{en}cing, or even steering\underline{,} politics and thus the entire state in its own selfish sense.
We must therefore seek the cause of the emergence of fasc\underline{ism} and communism through the reck\underline{less} liberalisation of the economies of the 19th and 20th centuries\underline{.}
It was a severe blow to the reputation of the United States, and the subsequent fi\underline{as}co in the violent attempt to release hostage\underline{s} made things worse\underline{.}
I know that I cannot achieve anything on my own; that is why I have spoken to several well-known figures about whether they also wish to stand for the Senat\underline{e}.
"I find the building funny\underline{,} it looks fut\underline{ur}istic\underline{,} and finally there is something interesting to see again," says Lisette Verhaig, a passer-by on the roadside.
"Norm\underline{ally}, the books\underline{h}elf\underline{s} are located along the facade\underline{,} and in the middle there is a large dark room, which is mostly uncomfortable and impersonal\underline{,}" says Win\underline{y} Maas.
Deutsche Welle\underline{:} At the beginning of the week, Germany signal\underline{led} that it would vote against the request for Palestinian observe\underline{r} status at the United Nations.
Now the influence of the United States in European politics is steadily diminish\underline{ing}, but at the moment the EU is not filling this vacuum\underline{,} who else is there?
On September 14, 2010, a Chinese company had the Ze\underline{gna} DF Pu\underline{ma} trademark protected there, an art name that also served at the Ermenegil\underline{do} Ze\underline{gna} fashion house.
In fact, if Freud\underline{enberg} falls under the last act of his brand drama\underline{,} then one would probably have to pay royal\underline{ties} to the other side for his own name, explains Wentz\underline{ler}.
This is where the Cauc\underline{asia}\underline{n} Tal\underline{yan} population lives, of which not much is known, except that it speaks perfectly Persian and Azerbaijan\underline{i} and is very long lasting\underline{.}
"Ba\underline{ku} became famous in May with the Eurovision song festival - and next year we have a festival of the oldest people in the world", says Fatulay\underline{eva}\underline{.}
It is a matter of interpretation\underline{,} as much in the draft that Mur\underline{si} has signed and will, in his words, be presented to the Egyptian\underline{s} for referendum\underline{.}
The 48\underline{-}year\underline{-}old human rights lawyer and leader of the Egyptian Human Rights Organization (EOHR\underline{)} defended the Muslim Brot\underline{her}hood when they were in prison or on trial under Mubarak\underline{.}
Just a generation ago, thousands of Norwegian\underline{s} were forced to leave their country in search of work and migrate\underline{d} mainly to the US.
There is still hatred of naming Anders Bre\underline{iv}ik - the racist right-wing extremist who shot 77 men, women and children last year.
Earl\underline{ier} this year, the military intervene\underline{d} to combat drug gangs operating in quarter\underline{s}, and violence against women is a particularly acute problem.
Manning told the official that he could use the covenant of his underwear or flip flo\underline{ps} to hurt himself\underline{,} but not.
The defense has indicated that Manning will commit fewer offences for guilty\underline{,} while other charges that are considered too extreme are to be challenged.
The Pen\underline{t}agon maintains its position that Manning has been held in accordance with the provisions applicable to all prisoners under the highest security arrangements in Qua\underline{n}tico\underline{.}
And then we would not now be trapped behind the silk curtain - with a pleasant life in the United States, but somehow lost.
The Arab Spring has created a new, uncertain situation, and whether they like it or not, Palestinians and Israelis have become part of these turmoil\underline{s}.
"The government should simply have banned cigarette\underline{s} completely - then we would have told ourselves ok\underline{ay}, that's it, we're going to close," he adds vis\underline{ib}\underline{ly} upset\underline{.}
And because most of us nowadays almost constantly stare at one screen or another, we no longer benefit from bo\underline{re}dom\underline{.}
The key experience of bo\underline{re}dom\underline{,} he says\underline{,} consists in "dis\underline{tur}\underline{bing} the attention process, coupled with bad humour and the feeling that time is slow\underline{".}
However, he was certain that "the young are perceived to be particularly bo\underline{ring}", mainly because children and teenagers do not have much influence on their daily routine\underline{.}
"With bo\underline{re}dom\underline{,} the brain wants to tell you to do something else," says Gary Marcus\underline{,} professor of psychology at New York University.
According to Oroz\underline{co}, on a September day, he and some friends were travelling by car in Lama\underline{r} near the Kan\underline{s}as border when they were stopped\underline{.}
The only tut\underline{or} who was openly recognized as Tory was Norman Stone\underline{,} a professor of contemporary history who had his seat in my college\underline{.}
He was hated not only to be a conservative\underline{,} but also because he had consulted Thatcher on foreign policy and written speeches for them.
This exhibition is the conclusion of a story whose only protagonist is "il signore\underline{"} Gar\underline{ava}\underline{ni}, but which could not have been written without his distinguished clientele\underline{.}
"I prefer it to everyone else because of its great love for women and because it emphasize\underline{s} our beauty\underline{,}" adds the ex-duches\underline{s} of Feria\underline{.}
They know that every step can cost their lives, as happened to a French tourist who crash\underline{ed} years ago on the steep slopes of Kawah Ijen.
It takes three hours for each route\underline{,} after which it is completely accomplished\underline{,} but at the end of the day it will have 138,000 rupees (11,5 euros\underline{).}
What looks like a terrible reward for such an almost inhuman effort is three times what it would earn with the fieldwork\underline{.}
Def\underline{y}ing the shadow\underline{s}, he climb\underline{s} into the cra\underline{ter} in the light of a small forehead lamp on his helmet\underline{,} which he bought from his own money.
However, there is concern that they can promote the life style of the single man and that they discourage construction companies from building large homes for families.
If they understand all sections\underline{,} they have solid foundations to talk to their children about the importance of opening a user account on the Internet.
The President of Ecuador\underline{,} Raf\underline{a}el Correa\underline{,} confirmed today that the creation of common citizenship is an objective, with 'South America actually learning something from Europe'.
Power never interested me personally\underline{,} but in such unjust circumstances as Ecuador\underline{,} this socio\underline{-}economic poverty can only be corrected by political power.
The request, led by Carlos D xedaz Ch xe1vez Mor\underline{ine}au, has now brought a criminal case against the National Bank and Securities Commission, which is accused of obstruct\underline{ing} justice.
He was granted the master\underline{y} of Va\underline{quer}\underline{os} with Gausse\underline{,} but from a distance, because in 1988 he was at the top of the association\underline{.}
Born in Fort Worth, Texas\underline{,} he was the son of actress and singer Mary Martin\underline{,} who played classical works like "South Pacific\underline{"} and "Peter Pan\underline{".}
"I have not written anything that I thought could harm or affect someone wise\underline{ly}," said the Associate\underline{d} Press at the time.
I would like to give them some comfort, such as 'no fear\underline{,} it's a bit inconv\underline{en}ient the first time, but it will go well for you'.
In this sense, the majority of American governments have been promul\underline{g}ating new laws since 2009 that make the registration or ballot process more difficult.
This phenomenon has grown in importance following the November 2010 elections, with 675 new republic\underline{an} representatives in 26 states.
Another study, this time from Europe, concluded that there is a difference in the mortality of patients with and without early detection\underline{.}
Despite progress in research, adopting a healthy lifestyle remains the best way to reduce the risk of developing it.
We know without a shadow of doubt that we have a real new particle and that it is very similar to the Hi\underline{gg}\underline{s}-Bo\underline{son} projected by the standard model.
By the way: in the early 1960\underline{s}, the pioneer\underline{s} of the laser in the Bell Lab\underline{s} did not suspect that their work would trigger such a revolution\underline{.}
Of course, this does not mean that the activities of the LHC will inevitably change our lives, but it means that you really never know...
I hope that in May we will be the smil\underline{ing} winner and tell us that, despite all the difficulties\underline{,} we have finally won them.
Moreover, in its report, the ECB provides for the re-evaluation of the various risks that are now considered to be highly significant if this currency is to succeed\underline{.}
Jobs will have to be made available to these young people who do not want to return to the obscur\underline{ant}ism of the former parties or to the corruption of certain leaders.
Former commanders of the anti-Sovi\underline{et} struggle are already trying to restore the provincial militia\underline{s}, which will escape the power of the central government.
No mining is possible without energy to process the iron or copper ore on site or without means of transport to export over the mountains\underline{.}
One day, it will also be necessary for Afghanistan and Pakistan, on which imports and exports are largely dependent\underline{,} to restore normal relations.
Liberal\underline{s}' fears are also fuel\underline{led} by the fact that the next rector of this university should be much less moderate than the current one.
However, it acknowledge\underline{s} 'that there may be ambigu\underline{ity} with regard to Article 220\underline{,} since the terms used are derived from the religious vocabulary\underline{.}
As early as the day the law came into force, it turned out that it was not only the registration documents of migrants that could be fals\underline{ified}\underline{.}
For the moment, the authorities can only promise guest workers who fall through the test for the first time that they will receive time for a basic language course.
An open letter has been published on the Internet, the authors of which - representatives of various arms associations - call on the authorities to refrain from 'no senseless tight\underline{en}ing'.
The experts analyze\underline{d} reports from the Ministry of the Interior and the Federal Stat\underline{istic}\underline{s} Service, criminal literature and publicly accessible data on arms portal\underline{s}.
"As a response he receives a photo and a description of the hiding place of the weapon\underline{,}" reports the press officer of the non-profit organization "Pravo na oryzh\underline{ie}" Dmitrij Ki\underline{s}low\underline{.}
For example, the Xbox console and the Ki\underline{n}ect sensors are a step forward, and nowadays no Xbox is sold without Ki\underline{n}ect because everyone is interested in motion control.
This is what makes work in the field of virtual reality so attractive to a researcher: we are only at the beginning of many topics\underline{.}
Then the time of the old free but not officially recognized painter\underline{s} ended\underline{,} and new and free painter\underline{s} like myself were incomprehensible\underline{.}
It is not easy to work in new times according to old rules; I am a man of truth\underline{,} honest\underline{y} and culture of the last century.
In my youth I have painted such pictures\underline{,} which even in a series with the works of Falk and Lario\underline{now} were displayed by a collect\underline{or}.
In the real Tsar\underline{,} it was different, because the Tsar may not understand much about culture, but they understood that proper experts are needed.
"The more dangerous it is even on flights to orbit", conclude\underline{s} Kosmonaut Wal\underline{er}i Pol\underline{ja}kov\underline{,} hero of the Soviet Union and hero of the Russian Federation\underline{.}
He can say: 'We are changing the law and allowing things', but he cannot say that we are acting as if nothing were.
The procurement law contains relatively strict rules on the formal execution of certain transactions - and this is also right to protect public competition.
Through your foreign travels, you have a comparison of what is happening in individual countries with accessibility\underline{,} how to deal with disabled people, etc.
At that time I started as a caretake\underline{r} at the Jedli  u2047 ka Institute\underline{,} where I met many young people who were interested in getting involved with something intensive\underline{.}
I always say that if people with disabilities succeed\underline{,} this is not only a step forward for them, it is a step forward for society as a whole.
The result is a desperate situation in the area of corruption\underline{,} mutual preference and legislation in which practically everything is criminal but nothing is punish\underline{able}.
In Germany, the situation is that, due to a lack of finance\underline{,} a Ministry of State is instruct\underline{ing} private legal entities closely linked to industry to draft legislation.
All violence then no longer comes from the people, as the Western constitution\underline{s} proclaim\underline{,} but from strong financial groups that prefer their own interests.
The Bal\underline{four} Declaration\underline{,} which has already been mentioned, created the precondition for mass migration from Jews to Palestine\underline{;} first clash\underline{es} with the local Arab population took place.
At the same time, it was unable to secure the release of the hostage\underline{s} in Iran, where the revolution resulted in the establishment of a theocra\underline{tic} regime.
In order to make the camouf\underline{lage} credible\underline{,} articles on this film project were published in professional journal\underline{s}, press conferences were held and the fi\underline{ct}\underline{it}ious production company had a real office.
And then there are the scenes from the CIA headquarters and other institutions - men in suit\underline{s} at the meeting table, on the corridor\underline{s} of office, on the telephone...
My advantage is that I can take away from any party what is best for our country, without any drawers and party dogma\underline{s}.
Or do you think that if you talk to people long enough, you will be able to impose\underline{,} for example, material and criminal liability\underline{?}
I always try to judge things for myself\underline{;} and if it does not work, I will return to the private sector in six years' time.
But I could not live on the senator's salary alone; for example, I could not finance my son\underline{'}s English school, which costs 30,000 a month.
Has Germany damaged its relations with the US by abstain\underline{ing} on important decisions, such as the vote on Palestine\underline{?}
It would, of course, be a little easier for the Germans if there were a coherent and uniform European policy, which is not the case at present.
This is a record and means that China is running the list of new applications around the world for the tenth consecutive time, the authority informs.
But a year later, the choir founded the association "Voices for Africa", which since then has taken care of the AIDS orphan\underline{s} in Esitjeni almost professionally.
According to the Robert Koch Institute\underline{,} the number of sy\underline{phil}\underline{is} infection\underline{s} more than doubled from 1697 in 2001 to 36\underline{98} in 2011\underline{.}
Although it is closest to the sun, there is also frozen water, as indicated by three studies published on Thursday in the magazine "Science".
Nobody brings the discovery of ice but related to the existence of life on the planet\underline{,} said the chief scientist of the Messenger probe\underline{,} Sean Solo\underline{mon}.
This star-forming region - unroman\underline{tic}ly called W5 by scientists - has discovered the Spitze\underline{r} telescope in the Cassi\underline{op}eia starscape\underline{,} at a distance of 6500 light years.
The man had been married three times and had 23 children; at the age of 136 he was said to have witnessed a daughter\underline{.}
Mir\underline{za}yeva\underline{'}s white teeth are perfect in Reih and Gli\underline{ed}. Under her heads\underline{car}f she hide\underline{s} long, dark blo\underline{nde} bra\underline{ces} that her son proud\underline{ly} reveals\underline{.}
230 Manat (approximately the same amount in euros\underline{),} Mir\underline{za}yeva receives monthly as a pension\underline{,} for local conditions an amount of which you can live well.
Indeed, the 234 articles that have been pushed through by the Islamic\underline{-}dominated 100-member Constitutional Assembly in a nightly, 15-hour pardon are sometimes worrying\underline{.}
Saeda feels abandoned\underline{,} even by the international community, which views the ideological struggle for direction on the Nil\underline{e} with a mixture of curiosity and tension\underline{.}
Norway has been very careful about its oil wealth - a large proportion of industry revenues are invested in a special fund for the benefit of future generations\underline{.}
In the years leading up to the global economic crisis, when everyone was throw\underline{ing} money that they did not own, Norway kept its wall\underline{et} firmly closed.
"My government is strongly committed to reducing violence," Pen\underline{a} Nie\underline{to} told US President Barack Obama at the Oval Office earlier this week.
Congress\underline{man} Ol\underline{ver}a admit\underline{s} that after 12 years outside the presidential palace of Los Pin\underline{os}, the party has great expectations of Enrique Pen\underline{a} Nie\underline{to}.
Irinea Bu\underline{en}dia fights with tear\underline{s} in a concrete building, typical of the depressed quarter\underline{,} when she shows me photos of her decea\underline{s}ed daughter Maria\underline{na} Luna.
Hosni Mubarak\underline{,} the secular despot that ruled Egypt for 30 years until his fall in 2011\underline{,} had little time left for Hamas\underline{.}
In diplomatic terms, the United States remains ste\underline{ad}fast in its position, and many European countries have blame\underline{d} Hamas for the latest escalation\underline{s} of violence.
Net\underline{an}yahu is doing well, and his Likud party has allied itself with an even more bell\underline{iger}\underline{ent} group in the run-up to the January 22 election under Avig\underline{dor} Liebe\underline{r}man.
On social media such as YouTube\underline{,} Twitter and Facebook\underline{,} Freeman has noticed an increase in brand experience reports written by "normal people".
James Yu\underline{,} the tobacco trade's "King of the Pack\underline{"} operator in downtown Sydney\underline{,} says that uniform packaging has made it difficult to fill up its shelves\underline{.}
This thanksgiving I spent unexpected\underline{ly} five hours at the airport when our plane was out due to mechanical problems and we had to wait for another plane\underline{.}
"Studie\underline{n} haben gezeigt, dass Kinder, die herum\underline{ha}mpel\underline{n} d xfcrfen\underline{,} mehr lernen und mehr Informationen behalten als diejenigen, die zum Still\underline{sitz}\underline{en} gezwungen werden," so Professor Fenske.
Chief Oates added that the police would continue to enforce urban regulations on mar\underline{i}juana growers and continue to pursue drug traffickers\underline{.}
Valentin\underline{o} presents these personal memories as troph\underline{ies} of his social rise from the modest fashion\underline{maker} in the city of Vo\underline{gh}\underline{era} in northern Italy to the idol of the international jet\underline{set}\underline{.}
"At least they don't show their til\underline{ts} on your beautiful carpet\underline{,} as some of the beautiful celebrities from pop music do," says Baroni\underline{n} Fiona Thyssen\underline{-}Bornemis\underline{za}.
"All invite\underline{es} felt important and loved\underline{,}" recall\underline{s} the "Top Model\underline{"} that began their career at the week of Haut\underline{e} Cou\underline{ture} in Paris in 1995.
"Val\underline{en}tino does not depend on fashion\underline{,} its obsession is timeless," explains this Italian aristo\underline{cra}\underline{t} who lives between Par xeds, New York and Bueno\underline{s} Aires\underline{.}
The grand finale of the exhibition in Somerset House is Marie\underline{-}Cha\underline{n}tal Mill\underline{er}'s wedding dress for her wedding with Pablo de Gre\underline{cia} in 1995.
The Singapore\underline{ans} blame their lack of children for the career\underline{s}, stress, and cost of real estate and child-rea\underline{ring}.
Their creative director Douglas Hamilton says that he wanted to use the power of music to get people to do their "national duty".
We are the worst in the world when it comes to reproduction\underline{,} so we realised that it was an issue we had to deal with.
We knew that the government had tried a lot, such as marketing perfume\underline{s} with pheromons or organizing speed dating evenings (fast flirts).
Meanwhile\underline{,} an immigration policy aimed at a dramatic increase in immigration in order to counter\underline{act} the reduction of the population has led to res\underline{ent}ment among the local population.
When asked about the text, they said that the content was presented to the press by the President of Peru\underline{,} Ollanta Hum\underline{ala}\underline{.}
"We will follow and execute the judgment on the differences that we are currently bringing to this international court\underline{,}" said Hum\underline{ala} and his Chile\underline{an} counterpart\underline{.}
"We will review all these avenue\underline{s} - they are not exclusive\underline{,} and the agreement with Nicaragua also requires talks with Nicaragua\underline{,}" he stressed\underline{.}
There are huge gap\underline{s} between health programs and ordinary citizens, explains Rica\underline{r}do Salazar\underline{,} journalist from Gua\underline{dal}\underline{aja}\underline{ra}, who has taken up the cause of HIV\underline{.}
It is estimated that 50,000 people live with HIV because for each registered case there are 4 or 5 people who do not know.
In an effort to pay long-term liabilities without affecting short-term liabilities\underline{,} the building company Homex launch\underline{es} stock certificates of more than 500 million pesos on the market.
I like to listen to music, watch videos of music of my time in YouTube\underline{,} enjoy my grand\underline{child}\underline{ren} and occasionally go to a basketball game.
Larry Hag\underline{man}, whose role as the oil magnate J.R. Ewing in the television series "Da\underline{lla}\underline{s}" became a symbol of the gre\underline{ed} of the 1980\underline{s}, is dead\underline{.}
The couple had two children, Preston and Heidi, and they lived for a long time in the California\underline{n} town of Mali\underline{bu}\underline{,} where many celebrities live.
If someone analyses what has happened in the world today as if we were thirty days away from it, it would be a really good period.
"In two hours there were no more places" said Restall about his course for high average students, who filled up with 35 students.
The measures adopted since 2009 have reduced the share of the registration of new voters by 17\% in 2010 compared to 2006.
At this stage, the doctors and nurses who care for them will no longer overwhelm them with so-called 'healing' care.
"I have no more desires in life," she says\underline{,} before accepting that she should be put on a mask to help her breath\underline{e}.
After Elsie Mon\underline{er}eau\underline{,} head of pal\underline{li}ative care for the home pal\underline{li}ative care company of the Montreal metropolitan area, 8\% of patients do not call for pain treatment.
In addition, the police of the "Mar\underline{teau} force" who, since 2009, has caused the "Can\underline{al}isation Cartel" of Montreal to be more cautious about the artificial increase in contracts\underline{...}
The next on the list would be Gill\underline{es} Va\underline{illa}\underline{n}court\underline{,} who has just resign\underline{ed} from his position as Mayor of Laval\underline{,} Quebec\underline{'}s third largest city.
From my early days at the centre of the preparato\underline{ry} training of the IN\underline{F} Cla\underline{ire}\underline{fo}\underline{n}tain\underline{e} up to my time at Saint\underline{-}Etienne\underline{,} I have always made step-by-step progress.
Would it be a great failure not to win the title in Ligue 1, as was the case last season?
It describes Bit\underline{co}in as "the virtual currency with the greatest success", "in competition with the dollar or euro" and "simil\underline{ar} to conventional currencies\underline{".}
Many young people want to leave the country, just like those who have benefited from American subsidies\underline{:} capital flight is considerable\underline{.}
All, including the armed parties, are obsessed with mobile phones\underline{;} television with its Turkish series, which represent a modern world, is everywhere\underline{.}
A very short period of time forcing the brother\underline{s} to abandon their plan to explain the text section by section to the Egyptian\underline{s}.
It is also a way for the president to regain his public and democratic legitimacy while the protest ra\underline{ges} throughout the country.
After reit\underline{er}ations in an interview with the American weekly show Time\underline{,} Moham\underline{ed} Mor\underline{si} seems convinced that Egyptian\underline{s} will be benevol\underline{ent}.
A journey within the city costs 6 skel\underline{es} regardless of the means of transport, including a transfer for a journey of up to 1.5 hours.
The Russian police know that most of our documents are forged and we are not registered\underline{,} and this leads to blackmail.
In doing so, the authorities are responding to recent events: injuries at shooting\underline{s} at wedding\underline{s} and seven deaths at the barrel of the Moscow lawyer Dmitri Win\underline{o}grad\underline{ov}.
"There is evidence that some cases were arson in order to cover up the absence of weapons\underline{,}" says the former militaryman.
As a potential customer, I do not just buy, but drive into the woods with the seller\underline{,} where we set up a target.
Viktor Baranez emphasize\underline{s} that when you place a request on a website, you can go out empty at the end and come behind bars\underline{.}
McDonald\underline{'}s says the company sell\underline{s} billions of portion\underline{s}, yet you are not given sick\underline{ness} days and you are not paid for your honest work!
The theme of expanded reality, which is popular among supporters of modern technologies, has been usually perceived lately by the lens of a special eye\underline{glas}\underline{s}.
Until now, humankind has largely remained stuck in the phase of working with pixels on flat screens, which are sometimes touched.
- Does this mean that you want the user to adapt to what a machine can and cannot afford at the time?
- Ki\underline{n}ect currently works with three "cam\underline{era}\underline{s}", one of which is actually an infrared transmit\underline{ter} and the other a receiver for the reflected signal\underline{.}
- In my lecture\underline{s} I often speak of the fact that expanded reality is the seventh breakthrough in the interaction between man and machine.
  u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047    u2047 .
"Th\underline{at} was just with the bio\underline{satellit}\underline{es}, but again it was only a single experiment\underline{,} and the research must continue," Vladimir Sy\underline{che}w noted\underline{.}
In a state of weight\underline{lessness}\underline{,} the muscle\underline{s} of the abdom\underline{en} and the pelv\underline{ic} system are rapidly reduced and the ability to squeeze out the child decrease\underline{s}.
Recently\underline{,} the Prime Minister said that the ODS would not harass entrepreneurs with controls - is the system now banned or permitted\underline{?}
The law will never be perfect, but it must be applied properly - and that is what I believe we lack.
Road\underline{s} in the Pil\underline{s}en district are now easily accessible\underline{,} but local attention is required and the way of driving is adapted to the weather\underline{.}
The road from Tel\underline{n}ice to Kn xednice is closed in   u2047 st xed n.K. according to traffic police.
The road between Tel\underline{n}ice and Kn xednice was blocked because of branches pressed from the snow to the road.
Five of our members are wheelchair users, i.e. wheelchair\underline{s} must be carried in the luggage compartment and, of course, we must carry many instrument cases and other luggage\underline{...}
At that time, there were already the first satellite technology projects and it was foreseeable that space exploration would have a future.
Three types of this missile were developed (Me\underline{te}or-1A, -1B and -1C), which differ\underline{ed} from each other in the size of the transport space for scientific instruments.
This is due to the principle of free trade and the free, unrest\underline{ric}\underline{ted} movement of private capital, which goes hand in hand with unbri\underline{d}led financial speculation\underline{.}
Lobby interests were also behind the fact that banana\underline{s} of the highest trade class in the EU must be at least 14 cm long and must not have a cur\underline{va}ture anoma\underline{ly}.
The EU thus established the maximum volume of food stocks in the territory of the Czech Republic on the day we joined the EU.
It is part of a revit\underline{al}ization project, which also includes underground parking, supermarket\underline{,} post office and a few adjoining houses with a total of 50 apartments.
There is a lift that runs through the middle of the mountain massif, but the true moments of reading and space are opened up by climbing the topography on foot.
Like Plu\underline{to}, which circle\underline{s} around the sun behind Nept\underline{une}\underline{,} Cer\underline{es} is not a "Planet\underline{"} according to the new definition of the International Astronom\underline{ical} Union of 2006.
The interior of the Gran Tele\underline{sc}\underline{op}io Canaria on the Canary Island of La Palma is huge - the mirror alone comes to 10.\underline{4} metres in diameter\underline{.}
Rub\underline{aba} Mir\underline{za}yeva lives in Cengemir\underline{an}, a tiny settlement near the town of Lerik\underline{.}
But the cult being driven around the nation u2019s father\underline{,} who ruled his country like a dictator\underline{,} knows little bound\underline{s} in Azerbaijan\underline{.}
He almost apologized, Mohammed Mor\underline{si} said, temporarily curtail\underline{ed} the powers of the Constitutional Court and broadened his powers 'to save the revolution\underline{'}.
That does not have to be the case, but it may mean that cl\underline{er}gy supervise\underline{s} legislation, which would de facto disenfranc\underline{h}ise the judiciary\underline{.}
The state should also, as it states in the draft, 'protect the true essence of the Egyptian family' and 'promote its moral\underline{ity} and values'.
However, the aim was not to disrupt commut\underline{ers} on their way to work, but to prevent demonstrators from reaching Parliament.
On a shedland near a large landfill site, the bodies of dozen\underline{s} of murdered women have been left behind in the last two years alone.
The US Army intelligence analyst, arrested in June 2010, is accused of steal\underline{ing} thousands of confidential documents during his service in Iraq.
Manning said that he had tried to stay on the move, because the day was forbidden to sleep or even to sit down.
When he turned around at night and guard\underline{s} could not see his face, he was wake\underline{n} up to turn back.
Just as Islamist\underline{s} have gained influence in the Arab world, Hamas has been able to pull powerful and rich friends alongside them.
In future diplomatic negotiations, Hamas may prove to be a player that cannot be pushed out even by Israel and the United States.
No, it is better to keep them in check behind the wall and punish them if they dare to raise their heads\underline{.}
Op\underline{pression} is already undermining democracy in the Jewish state, and the growth of the Arab population will only exacerbat\underline{e} this situation.
Like many people, I have always assumed that bo\underline{re}dom is a relatively recent phenomenon that has developed with increasing leisure time.
"Our authority has a duty to prosecut\underline{e} offences that were crimes at the time of the crime," Buck stated in a statement.
And the conflicting reactions across the state have revealed a deep division among local officials about the great green experiment\underline{.}
Color\underline{ado} and Washington are the first states to treat small quantities of mar\underline{i}juana like alcohol as national models for the legalisation of drugs\underline{.}
The 20-year\underline{-}old Luke Black\underline{,} Vice\underline{-}President of the conservative student association of the University of Nottingham\underline{,} said in a Sunday newspaper\underline{:} "There is a growing left-wing tendency in universities\underline{.}
Last year, the university voted not to grant an honor\underline{ary} title to Margaret Thatcher, a former student\underline{,} because of cuts in higher education.
In the first days of the first semester week, when new students get to know each other and the tut\underline{ors}, I got a foretaste of what will happen.
It is bad enough for me, but they know that your father is close to Margaret Thatcher, so it will be worse for you.
The prince\underline{s}s and leader of the fashion patri\underline{cia} della Giovampaola d'Ar\underline{enberg} cannot forget for the first time when she was wearing a Valentin\underline{o}.
When I was a teenage\underline{r} in Italy, I dream\underline{t} of finally having the age and the opportunity to wear one of his evening dress\underline{es}...
So we thought: why do we not do something as creative as possible to address this problem, such as comp\underline{os}ing rap\underline{?}
Singapore is a rich, high-tech city-state in south-east Asia, also known for the conserv\underline{at}ism of its rulers and its strict social controls\underline{.}
Tan Wei Ming, director of the National Pop\underline{ulation} Authority\underline{'}s marriage and family policy, says that this is due to 'bett\underline{er} education' and 'gre\underline{at}er career opportunities'.
"The people are very stressed\underline{,} the homes and education are expensive\underline{,} which is why many people are pushing it out" says a young manager\underline{.}
That is why the Singapore\underline{ans} have the last word when it comes to having children - the government can still do so much.
Is he aware of the dangers that he is exp\underline{os}ing himself by making known on the Internet situations that he would not share in real life?
"The Internet was created as a medium for the search for information, but with the appearance of these pages the rules of the game changed," she says\underline{.}
The summit was attended by the president\underline{s} of Brazil\underline{,} Dilma Rou\underline{s}eff\underline{,} Venezuela\underline{,} Hugo Ch xe1vez, Bolivia\underline{,} Evo Moral\underline{es}, and Argentina\underline{,} Cristina Kirch\underline{ner}.
'We hope that the electoral process in that country will serve to reopen it into the Union of South American Nations,' from which it is currently excluded\underline{.}
"I hope to be able to tell President Ortega that we will treat this matter as civilised and respectful as possible," Santo\underline{s} added.
"The greatest enemies of press freedom are not the evil and perverse politicians\underline{,} but bad journalists who seek and blackmail profit\underline{,}" he said.
"My political movement believed that it was I who guaranteed this likely victory\underline{,} so I must fulfill that responsibility," he said.
He is undoubtedly one of the oldest patients of the HIV unit of the Hospital Civil de Gua\underline{dal}\underline{aja}\underline{ra} (HCG), into which he came after several struggle\underline{s} in 1994\underline{.}
However, the decision opens the door to the largest glass manufacturer in Mexico to refer three inconsistencies to the United States Supreme Court.
"Larry was back in his beloved city of Dal\underline{las}\underline{,} where he played the icon\underline{ic} role he liked most," said the family.
The dramatic series of the CBS TV chain about the Ewing cl\underline{an} and other characters around it was broadcast from April 1978 to May 1991\underline{.}
In addition, Republican legislators in five other states have passed laws aimed at shortening the period for early voting.
There is an inevitable law in this world that prevents two objects from being in the same place at the same time.
It is not possible to break this rule - and do not try too much because you will hurt\underline{.}
The same applies to the Hi\underline{gg}\underline{s}-Bo\underline{son}, with the difference that another field, the Hi\underline{gg}\underline{s} field, must be "destruct\underline{ed}" for this bo\underline{son} to appear.
The disease does its job: an immense weakness prevents him from going to the toilet and even eating himself\underline{.}
Other road construction officials have admitted that they have let themselves be flat\underline{ten}ed by artificial\underline{ly} inflat\underline{ing} the bill\underline{s} by 30-40\% with false additional services.
Given what has been invested and the players we have, it is normal that much is expected of us.
The bitcoins in circulation are therefore limited to 21 million, but are divisible to a hundred mill\underline{i}metre\underline{s}, which leaves some room for manoeuvre\underline{...}
For his opponents\underline{,} the President persist\underline{s} in his "auto\underline{cra}\underline{tic} delirium\underline{"} by continuing to "break his word" and "rules the law underfoot\underline{".}
In addition to its religious aspect\underline{,} the text adopted yesterday is strongly criticised for the wide-ranging powers it grants to the President of the Republic.
While MEPs and civil rights activists are discussing the benefits of the law on compulsory language tests for migrants\underline{,} criminals are already trading in counterfeit certificates\underline{.}
A law came into force on 1 December, according to which every migrant worker must pass a test cert\underline{ifying} knowledge of the Russian language.
This law also exclude\underline{s} persons who received their training certificates and diploma\underline{s} prior to the collapse of the USS\underline{R} in 1991\underline{.}
"Man\underline{y} talk about protecting the rights of migrant workers," says the head of the representation of the Federal Migration Authority in Taji\underline{k}istan\underline{,} Viktor Sebelev\underline{.}
Baranez explains that these include weapons stolen from both police and law enforcement staff.
"The dealer brings the weapon to the city and sell\underline{s} it there for 900 euros per piece with two magazine\underline{s}," he says\underline{.}
Former militaryman Viktor Baranez tried to buy illegal weapons in the mid\underline{-19}\underline{90}s when he wrote an article on the subject.
According to Dmitry Ki\underline{s}low of the organization "Pravo na oryzh\underline{ie}" you can buy a Mak\underline{a}row gun for \$100 to \$300\underline{.}
Advoca\underline{tes} of Wal\underline{mar}t are pleased to note that protests have occurred only in nine states, and that they have not caused any losses to the company.
- Although Ki\underline{n}ect has put interaction on a physical level, much still plays out on the flat screen, sometimes in 3D.
Do you not think that in terms of applying the technology of the enlarged reality in everyday life, glass\underline{es} have the best prospects\underline{?}
In order to save humanity\underline{,} the important question arises as to how we can reproduce in weight\underline{lessness} or on the replacement planet\underline{?}
Given that this amendment is only in force for a short period of time, it has not yet had an impact on our audit\underline{s}.
The Prime Minister said recently that the ODS would not bury entrepreneurs with controls on the so-called 'black\underline{'} system - what exactly does that mean?
On the other hand, however, it is also tragic if the bid\underline{der} with the best offer is excluded solely because of formal errors\underline{.}
The text of the anthem is written by Tom xe1  u2047  Han xe1k, who also plays the main character of Jesus in the video clip\underline{,} Xi\underline{nd}l X sing\underline{s} with...
Moscow is not accessible to people with disabilities in comparison to Prague\underline{,} where it is still unusual for people in wheelchair\underline{s} to travel alone in the city centre.
The first mention of this company was made in 1954 in the November issue of Problemy, in which four major articles are devoted to space travel.
Since private capital has no social responsibility and therefore no responsibility for the unemployment it causes\underline{,} public expenditure is necessarily increasing.
Private capital, by its very nature, is unable to recognise and enforce the benefit for the whole of society.
"If my son\underline{s} did not want wars, there would be none\underline{,}" says Mayer Amschel Roth\underline{schild}\underline{'}s dying good beaker, wife\underline{,} in 1849\underline{.}
From a smile\underline{y} actor has become a respectable director\underline{,} and even as an actor he is no longer the target of iron\underline{ic} remarks\underline{.}
The feeling for the atmosphere of the place was one of the features that the director\underline{'}s previous films had removed from the standard Hollywood\underline{.}
The European Commission defended itself by arguing that it only harmonize\underline{s} the inconsistent national standards that would hinder trade.
He argued that the harvest was very high and that the state camps were overcrow\underline{ded} as a result of the so-called intervention purchases.
Later on, I clarified this and said that I would stand for the office of President if I were elected as a senator.
Then there are the media who want to deprive you of honour and who confuse the freedom of the word with freedom.
Six\underline{ty} per cent of the electorate did not go to the elections at all, and those who went mostly elected representatives of the establishment.
The fully gla\underline{z}ed interior is bright and clear, the burn\underline{ed} clink\underline{er} floor and the elegant street lantern\underline{s} speak the language of a public square\underline{.}
During the Libya\underline{n} uprising in March 2011\underline{,} Germany also abstained when it came to establishing a no-fly zone\underline{.}
If you look at relations between Obama and Prime Minister Net\underline{an}yahu, Obama is not so keen on Net\underline{an}yahu u2019s policies.
If, for example, we look at the euro crisis, every time Germany takes on a greater role, various anti-German feelings become clear.
Pat\underline{t}loch reports of cases where the court dismiss\underline{ed} complaints because, after the long period of time, the dispute\underline{d} name had become "market reality".
Fashion manufacturer Lacost\underline{e} lost in China against counterfeit\underline{ers} from Hong Kong and Singapore who turned the famous cro\underline{co}dile in the other direction.
The Robert Koch Institute assume\underline{s} that at least four out of five cases of sy\underline{phil}\underline{is} reported in Germany are transmitted through sexual contact between men.
The spread of HIV among het\underline{ero}\underline{sexual} adults is comparative\underline{ly} small in Germany - nevertheless\underline{:} this group accounts for approximately 20\% of new HIV infection\underline{s}.
Among other things, this state-san\underline{ction}\underline{ed} form of life is due to the fact that the HI virus has spread so rapidly in recent decades\underline{.}
However, the findings could help clarify how water and other building blocks of life have moved to other areas of the solar system.
The telescope is said to have been invented by Hans Lipper\underline{he}y in 1608 - even before Galileo Gali\underline{lei} used it for star observation a year later.
Here is documented the vita of about eight dozen Talyschen from the area, over 100.
His speech was addressed to the whole people, but above all to the Christian Cop\underline{ts}, the liberal\underline{s}, enlightened Muslims and secular\underline{s}.
This is so vague in legal terms that state institutions could even control the content of film art and literature with the help of this article\underline{.}
Hafez Abu Saeda is fur\underline{ious} about this forced constitutional process, which should have gone until February and involved all social forces.
The five million inhabitants of Norway enjoy one of the highest living standards - not only in Europe, but throughout the world.
Today, the population is growing rapidly - more than 13\% are immigrants\underline{,} attracted by a thriving labour market, high wages and comprehensive health care.
Since the early 1970 u2019s, the growth of one of the world u2019s largest oil and gas industries has been largely responsible for Norway u2019s current wealth\underline{.}
The agenda included all the issues that are expected when the heads of these two countries meet: immigration\underline{,} drugs and trade.
If they really had control of the West Bank, would they not launch rocket\underline{s}, just like their Gaza counterpart\underline{s}?
The hope - small for the near future - is that the ceasefire will give outsiders more influence to enforce this solution.
"It sounds like we need to be bo\underline{ring} more often, but bo\underline{re}dom is the tormenting, uncea\underline{s}ing desire to do something meaningful\underline{,}" he says\underline{.}
The room was very clean and comfortable.
The author A N Wilson gla\underline{mor}\underline{ous}ly stated that I had left the university because I was forced to drink from damaged cup\underline{s}.
I started commut\underline{ing} between Oxford and the home of my parents and found refuge with more open-minded friends and family in the city.
Despite the fact that I sh\underline{atter}\underline{ed} in shame\underline{,} I admitted that my parents had subjected me to brain\underline{wash}\underline{ing} and called it "old trump\underline{et}".
A government package for couples and parents grants up to \$1\underline{5,000} per child, extends maternity leave and distribute\underline{s} tax benefits.
But Lim Yew Soon, Director General of EL Developer\underline{s}, says that his "shoe boxes\underline{"} can be sold much faster than larger housing units\underline{.}
Por\underline{ras} then mentions some possibilities\underline{:} There are things you wouldn't tell a strange\underline{r}, why do you do it on the Internet?
Paraguay\underline{,} which has been excluded from the Unasur since 2011 after the removal of its president\underline{,} Fernando Lugo, has not taken part in the meeting.
He added that at the time there were 'founded assumption\underline{s} that Assange would be extradited to a third country and that his procedure would not be followed'.
This month, students analyze\underline{d} films with apocalyptic content and explore\underline{d} how to compare them with real life.
But none of the students survey\underline{ed} - and less a professor - said they believed in the last date of 21 December.
Over the past two years, they have promoted bill\underline{s} in 34 states that force voters to show a photo ID\underline{.}
Indeed, 11\% of US citizens, that is to say 21 million eligible people, do not have a photo ID issued by a government authority of their state.
Moreover, Republican legislators promoted laws in eight states in 2011 that abolished registration of voters on election day.
Of course, the democratic legislators and their supporters have strongly opposed the adoption of laws that restrict the registration of voters\underline{.}
This document (current\underline{ly} only in English, but a translation will soon be available) can be downloaded at http://ca.mov\underline{e}mber\underline{.}com/fr\underline{/}mens-health\underline{/}prostate\underline{-}can\underline{cer}\underline{-}screen\underline{ing} .
Encouraging data: 10 years after the ce\underline{s}sation of the cigarette\underline{,} the risk of dying of cancer is reduced by half.
In addition, Mr Beau\underline{lie}\underline{u} stresses the importance of talking to his doctor about his concerns and his pre-family burden\underline{.}
The permanent anti-cor\underline{r}uption unit\underline{,} launched in 2011\underline{,} is also making great efforts with its troops to government auditor\underline{s}, agents\underline{,} and analysts.
It is a piece\underline{me}al file, i.e. convert\underline{ing} a large file into a shorter and unique electronic fingerprint\underline{.}
It exhibit\underline{s} the collection of works by impression\underline{ists} and expression\underline{ists} Mon\underline{et}, Pissa\underline{ro}, Renoir, C xe9zanne\underline{,} Sisley, Mat\underline{isse}\underline{,} Mod\underline{iglia}\underline{ni}, Cha\underline{ga}ll and Picasso\underline{.}
By the way, this unusual sea, with a location of 417 metres below sea level, is the deepest sea in the world.
Migrant\underline{s} can test in all cities; already more than 160 centres have been opened in Russia.
The percentage of crimes with registered weapons is very low, according to the criminal law firm\underline{,} Vivili\underline{y} Les\underline{ni}kov\underline{,} the Russian service of the BBC\underline{.}
There are five such main channels\underline{,} says a former Colon\underline{el} Viktor Baranez, who worked for ten years in the Ministry of Education and the General Staff\underline{.}
"Peo\underline{ple} come like hungry fish to feed and then land in Siberia\underline{'}s labour camp and be allowed to snatch coal\underline{,}" he says\underline{.}
In addition to raising modest wages for simple Wal\underline{mar}t and fast-food workers, protest organize\underline{rs} pursue the goal of establishing trade unions\underline{.}
The gesture\underline{s} were not recorded by the object camera, but by a bra\underline{ce}let register\underline{ing} the movements of the bone\underline{s} and muscle\underline{s}.
There are also ri\underline{bb}\underline{ons} for the wrist that affect the nervous end of the finger\underline{s}, which is also a potential direction.
- Kir\underline{ill}\underline{,} why are you always in red and not in yellow or tur\underline{qu}\underline{ois}\underline{e} in the city?
Many were born there: N.O.M., Tequilajazzz\underline{,} and I also remember how cord came there with his project "Ucho Van Goga".
We need a cultural breeding ground because, for example, we now have more writer\underline{s} than readers\underline{,} and that is not right.
However, while the conditions on Mars are comparative\underline{ly} life-friendly\underline{,} the surface of Venus has a temperature of 500 degrees\underline{.}
In 1979\underline{,} qua\underline{il} eggs were sent into space to explore how weight\underline{lessness} affects embr\underline{yo} development.
From the main routes as well as from the road I/13 at the border of the districts   u2047 st xed n.L. and Lib\underline{er}ec bad traffic conditions are reported\underline{.}
For the establishment of the barrier\underline{-}free educational centre Stu\underline{de}o, which we have been working on for six years together with the association Tap at the Jedli  u2047 ka Institute\underline{.}
It is true that cooperation with well-known singer\underline{s} has helped us; moreover\underline{,} we have also started to actively promote us.
If you want to do something good, you cannot compromise on many things and also have to demand a certain degree of discipline\underline{.}
Poland started a close cooperation with ESA in 1994 and participated in several ESA projects over the following years.
Further space articles appeared in the Polish press after the war thanks to the work of the Polish Space Company (Pol\underline{ski}e Towar\underline{zy}\underline{s}two Astro\underline{nau}\underline{ty}cz\underline{ne}).
The liberal economic systems in the EU and in the globalised world are based on the principle of unreg\underline{ulate}\underline{d} economic competition.
A world in which every newborn child is implant\underline{ed} a chip at birth to subject this being to total control.
The film Argo by director and actor Ben Affleck describes an episode of this story that gave the US a small partial victory\underline{.}
Argo is his third feature film after the Krim\underline{i} Kein Kinderspiel (Gone Baby Gone, 2007) and the Th\underline{r}iller Stadt ohne Gnade (2010\underline{).}
Among the absurd\underline{ities} nominated\underline{,} for example, is the judgment of the European Court of Justice on the standardisation of insurance tariffs for men and women.
In the past, there has also been criticism of the factual ban on the use of the term 'butter\underline{auf}strich\underline{'} or the ban on the sale of conventional light bulb\underline{s}.
I have told myself all the time that I will start the battle for the castle after the result of the Senat\underline{e} elections.
I started my candida\underline{cy} on the condition that people are deeply dissati\underline{s}fied, but now I am no longer sure.
And so the city father\underline{s} recognized that there was only one way to master the statistics\underline{:} a library had to be made!
"You wouldn't believe it, but despite the many glass surface\underline{s} this house is a flagship project in terms of eco\underline{logy}\underline{,}" says Tro\underline{ub}orst.
For the time being, the optical gap\underline{s} in the library - currently 70,000 pieces - are to be filled\underline{.}
It shows the willingness to adopt positions that are independent of those of the United States or of European partners in the case of national interests.
Germany u2019s economic interests differ to a certain extent from those of the other major powers, and so Germany must protect its interests.
It must therefore be careful not to offend the public, but also the elite\underline{s}, in the Arab countries.
Szabo is also a member of the German Marshall Fund, where he specialize\underline{s} in German politics\underline{,} US foreign policy and transatlanti\underline{c} relations.
If the plain\underline{t}iff is unluck\underline{y}, he would even have to pay the pla\underline{gia}\underline{r}ator money because he violated his brand in China, says Pat\underline{t}loch\underline{.}
The CTMO Trade\underline{mark} Office in Beijing admitted that there were bottle\underline{n}eck\underline{s} in 2010 due to insufficient personnel and space equipment.
The internal costs could hardly be quant\underline{ified}\underline{;} the company archive even had to look through a hundred years old files to provide evidence\underline{.}
Then the voices of the singer\underline{s} slowly grow up - old, bass\underline{,} tenor and sopra\underline{no} - invade, begui\underline{ling} and persecut\underline{ing} themselves.
And Fiete Hopf\underline{,} the 29-year\underline{-}old conductor\underline{,} lift\underline{s} it almost from his cloth shoes when he brings them together with his smooth wild gesture\underline{s}.
More than forty percent of Swaziland's people carry the immun\underline{o}def\underline{ici}\underline{ency} virus\underline{,} dying at mid\underline{-}30 is no ra\underline{r}ity.
The probe messenger has found evidence that there is an ice sheet in the permanently shadow\underline{ed} region of the planet\underline{.}
For 30 years, from 1947 to 1975\underline{,} the Hal\underline{e} Tele\underline{scope} in the Pal\underline{o}mar Observatory near San Diego was the largest telescope in the world.
The small town is protected by a steep Soviet\underline{-}era architecture that does not want to fit into the picturesque mountain landscape\underline{.}
"We are not tired yet, the blood of our brother\underline{s} is not yet atonished\underline{,}" the Egyptian media quoted opposition politician Cha\underline{led} Ali\underline{.}
"And now the word human rights does not even appear in the new constitution\underline{",} he complain\underline{s} in conversation with the "World on Sunday\underline{".}
In the deepest winter it was then taken out after long fer\underline{ment}ation and consumed\underline{,} no doubt with the help of alcohol\underline{-}dam\underline{aging} senses.
In particular, as far as security and the economy are concerned, we hope for an interesting and real change that our country so desperately needs.
In Nezahualcoyo\underline{t}l, also known as Ciudad Neza, the contrast with the pave\underline{d} streets of Valle del Bra\underline{vo} could not be greater.
Pen\underline{a} Nie\underline{to}'s critics believe that he has at least failed to address the issue of women's murder\underline{s} during his term in office.
"They wrote (after discussing the concerns) "No problems," and that did not necessarily mean that I said nothing at all," said Manning.
An ethnic abbreviation - just as my friends in Boston call themselves 'Iren' or my friends in New York 'Italy'.
Israel has done well in recent years, particularly under Prime Minister Bin\underline{ya}min Net\underline{an}yahu, who has largely ignored the peace process.
'In an environment in which we are constantly being over-sti\underline{mul}\underline{ated}, it is difficult to worry once the noise is silence\underline{d}'.
But Smith also admit\underline{s} that no place or system can do more than serve as a rough guide\underline{.}
After the vote, he said that his authority would continue to pursue cases of mar\underline{i}juana ownership\underline{,} mainly to induce consumers to withdraw\underline{.}
Before the election day, some local authorities approved mor\underline{a}toria for new mar\underline{i}juana shops\underline{,} although they could only open in about a year.
We are guided by what the municipality has chosen and not by what the state has chosen\underline{.}
The last time this rate was above 2 - known as the replacement rate - was in 1976\underline{.}
"It is important for me to have my own money and time," says another man about twenty years old.
Or: Would you like to have a photo of you published, like the one you've published by a friend\underline{?}
"Every\underline{one} outside the Internet acts with respect, moral\underline{ity} and other principles, and the same must apply to social networks," he explains\underline{.}
Estuardo Guard\underline{ia}, university professor\underline{,} primary school teacher and educ\underline{ator}, comments that it is essential that parents read carefully the guidelines of social networks.
During the day, only the picture of the Presidential Meeting without sound was transmitted in the press room with the message "private session\underline{,} restricted audio\underline{".}
We are not dealing with human rights, we are not applying that word in this case, but there have been constant discussions\underline{.}
In order to properly assess this progress, it is important to remember that the average life expectancy of Mexican\underline{s} today is 76 years.
The first point would mean that international cooperation on insol\underline{v}ency procedures for companies with a cross-border profile is not known.
The world champion of basketball\underline{,} H xe9ctor "He\underline{tin}" Rey\underline{es}, was connected to basketball for more than 60 years and travelled the whole world.
Fe\underline{w} in Puerto Rico have such a great intellectual collection of the history of basketball in the country as H xe9ctor "He\underline{tin}" Rey\underline{es}.
I still know, as he said, that if Min\underline{cy} had allowed a championship for Bay\underline{amo}\underline{n}, Gausse would provide another.
The inclusion of five chapter\underline{s} for the second season was completed\underline{,} and a sixth chapter was just shot\underline{,} informed the broadcast\underline{er}.
There was no immediate explanation from Warn\underline{er} or TNT as to how Hag\underline{mann}'s loss would be dealt with in the series.
It is important to note that, unlike Quebec\underline{,} US citizens do not have a universal health card like the health card.
You have also restricted the right of individuals and groups to help those voters who wish to register\underline{.}
By contrast\underline{,} the whites, who represented 76\% of the electorate\underline{,} accounted for only 46\% of the voters who voted in advance.
Most important, however, is to talk to his doctor to determine whether or not he should be carried out.
"If there were no more smokers\underline{,} this value would rise to at least 50\%\underline{,}" emphasize\underline{s} Andr xe9 Beau\underline{lie}\underline{u}, spoke\underline{s}man for the Canadian cancer society.
The announcement of the likely discovery of the Hi\underline{gg}\underline{s}Bo\underline{son} caused a certain amount of attention last summer, and with good reason.
The analog\underline{y} with the electromagnetic field is helpful again to explain the relationship between the Hi\underline{gg}\underline{s} and the masses.
Some, like magnet\underline{s}, do so, but others do not - for example, a piece of paper would never keep itself on the fridge\underline{.}
Where\underline{ver} he has played, he has shown that he is a great player and a world star.
Pierre Noiza\underline{t}, who is also the author of a book about this currency, firmly believes in the potential of this technology as a transaction network.
They want to defend their centuries\underline{-}old and arch\underline{a}ic traditions\underline{,} even though j\underline{ih}\underline{ad}ists, Pakistanis, Arab\underline{s}, Uzbek\underline{s} and Taji\underline{ks} have joined them.
Former Mu\underline{ja}hed\underline{in}, the Afghan Government and current Taliban share a common desire to keep women in a subordinate position.
As I have heard in the campaigns\underline{,} people want a government that is not made up of th\underline{ieve}\underline{s}.
About 65\% of the population is under 25 years of age; Kabul now has 5 million inhabitants\underline{,} which is one fifth of the total population.
To everyone's surprise\underline{,} he announced on Wednesday that the constituent assembly would adopt its final version the next day.
In line with the military's wishes\underline{,} the examination of the defence budget will not be presented to Parliament, but to a national defence council\underline{.}
Similarly\underline{,} there will be no ban on civil proceedings in military courts\underline{,} as called for by the human rights associations\underline{.}
The fifth museum\underline{,} the Holocaust Museum or Ya\underline{d} Va\underline{s}hem in Tel Aviv\underline{,} tells of one of the most shock\underline{ing} chapter\underline{s} in history.
In Caesar\underline{e}a, the city of King Hero\underline{des}, you can walk through the Roman theatre and conquer the fortress of the Crusade\underline{rs}.
If you travel to Israel, don't worry about your poor English skills\underline{:} about 30\% of Israelis speak Russian.
Depend\underline{ing} on the brand, a rental car costs between 37 dollars per day (Hyundai Get\underline{z}) and 188 dollars (Audi A6, Volvo S80).
That is more than twice the cost of the official test: it costs a migrant three thousand rub\underline{les}.
The first channel is the army or the military, in other words weapons stolen during the fighting in the Caucasus\underline{.}
The Federal Security Service recently launched countless sham websites\underline{,} and buyer\underline{s} who want to buy weapons are getting on the net\underline{.}
The Federal Security Service recently launched countless sham websites\underline{,} and buyer\underline{s} who want to buy weapons are getting on the net\underline{.}
No one can yet predict whether the protests will increase even further or whether they will soon run out again.
Human movements are extremely dynamic and frankly\underline{,} the current 30 fps are not enough, especially for gesture\underline{s}.
In 2000, there was a survey in the press about the "Per\underline{son}alities of our City" award\underline{.}
- Recently we saw you in the role of the urban filmor player - a cultural city should have such a hero.
For cultural reasons, there are 300 people and not 10 thousand\underline{,} so there is less management, money, and everything is dying\underline{.}
Thus\underline{,} while for a newborn child weight\underline{lessness} is a much more natural state, the woman cannot do without gravity\underline{.}
In this respect, it should be noted that those countries that are an example to us also face problems.
As far as Czech legislation is concerned, what importance has been attached to your authority in rev\underline{ising} the procurement law, are you already feeling any effects?
I think that this law is certainly a step in the right direction and I hope that this adoption will be confirmed\underline{.}
The D5 motorway can be accessed virtually without restrictions\underline{,} but the road master\underline{s} recommend increased attention between 80 and 131 km.
The roads of the second and third classes are wet and therefore the reference to possible va\underline{in} sections applies here as well.
After the use of sc\underline{atter}\underline{ing} vehicles snow\underline{mat}\underline{ch} stays on the   u2047 ervenohor\underline{sk} xe9 sedlo pass and on the road towards Videlsk  u2047  k  u2047  xed  u2047 .
For this we want to use the marketing potential of the Maya\underline{n} calendar\underline{,} the end of which is predicted for the 21st of December at 11:10 a.m. in the morning.
On the day before, i.e. on 20 December, three concerts will take place simultaneously in Prague\underline{,} Brno and Ost\underline{r}ava from 21:00.
Since the students themselves do not have the means to visit the teachers\underline{,} we would like to help them in this way.
In Prague\underline{,} for example, there are Chinaski, Les\underline{bian} Support\underline{,} Il\underline{lust}\underline{r}ato\underline{sphere} with Dan B xe1rta, The Tap\underline{,} Mari xe1n Ban\underline{go} and Ji  u2047  xed Such  u2047 .
Well\underline{,} and over time, as our mode\underline{r}ator, L xe1  u2047 a Angel\underline{ovi}  u2047 , tend\underline{s} to say, this is somewhat out of control (laugh\underline{s}).
But this compassion is absolutely superfluous\underline{,} because people with disabilities are not lonely and abandoned beings that we should regret\underline{.}
Even before the Second World War, Polish cosmos enthusiasts engaged in space travel, although they did not always understand it.
In 1934   u2047 tern\underline{feld} won the Prix RE\underline{P}-Hirsch donated by Robert Esnault\underline{-}Pelterie and Andr xe9 Louis Hirsch for "Ent\underline{r}ance to Cosmonauticism".
Short\underline{ly} before the war, all projects for the military use of missile technology were coordinated by the Temporary Scientific Advisory Committee (Tym\underline{cz}\underline{as}owy Committee Doradcz\underline{o}-Naukow\underline{y}).
The rocket with a maximum altitude of 1800 m was about 80 cm long and weigh\underline{ed} less than 5 kg\underline{.}
The aim of these measures is to force our own people to accept the dictate\underline{s} of private capital, particularly in the area of wages\underline{.}
The result, today as then, is unprecedented decade\underline{nce} among elite\underline{s} who are not at all striving for deeper reforms.
In November 1979\underline{,} a mob of demonstrating Islamist students occupied the US Embassy in Tehra\underline{n} and took 52 diplomats hostage\underline{.}
The debacle in Iran contributed significantly to Jim\underline{my} Carter u2019s defeat against Ronald Reagan in the 1980 presidential election\underline{.}
Affleck and his team also have a similar effect on fi\underline{ct}\underline{it}ious scenes (the wrong film wand on a ba\underline{za}ar in Tehra\underline{n}).
The EU called for an American study which, according to balloon\underline{s}, is the leading cause of child suff\underline{oc}\underline{ation}.
As a simple citizen\underline{,} I have worked to ensure that the guide\underline{book} remains a free trade, and this has been achieved.
Convin\underline{c}ing politicians\underline{,} journalists and the public and trying to get them on our side to achieve these goals\underline{.}
I believe they are still approaching their role, but they are on the way to a more 'normal\underline{'} foreign policy.
Even if they do not like it, it is unpleasant for them and makes them much more unpopular - c'est la vie!
The Volvo buyer Geely originally used a blue and white logo reminiscent of BMW\underline{;} the dispute was settled\underline{,} Geely had to change it.
Last year, more than 1.4 million applications for trademark protection were received at the CTMO, almost one third more than in 2010.
Fifty singer\underline{s} have arrived\underline{,} between 23 and 69 years old, from the human genetic\underline{ist} to the houseman.
This cannot be taken for granted because, as obviously the disease is throughout the country, one prefer\underline{s} to keep quiet.
The name Trifid comes from the Latin word tri\underline{fi}dus (three-divid\underline{ed}, three-col\underline{lar}\underline{),} because dark strip\underline{es} of dust divide the glo\underline{wing} heart of the Starbur\underline{st} three-part\underline{s}.
The Keck Tele\underline{scope} is part of the Mauna Ke\underline{a} Observatory\underline{,} which looks into the sky next to it with the Sub\underline{ar}u Tele\underline{scope} and the IRT\underline{TF}\underline{.}
The incredible wealth that the country owe\underline{s} to its oil in the Caspian Sea has not yet arrived here in the province\underline{.}
Many ve\underline{il}ed women and Sala\underline{fi} adher\underline{ents} took part and shout\underline{ed}: 'The people are calling for the application of God's law'.
A battle for sovereignty over the symbolic Tahrir Square\underline{,} on which everything began, would have provoke\underline{d} civil war-like conditions.
Even from Sweden\underline{,} the old rival who was not so long ago much richer than Norway\underline{,} immigrants are flood\underline{ing}.
Op\underline{in}ions about the new head of state are divided in this densely populated\underline{,} extensive part of the country surrounding the capital.
"I hope, as president\underline{,} he is as he was as governor\underline{,}" says PRI congress\underline{man} Ol\underline{ver}a in Valle del Bra\underline{vo}.
He wants to ally himself with the United States and Canada and create a North American trade bloc modelled on the European Union.
Mexico has winners and losers, people for whom it offers opportunities, and others for whom it does not.
Expert\underline{s} say that the shack in the popularity of social media is precisely the population group to which the plan is directed\underline{.}
British American Tobac\underline{co} Australia says that, rather than marketing, industry is focusing on dealing with new legislation.
Today, 21 years later, Professor Larson says that he does not know whether the percentage of bo\underline{re}dom has risen or decline\underline{d}.
Hund\underline{red}s of irregularities surrounding mar\underline{i}juana have already been dropped here and in the State of Washington\underline{,} which approved similar measures.
The police in Grand Ju\underline{n}ction\underline{,} the largest town in the county\underline{,} no longer show adults for owning small quantities\underline{.}
I learned that the tut\underline{ors} not only dulled the mock\underline{ing} of Tory students, but also happily participated\underline{.}
The three years that preceded me stretch\underline{ed} before my spiritual eye to a pur\underline{g}atory of ost\underline{rac}\underline{ism} and isolation\underline{.}
Many years ago we went home for dinner after a fashion show in Piazza di Spagna in Rome\underline{.}
It was a red dress with flying rock and a dra\underline{ped} top with a decol\underline{let} xe9 that honour\underline{s} his name.
Anto has asthma, breath\underline{es} with difficulty\underline{,} husts frequently and his eyes are ir\underline{rit}\underline{ated} by the poison\underline{ous} gases from the volcano\underline{.}
With the basket on his back, with its 53 years, Unain\underline{ik} is only able to carry 50 kg\underline{.}
"The social networks are entertaining\underline{,} I can speak quickly to relatives in the distance or with friends" he says\underline{.}
The hosting President Ollanta Hum\underline{ala} opened the morning talks and ended the summit shortly after lunch in Lima\underline{.}
If I were to win\underline{,} it would be my last term as President, after which I retire from public life.
Nationally, the state is in fourth place in new and cu\underline{mul}\underline{ative} cases of AIDS\underline{,} and in 13th place in relation to HIV\underline{.}
On Friday\underline{,} Victoria Principal\underline{,} co-present\underline{er} of the original series, remembered Hag\underline{man} as a "enorm\underline{ous} personality on and outside the screen".
After the liver transplant\underline{,} he worked as a volunteer in a hospital to help fright\underline{en}ed patients\underline{.}
"I advise them, give them courage\underline{,} I meet them when their operations are imminent and after," he explained in 1996.
Every week, students examine apocalyptic issues such as nuclear war, zo\underline{mb}ies, viruses and germ\underline{s}, and global warming\underline{.}
Every week, students examine apocalyptic issues such as nuclear war, zo\underline{mb}ies, viruses and germ\underline{s}, and global warming\underline{.}
The Maya\underline{s} never predicted the end of the world; it is only a key point in the calendar\underline{,} said Restall\underline{.}
"Per\underline{hap}\underline{s} I call a few friends so that we can laugh together," said Sam\underline{ira} Ford\underline{,} a 20-year\underline{-}old student for communications\underline{.}
For example, electoral registration campaigns in the 2004 general election helped to register some 10 million citizens.
It is estimated that 30\% of cancer\underline{s} could be prevented if everyone eat\underline{s} well and moves sufficiently\underline{.}
For the Canadian cancer society, the fight against tobacco addiction remains a priority, despite the fall in the number of smokers\underline{.}
It must be stressed here, however, that these Bos\underline{ons} are not all as exotic creature\underline{s} as one might think.
The impact of this research on the general population is more difficult to predict\underline{,} but it would be wrong to assume that there were none\underline{.}
"In the course of our lives, we learn that a man is cry\underline{ing} while standing\underline{,}" says Pierre Bro\underline{de}ur, psycho\underline{logist} at the Victor\underline{-}Ga\underline{db}\underline{ois} Home.
But that does not necessarily mean 'I want you to slu\underline{mp} me', but 'I want my pain to be alleviate\underline{d}'.
By the way, engineers from the Montreal Road Construction Office, as well as entrepreneurs of Italian origin, such as Tony Ac\underline{cur}\underline{so} and Lino Za\underline{mb}ito\underline{,} were specifically charged\underline{.}
The latter has caused a stir by explaining to the Commission the functioning of the 'system' for obtaining public contracts\underline{.}
First of all, we want to become the first of our group before Porto\underline{,} so that we can play back the eight\underline{h} final as a home game.
The transaction is thus permanently linked to the chain of all other transactions\underline{,} and any modification would change the fingerprint\underline{.}
"Th\underline{re}e thousand dollars have been exchanged," says Jon Hol\underline{m}quist, who works for Coinabul\underline{,} convert\underline{ing} Bit\underline{co}ins into gold\underline{.}
Tolerated, sometimes supported by local insur\underline{gent}\underline{s}, the latter will no longer be there if Western countries become more discreet\underline{.}
During their exile in Iran or Pakistan, they had contact with the modern world and enjoyed its benefits.
In a country ruin\underline{ed} by 30 years of war, it would have been necessary for the infrastructure to be controlled by the state.
In addition, no longer refers to the protection of women, underscore\underline{s} Heba Mora\underline{y}ef of Human Rights Watch\underline{.}
In Caesar\underline{e}a you should visit the unique private Ralli Museum, where you can admire sculpture\underline{s} by Dali and Rod\underline{in}.
In Roman times, Caesar\underline{e}a was the most important city of Jud\underline{e}a and residence of the Roman governor\underline{s}, including Pont\underline{ius} Pil\underline{ate}.
Until now, this regulation only applies to migrants who want to work in the services sector, in the local housing sector and in the retail sector.
It is necessary to pass not only language tests\underline{,} but also tests into Russian history and the foundations of legislation.
On the other hand, before the law came into force, civil rights activists asked the following question several times in the press: what is the point of all this?
Furthermore, new arrival\underline{s} without language skills are offered places where active communication with people is not necessary.
"There is an own, sometimes artisan\underline{al} production and a mafia that organise\underline{s} smuggling\underline{,}" explains the former military man.
"You only need the right amount of money," says the ad on the website "Bu\underline{y} a gun or gun\underline{".}
I have heard about the following scheme\underline{:} the website is normally registered abroad and Russian laws are not applicable\underline{.}
US law prohibit\underline{s} corporate governance from standing in the way of this goal and exhor\underline{ting} or dismiss\underline{ing} trade union members.
It stimulate\underline{s} the possibility of manipulat\underline{ing} virtual objects in the air with bare hands and creating virtual open spaces\underline{.}
- We deal with the interaction of man and machine, but we want to expand the limits of this interaction\underline{.}
These can be laser sensors\underline{,} for example, because they offer good resolution in depth\underline{,} which is very important.
From this point of view, all current technologies are not good enough for us, as the developers of the algorithm\underline{s} have more work.
Note not only the resolution along the X and Y axis\underline{,} but also along the Z axis\underline{.}
Ros\underline{bal}\underline{t} continues the "Peter\underline{sburg} avant\underline{-}garde\underline{"} project dedicated to city dwell\underline{ers} who form the avant\underline{-}garde of art and culture.
We have very few cosmonaut\underline{s} who after long flights went well and got healthy offspring\underline{.}
Yet humanity must look for new ways in biotechnology\underline{,} radiation protection and artificial gra\underline{vit}\underline{ation}.
Even if adults feel that water is pleasant, it is a foreign environment, but infant\underline{s} feel that water is a natural element\underline{.}
In connection with public contracts\underline{,} the Czech Republic has good supervisory bodies and adequate laws, but falls behind in their application.
Nocturn\underline{al} snow\underline{-}dri\underline{ving} forced the road master\underline{s} to use the snow\underline{,} with about 3 cm of new snow falling in the   u2047 umperk district according to the road administration.
We also cooperate with other celebrities of the Czech cultural scene\underline{,} which is related to the fact that we perform many charity events and concerts\underline{...}
As part of the completion of the Jedli  u2047 ka Institute\underline{,} a separate building is to be built in which we will then be involved with this project.
And since I am a musician and play saxophone among others, I have founded a music company together with a colleague\underline{.}
This is logical in its own way, because everything new is considered with caution and will only be accepted after a long time.
They are people who can live and develop a full life, provided they have the means to do so.
Was it helpful for this success that you are a strict boss\underline{,} as many people hear?
It is not even clear whether the rocket should be used to launch or slow down the drain\underline{.}
The following year, the first PTA Chairman\underline{,} Kazimierz Za\underline{rank}\underline{ie}wi\underline{cz} (1902 - 1959\underline{),} became Deputy Chairman of the International Space Agency\underline{.}
Later an improved version, the RM\underline{-1}A, was built, and in 1959 the B  u2047 d xf3w Desert launched flight tests with the two-tier RM\underline{-2} rocket\underline{.}
The Met\underline{e}or-1A rocket had a transport space with 0.4 lit\underline{res} of capacity, Met\underline{e}or-1B with 0.4\underline{4} lit\underline{res} and Met\underline{e}or-1C with 0.62 lit\underline{res}.
In the years 1965 to 1968\underline{,} the Met\underline{e}or 2 rocket was developed at the Aviation Institute\underline{,} whose first flight tests began in October 1970\underline{.}
After the last wave of violence between Israel and Gaza\underline{,} there has been, as always, an innumerable response.
The cap\underline{tive} diplomats were finally released after 444 days after negotiations had been broker\underline{ed} by the Algeria\underline{n} Government.
The director also had to deal with the fact that history does not actually offer many exciting scenes in the cinema\underline{tic} sense.
Since the Czech Republic has another route to sea ports\underline{,} Pala\underline{s} says that the EU should pay us hundreds of millions of euros\underline{.}
But when I see something that I do not like, I try to propose a solution to change it.
But my goal is not the function, it is an instrument with which I can realize my vision\underline{s}.
As an independent non-parti\underline{san}\underline{,} I have far greater potential to gain support from all parties represented in Parliament.
I am not interested in whether someone is on the left or on the right; I want to connect people.
I have just started politics and I am trying to get the support of the majority for my programme.
The reason: At the opening a few weeks ago, every resident was invited to donate a book from his or her personal collection.
So they cannot be part of a broader line and must instead push things forward from their own position.
This conceal\underline{s} a name which is officially registered in China, but which has nothing to do with the companies of origin.
Both he and attorney Pat\underline{t}loch advise German companies to be very careful about dealing with China.
First of all there is the st\underline{ump}\underline{ing}: cow\underline{boy} boot\underline{s}, basketball boot\underline{s}, ladies pump\underline{s} and men u2019s slip\underline{pers} are looking for the clock on the parquet floor and quickly find it.
It is Monday evening, in the music room of the Institute of Medical Psycho\underline{logy} in Heidelberg\underline{,} the choir Imbon\underline{gi} is testing a new song\underline{.}
There are around 34 million HIV\underline{-}infec\underline{ted} people worldwide, according to Unaid\underline{s}, the United Nations programme to combat AIDS\underline{.}
A lot of things come together through sponsor\underline{ship}s, donation\underline{s} and, last but not least, the ga\underline{g}s that the choir sing\underline{s} all over Germany.
Although the small village is hardly found on maps\underline{,} in the valley of the Ezulwen\underline{i} River it is more than known.
Unnotic\underline{ed} by Earth\underline{'}s citizens, probes\underline{,} telescope\underline{s}, and small robots like Phoenix are exploring the depth\underline{s} of space.
This cloud of stars\underline{,} linked to the Rose\underline{t} Nebul\underline{a}, also constantly produces new baby stars - 5000 light years away from the Earth\underline{.}
Researchers suspect that it was born shortly after the big bang, when hydrogen was predominant\underline{ly} found in the universe\underline{.}
One of the tasks of the telescope is to search for light from the first stars and galaxies by the Big Bang.
With the Messenger probe launched in 2004 - the first to circle around Mercury - scientists now have certainty\underline{.}
Mir\underline{za}yeva\underline{,} who claims to have 143 descendants\underline{,} lives in a simple wooden house typical of the whole Caucasus region.
Eight people live under one roof\underline{,} including one of Mir\underline{za}yeva\underline{'}s son\underline{s} and one daughter\underline{,} both of whom have long been grand\underline{parent}\underline{s}.
"When he proclaim\underline{s} the referendum\underline{,} we will go to his palace and overthrow him," said the opposition\underline{ist} Jasser Said.
Now is the time to let the people decide at the ballot box what direction the country should take.
There are snow\underline{,} spectacular landscapes - and this st\underline{ub}born smell in the air that simply does not want to disappear\underline{.}
But actually everything is expensive here - a small glass of beer or a sandwich costs a proud 10 euros\underline{.}
Norwegian\underline{s} find it difficult to accept that someone in their peace-lov\underline{ing} country is capable of such brutal murder\underline{s}.
The forms, so fine, did not contain complaints about maltreatment, despite the fact that the officials had questioned Manning directly about his treatment.
Manning replied that his intention during this meeting was to reduce his observation status to "pre\underline{vention} of injuries\underline{".}
But Mexican\underline{s} who think in centuries\underline{,} not minutes, cannot ignore memories of this event.
They see us as a reminder of a hum\underline{ili}\underline{ating} defeat and look down on us because we are not Mexican enough.
But many Mexican Americans\underline{,} whom I know, feel that they are not part of either country.
But, while Israelis and Palestinians seem trapped in their historic conflict, the Middle East is changing around them.
Even if the cease\underline{-}fire agreed on 21 November lasts, the week-long battle\underline{s} have strengthened the hard people on both sides\underline{.}
Hard\underline{lin}ers may get their way, but the Arab Spring may be a stroke for them.
If it is up to them, it is ok\underline{ay} for us - and our children - to be bo\underline{red} at times.
If you are bo\underline{ring} and you use this energy to play guitar and cook\underline{,} you will be happy.
But prosecutor\underline{s} in Color\underline{ado} u2019s more conservative districts have announced that they will continue to pursue existing mar\underline{i}juana offences and still quote people on trial\underline{.}
It was an English student from the second year called James who presented himself as a member of the conservative student association\underline{.}
Every detail of his apartment, decoration\underline{,} food and music was recognized and felt his influence.
Since the elections, an attempt has been made to correct the problem of higher contributions and levie\underline{s} for foreign workers.
They are so popular, and the units are sold out by days and even weeks faster than the larger units\underline{.}
"I wouldn't share a photo that isn't mine\underline{,} or someone who makes the fool\underline{'}s head," he says\underline{.}
"If someone afflict\underline{s} me or asks me, I just remove it from my user account" he admit\underline{s}.
Another point is to make them understand that they must act online, as they do offline\underline{.}
On the official ASP\underline{A} website you can see that the document was published last Tuesday\underline{.}
Correa assured that if he lost the February 2013 elections, he would withdraw from political life.
Back then, even the director of a IM\underline{SS} clinic avoided saying goodbye 'because it led to a dead end'.
Among his cinema\underline{tic} works were well rated roles in "The Group", "Har\underline{ry} and Ton\underline{to}" and "Pri\underline{m}ary Color\underline{s}".
Ten episode\underline{s} of the new issue of "Da\underline{lla}\underline{s}" were aired a few months ago with great success on the TV channel TNT\underline{.}
"The Philippines do not participate at the end of the world," he wrote as an allusion to an exception of a higher instance.
In fact, Republican lawyers have recorded only 300 cases of electoral fraud in the United States in 10 years.
As a result, 180 bill\underline{s} were introduced in 2011 alone, restrict\underline{ing} the exercise of voting rights in 41 states.
Since 2011\underline{,} a dozen states have passed laws requiring voters to demonstrate their US citizenship\underline{.}
"The research shows that regular physical activity protects against wrath cancer throughout life," he adds\underline{.}
But for the phy\underline{s}icists it is not yet completely certain that it is really the Hi\underline{gg}\underline{s}.
In one corner are the good citizens, known as Fer\underline{mi}one, who follow the Paul\underline{i} principle.
In fact, not all particle\underline{s} and not all materials interact with the electromagnetic field.
There is currently no comparable person in Ligue 1 and he is one of the best trainers in Europe.
One of our most important goals is the Champion\underline{s} League\underline{.}
The opposite of the current monetary exchange based on central banks, identified transactions and processing fees between stakeholders\underline{.}
Nevertheless\underline{,} the European Central Bank (ECB) showed interest in this in a report on virtual currencies published in October.
With the difference that the user can choose a different address for each payment, which ensures anonym\underline{ity}.
The system can be easily implemented by vendor\underline{s}, and the latter do not need to install new terminal\underline{s} or computer programs.
There is a general trend whereby hierarch\underline{ical} systems are being reconsider\underline{ed} in favour of more horizontal systems.
They brought themselves into disreput\underline{e} and most of them were not themselves involved in the fighting\underline{.}
This reinforce\underline{s} the impression that the Western countries were only there to seize it.
Just a week ago, the Head of State granted this plenary two additional months to complete his work.
Israel's three main recreation areas are located on the shores of the Mediterranean, the Red Sea and the Dead Sea.
According to legend\underline{,} Fort\underline{una} is held by all those who touch the walls in the street with their sign.
What changes does the requirement to have language skills bring, both for Russians and for migrant workers?
"They want one or two hundred rub\underline{les} for cigarette\underline{s} and tea\underline{,}" says the Taji\underline{k} Umed Huzh\underline{k}adamov to journalists\underline{.}
Expert\underline{s} calculated the proportion of illegal weapons supplied by each of the five channels\underline{.}
People come like hungry fish to feed and then land in Siberia and are allowed to sap coal\underline{.}
According to critics\underline{,} Wal\underline{mar}t can often sell the goods so cheap\underline{ly} only because employees are poorly paid.
If Wal\underline{mar}t were to shift the wage increases entirely to customers, each purchase would cost them only 46 cent\underline{s} more in the future.
The input of information (the system receives more data) has been improved, but the output has not yet been decisive\underline{.}
- The present generation is basically a good starting point for our work in the field of three-dimensional detection\underline{.}
For my work I needed just such a device\underline{,} only without touch control and with more images per second.
- Many of my pictures are real pearl\underline{s} and clearly express the topical\underline{ity} and sharp\underline{ness} of the thoughts\underline{.}
Our gu\underline{ll} fle\underline{w} away, and no one on earth could have answered the following question: does it survive space flight\underline{?}
In June 1964\underline{,} just one year after her space flight\underline{,} the first female cosmonaut\underline{,} Valentin\underline{a} Ter\underline{es}hkow\underline{a}, gave birth to a daughter\underline{.}
It is as if the little ichtyander\underline{s} bear witness to the fact that life on the land descend\underline{ed} from the ocean\underline{.}
In principle this is logical\underline{,} since only two weeks pass from birth to the first swimming.
Public funds administer\underline{ed} by our districts and municipalities are subject to the control of the local audit offices\underline{.}
It is no longer snow\underline{ing} in the region, and only a thin snow blanket remains in the lower altitude\underline{s}.
Since it has snow\underline{ed} before and temperatures fell after that, ice can get smooth\underline{er} on the roads\underline{.}
It turned out that most people are interested in working with us and have fun with it.
Your foreign plans are not exactly small, so far you have already appeared in Madrid\underline{,} Brussels\underline{,} London or Moscow\underline{.}
The research work was carried out by the Institute Kom xf3rka Technik\underline{i} Uzbro\underline{je}nia in cooperation with Prof\underline{.} Mi\underline{e}czy\underline{s}law Wolf\underline{ke} and Prof\underline{.} Gu\underline{sta}w Mokrzy\underline{ck}iegi.
The first type, the RM\underline{-1}, was completed in 1957\underline{,} the first launch was on October 10, 1958\underline{.}
In other words, governments are exp\underline{os}ing their own people to private capital, regardless of the social consequences.
The details of this operation were kept secret for a long time.
Until then, women had an advantage in life insurance because, objectively, they represent a lower risk for insurance companies.
In the Senat\underline{e} you made it and then made your way to the castle\underline{.}
I have been told\underline{,} for example, that I would bri\underline{be} journalists or that I was an advise\underline{r} to Ji  u2047  xed Par\underline{ou}bek\underline{.}
As President, you have no powers in this respect and only the Senat\underline{e} as a whole can bring forward legislative proposals.
I also supported the invest\underline{ig}ative journalist Jan\underline{a} Lor\underline{en}cov xe1, who exposed fraud in the trade in light fuel oil.
You are driving an Aston Martin\underline{,} have a fortune of 60 million and have no money for your campaign\underline{?}
"We wanted to work with recycled materials here," explains Joop Tro\underline{ub}orst, project manager at the municipality of Sp\underline{ijk}\underline{en}isse\underline{,} on demand of the standard.
So one day we encountered a suitable agricultural waste product in a Fri\underline{s}ian farm\underline{.}
For many years now, a mill\underline{i}metre\underline{-}thin thin plastic flee\underline{ce} has been used as a root base in greenhouse\underline{s} and fields in the Netherlands\underline{.}
For the library\underline{,} the flee\underline{ce} was pressed to four cent\underline{i}metre thick plates\underline{,} for the first time in these quantities\underline{.}
Although the bookberg is under a glass crash\underline{,} even on sunny days the sun shine\underline{s} only briefly inside.
The wide wooden glue binders, which stand across the glass facade\underline{,} serve as a shade and capture much of the sunlight\underline{.}
After all, it signals that, as an international player, it must be taken seriously and its interests taken into account.
Does Germany see itself as an important international player - does Germany want to play a leading role at all?
The financial losses and process costs of the industries concerned are in the millions\underline{,} especially for expensive flagship products.
In 2009, Daimler lost a legal dispute with the construction machinery manufacturer Sany, the company that recently took over the German concrete pump manufacturer Put\underline{z}meister\underline{.}
Cu\underline{tting} of the male foreskin\underline{,} which demonstr\underline{ably} reduce the risk of contagion by half, is hardly accepted by the population.
In het\underline{ero}\underline{sexual} adults\underline{,} common sexual\underline{ly} transmitted diseases are Ch\underline{lam}\underline{y}dia infection\underline{s}, tri\underline{cho}\underline{mon}ads, candidos\underline{e} (Pilz), Tripper and Human Pap\underline{pil}\underline{oma}\underline{vir}\underline{es}.
"In total, we have already sent around 200 000 euros to Esitjeni," says Anne\underline{tte} Lennar\underline{tz}\underline{,} president of the association\underline{.}
The fo\underline{g}, which is 1400 light years away, consists of dust grain\underline{s}, which are ten to a hundred times smaller than ordinary house dust\underline{.}
Since then, the mirror\underline{s} of the optical telescope\underline{s} have become ever larger - and the insight\underline{s} they provide have become ever deeper\underline{.}
Advant\underline{age} of the favorable design: The telescope is fixed at its height angle - and thus limited in its mobility\underline{.}
On the Mauna Ke\underline{a}, too, a huge new telescope is to be created - with a mirror average of thirty meters\underline{.}
However, there is no reliable data for this, as the Messenger circle\underline{s} far closer to the North Pol\underline{e} around the planet\underline{.}
But this is the deepest south of Azerbaijan\underline{,} the border with Iran is only a few kilometres away.
I always washed my hair with milk\underline{,} so they never left me and kept their color\underline{.}
"And that he succeed\underline{s} is my responsibility, before the people and before God," he said on state television\underline{.}
As in previous constitution\underline{s}, the draft states that ju\underline{ris}\underline{pru}\underline{d}ence is based on the 'pri\underline{n}cip\underline{les} of Islamic law'.
The Muslim Brot\underline{her}hood said that both the opponents of the draft Constitution and the supporters had spoken out loud and clear.
Rakfisk is considered to be an important part of Norwegian history.
I stand in the snow and stand up for another dish - I have enough of Rakfisk.
On Saturday\underline{,} Mexico u2019s new president\underline{,} Enrique Pen\underline{a} Nie\underline{to}, will be given the leadership of the nation\underline{.}
"When I arrived at her home, it seemed that her body had been washed\underline{,}" Sen\underline{ora} Bu\underline{en}dia recall\underline{s}.
Manning had said that he had never had the opportunity to cover himself with his blanket during this count\underline{.}
This night, Manning said, his underwear\underline{,} flip flo\underline{ps} and glass\underline{es} had been removed from his cell\underline{.}
The hearing is scheduled to continue this weekend\underline{,} and the public prosecutor is expected to justify the conditions under which he is held.
I speak Spanish, at least good enough to speak in this language at both ends of an interview\underline{.}
But I do not have the vocabulary of a native speaker\underline{,} and I will not go away with my American accent either.
And Pen\underline{a} Nie\underline{to} vo\underline{wed} to continue Mexico\underline{'}s war against drug carte\underline{ls}\underline{,} even if he did not give any details on this.
And in most cases that person was in a profile - dark\underline{-}skin\underline{ned}\underline{,} uneduc\underline{ated}, from a poor village, etc.
They want to use Mexican Americans as provisional "amba\underline{s}sador\underline{s}" for Mexico\underline{,} who represent their interests in the United States.
A war with the local superpower will hardly help the new Arab governments to repair their economies\underline{.}
It was said that the laws would favour the black market, which would lead to cheaper and more accessible cigarette\underline{s}.
The Australian Government has banned Internet advertising from local companies and sites, but has no influence on international sites.
District prosecutor Pet\underline{e} Haut\underline{z}inger supported this decision, but also decided not to drop all outstanding property proceedings\underline{.}
"I don't think I'm wasting my time enforcing the law until it changes," he says\underline{.}
This evening, I sat at college alone at dinner\underline{,} when someone touched me slightly\underline{.}
I bought my first Valentin\underline{o}-Klei\underline{d} for a party in the castle of my cousin, Prince Ed\underline{ou}ard de Ligne\underline{.}
I am a patri\underline{otic} husband\underline{,} you are my patri\underline{otic} wife\underline{:} let us fulfil our civic duty and make life!
Every year, it spends USD 1 300 on policy measures to encourage citizens to have more children.
El Peri xf3dico interview\underline{ed} five young people aged between 10 and 15 who are often on the net\underline{.}
In this sense, he defended the project to create a South American citizenship that promotes the members of the Unasur.
Those who teach never commit themselves to anything, and in return we always sign everything to the South Americans\underline{.}
Correa also referred to the treatment of the health problems of Venezuela\underline{n} President Hugo Ch xe1vez in Cuba\underline{.}
The walls of his house are almost all decorated with photos and memories of his long career and bear witness to them.
And then I said goodbye to a championship in 1981\underline{,} the year of the debut of Jerome Min\underline{cy} at BSN.
At that time he preferred to enjoy his execution\underline{s} and those of Min\underline{cy} in the national team.
She is among the best, as well as those who won against the Dream Team at the 2004 Olympic\underline{s}.
The family of Larry and his closest friends were with him in Dal\underline{las} for the celebration\underline{s} of the harvest festival\underline{.}
Unlike Canada\underline{,} the US states are responsible for holding national elections.
They are proposed active monitoring and are offered treatment as the disease progresses.
The criteria for deciding who should be treated and who should not are determined with increasing accuracy\underline{.}
While one study found the reduction in the risk of prostate cancer\underline{,} another rather showed an increase.
With its Committee on dig\underline{n}ified death, Quebec recently discussed the delicate issue of the end of life.
Sitting at the table in front of a delicious lunch\underline{,} he resign\underline{ed} to be helped with food.
"My greatest wish is to heal my diarrhea, because it is hum\underline{ili}\underline{ating}," he says\underline{.}
Because\underline{,} according to several people working in the field of pal\underline{li}ative care, major events are taking place in the midst of these steps backward\underline{s}.
In the next few days she still awaits a last visit of her son\underline{,} who comes from Italy.
At the Victor\underline{-}Ga\underline{db}\underline{ois} Home, a group of volunteer\underline{s} are available to help with body care and food intake\underline{.}
This is where life continues in the best possible conditions, explains Dr. Christian\underline{e} Martel, one of the physician\underline{s} of the Home.
An "industry\underline{"} that was very expensive for Quebec\underline{'}s taxpayers\underline{,} especially in the 1990s and 2000s.
This means that a player like me has to face up and want to do his best.
To become a large European club\underline{,} Paris must win titles and make a name for itself in the long term.
Lyon and Marseille\underline{,} which were not good last season, were "dri\underline{ed}" by this new PS\underline{G}.
Thi\underline{ago} Silva\underline{,} one of the best defend\underline{ers} in the world, also allows everyone else to make progress.
A number of data related to this transaction is electronically signed by a double encryption system.
The computers "take\underline{"} the new transaction and add a number to it before it is "hack\underline{ed}".
The goal is to find the number that gives a special fingerprint (many zero\underline{s} at the beginning).
"It will take some time for Bit\underline{co}in to prevail\underline{,} but 2013 could be a turning point," he predict\underline{s}.
At that time, Kabul was empty and the country was overrun by war because of the struggle\underline{s} of the various insur\underline{gent} groups.
While the Egyptian President had to speak on television last night, demonstrations are scheduled for this afternoon\underline{.}
From Friday evening to the sunset on Saturday\underline{,} markets and shops are closed, and public transport is suspended\underline{.}
Most adventure\underline{rs} and people seeking rest came from Russia, France, Germany, Italy, England\underline{,} the USA and Ukraine.
Their only aim is to make money for the maintenance of the families that remain in their homeland\underline{.}
However, in future, the tests will become mandatory for all immigrant workers, according to the Federal Migration Agency\underline{.}
The initiative to introduce the tests was supported by members of the State Duma and the Federal Migration Authority\underline{.}
Some fake certificates cert\underline{ifying} the completion of the language test have already been seized by the staff of the Federal Migration Agency\underline{.}
Not all of them are satisfied that the Russian authorities want to combat the problems by 'throw\underline{ing} the screw\underline{s}'.
Wal\underline{mar}t sell\underline{s} all products, from dia\underline{pers}\underline{,} hunting gun\underline{s} and car batteries to vacuum cleaners, eggs and milk\underline{.}
The goods in the Wal\underline{mar}t stores are between 8 and 27\% cheaper on average than in large supermarket\underline{s}.
A typical Wal\underline{mar}t employee who earn\underline{s} \$9.5 an hour could not afford this increase, they said.
According to New York Times\underline{,} this was the biggest action of its kind in the history of the US fast-food industry.
We try to change this, work on real three-dimensional representation systems based on various technologies, including projection\underline{s}.
- If I remember correctly\underline{,} Microsoft, unlike Google, did not present its glass\underline{es} to the public.
I have chosen the color red as a fashion designer dealing with the look and image.
We gave them Tra\underline{chten}\underline{berg} and it started his great career\underline{,} but he learned the basics from us.
Now everyone pays attention to the clothes and is oriented towards the outside rather than the inside of the human being.
In the past, people formed large groups: the Bohemia\underline{n}s loved one thing and the ordinary people loved the other.
I have followers, and the most important thing is not to deceive them and not to destroy what has been achieved.
- Petersburg is not the capital of culture; in Moscow there is much more culture and a breeding ground.
The fourth generation of peas br\underline{ed} in orbit did not differ in any way from the earth\underline{ly} species\underline{.}
A newborn child cannot be put in a strain suit in orbit like an adult for training.
In the conversation for Akt\underline{u} xe1ln  u2047 .cz this is said by the Vice\underline{-}President of the Supreme Control Office (Nej\underline{vy}  u2047  xed kon\underline{tro}ln xed   u2047 ad\underline{,} NK  u2047 ), Mil\underline{o}slav Kal\underline{a}.
It is a parallel test that we started about two years ago.
The problem may arise\underline{,} however, that the rules become 'str\underline{eng}\underline{th}ier' and can no longer be observed\underline{.}
It should be noted\underline{,} however, that improving the situation always depends on the efforts of those concerned.
There are few truly unique things, and I dare say that Tap is one of them.
Entrance costs 400 CZK\underline{,} children up to 12 years of age free, tickets are available on pre-sale with Bohemia\underline{ticket}\underline{.}
The first RM missile\underline{s} were replaced by the Met\underline{e}or-1 missile\underline{s} developed between 1962 and 1965\underline{.}
The launch weight was 32\underline{.}5 kg\underline{.}
This is done on the one hand through economic pressure in the event of long-term unemployment and, on the other hand, by curtail\underline{ing} workers' rights.
Private capital insist\underline{s} narrow\underline{ly} on its position that the state must not lead the economy.
We will apply for refund\underline{s} to the EU," said the then Minister of Agriculture\underline{,} Jaroslav Pala\underline{s} (  u2047 SSD\underline{)} in autumn 2004.
If you create a business plan in a company, you also have an ideal goal and a vision\underline{.}
I say quite clearly that I am an amateur\underline{;} I am neither a genius nor an intellectual\underline{.}
I do not even have money for the presidential campaign\underline{;} my transparent account is only CZK 20,000\underline{.}
You say you want to change the Republic, but you do not want to invest your own money in it.
The fact that I do not have sponsor\underline{s} shows that my programme does not arouse too much interest.
We turned the classical room configuration on the head and stretch\underline{ed} the reading area from the inside to the outside.
The inside of the bookberg is well used: offices\underline{,} internet library\underline{,} chess club\underline{,} environmental center and house technology centre are in the centre.
However, I would not wish to attach too much importance to this, which is not a totally unilateral relationship.
I believe that the Obama administration secret\underline{ly} understands the European position.
I believe that in the future Germany will take a leading role in pushing Europe into a European position.
Wentz\underline{ler} is confident to bring the matter to a good conclusion and praise\underline{s} the professionalism of the courts\underline{.}
But he also says\underline{:} 'The process is extremely complicated and costs us a lot of time, money and nerve\underline{s}'.
About 2000 people live there, some still in simple mud huts and stra\underline{w} huts\underline{,} most of which are children.
In Esitjeni, the small thing that makes Swaziland sick is the highest HIV infection rate, the lowest life expectancy in the world according to Unicef.
Some of the pathogen\underline{s} of sexual\underline{ly} transmitted diseases can also be transmitted through lub\underline{ric}\underline{ation} infection\underline{s} and close body contact.
The picture published by the European Southern Observatory shows the tri\underline{fi}d nebul\underline{a} several thousand light years away in the constell\underline{ation} Sch xfctze\underline{.}
In this bright\underline{ly} illumin\underline{ating} galaxy with a small black hole\underline{,} there is no dust yet, only gas.
It looks into space right across two mirror\underline{s}, each with a diameter of 8.\underline{4} meters\underline{.}
Every computer owner can help with the "Se\underline{arch} for Extra\underline{terre}\underline{stri}\underline{al} Intelligence\underline{"} (SET\underline{I}) by providing computing power.
Until 2007, the Ke\underline{ckel}\underline{es}kop\underline{e} on the Hawaii\underline{an} volcano Mauna Ke\underline{a} was considered to be the largest in the world.
Since March 2009, the space telescope Ke\underline{pl}er has been looking for extrasol\underline{ar} planet\underline{s} - especially those that are habit\underline{able}.
The mini\underline{bus} ro\underline{am}s over the wind\underline{ing} road, past densely wood\underline{ed} hills\underline{,} ra\underline{ging} rivers and simple farmhouse\underline{s}.
However, the controversial star of the museum is the shepherd   u2047 ir\underline{ali} M xfcs\underline{l} xfcmov\underline{,} who is said to have become 168 years old.
And, given the oldest documented person who was 122 years old, M xfcs\underline{l} xfcmov u2019s age seems extremely dubious\underline{.}
The fact is, however, that the people of the region around Lerik are striking\underline{ly} often reaching bi\underline{bli}\underline{cal} age.
And perhaps Mir\underline{za}yeva\underline{'}s elder son is right: 'The elderly enjoy great respect in our culture'.
Nobel Peace Prize laureate and former Chairman of the International Atom\underline{ic} Energy Agency\underline{,} Moham\underline{ed} El-Bar\underline{ade}\underline{i}, declared that the draft Constitution was "on the dust\underline{bin} of history".
Could the country's secret of success have anything to do with the local appetite for pretty ro\underline{gue} fish?
Norway does not often get into the world press, and most people do not seem to be upset\underline{.}
"As long as we can ski in winter and hike in summer, we are happy," says Anna\underline{.}
There is a live TV circuit to a fly\underline{-}lined showmaster surrounded by plates with Rakfisk.
Before he was on an equal footing with the US President, Pen\underline{a} Nie\underline{to} was the governor of his home state, Mexico\underline{.}
Pla\underline{ques} with his name also hang outside a modern sports centre and an impressive interactive museum on climate change.
But, on the other side of the state, not many people share this view of their former governor\underline{.}
Hi\underline{d}den under motorway crossing\underline{s}, it is in many ways a suburb of Mexico City itself.
He said that he considered suicide in Kuwait and that he had become unconscious because of the heat\underline{.}
Mexican\underline{s} tend to accus\underline{e} emigr\underline{ants} - they remind them of difficult times, he says\underline{.}
By contrast\underline{,} the Brot\underline{her}hood has deteriorate\underline{d} with Hamas and its leaders are more dependent on popular views.
Blood\underline{y} missions to rep\underline{atri}\underline{ate} Hamas in Gaza will increasingly take their diplomatic toll over the years.
That would do more to create a Palestinian state than with the forthcoming application for UN observe\underline{r} status.
The Australian Government wants to stop young people from smoking by removing the gla\underline{mor}\underline{ous} image of tobacco consumption\underline{.}
Frank\underline{ly}, there is only one reason why I would stop, and that is my little girl\underline{.}
So bo\underline{re}dom differ\underline{s} from apath\underline{y} in that the person is not employed but wants to be.
At some point, we will all get bo\underline{red} - my delayed flight\underline{,} a scream\underline{ing} loud\underline{spe}\underline{ak}er, a particularly tir\underline{ing} film.
He believes that in reality people are only looking for a way to turn off and relax\underline{.}
The reactions are ambiguous even in places like the rural Mesa County\underline{,} where voters rejected the Mari\underline{hu}ana initiative.
Last week, Mont\underline{rose}\underline{,} a city in the West, decided on a six-month ban, which will probably be adopted next week.
They are calling for a place in their College Equality Committee to ensure that their opinions can be expressed freely\underline{.}
"This pose\underline{s} a threat to intellectual discourse and the well-being of members," she says\underline{.}
I felt that homosexual\underline{s} had to feel the more liberal legislation of the United States.
He hated the place, found it provincial and pet\underline{ty} and rejected it for his Marx\underline{ist}-determin\underline{istic} historical perspective\underline{.}
It was a pants\underline{,} a shirt\underline{,} a wa\underline{ist}coat type "Gill\underline{ette}\underline{"} and a jacket from the autumn\underline{/}winter collection 1971\underline{-19}\underline{72}\underline{.}
I saw him last time a month ago at a gala dinner at the Museum de Orsay.
There are people for whom their work is hell\underline{,} and others are working literally in hell\underline{.}
Anto has asthma, breath\underline{es} with difficulty\underline{,} hustles frequently and his eyes are ir\underline{rit}\underline{ated} because of the toxic gases\underline{.}
I will not retire\underline{,} I will die here because the volcano was my whole life.
"These are very confidential secret\underline{s}, my mother may know them, but not the whole world," he confirm\underline{s}.
According to the boy\underline{,} no one gave him any hints or asked him for his address or telephone number.
"We are the digital immigrants they are supposed to teach when we still learn for ourselves" he says\underline{.}
Correa explained that there is a risk that Assange\underline{'}s health and mental condition will be affected.
These funds were used for the acquisition of shares of the Admin\underline{ist}radora Prof\underline{es}ional de Hoteles (the professional hotel management).
Bartow then recommended Ray\underline{mond} Gausse\underline{,} who became a citizen and was one of our best shoot\underline{ers}.
I know when we first won the pre-Olympic tournament in Mexico against the US.
We had a number of good trainers like Julio Toro, Flor Mel xe9nde\underline{z}, Carlos Moral\underline{es}, Ray\underline{mond} Dal\underline{m}au, Arm\underline{and}ito Torre\underline{s}.
"He was an original person and lived life to the full," Gra\underline{y} explained in a communication.
Hag\underline{man} was diagnose\underline{d} with liver ci\underline{r}rhosis in 1992\underline{,} and admitted that he had dr\underline{unk} a lot for years.
In Temple\underline{,} the attend\underline{ant} Professor Barry Va\underline{cker} gives the course 'Media\underline{,} Culture and the End of the World'.
"I tried to inform the students about what is possible, probably, credible and impossible\underline{,}" said Va\underline{cker}.
The Supreme Court of the United States confirmed in 2008 the constitutional\underline{ity} of the Indian\underline{a} Law\underline{.}
The new restrictions have disproportionate\underline{ly} affected young people, minorities and low-income people.
For it is obvious that two out of three Hispan\underline{ic} voters prefer democratic parties.
The latter accounted for only 11\% of voters\underline{,} but 24\% of the citizens who voted in advance.
For example, in 1969 Will\underline{ard} Boy\underline{le} developed a small light sensor during his work in opt\underline{ics}\underline{.}
Last night we served Mr X a beer who died during the night.
53\% of patients admitted to the Victor\underline{-}Ga\underline{db}\underline{ois} home come from their homes\underline{,} 47\% come from the hospital\underline{.}
The 'Du\underline{ches}\underline{n}eau report' established a direct link between industry, secret financing of parties and bri\underline{ber}y of officials\underline{.}
He also confess\underline{ed} that he had organised an illegal fund\underline{raising} for former liberal Vice\underline{-}President Nathal\underline{ie} Norman\underline{de}au.
Following these revelation\underline{s}, Mr Tre\underline{mb}lay resign\underline{ed} in early November, which plunge\underline{d} Montreal into a serious crisis.
It can be explained by personal insight\underline{,} but also by the new dimension of the PS\underline{G}.
What do you think about the first months of Did\underline{ier} Deschamps at the head of the "Bleus"?
Before this meeting in Spain, I have never seen a similar game in my career\underline{.}
Each transaction between two users actually takes place between two email addresses in the form of an email.
Once this number has been found, the other nodes can easily check whether it is the right one.
But his country has been dependent on foreign aid since the 1950\underline{s} and long before.
Industry has not been rebuilt\underline{,} there are no functional res\underline{er}voir\underline{s} and important irrigation systems have not been repair\underline{ed}.
The Embassy has received dozen\underline{s} of written requests from local communities in the province of Kap\underline{isa}\underline{.}
85 largely Islamist members of this constituent assembly adopted the text yesterday in a strange atmosphere.
The latter also share their concerns about the text they see as threatening freedom.
In Israel, Ukrainian tourists expect holy sites, the navel of the world, and a sea of bri\underline{ne}.
The Promised Land is a land that unite\underline{s} the sp\underline{len}dour of Bibli\underline{cal} truth\underline{s}, modern comforts and untouched nature.
Here, according to Christian belief\underline{,} there is the navel of the world, which symbol\underline{ises} the sal\underline{v}ation of mankind\underline{.}
Its tur\underline{qu}\underline{ois}\underline{e} blue water has a high salt content and therefore does not swim easily on the surface\underline{.}
In Jaff\underline{a}, you can meet newly married couples from all over Israel and even other countries on photo appointment\underline{s}.
"The weapons were stolen by both Russian officers and the cauc\underline{as}ians themselves," says Baranez.
The vast majority of illegal weapons\underline{,} according to the invest\underline{ig}ators\underline{,} come from the army and the legal protection authorities.
He also gives me the hit ring\underline{s} only because he knows that I am not begg\underline{ing} him.
Internet search engines show search results for websites and groups in "Vkontakt\underline{e}", where weapons are offered "for different purposes".
Expert\underline{s} predict prices of between USD 100 and USD 900 when buying illegal fire\underline{arm}\underline{s}.
To do this, however, it is necessary to recognize not only the user but also his environment.
- What are your demands on modern cameras based on your work with Xbox Ki\underline{n}ect sensors\underline{?}
But the main thing is not the Megapixel\underline{s} themselves, but the quality of the mat\underline{r}ix and the depth\underline{.}
There is one problem that critics of this idea often point out: there is no tangible response!
It makes people think that it feels what it should feel when it sees something?
So far, the brain is only moderate\underline{ly} outnu\underline{mber}\underline{ed}, and we still have many years of work ahead of us.
Kir\underline{ill} Mill\underline{er} is a brilliant figure of the Petersburg avant\underline{-}garde at the end of the 1980\underline{s} and the beginning of the 1990s.
In society, anything that devia\underline{tes} from the grey standard generate\underline{s} aggression and bad behaviour\underline{.}
Let us save the world, for example, by prescri\underline{bing} that everyone has to dress up completely.
Perhaps\underline{,} however, we should not give a person a hand, but rather sp\underline{r}out his face.
Life would only be possible at large or in the orbit of Venus\underline{,} in space.
How can the project help you?
Do you see the adoption of this law rather positively\underline{,} or will the system be burden\underline{ed} with further bureaucracy\underline{?}
The R6 motorway and the first-class roads in the region are currently unrest\underline{ric}\underline{ted}.
However, attention is needed, for example, on bridge\underline{s} where the roads are sometimes pave\underline{d} and smooth\underline{.}
The road champion\underline{s} warn drivers against smooth ice\underline{,} which can occur especially in higher locations in the district of Par\underline{du}bic\underline{e}.
An extended layer of snow lies at altitude\underline{s} on the streets of Ry\underline{ch}nov nad Kn  u2047 nou and Tru\underline{t}nov districts\underline{.}
There is also fo\underline{g} on the east side, but the visibility will improve during the day.
Snow\underline{-}mat\underline{ch} now count\underline{s} on drivers travelling towards the height\underline{s} of the Ol\underline{o}mouc district\underline{.}
Original\underline{ly} from me, we developed the idea together with our graphic artist Honza Augusta.
The anthem on YouTube is already very popular, and will it also be heard at the benefit concerts\underline{?}
Dr. Jan Gadom\underline{ski} (18\underline{99} - 1966\underline{)} later became an important advocate of astronom\underline{y} and space travel.
In Polish journal\underline{s} he published hundreds of articles and wrote several books on these scientific discipline\underline{s}.
As early as 1925, a railway dr\underline{one} was built in Poland for which a rocket was planned\underline{.}
The documents that have been handed down show that research had reached the stage of practical tests\underline{.}
On the other hand there are the loose passage\underline{s} from Hollywood\underline{,} which are iron\underline{ic} and slightly exaggerate\underline{d}.
The name rum can only be used for sugar cane distill\underline{ate} products, not for sugar beet products.
"The people want me to save the republic\underline{,} but I'm just an amateur\underline{,}" Okam\underline{ura} says\underline{.}
Just take the direct election of the President, which was the cause of public pressure.
And Stefan Sp\underline{er}mon, IT technic\underline{ian} in a nearby large company, says\underline{:} 'But, it's nice, the house.'
Above all, Sp\underline{ijk}\underline{en}isse now has the first public cultural building in the history of its existence\underline{.}
Stefan Sp\underline{er}mon, the first skept\underline{ic} from the IT industry, already dared to enter the new library\underline{.}
And also the TCM teacher Cy\underline{n}thia Bogarde\underline{,} who even calls Boekenberg "a long overdue soul\underline{".}
"I think, thanks to our invitation\underline{,} now every resident has a certain relationship with this new house.
They are expected to play a more independent role, but they are not used to that.
Have these economic interests influenced the attitude of the Middle East conflict and the vote in the UN?
I believe that there is a great deal of understanding in Europe and even in the United States of America of the German position.
I therefore do not believe that this was such a dramatic rupture as the Libya\underline{n} question.
In the next two instances, Freud\underline{enberg} got right, but the opponent of the trial still fights today.
The association Voice\underline{s} for Africa has found sponsor\underline{s} in Germany for 180 AIDS cases in the village of Esitjeni.
Infec\underline{t}ious diseases can cause genital ulcer\underline{s}, ur\underline{in}ary ulcer\underline{s}, outflow\underline{s}, subcut\underline{an}eous aches and ve\underline{s}icles or warts.
Free condom\underline{s} would exist at every corner\underline{,} Anne\underline{tte} Lennar\underline{tz} says\underline{,} "but they are hardly used.
The water probably came from comets, or possibly asteroid\underline{s}, on the cur\underline{se}.
In the huge tri\underline{fi}d nebul\underline{a}, 5400 light years away from the Earth\underline{,} new stars emerge from gas and dust\underline{.}
The mirror of the Southern African Large Tele\underline{scope} in South Africa is segment\underline{ed} - to save costs.
Despite the comparative\underline{ly} small mirror diameter\underline{,} this is equivalent to that of the world's largest mirror telescope\underline{s}.
With the help of a radio telescope in Are\underline{ci}bo (Pu\underline{er}to Rico\underline{),} researchers listen to space for extraterre\underline{stri}\underline{al} signals\underline{.}
Its main mirror is supposed to cover 42 meters - and be made up of nearly 1000 mirror elements.
On February 2, 2011\underline{,} the Nasa announced that 1235 planet\underline{ary} candidates have been identified since the start of the mission\underline{.}
The James Webb Space Tele\underline{scope} (JWST) will not launch into space until 2018 at the earliest on board an Ariane\underline{5} rocket\underline{.}
But Rembrand\underline{t} Sc\underline{holz}\underline{,} an old-age researcher at the Max Planck Institute in Rostock\underline{,} has also heard of the senior citizens of Central Asia.
However, due to a lack of documents, there should be no scientific evidence of age, especially as there was no register of persons.
In the kitchen, guests can enjoy tea served in the typical arm\underline{a}du glass\underline{es}.
Through twitter\underline{,} he accused the supporters of Mor\underline{si} of wanting to carry a "clash against democracy."
And several judges announced that they did not want to monitor the referendum\underline{,} making it invalid\underline{.}
These measures are blatant violations of democratic rules of play and will lead Egypt into a new dictatorship\underline{.}
A demonstr\underline{ator} on the Tahrir warns: 'You are running a monster you can no longer control'.
For example, you can imagine the wet smell of Rakfisk, one of Norway\underline{'}s great delicacies\underline{.}
Around us people consume small fish cu\underline{bes} and consume large amounts of alcohol\underline{.}
After 81 years in power, the PRI was replaced by Vice\underline{nte} Fox in 2000.
When President Pen\underline{a} Nie\underline{to} receives the Presidential Bin\underline{ding} on Saturday\underline{,} he also assume\underline{s} a great responsibility.
Our identity may sometimes be blu\underline{r}red, but it is not true of our loyalty\underline{.}
The Israeli\underline{-}Ha\underline{mas} ceasefire may turn out to be an unexpected pillar of peace.
Indeed, Hamas in the West Bank, controlled by the rival\underline{,} moderate Palestinian group, Fatah\underline{,} is gaining in.
The Israeli missile defence system, 'Iron Dom\underline{e}', has proved itself and many of Hamas rocket\underline{s} have been destroyed\underline{.}
"The laws will lead to serious, unintended consequences," says Scott Mc\underline{In}tyre of British American Tobac\underline{co} Australia\underline{.}
Meanwhile\underline{,} they have been extended to more than 40 countries, including Brazil\underline{,} Turkey and Ukraine.
"I used to take an hour to sort a delivery, now I need four," Yu says\underline{.}
This forces the brain to get lost in interesting thoughts\underline{,} which may encourage creativity\underline{.}
Sometimes we believe that we are bo\underline{ring}, even if we only have difficulty in focusing\underline{.}
The child not only learns to talk, but also has more self-control in other areas.
My biggest dream has always been to get a place at Oxford University.
Well\underline{,} recent reports suggest that a new generation of moderate\underline{-}right students suffer similar persecution\underline{.}
In other universities\underline{,} conservative students say they are regarded as scape\underline{go}ats for the introduction of higher tu\underline{ition} fees\underline{.}
In the 1960\underline{s} and 1970\underline{s} the two lived in the Alps and were good friends.
I like the colors he uses very much; they have a lot of light and underline the face.
"I have always noticed his refine\underline{ment}, his calm\underline{ness}, his well-kept and perfect appearance\underline{",} admit\underline{s} D'Ar\underline{enberg}\underline{.}
Jorge insure\underline{s} to know 35 friends he has in FB and nine followers in Twitter\underline{.}
Unlike Jorge\underline{,} this boy would upload photos of acquaint\underline{ance}s in uncomfortable or embarrassing situations\underline{.}
Yes\underline{,} I would do that if he is unsym\underline{path}\underline{etic} to me or if I want to wipe him out.
Did you ask the other people for permission if you have labelled photos of celebration\underline{s}?
According to Guard\underline{ia}, children must be reminded of the lesson "You should not speak to strange\underline{rs}".
"I may meet President Daniel Ortega tomorrow (Satur\underline{day})," Santo\underline{s} said.
The change was to improve, I eat well, exercise and take the medication\underline{s}.
The issue is the first of four equal emissions, which promise to pay interest every 28 days.
This was the beginning of Min\underline{cy}, one of the best players Puerto Rico ever had.
And this without taking into account his career in the various league\underline{s} in which he played.
But it was his master\underline{ful} interpretation of the magical\underline{ly} despic\underline{able} J.R. that made Hag\underline{man} a superstar.
Martin was still a young man when she got Larry during her marriage with lawyer Ben Hag\underline{man}.
The 25-year\underline{-}old student Will Wekes\underline{a} for Psycho\underline{logy} and Nursing explains that he has seen all apocalyptic films\underline{.}
The new electoral laws require voters to present a photo ID and proof of US citizenship\underline{.}
Before the 2006 elections, no US state asked voters to present a photo ID\underline{.}
However, more than a hundred dollars are often required to obtain the required card.
For example, only 16 of the 34 states have passed laws requiring the presentation of a photo ID\underline{.}
However, the new rules introduced in 2012 will undoubtedly make it difficult to exercise the right to vote.
In too many cases, it increases the risk of developing cancer of the wrath or fat\underline{ten}ing arm\underline{.}
The preservation of meat by smoking\underline{,} dry\underline{ing} or salt\underline{ing} can lead to the formation of carcinogen\underline{s}.
A few weeks ago Mr. L. lived alone in his apartment in Mont xe9r xe9gie\underline{.}
Patient\underline{s} admitted to the Victor\underline{-}Ga\underline{db}\underline{ois} Pal\underline{li}ative Care Home are all suffering from cancer\underline{.}
For Mrs A., 89 years, the worst fear is to die 'conscious\underline{ly} and by suff\underline{oc}\underline{ation}'.
I fear that patients will die only because they do not receive adequate healthcare\underline{.}
At the same time, despite the worst prediction\underline{s}, several oncologist\underline{s} are treating their patients hard to the last day.
The chances of survival of H xe9l xe8ne Richard were already minimal when she discontinu\underline{ed} an arduous chemotherapy\underline{.}
However, it must be stated clearly that pal\underline{li}ative care is not om\underline{ni}pot\underline{ent} in pain treatment.
We can no longer pretend that we do not perceive this side of suffering\underline{.}
He is supported by co-train\underline{ers} like Claude Make\underline{le}le, who played in the same position as me.
He has a rich experience and won many titles with prestigious clubs\underline{.}
The confidence he has placed in me is also an explanation for my achievements\underline{.}
In view of the sums invested\underline{,} you were believed to be 15-point ahead of the game.
That is why he has come and prove\underline{s} that he is the star of Ligue 1.
With Bit\underline{co}in, all network nodes are simultaneously cu\underline{sto}\underline{dian}\underline{s} of the invoice book, auditor\underline{s}, money issuers as well as buyer\underline{s} and seller\underline{s}.
In order to reach the quo\underline{rum}\underline{,} 11 people, deputy members, were added yesterday morning in a hurry\underline{.}
And in the future the question could be raised as to the extent to which civilian judges are competent to decide on this.'
In your opinion, the only positive point is the ban on torture under Article 36\underline{.}
They are located on a rock face in the mountains at 450 meters above sea level.
And there are the names of the Jewish children and the lands in which they died.
The dead sea is even warmer and bathed all year round.
These secret\underline{s} lie in the old town of Tel Aviv\underline{,} the town of Jaff\underline{a} on the Mediterranean coast\underline{.}
The famous sea route connecting Egypt\underline{,} Syria\underline{,} Anatol\underline{ia} and Mesopot\underline{ami}\underline{a} ran through this city.
In particular, the immigration authorities spoke\underline{s}person\underline{s} said, it is a question of reducing the number of forced labourers.
If you do not have this status, there is no examination and therefore no official work.
Many migrants confirm that it is not easy to obtain official status in Russia.
At the moment, according to the authors\underline{,} every possible weapon for little money can be found in Moscow\underline{.}
The prices and assortment of goods made Wal\underline{mar}t one of the largest companies in the USA.
For them, this would be a year-on-year increase in spending of only \$1\underline{2.}\underline{39}\underline{.}
At present, according to federal and New York legislation, the minimum wage is \$7.25 an hour\underline{.}
I cannot understand how it is possible to spend so little money in New York.
In fact, any kind of interaction with computers is good, but each in its particular ni\underline{che}.
It is still relatively large, but could theoretical\underline{ly} be reduced to the size of a wristwatch\underline{.}
Where\underline{ver} the pictures of Kir\underline{ill} Mill\underline{er} are exhibit\underline{ed}, they attract large crowd\underline{s} of people.
I am attracted to theatre\underline{,} fashion\underline{,} music, in fact everything except literature\underline{.}
The gallery "D 137\underline{"} and the club "Griboedov" also have their origins in the art clinic\underline{.}
I won in the category "artist of the year" and I reached the peak\underline{.}
Caravan\underline{s} of spaceships with Earth inhabitants on board are looking for a replacement planet\underline{.}
The question of reproduction in space was first discussed by researchers with regard to flora\underline{.}
Homo sapiens is capable of abstract thinking and can create a similar emotional background\underline{.}
Without feeling the grace\underline{,} the body cannot train the skel\underline{e}ton and muscle\underline{s}.
A similar result appears to be the joint control of Czech and German auditor\underline{s}.
As a negative example, he leads the recruitment of Prime Minister Petr Ne  u2047 as to the so-called 'black\underline{'} system.
However, lowering threshold\underline{s} for contracts does not guarantee that we will achieve this objective.
In the district of Karl\underline{ov}y Vary, this morning the roads were easy to navigate\underline{,} and there were some smooth snow and ice\underline{.}
This is fro\underline{s}ty in the morning, with temperatures between 3 and 9 degrees below freezing\underline{.}
Of course, and at the very end, provided that everything works and that the end of the world does not happen...
The students of the Jedli  u2047 ka Institute are regularly supervise\underline{d} by lecture\underline{rs} who help them with various leisure activities.
It is not even self-evident there that a wheelchair user is left in the elevator\underline{,} for example.
Fortunately\underline{,} clubs are also being created there which try to highlight the problems of people with disabilities\underline{.}
From the very beginning I felt the potential that things could be tackled differently\underline{.}
The first impression the viewer usually has is, of course, compassion; that is only natural...
This is how it works everywhere\underline{,} in any band that wants to work seriously and achieve something.
We are an open group, people come and go, and that cannot be prevented\underline{.}
The committee was set up in 1937\underline{,} but after two years of work his work was finished from the beginning of the war.
The proof of this is the existence of a lobby that is practically om\underline{ni}pot\underline{ent} and om\underline{ni}present in all the Member States.
The history of humanity is primarily a history of struggle for power.
Who\underline{ever} tried to oppose this family had to pay with life for it.
A world in which the rest of the human population serves a small group of financial aristo\underline{c}rats\underline{.}
The fate of the hostage\underline{s} caused a wave of solidarity and anti-Iranian sentiment at home.
The plan, developed by the expert for "Ex\underline{filtration}\underline{",} Tony Mendez, also required Hollywood\underline{'}s cooperation.
A similar restriction already applies to children up to 14 years of age in the use of Christmas roast\underline{s}.
The Czech Republic, for example, then exceeded the fixed volume for canned mushroom\underline{s}, for which we were threatened with a large fine.
Mr Senator\underline{,} how do you think you can stand for President?
People have chosen such a senate composition that changes will be very difficult to enforce\underline{.}
Nevertheless\underline{,} I will fight for my vision\underline{s}, e.g. for the direct election of mayor\underline{s} and district leaders.
The cost of the campaign is basically covered by my salary as a senator.
So that is my proposal for the Sp\underline{ijk}\underline{en}isse bookberg, for the so-called Boekenberg\underline{!}
At the beginning of November the Buchberg was awarded the second prize "Best Library of NL 2012\underline{".}
A special pleasure are the black book shelves\underline{,} which are sometimes wall covering\underline{s}, sometimes arm\underline{or}, sometimes rod rail\underline{ing}s.
According to Stephen Szabo, an expert on US-European relations, Berlin is thus balancing on a narrow diplomatic level.
However, given the political situation here, the government cannot, of course, publicly defend this position.
I believe that the real differences are not as great as they always appear.
But I believe that the Germans understand that they must play a more independent role.
Five years ago, Freud\underline{enberg} offered the other side in va\underline{in} a "high six-digit euro amount" for settlement\underline{.}
For example, a Chinese manufacturer in Germany wanted to register the name Freud\underline{enberg} for shoes and leather\underline{.}
More than 300 of them no longer have parents because they have suc\underline{cum}\underline{bed} to the HI virus\underline{.}
According to European survey\underline{s}, three quarter\underline{s} of all infection\underline{s} affect young people aged between 15 and 25.
In the village itself, Zo\underline{d}wa Dlamini\underline{,} a confident and assert\underline{ive} woman\underline{,} manages the funds from Germany.
She also ensures that the orphan\underline{s} are well accommodate\underline{d}, for example, among the grand\underline{m}other\underline{s}.
The Gogos, as the old women on Zulu are the supports of the village.
'Aids is an absolute taboo\underline{'}, says Anne\underline{tte} Lennar\underline{tz}\underline{,} 'because it has to do with sexual\underline{ity}'.
The probe messenger has found evidence that there is ice on the planet Mercury\underline{.}
The ple\underline{ja}de cluster\underline{,} also called "The Seven Sister\underline{s}", can be seen with the naked eye at night.
This baby star could only be taken in its full beauty by the infrared detect\underline{ors} of the Spitze\underline{r} telescope\underline{.}
Saturn and its ring\underline{s}: How these were created is one of the great puzzle\underline{s} of astronom\underline{y}.
This group of galaxies\underline{,} called Arp 273, took up the Hubble space telescope for the nasa.
Tourist\underline{s} from Europe hardly come here, too difficult to get to from Azerbaijan\underline{'}s capital Baku.
She has always only eat\underline{en} what came from her own farm\underline{,} tomato\underline{es}, potatoes\underline{,} peas.
For this, another person forbid\underline{s} to insult or slander the Prophet Mohammed and his messenger\underline{s}.
"Instead of strengthening civil society, the President de facto suspend\underline{s} it," Saeda complain\underline{s}.
Inhabit\underline{ants} of the resort attribute to him the development of tourism and the construction of infrastructure.
He is a very direct man, very committed and has great plans for the country.
He is an excellent statesman, but above all he is someone who can listen\underline{.}
"But this is not possible if there were so many formal errors and omission\underline{s}," she says\underline{.}
Not to know what has happened to him or to the outside world has been a burden\underline{.}
We are also aware that many members of Mexico u2019s ruling class do not like us.
But there are reasons to believe that the dead\underline{ly} sta\underline{le}mate could finally come to an end.
And Hamas leaders may conclude that they have time on their side.
Chinese and Indonesia\underline{n} counterfeit\underline{ers} will offer far larger quantities of these products on the streets of Australia\underline{.}
The house walls of Pompeii ador\underline{n} a Latin gra\underline{ffi}\underline{ti} about bo\underline{re}dom dating back to the first century.
In order to measure these differences\underline{,} researchers developed a "scala to bo\underline{re}dom vulnerability\underline{"} in the 1980\underline{s}.
Instead\underline{,} our aim should be to feel comfortable away from the constant activity and technology giant\underline{.}
Not because of my rather unusual name or because I came from a private school.
People believe we are like the Bull\underline{ing}don Club without even getting to know us".
"Mi\underline{s}s Wyatt\underline{",} said the tut\underline{or} Harry Pit\underline{t} (decea\underline{s}ed), "ple\underline{ase} translate the first paragraph\underline{".}
"Do Thatcher supporters refuse to learn French, or are they just stupid\underline{?}" he asked me.
I insisted that I did not agree with Mrs Thatcher on all points.
In 1997 he took a professor\underline{ship} at Bilk\underline{ent} University in Ankara\underline{,} Turkey.
But no 18-year\underline{-}old should ever suffer such intimidation and malice in an educational institution\underline{.}
He sat at the table of Count\underline{es}s Jacqueline de Ribes\underline{,} a very good friend of mine\underline{.}
Kawah Ijen's mine\underline{work}\underline{ers} earn 5 euro cent\underline{s} for every kilo of sulphur they extract\underline{.}
"I don't know if someone answers me, I just invite them up," he adds\underline{.}
"It doesn\underline{'}t fright\underline{en} me because we have something in common, for example music," he says\underline{.}
The digital Natives are they, the children and young people who have grown up with this technology.
"If I have to die, then I would rather burst three times," is said in my case.
There are things that I would have introduced, such as regionalisation of lower categories\underline{.}
At least I see the result of the prescribed trainings and courses for trainers, table officials and referees.
And of course I enjoy the company of my wife Isabel\underline{,} who has always been with me.
He was creative\underline{,} generous\underline{,} fun, funny\underline{,} loving and talented\underline{,} and I will miss him very much.
In 1995, a malign\underline{ant} tum\underline{our} was found in his liver and he was subjected to a transplantation\underline{.}
In 2001 he named his memoirs "Hello Dar\underline{lin}: Tall (and Absolut\underline{e}ly Tru\underline{e}) Tal\underline{es} about My Life\underline{".}
For weeks before the beginning of the semester\underline{,} we received e-mails from students who asked if there were still places available.
The apocalyptic sec\underline{t} or religious mental\underline{ity} is actually only a question of consol\underline{ation} or its absence\underline{.}
"Never have I heard of a lesson where this is taught\underline{,}" he said.
Republican leaders justify their policies by the need to combat electoral fraud\underline{.}
Moreover, five million new voters in 2012 do not have such a card.
But one thing is certain: these new rules will have a negative impact on turnout.
This leads to greater hesitation on the part of men who are already indecisive in carrying out early detection tests\underline{.}
"To\underline{day} there are 1.5 million smokers in Quebec\underline{",} regret\underline{s} spoke\underline{s}man Andr xe9 Beau\underline{lie}\underline{u}.
They appear to increase the risk of breast\underline{,} wrath intest\underline{in}al, fat\underline{ten}ing, oesopha\underline{gus}\underline{,} pan\underline{cre}\underline{atic} and cer\underline{v}ical cancer\underline{.}
In recent years, several scientists have studied the link between vitamin supplement\underline{s} and cancer\underline{.}
The effect of vitamin D on cancer has not yet been clearly demonstrated either.
In addition, applications can also come from all the instruments surrounding research.
"It is always a shock\underline{,} you cannot be prepared for it," he says\underline{.}
"Th\underline{at} depends on the person's ability," he notes\underline{,} to accept a retro\underline{grade} step.
That is very little, bearing in mind that one day we will all die.
Patient\underline{s} without pain relief will increasingly have the opportunity to resort to this terminal sedation.
In May we were disappointed because we were strong enough to win\underline{.}
We have punished Afghan farmers in particular by treating them as terrorists\underline{.}
The convoys of truck\underline{s} and tank\underline{s} flood\underline{ed} by helicopter\underline{s} have reached Kabul without being attacked\underline{.}
President Kar\underline{za}  u2047  does not want any foreign controls\underline{,} especially on the occasion of the elections scheduled for April 2014\underline{.}
Traditional\underline{ly}, people of different faith\underline{s} leave signs there with wishes\underline{,} which are then fulfilled\underline{.}
For this there are many well-nour\underline{ished} cat\underline{s} that sp\underline{rin}\underline{kle} through the streets in peace and quiet.
In 2012\underline{,} more than three million tourists from all over the world visited Israel.
Language skills must be proven both for obtaining and for extending the work permit\underline{.}
In 2011\underline{,} a report was drawn up by the Center for Problem Analysis and State Administration\underline{.}
According to him, it is more common for dealers to obtain supplies in a stock\underline{pil}\underline{e}.
A weapon\underline{,} such as a TT\underline{-}type gun\underline{,} is purchased via an Ensign\underline{.}
According to Baranez, the buyer does not get the cat in the bag\underline{,} but can try everything.
But the creation of trade unions in the fast-food industry is also difficult for objective reasons.
There were loud protests this day before many other fast-food restaurants in Manhattan\underline{.}
An interesting method is currently using the second hand as a somewhat unusual projection document.
I used to be social, but now it hurt\underline{s} and is afraid to be so.
In fact, there are only two real planet\underline{s} that we could inhabit at least hypothe\underline{t}ically\underline{.}
Animal\underline{s} taken out of their natural habitat simply cannot follow their reproductive drive.
Here in a suspended state, the cosmonaut\underline{s} gain routine for work in open space.
For example, birth could also take place in a special chamber to blackmail the child.
Is there a similar authority here to our NK  u2047 , or does the system work differently\underline{?}
Temperatur\underline{es} dropped to -5 to -10   u2047 C, during the day it should become a bit warmer.
In East Bohemia\underline{,} it is mostly sunny or lighter today, and it remains largely rain\underline{-}free\underline{.}
The temperature ranges from -3 to +1   u2047 C, the wind is weak\underline{.}
However, in the south of Pil\underline{s}en and Tachov circle\underline{s} ice\underline{-}smooth can occur\underline{.}
Drive\underline{rs} should be particularly careful on the less frequent\underline{ed} roads in the area of   u2047 umava\underline{.}
What do you think about the end of the world happening in less than a month?
In December you will also realize a unique project with three concerts against the end of the world.
However, The Tap is a group of people with disabilities\underline{.}
But the band has only become known in recent years, or am I wrong?
Thanks to EU funding, we can also afford good lecture\underline{rs}, high-quality equipment and so on.
Who\underline{ever} has the will and the desire to participate is always welcome.
Find\underline{s} taking place the day before the predicted end of the world, Thursday\underline{,} 20.\underline{12}.2012 at 9 p.m.
It is certainly interesting to look at the issue from a broader perspective\underline{.}
Ultimate\underline{ly}, this means that individual economies are in permanent conflict with each other.
This situation is well known, so there is no need for specific statistics at this point.
Such a scandal was also exposed in the case of auxiliar\underline{y} staff working in the German Bundestag\underline{.}
The repeal of the law on voluntary work is not a solution here, at least not a permanent one.
At the same time, it is Affleck\underline{'}s first film that does not play in the director\underline{'}s hometown Boston\underline{.}
Affleck also prove\underline{s} this feeling in Argo, where Tehra\underline{n} is "play\underline{ed}" by Canada\underline{.}
The Par\underline{du}bic\underline{ian} gingerbread or the Ho  u2047 ic roll\underline{s} can boast of an EU brand.
A strong personality who points to maladministration can put pressure on the political scene\underline{.}
The thin fabric holds one or two seasons, after which it is rip\underline{e} for the bulk waste.
Germany abstained in the vote on the admission of Palestine\underline{.}
Germany wanted to demonstrate its independence without being too critical of Israel.
That is actually the old problem: you do not want to be surrounded by hostile countries.
It must be recep\underline{tive} to various neighbours and opinions\underline{,} and that is not easy.
A few additional letters are enough for copy\underline{ers} to register their trademarks\underline{.}
We know that the Chinese are world champion\underline{s} in copy\underline{ing} and injuring intellectual property.
However, deletion\underline{s} of dubious records in the trademark register are difficult to reach and go into money.
Last year, however, we had moved from the 'emerg\underline{ency} situation in the workflow to normality'.
Simpl\underline{ified}\underline{,} this means that each registration costs an average of 1280 yu\underline{an} or 160 euros\underline{.}
In Heidelberg the choir is testing Imbon\underline{gi} - and in Swaziland AIDS wa\underline{is}en are happy about it.
Sy\underline{phil}\underline{is} and Tripper are especially common in men who have sex with men.
It is really strange in a country where the King officially holds 14 wi\underline{ves}\underline{.}
The last absolute monarch of Sub\underline{-}Saharan Africa, King Mswati III\underline{,} is known for his excessive lifestyle\underline{.}
It should be at least 30 cent\underline{i}metre\underline{s} thick and possibly up to 20 metres thick\underline{.}
From time to time they send pictures to the earth\underline{:} small gap\underline{s} in infinite exp\underline{ans}\underline{es}.
They may be the remains of a Saturn Mon\underline{th} that disappeared without trace some 4.5 billion years ago.
Those who do not have technical abbreviations may call their nickname the Southern Fire\underline{wheel}\underline{.}
The photo of the Hubble space telescope shows an exc\underline{er}pt from the Iris\underline{ne}bel in the constell\underline{ation} Ke\underline{ph}eus.
It shows a ring of black holes\underline{,} 430 million light years away from Earth\underline{.}
It takes eight hours for the 323 km because the road is only one lane.
However, Pil\underline{ata} Fatulay\underline{eva} (48\underline{)} is convinced that Lerik is a tourist attraction\underline{.}
She is the director of the Museum of Long\underline{ev}\underline{ity}, probably the only one in the world.
She sit\underline{s} on the floor with a butter keg that she tire\underline{lessly} roll\underline{s} back and forth\underline{.}
For my whole life I have not once bought food in the supermarket\underline{.}
He was in power until 2003, and later his son Il\underline{ham} took over.
Is there enough caricature of the President or a joke at the expense of a lawyer\underline{?}
"The revolution has returned and we will win\underline{,}" said Ham\underline{din} Sabbahi, a third-place\underline{d} presidential candidate\underline{.}
They asked Mor\underline{si} to clean up the country and said: 'The Kor\underline{an} is our Constitution\underline{'}.
Not because he would share their view of the world, but because human rights are indivisible to him.
I am in the small town of Fagernes, about three hours from Oslo\underline{.}
Such a moose surge\underline{on} is definitely something different.
'What score do you have up there in the mountains for the best fish, Thor\underline{-}J xfcrgen?'
In the remote town of Valle del Bra\underline{vo}, for example, one likes to remember him.
He reject\underline{s} the opposition u2019s accus\underline{ations} that the new president lacks substance\underline{.}
Yet this is precisely what the families of the victims in Ciudad Neza fear most.
"My world sh\underline{rank} on Camp Araf\underline{jon}\underline{,} on this cage combined\underline{,}" said Manning on Thursday\underline{.}
He was allowed only one mattress\underline{,} a blanket\underline{,} flip flo\underline{ps}, clothes and glass\underline{es}.
He always had to sleep with light that penetrate\underline{d} his cell from the outside.
Sign\underline{s} pointed to two queue\underline{s}: one for "Me\underline{xi}\underline{can}\underline{os}" ("\underline{Me}\underline{xi}\underline{can}\underline{s}")\underline{,} the other for "Ex\underline{tra}njeros\underline{"} ("\underline{Aus}\underline{l} xe4nder\underline{").}
And in my grand\underline{fa}ther\underline{'}s homeland there was no need for shortcut\underline{s} or hy\underline{phen}\underline{s}.
So I took my American passport and put myself in the snake for extranjeros\underline{.}
Our Spanish will never be good enough, our ties to Mexico will never be strong enough.
At first sight\underline{,} optimism seems to be far from appropriate given the current situation.
Far away in the white house, it seems he is also opposed to participation.
Health warning\underline{s} and ill body parts on neutral green packet\underline{s} equal to all tobacco brands\underline{.}
Zi\underline{co} has sold up to 6,000 units to wholesale\underline{rs} and is waiting for new stocks\underline{.}
According to Plib\underline{ers}ek, the government has held talks with other countries considering similar packaging legislation.
So I had enough time to think about bo\underline{re}dom\underline{.}
But, while television can provide happiness in the short term, they eva\underline{po}rate in the long run.
Pit\underline{t} was a small man with a face like cake dough\underline{,} and quite ugly.
Would I ever be able to live a normal life at Oxford University?
One of my male friends, also Tory fan\underline{,} had suc\underline{cum}\underline{bed} to pressure and renounce\underline{d} his conviction\underline{s}.
It was my father who beat the last nail into the coffi\underline{n} of my Oxford career\underline{.}
I hi\underline{d} in my room and after five minutes I gave up my chicken\underline{s}.
When they went\underline{,} I packed a suit\underline{case} and took the first train to London.
"He never comes out of fashion because his designs are works of art" she conclude\underline{s}.
He likes people with good education and the highest titles, and they love him.
"It was a gift from him," says Naty Abascal, one of the designer\underline{'}s museums\underline{.}
About 400 wear\underline{ers} load their basket\underline{s} with sulphur on their shoulders on the cra\underline{ter} floor.
Of his five children, the elder, with his 30 years of age, also works as a sul\underline{fur} carrier\underline{.}
This is something just for the Internet, so we had to make it fun and funny\underline{.}
Possible that many of these ideas were creative\underline{,} but they did not necessarily lead to success.
I signed up on Twitter to express myself and write interesting tweets\underline{.}
Journalist\underline{s}' access to information about the summit was limited at all times.
Conflict\underline{s} are inevitable\underline{,} but they must be overcome in the pursuit of a common path.
They must be dealt with comprehensively so that they can be overcome and looked forward.
"In no case does it mean a return to President Ch xe1vez's state of health," he commented.
They were many fulfilling years, including the five championship\underline{s} in succession from 1971 to 1975\underline{.}
Was this group of the 1990 World Cup the best national team you ever saw\underline{?}
It was Krist\underline{in} who had shot the sister\underline{-}in-law of J.R. (interpret\underline{ed} by Mary Cro\underline{s}by).
He also campaign\underline{ed} against smoking and participated in several campaigns\underline{.}
And he reminds us that the bad is good for those with apocalyptic mental\underline{ity}.
For example, if nuclear material comes into the hands of terrorists\underline{,} a war could break out.
Despite the "pre\underline{v}ious doom" the students must study, prepare projects and take part in audit\underline{s}.
One thing is certain: these new rules will have a negative impact on turnout.
Before 2004, no state called for proof of citizenship\underline{.}
The most important thing is to make the right decision once a cancer has been identified\underline{.}
However, it is assumed that about 10\% of cancer\underline{s} are caused by inheritance\underline{.}
According to the Canadian cancer society, obesity and obesity also promote the outbreak of the disease\underline{.}
"The latter can damage body cells and lead to the development of cancer\underline{,}" he explains\underline{.}
The debate must resume shortly\underline{,} even though a draft law is being prepared.
The prostate cancer that consumed him had left him a two-year period.
The dying person is given a mouth care with brandy or pepsi.
Patient\underline{s} whose pain is not relieve\underline{d} say the same thing: 'I want to die'.
He is suspected of repeatedly receiving bri\underline{bes} in exchange for public contracts\underline{.}
Financial\underline{ly}, the PS\underline{G} is giving itself the means to make this project a reality.
But another team, that of Mont\underline{pell}\underline{ier}, has achieved an even better season.
That would mean ignor\underline{ing} our opponents and the French championship\underline{.}
The PS\underline{G} seems to be completely dependent on the performance of Zlat\underline{an} Ibra\underline{hi}movic\underline{.}
The national coach is strict\underline{,} close to the players and encourages victory\underline{.}
Blanc had reached his goal by qualify\underline{ing} us for the European Championship\underline{.}
Is the imdecision imposed on October 16 in Spain (1\underline{:}1) a prelude?
However, each time trade is controlled and processed by a central authority\underline{.}
To prevent inflation\underline{,} this reward is regularly halv\underline{ed}, probably before the end of 2012\underline{.}
In addition, the difficulty of the task is increased with each improvement in computing power.
The websites providing services for Bit\underline{co}in have been attacked and the Bit\underline{co}in insol\underline{es} stolen\underline{.}
The ECB also reports on the possibilities of money laundering through this anonymous service.
And ourselves with our 88 soldiers killed\underline{,} as well as the injured and the injured\underline{.}
From the end of 2014\underline{,} the Taliban will no longer be invaded in Kabul\underline{.}
Conditions have changed since their irre\underline{s}istible advance from 1994 to 1996.
Their takeover was then seen as a kind of liberation and return to security.
The most important figures of the anti-Sovi\underline{et} war returned to power in 2001.
This new initiative has only created an even greater division of the country.
The text adopted last night is made up of 234 articles\underline{.}
This refers in particular to the "Fiq\underline{h}" [Islam\underline{ic} ju\underline{ris}\underline{pru}\underline{d}ence, Note d. Red.].
The Mos\underline{lem} brother\underline{s} argue that these are marked\underline{ly} reduced compared to the former regime.
This is where believers take the ordeal or the Way of the Cross of Jesus Christ (in Latin\underline{:} Via Dol\underline{or}osa\underline{).}
Every year, 13 million guest workers come to Moscow\underline{,} St. Petersburg and other Russian cities.
Most of them are the citizens of Central Asia: Uzbekistan\underline{,} Taji\underline{k}istan and Turkmenistan\underline{.}
The second channel contains illegal weapons stolen by criminals.
At the moment I even come to some ring\underline{s} about a friend I trust.
It is not yet clear whether the spark of these protests will mobil\underline{ize} entire masses.
But we want to look forward to 5-10 years and anticipate the radical changes of this interaction\underline{.}
We must release the computer world into our physical world and make it more tangible\underline{.}
- We would ask you, for example, to give you this bubble can?
Not everyone understands how much this influences the interaction of man and machine.
I think the eight\underline{h} breakthrough could well be the integration of ta\underline{c}tile perception\underline{.}
- This is a good idea, we have not tried it yet.
Kir\underline{ill} Mill\underline{er} is one of the typical Petersburg social-phil\underline{oso}\underline{ph}ical artists who create new myth\underline{s}.
- At an exhibition at the Newskiy Palace of Culture\underline{,} where my works were exhibit\underline{ed}.
I will have an exhibition entitled 'The Russian Museum as Clow\underline{n}s'.
- There are abandoned women coming to him, where the sexual\underline{-}social sphere plays a role.
"Near Mars and Venus\underline{,}" says the scientific assistant of the Astronom\underline{ical} Stern\underline{berg} Institute Vladimir Sur\underline{din}\underline{.}
The breeding of insect\underline{s} followed, more precisely of tiny fruit flies (Dr\underline{oso}\underline{phil}\underline{a}), in orbit.
There was an experiment with rats that were already fer\underline{til}\underline{ized} into space.
The hydro\underline{labor}\underline{atory} in the Cosmonaut preparation centre is a compulsory station during flight preparation\underline{.}
"This is not enough time to forget something," says baby swim\underline{mer} teacher Marina Ak\underline{s}enowa.
He will simply miss what is fundamental to his life.
That is certainly not the case, but as I said, I do not like such comparison\underline{s}.
Otherwise they would have nothing of cooperation with our authority\underline{,} would they not?
As our controls take place after the event, there is a certain delay here.
You can also use all the second and third class roads\underline{,} including the mountain roads\underline{.}
Snow lies in particular on the roads in the Gian\underline{t} Mountains and the Orlick xe9 hor\underline{y} Mountains\underline{.}
This is one of the disasters to which we humans are so keen\underline{.}
It is a national benefit event that we have been planning for two years.
The anthem is to be sung by all perform\underline{ers} on all three concerts at the same time.
In addition, the anthems will be broadcast live on Czech television in a direct line.
Was it your goal to get it that far with The Tap\underline{?}
In 1933\underline{,} the Polish infant\underline{ry} began to deal with rocket\underline{-}power\underline{ed} missile\underline{s}.
The article by Prof\underline{.} M. Sub\underline{ot}owicz contains the proposal to create a space company.
Last week, the Constitutional Court repeal\underline{ed} the law on non-profit work.
Due to the large differences in the value of work (simil\underline{ar}) there are price tensions\underline{.}
The result is growing poverty, as well as increasing differences between rich and poor.
In every era we can make an Alexander the Great or Napoleon\underline{.}
In its conception\underline{,} the new world order is a world of master\underline{s} and slave\underline{s}.
"Mor\underline{e} incredible invention\underline{s} from the EU workshop can be nominated by the end of this year.
If everything worked without problems in our country, I would not stand anywhere\underline{.}
You are already looking for park bench\underline{,} dog and football\underline{-}play\underline{ing} guy\underline{s} and girls\underline{.}
They provide for atmosphere, but above all for the right hum\underline{id}ity in the literature mountains\underline{.}
Stephen Szabo: Germany does not support what the Israelis have done in Gaza\underline{.}
Is it difficult for Germany to adopt a clear position on important international issues?
On the one hand, Germany has large markets in the Middle East, especially in the Gulf States.
Of course, this is not easy for Germany, because of its relationship with Israel.
German companies are also legally copied in this way, such as the sports goods manufacturer Pu\underline{ma}.
In the major cities, there are multi-storey department stores that sell counterfeit\underline{s} almost exclusively\underline{.}
The Chinese are therefore still allowed to use an em\underline{ble}\underline{m} similar to the Mercedes star.
Almost 57,000 such cases were closed, 75 percent more than last year.
This also applies to the stock of all valid trademarks\underline{,} a total of 5.5 million pieces\underline{.}
Address\underline{ing} this, as the case of the German family business Freud\underline{enberg} shows, costs many times more.
It is true that the Germans managed to get rid of their illegal factory of imitated car parts.
But the mi\underline{mic} continued to secure China u2019s rights to the Freud\underline{enberg} brand.
The Group has long given up this business, but it was able to avoid registration\underline{.}
It guarantees the child school fees\underline{,} school uniform and a warm meal daily in the Gogo Center.
However, they often do not cause any pain or other symptom\underline{s} and therefore remain unnotic\underline{ed}.
The trip will always take you to Esitjeni, where the singer\underline{s} will visit their god\underline{child}\underline{ren}.
The US space agency NAS\underline{A} has demonstrated the existence of ice on the planet Mercury\underline{.}
The picture comes from a camera developed by German researchers from the Max Planck Institute\underline{.}
Like a red age, the helix nebul\underline{a} looks forward to the viewer on this infrared photo.
His similarity to an Earth\underline{ly} continent gave this nebul\underline{a} the title North America.
Here stands the Very Large Tele\underline{scope} - which honour\underline{s} its name.
With its four mirror\underline{s}, the telescope can also illumin\underline{ate} the medium infrared spectrum\underline{.}
For decades\underline{,} radar measurements have indicated that there is ice on the Mercury\underline{.}
Everything is green and ju\underline{ic}y, one might think you are in the Black Forest\underline{.}
"He was born here in the region in 1805\underline{,} he died in 1973\underline{,}" explains Fatulay\underline{eva}\underline{.}
So, has   u2047 ir\underline{ali} M xfcs\underline{l} xfcmov rec\underline{kon}ed with his age by a few decades\underline{?}
Far\underline{id} Mugimzadeh, the Azeri travel guide\underline{,} explains this with the special gene\underline{s} of the Tal\underline{yan}\underline{s}.
But everything got better when the "lov\underline{ed} father\underline{"} Heydar Ali\underline{y}ev took over the helm\underline{.}
If that is not a reason to stay alive for as long as possible.
But what is an insult and how it is to be punished remains unclear\underline{.}
I will propose a new security strategy that will enable us to achieve this objective.
But, at worst\underline{,} his government closed its eyes to the problem.
There were signs that it was beat\underline{en}, and the corps\underline{e} had already set in.
In April 2011 Manning was transferred to the military prison of Fort Leav\underline{en}worth\underline{,} Kan\underline{s}as.
If he is found guilty in all charges\underline{,} he is threatened with a life sentence\underline{.}
I stood there for a few seconds\underline{,} uncertain\underline{,} to which I should go.
I grew up in Central California and was called Mexican\underline{s} all my life.
We love the Mexican band Los Ti\underline{gre}\underline{s} del Nor\underline{te}, but also Bru\underline{ce} Spring\underline{ste}en.
Can there ever be lasting peace between Arab\underline{s} and Jews in the Middle East?
Out\underline{side} Arab nations should also encourage Hamas and Fatah to reach an agreement.
In a constantly elect\underline{r}ified world it is nice to be bo\underline{red} at times.
But the brain does not always know what to do best.
And he adds\underline{:} 'Self\underline{-}control transfers from one situation to another'.
In Weld County in northern Color\underline{ado}, District Prosecutor Ken Buck has a stronger view.
Several cities in Color\underline{ado} are not waiting for the federal authorities to act.
I told my father that I hated Oxford and why I did.
They would never do that, not in my city of dream\underline{ing} spi\underline{res}.
Valentin\underline{o} has always been fascina\underline{ted} by the stick\underline{y} and distant world of nobil\underline{ity}.
We were about 20 people, including Sharon Stone and John Kennedy Jr.
The life of Gar\underline{ava}\underline{ni} is not a story of obsession\underline{,} rather of mutual love.
Many of these customers say that the first Valentin\underline{o} is like the first love, "unforge\underline{t}table\underline{".}
For years with the "savoir\underline{-}  u2047 tre\underline{"} of the elite\underline{,} Valentin\underline{o} is now her best copy\underline{.}
This is the price he has to pay to achieve his dream\underline{.}
According to its national population authority\underline{,} the birth rate currently stands at 1.2 children per woman\underline{.}
The government is trying to ensure that not so many small apartments are built.
These apartments have a living area of 46 square meters and show a great sales success.
As a result, they are much better for our cash flow\underline{.}
When asked, he replied that he would never accept an invitation from a strange\underline{r}.
Jos xe9 joined Ask after reading a recommendation in Twitter\underline{.}
Then he explains a number of steps to configure a user account securely.
And one more question: must everyone know what you are doing at any moment?
And 'if Britain gives this carte blanc\underline{he} tomorrow, I think that is done'.
It is a problem between a South American State and a Central American State.
92\% of contagion occurs through sexual intercourse\underline{,} 6\% through blood and 2\% perinatal.
Indeed, Vitro is not the first case in which this scheme has been approved.
From then on, Ortiz took over "Cuco", who was a very good manager\underline{,}" says Rey\underline{es}.
"I know what should stand on the grave\underline{stone} of J.R.," Hag\underline{man} said in 1988\underline{.}
Several said that they want to go to celebration\underline{s} about 'the end of the world'.
In this sense, these measures are partly undermining the US democratic system.
In this sense, these measures are partly undermining the US democratic system.
What can all these research be 'good\underline{'}, asks Mrs Pla\underline{mond}\underline{on}?
A few hours later the team found a cure for this evil\underline{.}
Pal\underline{li}ative care is used when there are no other options.
This morning, his son will drink beer at the foot of the decea\underline{s}ed.
Chan\underline{tal} Rou\underline{le}au was one of the first to raise the alarm in Montreal\underline{.}
This summer's newcomers are used to playing high-level games.
In Ligue 1, Lyon has taken us to the top.
However, we will have our say against very good European teams\underline{.}
Within the team we respect both the player and the person.
Nothing particularly impressive compared to world trade of real currencies or financial products.
The decisive step is to enter this new transaction into this book.
Moreover, the owner manages his identity and can thus remain anonymous\underline{.}
In cities, state schools are full of girls and boys\underline{.}
Are the authorities under whose authority it will be under its command considered legitimate\underline{?}
AIF gives you the five main reasons for visiting Israel.
It is said that all who bathe in this river receive God's blessing\underline{.}
But at least the five most interesting ones should be visited\underline{.}
The Museum of Art in Tel Aviv is also worth a visit.
In each of the three places there are swimming pools\underline{,} water parks\underline{,} dolphin\underline{s} and ocean aria\underline{s}.
Tourist\underline{s} like to stroll through the narrow alleys named after signs of the Zo\underline{di}ac.
"The Great and Power\underline{ful}" leads to Moscow\underline{:} migrants save money for language.
Except\underline{ions} apply only to citizens of countries in which Russian is official.
Only organized recruitment will solve 90\% of the problems of foreign workers.
As teenagers\underline{,} these children immediately seize the first opportunity to earn money.
Meanwhile\underline{,} the majority of migrant workers remain illegally in Russia.
A fake registration can be done quickly and only for a thousand and a half.
Meanwhile\underline{,} the Ministry of the Interior stresses that the proliferation of illegal weapons is under control.
One in four American youth\underline{s} eventually sit\underline{s} behind Mc Donald\underline{'}s coffer\underline{s}.
That is why many of the low-paid Wal\underline{mar}t workers only buy in at their own workplace\underline{.}
The latter also complain about heavy working conditions, such as missing forklift\underline{s} or hand scanner\underline{s}.
All in all, the Wal\underline{mar}t cassette\underline{s} conducted almost 100 million transactions on Black Friday\underline{.}
Fe\underline{w} saw it as the main source of income or planned to stay there for longer.
Then we would be able to add virtual objects to the real world much more easily.
But overall, the future belongs to mixed modes of control, such as gesture\underline{s} and language.
Of course 8 Megapixel\underline{s} with a speed of 1000 fps would not be bad.
The speed and the number of images per second are also important.
In this world, Rot is the compromise between artist\underline{,} image consultant and society.
However, I want to enter into dialogue with the people through my provocation\underline{s}.
I am a hero of the past century, when culture meant something.
I started with pictures that usually come only at the end of the career\underline{.}
In Europe there are many curious people attending exhibitions or concerts\underline{.}
Art must be modern again, as it was at the beginning of the last century.
The last breeding cage with animals fle\underline{w} into orbit 16 years ago.
The problem of procre\underline{ation} in space has not yet been solved\underline{.}
"But what happens then?" is Wal\underline{er}i Pol\underline{ja}kov\underline{'}s not insignificant question.
You are talking about the problems with the practical implementation of the Czech procurement law.
However, the roads are mostly good for driving\underline{,} and sometimes you need to be careful\underline{.}
In the other areas of the district the roads are mostly unrest\underline{ric}\underline{ted}.
It is not as bad as it appears at first sight\underline{.}
And in what way must we catch up with the more developed countries?
The venue\underline{s} are: Incheba-Ar\underline{ena}\underline{/}Prag\underline{,} Fl xe9da/Brno and Plynojem/Ostra\underline{va}; 12 Czech bands and other musicians\underline{.}
Unfortunately\underline{,} the author of the draft and the details of this project remained unknown\underline{.}
However, research was interrupt\underline{ed} by the invasion of the German Wehrmacht\underline{.}
He held this position until his death in 1959\underline{.}
Count\underline{er} bri\underline{ber}y, unlawful injuring of benefits or with stone and sword\underline{.}
Here's wisdom\underline{!}
Ben Affleck has achieved a remarkable re-start of his career with this film.
Guidelines for balloon\underline{ing}, banana\underline{s} and circus\underline{es}
The actual vote will then take place until the end of February 2013\underline{,}" said Nacher.
Do you see yourself as a person in politics rather right or left?
From a Czech point of view, it seems to me that people tend to see me on the left.
I spoke to Radim Jan  u2047 ura\underline{,} for example, but he refused because of workload\underline{.}
And I am not obliged to fund the campaign from my own resources.
If I just wanted to make money, I would run for nothing.
Do you continue to work as an entrepreneur in order to have your income?
Sp\underline{ijk}\underline{en}isse\underline{,} a dorm\underline{i}tory just outside Rotterdam\underline{,} is a remarkable record holder\underline{.}
The project is also nominated for the Dutch National Wood Award 2012\underline{.}
Even hard-pressed architect\underline{s} and civil engineers shake their heads over the unknown material.
In this way, MV\underline{R}DV has achieved the royal discipline called the Ident\underline{ity} Foundation in jargon\underline{.}
Now, however, Germany must be careful about its special relationship with Israel.
At the same time, however, I do not believe that it supports the American position.
To make matters worse\underline{,} Europeans do not have a coherent and uniform policy.
But it certainly plays an important role in German considerations\underline{.}
From this point of view, Germany is in a much more difficult position than the US.
However, it enjoys protection for as long as the actual names\underline{men} do not complain\underline{.}
So Gucci simply becomes Lu-Gucci\underline{,} instead of Pra\underline{da} you have to enter Pra\underline{da}-Kny.
The procedure may take up to nine years, with an uncertain outcome\underline{.}
For more than seven years, the company has been fighting a Chinese pla\underline{gia}\underline{r}ator.
For 15 or 20 euros a month, you can take on a sponsor\underline{ship}.
Without a school leaving certificate\underline{,} there is no chance in a poor country.
Condom\underline{s} can reduce the risk of contagion, but they do not provide 100\% protection.
The temperature on the Mercury can reach up to 426 degrees Celsius\underline{.}
This dazz\underline{ling} glu\underline{t} of a dying star has captured the  Spitze\underline{r} telescope of the Nasa.
The Don\underline{ut}-shaped ring is made of material that the star eject\underline{ed} in the process of dying\underline{.}
A combination of normal and infra\underline{-}red photo provides for the spectacular colour\underline{ing}.
In this nebul\underline{a} is the bright\underline{est} group of young stars of our Mil\underline{ky} Way\underline{.}
View of the Observatory of the European Observatory (ESO) in the Chile\underline{an} Andes.
The European Extreme\underline{ly} Large Tele\underline{scope} is also planned at the Chile\underline{an} ESO observ\underline{atory}\underline{.}
They offer two mirror\underline{s} each with an average of ten meters\underline{.}
Since 24 April 1990, it has already supplied images from distant worlds.
Sc\underline{ient}\underline{ists} assume that ice exists at the southern pole of Mercury\underline{.}
A search for trace\underline{s} in the country where 97\underline{-}year\underline{-}old\underline{s} are comparative\underline{ly} young.
A search for trace\underline{s} in the country where 97\underline{-}year\underline{-}old\underline{s} are comparative\underline{ly} young.
With its 97 years it is relatively young for these width\underline{s}.
Because they are all afraid\underline{,} so far hopelessly divided into a confused opposition\underline{.}
After the dictator u2019s fall, up to 11,000 civilians were in military detention\underline{.}
Moreover, no article explicitly stipulat\underline{es} equality between men and women.
Equally dubious is the wording that 'infuri\underline{ation} of human beings\underline{'} is prohibited\underline{.}
Mor\underline{si} u2019s extension of power to all three state powers left the lawyer resign\underline{ed}.
It is one of the more expensive dishes you can buy here.
But it is precisely these, according to the family, that they have so far been denied\underline{.}
The authorities have treated me as if I were a mother\underline{-}in-law\underline{,} a trouble\underline{maker}\underline{,} a whi\underline{st}leb\underline{low}\underline{er}.
They want their verdict simply to be accepted and their mouth\underline{s} shut\underline{.}
The Public Prosecutor\underline{'}s Office contradict\underline{s} Brad\underline{ley} Manning's accus\underline{ations} that he had been mis\underline{tre}ated in prison\underline{.}
The hearing deals with Manning u2019s time in the Qua\underline{n}tico\underline{,} Virgin\underline{ia} military prison\underline{.}
The defense seeks to deport the indic\underline{t}ment for too harsh conditions of detention\underline{.}
The lib\underline{er}ated US Army is accused of having stolen thousands of confidential documents.
In January 2011\underline{,} Manning u2019s lawyer formally challenged Manning u2019s treatment.
Nav\underline{arre}\underline{tte} believes that Mexican Americans are trapped between two worlds.
If our families had not failed in Mexico\underline{,} they would not have gone\underline{.}
While she is an American citizen\underline{,} she sees herself as part of two countries.
You enjoy the best of both worlds, but none of them are root\underline{ed}.
The latest blood\underline{y} events seem to ni\underline{p} such hope in the bud\underline{.}
Why, too, do these insid\underline{ious} Palestinians pardon and leave their own state to them?
Israel u2019s defense budget is greater than that of its four Arab neighbor\underline{s} combined\underline{.}
Obama\underline{,} too, must play his part in getting Israel to negotiate\underline{.}
The United States has a vital interest in a stable Middle East.
But more and more academic\underline{s} and children's development experts say bo\underline{re}dom is something positive.
Then there is the question of how we actually define bo\underline{re}dom\underline{.}
"We have no real precedent to follow," he adds\underline{.}
In my first weeks in Oxford\underline{,} I belong\underline{ed} to such a minority\underline{.}
Should I turn to the Labour Party and repress my natural incli\underline{nation}\underline{?}
"But it is the best place in the world," he said.
Exhausted by my frequent travels to London, my emotional resistance became weak\underline{er}.
At that time he wrote two weekly column\underline{s} in the Mur\underline{d}och press.
Also the Argent\underline{ine} model Valeria Mazza does not forget the charisma of the fashion\underline{maker}\underline{.}
"It was a true dream\underline{,}" says the wi\underline{dow} of Rod\underline{rig}\underline{o} d'Ar\underline{enberg}\underline{.}
How is this definition applied to its everyday life and social networks?
This includes the mother who has the password to one of the accounts\underline{.}
The boy is not unaware of experiences that are known today as cyber\underline{bul}\underline{ly}ing.
"To say they should not do it does not work," he says\underline{.}
" For example, the age, or what one may share or publish\underline{,}" he explains\underline{.}
The cause of AIDS dying today is too late detection\underline{.}
Fabr\underline{i}zio was 21 years old when he was confirmed to be HIV positive.
- In my opinion, the problem is not access to treatment.
His message is a summary of the fight against AIDS in 2012\underline{.}
No one in Puerto Rico has dominated this plain as Pic\underline{ul} xedn.
What do you think is the best you have achieved in the association\underline{?}
There he met young designer Maj Axel\underline{sson} and married her.
Indian\underline{a} was the first state to make such a demand.
The Republican authorities rush\underline{ed} to extend this practice to other states.
These measures are clearly aimed at limiting hispan\underline{ic} voices\underline{.}
The US Advoca\underline{te} General intervene\underline{d} to suspend the most controversial laws.
The organization also recommends limiting the consumption of red meat\underline{.}
According to the Canadian cancer society, studies on vitamin E are contradictory\underline{.}
On this basis, the phy\underline{s}icists divide the particle\underline{s} into two categories\underline{.}
Return\underline{ing} to childhood is an unacceptable hum\underline{ili}\underline{ation} for some people.
But through the disease I really got to know my children.
In Quebec\underline{,} 11,700 inhabitants have a bed for pal\underline{li}ative care.
The implementation of this report was possible thanks to a scholarship for journal\underline{ism} from Canadian health research institute\underline{s}.
This season you have taken on a new dimension with PS\underline{G}.
These elements encourage me every day to improve my level of play.
They take advantage of the competition introduced by Carlo Ancel\underline{otti}\underline{...}
By the way, Carlo Ancel\underline{otti} gives me a lot about my playing position.
What do you think about the first part of the PS\underline{G} season?
Can the PS\underline{G} become a large European club in the short term?
This year, it is really important for us to draw attention to this title.
How did you experience the European Championship in 2012 with the French national team?
I saw things there that gave me strength\underline{.}
Today I manage to make good games a reality in the national team.
We have a good position in the qualification group for the World Cup\underline{.}
I hope that Did\underline{ier} Deschamps will lead the 'Bleus' to Brazil\underline{.}
With 15,000 computers on the network, some 200,000 transactions have already been recorded\underline{.}
In this way, the network can verify the authentic\underline{ity} of the transaction\underline{.}
French troops have left their responsibilities in Afghanistan (Kapisa and Sur\underline{o}bi).
Everything is imported\underline{;} nothing is produced except fruit and vegetables\underline{.}
What kind of souvenir do we leave after military expenditure of EUR 2 billion?
This is a new poker game by President Moham\underline{ed} Mor\underline{si}.
Representative\underline{s} of human rights organisations, religious minorities or civil society have acted equally\underline{.}
It is not surprising that most of the articles were adopted unanimously\underline{.}
According to them, the Islam\underline{isation} of the Constitution takes place through other articles\underline{.}
According to an old legend\underline{,} pag\underline{an} god\underline{s} lived on the summit.
In the evening you can even see them sleeping on the roof\underline{s} of parking cars\underline{.}
The cat\underline{s} like lively places and do not say no to treat\underline{s}.
Migrant\underline{s} without a profession\underline{,} education, language skills and medical evaluation encounter problems.
The Russian Ministry of the Interior plans to tight\underline{en} up the arms law for private arms owners\underline{.}
Especially many pistols and gun\underline{s} come from poor countries like Ky\underline{r}gy\underline{z}stan\underline{.}
There is no need for any papers or personal meetings\underline{.}
The weapon is distributed in middle\underline{-}rank\underline{ed} military weapons camps\underline{.}
The protests are supported by trade unions and several left-wing non-profit organizations\underline{.}
That is about 1.1\% more than they are now donating for wages\underline{.}
- Not necessarily\underline{,} but this is about mutual convergence\underline{.}
The new hero of Ros\underline{bal}\underline{t} is the extravag\underline{ant} artist Kir\underline{ill} Mill\underline{er}.
When the group started playing live, it became a "Leningrad".
Now there are micro\underline{com}muni\underline{ties} and it is difficult to please everyone.
- The performances of Sta\underline{s} Mich\underline{ai}low come several thousand\underline{!}
However, the bio\underline{satellit}\underline{e} "Bion" will contain only same-sex species\underline{.}
Will she be able to bring a child to the world after this flight\underline{?}
The Federal Republic of Germany may only control federal funds, which correspond\underline{s} to our state funds.
Is it then sensible to make the law even stricter\underline{?}
Such a system only puts bureaucracy under even greater pressure.
On the streets there are some smooth ice\underline{,} but mostly they are dry\underline{.}
However, there are about 30 cm of snow on the cre\underline{st}s of the Ore Mountains\underline{.}
What is the purpose of the concerts\underline{'} proceed\underline{s} against the end of the world?
We wanted to create a programme that appeal\underline{s} to all generations\underline{,} including children.
Even in Moscow\underline{,} where we were recently, there were no problems.
How many of them have been present since the beginning, i.e. since 1998?
The rocket was 1.4 m long and weigh\underline{ed} about 11.\underline{5} kg\underline{.}
This naturally raises the question of where this capital comes from?
For it is a man number, and his number is six hundred and sixty-six.'
Right before the occupation of the embassy six embassy staff fled\underline{.}
This ended after numerous complications in the residence of the Canadian ambassador\underline{.}
For this I need as much influence as possible and as strong a mandate as possible.
But do you not confirm what you have just said?
And the people concerned might have to say why they reject this.
People want to see me as a Sam\underline{ari}tan who saves the republic\underline{.}
But I wonder why we still need a library today.
No one is going to go to any of these old style libraries\underline{,} is it?
Nine years later, the EUR 30 million mountain was thrown up.
"No\underline{th}ing is worse than a half-empt\underline{y} library\underline{,}" says architect Win\underline{y} Maas.
I believe that this is what makes it so difficult for the Germans.
'The brand is being watered down, the universal\underline{ity} is disappear\underline{ing}, the image damage is enormous\underline{'}.
Yet 81\underline{,}500 appeal\underline{s} are still pending in office.
The trademark office CTMO rejected the Munich appeal\underline{.}
"Da\underline{ran} sehen man, wie viel uns das wert ist," sagt Wentz\underline{ler}.
The history of a link that crosses far more than 87\underline{33} kilometers\underline{.}
The bantu language flu\underline{ent}ly speaks in this room no one can sing\underline{,} but no one can sing\underline{.}
Fre\underline{quent} viral STI\underline{s} are HIV\underline{,} Human Pap\underline{pil}\underline{oma}\underline{vir}\underline{us}, Herpes genital\underline{is} or hepat\underline{itis}\underline{.}
Ch\underline{lam}\underline{y}dia infection\underline{s} among young people are much more common than in other population groups.
This is why experts recommend regular examination\underline{s}, especially for frequently changing sex partners.
Early diagnose\underline{d}, most STI\underline{s} can be healed and avoided late effects.
But also the many migrant workers who carry the virus through the country.
"Go\underline{ing} to Esitjeni, there is light" the people there say.
The mirror\underline{,} here in the picture, had an average of five meters\underline{.}
However, the most important impression\underline{s} from space are provided by the Hubble space telescope\underline{.}
There are currently 20 people over 100 years old.
Then she tells of her husband who was in the army\underline{.}
It was worst in the post-World War II period.
They live in the middle of the large family, are loved\underline{,} cared for and are happy.
The future constitution\underline{,} based on Sha\underline{ria} law, is highly controversial\underline{.}
Fear of a divine state on the Nil\underline{e} of grace\underline{s} of the powerful Muslim Brot\underline{her}hood\underline{.}
The opposition has been forming for weeks against Islamist sup\underline{rem}\underline{acy}\underline{.}
"Man\underline{y} people like the Aqua\underline{vit} more than the Rakfisk," says Havar\underline{d}.
Instead\underline{,} it only refers to the 'Ju\underline{ly} 22 incident\underline{'}.
Like most people here, their English is impec\underline{c}able.
But perhaps it is the severe dark\underline{ness} of the whole fish.
And the problems in the community are of crucial urban nature.
But her family believes that she was murdered by her companion\underline{.}
The Public Prosecutor claims\underline{:} Brad\underline{ley} Manning did not complain about maltreatment.
Many people are forced to leave Mexico because of lack of opportunities.
Mexico u2019s relationship with the United States is complicated and res\underline{ent}ful.
We are the descendants of these people and our loyalty is to them.
During his first term, he failed to present his own peace plan.
In apath\underline{y}, on the other hand, there is no urge to do anything.
But only 3\% of parents said they felt bo\underline{red}.
In Color\underline{ado}, there is no clear guideline for the new law on mar\underline{i}juana
And regulator\underline{s} in the state of Washington also scratch their heads pu\underline{zz}\underline{ling}ly.
Petro\underline{n}ella Wyatt\underline{:} I was promoted from Oxford because I am Tory.
During his time in the forties\underline{,} all political views were accepted.
Even my communist friends have always behave\underline{d} perfectly\underline{.}
"I love this palace\underline{,}" he says with his unmistakable Italian accent\underline{.}
Being in love with the nobil\underline{ity} does not have to be disadvantage\underline{ous}.
The most difficult profession in the world: the human work animals of Kawah Ijen
Anyone who does not take this issue lightly is the government of Singapore\underline{.}
On FB I upload beautiful pictures or pictures of games.
Even if someone would tell him a strange\underline{r}, he would ignore it.
Concl\underline{ud}ing the Unasur Summit without publishing the Lima Declaration
The final document also referred to the political situation in Paraguay\underline{.}
"South America must learn in the integration of citizens," says Raf\underline{a}el Correa
"Th\underline{at} would affect everyone's health," he added.
Today it is possible to survive this syndrome with quality of life.
As you know, Az\underline{c} xe1rraga Andrade is the main shareholder of the Posadas chain\underline{.}
I like the work of Leo Arill\underline{.}
Student\underline{s}, for their part, assure that the course is one of the most interesting.
Arizona was the first state to make such a demand.
Several bill\underline{s} have been blocked by the veto\underline{es} of democratic governor\underline{s}.
There are cancer\underline{s} that are aggressive and others that are indol\underline{ent}.
Smoking is responsible for 85\% of cases of lung cancer\underline{.}
However, such deviation\underline{s} have not yet been found at CERN\underline{.}
Pal\underline{li}ative care - the best way to die... | Le Devoir
However, much remains to be done in this important area.
"We help relatives and patients alike\underline{,}" reports nursing director Nathal\underline{ie} Sav\underline{ard}.
However, she told me that I had finished\underline{!}
I think he will win more titles in Paris.
I had an encouraging conversation with him in January.
We finished the season with a very strong performance.
Do you think that the media expect too much from PS\underline{G}?
This means that Ibra\underline{hi}movic is powerful and score\underline{s} many goals\underline{.}
Unfortunately\underline{,} my injury prevented me from spending some time playing\underline{.}
This has been my hope since my baptism with the "Bleus".
Some thousand websites accept Bit\underline{co}in as a donation or as a means of payment.
The social network Facebook has also developed such a system.
The computer that did the job gets 50 bitcoins.
The life of the network has already had ups and downs.
Young people are fed up with war and its ideologie\underline{s}.
The withdrawal of French combat troops was completed on 20 November.
'Sham\underline{e}' responds to liberal\underline{s}, who see this as nothing more than a propaganda shot\underline{.}
With this constitution\underline{,} we remain within the framework of the civil state.
Visit the River Jordan where Jesus was ba\underline{pt}\underline{ized}.
From the foot of the mountain you can reach it by a shuttle bus.
Not all of them can be visited in just one trip.
In the carefully restored theatre\underline{,} evening concerts and opera\underline{s} are performed today.
According to Jewish tradition\underline{,} the Sabbath is celebrated in Israel on Saturday\underline{.}
There are no stra\underline{y} dogs in the streets of Israeli cities.
Their rights must, however, be protected before they leave.
The reason is bureaucratic obstacles and, of course, linguistic difficulties\underline{.}
In addition, legalization costs money: 12 to 16 thousand rub\underline{les}.
According to Baranez, arms manufacturers also contribute to the black market.
He got a photo album showing "every\underline{th}ing possible".
"I felt like a luxury shop\underline{,}" the militaryman recall\underline{s}.
"Kaufe eine TT\underline{.}
They also called for the formation of trade unions in the fast-food industry.
- Please describe briefly what research your group is doing.
In a cl\underline{own} all this gets blu\underline{r}red and lose\underline{s} its tragedy\underline{.}
- Nowadays\underline{,} commercial art must be careful\underline{,} considerate and flat\underline{ter}ing.
Consumption has no culture at all; that is quite different.
But not all of them can deal with culture.
The project is financed by grants from the City of St. Petersburg\underline{.}
As early as half a century before, experiment\underline{s} with plants were carried out.
Ten hours later, the newborn\underline{s} u2019 instinct\underline{s} were completely mu\underline{ted}.
The most valuable thing that humanity possess\underline{es} is the female organism\underline{.}
Up to now, the birth of children in space has been mere theory\underline{.}
As far as German legislation is concerned, is it easier than ours?
Is this perhaps because the auditor\underline{s} there are better?
On these roads\underline{,} however, there are some snow residue\underline{s} that have disappeared or disappeared\underline{.}
Greater attention is therefore needed, especially in higher locations\underline{.}
The roads I/43 and I/34 at Svita\underline{vy} are chemical\underline{ly} treated\underline{.}
The first-class roads are mostly dry but frozen\underline{.}
In northern Bohemia\underline{,} the road master\underline{s} report several difficult road sections\underline{.}
  u2047 imon Ornest: At our concerts we want to collect positive energy.
We try to involve these people intensive\underline{ly} in our projects.
There are still many things in which we hang\underline{...}
Poland u2019s path to space, of course, began much earlier.
Both projects were concerned with the military use of rocket propul\underline{sion}.
The maximum altitude for all three types was 37 km.
The repeal of the law on non-profit work is not a solution.
This decision gave rise to lively public debate.
These ideas did not come from Brussels\underline{,} however, but from Prague\underline{.}
I am not concerned with being a senator or president\underline{.}
And you will not get far in politics in the long term.
I try to find allies for my views and vision\underline{s}.
That sounds a bit like Okam\underline{ura} saving the Czech Republic.
But that is not related to the level of salary\underline{.}
For example, in spring my deputy becomes the general manager of the travel agency\underline{.}
About 200,000 to 400,000\underline{,} and that is still the case.
The full discussion can be found in the Saturday issue of Pr xe1vo.
The 80,000\underline{-}inhabit\underline{ant} community has the lowest education rate in the whole of the Netherlands\underline{.}
What does a "normal\underline{"} foreign policy actually mean from a German point of view?
Germany may even gain some respect with this.
There are different views on the Palestinian initiative in Europe.
The United States, on the other hand, has clearly declared itself in favour of a veto\underline{.}
Are there differences of opinion between the United States and many European nations\underline{?}
"Marke\underline{t} protection" in China: When Pu\underline{ma} and Arm\underline{ani} suddenly become Chinese.
And even then it is not clear whether they are right.
Pat\underline{t}loch opens a folder with trademark registration\underline{s} in Beijing\underline{.}
As a result, the stock of unprocess\underline{ed} appeal procedures had fallen by 22\%\underline{.}
Or we will be pushed out of the market in the segment in question.
The bacteria\underline{l} STI\underline{s} include sy\underline{phil}\underline{is}, ch\underline{lam}\underline{y}dia and tripper (gon\underline{or}rhoe\underline{a}).
That is about a tenth of the year before.
The ice sheet may be up to 20 metres thick\underline{.}
The Spitze\underline{r} Teleskop of the Nasa shot this photo of the Gala\underline{ctic} Bir\underline{th}room\underline{.}
With the telescope\underline{,} however, the colors are more visible\underline{.}
One of the largest and sharp\underline{est} shot\underline{s} of the Hubble telescope\underline{:} the Jacuzzi Galaxie\underline{.}
Depend\underline{ing} on the colour\underline{,} photographs of spiral galaxies become true works of art.
This Starbur\underline{t} recorded the Hubble telescope in the Spi\underline{ral} Gala\underline{x}y M83\underline{.}
This image was assembled from optical and X-ray images of different telescope\underline{s}.
The picture shows the latest launch preparations at the Ke\underline{pl}er space telescope\underline{.}
The primary mirror of the space infrared telescope has a diameter of 6.\underline{5} metres.
In southern Azerbaijan\underline{,} many people reach a bi\underline{bli}\underline{cal} age.
In southern Azerbaijan\underline{,} many people reach a bi\underline{bli}\underline{cal} age.
This is my grand\underline{fa}ther\underline{,} he was 120 years old.
Museum director Fatulay\underline{eva}\underline{,} on the other hand, believes that it is nutrition\underline{al}.
The propaganda sounds strange from the mouth of an old woman\underline{.}
Riva\underline{l} demonstrations in Cairo reveal the country u2019s deep division\underline{.}
These courts served to op\underline{press} opponents during Mubarak u2019s rule.
A majority in the Islamist\underline{s} u2019 draft is considered certain.
Rakfisk from Norway\underline{:} Is this the most od\underline{ious} fish in the world?
We are, as they say, a prudent people.
"And naturally eat Rakfisk," she adds with carefree laugh\underline{ter}.
But in the evening the ham\underline{fish} is on the menu again.
A man falls from his chair\underline{,} possibly overwhelm\underline{ed} by the Aqua\underline{vit}\underline{.}
According to the official version of the events, Maria\underline{na} committed suicide in 2010.
The officials asked Manning questions and wrote his answers\underline{.}
In their opinion, our existence is a symbol of failure.
And in the United States we are seen as Mexican\underline{s}.
This includes a peace agreement between Israel and the Palestinians\underline{.}
As a result, Australia is introducing the strict\underline{est} regulations for tobacco packaging worldwide.
Other\underline{s} say that the laws have boost\underline{ed} their business.
Canada was the first country to issue photographic warning\underline{s} in 2001.
Hard\underline{er} legislation is being considered in Great Britain\underline{,} New Zealand\underline{,} South Africa and India.
"In fact, bo\underline{re}dom has a very long history," he says\underline{.}
Not only today u2019s university students are being attacked for their views.
Yes\underline{,} ran\underline{,} because I suffered from systematic harassment and threats\underline{.}
As an incredibly sh\underline{y} 18-year\underline{-}old\underline{,} I arrived in September 1986\underline{.}
The hatred for the Conservative Party had reached its height\underline{.}
Most Tory first semester\underline{s} claim to be Labour supporters\underline{.}
In a local pub\underline{,} I tried later to make a mistake\underline{.}
Would I be able to meet like-minded people only after dark\underline{ness} has collapsed\underline{?}
"He was impec\underline{c}able; time leaves no trace of it".
It is the biggest problem in that country.
The friend of a friend was blackmailed in a social network.
That is my opinion, and that is how it is in our hospital\underline{.}
Everything is different when you know you have AIDS\underline{.}
Some think they will die and want to hear nothing.
There are 13,435 cu\underline{mul}\underline{ative} cases (12\underline{,}158 AIDS and 1,317 HIV\underline{).}
Two\underline{-}band Kara\underline{mbo}\underline{le}: a blow for Vitro and for the country.
It should read 'Her\underline{e} is the honourable citizen J.R. Ewing\underline{'}.
This is the only business he has not won.
A Republican strategy to counter Obama u2019s re-election
Men of African\underline{-}American origin also run a higher risk.
Unfortunately\underline{,} there is no miracle cure for cancer prevention\underline{.}
It is also a risk factor for several other types of cancer\underline{.}
Both at the level of physical\underline{,} emotional or spiritual comfort.
In the Victor\underline{-}Ga\underline{db}\underline{ois} home is not a day like the other.
She says that the procedure is 'painful but positive'.
At that time I had just recovered from a series of injuries\underline{.}
What is the goal of the association in this competition?
We will try to come as far as possible.
This makes it all the better to speak of a 'lat\underline{an} dependency\underline{'}.
This encourages others to improve their level of play.
I was keen to participate in this European Championship\underline{.}
With Bit\underline{co}in you can pay and sell without a bank.
Other\underline{s} like the WordPress blog platform accept them.
NATO and the US are expected to follow by the end of 2014\underline{.}
The rumour has spread that Afghanistan has immense mineral resources.
A referendum should be held within 14 days.
The majority of Liberal\underline{s} did not comply with the request.
This is the first signs of theocracy\underline{.}'
That word was not in the previous Constitution\underline{.}
It was here that Jesus appeared to his discip\underline{les} after the resurrect\underline{ion}.
Only mountaineers can reach the ruins on their own.
All the others take an aerial cable\underline{way} to this historic summit.
Among them is the Israel Museum near the Knesset (par\underline{lia}\underline{ment}).
Entrance is free and donation\underline{s} are rejected in principle.
The city is mentioned in ancient Greek and ancient Egyptian legend\underline{s}.
Only migrants with legal status must pass the test.
The fake papers were printed with an ordinary color printer\underline{.}
The weapons enter the black market via several channels\underline{.}
The weapon is exhibit\underline{ed} and handed over by the fence\underline{.}
Buyer\underline{s} and seller\underline{s} often find each other about acquaint\underline{ance}s.
The price of the weapon I learned only there.
There, users place their orders and ask questions.
Until now, this sector of the economy has hardly been organized by trade unions\underline{.}
No one in this expensive city deserves less than them.
And, first of all, we should get rid of this disgust\underline{ed} virtual reality hell\underline{o}!
Is there a lack of resolution, depth or anything else?
- Should the number of cameras not be increased?
And the third camera is actually an ordinary RGB camera.
Or exacerbat\underline{e} the problem, because more calculation\underline{s} would be needed.
What are your group's responses to this objection\underline{?}
Each of my past provocation\underline{s} was an invitation to talk.
- When did you know that you have to become a painter\underline{?}
Tra\underline{chten}\underline{berg} moderate\underline{d} many programs before the time of "Ha\underline{lli}\underline{-}Ga\underline{lli}\underline{".}
I love the gro\underline{tes}que, and I have gro\underline{tes}que ideas.
Now you have to consider who you will like.
In contrast to animals, man could do this in principle.
But women have been flying into space for 50 years.
"After all, no one answered this question," said Space veteran Wach\underline{tang} Wa\underline{tsch}\underline{n}adse.
The father of the child, Andrijan Nikola\underline{ev}\underline{,} was also cosmonaut\underline{.}
NK  u2047  CEO\underline{:} Control of the black system fails due to the fault of politics\underline{.}
First of all, let us say which route is not effective.
On the streets of the Czech Republic there are some snow and ice smooth\underline{ness}.
According to the district street guard\underline{s}, the view was limited due to fo\underline{g}.
"In the   u2047 umperk district there are still snow residue\underline{s} in the high altitude\underline{s}.
Ice smooth\underline{ness} is reported in particular from the area around   u2047 t  u2047 t xed.
How did you cooperate with both of them?
Several groups and perform\underline{ers} perform at each concert\underline{.}
So far, these are only individual cases of particularly willing personalities.
The information on this comes exclusively from the contemporary press.
In 1962\underline{,} however, further development was halted.
The number of people affected is already in the millions\underline{.}
The movie Argo: If's worst\underline{,} call Hollywood\underline{.}
"We are disadvantaged by the fact that we do not have a sea.
You do not like someone calling you populist\underline{s}.
But without Parliament's support, you will only have keywords.
Are you thinking about setting up your own party?
My private assets are estimated at about CZK 60 million.
I have already put 2.5 million into the campaign\underline{.}
Did\underline{n}'t you say that you'll be driving back these activities?
However, as President, I would stop my actions altogether\underline{.}
Everyone knows that his book is part of this building.
The Germans find themselves between the fronts.
Because of American domestic politics\underline{,} these differences have always existed\underline{.}
The Germans will simply have to play a greater role.
Arm\underline{ani} is a world-famous brand, Polo Ralph Lauren also.
Every week a new case lands on my desk\underline{.}
This means women who fish for rich men.
"Th\underline{at} is damaging to business, you have to fight it," says Pat\underline{t}loch\underline{.}
As is so often the case in China, the figures are impressive\underline{.}
1.8 billion yu\underline{an} had been collected in 2011\underline{.}
The matter is now before the Supreme Court.
The dangers in the Far East are even threatening to slip back to Europe.
Then when imitators secure unprotected brands there.
Otherwise\underline{,} this can be much more expensive than registration\underline{.}
More than 40\% of the population are now HIV positive.
Human pap\underline{illa}\underline{vir}\underline{use}s are also common in young people.
Culture is another - flesh to flesh\underline{.}'
The eight planet\underline{s} of our solar system, as well as the dwar\underline{f} planet Cer\underline{es}.
Nevertheless\underline{,} it reaches a diameter of about 11 meters\underline{.}
The hobby\underline{-}eberly tele\underline{s}coping in Texas is also fixed in the height angle\underline{.}
Daily drink butter - and get 168 years old
The journey through the Talysch Mountains is wild\underline{ly} romantic\underline{.}
At the age of 136\underline{,} yet another child was born\underline{.}
So why do so many high-ris\underline{e} people live here in the south?
Also problematic\underline{:} civilian military jurisdiction should continue to be maintained\underline{.}
But without civil-socie\underline{ty} organizations\underline{,} democracy cannot work.
They are placed in a bunch of dirty\underline{,} wet sportswear\underline{.}
We are not very donor\underline{,} we do not like boast\underline{ing}.
Currently\underline{,} the traffic in Mexico City is particularly bad.
The material was then published by Wiki\underline{Le}\underline{ak}s on the Internet.
Wiki\underline{Le}\underline{ak}s never confirmed Manning as a source of information.
And Monte\underline{zu}ma u2019s children go on the war trail\underline{.}
Israeli hardliners, on the other hand, draw the opposite conclusion.
For at least a while, Israel will be able to sleep calm\underline{ly}.
So should we welcome bo\underline{re}dom with open arms\underline{?}
bo\underline{re}dom can almost sound like depression\underline{.}
But, in general, teenagers are a rather tight pile\underline{.}
Advoca\underline{tes} of the legalization movement hope that the Ministry of Justice will yield\underline{.}
I returned to my room with hanging head.
Anyone suspected of being Tory is harass\underline{ed}.
"You will not be happy here," he told me.
It would break my heart if you walked.
Valentin\underline{o} has always preferred the elegance of ce\underline{leb}\underline{r}ity.
At the end of the 1990s, this eventually happened\underline{.}
It is already having an impact on the housing market.
"He has never known who it was," he assure\underline{s}.
According to Jos xe9, the victim has not closed the user account.
"But I know this is cyber\underline{bul}\underline{ly}ing," he explains\underline{.}
Peru presides over time of the regional bloc\underline{.}
Today, his parents only know that he had cancer\underline{.}
I live a normal life, like everyone else.
Among the risk factors for new infection\underline{s} are young people.
But Mexican laws recognize this possibility.
The vote would have gone 45\% against 37\%\underline{.}
The investment is more than \$1\underline{.}5 billion.
His figures at the level of international tournaments are impressive\underline{.}
Today the children make unnecessary travel and games.
This made the series record at that time.
Beginning of the course which studies the "end of the world"
This is mainly the case in the English speaking world.
Prostate cancer detection\underline{:} should the test be made or not?
We have obtained the opinion of two specialists\underline{.}
I therefore recommend that the test be carried out.
'The screening test does not lead to cancer\underline{'}.
They saw scientific applications, but nothing else.
Le Devoir has tried to look at this more closely.
They have a maximum life expectancy of three months.
Dia\underline{bet}\underline{ics} no longer have to control their blood sugar levels.
Sewer\underline{age} contracts\underline{,} the costs of which were artificial\underline{ly} inflat\underline{ed} by him.
In Montreal\underline{,} the 'system' of corruption worked smoothly\underline{.}
The technical staff also gave me a lot.
And with a game, this is even easier\underline{.}
You also know that every training unit is crucial.
Is Ancel\underline{otti} the right person for the job?
Last season we were close.
Normal\underline{ly} you should be master with 79 points...
I believe that this year is the right one.
One wonder\underline{s} what more people expect.
We could never win with 4-0 every weekend\underline{.}
A team builds up over time.
In the Champion\underline{s} League we have shown strength\underline{.}
This shows that Ligue 1 is exciting\underline{.}
He also respects the people around him.
Major players like Wikipedia refuse donation\underline{s} of this kind.
"The present is not a concrete religious commitment.
But most of the san\underline{c}tuaries are in Jerusalem\underline{.}
The ski slopes have a total length of 45 kilometres\underline{.}
There are almost 300 museums in this country.
Insurance costs an additional \$15 per day.
Museum tickets cost an average of 30 tickets\underline{.}
"It is difficult without language skills\underline{,}" they admit\underline{.}
Civil rights activists emphasize the following important aspect of the law.
Supplier\underline{s}: from factories to officers
Other illegally sold weapons come from military stock\underline{pil}\underline{es}.
In many military camps\underline{,} explosion\underline{s} often occurred\underline{.}
Another channel of the black market is smuggling\underline{.}
According to him, the schemes have not changed.
"Of course without license\underline{",} asks user "Iwan\underline{"} (liter\underline{al} quote\underline{).}
The buyer transfers the money via a bank machine.
On the other hand, corporate governance does not make it easy for them.
'The brain can only be moderate\underline{ly} overrun\underline{'}.
- What can we expect in the future?
It is popular, but is it not overvalue\underline{d}?
- Oh, that would be very hard to see.
- Have you tried to outrun the brain\underline{?}
I understood that I must go down this road.
It is difficult for art to grow up on our stones\underline{.}
I do not think there are many choices\underline{.}
Without a solid base, the chic\underline{ks} sw\underline{ung} wild\underline{.}
The chic\underline{ks} did not react to light and sound.
For ethical reasons, such experiment\underline{s} are not carried out.
Well\underline{,} we get around this through birth\underline{-}inducing aids.
Can you introduce the project to our readers\underline{?}
You can find more information on www.kpks\underline{.}cz\underline{.}
Are similar major events planned for the future?
How do you manage these trips logistical\underline{ly} and organisational\underline{ly}?
In the show business today, one often copies the other.
Then the versions Met\underline{e}or-2\underline{H} and Met\underline{e}or-3 were built.
This is expressed in particular in changes to existing laws.
Affleck\underline{'}s film is a special combination of several film genre\underline{s}.
Do you not turn your back on your voters\underline{?}
For me, however, this right-wing thinking is completely unimport\underline{ant}.
In the Senat\underline{e}, we are therefore only two independents.
You talk about asset declarations\underline{,} what would your opinion be?
I have no 15 million for the campaign\underline{.}
As promised\underline{,} I have partially reduced my activities.
But I must also live on something.
Which monthly income were you used to as an entrepreneur\underline{?}
The success of the education offensive was limited.
After 105 steps you arrive at the summit.
However young and uneduc\underline{ated} they may be.
This is finally a starting point for identity\underline{.}
A foreign policy like France or Britain\underline{.}
That is what they are doing with the euro.
Or does Germany still find leadership difficult?
The Chinese call the "Bang Mingpai", a front-passenger brand.
The Chinese authorities are not aware of their guilt\underline{.}
The Chinese authorities are not aware of the guilt\underline{.}
23.\underline{5} million people live from this in southern Africa.
Imbon\underline{gi} means on Zulu story\underline{t}eller\underline{s} or even praise\underline{-}lov\underline{ers}.
Fil\underline{t}l xe4use and Kr xe4tze belong to the parasitic STI\underline{.}
How has the number of infection\underline{s} developed?
The number of new HIV infection\underline{s} has decreased since 2007.
It is 700 light years away in the Aqua\underline{r}ius starscape\underline{.}
In Arizona\underline{,} USA, the Large Bin\underline{oc}\underline{ular} Tele\underline{scope} stands\underline{.}
The radio telescope has a diameter of 305 meters\underline{.}
However, images can only be expected in 2018 at the earliest\underline{.}
Here you can see an illustration\underline{.}
"Sham\underline{po}o I never used," says Mir\underline{za}yeva\underline{.}
After all, Azerbaijan u2019s elderly are not in need.
In plain language, this means nothing other than censorship\underline{.}
Clearly\underline{,} Mor\underline{si} u2019s supporters did not want to risk that.
Mexico u2019s Enrique Pen\underline{a} Nie\underline{to} faces a difficult start.
I thought I would die in this cage.
I am afraid you have to go through it alone, Amigo\underline{s}.
Perhaps this will only lead to more blood\underline{s}hed\underline{.}
A war that is neither lost nor won.
Military\underline{ly}, Hamas is no longer a threat\underline{.}
Australian laws on uniform cigarette packaging are coming into force.
But some people are bo\underline{red} easier than others.
So back to my question of origin: is bo\underline{re}dom healthy\underline{?}
I do not think we should celebrate bo\underline{re}dom\underline{.}
Nor should we be too critical of them.
"I know who you are," he said kindly\underline{.}
You are welcome to call me a wine squirrel\underline{.}
Valentin\underline{o} is a spectacular\underline{,} generous and elegant host\underline{.}
So why do the Singapore\underline{ans} not have more children?
What is private for someone under 16 years of age?
I also spend my time with acquaint\underline{ance}s.
Do you know what others publish about you?
- So why are people still dying from it?
Who was the best player in Puerto Rico\underline{?}
Who was the best coach from Puerto Rico\underline{?}
"The people don't think otherwise," he says\underline{.}
Should the test be made or not?
It greatly damages people's health.
However, their investigations are not concl\underline{us}ive at the moment.
"I have good children," she adds\underline{.}
And death is part of everyday life.
A permanent anti-cor\underline{r}uption unit launched in 2011\underline{.}
I make progress on their side every day.
But I do not break out in enthusiasm\underline{.}
What he has done is truly exceptional\underline{.}
Everyone has worked for everyone else.
However, cash also has these shortcomings\underline{.}
The private initiative is given priority.
A Constitution with the Bre\underline{ach} Barrier in Egypt
Another point of contention is the powers of the army\underline{.}
Advoca\underline{tes} of the Head of State will march on Saturday\underline{.}
There are no museum guides or souvenir shops\underline{.}
When entering the room, there is complete dark\underline{ness}.
In fact, it is an underground funicular\underline{.}
Bicycle rental costs 15 sc\underline{ram}\underline{ble}\underline{s} per day.
We receive many complaints from our migrants\underline{.}
'Ho\underline{pe}fully welcome' or 'ban\underline{ned} access for unauthorised persons'
'Don\underline{'}t sh\underline{y} away from the cost of false papers\underline{'}
The share of legal weapons in crime is very low.
Newcomers are looking for weapons in different ways.
You have to wait up to a month and a half.
In the US, fast-food and supermarket workers strike\underline{.}
Ju\underline{ma}ane William\underline{s}, member of the New York City Council.
The most important reason is the high staff turnover\underline{.}
They say it and at the same time indicate it.
- Normal\underline{ly} I just say it.
It is not used to calculate the depth of the object\underline{.}
More cameras might solve the problem...
- Your works have an unmistakable style.
- Can commercial art also be beautiful?
I'm not one hundred dollar notes that everyone likes.
Now every cult star has about 100 followers.
That is the culture I support.
There are good advise\underline{rs} in Moscow at the moment.
A normal chic\underline{k} develops\underline{.}
Four days later they simply died.
The experiment\underline{s} will continue in the spring of 2013\underline{.}
After landing\underline{,} the space council\underline{s} got offspring\underline{.}
The greatest risk was at Ter\underline{es}hkov\underline{a}.
On the other hand, the child also needs artificial gravity\underline{.}
Is the black system now prohibited or permitted\underline{?}
What criteria did you choose?
How have you experienced these things so far?
I think that is perfectly normal.
Currently\underline{,} The Tap has twenty members.
These bill\underline{s} will then be passed in the Bundestag\underline{.}
Terror\underline{ist} attacks have taken place on both sides\underline{.}
Too much action in too many places
Cur\underline{ious} invention\underline{s} are also present at home.
I had no ambition to become a politician\underline{.}
For me, it is important that we move forward.
And if it is just decorative\underline{.}
This was eventually enforced by NATO.
That certainly has a role to play.
This has always been a sensitive issue.
That does not make it easy for the Germans.
The word is derived from "Bang Dakuan".
Sometimes the law of the jungle prevail\underline{s} here.
70 of them attend secondary school.
What are the most important sexual\underline{ly} transmitted diseases\underline{?}
Not all sexual\underline{ly} transmitted diseases are subject to notification\underline{.}
What are the symptom\underline{s} of a sexual illness\underline{?}
Messenger\underline{:} NAS\underline{A} discover\underline{s} ice on Mercury\underline{.}
The larger spiral galaxy is called scientists UG\underline{C} 1810.
Our insight\underline{s} into space: The most important telescope\underline{s}
There is even a museum for longev\underline{ity}.
There is even a museum for longev\underline{ity}.
The word 'human rights' is missing from the Constitution\underline{.}
The Egyptian President did not save with pathos.
'The word human rights does not even occur\underline{'}
The spectacle is similar to the Eurovision Song Contest\underline{.}
In Mexico we are seen as Americans\underline{.}
Perhaps we are more "mexi\underline{can}\underline{"} than I thought.
Both sides need external impetus\underline{.}
But that is a regrettable\underline{,} short-sighted prospect\underline{.}
The tobacco lobby fought hard against the law.
This is a good deal for us.
A WTO decision is expected in mid\underline{-2013}\underline{.}
"We are treated like criminals," Oroz\underline{co} said.
Our municipality voted against this amendment.
Even Stalin\underline{ists} would have been fright\underline{en}ed by the atmosphere.
This trick should prove unsuccessful\underline{.}
"How did Tories have sex\underline{?}" one asked me.
I'm sure you just neck\underline{.}
Valeria Mazza\underline{,} in a dress of Valentin\underline{o}.
Singapore Need\underline{s} Baby\underline{s} to Save the Economy
The offline Private offline is private online.
The case of 14-year\underline{-}old Jos xe9 is different.
Promis\underline{cu}\underline{ity} should not be encouraged\underline{.}
H xe9ctor 'He\underline{tin}' Rey\underline{es}: 'Ba\underline{s}ket\underline{ball} was my life'
He enjoyed all those who knew him.
Student\underline{s} and professor\underline{s} take this date lightly.
These restrictions are not without consequences.
The same applies to the Hispan\underline{ic} population.
They were able to partially limit the damage.
To make dying more pleasant.
'PS\underline{G} is not the FC Barcelona!'
Everything goes very fast in football\underline{.}
Ancel\underline{otti} respects all the technicians\underline{.}
He had contact with big players.
From now on, everything is possible.
He already has the budget for this...
That is not the case today.
Of course, this would be a great disappointment\underline{.}
We have concluded with 79 points.
We are not the FC Barcelona!
Like Lauren\underline{t} Blanc\underline{.}
But I do not want to make a comparison\underline{.}
This game has given us confidence.
In November a "Me\underline{ga} Final Sale" was launched\underline{.}
Some are very close to the Mos\underline{lem} brother\underline{s}.
Making a Boost\underline{ing} Trip
Ukraine is also mentioned there.
The surrounding landscape is indescri\underline{b}ably beautiful.
And the working week begins on Sunday morning.
The sense, the problem and the protection of rights
'You feel hum\underline{ili}\underline{ated} and inferior\underline{'}.
Screenshot of a Web site that accepts Weapons Order\underline{s}
Military commentator and former militaryman Viktor Baranez
The persons responsible accept the orders\underline{.}
- What do you think about voice control?
Own taste instead of culture - ro\underline{s}bal\underline{t}.ru.
Our staff and regular guests went there.
The deception disappear\underline{s} through disguise\underline{.}
We see the disintegration of cultures\underline{.}
It says\underline{:} intellectual culture and consumer culture.
Now only your own taste count\underline{s}.
- What is Petersburg for you?
We have far fewer\underline{.}
In principle, nothing special was stated.
Water is the weight\underline{lessness}\underline{.}
How does the control system work in Germany?
I do not think that is the way it should be.
This information comes from the district street master\underline{ies}.
District   u2047 st xed nad Lab\underline{em}, Lib\underline{er}ec District\underline{.}
The clear answer here is yes\underline{.}
Much is not written about them.
However, it is difficult to inspire enthusiasm\underline{.}
Ban\underline{ana}s must be 14 cm long.
EU: Bizar\underline{re} Regulation\underline{s} are the Except\underline{ion}
How do you intend to solve this problem?
And that is what you want to approach.
All have internet, iPad and e-book\underline{s}.
The first impression\underline{:} Book Eldor\underline{ado} under cheese bell\underline{.}
Opti\underline{cs}\underline{,} haptic\underline{s} and smell are foreign.
Heated and cool\underline{ed} with geother\underline{mal} heat\underline{.}
Lisette Verhaig was also there.
The shelves are filled up to the top.
Szabo: 'German\underline{s} must play a greater role'.
Famous cases also concern graphic elements.
"You have to watch out hell\underline{ish}ly," says Wentz\underline{ler}.
In 2011\underline{,} there were around 2700 cases.
The Starwiege always produces new youngsters.
However, there is no birth certificate\underline{.}
The revolution has returned to Cairo\underline{.}
He was beat\underline{en} up, convicted and imprisoned for this.
Take a selection of rip\underline{e} cheese\underline{s}.
And leave it there a week.
Spirit\underline{u}osis can replace the smell\underline{.}
It faces a complex task.
Later\underline{,} I decided to opt for Mexican\underline{-}American\underline{.}
This clearly applies to the United States.
Many Australian smokers are defiant.
I will come back to that.
My father collapsed in tear\underline{s}.
But the truth was less amusing\underline{.}
Why do I mention this now?
In my eyes\underline{,} tear\underline{s} were wa\underline{king} up.
Unfortunately\underline{,} it is as it is.
The relief only took a short time.
'Val\underline{en}tino prefer\underline{s} elegance to ce\underline{leb}\underline{r}ity'.
Yet he is a star.
Naty Abascal and the Fashion\underline{maker}\underline{,} 2006
I still remember perfectly\underline{.}
'The population of Singapore must grow\underline{'}.
But everything has had little success so far.
They threatened him and demanded money.
'He only made it private'.
At present, this judgment is not being implemented.
This also applies if we lose\underline{.}
He hi\underline{d} it from his family.
At that time, AIDS was synonymous with death.
And the most important thing is prevention\underline{.}
This is not taken into account by the Court of App\underline{e}al.
Rey\underline{es} did not exaggerate this statement.
That was without doubt Pic\underline{ul} xedn Ortiz.
What remains to be done?
The Internet has increased these speculation\underline{s}.
We have a pardon from the Pope\underline{.}
Several remain completely unresolved\underline{.}
The breakfast was very poor.
The courage of ordinary death.
Problem of access to pal\underline{li}ative care
Large\underline{-}scale property scandal\underline{s} in Quebec
70\% undecla\underline{red} money in election campaigns
How do you explain this progress?
But we are lu\underline{r}king in ambush.
We are trying to create a game concept.
He has achieved promising results.
We have left Afghanistan.
An army is now in place.
Av\underline{oid}\underline{ing} the holy sites
Doing Something for Health
Touch\underline{ing} the Secret\underline{s} of Antiqu\underline{ity}
Is it also sold to minor\underline{s}?
A Mak\underline{a}row for \$100
The hands feel nothing at all!
It perceive\underline{s} pressure perfectly\underline{!}
Nowadays\underline{,} there are often misunderstanding\underline{s}.
- Kir\underline{ill}\underline{,} what is missing Petersburg\underline{?}
They say: servant\underline{s} of culture.
Global warming or clash with kill\underline{er}steroid\underline{.}
But then the problem begins\underline{.}
What exactly was this about?
Where is the way out?
Par\underline{du}bic\underline{e} and Hradec Kr xe1lov xe9 districts
So far no traffic disturbance\underline{s} have been reported\underline{.}
Who is the origin of this idea?
Only one: L xe1  u2047 a Angel\underline{ovi}  u2047 .
This trend is therefore systemic.
Let us talk about your vision\underline{s}.
To do this, you need to change laws.
I have no other option.
That is not very convincing\underline{.}
Should I make a debt?
The Long Road to Book
The urban ambience is perfect.
And everywhere books\underline{,} books\underline{,} books\underline{.}
That is cheap and time-efficient\underline{.}
Don\underline{ations} for the New Soul
The room climate is very pleasant.
The rest is done by fully automatic roll\underline{ers}.
Then Berlin abstained\underline{.}
But what is Arm\underline{ani} Polo\underline{?}
Swaziland is home to 245000 AIDS sw\underline{ast}\underline{ika}\underline{s}.
Fact\underline{s} on sexual\underline{ly} transmitted infection\underline{s}
How can we protect ourselves?
A King with 14 Wives
Its peculiar\underline{ity}: the high volume of light.
Butter mel\underline{ted} every day
Two toddler\underline{s} also jump around.
Mon\underline{th}ly pensions Enough to Life
We must make the transition\underline{.}
Should the judiciary be removed\underline{?}
A great deal of the draft convention is a matter of interpretation\underline{.}
'The Kor\underline{an} is our Constitution\underline{'}
"Her\underline{e} are our points, Havar\underline{d}".
But that was Mexico\underline{.}
I was simply Americans\underline{.}
Want to talk about res\underline{ent}ments\underline{?}
There is more than enough.
Old Battle\underline{s}, New Middle East
Israelis\underline{,} too, should think more long-term.
The pictures do not affect me.
Professor Eastwood agrees\underline{.}
But is it one?
Many questions remain.
Other students shared his opinion.
I was pervert\underline{ed} and dirty\underline{.}
They beat each other, do they?
It was rare\underline{.}
His hum\underline{id} eyes were cloud\underline{y}.
Give it a chance.
And this says a prince\underline{s}s...
The children can have others.
"This is decided," he explained\underline{.}
This is a difficult issue.
He was 81 years old.
The courses were very popular.
This goes further.
Imagine\underline{...}
How to make clean.
Great players have come.
We fully accept that.
How does this network work?
Interior Ministry ignore\underline{s} illegal weapons markets
Where do the weapons come from?
Shopping from the Sofa
46 cent\underline{s} a year?
Who\underline{,} if not me?
The task is difficult.
Nevertheless\underline{,} there is still a risk.
Poland and space.
This concerns the whole of Latin America.
Israel: Labor\underline{atory} of Chaos\underline{.}
I am not a savi\underline{our}\underline{.}
You have no money?
The concept has got off the ground.
Sp\underline{ijk}\underline{en}isse has written literary history.
It costs a lot to tackle this.
We have to watch out hell\underline{ish}ly
World Aid\underline{s} Day\underline{:} Stop\underline{,} sing\underline{,} help
Forty per cent are infected\underline{.}
Who are the main groups affected?
But what does 'pri\underline{n}cip\underline{les}' mean?
'The revolution has returned\underline{'}
This could take rev\underline{en}ge.
I get some bargain\underline{s}.
You chat and laugh\underline{.}
This is based on reciprocity\underline{.}
That will not happen.
Too many wound\underline{ed} feelings\underline{.}
I simply ignore them.
I do not want to lie\underline{.}
My friends were confused\underline{.}
The other students kidnapped\underline{.}
My door was closed.
I never returned\underline{.}
The proportion\underline{s} are perfect.
The "King" of Fashion
Singapore is a city-state\underline{.}
Most are relatives.
They are the same rules.
Condom\underline{s} behind the counter
Dragon Mart is surrounded
'Ba\underline{s}ket\underline{ball} was my life'.
I am proud of that.
What are you doing today?
Larry Hag\underline{man} is Dead
Prevent\underline{ing} the disease
The Hi\underline{gg}\underline{s}-Bo\underline{son} Analysis
No Om\underline{ni}pot\underline{ent} Care
It is like disappointment\underline{.}
Visit unique museums\underline{.}
Tourist list
Don\underline{'}t sh\underline{y}, boss\underline{!}
'As in the luxury shop\underline{'}
Military commentator Viktor Baranez
- How?
Clow\underline{n}s are timeless.
- Good cultural experts\underline{.}
Bir\underline{th} in Space
Earth in danger\underline{.}
Combin\underline{ation} of Genres
Yes\underline{,} that is true.
Help\underline{ing} Self\underline{-}hel\underline{p}
Poly\underline{gam}\underline{y} instead of democracy.
The final station is Lerik\underline{.}
A Direct Man
My Mexican\underline{-}American identity crisis.
That is fair.
I ran away.
I st\underline{umble}\underline{d}.
You are dirty\underline{.}
He seemed disbeliev\underline{ing}.
Fashion show of origin
Too much stress
Key Data from Jalis\underline{co}
AC\underline{TA} is Dead
Foundation of Comp\underline{et}ival
Bay\underline{am} xf3n in the Heart
Want it?'
I enjoy it.
Weight
Nu\underline{tri}\underline{tion}
Stable\underline{r} Field
And after that?
Stars gli\underline{tter}\underline{.}
Number\underline{s}
'Free cash\underline{!}'
Pil\underline{s}en District
District Ol\underline{o}mouc
Not Mexico\underline{.}
And no.
1.2 Children
Unexpec\underline{ted} consequences
General balance sheet
Homex Long term
Vitamin\underline{s}
Impact\underline{s}
Regular\underline{ly}.
Of course.
Dis\underline{s}ati\underline{s}fied
Karl\underline{ov}y Vary
Under\underline{stand}ably\underline{.}
Why?
One-two\underline{-}three-four\underline{.}
Well\underline{.}
Hmmm.
Yes\underline{.}
Privacy
Key Question\underline{s}
Monitoring

